Thrust Microstepping via Acceleration Feedback in Quadrotor Control for Aerial Grasping of Dynamic Payload

In this work, we propose an end-to-end Thrust Microstepping and Decoupled Control (TMDC) of quadrotors. TMDC focuses on precise off-centered aerial grasping of payloads dynamically, which are attached rigidly to the UAV body via a gripper contrary to the swinging payload. The dynamic payload grasping quickly changes UAV's mass, inertia etc, causing instability while performing a grasping operation in-air. We identify that to handle unknown payload grasping, the role of thrust controller is crucial. Hence, we focus on thrust control without involving system parameters such as mass etc. TMDC is based on our novel Thrust Microstepping via Acceleration Feedback (TMAF) thrust controller and Decoupled Motion Control (DMC). TMAF precisely estimates the desired thrust even at smaller loop rates while DMC decouples the horizontal and vertical motion to counteract disturbances in the case of dynamic payloads. We prove the controller's efficacy via exhaustive experiments in practically interesting and adverse real-world cases, such as fully onboard state estimation without any positioning sensor, narrow and indoor flying workspaces with intense wind turbulence, heavy payloads, non-uniform loop rates, etc. Our TMDC outperforms recent direct acceleration feedback thrust controller (DA) and geometric tracking control (GT) in flying stably for aerial grasping and achieves RMSE below 0.04m in contrast to 0.15m of DA and 0.16m of GT.

==> exp_plots/ablations/th_tmaf.tex <==
\addplot[
    fill=white!60!clr4,draw = clr4,opacity=\opacty,
    line width= \linew pt,
    forget plot
    ]
 %%
coordinates {
(0,0)
(0, 42.8529)
(0.00202737, 42.874)
(0.00405474, 43.3493)
(0.00608211, 44.3087)
(0.00810948, 45.1571)
(0.0101368, 45.4616)
(0.0121642, 45.2062)
(0.0141916, 44.4494)
(0.016219, 43.7113)
(0.0182463, 42.8026)
(0.0202737, 42.143)
(0.0223011, 42.1627)
(0.0243284, 42.4557)
(0.0263558, 43.3365)
(0.0283832, 44.3444)
(0.0304105, 45.1208)
(0.0324379, 45.7988)
(0.0344653, 46.0964)
(0.0364927, 45.9286)
(0.03852, 45.4368)
(0.0405474, 44.7849)
(0.0425748, 44.3042)
(0.0446021, 44.1087)
(0.0466295, 43.9339)
(0.0486569, 43.2668)
(0.0506842, 42.9405)
(0.0527116, 42.913)
(0.054739, 43.4107)
(0.0567663, 43.9783)
(0.0587937, 44.9973)
(0.0608211, 45.766)
(0.0628485, 46.1436)
(0.0648758, 46.4101)
(0.0669032, 46.0421)
(0.0689306, 45.3205)
(0.0709579, 43.8119)
(0.0729853, 43.0038)
(0.0750127, 42.6237)
(0.07704, 42.7843)
(0.0790674, 43.6338)
(0.0810948, 44.2799)
(0.0831221, 44.8816)
(0.0851495, 45.3719)
(0.0871769, 45.601)
(0.0892043, 45.7236)
(0.0912316, 45.543)
(0.093259, 45.1559)
(0.0952864, 44.5829)
(0.0973137, 44.4686)
(0.0993411, 44.5305)
(0.101368, 44.9695)
(0.103396, 44.8546)
(0.105423, 44.6039)
(0.107451, 44.3339)
(0.109478, 44.3439)
(0.111505, 45.0457)
(0.113533, 45.7646)
(0.11556, 46.1522)
(0.117587, 46.1698)
(0.119615, 46.0527)
(0.121642, 45.6295)
(0.12367, 45.3018)
(0.125697, 44.9722)
(0.127724, 44.9336)
(0.129752, 49.9394)
(0.131779, 60.2111)
(0.133806, 63.2924)
(0.135834, 61.4151)
(0.137861, 56.3174)
(0.139888, 48.919)
(0.141916, 43.2396)
(0.143943, 37.5092)
(0.145971, 35.8512)
(0.147998, 37.4319)
(0.150025, 41.1802)
(0.152053, 45.8073)
(0.15408, 50.2228)
(0.156107, 51.7207)
(0.158135, 51.5524)
(0.160162, 49.7639)
(0.16219, 46.7125)
(0.164217, 43.5428)
(0.166244, 41.3862)
(0.168272, 39.7571)
(0.170299, 39.5461)
(0.172326, 40.3193)
(0.174354, 41.6438)
(0.176381, 43.7455)
(0.178409, 45.392)
(0.180436, 47.1982)
(0.182463, 48.1598)
(0.184491, 48.2826)
(0.186518, 46.9686)
(0.188545, 45.2342)
(0.190573, 43.6189)
(0.1926, 42.5916)
(0.194627, 41.5423)
(0.196655, 42.7455)
(0.198682, 54.0424)
(0.20071, 70.8312)
(0.202737, 75.2483)
(0.204764, 73.9026)
(0.206792, 64.8306)
(0.208819, 53.4603)
(0.210846, 42.7635)
(0.212874, 35.0246)
(0.214901, 31.629)
(0.216929, 31.8727)
(0.218956, 36.3008)
(0.220983, 43.3948)
(0.223011, 48.9601)
(0.225038, 53.0914)
(0.227065, 53.9906)
(0.229093, 52.5634)
(0.23112, 49.694)
(0.233147, 45.597)
(0.235175, 41.8997)
(0.237202, 39.8555)
(0.23923, 39.4845)
(0.241257, 40.7214)
(0.243284, 42.3097)
(0.245312, 45.1872)
(0.247339, 47.3458)
(0.249366, 48.329)
(0.251394, 47.8477)
(0.253421, 46.0377)
(0.255449, 44.45)
(0.257476, 42.5545)
(0.259503, 41.4833)
(0.261531, 41.5483)
(0.263558, 42.4531)
(0.265585, 43.9997)
(0.267613, 45.6293)
(0.26964, 46.6619)
(0.271668, 47.1702)
(0.273695, 46.9095)
(0.275722, 45.8833)
(0.27775, 44.7427)
(0.279777, 51.7408)
(0.281804, 59.9131)
(0.283832, 61.825)
(0.285859, 59.2831)
(0.287886, 53.5799)
(0.289914, 46.7423)
(0.291941, 39.6554)
(0.293969, 35.6425)
(0.295996, 34.059)
(0.298023, 35.6982)
(0.300051, 39.8483)
(0.302078, 45.7389)
(0.304105, 50.9733)
(0.306133, 52.7472)
(0.30816, 52.7965)
(0.310188, 50.5402)
(0.312215, 46.6897)
(0.314242, 42.3976)
(0.31627, 38.5309)
(0.318297, 37.0701)
(0.320324, 37.5208)
(0.322352, 39.956)
(0.324379, 43.3671)
(0.326407, 46.6394)
(0.328434, 48.3845)
(0.330461, 48.9054)
(0.332489, 48.0479)
(0.334516, 46.4672)
(0.336543, 44.1916)
(0.338571, 42.2033)
(0.340598, 41.0191)
(0.342625, 41.1077)
(0.344653, 42.5321)
(0.34668, 44.552)
(0.348708, 46.3678)
(0.350735, 48.0596)
(0.352762, 48.9831)
(0.35479, 48.7469)
(0.356817, 47.5905)
(0.358844, 45.8217)
(0.360872, 43.9389)
(0.362899, 42.0172)
(0.364927, 40.6925)
(0.366954, 40.878)
(0.368981, 41.7787)
(0.371009, 44.9677)
(0.373036, 58.0406)
(0.375063, 65.3829)
(0.377091, 65.5267)
(0.379118, 62.6693)
(0.381145, 57.3187)
(0.383173, 51.8903)
(0.3852, 45.75)
(0.387228, 39.7655)
(0.389255, 35.8349)
(0.391282, 34.8429)
(0.39331, 37.1926)
(0.395337, 40.1981)
(0.397364, 43.5179)
(0.399392, 46.2697)
(0.401419, 47.6711)
(0.403447, 46.9811)
(0.405474, 45.9508)
(0.407501, 44.081)
(0.409529, 42.3093)
(0.411556, 40.8428)
(0.413583, 40.3001)
(0.415611, 41.235)
(0.417638, 42.4615)
(0.419666, 44.5173)
(0.421693, 46.2435)
(0.42372, 46.8847)
(0.425748, 46.5286)
(0.427775, 45.0521)
(0.429802, 43.5618)
(0.43183, 42.6129)
(0.433857, 41.7532)
(0.435884, 41.8659)
(0.437912, 42.7042)
(0.439939, 43.8332)
(0.441967, 44.6079)
(0.443994, 45.6559)
(0.446021, 45.0717)
(0.448049, 44.2917)
(0.450076, 43.8012)
(0.452103, 43.6575)
(0.454131, 43.482)
(0.456158, 43.4207)
(0.458185, 43.8915)
(0.460213, 44.9341)
(0.46224, 45.7491)
(0.464268, 46.102)
(0.466295, 46.1734)
(0.468322, 45.8418)
(0.47035, 45.1389)
(0.472377, 44.2306)
(0.474404, 43.6532)
(0.476432, 43.9542)
(0.478459, 44.8055)
(0.480487, 45.388)
(0.482514, 46.3025)
(0.484541, 47.5247)
(0.486569, 48.284)
(0.488596, 52.5819)
(0.490623, 66.3218)
(0.492651, 70.8469)
(0.494678, 65.2855)
(0.496706, 58.4736)
(0.498733, 49.4486)
(0.50076, 40.8227)
(0.502788, 35.8415)
(0.504815, 35.785)
(0.506842, 39.3939)
(0.50887, 43.9918)
(0.510897, 48.47)
(0.512924, 51.1024)
(0.514952, 51.3743)
(0.516979, 50.0104)
(0.519007, 47.0469)
(0.521034, 43.9013)
(0.523061, 39.4269)
(0.525089, 37.0271)
(0.527116, 36.7658)
(0.529143, 37.4321)
(0.531171, 40.3432)
(0.533198, 43.6969)
(0.535226, 47.0477)
(0.537253, 49.3316)
(0.53928, 50.0393)
(0.541308, 49.1153)
(0.543335, 47.3476)
(0.545362, 44.3783)
(0.54739, 40.9252)
(0.549417, 39.4797)
(0.551444, 39.7387)
(0.553472, 40.7731)
(0.555499, 42.6392)
(0.557527, 44.4476)
(0.559554, 46.3884)
(0.561581, 47.3738)
(0.563609, 47.7357)
(0.565636, 47.4294)
(0.567663, 46.4706)
(0.569691, 45.9892)
(0.571718, 45.8258)
(0.573746, 45.4769)
(0.575773, 44.8695)
(0.5778, 43.5469)
(0.579828, 42.9151)
(0.581855, 42.9629)
(0.583882, 43.6057)
(0.58591, 44.5506)
(0.587937, 45.4805)
(0.589965, 46.0889)
(0.591992, 46.3703)
(0.594019, 46.0161)
(0.596047, 45.5233)
(0.598074, 44.6485)
(0.600101, 43.8256)
(0.602129, 43.3946)
(0.604156, 43.076)
(0.606184, 43.0193)
(0.608211, 42.9962)
(0.610238, 43.4588)
(0.612266, 43.9009)
(0.614293, 44.3438)
(0.61632, 44.266)
(0.618348, 43.8964)
(0.620375, 43.1445)
(0.622402, 42.5741)
(0.62443, 42.6554)
(0.626457, 43.0445)
(0.628485, 43.4932)
(0.630512, 43.9654)
(0.632539, 44.4986)
(0.634567, 44.9989)
(0.636594, 45.1409)
(0.638621, 45.2501)
(0.640649, 44.9669)
(0.642676, 44.5457)
(0.644704, 44.3025)
(0.646731, 43.9714)
(0.648758, 43.8717)
(0.650786, 43.9239)
(0.652813, 44.3696)
(0.65484, 44.9139)
(0.656868, 45.4464)
(0.658895, 45.8104)
(0.660922, 45.7396)
(0.66295, 45.1662)
(0.664977, 44.1836)
(0.667005, 43.3939)
(0.669032, 43.2151)
(0.671059, 43.0714)
(0.673087, 43.3447)
(0.675114, 43.7549)
(0.677141, 44.5149)
(0.679169, 45.494)
(0.681196, 46.2401)
(0.683224, 46.8954)
(0.685251, 47.9496)
(0.687278, 47.9354)
(0.689306, 47.4747)
(0.691333, 46.5108)
(0.69336, 45.1846)
(0.695388, 43.8534)
(0.697415, 43.3043)
(0.699443, 43.2974)
(0.70147, 44.2621)
(0.703497, 45.1674)
(0.705525, 45.9084)
(0.707552, 46.3873)
(0.709579, 47.1385)
(0.711607, 47.2289)
(0.713634, 47.2207)
(0.715661, 46.9103)
(0.717689, 46.742)
(0.719716, 46.3877)
(0.721744, 45.5953)
(0.723771, 44.2658)
(0.725798, 43.7674)
(0.727826, 43.9973)
(0.729853, 44.5307)
(0.73188, 45.7943)
(0.733908, 46.8926)
(0.735935, 47.3375)
(0.737962, 47.3215)
(0.73999, 46.8187)
(0.742017, 46.0385)
(0.744045, 44.9038)
(0.746072, 44.2607)
(0.748099, 43.6991)
(0.750127, 43.3981)
(0.752154, 43.3756)
(0.754181, 43.2674)
(0.756209, 43.246)
(0.758236, 43.5003)
(0.760264, 44.1895)
(0.762291, 44.4971)
(0.764318, 44.6406)
(0.766346, 44.6507)
(0.768373, 44.7312)
(0.7704, 44.8379)
(0.772428, 45.4163)
(0.774455, 45.3908)
(0.776483, 45.0894)
(0.77851, 44.4051)
(0.780537, 43.5061)
(0.782565, 42.8657)
(0.784592, 42.3026)
(0.786619, 42.1276)
(0.788647, 42.3872)
(0.790674, 43.1717)
(0.792701, 43.9212)
(0.794729, 44.3953)
(0.796756, 44.5083)
(0.798784, 44.468)
(0.800811, 43.9949)
(0.802838, 43.7455)
(0.804866, 43.3299)
(0.806893, 42.8275)
(0.80892, 42.6614)
(0.810948, 42.6286)
(0.812975, 42.9553)
(0.815003, 43.0287)
(0.81703, 43.1803)
(0.819057, 43.447)
(0.821085, 43.5979)
(0.823112, 43.7705)
(0.825139, 43.916)
(0.827167, 43.9892)
(0.829194, 43.936)
(0.831222, 44.0978)
(0.833249, 44.033)
(0.835276, 43.9964)
(0.837304, 43.873)
(0.839331, 43.7631)
(0.841358, 43.7855)
(0.843386, 44.0824)
(0.845413, 44.4853)
(0.84744, 44.8221)
(0.849468, 45.1486)
(0.851495, 45.6751)
(0.853523, 45.9639)
(0.85555, 46.0511)
(0.857577, 45.3984)
(0.859605, 44.916)
(0.861632, 44.3635)
(0.863659, 43.996)
(0.865687, 43.7888)
(0.867714, 44.0958)
(0.869741, 44.5981)
(0.871769, 45.2786)
(0.873796, 45.5104)
(0.875824, 45.5053)
(0.877851, 45.3227)
(0.879878, 44.034)
(0.881906, 43.208)
(0.883933, 42.4315)
(0.885961, 42.3606)
(0.887988, 42.5323)
(0.890015, 43.0959)
(0.892043, 43.1676)
(0.89407, 43.0699)
(0.896097, 43.2848)
(0.898125, 43.7578)
(0.900152, 43.9855)
(0.902179, 44.5921)
(0.904207, 45.2591)
(0.906234, 45.7021)
(0.908262, 46.323)
(0.910289, 46.4844)
(0.912316, 46.6369)
(0.914344, 46.5327)
(0.916371, 46.2089)
(0.918398, 45.8914)
(0.920426, 45.5075)
(0.922453, 45.0235)
(0.92448, 44.4174)
(0.926508, 44.2845)
(0.928535, 44.4314)
(0.930563, 44.3439)
(0.93259, 44.5652)
(0.934617, 44.8401)
(0.936645, 45.9093)
(0.938672, 55.6595)
(0.940699, 66.8652)
(0.942727, 69.9289)
(0.944754, 66.5296)
(0.946782, 59.0098)
(0.948809, 49.8256)
(0.950836, 40.944)
(0.952864, 34.446)
(0.954891, 30.9601)
(0.956918, 31.3145)
(0.958946, 35.617)
(0.960973, 41.992)
(0.963001, 48.4926)
(0.965028, 53.3094)
(0.967055, 55.6943)
(0.969083, 54.6929)
(0.97111, 51.8929)
(0.973137, 47.5991)
(0.975165, 43.2205)
(0.977192, 39.9954)
(0.979219, 38.8621)
(0.981247, 38.9054)
(0.983274, 39.186)
(0.985302, 40.7918)
(0.987329, 43.3139)
(0.989356, 45.2519)
(0.991384, 46.8848)
(0.993411, 47.2914)
(0.995438, 46.7733)
(0.997466, 45.6007)
(0.999493, 44.1618)
(1,0)
};

==> exp_plots/ablations/th_tmaf_1_no_fill.tex <==
\addplot[
    fill=none,draw = clr4,opacity=1.0,
    line width= \linew pt
    ]
 %%
coordinates {
(0, 0)
(0, 42.8529)
(0.00202737, 42.874)
(0.00405474, 43.3493)
(0.00608211, 44.3087)
(0.00810948, 45.1571)
(0.0101368, 45.4616)
(0.0121642, 45.2062)
(0.0141916, 44.4494)
(0.016219, 43.7113)
(0.0182463, 42.8026)
(0.0202737, 42.143)
(0.0223011, 42.1627)
(0.0243284, 42.4557)
(0.0263558, 43.3365)
(0.0283832, 44.3444)
(0.0304105, 45.1208)
(0.0324379, 45.7988)
(0.0344653, 46.0964)
(0.0364927, 45.9286)
(0.03852, 45.4368)
(0.0405474, 44.7849)
(0.0425748, 44.3042)
(0.0446021, 44.1087)
(0.0466295, 43.9339)
(0.0486569, 43.2668)
(0.0506842, 42.9405)
(0.0527116, 42.913)
(0.054739, 43.4107)
(0.0567663, 43.9783)
(0.0587937, 44.9973)
(0.0608211, 45.766)
(0.0628485, 46.1436)
(0.0648758, 46.4101)
(0.0669032, 46.0421)
(0.0689306, 45.3205)
(0.0709579, 43.8119)
(0.0729853, 43.0038)
(0.0750127, 42.6237)
(0.07704, 42.7843)
(0.0790674, 43.6338)
(0.0810948, 44.2799)
(0.0831221, 44.8816)
(0.0851495, 45.3719)
(0.0871769, 45.601)
(0.0892043, 45.7236)
(0.0912316, 45.543)
(0.093259, 45.1559)
(0.0952864, 44.5829)
(0.0973137, 44.4686)
(0.0993411, 44.5305)
(0.101368, 44.9695)
(0.103396, 44.8546)
(0.105423, 44.6039)
(0.107451, 44.3339)
(0.109478, 44.3439)
(0.111505, 45.0457)
(0.113533, 45.7646)
(0.11556, 46.1522)
(0.117587, 46.1698)
(0.119615, 46.0527)
(0.121642, 45.6295)
(0.12367, 45.3018)
(0.125697, 44.9722)
(0.127724, 44.9336)
(0.129752, 49.9394)
(0.131779, 60.2111)
(0.133806, 63.2924)
(0.135834, 61.4151)
(0.137861, 56.3174)
(0.139888, 48.919)
(0.141916, 43.2396)
(0.143943, 37.5092)
(0.145971, 35.8512)
(0.147998, 37.4319)
(0.150025, 41.1802)
(0.152053, 45.8073)
(0.15408, 50.2228)
(0.156107, 51.7207)
(0.158135, 51.5524)
(0.160162, 49.7639)
(0.16219, 46.7125)
(0.164217, 43.5428)
(0.166244, 41.3862)
(0.168272, 39.7571)
(0.170299, 39.5461)
(0.172326, 40.3193)
(0.174354, 41.6438)
(0.176381, 43.7455)
(0.178409, 45.392)
(0.180436, 47.1982)
(0.182463, 48.1598)
(0.184491, 48.2826)
(0.186518, 46.9686)
(0.188545, 45.2342)
(0.190573, 43.6189)
(0.1926, 42.5916)
(0.194627, 41.5423)
(0.196655, 42.7455)
(0.198682, 54.0424)
(0.20071, 70.8312)
(0.202737, 75.2483)
(0.204764, 73.9026)
(0.206792, 64.8306)
(0.208819, 53.4603)
(0.210846, 42.7635)
(0.212874, 35.0246)
(0.214901, 31.629)
(0.216929, 31.8727)
(0.218956, 36.3008)
(0.220983, 43.3948)
(0.223011, 48.9601)
(0.225038, 53.0914)
(0.227065, 53.9906)
(0.229093, 52.5634)
(0.23112, 49.694)
(0.233147, 45.597)
(0.235175, 41.8997)
(0.237202, 39.8555)
(0.23923, 39.4845)
(0.241257, 40.7214)
(0.243284, 42.3097)
(0.245312, 45.1872)
(0.247339, 47.3458)
(0.249366, 48.329)
(0.251394, 47.8477)
(0.253421, 46.0377)
(0.255449, 44.45)
(0.257476, 42.5545)
(0.259503, 41.4833)
(0.261531, 41.5483)
(0.263558, 42.4531)
(0.265585, 43.9997)
(0.267613, 45.6293)
(0.26964, 46.6619)
(0.271668, 47.1702)
(0.273695, 46.9095)
(0.275722, 45.8833)
(0.27775, 44.7427)
(0.279777, 51.7408)
(0.281804, 59.9131)
(0.283832, 61.825)
(0.285859, 59.2831)
(0.287886, 53.5799)
(0.289914, 46.7423)
(0.291941, 39.6554)
(0.293969, 35.6425)
(0.295996, 34.059)
(0.298023, 35.6982)
(0.300051, 39.8483)
(0.302078, 45.7389)
(0.304105, 50.9733)
(0.306133, 52.7472)
(0.30816, 52.7965)
(0.310188, 50.5402)
(0.312215, 46.6897)
(0.314242, 42.3976)
(0.31627, 38.5309)
(0.318297, 37.0701)
(0.320324, 37.5208)
(0.322352, 39.956)
(0.324379, 43.3671)
(0.326407, 46.6394)
(0.328434, 48.3845)
(0.330461, 48.9054)
(0.332489, 48.0479)
(0.334516, 46.4672)
(0.336543, 44.1916)
(0.338571, 42.2033)
(0.340598, 41.0191)
(0.342625, 41.1077)
(0.344653, 42.5321)
(0.34668, 44.552)
(0.348708, 46.3678)
(0.350735, 48.0596)
(0.352762, 48.9831)
(0.35479, 48.7469)
(0.356817, 47.5905)
(0.358844, 45.8217)
(0.360872, 43.9389)
(0.362899, 42.0172)
(0.364927, 40.6925)
(0.366954, 40.878)
(0.368981, 41.7787)
(0.371009, 44.9677)
(0.373036, 58.0406)
(0.375063, 65.3829)
(0.377091, 65.5267)
(0.379118, 62.6693)
(0.381145, 57.3187)
(0.383173, 51.8903)
(0.3852, 45.75)
(0.387228, 39.7655)
(0.389255, 35.8349)
(0.391282, 34.8429)
(0.39331, 37.1926)
(0.395337, 40.1981)
(0.397364, 43.5179)
(0.399392, 46.2697)
(0.401419, 47.6711)
(0.403447, 46.9811)
(0.405474, 45.9508)
(0.407501, 44.081)
(0.409529, 42.3093)
(0.411556, 40.8428)
(0.413583, 40.3001)
(0.415611, 41.235)
(0.417638, 42.4615)
(0.419666, 44.5173)
(0.421693, 46.2435)
(0.42372, 46.8847)
(0.425748, 46.5286)
(0.427775, 45.0521)
(0.429802, 43.5618)
(0.43183, 42.6129)
(0.433857, 41.7532)
(0.435884, 41.8659)
(0.437912, 42.7042)
(0.439939, 43.8332)
(0.441967, 44.6079)
(0.443994, 45.6559)
(0.446021, 45.0717)
(0.448049, 44.2917)
(0.450076, 43.8012)
(0.452103, 43.6575)
(0.454131, 43.482)
(0.456158, 43.4207)
(0.458185, 43.8915)
(0.460213, 44.9341)
(0.46224, 45.7491)
(0.464268, 46.102)
(0.466295, 46.1734)
(0.468322, 45.8418)
(0.47035, 45.1389)
(0.472377, 44.2306)
(0.474404, 43.6532)
(0.476432, 43.9542)
(0.478459, 44.8055)
(0.480487, 45.388)
(0.482514, 46.3025)
(0.484541, 47.5247)
(0.486569, 48.284)
(0.488596, 52.5819)
(0.490623, 66.3218)
(0.492651, 70.8469)
(0.494678, 65.2855)
(0.496706, 58.4736)
(0.498733, 49.4486)
(0.50076, 40.8227)
(0.502788, 35.8415)
(0.504815, 35.785)
(0.506842, 39.3939)
(0.50887, 43.9918)
(0.510897, 48.47)
(0.512924, 51.1024)
(0.514952, 51.3743)
(0.516979, 50.0104)
(0.519007, 47.0469)
(0.521034, 43.9013)
(0.523061, 39.4269)
(0.525089, 37.0271)
(0.527116, 36.7658)
(0.529143, 37.4321)
(0.531171, 40.3432)
(0.533198, 43.6969)
(0.535226, 47.0477)
(0.537253, 49.3316)
(0.53928, 50.0393)
(0.541308, 49.1153)
(0.543335, 47.3476)
(0.545362, 44.3783)
(0.54739, 40.9252)
(0.549417, 39.4797)
(0.551444, 39.7387)
(0.553472, 40.7731)
(0.555499, 42.6392)
(0.557527, 44.4476)
(0.559554, 46.3884)
(0.561581, 47.3738)
(0.563609, 47.7357)
(0.565636, 47.4294)
(0.567663, 46.4706)
(0.569691, 45.9892)
(0.571718, 45.8258)
(0.573746, 45.4769)
(0.575773, 44.8695)
(0.5778, 43.5469)
(0.579828, 42.9151)
(0.581855, 42.9629)
(0.583882, 43.6057)
(0.58591, 44.5506)
(0.587937, 45.4805)
(0.589965, 46.0889)
(0.591992, 46.3703)
(0.594019, 46.0161)
(0.596047, 45.5233)
(0.598074, 44.6485)
(0.600101, 43.8256)
(0.602129, 43.3946)
(0.604156, 43.076)
(0.606184, 43.0193)
(0.608211, 42.9962)
(0.610238, 43.4588)
(0.612266, 43.9009)
(0.614293, 44.3438)
(0.61632, 44.266)
(0.618348, 43.8964)
(0.620375, 43.1445)
(0.622402, 42.5741)
(0.62443, 42.6554)
(0.626457, 43.0445)
(0.628485, 43.4932)
(0.630512, 43.9654)
(0.632539, 44.4986)
(0.634567, 44.9989)
(0.636594, 45.1409)
(0.638621, 45.2501)
(0.640649, 44.9669)
(0.642676, 44.5457)
(0.644704, 44.3025)
(0.646731, 43.9714)
(0.648758, 43.8717)
(0.650786, 43.9239)
(0.652813, 44.3696)
(0.65484, 44.9139)
(0.656868, 45.4464)
(0.658895, 45.8104)
(0.660922, 45.7396)
(0.66295, 45.1662)
(0.664977, 44.1836)
(0.667005, 43.3939)
(0.669032, 43.2151)
(0.671059, 43.0714)
(0.673087, 43.3447)
(0.675114, 43.7549)
(0.677141, 44.5149)
(0.679169, 45.494)
(0.681196, 46.2401)
(0.683224, 46.8954)
(0.685251, 47.9496)
(0.687278, 47.9354)
(0.689306, 47.4747)
(0.691333, 46.5108)
(0.69336, 45.1846)
(0.695388, 43.8534)
(0.697415, 43.3043)
(0.699443, 43.2974)
(0.70147, 44.2621)
(0.703497, 45.1674)
(0.705525, 45.9084)
(0.707552, 46.3873)
(0.709579, 47.1385)
(0.711607, 47.2289)
(0.713634, 47.2207)
(0.715661, 46.9103)
(0.717689, 46.742)
(0.719716, 46.3877)
(0.721744, 45.5953)
(0.723771, 44.2658)
(0.725798, 43.7674)
(0.727826, 43.9973)
(0.729853, 44.5307)
(0.73188, 45.7943)
(0.733908, 46.8926)
(0.735935, 47.3375)
(0.737962, 47.3215)
(0.73999, 46.8187)
(0.742017, 46.0385)
(0.744045, 44.9038)
(0.746072, 44.2607)
(0.748099, 43.6991)
(0.750127, 43.3981)
(0.752154, 43.3756)
(0.754181, 43.2674)
(0.756209, 43.246)
(0.758236, 43.5003)
(0.760264, 44.1895)
(0.762291, 44.4971)
(0.764318, 44.6406)
(0.766346, 44.6507)
(0.768373, 44.7312)
(0.7704, 44.8379)
(0.772428, 45.4163)
(0.774455, 45.3908)
(0.776483, 45.0894)
(0.77851, 44.4051)
(0.780537, 43.5061)
(0.782565, 42.8657)
(0.784592, 42.3026)
(0.786619, 42.1276)
(0.788647, 42.3872)
(0.790674, 43.1717)
(0.792701, 43.9212)
(0.794729, 44.3953)
(0.796756, 44.5083)
(0.798784, 44.468)
(0.800811, 43.9949)
(0.802838, 43.7455)
(0.804866, 43.3299)
(0.806893, 42.8275)
(0.80892, 42.6614)
(0.810948, 42.6286)
(0.812975, 42.9553)
(0.815003, 43.0287)
(0.81703, 43.1803)
(0.819057, 43.447)
(0.821085, 43.5979)
(0.823112, 43.7705)
(0.825139, 43.916)
(0.827167, 43.9892)
(0.829194, 43.936)
(0.831222, 44.0978)
(0.833249, 44.033)
(0.835276, 43.9964)
(0.837304, 43.873)
(0.839331, 43.7631)
(0.841358, 43.7855)
(0.843386, 44.0824)
(0.845413, 44.4853)
(0.84744, 44.8221)
(0.849468, 45.1486)
(0.851495, 45.6751)
(0.853523, 45.9639)
(0.85555, 46.0511)
(0.857577, 45.3984)
(0.859605, 44.916)
(0.861632, 44.3635)
(0.863659, 43.996)
(0.865687, 43.7888)
(0.867714, 44.0958)
(0.869741, 44.5981)
(0.871769, 45.2786)
(0.873796, 45.5104)
(0.875824, 45.5053)
(0.877851, 45.3227)
(0.879878, 44.034)
(0.881906, 43.208)
(0.883933, 42.4315)
(0.885961, 42.3606)
(0.887988, 42.5323)
(0.890015, 43.0959)
(0.892043, 43.1676)
(0.89407, 43.0699)
(0.896097, 43.2848)
(0.898125, 43.7578)
(0.900152, 43.9855)
(0.902179, 44.5921)
(0.904207, 45.2591)
(0.906234, 45.7021)
(0.908262, 46.323)
(0.910289, 46.4844)
(0.912316, 46.6369)
(0.914344, 46.5327)
(0.916371, 46.2089)
(0.918398, 45.8914)
(0.920426, 45.5075)
(0.922453, 45.0235)
(0.92448, 44.4174)
(0.926508, 44.2845)
(0.928535, 44.4314)
(0.930563, 44.3439)
(0.93259, 44.5652)
(0.934617, 44.8401)
(0.936645, 45.9093)
(0.938672, 55.6595)
(0.940699, 66.8652)
(0.942727, 69.9289)
(0.944754, 66.5296)
(0.946782, 59.0098)
(0.948809, 49.8256)
(0.950836, 40.944)
(0.952864, 34.446)
(0.954891, 30.9601)
(0.956918, 31.3145)
(0.958946, 35.617)
(0.960973, 41.992)
(0.963001, 48.4926)
(0.965028, 53.3094)
(0.967055, 55.6943)
(0.969083, 54.6929)
(0.97111, 51.8929)
(0.973137, 47.5991)
(0.975165, 43.2205)
(0.977192, 39.9954)
(0.979219, 38.8621)
(0.981247, 38.9054)
(0.983274, 39.186)
(0.985302, 40.7918)
(0.987329, 43.3139)
(0.989356, 45.2519)
(0.991384, 46.8848)
(0.993411, 47.2914)
(0.995438, 46.7733)
(0.997466, 45.6007)
(0.999493, 44.1618)
(1,0)
};

==> exp_plots/circle_traj__battery_combined/des_traj.tex <==
\addplot3[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates{
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0, 0, 0.5)
(0.035, 0, 0.5)
(0.06125, 0, 0.5)
(0.09625, 0, 0.5)
(0.1225, 0, 0.5)
(0.1575, 0, 0.5)
(0.18375, 0, 0.5)
(0.21875, 0, 0.5)
(0.245, 0, 0.5)
(0.28, 0, 0.5)
(0.30625, 0, 0.5)
(0.34125, 0, 0.5)
(0.3675, 0, 0.5)
(0.4025, 0, 0.5)
(0.42875, 0, 0.5)
(0.46375, 0, 0.5)
(0.49, 0, 0.5)
(0.525, 0, 0.5)
(0.56, 0, 0.5)
(0.58625, 0, 0.5)
(0.62125, 0, 0.5)
(0.6475, 0, 0.5)
(0.67375, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.69125, 0, 0.5)
(0.698786, 0.0412096, 0.5)
(0.695148, 0.0822762, 0.5)
(0.68655, 0.136563, 0.5)
(0.677319, 0.176744, 0.5)
(0.661364, 0.229341, 0.5)
(0.646716, 0.267878, 0.5)
(0.623705, 0.317793, 0.5)
(0.603914, 0.35396, 0.5)
(0.574281, 0.400252, 0.5)
(0.549722, 0.433366, 0.5)
(0.514026, 0.475161, 0.5)
(0.485161, 0.504597, 0.5)
(0.444075, 0.541107, 0.5)
(0.41145, 0.566312, 0.5)
(0.365749, 0.596848, 0.5)
(0.329978, 0.617345, 0.5)
(0.280524, 0.641332, 0.5)
(0.242282, 0.656734, 0.5)
(0.190008, 0.673719, 0.5)
(0.136563, 0.68655, 0.5)
(0.0822762, 0.695148, 0.5)
(0.0412095, 0.698786, 0.5)
(-0.0137436, 0.699865, 0.5)
(-0.0549213, 0.697842, 0.5)
(-0.109504, 0.691382, 0.5)
(-0.150016, 0.683736, 0.5)
(-0.203199, 0.669858, 0.5)
(-0.242282, 0.656734, 0.5)
(-0.293062, 0.6357, 0.5)
(-0.342035, 0.610747, 0.5)
(-0.377397, 0.589552, 0.5)
(-0.422489, 0.558124, 0.5)
(-0.454614, 0.532284, 0.5)
(-0.494975, 0.494975, 0.5)
(-0.523256, 0.464977, 0.5)
(-0.549722, 0.433366, 0.5)
(-0.582029, 0.388899, 0.5)
(-0.603914, 0.35396, 0.5)
(-0.629824, 0.305487, 0.5)
(-0.65185, 0.255129, 0.5)
(-0.66574, 0.216312, 0.5)
(-0.680659, 0.163412, 0.5)
(-0.689099, 0.123057, 0.5)
(-0.696629, 0.068612, 0.5)
(-0.69946, 0.0274818, 0.5)
(-0.69946, -0.0274819, 0.5)
(-0.696629, -0.0686119, 0.5)
(-0.689099, -0.123057, 0.5)
(-0.680659, -0.163412, 0.5)
(-0.669858, -0.203199, 0.5)
(-0.65185, -0.255129, 0.5)
(-0.629824, -0.305486, 0.5)
(-0.610747, -0.342035, 0.5)
(-0.582029, -0.388899, 0.5)
(-0.558124, -0.422489, 0.5)
(-0.523256, -0.464977, 0.5)
(-0.494975, -0.494975, 0.5)
(-0.454614, -0.532284, 0.5)
(-0.422489, -0.558124, 0.5)
(-0.377397, -0.589552, 0.5)
(-0.342035, -0.610747, 0.5)
(-0.293062, -0.6357, 0.5)
(-0.242282, -0.656734, 0.5)
(-0.203199, -0.669858, 0.5)
(-0.150016, -0.683736, 0.5)
(-0.109504, -0.691382, 0.5)
(-0.0549214, -0.697842, 0.5)
(-0.0137437, -0.699865, 0.5)
(0.0412094, -0.698786, 0.5)
(0.0822762, -0.695148, 0.5)
(0.136563, -0.68655, 0.5)
(0.176744, -0.677319, 0.5)
(0.229341, -0.661364, 0.5)
(0.267879, -0.646716, 0.5)
(0.317793, -0.623704, 0.5)
(0.365749, -0.596848, 0.5)
(0.41145, -0.566312, 0.5)
(0.444075, -0.541107, 0.5)
(0.485161, -0.504597, 0.5)
(0.514026, -0.475161, 0.5)
(0.549722, -0.433366, 0.5)
(0.574281, -0.400251, 0.5)
(0.603914, -0.35396, 0.5)
(0.623705, -0.317793, 0.5)
(0.646716, -0.267878, 0.5)
(0.661364, -0.229341, 0.5)
(0.677319, -0.176744, 0.5)
(0.68655, -0.136563, 0.5)
(0.695148, -0.0822761, 0.5)
(0.698786, -0.0412096, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0.699865, -0.0137436, 0.5)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
(0, 0, 0)
};


==> exp_plots/circle_traj__battery_combined/executed_traj.tex <==
\addplot3[
    fill=none,draw = currclr,
    line width= \linew pt,
    ]
coordinates{
(0, 0, 0)
(0.000225173, -0.000680207, -0.00047671)
(0.000992686, -0.00124644, -0.000801834)
(0.00139729, -0.00188739, -0.00124664)
(0.00169712, -0.00250819, -0.00173096)
(0.00187755, -0.00310809, -0.00217679)
(0.00204896, -0.00362289, -0.00257835)
(0.00252778, -0.00418184, -0.00280389)
(0.00292652, -0.00517583, -0.0029648)
(0.00317233, -0.00654218, -0.00326375)
(0.00311288, -0.00748293, -0.00341146)
(0.00288928, -0.00766392, -0.00308097)
(0.00207986, -0.00824461, -0.00294752)
(0.00189187, -0.00876934, -0.00281819)
(0.00134598, -0.00910946, -0.00230029)
(0.00161949, -0.00964368, -0.00164266)
(0.00273117, -0.0106637, 0.00015738)
(0.00320743, -0.0118347, 0.00299832)
(0.00102492, -0.0132043, 0.00678307)
(-0.00567202, -0.0174091, 0.0127885)
(-0.0184304, -0.0250047, 0.0214453)
(-0.0337412, -0.0365586, 0.0378601)
(-0.0476533, -0.0519272, 0.0585692)
(-0.0582865, -0.0697991, 0.0845493)
(-0.0669481, -0.0885745, 0.113654)
(-0.0691571, -0.108574, 0.141566)
(-0.0667346, -0.125911, 0.171486)
(-0.0617554, -0.141516, 0.20205)
(-0.0527366, -0.153452, 0.231361)
(-0.039684, -0.159334, 0.260946)
(-0.0234124, -0.159134, 0.289052)
(-0.00728579, -0.154821, 0.314547)
(0.0057014, -0.147084, 0.337877)
(0.0134535, -0.136464, 0.362736)
(0.0161419, -0.123178, 0.388069)
(0.0161479, -0.108737, 0.413742)
(0.0138531, -0.0922282, 0.435603)
(0.0103267, -0.0750075, 0.453314)
(0.00530259, -0.0585755, 0.468073)
(-0.000210634, -0.0453907, 0.480348)
(-0.00438461, -0.0356831, 0.490493)
(-0.00658255, -0.0297127, 0.498815)
(-0.00637375, -0.0266939, 0.504687)
(-0.00510553, -0.0261443, 0.508187)
(-0.00311082, -0.0273879, 0.5126)
(-0.00113438, -0.0297599, 0.517261)
(-0.00138338, -0.03327, 0.518268)
(-0.00241299, -0.0394879, 0.511331)
(-0.00368256, -0.046461, 0.503178)
(-0.00488339, -0.0536421, 0.496819)
(-0.00748578, -0.0608785, 0.490738)
(-0.0116019, -0.0679727, 0.484338)
(-0.0164083, -0.0749222, 0.479233)
(-0.020053, -0.0815074, 0.476864)
(-0.0235583, -0.0872862, 0.476695)
(-0.0256753, -0.0922156, 0.477493)
(-0.0271972, -0.095614, 0.47988)
(-0.0273415, -0.0974776, 0.481887)
(-0.0253224, -0.0954048, 0.484942)
(-0.0222815, -0.0920711, 0.489219)
(-0.0198294, -0.0884705, 0.495037)
(-0.0173239, -0.0848462, 0.501107)
(-0.014518, -0.0808607, 0.506861)
(-0.0132673, -0.0757284, 0.512149)
(-0.0134328, -0.0664705, 0.516924)
(-0.0138698, -0.0555243, 0.51984)
(-0.015795, -0.0439108, 0.520901)
(-0.0180661, -0.0330837, 0.520812)
(-0.021166, -0.0234065, 0.521523)
(-0.023215, -0.0183196, 0.521128)
(-0.0245234, -0.0164048, 0.51921)
(-0.0245219, -0.0183022, 0.516773)
(-0.0240816, -0.0223521, 0.516157)
(-0.024057, -0.0287219, 0.51456)
(-0.0240238, -0.0374504, 0.510233)
(-0.023756, -0.0478335, 0.505287)
(-0.0221907, -0.0582723, 0.501435)
(-0.019607, -0.0680976, 0.499034)
(-0.0172579, -0.0764166, 0.497687)
(-0.0151506, -0.0834828, 0.496819)
(-0.0130773, -0.0890769, 0.496953)
(-0.010691, -0.0928438, 0.49898)
(-0.00884883, -0.0938376, 0.501422)
(-0.00775501, -0.0930822, 0.504151)
(-0.00725708, -0.0892293, 0.508043)
(-0.00732094, -0.0842066, 0.51265)
(-0.00858179, -0.0782628, 0.518049)
(-0.00982189, -0.0726511, 0.521643)
(-0.0116941, -0.0652635, 0.523715)
(-0.0142142, -0.0570238, 0.52538)
(-0.017076, -0.0491542, 0.52558)
(-0.019646, -0.0423135, 0.524104)
(-0.0211927, -0.0363611, 0.521864)
(-0.0202907, -0.0319292, 0.517767)
(-0.0161124, -0.0293009, 0.511927)
(-0.00644612, -0.0293815, 0.504497)
(0.00829363, -0.0310173, 0.49885)
(0.027639, -0.0344358, 0.497296)
(0.0504913, -0.0400731, 0.500174)
(0.0757953, -0.0465036, 0.503905)
(0.104143, -0.0541413, 0.506987)
(0.135607, -0.0620673, 0.509182)
(0.167875, -0.0695197, 0.509858)
(0.200509, -0.0748667, 0.509755)
(0.233894, -0.0792812, 0.509236)
(0.267209, -0.0826693, 0.510576)
(0.297316, -0.0843094, 0.512639)
(0.326563, -0.0848289, 0.512627)
(0.355913, -0.0844745, 0.511223)
(0.385738, -0.0819114, 0.509026)
(0.415705, -0.0772507, 0.505086)
(0.445293, -0.0707875, 0.500316)
(0.475414, -0.0627835, 0.496933)
(0.505923, -0.0524527, 0.495631)
(0.537235, -0.0429408, 0.495469)
(0.56781, -0.0342369, 0.494555)
(0.597815, -0.02721, 0.492324)
(0.625251, -0.0216666, 0.489804)
(0.649243, -0.0177191, 0.48779)
(0.669977, -0.0183043, 0.486647)
(0.686028, -0.0217919, 0.486283)
(0.697437, -0.0295395, 0.487289)
(0.704263, -0.0426755, 0.491266)
(0.707333, -0.0576093, 0.495792)
(0.70554, -0.0744111, 0.500634)
(0.700429, -0.0903108, 0.504547)
(0.692972, -0.104479, 0.507826)
(0.685917, -0.115806, 0.509875)
(0.678878, -0.124534, 0.511664)
(0.671348, -0.130689, 0.513207)
(0.664675, -0.133648, 0.514179)
(0.659477, -0.134357, 0.513205)
(0.65678, -0.131887, 0.511313)
(0.655948, -0.127204, 0.508505)
(0.65766, -0.1216, 0.506015)
(0.662237, -0.111709, 0.503311)
(0.668674, -0.0972954, 0.500181)
(0.675679, -0.0821967, 0.497583)
(0.682469, -0.0685731, 0.495271)
(0.687056, -0.0569503, 0.492722)
(0.691048, -0.0478973, 0.488916)
(0.693441, -0.0416291, 0.48495)
(0.694934, -0.0389557, 0.480355)
(0.695081, -0.0393448, 0.476893)
(0.694857, -0.0435181, 0.473835)
(0.693597, -0.0512516, 0.471918)
(0.69195, -0.0609336, 0.470353)
(0.690313, -0.0716381, 0.469619)
(0.688182, -0.0856218, 0.470791)
(0.686446, -0.10014, 0.472252)
(0.686115, -0.112908, 0.47501)
(0.686946, -0.121193, 0.477595)
(0.689485, -0.125691, 0.480678)
(0.691448, -0.125428, 0.485512)
(0.692323, -0.122799, 0.490526)
(0.692929, -0.11646, 0.494083)
(0.692939, -0.106626, 0.495699)
(0.694392, -0.0900311, 0.494403)
(0.694573, -0.0688142, 0.492557)
(0.694239, -0.0448565, 0.488204)
(0.694076, -0.0238093, 0.484271)
(0.693887, -0.0063624, 0.481578)
(0.69394, 0.00726877, 0.47915)
(0.695334, 0.0131359, 0.478708)
(0.698478, 0.0141142, 0.479264)
(0.70233, 0.00557423, 0.480454)
(0.705094, -0.00774438, 0.483947)
(0.707432, -0.0247966, 0.487042)
(0.708882, -0.0439222, 0.489815)
(0.709246, -0.0636225, 0.492146)
(0.707182, -0.0805388, 0.494245)
(0.703504, -0.0955599, 0.49564)
(0.696641, -0.107852, 0.499246)
(0.688655, -0.116364, 0.503132)
(0.681106, -0.117311, 0.505999)
(0.676017, -0.1103, 0.508004)
(0.673826, -0.0916116, 0.508775)
(0.675803, -0.0648006, 0.508362)
(0.680485, -0.0281932, 0.507478)
(0.685589, 0.0173939, 0.506996)
(0.688782, 0.0696062, 0.505018)
(0.68815, 0.128845, 0.501422)
(0.684393, 0.190094, 0.498059)
(0.674573, 0.250958, 0.497861)
(0.657236, 0.309091, 0.498351)
(0.632379, 0.363489, 0.498806)
(0.600027, 0.412285, 0.500475)
(0.560082, 0.454633, 0.501494)
(0.51426, 0.491162, 0.502253)
(0.462974, 0.520636, 0.504175)
(0.406288, 0.545196, 0.507254)
(0.344891, 0.566062, 0.510363)
(0.282939, 0.583666, 0.512009)
(0.221575, 0.601948, 0.511867)
(0.164278, 0.619064, 0.510513)
(0.112385, 0.631747, 0.508786)
(0.0653683, 0.639212, 0.506765)
(0.0206393, 0.643754, 0.505219)
(-0.0226518, 0.642351, 0.502044)
(-0.06469, 0.637383, 0.499078)
(-0.106143, 0.627597, 0.496439)
(-0.148049, 0.615236, 0.495672)
(-0.190773, 0.597928, 0.494108)
(-0.235294, 0.575915, 0.493137)
(-0.280574, 0.55138, 0.493954)
(-0.326274, 0.525651, 0.496798)
(-0.369724, 0.500775, 0.498677)
(-0.411943, 0.47619, 0.499235)
(-0.451801, 0.45095, 0.500002)
(-0.489709, 0.419042, 0.499764)
(-0.524901, 0.383003, 0.499486)
(-0.559069, 0.345265, 0.50152)
(-0.58938, 0.307694, 0.500943)
(-0.616968, 0.272457, 0.500124)
(-0.641724, 0.23734, 0.500899)
(-0.66424, 0.201489, 0.498348)
(-0.683717, 0.163107, 0.493537)
(-0.700666, 0.123066, 0.490063)
(-0.715833, 0.0816726, 0.488473)
(-0.726341, 0.0392004, 0.488709)
(-0.732555, -0.00590251, 0.488929)
(-0.734848, -0.0475793, 0.488228)
(-0.733083, -0.0905128, 0.486323)
(-0.727455, -0.137366, 0.483818)
(-0.71451, -0.19025, 0.481333)
(-0.696522, -0.241608, 0.479281)
(-0.675182, -0.295838, 0.477589)
(-0.650285, -0.352293, 0.477197)
(-0.622876, -0.407839, 0.479202)
(-0.59403, -0.461275, 0.48146)
(-0.564047, -0.512327, 0.4836)
(-0.531677, -0.565247, 0.485002)
(-0.498158, -0.616592, 0.485609)
(-0.463964, -0.662661, 0.484419)
(-0.429894, -0.703777, 0.483662)
(-0.393934, -0.740231, 0.482603)
(-0.3554, -0.770925, 0.480214)
(-0.313536, -0.795903, 0.47725)
(-0.269271, -0.813959, 0.474631)
(-0.223758, -0.824793, 0.473298)
(-0.17818, -0.825537, 0.470671)
(-0.131259, -0.816528, 0.467393)
(-0.0846001, -0.801057, 0.464374)
(-0.0377032, -0.779988, 0.463943)
(0.00868349, -0.755731, 0.464863)
(0.0578554, -0.731469, 0.467241)
(0.109388, -0.705315, 0.471315)
(0.160053, -0.678705, 0.475532)
(0.209123, -0.652736, 0.480886)
(0.256472, -0.628371, 0.485256)
(0.302204, -0.606552, 0.489384)
(0.347627, -0.586664, 0.493156)
(0.390412, -0.566965, 0.498563)
(0.430825, -0.548056, 0.503798)
(0.469005, -0.529037, 0.508736)
(0.50477, -0.507822, 0.512433)
(0.53803, -0.483433, 0.514716)
(0.5691, -0.459022, 0.516731)
(0.598661, -0.433074, 0.515524)
(0.626912, -0.40608, 0.512221)
(0.652156, -0.371303, 0.507882)
(0.672671, -0.330066, 0.501837)
(0.688774, -0.289624, 0.49636)
(0.702388, -0.247527, 0.493926)
(0.714385, -0.207024, 0.492871)
(0.723815, -0.169052, 0.493047)
(0.731435, -0.135617, 0.494783)
(0.735914, -0.108204, 0.499302)
(0.737288, -0.0853412, 0.502561)
(0.736347, -0.0692298, 0.503188)
(0.734729, -0.0592333, 0.503561)
(0.733098, -0.0558521, 0.504346)
(0.731378, -0.0563034, 0.504904)
(0.728151, -0.0589973, 0.504273)
(0.723106, -0.0674598, 0.501362)
(0.717471, -0.0791889, 0.498372)
(0.711749, -0.094419, 0.496159)
(0.706326, -0.110578, 0.494595)
(0.700798, -0.125619, 0.493462)
(0.695537, -0.13756, 0.492344)
(0.690374, -0.146051, 0.493444)
(0.685751, -0.151222, 0.493386)
(0.682273, -0.154016, 0.493511)
(0.680105, -0.153205, 0.493934)
(0.678987, -0.149807, 0.494494)
(0.679592, -0.143019, 0.494463)
(0.680341, -0.131294, 0.493314)
(0.681175, -0.114101, 0.491135)
(0.683056, -0.0948708, 0.488883)
(0.685236, -0.0741545, 0.487355)
(0.688549, -0.0553414, 0.486008)
(0.693147, -0.0405429, 0.485576)
(0.698601, -0.030775, 0.485292)
(0.705816, -0.0279057, 0.484274)
(0.713296, -0.029346, 0.485162)
(0.720061, -0.0329512, 0.486964)
(0.726323, -0.0410812, 0.489782)
(0.732289, -0.0518991, 0.494234)
(0.737506, -0.0651493, 0.499119)
(0.740117, -0.0795027, 0.504109)
(0.740707, -0.0945063, 0.507894)
(0.73819, -0.108201, 0.510236)
(0.734367, -0.119489, 0.510761)
(0.728728, -0.127691, 0.510088)
(0.7224, -0.133113, 0.50847)
(0.7155, -0.135481, 0.505977)
(0.70883, -0.133433, 0.501932)
(0.703226, -0.127921, 0.497721)
(0.699552, -0.119204, 0.492475)
(0.697107, -0.108679, 0.490444)
(0.696138, -0.0975153, 0.488975)
(0.696867, -0.086686, 0.487971)
(0.699632, -0.0792279, 0.488997)
(0.703138, -0.0744063, 0.49243)
(0.708092, -0.0728731, 0.497989)
(0.712521, -0.0728162, 0.502532)
(0.714851, -0.0744912, 0.506213)
(0.717278, -0.0776006, 0.50774)
(0.720007, -0.0823161, 0.509174)
(0.720665, -0.0867757, 0.509208)
(0.717397, -0.0920407, 0.509474)
(0.707538, -0.0938149, 0.503626)
(0.688974, -0.0920106, 0.495895)
(0.65845, -0.0883825, 0.486151)
(0.616414, -0.082388, 0.471656)
(0.562595, -0.076707, 0.455716)
(0.49707, -0.0704944, 0.440334)
(0.424488, -0.0658846, 0.424314)
(0.343356, -0.0631852, 0.409918)
(0.257829, -0.060264, 0.395584)
(0.176993, -0.0566959, 0.38146)
(0.103515, -0.0539533, 0.369284)
(0.0391892, -0.055944, 0.357717)
(-0.011835, -0.0629354, 0.344392)
(-0.0495923, -0.0722542, 0.332024)
(-0.074585, -0.0797126, 0.32111)
(-0.0855541, -0.0838574, 0.309692)
(-0.0845024, -0.0865035, 0.298346)
(-0.0732475, -0.088522, 0.286624)
(-0.0540769, -0.0886207, 0.274837)
(-0.029815, -0.0864946, 0.263543)
(-0.00486043, -0.0805295, 0.253706)
(0.0181289, -0.0697478, 0.244245)
(0.0378048, -0.0549473, 0.235567)
(0.0523996, -0.0390432, 0.22842)
(0.0621321, -0.0237546, 0.220824)
(0.0668716, -0.00924309, 0.213939)
(0.066149, 0.00144051, 0.20739)
(0.0608658, 0.00583605, 0.200703)
(0.0517558, 0.00485345, 0.195057)
(0.043142, 0.000510009, 0.188816)
(0.032054, -0.0133467, 0.181334)
(0.0198346, -0.0314476, 0.170181)
(0.00775821, -0.0522268, 0.159158)
(-0.00334577, -0.073382, 0.148956)
(-0.0133752, -0.0927908, 0.139884)
(-0.0221866, -0.111165, 0.131072)
(-0.027483, -0.126832, 0.121939)
(-0.0313185, -0.13793, 0.115128)
(-0.0322671, -0.14198, 0.106879)
(-0.0290394, -0.139293, 0.0966293)
(-0.0239756, -0.13026, 0.0851788)
(-0.0173374, -0.115925, 0.0737807)
(-0.0104428, -0.0985366, 0.0625262)
(-0.00505764, -0.079093, 0.0522328)
(0.000770438, -0.0607731, 0.0425477)
(0.00573119, -0.0444252, 0.0338384)
(0.00996953, -0.0300535, 0.0268771)
(0.0130035, -0.0172527, 0.0211603)
(0.0147414, -0.00671031, 0.016556)
(0.0154509, 0.000824729, 0.0136813)
(0.0156008, 0.00542417, 0.0118248)
(0.0158209, 0.00815899, 0.0107397)
(0.0156272, 0.0089531, 0.0102305)
(0.0153382, 0.00909151, 0.0100162)
(0.0154086, 0.00888808, 0.00980928)
(0.0154034, 0.00863112, 0.00970212)
(0.0154599, 0.00832042, 0.00962418)
(0.0154315, 0.00791448, 0.00949781)
(0.0154753, 0.00744884, 0.00946266)
(0.0153586, 0.00697969, 0.0094368)
(0.0154204, 0.00677099, 0.00940917)
(0.0153438, 0.00718818, 0.00858028)
(0.0152369, 0.00767881, 0.00771092)
(0.0150335, 0.00819443, 0.00687809)
(0.0151244, 0.00879669, 0.0059848)
(0.0150218, 0.00943176, 0.00515812)
(0.0148127, 0.0100344, 0.00440353)
(0.0146107, 0.0107161, 0.00367303)
(0.0145638, 0.0113433, 0.0030464)
(0.0141647, 0.0119485, 0.0024821)
(0.01375, 0.0124781, 0.00204858)
(0.0135853, 0.0129071, 0.00203142)
(0.0131568, 0.0130082, 0.00198329)
(0.0128796, 0.0130917, 0.00193376)
(0.0127551, 0.0132984, 0.00188162)
(0.012606, 0.0134463, 0.00183642)
(0.0122813, 0.0135609, 0.00172756)
(0.0119503, 0.0135292, 0.00151405)
(0.011584, 0.0134324, 0.0013811)
(0.0115741, 0.0130791, 0.00137622)
(0.011699, 0.0129407, 0.00136872)
(0.0118078, 0.0129367, 0.00139763)
(0.0117784, 0.013019, 0.00147847)
(0.0118801, 0.0131074, 0.00150882)
(0.0119583, 0.0132028, 0.00154715)
(0.0120733, 0.013313, 0.00159999)
};


==> exp_plots/circle_traj__battery_combined/th_new.tex <==
\addplot[
    fill=white!60!desclr,draw = desclr,opacity=\opacty,
    line width= \linew pt,
    forget plot
    ]
 %%
coordinates {
(0.075, 1.36613)
(0.15, 2.70863)
(0.225, 4.00956)
(0.3, 5.21807)
(0.375, 6.35432)
(0.45, 7.39491)
(0.525, 8.33023)
(0.6, 9.13845)
(0.675, 9.79848)
(0.75, 10.3008)
(0.825, 10.6788)
(0.9, 10.854)
(0.975, 11.019)
(1.05, 11.247)
(1.125, 11.9053)
(1.2, 12.733)
(1.275, 13.7056)
(1.35, 14.8577)
(1.425, 16.0872)
(1.5, 17.4591)
(1.575, 18.921)
(1.65, 20.4592)
(1.725, 22.016)
(1.8, 23.6272)
(1.875, 25.2494)
(1.95, 26.8367)
(2.025, 28.3997)
(2.1, 29.9923)
(2.175, 31.6164)
(2.25, 33.3008)
(2.325, 35.0173)
(2.4, 36.751)
(2.475, 38.4906)
(2.55, 40.1852)
(2.625, 41.7305)
(2.7, 43.0383)
(2.775, 43.9918)
(2.85, 44.6145)
(2.925, 45.0578)
(3, 45.4658)
(3.075, 45.9487)
(3.15, 46.4592)
(3.225, 46.7757)
(3.3, 46.6932)
(3.375, 46.2366)
(3.45, 45.6448)
(3.525, 45.2917)
(3.6, 45.409)
(3.675, 45.986)
(3.75, 46.7678)
(3.825, 47.208)
(3.9, 47.1801)
(3.975, 46.8438)
(4.05, 46.574)
(4.125, 46.6317)
(4.2, 46.9675)
(4.275, 47.4155)
(4.35, 47.6814)
(4.425, 47.7401)
(4.5, 47.7144)
(4.575, 47.7825)
(4.65, 47.9628)
(4.725, 48.2522)
(4.8, 48.5858)
(4.875, 48.8813)
(4.95, 48.9728)
(5.025, 48.8421)
(5.1, 48.7041)
(5.175, 48.6662)
(5.25, 48.6513)
(5.325, 48.5817)
(5.4, 48.4666)
(5.475, 48.4811)
(5.55, 48.6607)
(5.625, 48.9467)
(5.7, 49.2177)
(5.775, 49.3363)
(5.85, 49.2692)
(5.925, 49.0924)
(6, 48.9288)
(6.075, 48.9026)
(6.15, 49.0134)
(6.225, 49.0258)
(6.3, 48.9114)
(6.375, 48.6573)
(6.45, 48.3651)
(6.525, 48.0848)
(6.6, 47.9638)
(6.675, 48.0443)
(6.75, 48.3126)
(6.825, 48.6581)
(6.9, 48.9293)
(6.975, 49.1401)
(7.05, 49.3255)
(7.125, 49.4398)
(7.2, 49.4572)
(7.275, 49.3809)
(7.35, 49.1932)
(7.425, 48.9658)
(7.5, 48.7667)
(7.575, 48.6909)
(7.65, 48.7854)
(7.725, 48.95)
(7.8, 49.1774)
(7.875, 49.402)
(7.95, 49.479)
(8.025, 49.4743)
(8.1, 49.4676)
(8.175, 49.6423)
(8.25, 50.0949)
(8.325, 50.5818)
(8.4, 50.9412)
(8.475, 51.1872)
(8.55, 51.2094)
(8.625, 51.0666)
(8.7, 50.7587)
(8.775, 50.4168)
(8.85, 50.095)
(8.925, 49.796)
(9, 49.6132)
(9.075, 49.5528)
(9.15, 49.5588)
(9.225, 49.4453)
(9.3, 49.1698)
(9.375, 48.9081)
(9.45, 48.7773)
(9.525, 48.8265)
(9.6, 49.0181)
(9.675, 49.1799)
(9.75, 49.2985)
(9.825, 49.352)
(9.9, 49.3731)
(9.975, 49.482)
(10.05, 49.6883)
(10.125, 49.8761)
(10.2, 49.9248)
(10.275, 49.9903)
(10.35, 50.0333)
(10.425, 50.0186)
(10.5, 49.9426)
(10.575, 49.7894)
(10.65, 49.71)
(10.725, 49.7985)
(10.8, 49.9247)
(10.875, 50.0007)
(10.95, 50.0614)
(11.025, 50.0675)
(11.1, 49.8535)
(11.175, 49.518)
(11.25, 49.3601)
(11.325, 49.4004)
(11.4, 49.5536)
(11.475, 49.7902)
(11.55, 50.0054)
(11.625, 50.0852)
(11.7, 49.9916)
(11.775, 49.7736)
(11.85, 49.6115)
(11.925, 49.6176)
(12, 49.8415)
(12.075, 50.2202)
(12.15, 50.5768)
(12.225, 50.6446)
(12.3, 50.384)
(12.375, 49.9979)
(12.45, 49.8128)
(12.525, 49.892)
(12.6, 50.2424)
(12.675, 50.641)
(12.75, 50.8914)
(12.825, 50.9498)
(12.9, 50.9435)
(12.975, 50.9068)
(13.05, 50.9578)
(13.125, 50.9589)
(13.2, 50.8988)
(13.275, 50.838)
(13.35, 50.7012)
(13.425, 50.5659)
(13.5, 50.3666)
(13.575, 50.0374)
(13.65, 49.6731)
(13.725, 49.319)
(13.8, 49.0889)
(13.875, 48.9395)
(13.95, 48.8637)
(14.025, 48.7758)
(14.1, 48.758)
(14.175, 48.8456)
(14.25, 49.0218)
(14.325, 49.2906)
(14.4, 49.5732)
(14.475, 49.7225)
(14.55, 49.7295)
(14.625, 49.6111)
(14.7, 49.4209)
(14.775, 49.3338)
(14.85, 49.4598)
(14.925, 49.6971)
(15, 49.9393)
(15.075, 50.0752)
(15.15, 50.0188)
(15.225, 49.8873)
(15.3, 49.7672)
(15.375, 49.9261)
(15.45, 50.1874)
(15.525, 50.3923)
(15.6, 50.3775)
(15.675, 50.1981)
(15.75, 50.0339)
(15.825, 49.8779)
(15.9, 49.7537)
(15.975, 49.5072)
(16.05, 49.167)
(16.125, 48.9922)
(16.2, 48.9579)
(16.275, 49.0644)
(16.35, 49.1144)
(16.425, 49.0372)
(16.5, 48.8539)
(16.575, 48.6503)
(16.65, 48.6911)
(16.725, 48.9187)
(16.8, 49.1223)
(16.875, 49.1287)
(16.95, 49.0235)
(17.025, 48.9824)
(17.1, 48.9912)
(17.175, 49.0592)
(17.25, 49.2104)
(17.325, 49.4056)
(17.4, 49.4584)
(17.475, 49.4236)
(17.55, 49.3417)
(17.625, 49.245)
(17.7, 49.2301)
(17.775, 49.2522)
(17.85, 49.2631)
(17.925, 49.2832)
(18, 49.3444)
(18.075, 49.4432)
(18.15, 49.5664)
(18.225, 49.6885)
(18.3, 49.8385)
(18.375, 49.9423)
(18.45, 49.9191)
(18.525, 49.7685)
(18.6, 49.5694)
(18.675, 49.2904)
(18.75, 48.9105)
(18.825, 48.5593)
(18.9, 48.4194)
(18.975, 48.5255)
(19.05, 48.7448)
(19.125, 49.0231)
(19.2, 49.2086)
(19.275, 49.2741)
(19.35, 49.3675)
(19.425, 49.4577)
(19.5, 49.5689)
(19.575, 49.6719)
(19.65, 49.6958)
(19.725, 49.6074)
(19.8, 49.2762)
(19.875, 48.863)
(19.95, 48.6655)
(20.025, 48.954)
(20.1, 49.5646)
(20.175, 50.2286)
(20.25, 50.6323)
(20.325, 50.6708)
(20.4, 50.3584)
(20.475, 49.8709)
(20.55, 49.4543)
(20.625, 49.2872)
(20.7, 49.4078)
(20.775, 49.581)
(20.85, 49.6038)
(20.925, 49.457)
(21, 49.134)
(21.075, 48.7413)
(21.15, 48.4579)
(21.225, 48.4204)
(21.3, 48.4336)
(21.375, 48.4826)
(21.45, 48.5322)
(21.525, 48.4724)
(21.6, 48.3247)
(21.675, 48.1333)
(21.75, 47.999)
(21.825, 48.036)
(21.9, 48.1291)
(21.975, 48.1661)
(22.05, 48.0556)
(22.125, 47.8254)
(22.2, 47.5743)
(22.275, 47.3386)
(22.35, 47.141)
(22.425, 46.9749)
(22.5, 46.8542)
(22.575, 46.787)
(22.65, 46.7448)
(22.725, 46.7179)
(22.8, 46.6893)
(22.875, 46.5866)
(22.95, 46.4217)
(23.025, 46.3068)
(23.1, 46.3114)
(23.175, 46.679)
(23.25, 47.0693)
(23.325, 47.1458)
(23.4, 46.9757)
(23.475, 46.7558)
(23.55, 46.6073)
(23.625, 46.5714)
(23.7, 46.616)
(23.775, 46.6491)
(23.85, 46.725)
(23.925, 46.7124)
(24, 46.4435)
(24.075, 45.9065)
(24.15, 45.449)
(24.225, 45.1065)
(24.3, 44.7637)
(24.375, 44.3066)
(24.45, 43.644)
(24.525, 42.9851)
(24.6, 42.3502)
(24.675, 41.6659)
(24.75, 41.001)
(24.825, 40.372)
(24.9, 39.7537)
(24.975, 39.0283)
(25.05, 38.2784)
(25.125, 37.5436)
(25.2, 36.8971)
(25.275, 36.2589)
(25.35, 35.6095)
(25.425, 34.9852)
(25.5, 34.3734)
(25.575, 33.7668)
(25.65, 33.1264)
(25.725, 32.4324)
(25.8, 31.6715)
(25.875, 30.9011)
(25.95, 30.1412)
(26.025, 29.3248)
(26.1, 28.4831)
(26.175, 27.6243)
(26.25, 26.7439)
(26.325, 25.8448)
(26.4, 24.9256)
(26.475, 24.0192)
(26.55, 23.104)
(26.625, 22.1885)
(26.7, 21.2298)
(26.775, 20.2462)
(26.85, 19.2979)
(26.925, 18.3618)
(27, 17.3874)
(27.075, 16.4077)
(27.15, 15.3833)
(27.225, 14.3625)
(27.3, 13.4122)
(27.375, 12.5957)
(27.45, 11.9085)
(27.525, 11.3478)
(27.6, 10.9018)
(27.675, 10.5569)
(27.75, 10.3075)
(27.825, 10.1456)
(27.9, 10.0512)
(27.975, 10.0106)
(28.05, 10)
(28.125, 10)
(28.2, 10)
(28.275, 10)
(28.35, 10)
(28.425, 10)
(28.5, 10)
(28.575, 10)
(28.65, 10)
(28.725, 10)
(28.8, 10)
(28.875, 10)
(28.95, 10)
(29.025, 10)
(29.1, 10)
(29.175, 10)
(29.25, 10)
(29.325, 10)
(29.4, 10)
(29.475, 10)
(29.55, 10)
(29.625, 10)
(29.7, 10)
(29.775, 10)
(29.85, 10)
(29.925, 10)
(30, 10)
(30.075, 10)
(30.15, 10)
(30.225, 10)
(30.3, 10)
(30.375, 10)
(30.45, 10)
(30.525, 10)
(30.6, 10)
(30.675, 10)
(30.75, 10)
(30.825, 10)
(30.9, 10)
(30.975, 10)
(31.05, 10)
(31.125, 10)
(31.2, 10)
(31.275, 10)
(31.35, 10)
(31.425, 10)
(31.5, 10)
(31.575, 10)
(31.65, 10)
(31.725, 10)
(31.8, 10)
(31.875, 10)
(31.95, 10)
(32.025, 10)
(32.1, 10)
(32.175, 10)
(32.25, 10)
};

==> exp_plots/circle_traj__battery_combined/th_new_no_fill.tex <==
\addplot[
    fill=none,draw = desclr,opacity=1.0,
    line width= \linew pt
    ]
 %%
coordinates {
(0.075, 1.36613)
(0.15, 2.70863)
(0.225, 4.00956)
(0.3, 5.21807)
(0.375, 6.35432)
(0.45, 7.39491)
(0.525, 8.33023)
(0.6, 9.13845)
(0.675, 9.79848)
(0.75, 10.3008)
(0.825, 10.6788)
(0.9, 10.854)
(0.975, 11.019)
(1.05, 11.247)
(1.125, 11.9053)
(1.2, 12.733)
(1.275, 13.7056)
(1.35, 14.8577)
(1.425, 16.0872)
(1.5, 17.4591)
(1.575, 18.921)
(1.65, 20.4592)
(1.725, 22.016)
(1.8, 23.6272)
(1.875, 25.2494)
(1.95, 26.8367)
(2.025, 28.3997)
(2.1, 29.9923)
(2.175, 31.6164)
(2.25, 33.3008)
(2.325, 35.0173)
(2.4, 36.751)
(2.475, 38.4906)
(2.55, 40.1852)
(2.625, 41.7305)
(2.7, 43.0383)
(2.775, 43.9918)
(2.85, 44.6145)
(2.925, 45.0578)
(3, 45.4658)
(3.075, 45.9487)
(3.15, 46.4592)
(3.225, 46.7757)
(3.3, 46.6932)
(3.375, 46.2366)
(3.45, 45.6448)
(3.525, 45.2917)
(3.6, 45.409)
(3.675, 45.986)
(3.75, 46.7678)
(3.825, 47.208)
(3.9, 47.1801)
(3.975, 46.8438)
(4.05, 46.574)
(4.125, 46.6317)
(4.2, 46.9675)
(4.275, 47.4155)
(4.35, 47.6814)
(4.425, 47.7401)
(4.5, 47.7144)
(4.575, 47.7825)
(4.65, 47.9628)
(4.725, 48.2522)
(4.8, 48.5858)
(4.875, 48.8813)
(4.95, 48.9728)
(5.025, 48.8421)
(5.1, 48.7041)
(5.175, 48.6662)
(5.25, 48.6513)
(5.325, 48.5817)
(5.4, 48.4666)
(5.475, 48.4811)
(5.55, 48.6607)
(5.625, 48.9467)
(5.7, 49.2177)
(5.775, 49.3363)
(5.85, 49.2692)
(5.925, 49.0924)
(6, 48.9288)
(6.075, 48.9026)
(6.15, 49.0134)
(6.225, 49.0258)
(6.3, 48.9114)
(6.375, 48.6573)
(6.45, 48.3651)
(6.525, 48.0848)
(6.6, 47.9638)
(6.675, 48.0443)
(6.75, 48.3126)
(6.825, 48.6581)
(6.9, 48.9293)
(6.975, 49.1401)
(7.05, 49.3255)
(7.125, 49.4398)
(7.2, 49.4572)
(7.275, 49.3809)
(7.35, 49.1932)
(7.425, 48.9658)
(7.5, 48.7667)
(7.575, 48.6909)
(7.65, 48.7854)
(7.725, 48.95)
(7.8, 49.1774)
(7.875, 49.402)
(7.95, 49.479)
(8.025, 49.4743)
(8.1, 49.4676)
(8.175, 49.6423)
(8.25, 50.0949)
(8.325, 50.5818)
(8.4, 50.9412)
(8.475, 51.1872)
(8.55, 51.2094)
(8.625, 51.0666)
(8.7, 50.7587)
(8.775, 50.4168)
(8.85, 50.095)
(8.925, 49.796)
(9, 49.6132)
(9.075, 49.5528)
(9.15, 49.5588)
(9.225, 49.4453)
(9.3, 49.1698)
(9.375, 48.9081)
(9.45, 48.7773)
(9.525, 48.8265)
(9.6, 49.0181)
(9.675, 49.1799)
(9.75, 49.2985)
(9.825, 49.352)
(9.9, 49.3731)
(9.975, 49.482)
(10.05, 49.6883)
(10.125, 49.8761)
(10.2, 49.9248)
(10.275, 49.9903)
(10.35, 50.0333)
(10.425, 50.0186)
(10.5, 49.9426)
(10.575, 49.7894)
(10.65, 49.71)
(10.725, 49.7985)
(10.8, 49.9247)
(10.875, 50.0007)
(10.95, 50.0614)
(11.025, 50.0675)
(11.1, 49.8535)
(11.175, 49.518)
(11.25, 49.3601)
(11.325, 49.4004)
(11.4, 49.5536)
(11.475, 49.7902)
(11.55, 50.0054)
(11.625, 50.0852)
(11.7, 49.9916)
(11.775, 49.7736)
(11.85, 49.6115)
(11.925, 49.6176)
(12, 49.8415)
(12.075, 50.2202)
(12.15, 50.5768)
(12.225, 50.6446)
(12.3, 50.384)
(12.375, 49.9979)
(12.45, 49.8128)
(12.525, 49.892)
(12.6, 50.2424)
(12.675, 50.641)
(12.75, 50.8914)
(12.825, 50.9498)
(12.9, 50.9435)
(12.975, 50.9068)
(13.05, 50.9578)
(13.125, 50.9589)
(13.2, 50.8988)
(13.275, 50.838)
(13.35, 50.7012)
(13.425, 50.5659)
(13.5, 50.3666)
(13.575, 50.0374)
(13.65, 49.6731)
(13.725, 49.319)
(13.8, 49.0889)
(13.875, 48.9395)
(13.95, 48.8637)
(14.025, 48.7758)
(14.1, 48.758)
(14.175, 48.8456)
(14.25, 49.0218)
(14.325, 49.2906)
(14.4, 49.5732)
(14.475, 49.7225)
(14.55, 49.7295)
(14.625, 49.6111)
(14.7, 49.4209)
(14.775, 49.3338)
(14.85, 49.4598)
(14.925, 49.6971)
(15, 49.9393)
(15.075, 50.0752)
(15.15, 50.0188)
(15.225, 49.8873)
(15.3, 49.7672)
(15.375, 49.9261)
(15.45, 50.1874)
(15.525, 50.3923)
(15.6, 50.3775)
(15.675, 50.1981)
(15.75, 50.0339)
(15.825, 49.8779)
(15.9, 49.7537)
(15.975, 49.5072)
(16.05, 49.167)
(16.125, 48.9922)
(16.2, 48.9579)
(16.275, 49.0644)
(16.35, 49.1144)
(16.425, 49.0372)
(16.5, 48.8539)
(16.575, 48.6503)
(16.65, 48.6911)
(16.725, 48.9187)
(16.8, 49.1223)
(16.875, 49.1287)
(16.95, 49.0235)
(17.025, 48.9824)
(17.1, 48.9912)
(17.175, 49.0592)
(17.25, 49.2104)
(17.325, 49.4056)
(17.4, 49.4584)
(17.475, 49.4236)
(17.55, 49.3417)
(17.625, 49.245)
(17.7, 49.2301)
(17.775, 49.2522)
(17.85, 49.2631)
(17.925, 49.2832)
(18, 49.3444)
(18.075, 49.4432)
(18.15, 49.5664)
(18.225, 49.6885)
(18.3, 49.8385)
(18.375, 49.9423)
(18.45, 49.9191)
(18.525, 49.7685)
(18.6, 49.5694)
(18.675, 49.2904)
(18.75, 48.9105)
(18.825, 48.5593)
(18.9, 48.4194)
(18.975, 48.5255)
(19.05, 48.7448)
(19.125, 49.0231)
(19.2, 49.2086)
(19.275, 49.2741)
(19.35, 49.3675)
(19.425, 49.4577)
(19.5, 49.5689)
(19.575, 49.6719)
(19.65, 49.6958)
(19.725, 49.6074)
(19.8, 49.2762)
(19.875, 48.863)
(19.95, 48.6655)
(20.025, 48.954)
(20.1, 49.5646)
(20.175, 50.2286)
(20.25, 50.6323)
(20.325, 50.6708)
(20.4, 50.3584)
(20.475, 49.8709)
(20.55, 49.4543)
(20.625, 49.2872)
(20.7, 49.4078)
(20.775, 49.581)
(20.85, 49.6038)
(20.925, 49.457)
(21, 49.134)
(21.075, 48.7413)
(21.15, 48.4579)
(21.225, 48.4204)
(21.3, 48.4336)
(21.375, 48.4826)
(21.45, 48.5322)
(21.525, 48.4724)
(21.6, 48.3247)
(21.675, 48.1333)
(21.75, 47.999)
(21.825, 48.036)
(21.9, 48.1291)
(21.975, 48.1661)
(22.05, 48.0556)
(22.125, 47.8254)
(22.2, 47.5743)
(22.275, 47.3386)
(22.35, 47.141)
(22.425, 46.9749)
(22.5, 46.8542)
(22.575, 46.787)
(22.65, 46.7448)
(22.725, 46.7179)
(22.8, 46.6893)
(22.875, 46.5866)
(22.95, 46.4217)
(23.025, 46.3068)
(23.1, 46.3114)
(23.175, 46.679)
(23.25, 47.0693)
(23.325, 47.1458)
(23.4, 46.9757)
(23.475, 46.7558)
(23.55, 46.6073)
(23.625, 46.5714)
(23.7, 46.616)
(23.775, 46.6491)
(23.85, 46.725)
(23.925, 46.7124)
(24, 46.4435)
(24.075, 45.9065)
(24.15, 45.449)
(24.225, 45.1065)
(24.3, 44.7637)
(24.375, 44.3066)
(24.45, 43.644)
(24.525, 42.9851)
(24.6, 42.3502)
(24.675, 41.6659)
(24.75, 41.001)
(24.825, 40.372)
(24.9, 39.7537)
(24.975, 39.0283)
(25.05, 38.2784)
(25.125, 37.5436)
(25.2, 36.8971)
(25.275, 36.2589)
(25.35, 35.6095)
(25.425, 34.9852)
(25.5, 34.3734)
(25.575, 33.7668)
(25.65, 33.1264)
(25.725, 32.4324)
(25.8, 31.6715)
(25.875, 30.9011)
(25.95, 30.1412)
(26.025, 29.3248)
(26.1, 28.4831)
(26.175, 27.6243)
(26.25, 26.7439)
(26.325, 25.8448)
(26.4, 24.9256)
(26.475, 24.0192)
(26.55, 23.104)
(26.625, 22.1885)
(26.7, 21.2298)
(26.775, 20.2462)
(26.85, 19.2979)
(26.925, 18.3618)
(27, 17.3874)
(27.075, 16.4077)
(27.15, 15.3833)
(27.225, 14.3625)
(27.3, 13.4122)
(27.375, 12.5957)
(27.45, 11.9085)
(27.525, 11.3478)
(27.6, 10.9018)
(27.675, 10.5569)
(27.75, 10.3075)
(27.825, 10.1456)
(27.9, 10.0512)
(27.975, 10.0106)
(28.05, 10)
(28.125, 10)
(28.2, 10)
(28.275, 10)
(28.35, 10)
(28.425, 10)
(28.5, 10)
(28.575, 10)
(28.65, 10)
(28.725, 10)
(28.8, 10)
(28.875, 10)
(28.95, 10)
(29.025, 10)
(29.1, 10)
(29.175, 10)
(29.25, 10)
(29.325, 10)
(29.4, 10)
(29.475, 10)
(29.55, 10)
(29.625, 10)
(29.7, 10)
(29.775, 10)
(29.85, 10)
(29.925, 10)
(30, 10)
(30.075, 10)
(30.15, 10)
(30.225, 10)
(30.3, 10)
(30.375, 10)
(30.45, 10)
(30.525, 10)
(30.6, 10)
(30.675, 10)
(30.75, 10)
(30.825, 10)
(30.9, 10)
(30.975, 10)
(31.05, 10)
(31.125, 10)
(31.2, 10)
(31.275, 10)
(31.35, 10)
(31.425, 10)
(31.5, 10)
(31.575, 10)
(31.65, 10)
(31.725, 10)
(31.8, 10)
(31.875, 10)
(31.95, 10)
(32.025, 10)
(32.1, 10)
(32.175, 10)
(32.25, 10)
};

==> exp_plots/circle_traj__battery_combined/th_old.tex <==
\addplot[
    fill=white!60!currclr,draw = currclr,opacity=\opacty,
    line width= \linew pt,
    forget plot
    ]
 %%
coordinates{
(0, 0)
(0.075, 2.18577)
(0.15, 4.23483)
(0.225, 6.06637)
(0.3, 7.61336)
(0.375, 8.81445)
(0.45, 9.62203)
(0.525, 10.0041)
(0.6, 10.001)
(0.675, 10)
(0.75, 10)
(0.825, 10)
(0.9, 10)
(0.975, 10.0275)
(1.05, 10.3011)
(1.125, 11.3187)
(1.2, 12.5678)
(1.275, 13.9688)
(1.35, 15.531)
(1.425, 17.1107)
(1.5, 18.7003)
(1.575, 20.2407)
(1.65, 21.6878)
(1.725, 23.128)
(1.8, 24.59)
(1.875, 26.1403)
(1.95, 27.7055)
(2.025, 29.1915)
(2.1, 30.7221)
(2.175, 32.2848)
(2.25, 33.8484)
(2.325, 35.4759)
(2.4, 37.0323)
(2.475, 38.6641)
(2.55, 40.3316)
(2.625, 42.0447)
(2.7, 43.7557)
(2.775, 45.4511)
(2.85, 47.1042)
(2.925, 48.5143)
(3, 49.7109)
(3.075, 50.5763)
(3.15, 50.9001)
(3.225, 50.8352)
(3.3, 50.859)
(3.375, 51.3642)
(3.45, 52.2496)
(3.525, 53.0365)
(3.6, 53.4759)
(3.675, 53.2775)
(3.75, 52.4155)
(3.825, 51.2706)
(3.9, 50.6357)
(3.975, 50.5147)
(4.05, 50.8751)
(4.125, 51.8005)
(4.2, 52.9173)
(4.275, 54.0399)
(4.35, 54.8377)
(4.425, 55.1289)
(4.5, 55.0411)
(4.575, 54.8106)
(4.65, 54.5534)
(4.725, 54.4343)
(4.8, 54.4356)
(4.875, 54.6173)
(4.95, 55.004)
(5.025, 55.598)
(5.1, 56.2317)
(5.175, 56.7723)
(5.25, 57.1362)
(5.325, 57.4266)
(5.4, 57.6587)
(5.475, 57.7641)
(5.55, 57.7821)
(5.625, 57.6962)
(5.7, 57.6361)
(5.775, 57.6551)
(5.85, 57.6862)
(5.925, 57.7162)
(6, 57.8805)
(6.075, 58.1619)
(6.15, 58.3586)
(6.225, 58.4077)
(6.3, 58.3772)
(6.375, 58.3561)
(6.45, 58.3923)
(6.525, 58.5746)
(6.6, 58.8166)
(6.675, 59.0426)
(6.75, 59.1795)
(6.825, 59.3527)
(6.9, 59.5716)
(6.975, 59.8604)
(7.05, 60.0358)
(7.125, 59.9421)
(7.2, 59.5511)
(7.275, 58.9524)
(7.35, 58.3756)
(7.425, 57.8361)
(7.5, 57.716)
(7.575, 58.1317)
(7.65, 58.4036)
(7.725, 58.3036)
(7.8, 57.7273)
(7.875, 56.9171)
(7.95, 56.3435)
(8.025, 56.284)
(8.1, 56.7087)
(8.175, 57.6578)
(8.25, 58.7531)
(8.325, 59.8581)
(8.4, 61.1647)
(8.475, 62.2102)
(8.55, 62.8903)
(8.625, 63.0502)
(8.7, 62.7938)
(8.775, 62.2151)
(8.85, 61.7648)
(8.925, 61.4629)
(9, 61.4237)
(9.075, 61.5971)
(9.15, 61.9773)
(9.225, 62.4324)
(9.3, 62.9563)
(9.375, 63.31)
(9.45, 63.3505)
(9.525, 63.1528)
(9.6, 62.9595)
(9.675, 62.8155)
(9.75, 62.7205)
(9.825, 62.696)
(9.9, 62.7578)
(9.975, 62.866)
(10.05, 63.0208)
(10.125, 63.1691)
(10.2, 63.326)
(10.275, 63.5245)
(10.35, 63.6796)
(10.425, 63.8102)
(10.5, 63.9351)
(10.575, 63.917)
(10.65, 63.7494)
(10.725, 63.5991)
(10.8, 63.2352)
(10.875, 62.5693)
(10.95, 62.1163)
(11.025, 61.8826)
(11.1, 61.9188)
(11.175, 62.0692)
(11.25, 62.1301)
(11.325, 62.1793)
(11.4, 62.2383)
(11.475, 62.1529)
(11.55, 62.0634)
(11.625, 62.1451)
(11.7, 62.3835)
(11.775, 62.7952)
(11.85, 63.269)
(11.925, 63.6505)
(12, 63.8358)
(12.075, 63.8636)
(12.15, 63.8834)
(12.225, 63.9571)
(12.3, 64.1877)
(12.375, 64.3829)
(12.45, 64.5807)
(12.525, 64.9018)
(12.6, 65.5289)
(12.675, 66.4754)
(12.75, 67.3216)
(12.825, 67.8582)
(12.9, 68.1078)
(12.975, 68.1963)
(13.05, 68.2294)
(13.125, 68.1083)
(13.2, 67.7196)
(13.275, 67.1999)
(13.35, 66.6762)
(13.425, 66.259)
(13.5, 66.0807)
(13.575, 66.1152)
(13.65, 66.2543)
(13.725, 66.4213)
(13.8, 66.4148)
(13.875, 66.2838)
(13.95, 66.1002)
(14.025, 65.9636)
(14.1, 65.7993)
(14.175, 65.7194)
(14.25, 65.7551)
(14.325, 65.9315)
(14.4, 66.1894)
(14.475, 66.4504)
(14.55, 66.7255)
(14.625, 67.0051)
(14.7, 67.2594)
(14.775, 67.5043)
(14.85, 67.6911)
(14.925, 67.7555)
(15, 67.8016)
(15.075, 67.8907)
(15.15, 68.1037)
(15.225, 68.4094)
(15.3, 68.5849)
(15.375, 68.6004)
(15.45, 68.4187)
(15.525, 68.22)
(15.6, 68.1285)
(15.675, 68.0837)
(15.75, 68.1279)
(15.825, 68.2089)
(15.9, 68.3749)
(15.975, 68.6272)
(16.05, 68.9472)
(16.125, 69.2039)
(16.2, 69.3107)
(16.275, 69.3132)
(16.35, 69.1475)
(16.425, 68.7414)
(16.5, 68.2586)
(16.575, 67.9535)
(16.65, 67.9017)
(16.725, 67.9997)
(16.8, 68.2722)
(16.875, 68.7144)
(16.95, 69.1553)
(17.025, 69.4761)
(17.1, 69.6179)
(17.175, 69.6463)
(17.25, 69.3426)
(17.325, 68.9573)
(17.4, 68.5098)
(17.475, 68.1087)
(17.55, 67.9165)
(17.625, 67.9118)
(17.7, 68.0244)
(17.775, 68.2757)
(17.85, 68.5058)
(17.925, 68.7524)
(18, 69.0075)
(18.075, 69.3207)
(18.15, 69.7168)
(18.225, 70.0442)
(18.3, 70.1575)
(18.375, 70.1042)
(18.45, 69.9011)
(18.525, 69.6057)
(18.6, 69.3505)
(18.675, 69.3679)
(18.75, 69.6284)
(18.825, 69.7071)
(18.9, 69.677)
(18.975, 69.5904)
(19.05, 69.3913)
(19.125, 69.2797)
(19.2, 69.3005)
(19.275, 69.4169)
(19.35, 69.5598)
(19.425, 69.5532)
(19.5, 69.6666)
(19.575, 69.7775)
(19.65, 69.8621)
(19.725, 69.7757)
(19.8, 69.7274)
(19.875, 69.6972)
(19.95, 69.6114)
(20.025, 69.3247)
(20.1, 68.85)
(20.175, 68.3718)
(20.25, 67.9477)
(20.325, 67.4781)
(20.4, 67.0791)
(20.475, 66.8692)
(20.55, 66.8755)
(20.625, 67.1161)
(20.7, 67.486)
(20.775, 67.8316)
(20.85, 68.0902)
(20.925, 68.0455)
(21, 67.7425)
(21.075, 67.2502)
(21.15, 66.7004)
(21.225, 66.2326)
(21.3, 65.8859)
(21.375, 65.6965)
(21.45, 65.633)
(21.525, 65.6673)
(21.6, 65.7184)
(21.675, 65.6733)
(21.75, 65.5262)
(21.825, 65.2746)
(21.9, 64.9259)
(21.975, 64.5328)
(22.05, 64.1039)
(22.125, 63.6958)
(22.2, 63.3855)
(22.275, 63.1873)
(22.35, 63.1749)
(22.425, 63.3639)
(22.5, 63.6684)
(22.575, 63.9967)
(22.65, 64.2418)
(22.725, 64.4003)
(22.8, 64.3888)
(22.875, 64.188)
(22.95, 63.9026)
(23.025, 63.5382)
(23.1, 63.0514)
(23.175, 62.5368)
(23.25, 62.2042)
(23.325, 62.0546)
(23.4, 62.1042)
(23.475, 62.088)
(23.55, 62.1571)
(23.625, 62.2593)
(23.7, 62.3309)
(23.775, 62.1371)
(23.85, 61.811)
(23.925, 61.4388)
(24, 60.93)
(24.075, 60.4294)
(24.15, 60.1182)
(24.225, 60.1763)
(24.3, 60.4074)
(24.375, 60.6541)
(24.45, 61.0324)
(24.525, 61.4938)
(24.6, 61.8057)
(24.675, 61.5929)
(24.75, 60.4211)
(24.825, 59.3553)
(24.9, 58.3047)
(24.975, 57.3069)
(25.05, 56.3103)
(25.125, 55.4003)
(25.2, 54.6511)
(25.275, 53.995)
(25.35, 53.2967)
(25.425, 52.5996)
(25.5, 51.8523)
(25.575, 51.1409)
(25.65, 50.3676)
(25.725, 49.5382)
(25.8, 48.7434)
(25.875, 47.9898)
(25.95, 47.1552)
(26.025, 46.3321)
(26.1, 45.5455)
(26.175, 44.7442)
(26.25, 43.9201)
(26.325, 43.0539)
(26.4, 42.1848)
(26.475, 41.3122)
(26.55, 40.4052)
(26.625, 39.4563)
(26.7, 38.4942)
(26.775, 37.4721)
(26.85, 36.4371)
(26.925, 35.3724)
(27, 34.2976)
(27.075, 33.1895)
(27.15, 32.0826)
(27.225, 30.9922)
(27.3, 29.9457)
(27.375, 28.9756)
(27.45, 28.1109)
(27.525, 27.323)
(27.6, 26.6507)
(27.675, 25.9977)
(27.75, 25.2833)
(27.825, 24.5057)
(27.9, 23.6511)
(27.975, 22.7821)
(28.05, 21.9254)
(28.125, 21.0265)
(28.2, 20.1324)
(28.275, 19.2659)
(28.35, 18.4172)
(28.425, 17.4901)
(28.5, 16.5134)
(28.575, 15.5497)
(28.65, 14.5136)
(28.725, 13.4678)
(28.8, 12.4122)
(28.875, 11.5522)
(28.95, 10.9151)
(29.025, 10.4727)
(29.1, 10.196)
(29.175, 10.0567)
(29.25, 10.0054)
(29.325, 10)
(29.4, 10)
(29.475, 10)
(29.55, 10)
(29.625, 10)
(29.7, 10)
(29.775, 10)
(29.85, 10)
(29.925, 10)
(30, 10)
(30.075, 10)
(30.15, 10)
(30.225, 10)
(30.3, 10)
(30.375, 10)
(30.45, 10)
(30.525, 10)
(30.6, 10)
(30.675, 10)
(30.75, 10)
(30.825, 10)
(30.9, 10)
(30.975, 10)
(31.05, 10)
(31.125, 10)
(31.2, 10)
(31.275, 10)
(31.35, 10)
(31.425, 10)
(31.5, 10)
(31.575, 10)
(31.65, 10)
(31.725, 10)
(31.8, 10)
(31.875, 10)
(31.95, 10)
(32.025, 10)
(32.1, 10)
(32.175, 10)
(32.25, 10)
(32.325, 10)
(32.4, 10)
(32.475, 10)
(32.55, 10)
(32.625, 10)
(32.7, 10)
(32.775, 10)
(32.85, 10)
(32.925, 10)
(33, 10)
(33.075, 10)
(33.15, 10)
(33.225, 10)
(33.3, 10)
(33.375, 10)
(33.45, 10)
(33.525, 10)
(33.6, 10)
(33.675, 10)
(33.75, 10)
(33.825, 10)
};

==> exp_plots/circle_traj__battery_combined/th_old_no_fill.tex <==
\addplot[
    fill=none,draw = currclr,opacity=1.0,
    line width= \linew pt,
    ]
 %%
coordinates{
(0, 0)
(0.075, 2.18577)
(0.15, 4.23483)
(0.225, 6.06637)
(0.3, 7.61336)
(0.375, 8.81445)
(0.45, 9.62203)
(0.525, 10.0041)
(0.6, 10.001)
(0.675, 10)
(0.75, 10)
(0.825, 10)
(0.9, 10)
(0.975, 10.0275)
(1.05, 10.3011)
(1.125, 11.3187)
(1.2, 12.5678)
(1.275, 13.9688)
(1.35, 15.531)
(1.425, 17.1107)
(1.5, 18.7003)
(1.575, 20.2407)
(1.65, 21.6878)
(1.725, 23.128)
(1.8, 24.59)
(1.875, 26.1403)
(1.95, 27.7055)
(2.025, 29.1915)
(2.1, 30.7221)
(2.175, 32.2848)
(2.25, 33.8484)
(2.325, 35.4759)
(2.4, 37.0323)
(2.475, 38.6641)
(2.55, 40.3316)
(2.625, 42.0447)
(2.7, 43.7557)
(2.775, 45.4511)
(2.85, 47.1042)
(2.925, 48.5143)
(3, 49.7109)
(3.075, 50.5763)
(3.15, 50.9001)
(3.225, 50.8352)
(3.3, 50.859)
(3.375, 51.3642)
(3.45, 52.2496)
(3.525, 53.0365)
(3.6, 53.4759)
(3.675, 53.2775)
(3.75, 52.4155)
(3.825, 51.2706)
(3.9, 50.6357)
(3.975, 50.5147)
(4.05, 50.8751)
(4.125, 51.8005)
(4.2, 52.9173)
(4.275, 54.0399)
(4.35, 54.8377)
(4.425, 55.1289)
(4.5, 55.0411)
(4.575, 54.8106)
(4.65, 54.5534)
(4.725, 54.4343)
(4.8, 54.4356)
(4.875, 54.6173)
(4.95, 55.004)
(5.025, 55.598)
(5.1, 56.2317)
(5.175, 56.7723)
(5.25, 57.1362)
(5.325, 57.4266)
(5.4, 57.6587)
(5.475, 57.7641)
(5.55, 57.7821)
(5.625, 57.6962)
(5.7, 57.6361)
(5.775, 57.6551)
(5.85, 57.6862)
(5.925, 57.7162)
(6, 57.8805)
(6.075, 58.1619)
(6.15, 58.3586)
(6.225, 58.4077)
(6.3, 58.3772)
(6.375, 58.3561)
(6.45, 58.3923)
(6.525, 58.5746)
(6.6, 58.8166)
(6.675, 59.0426)
(6.75, 59.1795)
(6.825, 59.3527)
(6.9, 59.5716)
(6.975, 59.8604)
(7.05, 60.0358)
(7.125, 59.9421)
(7.2, 59.5511)
(7.275, 58.9524)
(7.35, 58.3756)
(7.425, 57.8361)
(7.5, 57.716)
(7.575, 58.1317)
(7.65, 58.4036)
(7.725, 58.3036)
(7.8, 57.7273)
(7.875, 56.9171)
(7.95, 56.3435)
(8.025, 56.284)
(8.1, 56.7087)
(8.175, 57.6578)
(8.25, 58.7531)
(8.325, 59.8581)
(8.4, 61.1647)
(8.475, 62.2102)
(8.55, 62.8903)
(8.625, 63.0502)
(8.7, 62.7938)
(8.775, 62.2151)
(8.85, 61.7648)
(8.925, 61.4629)
(9, 61.4237)
(9.075, 61.5971)
(9.15, 61.9773)
(9.225, 62.4324)
(9.3, 62.9563)
(9.375, 63.31)
(9.45, 63.3505)
(9.525, 63.1528)
(9.6, 62.9595)
(9.675, 62.8155)
(9.75, 62.7205)
(9.825, 62.696)
(9.9, 62.7578)
(9.975, 62.866)
(10.05, 63.0208)
(10.125, 63.1691)
(10.2, 63.326)
(10.275, 63.5245)
(10.35, 63.6796)
(10.425, 63.8102)
(10.5, 63.9351)
(10.575, 63.917)
(10.65, 63.7494)
(10.725, 63.5991)
(10.8, 63.2352)
(10.875, 62.5693)
(10.95, 62.1163)
(11.025, 61.8826)
(11.1, 61.9188)
(11.175, 62.0692)
(11.25, 62.1301)
(11.325, 62.1793)
(11.4, 62.2383)
(11.475, 62.1529)
(11.55, 62.0634)
(11.625, 62.1451)
(11.7, 62.3835)
(11.775, 62.7952)
(11.85, 63.269)
(11.925, 63.6505)
(12, 63.8358)
(12.075, 63.8636)
(12.15, 63.8834)
(12.225, 63.9571)
(12.3, 64.1877)
(12.375, 64.3829)
(12.45, 64.5807)
(12.525, 64.9018)
(12.6, 65.5289)
(12.675, 66.4754)
(12.75, 67.3216)
(12.825, 67.8582)
(12.9, 68.1078)
(12.975, 68.1963)
(13.05, 68.2294)
(13.125, 68.1083)
(13.2, 67.7196)
(13.275, 67.1999)
(13.35, 66.6762)
(13.425, 66.259)
(13.5, 66.0807)
(13.575, 66.1152)
(13.65, 66.2543)
(13.725, 66.4213)
(13.8, 66.4148)
(13.875, 66.2838)
(13.95, 66.1002)
(14.025, 65.9636)
(14.1, 65.7993)
(14.175, 65.7194)
(14.25, 65.7551)
(14.325, 65.9315)
(14.4, 66.1894)
(14.475, 66.4504)
(14.55, 66.7255)
(14.625, 67.0051)
(14.7, 67.2594)
(14.775, 67.5043)
(14.85, 67.6911)
(14.925, 67.7555)
(15, 67.8016)
(15.075, 67.8907)
(15.15, 68.1037)
(15.225, 68.4094)
(15.3, 68.5849)
(15.375, 68.6004)
(15.45, 68.4187)
(15.525, 68.22)
(15.6, 68.1285)
(15.675, 68.0837)
(15.75, 68.1279)
(15.825, 68.2089)
(15.9, 68.3749)
(15.975, 68.6272)
(16.05, 68.9472)
(16.125, 69.2039)
(16.2, 69.3107)
(16.275, 69.3132)
(16.35, 69.1475)
(16.425, 68.7414)
(16.5, 68.2586)
(16.575, 67.9535)
(16.65, 67.9017)
(16.725, 67.9997)
(16.8, 68.2722)
(16.875, 68.7144)
(16.95, 69.1553)
(17.025, 69.4761)
(17.1, 69.6179)
(17.175, 69.6463)
(17.25, 69.3426)
(17.325, 68.9573)
(17.4, 68.5098)
(17.475, 68.1087)
(17.55, 67.9165)
(17.625, 67.9118)
(17.7, 68.0244)
(17.775, 68.2757)
(17.85, 68.5058)
(17.925, 68.7524)
(18, 69.0075)
(18.075, 69.3207)
(18.15, 69.7168)
(18.225, 70.0442)
(18.3, 70.1575)
(18.375, 70.1042)
(18.45, 69.9011)
(18.525, 69.6057)
(18.6, 69.3505)
(18.675, 69.3679)
(18.75, 69.6284)
(18.825, 69.7071)
(18.9, 69.677)
(18.975, 69.5904)
(19.05, 69.3913)
(19.125, 69.2797)
(19.2, 69.3005)
(19.275, 69.4169)
(19.35, 69.5598)
(19.425, 69.5532)
(19.5, 69.6666)
(19.575, 69.7775)
(19.65, 69.8621)
(19.725, 69.7757)
(19.8, 69.7274)
(19.875, 69.6972)
(19.95, 69.6114)
(20.025, 69.3247)
(20.1, 68.85)
(20.175, 68.3718)
(20.25, 67.9477)
(20.325, 67.4781)
(20.4, 67.0791)
(20.475, 66.8692)
(20.55, 66.8755)
(20.625, 67.1161)
(20.7, 67.486)
(20.775, 67.8316)
(20.85, 68.0902)
(20.925, 68.0455)
(21, 67.7425)
(21.075, 67.2502)
(21.15, 66.7004)
(21.225, 66.2326)
(21.3, 65.8859)
(21.375, 65.6965)
(21.45, 65.633)
(21.525, 65.6673)
(21.6, 65.7184)
(21.675, 65.6733)
(21.75, 65.5262)
(21.825, 65.2746)
(21.9, 64.9259)
(21.975, 64.5328)
(22.05, 64.1039)
(22.125, 63.6958)
(22.2, 63.3855)
(22.275, 63.1873)
(22.35, 63.1749)
(22.425, 63.3639)
(22.5, 63.6684)
(22.575, 63.9967)
(22.65, 64.2418)
(22.725, 64.4003)
(22.8, 64.3888)
(22.875, 64.188)
(22.95, 63.9026)
(23.025, 63.5382)
(23.1, 63.0514)
(23.175, 62.5368)
(23.25, 62.2042)
(23.325, 62.0546)
(23.4, 62.1042)
(23.475, 62.088)
(23.55, 62.1571)
(23.625, 62.2593)
(23.7, 62.3309)
(23.775, 62.1371)
(23.85, 61.811)
(23.925, 61.4388)
(24, 60.93)
(24.075, 60.4294)
(24.15, 60.1182)
(24.225, 60.1763)
(24.3, 60.4074)
(24.375, 60.6541)
(24.45, 61.0324)
(24.525, 61.4938)
(24.6, 61.8057)
(24.675, 61.5929)
(24.75, 60.4211)
(24.825, 59.3553)
(24.9, 58.3047)
(24.975, 57.3069)
(25.05, 56.3103)
(25.125, 55.4003)
(25.2, 54.6511)
(25.275, 53.995)
(25.35, 53.2967)
(25.425, 52.5996)
(25.5, 51.8523)
(25.575, 51.1409)
(25.65, 50.3676)
(25.725, 49.5382)
(25.8, 48.7434)
(25.875, 47.9898)
(25.95, 47.1552)
(26.025, 46.3321)
(26.1, 45.5455)
(26.175, 44.7442)
(26.25, 43.9201)
(26.325, 43.0539)
(26.4, 42.1848)
(26.475, 41.3122)
(26.55, 40.4052)
(26.625, 39.4563)
(26.7, 38.4942)
(26.775, 37.4721)
(26.85, 36.4371)
(26.925, 35.3724)
(27, 34.2976)
(27.075, 33.1895)
(27.15, 32.0826)
(27.225, 30.9922)
(27.3, 29.9457)
(27.375, 28.9756)
(27.45, 28.1109)
(27.525, 27.323)
(27.6, 26.6507)
(27.675, 25.9977)
(27.75, 25.2833)
(27.825, 24.5057)
(27.9, 23.6511)
(27.975, 22.7821)
(28.05, 21.9254)
(28.125, 21.0265)
(28.2, 20.1324)
(28.275, 19.2659)
(28.35, 18.4172)
(28.425, 17.4901)
(28.5, 16.5134)
(28.575, 15.5497)
(28.65, 14.5136)
(28.725, 13.4678)
(28.8, 12.4122)
(28.875, 11.5522)
(28.95, 10.9151)
(29.025, 10.4727)
(29.1, 10.196)
(29.175, 10.0567)
(29.25, 10.0054)
(29.325, 10)
(29.4, 10)
(29.475, 10)
(29.55, 10)
(29.625, 10)
(29.7, 10)
(29.775, 10)
(29.85, 10)
(29.925, 10)
(30, 10)
(30.075, 10)
(30.15, 10)
(30.225, 10)
(30.3, 10)
(30.375, 10)
(30.45, 10)
(30.525, 10)
(30.6, 10)
(30.675, 10)
(30.75, 10)
(30.825, 10)
(30.9, 10)
(30.975, 10)
(31.05, 10)
(31.125, 10)
(31.2, 10)
(31.275, 10)
(31.35, 10)
(31.425, 10)
(31.5, 10)
(31.575, 10)
(31.65, 10)
(31.725, 10)
(31.8, 10)
(31.875, 10)
(31.95, 10)
(32.025, 10)
(32.1, 10)
(32.175, 10)
(32.25, 10)
(32.325, 10)
(32.4, 10)
(32.475, 10)
(32.55, 10)
(32.625, 10)
(32.7, 10)
(32.775, 10)
(32.85, 10)
(32.925, 10)
(33, 10)
(33.075, 10)
(33.15, 10)
(33.225, 10)
(33.3, 10)
(33.375, 10)
(33.45, 10)
(33.525, 10)
(33.6, 10)
(33.675, 10)
(33.75, 10)
(33.825, 10)
};

==> exp_plots/constrained_ws/az.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0)
(0.0759494, 0.000747469)
(0.151899, -0.00455524)
(0.227848, -0.0046282)
(0.303797, -0.00423182)
(0.379747, -0.0107903)
(0.455696, -0.0188462)
(0.531646, -0.030216)
(0.607595, -0.0304064)
(0.683544, -0.00780636)
(0.759494, 0.00186311)
(0.835443, 0.0178705)
(0.911392, 0.0237428)
(0.987342, 0.0180555)
(1.06329, 0.00967672)
(1.13924, 0.00121879)
(1.21519, -0.00962183)
(1.29114, -0.0024892)
(1.36709, -0.0117491)
(1.44304, -0.0200031)
(1.51899, -0.00838209)
(1.59494, -0.00297075)
(1.67089, -0.0134158)
(1.74684, -0.0106662)
(1.82278, 0.00590629)
(1.89873, 0.013764)
(1.97468, 0.0190151)
(2.05063, -0.0104788)
(2.12658, -0.000686378)
(2.20253, 0.0169866)
(2.27848, 0.0307085)
(2.35443, 0.0639514)
(2.43038, 0.0626377)
(2.50633, 0.0595726)
(2.58228, 0.0596556)
(2.65823, 0.0943555)
(2.73418, 0.174411)
(2.81013, 0.322981)
(2.88608, 0.427967)
(2.96203, 0.438989)
(3.03797, 0.345729)
(3.11392, 0.173314)
(3.18987, 0.0361)
(3.26582, -0.0439762)
(3.34177, -0.101039)
(3.41772, -0.19073)
(3.49367, -0.28991)
(3.56962, -0.300305)
(3.64557, -0.162716)
(3.72152, 0.0652185)
(3.79747, 0.292656)
(3.87342, 0.406862)
(3.94937, 0.299777)
(4.02532, -0.00995444)
(4.10127, -0.312789)
(4.17722, -0.423487)
(4.25316, -0.288732)
(4.32911, -0.00846884)
(4.40506, 0.204101)
(4.48101, 0.256458)
(4.55696, 0.0769439)
(4.63291, -0.0941336)
(4.70886, -0.120086)
(4.78481, -0.0314119)
(4.86076, 0.102218)
(4.93671, 0.228686)
(5.01266, 0.236269)
(5.08861, 0.0990517)
(5.16456, -0.0138261)
(5.24051, -0.088094)
(5.31646, -0.11738)
(5.39241, -0.0561154)
(5.46835, 0.044327)
(5.5443, 0.107455)
(5.62025, 0.165948)
(5.6962, 0.210511)
(5.77215, 0.19497)
(5.8481, 0.117001)
(5.92405, 0.0120057)
(6, -0.147291)
(6.07595, -0.279885)
(6.1519, -0.289214)
(6.22785, -0.140196)
(6.3038, 0.0219963)
(6.37975, 0.175253)
(6.4557, 0.225855)
(6.53165, 0.168517)
(6.60759, 0.0370069)
(6.68354, -0.13087)
(6.75949, -0.239701)
(6.83544, -0.262754)
(6.91139, -0.230732)
(6.98734, -0.130636)
(7.06329, 0.0469638)
(7.13924, 0.216813)
(7.21519, 0.263794)
(7.29114, 0.21214)
(7.36709, 0.0794639)
(7.44304, -0.119913)
(7.51899, -0.250579)
(7.59494, -0.272242)
(7.67089, -0.261197)
(7.74684, -0.165481)
(7.82278, -0.059643)
(7.89873, -0.056676)
(7.97468, -0.0663264)
(8.05063, -0.0813792)
(8.12658, -0.123266)
(8.20253, -0.142756)
(8.27848, -0.145828)
(8.35443, -0.124083)
(8.43038, -0.0610176)
(8.50633, -0.0402947)
(8.58228, -0.087806)
(8.65823, -0.167994)
(8.73418, -0.206094)
(8.81013, -0.151118)
(8.88608, -0.0230557)
(8.96203, 0.100194)
(9.03798, 0.19918)
(9.11392, 0.286876)
(9.18987, 0.316212)
(9.26582, 0.301014)
(9.34177, 0.210582)
(9.41772, 0.0482523)
(9.49367, -0.142165)
(9.56962, -0.25527)
(9.64557, -0.223017)
(9.72152, -0.069437)
(9.79747, 0.104175)
(9.87342, 0.205963)
(9.94937, 0.201003)
(10.0253, 0.162682)
(10.1013, 0.0941298)
(10.1772, 0.0584696)
(10.2532, 0.0363659)
(10.3291, 0.0484123)
(10.4051, 0.0987718)
(10.481, 0.177647)
(10.557, 0.204425)
(10.6329, 0.158569)
(10.7089, 0.0650562)
(10.7848, -0.0824419)
(10.8608, -0.172913)
(10.9367, -0.118725)
(11.0127, 0.000757731)
(11.0886, 0.156684)
(11.1646, 0.2509)
(11.2405, 0.184379)
(11.3165, -0.00278138)
(11.3924, -0.230218)
(11.4684, -0.40484)
(11.5443, -0.421668)
(11.6203, -0.289805)
(11.6962, -0.0462855)
(11.7722, 0.163763)
(11.8481, 0.276915)
(11.9241, 0.309023)
(12, 0.228259)
(12.0759, 0.0239131)
(12.1519, -0.192004)
(12.2278, -0.30362)
(12.3038, -0.30219)
(12.3797, -0.167804)
(12.4557, 0.0375905)
(12.5316, 0.226428)
(12.6076, 0.321993)
(12.6835, 0.29468)
(12.7595, 0.123679)
(12.8354, -0.0907648)
(12.9114, -0.214578)
(12.9873, -0.23518)
(13.0633, -0.173761)
(13.1392, -0.0861396)
(13.2152, 0.0625454)
(13.2911, 0.183363)
(13.3671, 0.209145)
(13.443, 0.097736)
(13.519, -0.0577787)
(13.5949, -0.0316414)
(13.6709, 0.00862424)
(13.7468, 0.105587)
(13.8228, 0.088333)
(13.8987, -0.0256519)
(13.9747, -0.15375)
(14.0506, -0.268607)
(14.1266, -0.288327)
(14.2025, -0.244394)
(14.2785, -0.0817253)
(14.3544, 0.166452)
(14.4304, 0.365998)
(14.5063, 0.4926)
(14.5823, 0.458911)
(14.6582, 0.284764)
(14.7342, 0.0229014)
(14.8101, -0.24778)
(14.8861, -0.34332)
(14.962, -0.250252)
(15.038, -0.0527674)
(15.1139, 0.161723)
(15.1899, 0.226733)
(15.2658, 0.147053)
(15.3418, -0.000786766)
(15.4177, -0.122372)
(15.4937, -0.16771)
(15.5696, -0.119181)
(15.6456, -0.101671)
(15.7215, -0.116023)
(15.7975, -0.16656)
(15.8734, -0.235385)
(15.9494, -0.24098)
(16.0253, -0.208439)
(16.1013, -0.100498)
(16.1772, 0.0165212)
(16.2532, 0.107946)
(16.3291, 0.117877)
(16.4051, 0.117261)
(16.481, 0.169751)
(16.557, 0.186479)
(16.6329, 0.161064)
(16.7089, 0.0756419)
(16.7848, -0.067024)
(16.8608, -0.187233)
(16.9367, -0.297493)
(17.0127, -0.351014)
(17.0886, -0.284782)
(17.1646, -0.123922)
(17.2405, 0.0591964)
(17.3165, 0.211658)
(17.3924, 0.2777)
(17.4684, 0.233334)
(17.5443, 0.122241)
(17.6203, 0.0164546)
(17.6962, -0.0686166)
(17.7722, -0.118578)
(17.8481, -0.181729)
(17.9241, -0.214877)
(18, -0.164626)
(18.076, -0.061815)
(18.1519, 0.0863642)
(18.2278, 0.205399)
(18.3038, 0.246923)
(18.3797, 0.188215)
(18.4557, 0.0434664)
(18.5316, -0.191897)
(18.6076, -0.350206)
(18.6835, -0.310127)
(18.7595, -0.0551131)
(18.8354, 0.27787)
(18.9114, 0.46501)
(18.9873, 0.386991)
(19.0633, 0.0614894)
(19.1392, -0.379367)
(19.2152, -0.637225)
(19.2911, -0.565611)
(19.3671, -0.222147)
(19.443, 0.170514)
(19.519, 0.484261)
(19.5949, 0.623016)
(19.6709, 0.506655)
(19.7468, 0.262677)
(19.8228, -0.00313274)
(19.8987, -0.221406)
(19.9747, -0.377392)
(20.0506, -0.412358)
(20.1266, -0.289958)
(20.2025, -0.0947667)
(20.2785, 0.107766)
(20.3544, 0.180929)
(20.4304, 0.0638978)
(20.5063, -0.0804019)
(20.5823, -0.219215)
(20.6582, -0.248065)
(20.7342, -0.169642)
(20.8101, 0.000333533)
(20.8861, 0.183146)
(20.962, 0.330252)
(21.038, 0.398191)
(21.1139, 0.323979)
(21.1899, 0.154237)
(21.2658, -0.052522)
(21.3418, -0.134251)
(21.4177, -0.0124543)
(21.4937, 0.155438)
(21.5696, 0.217776)
(21.6456, 0.119037)
(21.7215, -0.0700444)
(21.7975, -0.259166)
(21.8734, -0.325467)
(21.9494, -0.22517)
(22.0253, 0.00582261)
(22.1013, 0.250683)
(22.1772, 0.286384)
(22.2532, 0.184526)
(22.3291, 0.0291958)
(22.4051, -0.0902472)
(22.481, -0.0709086)
(22.557, 0.0468584)
(22.6329, 0.162656)
(22.7089, 0.158785)
(22.7848, 0.0526214)
(22.8608, -0.0533154)
(22.9367, -0.164922)
(23.0127, -0.23347)
(23.0886, -0.204089)
(23.1646, -0.158682)
(23.2405, -0.081593)
(23.3165, -0.0701673)
(23.3924, -0.0383653)
(23.4684, 0.0602211)
(23.5443, 0.163829)
(23.6203, 0.282325)
(23.6962, 0.307965)
(23.7722, 0.189372)
(23.8481, -0.0150617)
(23.9241, -0.149881)
(24, -0.179031)
(24.076, -0.0749729)
(24.1519, 0.114505)
(24.2278, 0.158517)
(24.3038, 0.0996982)
(24.3797, -0.0035325)
(24.4557, -0.0591924)
(24.5316, 0.133298)
(24.6076, 0.137723)
(24.6835, 0.00533918)
(24.7595, -0.0328081)
(24.8354, 0.0155287)
(24.9114, -0.0185511)
(24.9873, -0.006279)
(25.0633, 0.00725569)
(25.1392, 0.00755486)
(25.2152, -0.00833564)
(25.2911, -0.0198093)
(25.3671, -0.0153377)
(25.443, -0.00343996)
(25.519, 0.010284)
(25.5949, 0.0157706)
(25.6709, 0.0136257)
(25.7468, 0.0146574)
(25.8228, 0.0199511)
(25.8987, 0.0343502)
(25.9747, 0.0317685)
(26.0506, 0.0325557)
(26.1266, 0.02289)
(26.2025, 0.0278056)
(26.2785, 0.0201864)
(26.3544, 0.0137333)
(26.4304, 0.0153266)
(26.5063, 0.0126948)
(26.5823, 0.0071583)
(26.6582, 0.00219118)
(26.7342, -0.00480928)
(26.8101, -0.000966339)
(26.8861, 0.020131)
(26.962, 0.0224666)
(27.038, 0.00591744)
(27.1139, -0.000136518)
(27.1899, 0.00798164)
(27.2658, 0.010347)
(27.3418, 0.0117662)
(27.4177, 0.01852)
(27.4937, 0.0370943)
(27.5696, 0.0260385)
(27.6456, 0.0222136)
(27.7215, 0.00500612)
(27.7975, -0.00194497)
(27.8734, -0.00322499)
(27.9494, 0.00476606)
(28.0253, 0.0057535)
(28.1013, 0.00228154)
(28.1772, 0.00557141)
(28.2532, 0.00711555)
(28.3291, 0.00217821)
(28.4051, -0.00295251)
(28.481, -0.00151857)
(28.557, 0.00192557)
(28.6329, -0.0124402)
(28.7089, -0.0189001)
(28.7848, -0.0341049)
(28.8608, -0.0260541)
(28.9367, -0.00165994)
(29.0127, 0.00524274)
(29.0886, -0.0130647)
(29.1646, -0.0110712)
(29.2405, -0.00314981)
(29.3165, -0.00935252)
(29.3924, 0.0033621)
(29.4684, 0.00655487)
(29.5443, 0.0016865)
(29.6203, -0.00554602)
(29.6962, -0.00468466)
(29.7722, -0.00690865)
(29.8481, -0.020092)
(29.9241, -0.0217042)
(30, -0.0159947)
(30.076, -0.0118604)
(30.1519, -0.00867342)
(30.2278, -0.00312201)
(30.3038, 0.00553237)
(30.3797, 0.00676846)
(30.4557, 0.0165133)
(30.5316, 0.0276316)
(30.6076, 0.029769)
(30.6835, 0.00133545)
(30.7595, -0.00579251)
(30.8354, -0.00185148)
(30.9114, -0.00419084)
(30.9873, -0.00383972)
(31.0633, -0.00341841)
(31.1392, -0.00415538)
(31.2152, 0.00752279)
(31.2911, 0.0108329)
(31.3671, 0.0108109)
(31.443, -0.00184309)
(31.519, -0.0139782)
(31.5949, -0.0139216)
(31.6709, -0.0159837)
(31.7468, -0.0158605)
(31.8228, -0.0137735)
(31.8987, -0.0147785)
(31.9747, -0.0224626)
(32.0506, -0.00900306)
};

==> exp_plots/constrained_ws/az_des.tex <==
\addplot[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates {
(0, 0)
(0.0759494, -0.00124221)
(0.151899, -0.0038986)
(0.227848, -0.00421314)
(0.303797, -0.00719155)
(0.379747, -0.00491799)
(0.455696, 0.00252226)
(0.531646, 0.00911956)
(0.607595, 0.0146376)
(0.683544, 0.0161779)
(0.759494, 0.00401379)
(0.835443, -0.000876467)
(0.911392, -0.00208874)
(0.987342, -0.00846303)
(1.06329, -0.0233622)
(1.13924, 0.191387)
(1.21519, 0.316527)
(1.29114, 0.393194)
(1.36709, 0.429311)
(1.44304, 0.430279)
(1.51899, 0.429035)
(1.59494, 0.432232)
(1.67089, 0.438326)
(1.74684, 0.439381)
(1.82278, 0.429915)
(1.89873, 0.418983)
(1.97468, 0.410391)
(2.05063, 0.408047)
(2.12658, 0.413911)
(2.20253, 0.42936)
(2.27848, 0.452873)
(2.35443, 0.437141)
(2.43038, 0.43503)
(2.50633, 0.440192)
(2.58228, 0.480533)
(2.65823, 0.493328)
(2.73418, 0.44578)
(2.81013, 0.376299)
(2.88608, 0.30905)
(2.96203, 0.23715)
(3.03797, 0.179256)
(3.11392, 0.124993)
(3.18987, 0.000331506)
(3.26582, -0.107324)
(3.34177, -0.149345)
(3.41772, -0.113416)
(3.49367, -0.0488727)
(3.56962, 0.0614188)
(3.64557, 0.143466)
(3.72152, 0.165014)
(3.79747, 0.133589)
(3.87342, 0.0833886)
(3.94937, -0.0391067)
(4.02532, -0.0880377)
(4.10127, -0.0443031)
(4.17722, 0.00415116)
(4.25316, 0.0394311)
(4.32911, 0.0638232)
(4.40506, 0.0567321)
(4.48101, 0.0551467)
(4.55696, 0.0636757)
(4.63291, 0.0808605)
(4.70886, 0.094625)
(4.78481, 0.105265)
(4.86076, 0.0642282)
(4.93671, 0.0488345)
(5.01266, 0.0467322)
(5.08861, -0.0393879)
(5.16456, -0.0457663)
(5.24051, 0.0174162)
(5.31646, 0.0845949)
(5.39241, 0.148686)
(5.46835, 0.155731)
(5.5443, 0.145513)
(5.62025, 0.134768)
(5.6962, 0.108407)
(5.77215, 0.0266951)
(5.8481, -0.0322755)
(5.92405, -0.0811968)
(6, -0.0795686)
(6.07595, -0.0258495)
(6.1519, 0.072007)
(6.22785, 0.142338)
(6.3038, 0.149617)
(6.37975, 0.0729701)
(6.4557, -0.00999828)
(6.53165, -0.0408278)
(6.60759, -0.051694)
(6.68354, -0.0299357)
(6.75949, 0.0328209)
(6.83544, 0.0882916)
(6.91139, 0.10239)
(6.98734, 0.103714)
(7.06329, 0.0879268)
(7.13924, 0.10031)
(7.21519, -0.0304467)
(7.29114, -0.113756)
(7.36709, -0.163823)
(7.44304, -0.237671)
(7.51899, -0.279894)
(7.59494, -0.259463)
(7.67089, -0.241633)
(7.74684, -0.177477)
(7.82278, -0.119293)
(7.89873, -0.107119)
(7.97468, -0.108921)
(8.05063, -0.0664999)
(8.12658, -0.0389305)
(8.20253, -0.039414)
(8.27848, -0.086011)
(8.35443, -0.128225)
(8.43038, -0.147653)
(8.50633, -0.136493)
(8.58228, -0.103344)
(8.65823, -0.054424)
(8.73418, -0.0114324)
(8.81013, 0.105153)
(8.88608, 0.170991)
(8.96203, 0.18836)
(9.03798, 0.189102)
(9.11392, 0.168287)
(9.18987, 0.13437)
(9.26582, 0.0654156)
(9.34177, -0.014595)
(9.41772, -0.044136)
(9.49367, -0.0168907)
(9.56962, 0.0214498)
(9.64557, 0.0721423)
(9.72152, 0.102888)
(9.79747, 0.105647)
(9.87342, 0.083422)
(9.94937, 0.0554757)
(10.0253, 0.0378431)
(10.1013, 0.0329394)
(10.1772, 0.0542262)
(10.2532, 0.0791979)
(10.3291, 0.0966975)
(10.4051, 0.111423)
(10.481, 0.109387)
(10.557, 0.057878)
(10.6329, 0.0215771)
(10.7089, 0.00890371)
(10.7848, 0.0195948)
(10.8608, 0.0469313)
(10.9367, 0.0763025)
(11.0127, 0.0645031)
(11.0886, 0.00104749)
(11.1646, -0.0945187)
(11.2405, -0.142064)
(11.3165, -0.17451)
(11.3924, -0.175034)
(11.4684, -0.120906)
(11.5443, -0.0483216)
(11.6203, 0.0129703)
(11.6962, 0.10481)
(11.7722, 0.132876)
(11.8481, 0.0991505)
(11.9241, 0.0503518)
(12, -0.0184363)
(12.0759, -0.0812726)
(12.1519, -0.0826945)
(12.2278, -0.068428)
(12.3038, -0.029713)
(12.3797, 0.0240449)
(12.4557, 0.0657034)
(12.5316, 0.0821481)
(12.6076, 0.076425)
(12.6835, 0.020343)
(12.7595, -0.0570651)
(12.8354, -0.157501)
(12.9114, -0.18848)
(12.9873, -0.132345)
(13.0633, -0.0667926)
(13.1392, 0.00172579)
(13.2152, 0.0457022)
(13.2911, 0.0463431)
(13.3671, 0.039084)
(13.443, 0.0314697)
(13.519, 0.0404228)
(13.5949, 0.0611725)
(13.6709, 0.0496767)
(13.7468, 0.010837)
(13.8228, -0.0201128)
(13.8987, -0.0291063)
(13.9747, -0.0181777)
(14.0506, -0.050698)
(14.1266, -0.0650432)
(14.2025, -0.0330492)
(14.2785, 0.0601261)
(14.3544, 0.159717)
(14.4304, 0.204428)
(14.5063, 0.180742)
(14.5823, 0.120455)
(14.6582, -0.0402139)
(14.7342, -0.103702)
(14.8101, -0.103564)
(14.8861, -0.0773578)
(14.962, -0.0267363)
(15.038, 0.0139373)
(15.1139, 0.00733971)
(15.1899, -0.0196859)
(15.2658, -0.0314365)
(15.3418, -0.0522779)
(15.4177, -0.0971081)
(15.4937, -0.107428)
(15.5696, -0.118064)
(15.6456, -0.11678)
(15.7215, -0.0989115)
(15.7975, -0.0606305)
(15.8734, -0.026441)
(15.9494, -0.00254038)
(16.0253, 0.0083731)
(16.1013, 0.0236032)
(16.1772, 0.0349594)
(16.2532, 0.0696487)
(16.3291, 0.0871716)
(16.4051, 0.084234)
(16.481, 0.0588708)
(16.557, 0.0100388)
(16.6329, -0.026111)
(16.7089, -0.0359038)
(16.7848, -0.0368442)
(16.8608, -0.0276513)
(16.9367, -0.00935988)
(17.0127, 0.0348367)
(17.0886, -0.00782325)
(17.1646, -0.042057)
(17.2405, -0.0486514)
(17.3165, 0.0101245)
(17.3924, 0.0316791)
(17.4684, 0.00547701)
(17.5443, -0.0437193)
(17.6203, -0.0906267)
(17.6962, -0.121871)
(17.7722, -0.114973)
(17.8481, -0.0893715)
(17.9241, -0.0536505)
(18, -0.043698)
(18.076, -0.0417788)
(18.1519, -0.0469787)
(18.2278, -0.0387994)
(18.3038, -0.0476122)
(18.3797, -0.0661312)
(18.4557, -0.0800632)
(18.5316, -0.0529263)
(18.6076, 0.0181168)
(18.6835, 0.0869762)
(18.7595, 0.108662)
(18.8354, 0.0768512)
(18.9114, 0.00590653)
(18.9873, -0.126665)
(19.0633, -0.200889)
(19.1392, -0.172092)
(19.2152, -0.0963583)
(19.2911, -0.017977)
(19.3671, 0.0994308)
(19.443, 0.211022)
(19.519, 0.200678)
(19.5949, 0.118265)
(19.6709, 0.0147039)
(19.7468, -0.138711)
(19.8228, -0.257664)
(19.8987, -0.255892)
(19.9747, -0.204616)
(20.0506, -0.158648)
(20.1266, -0.105807)
(20.2025, -0.0838776)
(20.2785, -0.0803452)
(20.3544, -0.0538154)
(20.4304, -0.0268289)
(20.5063, 0.00720721)
(20.5823, 0.0387452)
(20.6582, 0.0504331)
(20.7342, 0.0854914)
(20.8101, 0.176904)
(20.8861, 0.210047)
(20.962, 0.185393)
(21.038, 0.110094)
(21.1139, 0.0370646)
(21.1899, 0.00840433)
(21.2658, 0.0140068)
(21.3418, 0.0284127)
(21.4177, 0.0404773)
(21.4937, 0.0236868)
(21.5696, 0.0129605)
(21.6456, 0.0232689)
(21.7215, 0.014573)
(21.7975, 0.00482216)
(21.8734, 0.0273207)
(21.9494, 0.0439309)
(22.0253, 0.0334461)
(22.1013, 0.0322131)
(22.1772, -0.00180085)
(22.2532, -0.0400973)
(22.3291, -0.0496016)
(22.4051, -0.0375352)
(22.481, -0.0153536)
(22.557, 0.00265309)
(22.6329, 0.000104209)
(22.7089, -0.0279077)
(22.7848, -0.088336)
(22.8608, -0.155904)
(22.9367, -0.182877)
(23.0127, -0.164708)
(23.0886, -0.143386)
(23.1646, -0.077416)
(23.2405, 0.0222294)
(23.3165, 0.0995684)
(23.3924, 0.105989)
(23.4684, 0.120133)
(23.5443, 0.0906363)
(23.6203, 0.0383149)
(23.6962, -0.0109741)
(23.7722, -0.0617514)
(23.8481, -0.112516)
(23.9241, -0.100126)
(24, -0.0345465)
(24.076, 0.0237199)
(24.1519, 0.0355832)
(24.2278, 0.00927098)
(24.3038, -0.0332017)
(24.3797, -0.068992)
(24.4557, -0.0803715)
(24.5316, -0.103058)
(24.6076, -0.155496)
(24.6835, -0.195294)
(24.7595, -0.204422)
(24.8354, -0.211442)
(24.9114, -0.19043)
(24.9873, -0.183088)
(25.0633, -0.226519)
(25.1392, -0.199816)
(25.2152, -0.181845)
(25.2911, -0.185407)
(25.3671, -0.204075)
(25.443, -0.221622)
(25.519, -0.246407)
(25.5949, -0.257072)
(25.6709, -0.248849)
(25.7468, -0.24805)
(25.8228, -0.266427)
(25.8987, -0.248223)
(25.9747, -0.228995)
(26.0506, -0.226231)
(26.1266, -0.223311)
(26.2025, -0.187867)
(26.2785, -0.179654)
(26.3544, -0.178445)
(26.4304, -0.188522)
(26.5063, -0.206674)
(26.5823, -0.236843)
(26.6582, -0.256497)
(26.7342, -0.267414)
(26.8101, -0.269676)
(26.8861, -0.267748)
(26.962, -0.266776)
(27.038, -0.268406)
(27.1139, -0.259435)
(27.1899, -0.258857)
(27.2658, -0.25709)
(27.3418, -0.244437)
(27.4177, -0.247515)
(27.4937, -0.268039)
(27.5696, -0.271218)
(27.6456, -0.264853)
(27.7215, -0.257267)
(27.7975, -0.247639)
(27.8734, -0.244637)
(27.9494, -0.250305)
(28.0253, -0.268342)
(28.1013, -0.286381)
(28.1772, -0.296624)
(28.2532, -0.303245)
(28.3291, -0.307269)
(28.4051, -0.306124)
(28.481, -0.302389)
(28.557, -0.300249)
(28.6329, -0.2998)
(28.7089, -0.298383)
(28.7848, -0.300472)
(28.8608, -0.29845)
(28.9367, -0.306634)
(29.0127, -0.309844)
(29.0886, -0.297129)
(29.1646, -0.300742)
(29.2405, -0.306859)
(29.3165, -0.309201)
(29.3924, -0.313078)
(29.4684, -0.319421)
(29.5443, -0.319248)
(29.6203, -0.304485)
(29.6962, -0.304533)
(29.7722, -0.307715)
(29.8481, -0.309958)
(29.9241, -0.310472)
(30, -0.305362)
(30.076, -0.301752)
(30.1519, -0.303139)
(30.2278, -0.309025)
(30.3038, -0.327499)
(30.3797, -0.360652)
(30.4557, -0.376824)
(30.5316, -0.376707)
(30.6076, -0.376559)
(30.6835, -0.368668)
(30.7595, -0.355676)
(30.8354, -0.347227)
(30.9114, -0.342608)
(30.9873, -0.342992)
(31.0633, -0.347923)
(31.1392, -0.355063)
(31.2152, -0.36235)
(31.2911, -0.362726)
(31.3671, -0.364464)
(31.443, -0.35683)
(31.519, -0.349928)
(31.5949, -0.346504)
(31.6709, -0.347075)
(31.7468, -0.359901)
(31.8228, -0.378343)
(31.8987, -0.374233)
(31.9747, -0.366574)
(32.0506, -0.368938)
};

==> exp_plots/constrained_ws/plot.tex <==
%%    
\begin{figure}[t]
\centering

\begin{tikzpicture}


\FPeval{\xshfta}{0}
\FPeval{\xshftb}{0}
\FPeval{\xshftc}{0}
\FPeval{\xshftd}{0}



\FPeval{\yshfta}{0-0}
\FPeval{\yshftb}{0-9}
\FPeval{\yshftc}{0-18}
\FPeval{\yshftd}{0-27.9}


\FPeval{\pltw}{110}
\FPeval{\plth}{24}

\FPeval{\scal}{0.5}


\FPeval{\mrksize}{0.3}

%
\colorlet{desclr}{white!0!magenta}
\colorlet{currclr}{blue!60!green}

\colorlet{gridclr}{white!85!black}
\colorlet{dlegendclr}{white!80!black}
\colorlet{axisclr}{white!75!black}
\colorlet{axisbgclr}{white!99!black}

\colorlet{dlegendclr}{white!80!black}
\colorlet{legendclr}{white!100!black}






\FPeval{\lscale}{0.6}
\FPeval{\limscale}{0.5}
\FPeval{\lxshft}{95.5}
\FPeval{\lyshft}{9.0}

  
\FPeval{\titlescale}{0.7}
\FPeval{\titlexshift}{21.0}
\FPeval{\titleyshift}{13.7}

\colorlet{gpudclr}{white!80!black}
\colorlet{gpuclr}{white!90!black}
\colorlet{gputxtclr}{white!0!black}

\FPeval{\labelscale}{1.0}
\FPeval{\ticklabelscale}{0.9}

\FPeval{\xlabelxshift}{0+15}
\FPeval{\xlabelyshift}{0+0.5}
\FPeval{\ylabelxshift}{0+4.0}
\FPeval{\ylabelyshift}{0+6.2}


\FPeval{\linew}{1.5}
\FPeval{\dashon}{5.0}
\FPeval{\dashoff}{3.0}

\FPeval{\xshfttakeoff}{0-16}
\FPeval{\xshfthover}{0}
\FPeval{\xshftland}{16}
%
%
\node (a) [xshift = \xshfta ex, yshift=\yshfta ex, scale=\scal]{
\tikz{
%
\pgfplotsset{width=\pltw ex, height=\plth ex}
\begin{axis}[
   axis background style={fill=axisbgclr},
    title={},
    xlabel={},
    ylabel={ X (m)},
    xmin=0, xmax=28,
    ymin=-1, ymax=1,
    xtick={0, 8, 16, 24, 32},
    ytick={-0.5, 0, 0.5},
    xticklabels={$0$, $8$, $16$, $24$, $32$},
    yticklabels={$-1$, $0$, $1$},
     axis line style={axisclr},
    legend image post style={scale =\limscale},
    legend style={at={(\lxshft ex,\lyshft ex)},anchor=south, legend columns = 1, draw = {dlegendclr}, fill={legendclr}, nodes={scale=\lscale}},
    ymajorgrids=true, 
    xmajorgrids=true,
    grid style={dashed, gridclr},
    major tick length=1ex,
    x label style={at={(\xlabelxshift ex, \xlabelyshift ex)},scale=\labelscale},
    y label style={at={(\ylabelxshift ex, \ylabelyshift ex)},scale=\labelscale},
    xticklabel style={scale=\ticklabelscale},
    yticklabel style={scale=\ticklabelscale},
%    ybar,
%    bar width = 4pt,
]
%
%
\input{exp_plots/constrained_ws/x_des}
%
\input{exp_plots/constrained_ws/x}
%
%
%%   
  \legend{Ref, SLAM}
  %
\end{axis}
%
% \node [draw=gpudclr,fill=gpuclr,rounded corners=0.2ex, minimum width=10.0ex, xshift=\titlexshift ex, yshift=\titleyshift ex, scale=\titlescale]{\textcolor{gputxtclr}{\textbf{Step-X}}};
}};
%
%    
%
%
\node (b) [xshift = \xshftb ex, yshift=\yshftb ex, scale=\scal]{
\tikz{
%
\pgfplotsset{width=\pltw ex, height=\plth ex}
\begin{axis}[
   axis background style={fill=axisbgclr},
    title={},
    xlabel={},
    ylabel={ Y (m)},
    xmin=0, xmax=28,
    ymin=-1, ymax=1,
    xtick={0, 8, 16, 24, 32},
    ytick={-1, 0, 1},
    xticklabels={$0$, $8$, $16$, $24$, $32$},
    yticklabels={$-1$, $0$, $1$},
     axis line style={axisclr},
    legend image post style={scale =\limscale},
    legend style={at={(\lxshft ex,\lyshft ex)},anchor=south, legend columns = 1, draw = {dlegendclr}, fill={legendclr}, nodes={scale=\lscale}},
    ymajorgrids=true, 
    xmajorgrids=true,
    grid style={dashed, gridclr},
    major tick length=1ex,
    x label style={at={(\xlabelxshift ex, \xlabelyshift ex)},scale=\labelscale},
    y label style={at={(\ylabelxshift ex, \ylabelyshift ex)},scale=\labelscale},
    xticklabel style={scale=\ticklabelscale},
    yticklabel style={scale=\ticklabelscale},
%    ybar,
%    bar width = 4pt,
]
%
\input{exp_plots/constrained_ws/y}
%
%
\input{exp_plots/constrained_ws/y_des}
%
%% 
  \legend{Ref, SLAM}
  %
\end{axis}
%
% \node [draw=gpudclr,fill=gpuclr,rounded corners=0.2ex, minimum width=10.0ex, xshift=\titlexshift ex, yshift=\titleyshift ex, scale=\titlescale]{\textcolor{gputxtclr}{\textbf{Step-X}}};
}};
%
% 
%
\node (c) [xshift = \xshftc ex, yshift=\yshftc ex, scale=\scal]{
\tikz{
%
\pgfplotsset{width=\pltw ex, height=\plth ex}
\begin{axis}[
   axis background style={fill=axisbgclr},
    title={},
    xlabel={},
    ylabel={ Z (m)},
    xmin=0, xmax=28,
    ymin=-1, ymax=1,
    xtick={0, 8, 16, 24, 32},
    ytick={-1, 0, 1},
    xticklabels={$0$, $8$, $16$, $24$, $32$},
    yticklabels={$-1$, $0$, $1$},
     axis line style={axisclr},
    legend image post style={scale =\limscale},
    legend style={at={(\lxshft ex,\lyshft ex)},anchor=south, legend columns = 1, draw = {dlegendclr}, fill={legendclr}, nodes={scale=\lscale}},
    ymajorgrids=true, 
    xmajorgrids=true,
    grid style={dashed, gridclr},
    major tick length=1ex,
    x label style={at={(\xlabelxshift ex, \xlabelyshift ex)},scale=\labelscale},
    y label style={at={(\ylabelxshift ex, \ylabelyshift ex)},scale=\labelscale},
    xticklabel style={scale=\ticklabelscale},
    yticklabel style={scale=\ticklabelscale},
%    ybar,
%    bar width = 4pt,
]
%
\input{exp_plots/constrained_ws/z}
%
%
\input{exp_plots/constrained_ws/z_des}
%
%% 
  \legend{Ref, SLAM}
  %
\end{axis}
%
% \node [draw=gpudclr,fill=gpuclr,rounded corners=0.2ex, minimum width=10.0ex, xshift=\titlexshift ex, yshift=\titleyshift ex, scale=\titlescale]{\textcolor{gputxtclr}{\textbf{Step-X}}};
}};
%
% 
%
\node (d) [xshift = \xshftd ex, yshift=\yshftd ex, scale=\scal]{
\tikz{
%
\pgfplotsset{width=\pltw ex, height=\plth ex}
\begin{axis}[
   axis background style={fill=axisbgclr},
    title={},
    xlabel={Time (s)},
    ylabel={ Yaw ($^\text{o}$)},
    xmin=0, xmax=28,
    ymin=-30, ymax=30,
    xtick={0, 8, 16, 24, 32},
    ytick={-1, 0, 1},
    xticklabels={$0$, $8$, $16$, $24$, $32$},
    yticklabels={$-30$, $0$, $30$},
     axis line style={axisclr},
    legend image post style={scale =\limscale},
    legend style={at={(\lxshft ex,\lyshft ex)},anchor=south, legend columns = 1, draw = {dlegendclr}, fill={legendclr}, nodes={scale=\lscale}},
    ymajorgrids=true, 
    xmajorgrids=true,
    grid style={dashed, gridclr},
    major tick length=1ex,
    x label style={at={(\xlabelxshift ex, \xlabelyshift ex)},scale=\labelscale},
    y label style={at={(\ylabelxshift ex, \ylabelyshift ex)},scale=\labelscale},
    xticklabel style={scale=\ticklabelscale},
    yticklabel style={scale=\ticklabelscale},
%    ybar,
%    bar width = 4pt,
]
%
\input{exp_plots/constrained_ws/yaw}
%
%
%
\input{exp_plots/constrained_ws/yaw_des}
%
%% 
  \legend{Ref, SLAM}
  %
\end{axis}
%
% \node [draw=gpudclr,fill=gpuclr,rounded corners=0.2ex, minimum width=10.0ex, xshift=\titlexshift ex, yshift=\titleyshift ex, scale=\titlescale]{\textcolor{gputxtclr}{\textbf{Step-X}}};
}};
%
% 
%
%
\node (t) [xshift=\xshfttakeoff ex, yshift=5 ex]{\scriptsize Takeoff};
\node (h) [xshift=\xshfthover ex, yshift=5 ex]{\scriptsize Hover};
\node (l) [xshift=\xshftland ex, yshift=5 ex]{\scriptsize Land};
%%
%
 
\end{tikzpicture}
%
%
\caption{Takeoff-Hover-Land performance in constrained workspace.}
%
\label{fig:constrndwsTHL}
%
%\vspace{-3ex}
\end{figure}
%
%
%
%%


==> exp_plots/constrained_ws/thrust.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0)
(0.0759494, 10)
(0.151899, 10.0267)
(0.227848, 10.0074)
(0.303797, 10.0024)
(0.379747, 10.1269)
(0.455696, 10.3448)
(0.531646, 10.5542)
(0.607595, 10.744)
(0.683544, 10.5162)
(0.759494, 10.4034)
(0.835443, 10.2353)
(0.911392, 10.1771)
(0.987342, 10.1465)
(1.06329, 10)
(1.13924, 13.7695)
(1.21519, 15.6966)
(1.29114, 16.6916)
(1.36709, 18.1917)
(1.44304, 19.9313)
(1.51899, 21.547)
(1.59494, 22.7526)
(1.67089, 24.5209)
(1.74684, 26.1403)
(1.82278, 27.3747)
(1.89873, 28.545)
(1.97468, 29.828)
(2.05063, 31.5719)
(2.12658, 33.043)
(2.20253, 34.456)
(2.27848, 35.9212)
(2.35443, 36.8659)
(2.43038, 37.8585)
(2.50633, 39.3724)
(2.58228, 41.1792)
(2.65823, 42.2836)
(2.73418, 42.3499)
(2.81013, 41.2178)
(2.88608, 40.0527)
(2.96203, 39.5136)
(3.03797, 39.5626)
(3.11392, 40.4276)
(3.18987, 40.5712)
(3.26582, 39.2738)
(3.34177, 39.3019)
(3.41772, 40.6572)
(3.49367, 42.423)
(3.56962, 44.2461)
(3.64557, 44.3962)
(3.72152, 43.0268)
(3.79747, 41.1123)
(3.87342, 39.3165)
(3.94937, 38.3995)
(4.02532, 40.3868)
(4.10127, 43.1634)
(4.17722, 45.5131)
(4.25316, 44.984)
(4.32911, 43.3247)
(4.40506, 41.4678)
(4.48101, 41.3702)
(4.55696, 43.4263)
(4.63291, 45.2982)
(4.70886, 45.4956)
(4.78481, 44.9719)
(4.86076, 43.6199)
(4.93671, 42.4389)
(5.01266, 42.2235)
(5.08861, 42.4568)
(5.16456, 42.985)
(5.24051, 44.3089)
(5.31646, 45.1202)
(5.39241, 45.8365)
(5.46835, 45.164)
(5.5443, 45.0008)
(5.62025, 44.6772)
(5.6962, 44.1932)
(5.77215, 42.7678)
(5.8481, 42.5147)
(5.92405, 42.5888)
(6, 43.8659)
(6.07595, 45.9229)
(6.1519, 47.2194)
(6.22785, 47.164)
(6.3038, 46.6102)
(6.37975, 45.1552)
(6.4557, 43.1362)
(6.53165, 43.3021)
(6.60759, 43.9869)
(6.68354, 45.5992)
(6.75949, 47.1818)
(6.83544, 48.4451)
(6.91139, 48.9914)
(6.98734, 49.3545)
(7.06329, 47.9777)
(7.13924, 46.2863)
(7.21519, 45.0319)
(7.29114, 43.7639)
(7.36709, 44.1944)
(7.44304, 44.7674)
(7.51899, 44.8796)
(7.59494, 44.7641)
(7.67089, 44.9323)
(7.74684, 44.2231)
(7.82278, 43.8349)
(7.89873, 43.8628)
(7.97468, 44.0679)
(8.05063, 44.5192)
(8.12658, 45.151)
(8.20253, 45.2906)
(8.27848, 45.2752)
(8.35443, 45.0321)
(8.43038, 44.0762)
(8.50633, 43.7356)
(8.58228, 44.5017)
(8.65823, 45.7204)
(8.73418, 46.9239)
(8.81013, 48.1873)
(8.88608, 48.2345)
(8.96203, 47.6188)
(9.03798, 47.2562)
(9.11392, 46.4533)
(9.18987, 45.4891)
(9.26582, 44.2923)
(9.34177, 43.517)
(9.41772, 44.3806)
(9.49367, 46.4081)
(9.56962, 48.1343)
(9.64557, 48.7382)
(9.72152, 48.2252)
(9.79747, 47.0985)
(9.87342, 46.4327)
(9.94937, 46.1035)
(10.0253, 46.0487)
(10.1013, 46.1067)
(10.1772, 46.4018)
(10.2532, 46.7921)
(10.3291, 46.9983)
(10.4051, 46.6379)
(10.481, 45.9718)
(10.557, 44.9605)
(10.6329, 44.6945)
(10.7089, 45.4041)
(10.7848, 46.6718)
(10.8608, 48.183)
(10.9367, 48.1951)
(11.0127, 47.2766)
(11.0886, 45.2489)
(11.1646, 43.2009)
(11.2405, 42.5201)
(11.3165, 43.4096)
(11.3924, 45.1008)
(11.4684, 47.2864)
(11.5443, 48.6413)
(11.6203, 48.6514)
(11.6962, 48.2096)
(11.7722, 47.1716)
(11.8481, 46.121)
(11.9241, 44.9544)
(12, 44.4802)
(12.0759, 45.3037)
(12.1519, 47.2511)
(12.2278, 48.5493)
(12.3038, 49.2075)
(12.3797, 49.1501)
(12.4557, 48.2153)
(12.5316, 46.826)
(12.6076, 45.5265)
(12.6835, 44.4481)
(12.7595, 44.8027)
(12.8354, 45.7201)
(12.9114, 45.9832)
(12.9873, 46.8731)
(13.0633, 46.8758)
(13.1392, 47.038)
(13.2152, 46.1595)
(13.2911, 44.9125)
(13.3671, 44.3982)
(13.443, 44.8502)
(13.519, 47.5458)
(13.5949, 46.5755)
(13.6709, 46.3082)
(13.7468, 44.9724)
(13.8228, 44.7665)
(13.8987, 46.0593)
(13.9747, 47.4592)
(14.0506, 49.0526)
(14.1266, 49.4152)
(14.2025, 50.0732)
(14.2785, 50.349)
(14.3544, 49.0744)
(14.4304, 47.8703)
(14.5063, 45.9169)
(14.5823, 44.8835)
(14.6582, 43.5199)
(14.7342, 44.5686)
(14.8101, 46.9371)
(14.8861, 48.1792)
(14.962, 47.9643)
(15.038, 47.1195)
(15.1139, 45.2779)
(15.1899, 44.0987)
(15.2658, 44.4476)
(15.3418, 45.2215)
(15.4177, 45.0125)
(15.4937, 44.9481)
(15.5696, 44.5493)
(15.6456, 44.4776)
(15.7215, 44.9233)
(15.7975, 45.8585)
(15.8734, 47.4067)
(15.9494, 47.9801)
(16.0253, 48.4913)
(16.1013, 48.2785)
(16.1772, 47.5657)
(16.2532, 47.1208)
(16.3291, 47.3827)
(16.4051, 47.3796)
(16.481, 46.184)
(16.557, 45.0935)
(16.6329, 44.5739)
(16.7089, 45.0815)
(16.7848, 46.1602)
(16.8608, 47.0594)
(16.9367, 48.7194)
(17.0127, 50.3952)
(17.0886, 51.4725)
(17.1646, 50.2714)
(17.2405, 48.8224)
(17.3165, 48.3559)
(17.3924, 47.329)
(17.4684, 46.545)
(17.5443, 46.5432)
(17.6203, 46.6174)
(17.6962, 46.7816)
(17.7722, 47.023)
(17.8481, 47.8657)
(17.9241, 48.9964)
(18, 48.9542)
(18.076, 48.0479)
(18.1519, 46.8986)
(18.2278, 45.7829)
(18.3038, 44.5426)
(18.3797, 44.1543)
(18.4557, 44.6839)
(18.5316, 47.0049)
(18.6076, 49.5638)
(18.6835, 50.5346)
(18.7595, 48.957)
(18.8354, 45.3593)
(18.9114, 42.9457)
(18.9873, 41.2061)
(19.0633, 42.2148)
(19.1392, 46.8496)
(19.2152, 50.2805)
(19.2911, 51.477)
(19.3671, 50.7441)
(19.443, 49.7142)
(19.519, 47.4861)
(19.5949, 44.4316)
(19.6709, 43.2991)
(19.7468, 42.956)
(19.8228, 42.9909)
(19.8987, 44.1764)
(19.9747, 45.9661)
(20.0506, 46.9389)
(20.1266, 46.8143)
(20.2025, 45.473)
(20.2785, 43.4506)
(20.3544, 42.4248)
(20.4304, 43.5304)
(20.5063, 45.1992)
(20.5823, 46.716)
(20.6582, 47.5461)
(20.7342, 47.9153)
(20.8101, 47.4454)
(20.8861, 46.9961)
(20.962, 45.4651)
(21.038, 43.7116)
(21.1139, 43.1883)
(21.1899, 43.8994)
(21.2658, 45.8294)
(21.3418, 46.3117)
(21.4177, 45.1094)
(21.4937, 43.0456)
(21.5696, 42.094)
(21.6456, 43.001)
(21.7215, 44.7282)
(21.7975, 46.349)
(21.8734, 47.7196)
(21.9494, 47.7729)
(22.0253, 46.0845)
(22.1013, 43.4352)
(22.1772, 42.8069)
(22.2532, 42.7946)
(22.3291, 43.8265)
(22.4051, 44.1867)
(22.481, 44.1982)
(22.557, 42.9449)
(22.6329, 42.0381)
(22.7089, 41.4821)
(22.7848, 41.6654)
(22.8608, 41.579)
(22.9367, 41.7944)
(23.0127, 42.8158)
(23.0886, 42.7444)
(23.1646, 42.9951)
(23.2405, 43.5974)
(23.3165, 44.9786)
(23.3924, 44.9294)
(23.4684, 44.3613)
(23.5443, 43.335)
(23.6203, 41.5005)
(23.6962, 40.2046)
(23.7722, 39.9899)
(23.8481, 40.8521)
(23.9241, 42.0085)
(24, 42.3979)
(24.076, 42.2748)
(24.1519, 40.6547)
(24.2278, 39.9966)
(24.3038, 40.2038)
(24.3797, 40.4685)
(24.4557, 40.7037)
(24.5316, 37.0511)
(24.6076, 35.4267)
(24.6835, 36.4151)
(24.7595, 37.2282)
(24.8354, 34.4696)
(24.9114, 34.1114)
(24.9873, 33.802)
(25.0633, 32.4894)
(25.1392, 31.6398)
(25.2152, 31.4247)
(25.2911, 31.0139)
(25.3671, 30.1564)
(25.443, 29.0875)
(25.519, 28.1135)
(25.5949, 27.0538)
(25.6709, 26.5215)
(25.7468, 25.5031)
(25.8228, 24.2295)
(25.8987, 23.2733)
(25.9747, 22.7137)
(26.0506, 21.6573)
(26.1266, 20.9723)
(26.2025, 20.2537)
(26.2785, 19.5907)
(26.3544, 18.9095)
(26.4304, 18.1477)
(26.5063, 17.312)
(26.5823, 16.2223)
(26.6582, 15.4093)
(26.7342, 14.4885)
(26.8101, 13.424)
(26.8861, 12.3132)
(26.962, 11.4001)
(27.038, 10.6199)
(27.1139, 10)
(27.1899, 10)
(27.2658, 10)
(27.3418, 10)
(27.4177, 10)
(27.4937, 10)
(27.5696, 10)
(27.6456, 10)
(27.7215, 10)
(27.7975, 10)
(27.8734, 10)
(27.9494, 10)
(28.0253, 10)
(28.1013, 10)
(28.1772, 10)
(28.2532, 10)
(28.3291, 10)
(28.4051, 10)
(28.481, 10)
(28.557, 10)
(28.6329, 10)
(28.7089, 10)
(28.7848, 10)
(28.8608, 10)
(28.9367, 10)
(29.0127, 10)
(29.0886, 10)
(29.1646, 10)
(29.2405, 10)
(29.3165, 10)
(29.3924, 10)
(29.4684, 10)
(29.5443, 10)
(29.6203, 10)
(29.6962, 10)
(29.7722, 10)
(29.8481, 10)
(29.9241, 10)
(30, 10)
(30.076, 10)
(30.1519, 10)
(30.2278, 10)
(30.3038, 10)
(30.3797, 10)
(30.4557, 10)
(30.5316, 10)
(30.6076, 10)
(30.6835, 10)
(30.7595, 10)
(30.8354, 10)
(30.9114, 10)
(30.9873, 10)
(31.0633, 10)
(31.1392, 10)
(31.2152, 10)
(31.2911, 10)
(31.3671, 10)
(31.443, 10)
(31.519, 10)
(31.5949, 10)
(31.6709, 10)
(31.7468, 10)
(31.8228, 10)
(31.8987, 10)
(31.9747, 10)
(32.0506, 10)
};

==> exp_plots/constrained_ws/x.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0)
(0.0759494, 0.000101239)
(0.151899, -9.24942e-05)
(0.227848, 0.000150503)
(0.303797, 0.000319523)
(0.379747, -0.000386219)
(0.455696, -0.000473289)
(0.531646, -0.00047636)
(0.607595, -0.000820267)
(0.683544, -0.00084717)
(0.759494, -0.000938196)
(0.835443, -0.000495293)
(0.911392, -0.000172369)
(0.987342, -0.000380995)
(1.06329, -0.000716427)
(1.13924, -0.000623753)
(1.21519, -0.000981581)
(1.29114, -0.0015712)
(1.36709, -0.00129485)
(1.44304, -0.00144904)
(1.51899, -0.0013774)
(1.59494, -0.000420017)
(1.67089, -0.000829021)
(1.74684, -0.00168274)
(1.82278, -0.000905574)
(1.89873, 8.66616e-05)
(1.97468, -0.000316736)
(2.05063, -0.00063437)
(2.12658, 0.000340426)
(2.20253, 0.000889308)
(2.27848, 0.000477743)
(2.35443, 4.66092e-05)
(2.43038, 0.000744283)
(2.50633, -0.000387646)
(2.58228, -0.00139821)
(2.65823, 0.00190617)
(2.73418, 0.00356289)
(2.81013, 0.00373326)
(2.88608, 0.00101636)
(2.96203, -0.00529277)
(3.03797, -0.0109387)
(3.11392, -0.0244766)
(3.18987, -0.0400335)
(3.26582, -0.0475538)
(3.34177, -0.0604434)
(3.41772, -0.0725463)
(3.49367, -0.0806266)
(3.56962, -0.0862673)
(3.64557, -0.0883807)
(3.72152, -0.0887107)
(3.79747, -0.0799423)
(3.87342, -0.0723515)
(3.94937, -0.0674546)
(4.02532, -0.0605281)
(4.10127, -0.047674)
(4.17722, -0.0440246)
(4.25316, -0.0334033)
(4.32911, -0.0223581)
(4.40506, -0.0188692)
(4.48101, -0.0133644)
(4.55696, -0.0149596)
(4.63291, -0.018063)
(4.70886, -0.0230831)
(4.78481, -0.0255839)
(4.86076, -0.027767)
(4.93671, -0.0300812)
(5.01266, -0.0321571)
(5.08861, -0.0374975)
(5.16456, -0.0405278)
(5.24051, -0.0446817)
(5.31646, -0.0427593)
(5.39241, -0.0411138)
(5.46835, -0.0326176)
(5.5443, -0.0252624)
(5.62025, -0.0142363)
(5.6962, -0.00864033)
(5.77215, 0.00267359)
(5.8481, 0.0140792)
(5.92405, 0.0217937)
(6, 0.0251912)
(6.07595, 0.0257348)
(6.1519, 0.0252773)
(6.22785, 0.0251514)
(6.3038, 0.0252192)
(6.37975, 0.0232554)
(6.4557, 0.0225664)
(6.53165, 0.0248136)
(6.60759, 0.0272257)
(6.68354, 0.0271772)
(6.75949, 0.0227176)
(6.83544, 0.0227474)
(6.91139, 0.0214524)
(6.98734, 0.0180422)
(7.06329, 0.0160421)
(7.13924, 0.00784208)
(7.21519, 0.00536754)
(7.29114, 0.001567)
(7.36709, -0.00474153)
(7.44304, -0.00730608)
(7.51899, -0.0115705)
(7.59494, -0.0134439)
(7.67089, -0.016659)
(7.74684, -0.0195873)
(7.82278, -0.0231101)
(7.89873, -0.0262888)
(7.97468, -0.0284729)
(8.05063, -0.0316435)
(8.12658, -0.0340059)
(8.20253, -0.0398674)
(8.27848, -0.0414349)
(8.35443, -0.0406487)
(8.43038, -0.0426876)
(8.50633, -0.0470634)
(8.58228, -0.0490964)
(8.65823, -0.0476192)
(8.73418, -0.0496038)
(8.81013, -0.0554609)
(8.88608, -0.0563514)
(8.96203, -0.0523658)
(9.03798, -0.0490732)
(9.11392, -0.0476933)
(9.18987, -0.0476526)
(9.26582, -0.0507049)
(9.34177, -0.0540584)
(9.41772, -0.0559142)
(9.49367, -0.0572582)
(9.56962, -0.0594728)
(9.64557, -0.0582307)
(9.72152, -0.0539028)
(9.79747, -0.0496287)
(9.87342, -0.0447807)
(9.94937, -0.0408875)
(10.0253, -0.0361385)
(10.1013, -0.0300309)
(10.1772, -0.0264083)
(10.2532, -0.0237607)
(10.3291, -0.017337)
(10.4051, -0.0111627)
(10.481, -0.00748495)
(10.557, -0.0072505)
(10.6329, -0.00748513)
(10.7089, -0.0115817)
(10.7848, -0.0175847)
(10.8608, -0.0244519)
(10.9367, -0.0434608)
(11.0127, -0.048637)
(11.0886, -0.055532)
(11.1646, -0.058972)
(11.2405, -0.0598594)
(11.3165, -0.0527776)
(11.3924, -0.0442203)
(11.4684, -0.0385766)
(11.5443, -0.0307924)
(11.6203, -0.0270283)
(11.6962, -0.0246726)
(11.7722, -0.0216135)
(11.8481, -0.0214822)
(11.9241, -0.0232589)
(12, -0.0305585)
(12.0759, -0.0315323)
(12.1519, -0.0334357)
(12.2278, -0.0356755)
(12.3038, -0.0319845)
(12.3797, -0.0337102)
(12.4557, -0.0326302)
(12.5316, -0.0283435)
(12.6076, -0.026905)
(12.6835, -0.0274747)
(12.7595, -0.0263377)
(12.8354, -0.0247519)
(12.9114, -0.019875)
(12.9873, -0.0177509)
(13.0633, -0.0155644)
(13.1392, -0.0124393)
(13.2152, -0.0112727)
(13.2911, -0.00806411)
(13.3671, -0.0107642)
(13.443, -0.0166683)
(13.519, -0.0215992)
(13.5949, -0.0304149)
(13.6709, -0.0368919)
(13.7468, -0.041642)
(13.8228, -0.0488494)
(13.8987, -0.0546591)
(13.9747, -0.0594334)
(14.0506, -0.0618388)
(14.1266, -0.0607265)
(14.2025, -0.0613889)
(14.2785, -0.0617137)
(14.3544, -0.0612672)
(14.4304, -0.0561216)
(14.5063, -0.054036)
(14.5823, -0.0485455)
(14.6582, -0.0440595)
(14.7342, -0.0303302)
(14.8101, -0.0211699)
(14.8861, -0.0157799)
(14.962, -0.0096087)
(15.038, -0.00347695)
(15.1139, -0.0016326)
(15.1899, -0.00170712)
(15.2658, -0.00568673)
(15.3418, -0.00805138)
(15.4177, -0.0112128)
(15.4937, -0.0150037)
(15.5696, -0.0220976)
(15.6456, -0.0256237)
(15.7215, -0.0285107)
(15.7975, -0.0309777)
(15.8734, -0.0323547)
(15.9494, -0.0339327)
(16.0253, -0.0351422)
(16.1013, -0.0359264)
(16.1772, -0.0356896)
(16.2532, -0.0360449)
(16.3291, -0.0382555)
(16.4051, -0.037363)
(16.481, -0.0339581)
(16.557, -0.0287526)
(16.6329, -0.026452)
(16.7089, -0.0254463)
(16.7848, -0.0258033)
(16.8608, -0.0257999)
(16.9367, -0.0263461)
(17.0127, -0.0266891)
(17.0886, -0.0297718)
(17.1646, -0.0352851)
(17.2405, -0.0367487)
(17.3165, -0.0382137)
(17.3924, -0.038985)
(17.4684, -0.0373531)
(17.5443, -0.038239)
(17.6203, -0.038037)
(17.6962, -0.0445045)
(17.7722, -0.0444068)
(17.8481, -0.0437533)
(17.9241, -0.0434328)
(18, -0.0483413)
(18.076, -0.0511302)
(18.1519, -0.0530475)
(18.2278, -0.0481024)
(18.3038, -0.0477769)
(18.3797, -0.0482187)
(18.4557, -0.0466967)
(18.5316, -0.0416264)
(18.6076, -0.0383402)
(18.6835, -0.0376267)
(18.7595, -0.0367606)
(18.8354, -0.0351855)
(18.9114, -0.0368832)
(18.9873, -0.0386753)
(19.0633, -0.0383417)
(19.1392, -0.0405427)
(19.2152, -0.041623)
(19.2911, -0.0427861)
(19.3671, -0.0392038)
(19.443, -0.0273605)
(19.519, -0.0191765)
(19.5949, -0.0132046)
(19.6709, 0.000645065)
(19.7468, 0.0043266)
(19.8228, 0.00794741)
(19.8987, 0.00814423)
(19.9747, 0.0150473)
(20.0506, 0.0139897)
(20.1266, 0.00725341)
(20.2025, 0.00331655)
(20.2785, -0.00469358)
(20.3544, -0.0109581)
(20.4304, -0.0174898)
(20.5063, -0.0255319)
(20.5823, -0.0321123)
(20.6582, -0.0303962)
(20.7342, -0.0264203)
(20.8101, -0.0276232)
(20.8861, -0.025751)
(20.962, -0.0265572)
(21.038, -0.0267577)
(21.1139, -0.0326064)
(21.1899, -0.0359003)
(21.2658, -0.0421811)
(21.3418, -0.0401359)
(21.4177, -0.0391827)
(21.4937, -0.0324245)
(21.5696, -0.0279522)
(21.6456, -0.0187817)
(21.7215, -0.0125635)
(21.7975, -0.0063074)
(21.8734, 0.00118336)
(21.9494, 0.00887592)
(22.0253, 0.0118444)
(22.1013, 0.0148647)
(22.1772, 0.0132608)
(22.2532, 0.0092051)
(22.3291, 0.000326907)
(22.4051, -0.00799793)
(22.481, -0.0142304)
(22.557, -0.0214329)
(22.6329, -0.0260143)
(22.7089, -0.0289541)
(22.7848, -0.0321487)
(22.8608, -0.0334443)
(22.9367, -0.0357043)
(23.0127, -0.0352777)
(23.0886, -0.0362675)
(23.1646, -0.0361218)
(23.2405, -0.0325459)
(23.3165, -0.0337339)
(23.3924, -0.0374591)
(23.4684, -0.0378782)
(23.5443, -0.0372618)
(23.6203, -0.0333888)
(23.6962, -0.0319565)
(23.7722, -0.0328378)
(23.8481, -0.0299729)
(23.9241, -0.0275076)
(24, -0.0264782)
(24.076, -0.026596)
(24.1519, -0.0258939)
(24.2278, -0.0263445)
(24.3038, -0.0260996)
(24.3797, -0.0265498)
(24.4557, -0.0263701)
(24.5316, -0.0269492)
(24.6076, -0.0273957)
(24.6835, -0.0270817)
(24.7595, -0.0266207)
(24.8354, -0.02618)
(24.9114, -0.0261233)
(24.9873, -0.0258683)
(25.0633, -0.0263578)
(25.1392, -0.0264389)
(25.2152, -0.0264263)
(25.2911, -0.0269322)
(25.3671, -0.0286304)
(25.443, -0.0288973)
(25.519, -0.0282948)
(25.5949, -0.0277685)
(25.6709, -0.0282024)
(25.7468, -0.0275338)
(25.8228, -0.0286171)
(25.8987, -0.0287096)
(25.9747, -0.0295937)
(26.0506, -0.0306822)
(26.1266, -0.0301251)
(26.2025, -0.0296462)
(26.2785, -0.0298889)
(26.3544, -0.0289035)
(26.4304, -0.0305786)
(26.5063, -0.0294217)
(26.5823, -0.0288775)
(26.6582, -0.0278159)
(26.7342, -0.0281461)
(26.8101, -0.0275054)
(26.8861, -0.0272312)
(26.962, -0.0275608)
(27.038, -0.0276217)
(27.1139, -0.027267)
(27.1899, -0.026963)
(27.2658, -0.0283784)
(27.3418, -0.0285005)
(27.4177, -0.029199)
(27.4937, -0.030484)
(27.5696, -0.0304936)
(27.6456, -0.031798)
(27.7215, -0.0321446)
(27.7975, -0.0301329)
(27.8734, -0.0302942)
(27.9494, -0.0298343)
(28.0253, -0.0292793)
(28.1013, -0.028439)
(28.1772, -0.0282505)
(28.2532, -0.0273796)
(28.3291, -0.0265252)
(28.4051, -0.0265876)
(28.481, -0.0260748)
(28.557, -0.0260802)
(28.6329, -0.0255746)
(28.7089, -0.0262419)
(28.7848, -0.0252147)
(28.8608, -0.0257354)
(28.9367, -0.0265124)
(29.0127, -0.0262335)
(29.0886, -0.026084)
(29.1646, -0.0276404)
(29.2405, -0.0270721)
(29.3165, -0.0284078)
(29.3924, -0.0294742)
(29.4684, -0.0294222)
(29.5443, -0.0285855)
(29.6203, -0.0273562)
(29.6962, -0.0263362)
(29.7722, -0.0263595)
(29.8481, -0.0258464)
(29.9241, -0.0255486)
(30, -0.0255959)
(30.076, -0.0260349)
(30.1519, -0.0261338)
(30.2278, -0.0263555)
(30.3038, -0.0264727)
(30.3797, -0.0266844)
(30.4557, -0.026814)
(30.5316, -0.0273101)
(30.6076, -0.0274248)
(30.6835, -0.0276622)
(30.7595, -0.0282009)
};

==> exp_plots/constrained_ws/x_des.tex <==
\addplot[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates {
(0, 0)
(0.0759494, 0)
(0.151899, 0)
(0.227848, 0)
(0.303797, 0)
(0.379747, 0)
(0.455696, 0)
(0.531646, 0)
(0.607595, 0)
(0.683544, 0)
(0.759494, 0)
(0.835443, 0)
(0.911392, 0)
(0.987342, 0)
(1.06329, 0)
(1.13924, 0)
(1.21519, 0)
(1.29114, 0)
(1.36709, 0)
(1.44304, 0)
(1.51899, 0)
(1.59494, 0)
(1.67089, 0)
(1.74684, 0)
(1.82278, 0)
(1.89873, 0)
(1.97468, 0)
(2.05063, 0)
(2.12658, 0)
(2.20253, 0)
(2.27848, 0)
(2.35443, 0)
(2.43038, 0)
(2.50633, 0)
(2.58228, 0)
(2.65823, 0)
(2.73418, 0)
(2.81013, 0)
(2.88608, 0)
(2.96203, 0)
(3.03797, 0)
(3.11392, 0)
(3.18987, 0)
(3.26582, 0)
(3.34177, 0)
(3.41772, 0)
(3.49367, 0)
(3.56962, 0)
(3.64557, 0)
(3.72152, 0)
(3.79747, 0)
(3.87342, 0)
(3.94937, 0)
(4.02532, 0)
(4.10127, 0)
(4.17722, 0)
(4.25316, 0)
(4.32911, 0)
(4.40506, 0)
(4.48101, 0)
(4.55696, 0)
(4.63291, 0)
(4.70886, 0)
(4.78481, 0)
(4.86076, 0)
(4.93671, 0)
(5.01266, 0)
(5.08861, 0)
(5.16456, 0)
(5.24051, 0)
(5.31646, 0)
(5.39241, 0)
(5.46835, 0)
(5.5443, 0)
(5.62025, 0)
(5.6962, 0)
(5.77215, 0)
(5.8481, 0)
(5.92405, 0)
(6, 0)
(6.07595, 0)
(6.1519, 0)
(6.22785, 0)
(6.3038, 0)
(6.37975, 0)
(6.4557, 0)
(6.53165, 0)
(6.60759, 0)
(6.68354, 0)
(6.75949, 0)
(6.83544, 0)
(6.91139, 0)
(6.98734, 0)
(7.06329, 0)
(7.13924, 0)
(7.21519, 0)
(7.29114, 0)
(7.36709, 0)
(7.44304, 0)
(7.51899, 0)
(7.59494, 0)
(7.67089, 0)
(7.74684, 0)
(7.82278, 0)
(7.89873, 0)
(7.97468, 0)
(8.05063, 0)
(8.12658, 0)
(8.20253, 0)
(8.27848, 0)
(8.35443, 0)
(8.43038, 0)
(8.50633, 0)
(8.58228, 0)
(8.65823, 0)
(8.73418, 0)
(8.81013, 0)
(8.88608, 0)
(8.96203, 0)
(9.03798, 0)
(9.11392, 0)
(9.18987, 0)
(9.26582, 0)
(9.34177, 0)
(9.41772, 0)
(9.49367, 0)
(9.56962, 0)
(9.64557, 0)
(9.72152, 0)
(9.79747, 0)
(9.87342, 0)
(9.94937, 0)
(10.0253, 0)
(10.1013, 0)
(10.1772, 0)
(10.2532, 0)
(10.3291, 0)
(10.4051, 0)
(10.481, 0)
(10.557, 0)
(10.6329, 0)
(10.7089, 0)
(10.7848, 0)
(10.8608, 0)
(10.9367, 0)
(11.0127, 0)
(11.0886, 0)
(11.1646, 0)
(11.2405, 0)
(11.3165, 0)
(11.3924, 0)
(11.4684, 0)
(11.5443, 0)
(11.6203, 0)
(11.6962, 0)
(11.7722, 0)
(11.8481, 0)
(11.9241, 0)
(12, 0)
(12.0759, 0)
(12.1519, 0)
(12.2278, 0)
(12.3038, 0)
(12.3797, 0)
(12.4557, 0)
(12.5316, 0)
(12.6076, 0)
(12.6835, 0)
(12.7595, 0)
(12.8354, 0)
(12.9114, 0)
(12.9873, 0)
(13.0633, 0)
(13.1392, 0)
(13.2152, 0)
(13.2911, 0)
(13.3671, 0)
(13.443, 0)
(13.519, 0)
(13.5949, 0)
(13.6709, 0)
(13.7468, 0)
(13.8228, 0)
(13.8987, 0)
(13.9747, 0)
(14.0506, 0)
(14.1266, 0)
(14.2025, 0)
(14.2785, 0)
(14.3544, 0)
(14.4304, 0)
(14.5063, 0)
(14.5823, 0)
(14.6582, 0)
(14.7342, 0)
(14.8101, 0)
(14.8861, 0)
(14.962, 0)
(15.038, 0)
(15.1139, 0)
(15.1899, 0)
(15.2658, 0)
(15.3418, 0)
(15.4177, 0)
(15.4937, 0)
(15.5696, 0)
(15.6456, 0)
(15.7215, 0)
(15.7975, 0)
(15.8734, 0)
(15.9494, 0)
(16.0253, 0)
(16.1013, 0)
(16.1772, 0)
(16.2532, 0)
(16.3291, 0)
(16.4051, 0)
(16.481, 0)
(16.557, 0)
(16.6329, 0)
(16.7089, 0)
(16.7848, 0)
(16.8608, 0)
(16.9367, 0)
(17.0127, 0)
(17.0886, 0)
(17.1646, 0)
(17.2405, 0)
(17.3165, 0)
(17.3924, 0)
(17.4684, 0)
(17.5443, 0)
(17.6203, 0)
(17.6962, 0)
(17.7722, 0)
(17.8481, 0)
(17.9241, 0)
(18, 0)
(18.076, 0)
(18.1519, 0)
(18.2278, 0)
(18.3038, 0)
(18.3797, 0)
(18.4557, 0)
(18.5316, 0)
(18.6076, 0)
(18.6835, 0)
(18.7595, 0)
(18.8354, 0)
(18.9114, 0)
(18.9873, 0)
(19.0633, 0)
(19.1392, 0)
(19.2152, 0)
(19.2911, 0)
(19.3671, 0)
(19.443, 0)
(19.519, 0)
(19.5949, 0)
(19.6709, 0)
(19.7468, 0)
(19.8228, 0)
(19.8987, 0)
(19.9747, 0)
(20.0506, 0)
(20.1266, 0)
(20.2025, 0)
(20.2785, 0)
(20.3544, 0)
(20.4304, 0)
(20.5063, 0)
(20.5823, 0)
(20.6582, 0)
(20.7342, 0)
(20.8101, 0)
(20.8861, 0)
(20.962, 0)
(21.038, 0)
(21.1139, 0)
(21.1899, 0)
(21.2658, 0)
(21.3418, 0)
(21.4177, 0)
(21.4937, 0)
(21.5696, 0)
(21.6456, 0)
(21.7215, 0)
(21.7975, 0)
(21.8734, 0)
(21.9494, 0)
(22.0253, 0)
(22.1013, 0)
(22.1772, 0)
(22.2532, 0)
(22.3291, 0)
(22.4051, 0)
(22.481, 0)
(22.557, 0)
(22.6329, 0)
(22.7089, 0)
(22.7848, 0)
(22.8608, 0)
(22.9367, 0)
(23.0127, 0)
(23.0886, 0)
(23.1646, 0)
(23.2405, 0)
(23.3165, 0)
(23.3924, 0)
(23.4684, 0)
(23.5443, 0)
(23.6203, 0)
(23.6962, 0)
(23.7722, 0)
(23.8481, 0)
(23.9241, 0)
(24, 0)
(24.076, 0)
(24.1519, 0)
(24.2278, 0)
(24.3038, 0)
(24.3797, 0)
(24.4557, 0)
(24.5316, 0)
(24.6076, 0)
(24.6835, 0)
(24.7595, 0)
(24.8354, 0)
(24.9114, 0)
(24.9873, 0)
(25.0633, 0)
(25.1392, 0)
(25.2152, 0)
(25.2911, 0)
(25.3671, 0)
(25.443, 0)
(25.519, 0)
(25.5949, 0)
(25.6709, 0)
(25.7468, 0)
(25.8228, 0)
(25.8987, 0)
(25.9747, 0)
(26.0506, 0)
(26.1266, 0)
(26.2025, 0)
(26.2785, 0)
(26.3544, 0)
(26.4304, 0)
(26.5063, 0)
(26.5823, 0)
(26.6582, 0)
(26.7342, 0)
(26.8101, 0)
(26.8861, 0)
(26.962, 0)
(27.038, 0)
(27.1139, 0)
(27.1899, 0)
(27.2658, 0)
(27.3418, 0)
(27.4177, 0)
(27.4937, 0)
(27.5696, 0)
(27.6456, 0)
(27.7215, 0)
(27.7975, 0)
(27.8734, 0)
(27.9494, 0)
(28.0253, 0)
(28.1013, 0)
(28.1772, 0)
(28.2532, 0)
(28.3291, 0)
(28.4051, 0)
(28.481, 0)
(28.557, 0)
(28.6329, 0)
(28.7089, 0)
(28.7848, 0)
(28.8608, 0)
(28.9367, 0)
(29.0127, 0)
(29.0886, 0)
(29.1646, 0)
(29.2405, 0)
(29.3165, 0)
(29.3924, 0)
(29.4684, 0)
(29.5443, 0)
(29.6203, 0)
(29.6962, 0)
(29.7722, 0)
(29.8481, 0)
(29.9241, 0)
(30, 0)
(30.076, 0)
(30.1519, 0)
(30.2278, 0)
(30.3038, 0)
(30.3797, 0)
(30.4557, 0)
(30.5316, 0)
(30.6076, 0)
(30.6835, 0)
(30.7595, 0)
(30.8354, 0)
(30.9114, 0)
(30.9873, 0)
(31.0633, 0)
(31.1392, 0)
(31.2152, 0)
(31.2911, 0)
(31.3671, 0)
(31.443, 0)
(31.519, 0)
(31.5949, 0)
(31.6709, 0)
(31.7468, 0)
(31.8228, 0)
(31.8987, 0)
(31.9747, 0)
(32.0506, 0)
};

==> exp_plots/constrained_ws/y.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0)
(0.0759494, 7.58332e-05)
(0.151899, -0.000201016)
(0.227848, -0.000183111)
(0.303797, 2.15727e-05)
(0.379747, 9.91392e-05)
(0.455696, 0.000307189)
(0.531646, 0.000423447)
(0.607595, 0.00022654)
(0.683544, 0.00024285)
(0.759494, 0.000469587)
(0.835443, 0.00060386)
(0.911392, 0.000482769)
(0.987342, 0.000519552)
(1.06329, 0.000166293)
(1.13924, -0.000216946)
(1.21519, 0.000205172)
(1.29114, 0.000611079)
(1.36709, 0.00114407)
(1.44304, 0.00139208)
(1.51899, 0.000636707)
(1.59494, 0.000347424)
(1.67089, 0.00114216)
(1.74684, 0.000921534)
(1.82278, 0.000674953)
(1.89873, -0.000557594)
(1.97468, -0.000280067)
(2.05063, -0.000382509)
(2.12658, 0.000567059)
(2.20253, 0.000489754)
(2.27848, 0.000875243)
(2.35443, 0.00077916)
(2.43038, -0.00307519)
(2.50633, -0.00285418)
(2.58228, -0.00380727)
(2.65823, -0.00893974)
(2.73418, -0.0122262)
(2.81013, -0.0116876)
(2.88608, -0.010191)
(2.96203, -0.00900317)
(3.03797, -0.00581825)
(3.11392, -0.00421786)
(3.18987, 0.000334927)
(3.26582, 0.0034604)
(3.34177, 0.00323301)
(3.41772, -0.00149371)
(3.49367, -0.00130728)
(3.56962, -0.000964061)
(3.64557, 0.00582289)
(3.72152, 0.012103)
(3.79747, 0.0200399)
(3.87342, 0.0291581)
(3.94937, 0.0370141)
(4.02532, 0.0423495)
(4.10127, 0.0406994)
(4.17722, 0.0381641)
(4.25316, 0.0379129)
(4.32911, 0.0393841)
(4.40506, 0.0360934)
(4.48101, 0.0381203)
(4.55696, 0.0365218)
(4.63291, 0.0361347)
(4.70886, 0.0335829)
(4.78481, 0.0306714)
(4.86076, 0.0271596)
(4.93671, 0.0232493)
(5.01266, 0.0208419)
(5.08861, 0.0159371)
(5.16456, 0.0131263)
(5.24051, 0.0107344)
(5.31646, 0.00983153)
(5.39241, 0.0099397)
(5.46835, 0.0104306)
(5.5443, 0.0101332)
(5.62025, 0.0111034)
(5.6962, 0.0121641)
(5.77215, 0.0134059)
(5.8481, 0.0152562)
(5.92405, 0.0126807)
(6, 0.0123098)
(6.07595, 0.0112736)
(6.1519, 0.0111866)
(6.22785, 0.0118382)
(6.3038, 0.0141405)
(6.37975, 0.0134192)
(6.4557, 0.0126219)
(6.53165, 0.0176494)
(6.60759, 0.019688)
(6.68354, 0.0196258)
(6.75949, 0.0119673)
(6.83544, 0.0109801)
(6.91139, 0.0131118)
(6.98734, 0.0120902)
(7.06329, 0.011729)
(7.13924, 0.0011287)
(7.21519, 0.00228388)
(7.29114, 0.00183888)
(7.36709, 0.00145943)
(7.44304, 0.00228302)
(7.51899, -0.000716907)
(7.59494, 0.00147018)
(7.67089, 0.00112451)
(7.74684, 0.00359947)
(7.82278, 0.00408815)
(7.89873, 0.00660398)
(7.97468, 0.00729195)
(8.05063, 0.00693821)
(8.12658, 0.00537123)
(8.20253, 0.00306523)
(8.27848, 0.00663036)
(8.35443, 0.0112537)
(8.43038, 0.0122133)
(8.50633, 0.0117769)
(8.58228, 0.0105597)
(8.65823, 0.00868771)
(8.73418, 0.0063179)
(8.81013, -0.00342071)
(8.88608, -0.00936045)
(8.96203, -0.00974163)
(9.03798, -0.0119579)
(9.11392, -0.0106087)
(9.18987, -0.0127932)
(9.26582, -0.0159644)
(9.34177, -0.0176522)
(9.41772, -0.0167066)
(9.49367, -0.0160509)
(9.56962, -0.0152663)
(9.64557, -0.0143098)
(9.72152, -0.01174)
(9.79747, -0.0109292)
(9.87342, -0.00857306)
(9.94937, -0.0113858)
(10.0253, -0.0116414)
(10.1013, -0.0079878)
(10.1772, -0.00761613)
(10.2532, -0.0101591)
(10.3291, -0.00889034)
(10.4051, -0.00559665)
(10.481, -0.00330363)
(10.557, -0.00248443)
(10.6329, 0.00407956)
(10.7089, 0.00924791)
(10.7848, 0.0123436)
(10.8608, 0.0123292)
(10.9367, 0.00553627)
(11.0127, 0.0108763)
(11.0886, 0.00656061)
(11.1646, 0.0044576)
(11.2405, 0.00109653)
(11.3165, 0.00794238)
(11.3924, 0.0151334)
(11.4684, 0.0210995)
(11.5443, 0.0260102)
(11.6203, 0.0316092)
(11.6962, 0.0369562)
(11.7722, 0.0412869)
(11.8481, 0.0442227)
(11.9241, 0.0470679)
(12, 0.0448799)
(12.0759, 0.0464718)
(12.1519, 0.0422449)
(12.2278, 0.0402333)
(12.3038, 0.0395767)
(12.3797, 0.0352122)
(12.4557, 0.0335018)
(12.5316, 0.0355244)
(12.6076, 0.0351351)
(12.6835, 0.0308541)
(12.7595, 0.0252997)
(12.8354, 0.0205972)
(12.9114, 0.0164977)
(12.9873, 0.0103905)
(13.0633, 0.00695932)
(13.1392, 0.00349848)
(13.2152, -0.00361977)
(13.2911, -0.00404603)
(13.3671, -0.00906228)
(13.443, -0.0142365)
(13.519, -0.0136656)
(13.5949, -0.0139469)
(13.6709, -0.0151006)
(13.7468, -0.0149041)
(13.8228, -0.0164265)
(13.8987, -0.018421)
(13.9747, -0.0191579)
(14.0506, -0.0191742)
(14.1266, -0.0198221)
(14.2025, -0.0219822)
(14.2785, -0.0237552)
(14.3544, -0.0259839)
(14.4304, -0.0324874)
(14.5063, -0.0382091)
(14.5823, -0.0385324)
(14.6582, -0.0381462)
(14.7342, -0.0369361)
(14.8101, -0.0335153)
(14.8861, -0.0386713)
(14.962, -0.0420041)
(15.038, -0.0422804)
(15.1139, -0.0448909)
(15.1899, -0.0454963)
(15.2658, -0.0451244)
(15.3418, -0.0411854)
(15.4177, -0.0388216)
(15.4937, -0.0357971)
(15.5696, -0.033052)
(15.6456, -0.0311695)
(15.7215, -0.0243775)
(15.7975, -0.0171092)
(15.8734, -0.0110411)
(15.9494, -0.00588639)
(16.0253, -0.00278051)
(16.1013, -0.00241683)
(16.1772, -0.00323761)
(16.2532, -0.00409782)
(16.3291, -0.00550986)
(16.4051, -0.00643761)
(16.481, -0.00705315)
(16.557, -0.00469781)
(16.6329, -0.000749551)
(16.7089, 0.000719686)
(16.7848, 0.000380129)
(16.8608, 0.00292778)
(16.9367, 0.00587366)
(17.0127, 0.00684682)
(17.0886, 0.00882539)
(17.1646, 0.0131304)
(17.2405, 0.0155706)
(17.3165, 0.0189019)
(17.3924, 0.0214863)
(17.4684, 0.0344816)
(17.5443, 0.038108)
(17.6203, 0.0401179)
(17.6962, 0.0421055)
(17.7722, 0.0452079)
(17.8481, 0.0438453)
(17.9241, 0.0427658)
(18, 0.0392021)
(18.076, 0.0361388)
(18.1519, 0.0333937)
(18.2278, 0.0297758)
(18.3038, 0.025779)
(18.3797, 0.0195728)
(18.4557, 0.0152611)
(18.5316, 0.0143294)
(18.6076, 0.0118035)
(18.6835, 0.00574283)
(18.7595, 0.00185762)
(18.8354, -0.000416186)
(18.9114, -0.00565041)
(18.9873, -0.00814439)
(19.0633, -0.0107399)
(19.1392, -0.0145278)
(19.2152, -0.0163919)
(19.2911, -0.0162485)
(19.3671, -0.0148767)
(19.443, -0.00790836)
(19.519, -0.00420078)
(19.5949, 0.00264359)
(19.6709, 0.0150728)
(19.7468, 0.0196385)
(19.8228, 0.0232836)
(19.8987, 0.029726)
(19.9747, 0.0380377)
(20.0506, 0.0460325)
(20.1266, 0.0514076)
(20.2025, 0.0535143)
(20.2785, 0.0576846)
(20.3544, 0.0611017)
(20.4304, 0.0611434)
(20.5063, 0.0567703)
(20.5823, 0.0553122)
(20.6582, 0.0553785)
(20.7342, 0.0558561)
(20.8101, 0.0536942)
(20.8861, 0.0533814)
(20.962, 0.0522401)
(21.038, 0.0506519)
(21.1139, 0.0431482)
(21.1899, 0.0374864)
(21.2658, 0.029495)
(21.3418, 0.0269193)
(21.4177, 0.021938)
(21.4937, 0.0245441)
(21.5696, 0.0229722)
(21.6456, 0.0256459)
(21.7215, 0.0260075)
(21.7975, 0.0229932)
(21.8734, 0.0150445)
(21.9494, 0.0172533)
(22.0253, 0.0119692)
(22.1013, 0.0102505)
(22.1772, 0.00280177)
(22.2532, 0.0016417)
(22.3291, -0.00556634)
(22.4051, -0.0120274)
(22.481, -0.0135543)
(22.557, -0.0132896)
(22.6329, -0.0145853)
(22.7089, -0.015695)
(22.7848, -0.0139244)
(22.8608, -0.00454996)
(22.9367, -0.00703382)
(23.0127, -0.00422275)
(23.0886, -0.00285146)
(23.1646, -0.000693075)
(23.2405, 0.00209617)
(23.3165, 0.00028933)
(23.3924, -0.00244602)
(23.4684, -0.00309485)
(23.5443, -0.0039276)
(23.6203, -0.00952598)
(23.6962, -0.01605)
(23.7722, -0.0202881)
(23.8481, -0.0210481)
(23.9241, -0.017655)
(24, -0.0153909)
(24.076, -0.0137754)
(24.1519, -0.0131405)
(24.2278, -0.0127108)
(24.3038, -0.0121957)
(24.3797, -0.0122141)
(24.4557, -0.0122403)
(24.5316, -0.0132521)
(24.6076, -0.0134722)
(24.6835, -0.0137567)
(24.7595, -0.0138163)
(24.8354, -0.0134893)
(24.9114, -0.0133599)
(24.9873, -0.0129559)
(25.0633, -0.0132784)
(25.1392, -0.0134427)
(25.2152, -0.0137)
(25.2911, -0.0141266)
(25.3671, -0.0140375)
(25.443, -0.0140465)
(25.519, -0.0144602)
(25.5949, -0.0146127)
(25.6709, -0.0144973)
(25.7468, -0.014738)
(25.8228, -0.0144987)
(25.8987, -0.0149331)
(25.9747, -0.0145967)
(26.0506, -0.01286)
(26.1266, -0.0134829)
(26.2025, -0.0131153)
(26.2785, -0.0135297)
(26.3544, -0.0140917)
(26.4304, -0.0143652)
(26.5063, -0.0134348)
(26.5823, -0.0117024)
(26.6582, -0.0109224)
(26.7342, -0.0124174)
(26.8101, -0.00844417)
(26.8861, -0.00944485)
(26.962, -0.0115571)
(27.038, -0.0103154)
(27.1139, -0.00951967)
(27.1899, -0.0117881)
(27.2658, -0.0143815)
(27.3418, -0.0142419)
(27.4177, -0.0135599)
(27.4937, -0.0128877)
(27.5696, -0.0124855)
(27.6456, -0.0140413)
(27.7215, -0.0144335)
(27.7975, -0.0146254)
(27.8734, -0.0143131)
(27.9494, -0.0148037)
(28.0253, -0.01406)
(28.1013, -0.0118224)
(28.1772, -0.0109472)
(28.2532, -0.0089163)
(28.3291, -0.00793805)
(28.4051, -0.00999009)
(28.481, -0.0112639)
(28.557, -0.00907494)
(28.6329, -0.00848819)
(28.7089, -0.00748508)
(28.7848, -0.00829186)
(28.8608, -0.00709606)
(28.9367, -0.00781712)
(29.0127, -0.00690756)
(29.0886, -0.0078984)
(29.1646, -0.0109918)
(29.2405, -0.00946408)
(29.3165, -0.00967136)
(29.3924, -0.011785)
(29.4684, -0.0129578)
(29.5443, -0.0111616)
(29.6203, -0.00990257)
(29.6962, -0.0102687)
(29.7722, -0.0109643)
(29.8481, -0.010927)
(29.9241, -0.0108937)
(30, -0.0113146)
(30.076, -0.0111791)
(30.1519, -0.0112291)
(30.2278, -0.0110803)
(30.3038, -0.0110354)
(30.3797, -0.0109351)
(30.4557, -0.0110331)
(30.5316, -0.0102884)
(30.6076, -0.00952516)
(30.6835, -0.00916045)
(30.7595, -0.00953066)
};

==> exp_plots/constrained_ws/y_des.tex <==
\addplot[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates {
(0, 0)
(0.0759494, 0)
(0.151899, 0)
(0.227848, 0)
(0.303797, 0)
(0.379747, 0)
(0.455696, 0)
(0.531646, 0)
(0.607595, 0)
(0.683544, 0)
(0.759494, 0)
(0.835443, 0)
(0.911392, 0)
(0.987342, 0)
(1.06329, 0)
(1.13924, 0)
(1.21519, 0)
(1.29114, 0)
(1.36709, 0)
(1.44304, 0)
(1.51899, 0)
(1.59494, 0)
(1.67089, 0)
(1.74684, 0)
(1.82278, 0)
(1.89873, 0)
(1.97468, 0)
(2.05063, 0)
(2.12658, 0)
(2.20253, 0)
(2.27848, 0)
(2.35443, 0)
(2.43038, 0)
(2.50633, 0)
(2.58228, 0)
(2.65823, 0)
(2.73418, 0)
(2.81013, 0)
(2.88608, 0)
(2.96203, 0)
(3.03797, 0)
(3.11392, 0)
(3.18987, 0)
(3.26582, 0)
(3.34177, 0)
(3.41772, 0)
(3.49367, 0)
(3.56962, 0)
(3.64557, 0)
(3.72152, 0)
(3.79747, 0)
(3.87342, 0)
(3.94937, 0)
(4.02532, 0)
(4.10127, 0)
(4.17722, 0)
(4.25316, 0)
(4.32911, 0)
(4.40506, 0)
(4.48101, 0)
(4.55696, 0)
(4.63291, 0)
(4.70886, 0)
(4.78481, 0)
(4.86076, 0)
(4.93671, 0)
(5.01266, 0)
(5.08861, 0)
(5.16456, 0)
(5.24051, 0)
(5.31646, 0)
(5.39241, 0)
(5.46835, 0)
(5.5443, 0)
(5.62025, 0)
(5.6962, 0)
(5.77215, 0)
(5.8481, 0)
(5.92405, 0)
(6, 0)
(6.07595, 0)
(6.1519, 0)
(6.22785, 0)
(6.3038, 0)
(6.37975, 0)
(6.4557, 0)
(6.53165, 0)
(6.60759, 0)
(6.68354, 0)
(6.75949, 0)
(6.83544, 0)
(6.91139, 0)
(6.98734, 0)
(7.06329, 0)
(7.13924, 0)
(7.21519, 0)
(7.29114, 0)
(7.36709, 0)
(7.44304, 0)
(7.51899, 0)
(7.59494, 0)
(7.67089, 0)
(7.74684, 0)
(7.82278, 0)
(7.89873, 0)
(7.97468, 0)
(8.05063, 0)
(8.12658, 0)
(8.20253, 0)
(8.27848, 0)
(8.35443, 0)
(8.43038, 0)
(8.50633, 0)
(8.58228, 0)
(8.65823, 0)
(8.73418, 0)
(8.81013, 0)
(8.88608, 0)
(8.96203, 0)
(9.03798, 0)
(9.11392, 0)
(9.18987, 0)
(9.26582, 0)
(9.34177, 0)
(9.41772, 0)
(9.49367, 0)
(9.56962, 0)
(9.64557, 0)
(9.72152, 0)
(9.79747, 0)
(9.87342, 0)
(9.94937, 0)
(10.0253, 0)
(10.1013, 0)
(10.1772, 0)
(10.2532, 0)
(10.3291, 0)
(10.4051, 0)
(10.481, 0)
(10.557, 0)
(10.6329, 0)
(10.7089, 0)
(10.7848, 0)
(10.8608, 0)
(10.9367, 0)
(11.0127, 0)
(11.0886, 0)
(11.1646, 0)
(11.2405, 0)
(11.3165, 0)
(11.3924, 0)
(11.4684, 0)
(11.5443, 0)
(11.6203, 0)
(11.6962, 0)
(11.7722, 0)
(11.8481, 0)
(11.9241, 0)
(12, 0)
(12.0759, 0)
(12.1519, 0)
(12.2278, 0)
(12.3038, 0)
(12.3797, 0)
(12.4557, 0)
(12.5316, 0)
(12.6076, 0)
(12.6835, 0)
(12.7595, 0)
(12.8354, 0)
(12.9114, 0)
(12.9873, 0)
(13.0633, 0)
(13.1392, 0)
(13.2152, 0)
(13.2911, 0)
(13.3671, 0)
(13.443, 0)
(13.519, 0)
(13.5949, 0)
(13.6709, 0)
(13.7468, 0)
(13.8228, 0)
(13.8987, 0)
(13.9747, 0)
(14.0506, 0)
(14.1266, 0)
(14.2025, 0)
(14.2785, 0)
(14.3544, 0)
(14.4304, 0)
(14.5063, 0)
(14.5823, 0)
(14.6582, 0)
(14.7342, 0)
(14.8101, 0)
(14.8861, 0)
(14.962, 0)
(15.038, 0)
(15.1139, 0)
(15.1899, 0)
(15.2658, 0)
(15.3418, 0)
(15.4177, 0)
(15.4937, 0)
(15.5696, 0)
(15.6456, 0)
(15.7215, 0)
(15.7975, 0)
(15.8734, 0)
(15.9494, 0)
(16.0253, 0)
(16.1013, 0)
(16.1772, 0)
(16.2532, 0)
(16.3291, 0)
(16.4051, 0)
(16.481, 0)
(16.557, 0)
(16.6329, 0)
(16.7089, 0)
(16.7848, 0)
(16.8608, 0)
(16.9367, 0)
(17.0127, 0)
(17.0886, 0)
(17.1646, 0)
(17.2405, 0)
(17.3165, 0)
(17.3924, 0)
(17.4684, 0)
(17.5443, 0)
(17.6203, 0)
(17.6962, 0)
(17.7722, 0)
(17.8481, 0)
(17.9241, 0)
(18, 0)
(18.076, 0)
(18.1519, 0)
(18.2278, 0)
(18.3038, 0)
(18.3797, 0)
(18.4557, 0)
(18.5316, 0)
(18.6076, 0)
(18.6835, 0)
(18.7595, 0)
(18.8354, 0)
(18.9114, 0)
(18.9873, 0)
(19.0633, 0)
(19.1392, 0)
(19.2152, 0)
(19.2911, 0)
(19.3671, 0)
(19.443, 0)
(19.519, 0)
(19.5949, 0)
(19.6709, 0)
(19.7468, 0)
(19.8228, 0)
(19.8987, 0)
(19.9747, 0)
(20.0506, 0)
(20.1266, 0)
(20.2025, 0)
(20.2785, 0)
(20.3544, 0)
(20.4304, 0)
(20.5063, 0)
(20.5823, 0)
(20.6582, 0)
(20.7342, 0)
(20.8101, 0)
(20.8861, 0)
(20.962, 0)
(21.038, 0)
(21.1139, 0)
(21.1899, 0)
(21.2658, 0)
(21.3418, 0)
(21.4177, 0)
(21.4937, 0)
(21.5696, 0)
(21.6456, 0)
(21.7215, 0)
(21.7975, 0)
(21.8734, 0)
(21.9494, 0)
(22.0253, 0)
(22.1013, 0)
(22.1772, 0)
(22.2532, 0)
(22.3291, 0)
(22.4051, 0)
(22.481, 0)
(22.557, 0)
(22.6329, 0)
(22.7089, 0)
(22.7848, 0)
(22.8608, 0)
(22.9367, 0)
(23.0127, 0)
(23.0886, 0)
(23.1646, 0)
(23.2405, 0)
(23.3165, 0)
(23.3924, 0)
(23.4684, 0)
(23.5443, 0)
(23.6203, 0)
(23.6962, 0)
(23.7722, 0)
(23.8481, 0)
(23.9241, 0)
(24, 0)
(24.076, 0)
(24.1519, 0)
(24.2278, 0)
(24.3038, 0)
(24.3797, 0)
(24.4557, 0)
(24.5316, 0)
(24.6076, 0)
(24.6835, 0)
(24.7595, 0)
(24.8354, 0)
(24.9114, 0)
(24.9873, 0)
(25.0633, 0)
(25.1392, 0)
(25.2152, 0)
(25.2911, 0)
(25.3671, 0)
(25.443, 0)
(25.519, 0)
(25.5949, 0)
(25.6709, 0)
(25.7468, 0)
(25.8228, 0)
(25.8987, 0)
(25.9747, 0)
(26.0506, 0)
(26.1266, 0)
(26.2025, 0)
(26.2785, 0)
(26.3544, 0)
(26.4304, 0)
(26.5063, 0)
(26.5823, 0)
(26.6582, 0)
(26.7342, 0)
(26.8101, 0)
(26.8861, 0)
(26.962, 0)
(27.038, 0)
(27.1139, 0)
(27.1899, 0)
(27.2658, 0)
(27.3418, 0)
(27.4177, 0)
(27.4937, 0)
(27.5696, 0)
(27.6456, 0)
(27.7215, 0)
(27.7975, 0)
(27.8734, 0)
(27.9494, 0)
(28.0253, 0)
(28.1013, 0)
(28.1772, 0)
(28.2532, 0)
(28.3291, 0)
(28.4051, 0)
(28.481, 0)
(28.557, 0)
(28.6329, 0)
(28.7089, 0)
(28.7848, 0)
(28.8608, 0)
(28.9367, 0)
(29.0127, 0)
(29.0886, 0)
(29.1646, 0)
(29.2405, 0)
(29.3165, 0)
(29.3924, 0)
(29.4684, 0)
(29.5443, 0)
(29.6203, 0)
(29.6962, 0)
(29.7722, 0)
(29.8481, 0)
(29.9241, 0)
(30, 0)
(30.076, 0)
(30.1519, 0)
(30.2278, 0)
(30.3038, 0)
(30.3797, 0)
(30.4557, 0)
(30.5316, 0)
(30.6076, 0)
(30.6835, 0)
(30.7595, 0)
(30.8354, 0)
(30.9114, 0)
(30.9873, 0)
(31.0633, 0)
(31.1392, 0)
(31.2152, 0)
(31.2911, 0)
(31.3671, 0)
(31.443, 0)
(31.519, 0)
(31.5949, 0)
(31.6709, 0)
(31.7468, 0)
(31.8228, 0)
(31.8987, 0)
(31.9747, 0)
(32.0506, 0)
};

==> exp_plots/constrained_ws/z.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0)
(0.0759494, -0.000114136)
(0.151899, -0.000181683)
(0.227848, -0.000239642)
(0.303797, -0.000146243)
(0.379747, -0.000189412)
(0.455696, -0.000445302)
(0.531646, -0.000386771)
(0.607595, -0.000221404)
(0.683544, -9.00594e-05)
(0.759494, -0.000345655)
(0.835443, -0.000642775)
(0.911392, -0.000970421)
(0.987342, -0.000672392)
(1.06329, -0.000648939)
(1.13924, -0.000531116)
(1.21519, -0.000578516)
(1.29114, -0.000751874)
(1.36709, -0.000746395)
(1.44304, -0.00141798)
(1.51899, -0.00191018)
(1.59494, -0.00298892)
(1.67089, -0.00280792)
(1.74684, -0.00203331)
(1.82278, -0.00196883)
(1.89873, -0.00222719)
(1.97468, -0.00161685)
(2.05063, -0.00154427)
(2.12658, -0.00144218)
(2.20253, -0.00142585)
(2.27848, -0.0018377)
(2.35443, -0.000415836)
(2.43038, 0.000531595)
(2.50633, 0.00199113)
(2.58228, 0.00352976)
(2.65823, 0.00382629)
(2.73418, 0.0114853)
(2.81013, 0.0290368)
(2.88608, 0.0524662)
(2.96203, 0.0640295)
(3.03797, 0.0700564)
(3.11392, 0.0855613)
(3.18987, 0.102459)
(3.26582, 0.108156)
(3.34177, 0.112277)
(3.41772, 0.119286)
(3.49367, 0.13185)
(3.56962, 0.139626)
(3.64557, 0.141683)
(3.72152, 0.151204)
(3.79747, 0.159488)
(3.87342, 0.168074)
(3.94937, 0.176069)
(4.02532, 0.181836)
(4.10127, 0.17962)
(4.17722, 0.190753)
(4.25316, 0.196045)
(4.32911, 0.208447)
(4.40506, 0.217248)
(4.48101, 0.230465)
(4.55696, 0.24507)
(4.63291, 0.262278)
(4.70886, 0.276474)
(4.78481, 0.290437)
(4.86076, 0.306218)
(4.93671, 0.313322)
(5.01266, 0.313942)
(5.08861, 0.322241)
(5.16456, 0.325817)
(5.24051, 0.331322)
(5.31646, 0.334885)
(5.39241, 0.342081)
(5.46835, 0.355119)
(5.5443, 0.36211)
(5.62025, 0.365333)
(5.6962, 0.370828)
(5.77215, 0.396857)
(5.8481, 0.422957)
(5.92405, 0.438525)
(6, 0.445654)
(6.07595, 0.458441)
(6.1519, 0.469631)
(6.22785, 0.477511)
(6.3038, 0.493403)
(6.37975, 0.506758)
(6.4557, 0.52036)
(6.53165, 0.526457)
(6.60759, 0.527823)
(6.68354, 0.529534)
(6.75949, 0.536248)
(6.83544, 0.539985)
(6.91139, 0.537447)
(6.98734, 0.537021)
(7.06329, 0.538552)
(7.13924, 0.542076)
(7.21519, 0.555873)
(7.29114, 0.565258)
(7.36709, 0.570086)
(7.44304, 0.568354)
(7.51899, 0.564083)
(7.59494, 0.556542)
(7.67089, 0.550883)
(7.74684, 0.539915)
(7.82278, 0.522034)
(7.89873, 0.513526)
(7.97468, 0.508907)
(8.05063, 0.507428)
(8.12658, 0.507708)
(8.20253, 0.509827)
(8.27848, 0.50979)
(8.35443, 0.508528)
(8.43038, 0.506319)
(8.50633, 0.50676)
(8.58228, 0.505766)
(8.65823, 0.502752)
(8.73418, 0.499046)
(8.81013, 0.495937)
(8.88608, 0.495072)
(8.96203, 0.49616)
(9.03798, 0.495806)
(9.11392, 0.494198)
(9.18987, 0.491328)
(9.26582, 0.489998)
(9.34177, 0.487206)
(9.41772, 0.486715)
(9.49367, 0.485575)
(9.56962, 0.485177)
(9.64557, 0.484552)
(9.72152, 0.48635)
(9.79747, 0.489399)
(9.87342, 0.48878)
(9.94937, 0.491226)
(10.0253, 0.49115)
(10.1013, 0.493866)
(10.1772, 0.496089)
(10.2532, 0.497251)
(10.3291, 0.498055)
(10.4051, 0.501535)
(10.481, 0.503305)
(10.557, 0.504518)
(10.6329, 0.506802)
(10.7089, 0.49915)
(10.7848, 0.495026)
(10.8608, 0.492734)
(10.9367, 0.492098)
(11.0127, 0.491146)
(11.0886, 0.489317)
(11.1646, 0.485468)
(11.2405, 0.487893)
(11.3165, 0.484698)
(11.3924, 0.487418)
(11.4684, 0.490583)
(11.5443, 0.490367)
(11.6203, 0.485133)
(11.6962, 0.479298)
(11.7722, 0.481329)
(11.8481, 0.482698)
(11.9241, 0.483572)
(12, 0.485714)
(12.0759, 0.490793)
(12.1519, 0.494466)
(12.2278, 0.495108)
(12.3038, 0.500567)
(12.3797, 0.499274)
(12.4557, 0.501446)
(12.5316, 0.500149)
(12.6076, 0.498714)
(12.6835, 0.495552)
(12.7595, 0.495031)
(12.8354, 0.498878)
(12.9114, 0.50281)
(12.9873, 0.506557)
(13.0633, 0.505471)
(13.1392, 0.506883)
(13.2152, 0.508413)
(13.2911, 0.510448)
(13.3671, 0.510198)
(13.443, 0.508759)
(13.519, 0.510056)
(13.5949, 0.515399)
(13.6709, 0.518008)
(13.7468, 0.518919)
(13.8228, 0.518828)
(13.8987, 0.516723)
(13.9747, 0.518693)
(14.0506, 0.520094)
(14.1266, 0.520834)
(14.2025, 0.520649)
(14.2785, 0.517082)
(14.3544, 0.514672)
(14.4304, 0.513516)
(14.5063, 0.511989)
(14.5823, 0.512593)
(14.6582, 0.512297)
(14.7342, 0.51429)
(14.8101, 0.508579)
(14.8861, 0.5035)
(14.962, 0.498719)
(15.038, 0.496571)
(15.1139, 0.494725)
(15.1899, 0.493813)
(15.2658, 0.494195)
(15.3418, 0.494112)
(15.4177, 0.495877)
(15.4937, 0.497237)
(15.5696, 0.495113)
(15.6456, 0.49757)
(15.7215, 0.496113)
(15.7975, 0.493938)
(15.8734, 0.490729)
(15.9494, 0.487005)
(16.0253, 0.485955)
(16.1013, 0.484547)
(16.1772, 0.486155)
(16.2532, 0.487876)
(16.3291, 0.489188)
(16.4051, 0.489922)
(16.481, 0.489735)
(16.557, 0.486314)
(16.6329, 0.484285)
(16.7089, 0.482697)
(16.7848, 0.481272)
(16.8608, 0.479368)
(16.9367, 0.464358)
(17.0127, 0.45704)
(17.0886, 0.4533)
(17.1646, 0.445861)
(17.2405, 0.442188)
(17.3165, 0.432313)
(17.3924, 0.42466)
(17.4684, 0.415944)
(17.5443, 0.40292)
(17.6203, 0.389571)
(17.6962, 0.377495)
(17.7722, 0.361808)
(17.8481, 0.361627)
(17.9241, 0.359343)
(18, 0.359986)
(18.076, 0.363251)
(18.1519, 0.365358)
(18.2278, 0.356738)
(18.3038, 0.351325)
(18.3797, 0.343545)
(18.4557, 0.338565)
(18.5316, 0.331577)
(18.6076, 0.325755)
(18.6835, 0.315477)
(18.7595, 0.308247)
(18.8354, 0.301163)
(18.9114, 0.295171)
(18.9873, 0.291132)
(19.0633, 0.278527)
(19.1392, 0.270558)
(19.2152, 0.267578)
(19.2911, 0.272099)
(19.3671, 0.271766)
(19.443, 0.264526)
(19.519, 0.263849)
(19.5949, 0.255033)
(19.6709, 0.238691)
(19.7468, 0.227561)
(19.8228, 0.218512)
(19.8987, 0.200931)
(19.9747, 0.17841)
(20.0506, 0.172289)
(20.1266, 0.167877)
(20.2025, 0.164363)
(20.2785, 0.157914)
(20.3544, 0.154541)
(20.4304, 0.147824)
(20.5063, 0.149754)
(20.5823, 0.151262)
(20.6582, 0.154514)
(20.7342, 0.155863)
(20.8101, 0.154174)
(20.8861, 0.154225)
(20.962, 0.153907)
(21.038, 0.151795)
(21.1139, 0.146187)
(21.1899, 0.137709)
(21.2658, 0.125264)
(21.3418, 0.119451)
(21.4177, 0.120633)
(21.4937, 0.121741)
(21.5696, 0.123684)
(21.6456, 0.126508)
(21.7215, 0.125212)
(21.7975, 0.121053)
(21.8734, 0.117942)
(21.9494, 0.116672)
(22.0253, 0.10828)
(22.1013, 0.104473)
(22.1772, 0.0897044)
(22.2532, 0.0707032)
(22.3291, 0.0661218)
(22.4051, 0.0635685)
(22.481, 0.0640336)
(22.557, 0.0662094)
(22.6329, 0.0702598)
(22.7089, 0.0706585)
(22.7848, 0.0732067)
(22.8608, 0.0724612)
(22.9367, 0.0654252)
(23.0127, 0.0571761)
(23.0886, 0.0482952)
(23.1646, 0.0423134)
(23.2405, 0.0395862)
(23.3165, 0.0379206)
(23.3924, 0.0355996)
(23.4684, 0.0298609)
(23.5443, 0.0278119)
(23.6203, 0.0160651)
(23.6962, 0.0104603)
(23.7722, 0.00700214)
(23.8481, 0.00510291)
(23.9241, 0.00488512)
(24, 0.00495402)
(24.076, 0.00580284)
(24.1519, 0.00572824)
(24.2278, 0.00638142)
(24.3038, 0.00651844)
(24.3797, 0.00664977)
(24.4557, 0.00659077)
(24.5316, 0.00600826)
(24.6076, 0.00611584)
(24.6835, 0.00624301)
(24.7595, 0.00628953)
(24.8354, 0.0063109)
(24.9114, 0.00659671)
(24.9873, 0.00659008)
(25.0633, 0.00639381)
(25.1392, 0.00648375)
(25.2152, 0.00661176)
(25.2911, 0.00649322)
(25.3671, 0.00631355)
(25.443, 0.00604722)
(25.519, 0.00631779)
(25.5949, 0.00639576)
(25.6709, 0.00665706)
(25.7468, 0.00674828)
(25.8228, 0.00485555)
(25.8987, 0.00447415)
(25.9747, 0.00478034)
(26.0506, 0.00248294)
(26.1266, 0.00129605)
(26.2025, 0.00108744)
(26.2785, 0.000997579)
(26.3544, 0.00079928)
(26.4304, 0.000676205)
(26.5063, -0.000402979)
(26.5823, 0.00280497)
(26.6582, 0.0037545)
(26.7342, 0.000664942)
(26.8101, 0.00387012)
(26.8861, 0.00305898)
(26.962, 0.00295232)
(27.038, 0.00445533)
(27.1139, 0.00389048)
(27.1899, 0.000656949)
(27.2658, -0.00144058)
(27.3418, -0.00152573)
(27.4177, 0.0027624)
(27.4937, 0.00407064)
(27.5696, 0.00406594)
(27.6456, 0.00351437)
(27.7215, 0.00347534)
(27.7975, 0.00200163)
(27.8734, 0.00163195)
(27.9494, 0.00161133)
(28.0253, 0.00135009)
(28.1013, 0.00258544)
(28.1772, 0.00367631)
(28.2532, 0.00399252)
(28.3291, 0.00523746)
(28.4051, 0.00153806)
(28.481, 0.000418099)
(28.557, 0.000349841)
(28.6329, 0.00134764)
(28.7089, 0.00433724)
(28.7848, 0.00331194)
(28.8608, 0.00498283)
(28.9367, 0.0039623)
(29.0127, 0.00411579)
(29.0886, 0.00335259)
(29.1646, 0.00225308)
(29.2405, 0.0034392)
(29.3165, 0.00598814)
(29.3924, 0.00408274)
(29.4684, 0.00239835)
(29.5443, 0.00459979)
(29.6203, 0.00580738)
(29.6962, 0.00381588)
(29.7722, 0.00185665)
(29.8481, 0.000577531)
(29.9241, 0.00010038)
(30, -0.000376498)
(30.076, -0.00032419)
(30.1519, -0.00015909)
(30.2278, 0.000467159)
(30.3038, 0.000551011)
(30.3797, 0.000514467)
(30.4557, 0.000624691)
(30.5316, 0.000903017)
(30.6076, 0.00119636)
(30.6835, 0.00159439)
(30.7595, 0.00172655)
};

==> exp_plots/constrained_ws/z_des.tex <==
\addplot[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates {
(0, 0)
(0.0759494, 0)
(0.151899, 0)
(0.227848, 0)
(0.303797, 0)
(0.379747, 0)
(0.455696, 0)
(0.531646, 0)
(0.607595, 0)
(0.683544, 0)
(0.759494, 0)
(0.835443, 0)
(0.911392, 0)
(0.987342, 0)
(1.06329, 0)
(1.13924, 0)
(1.21519, 0)
(1.29114, 0)
(1.36709, 0)
(1.44304, 0)
(1.51899, 0)
(1.59494, 0)
(1.67089, 0)
(1.74684, 0)
(1.82278, 0)
(1.89873, 0)
(1.97468, 0)
(2.05063, 0)
(2.12658, 0)
(2.20253, 0)
(2.27848, 0)
(2.35443, 0)
(2.43038, 0)
(2.50633, 0)
(2.58228, 0)
(2.65823, 0)
(2.73418, 0)
(2.81013, 0)
(2.88608, 0)
(2.96203, 0)
(3.03797, 0)
(3.11392, 0)
(3.18987, 0)
(3.26582, 0)
(3.34177, 0)
(3.41772, 0)
(3.49367, 0)
(3.56962, 0)
(3.64557, 0)
(3.72152, 0)
(3.79747, 0)
(3.87342, 0)
(3.94937, 0)
(4.02532, 0)
(4.10127, 0)
(4.17722, 0)
(4.25316, 0)
(4.32911, 0)
(4.40506, 0)
(4.48101, 0)
(4.55696, 0)
(4.63291, 0)
(4.70886, 0)
(4.78481, 0)
(4.86076, 0)
(4.93671, 0)
(5.01266, 0)
(5.08861, 0)
(5.16456, 0)
(5.24051, 0)
(5.31646, 0)
(5.39241, 0)
(5.46835, 0)
(5.5443, 0)
(5.62025, 0)
(5.6962, 0)
(5.77215, 0)
(5.8481, 0)
(5.92405, 0)
(6, 0)
(6.07595, 0)
(6.1519, 0)
(6.22785, 0)
(6.3038, 0)
(6.37975, 0)
(6.4557, 0)
(6.53165, 0)
(6.60759, 0)
(6.68354, 0)
(6.75949, 0)
(6.83544, 0)
(6.91139, 0)
(6.98734, 0)
(7.06329, 0)
(7.13924, 0.5)
(7.21519, 0.5)
(7.29114, 0.5)
(7.36709, 0.5)
(7.44304, 0.5)
(7.51899, 0.5)
(7.59494, 0.5)
(7.67089, 0.5)
(7.74684, 0.5)
(7.82278, 0.5)
(7.89873, 0.5)
(7.97468, 0.5)
(8.05063, 0.5)
(8.12658, 0.5)
(8.20253, 0.5)
(8.27848, 0.5)
(8.35443, 0.5)
(8.43038, 0.5)
(8.50633, 0.5)
(8.58228, 0.5)
(8.65823, 0.5)
(8.73418, 0.5)
(8.81013, 0.5)
(8.88608, 0.5)
(8.96203, 0.5)
(9.03798, 0.5)
(9.11392, 0.5)
(9.18987, 0.5)
(9.26582, 0.5)
(9.34177, 0.5)
(9.41772, 0.5)
(9.49367, 0.5)
(9.56962, 0.5)
(9.64557, 0.5)
(9.72152, 0.5)
(9.79747, 0.5)
(9.87342, 0.5)
(9.94937, 0.5)
(10.0253, 0.5)
(10.1013, 0.5)
(10.1772, 0.5)
(10.2532, 0.5)
(10.3291, 0.5)
(10.4051, 0.5)
(10.481, 0.5)
(10.557, 0.5)
(10.6329, 0.5)
(10.7089, 0.5)
(10.7848, 0.5)
(10.8608, 0.5)
(10.9367, 0.5)
(11.0127, 0.5)
(11.0886, 0.5)
(11.1646, 0.5)
(11.2405, 0.5)
(11.3165, 0.5)
(11.3924, 0.5)
(11.4684, 0.5)
(11.5443, 0.5)
(11.6203, 0.5)
(11.6962, 0.5)
(11.7722, 0.5)
(11.8481, 0.5)
(11.9241, 0.5)
(12, 0.5)
(12.0759, 0.5)
(12.1519, 0.5)
(12.2278, 0.5)
(12.3038, 0.5)
(12.3797, 0.5)
(12.4557, 0.5)
(12.5316, 0.5)
(12.6076, 0.5)
(12.6835, 0.5)
(12.7595, 0.5)
(12.8354, 0.5)
(12.9114, 0.5)
(12.9873, 0.5)
(13.0633, 0.5)
(13.1392, 0.5)
(13.2152, 0.5)
(13.2911, 0.5)
(13.3671, 0.5)
(13.443, 0.5)
(13.519, 0.5)
(13.5949, 0.5)
(13.6709, 0.5)
(13.7468, 0.5)
(13.8228, 0.5)
(13.8987, 0.5)
(13.9747, 0.5)
(14.0506, 0.5)
(14.1266, 0.5)
(14.2025, 0.5)
(14.2785, 0.5)
(14.3544, 0.5)
(14.4304, 0.5)
(14.5063, 0.5)
(14.5823, 0.5)
(14.6582, 0.5)
(14.7342, 0.5)
(14.8101, 0.5)
(14.8861, 0.5)
(14.962, 0.5)
(15.038, 0.5)
(15.1139, 0.5)
(15.1899, 0.5)
(15.2658, 0.5)
(15.3418, 0.5)
(15.4177, 0.5)
(15.4937, 0.5)
(15.5696, 0.5)
(15.6456, 0.5)
(15.7215, 0.5)
(15.7975, 0.5)
(15.8734, 0.5)
(15.9494, 0.5)
(16.0253, 0.5)
(16.1013, 0.5)
(16.1772, 0.5)
(16.2532, 0.5)
(16.3291, 0.5)
(16.4051, 0.5)
(16.481, 0.5)
(16.557, 0.5)
(16.6329, 0.5)
(16.7089, 0.5)
(16.7848, 0.5)
(16.8608, 0.5)
(16.9367, 0.5)
(17.0127, 0.5)
(17.0886, 0)
(17.1646, 0)
(17.2405, 0)
(17.3165, 0)
(17.3924, 0)
(17.4684, 0)
(17.5443, 0)
(17.6203, 0)
(17.6962, 0)
(17.7722, 0)
(17.8481, 0)
(17.9241, 0)
(18, 0)
(18.076, 0)
(18.1519, 0)
(18.2278, 0)
(18.3038, 0)
(18.3797, 0)
(18.4557, 0)
(18.5316, 0)
(18.6076, 0)
(18.6835, 0)
(18.7595, 0)
(18.8354, 0)
(18.9114, 0)
(18.9873, 0)
(19.0633, 0)
(19.1392, 0)
(19.2152, 0)
(19.2911, 0)
(19.3671, 0)
(19.443, 0)
(19.519, 0)
(19.5949, 0)
(19.6709, 0)
(19.7468, 0)
(19.8228, 0)
(19.8987, 0)
(19.9747, 0)
(20.0506, 0)
(20.1266, 0)
(20.2025, 0)
(20.2785, 0)
(20.3544, 0)
(20.4304, 0)
(20.5063, 0)
(20.5823, 0)
(20.6582, 0)
(20.7342, 0)
(20.8101, 0)
(20.8861, 0)
(20.962, 0)
(21.038, 0)
(21.1139, 0)
(21.1899, 0)
(21.2658, 0)
(21.3418, 0)
(21.4177, 0)
(21.4937, 0)
(21.5696, 0)
(21.6456, 0)
(21.7215, 0)
(21.7975, 0)
(21.8734, 0)
(21.9494, 0)
(22.0253, 0)
(22.1013, 0)
(22.1772, 0)
(22.2532, 0)
(22.3291, 0)
(22.4051, 0)
(22.481, 0)
(22.557, 0)
(22.6329, 0)
(22.7089, 0)
(22.7848, 0)
(22.8608, 0)
(22.9367, 0)
(23.0127, 0)
(23.0886, 0)
(23.1646, 0)
(23.2405, 0)
(23.3165, 0)
(23.3924, 0)
(23.4684, 0)
(23.5443, 0)
(23.6203, 0)
(23.6962, 0)
(23.7722, 0)
(23.8481, 0)
(23.9241, 0)
(24, 0)
(24.076, 0)
(24.1519, 0)
(24.2278, 0)
(24.3038, 0)
(24.3797, 0)
(24.4557, 0)
(24.5316, 0)
(24.6076, 0)
(24.6835, 0)
(24.7595, 0)
(24.8354, 0)
(24.9114, 0)
(24.9873, 0)
(25.0633, 0)
(25.1392, 0)
(25.2152, 0)
(25.2911, 0)
(25.3671, 0)
(25.443, 0)
(25.519, 0)
(25.5949, 0)
(25.6709, 0)
(25.7468, 0)
(25.8228, 0)
(25.8987, 0)
(25.9747, 0)
(26.0506, 0)
(26.1266, 0)
(26.2025, 0)
(26.2785, 0)
(26.3544, 0)
(26.4304, 0)
(26.5063, 0)
(26.5823, 0)
(26.6582, 0)
(26.7342, 0)
(26.8101, 0)
(26.8861, 0)
(26.962, 0)
(27.038, 0)
(27.1139, 0)
(27.1899, 0)
(27.2658, 0)
(27.3418, 0)
(27.4177, 0)
(27.4937, 0)
(27.5696, 0)
(27.6456, 0)
(27.7215, 0)
(27.7975, 0)
(27.8734, 0)
(27.9494, 0)
(28.0253, 0)
(28.1013, 0)
(28.1772, 0)
(28.2532, 0)
(28.3291, 0)
(28.4051, 0)
(28.481, 0)
(28.557, 0)
(28.6329, 0)
(28.7089, 0)
(28.7848, 0)
(28.8608, 0)
(28.9367, 0)
(29.0127, 0)
(29.0886, 0)
(29.1646, 0)
(29.2405, 0)
(29.3165, 0)
(29.3924, 0)
(29.4684, 0)
(29.5443, 0)
(29.6203, 0)
(29.6962, 0)
(29.7722, 0)
(29.8481, 0)
(29.9241, 0)
(30, 0)
(30.076, 0)
(30.1519, 0)
(30.2278, 0)
(30.3038, 0)
(30.3797, 0)
(30.4557, 0)
(30.5316, 0)
(30.6076, 0)
(30.6835, 0)
(30.7595, 0)
(30.8354, 0)
(30.9114, 0)
(30.9873, 0)
(31.0633, 0)
(31.1392, 0)
(31.2152, 0)
(31.2911, 0)
(31.3671, 0)
(31.443, 0)
(31.519, 0)
(31.5949, 0)
(31.6709, 0)
(31.7468, 0)
(31.8228, 0)
(31.8987, 0)
(31.9747, 0)
(32.0506, 0)
};

==> exp_plots/disturb_rej__tmaf_vs_da/z_da.tex <==
\addplot[
    fill=white!60!clr1,draw = clr1,opacity=\opacty,
    line width= \linew pt,
    forget plot
    ]
 %%
coordinates {
(0, 0)
(0, 0.471387)
(0.00202737, 0.48262)
(0.00405474, 0.486467)
(0.00608211, 0.488517)
(0.00810948, 0.490497)
(0.0101368, 0.487741)
(0.0121642, 0.486048)
(0.0141916, 0.486095)
(0.016219, 0.48678)
(0.0182463, 0.488558)
(0.0202737, 0.491268)
(0.0223011, 0.490948)
(0.0243284, 0.487946)
(0.0263558, 0.486111)
(0.0283832, 0.483317)
(0.0304105, 0.481825)
(0.0324379, 0.473578)
(0.0344653, 0.46873)
(0.0364927, 0.459516)
(0.03852, 0.456711)
(0.0405474, 0.455482)
(0.0425748, 0.453891)
(0.0446021, 0.454005)
(0.0466295, 0.455106)
(0.0486569, 0.456313)
(0.0506842, 0.45512)
(0.0527116, 0.446292)
(0.054739, 0.438033)
(0.0567663, 0.439949)
(0.0587937, 0.444936)
(0.0608211, 0.44346)
(0.0628485, 0.437291)
(0.0648758, 0.435224)
(0.0669032, 0.433808)
(0.0689306, 0.433393)
(0.0709579, 0.434188)
(0.0729853, 0.432808)
(0.0750127, 0.435335)
(0.07704, 0.438234)
(0.0790674, 0.443265)
(0.0810948, 0.443798)
(0.0831221, 0.443657)
(0.0851495, 0.431689)
(0.0871769, 0.413714)
(0.0892043, 0.396536)
(0.0912316, 0.367508)
(0.093259, 0.335927)
(0.0952864, 0.296951)
(0.0973137, 0.272544)
(0.0993411, 0.250914)
(0.101368, 0.237139)
(0.103396, 0.228207)
(0.105423, 0.227876)
(0.107451, 0.215818)
(0.109478, 0.206176)
(0.111505, 0.206059)
(0.113533, 0.201778)
(0.11556, 0.214435)
(0.117587, 0.21915)
(0.119615, 0.229817)
(0.121642, 0.235599)
(0.12367, 0.241766)
(0.125697, 0.242905)
(0.127724, 0.266884)
(0.129752, 0.284988)
(0.131779, 0.305535)
(0.133806, 0.325163)
(0.135834, 0.336461)
(0.137861, 0.338138)
(0.139888, 0.343769)
(0.141916, 0.35383)
(0.143943, 0.366687)
(0.145971, 0.374858)
(0.147998, 0.384698)
(0.150025, 0.379906)
(0.152053, 0.384558)
(0.15408, 0.381454)
(0.156107, 0.380826)
(0.158135, 0.39832)
(0.160162, 0.400954)
(0.16219, 0.441383)
(0.164217, 0.460321)
(0.166244, 0.47459)
(0.168272, 0.481444)
(0.170299, 0.481081)
(0.172326, 0.4831)
(0.174354, 0.498825)
(0.176381, 0.509661)
(0.178409, 0.52377)
(0.180436, 0.530637)
(0.182463, 0.534517)
(0.184491, 0.539959)
(0.186518, 0.538489)
(0.188545, 0.536754)
(0.190573, 0.528956)
(0.1926, 0.525067)
(0.194627, 0.521767)
(0.196655, 0.520205)
(0.198682, 0.520271)
(0.20071, 0.520275)
(0.202737, 0.521252)
(0.204764, 0.52779)
(0.206792, 0.529019)
(0.208819, 0.534668)
(0.210846, 0.538335)
(0.212874, 0.541914)
(0.214901, 0.538917)
(0.216929, 0.536293)
(0.218956, 0.536289)
(0.220983, 0.533945)
(0.223011, 0.532627)
(0.225038, 0.532812)
(0.227065, 0.533681)
(0.229093, 0.534619)
(0.23112, 0.538073)
(0.233147, 0.537726)
(0.235175, 0.534941)
(0.237202, 0.531903)
(0.23923, 0.52696)
(0.241257, 0.520427)
(0.243284, 0.518789)
(0.245312, 0.441319)
(0.247339, 0.397156)
(0.249366, 0.349347)
(0.251394, 0.295883)
(0.253421, 0.244275)
(0.255449, 0.210114)
(0.257476, 0.210349)
(0.259503, 0.201614)
(0.261531, 0.211941)
(0.263558, 0.207465)
(0.265585, 0.196424)
(0.267613, 0.189694)
(0.26964, 0.184488)
(0.271668, 0.182724)
(0.273695, 0.186692)
(0.275722, 0.188264)
(0.27775, 0.190562)
(0.279777, 0.215269)
(0.281804, 0.228377)
(0.283832, 0.243097)
(0.285859, 0.285658)
(0.287886, 0.306022)
(0.289914, 0.331769)
(0.291941, 0.372853)
(0.293969, 0.398143)
(0.295996, 0.418655)
(0.298023, 0.442004)
(0.300051, 0.452034)
(0.302078, 0.460205)
(0.304105, 0.460335)
(0.306133, 0.481782)
(0.30816, 0.500664)
(0.310188, 0.507659)
(0.312215, 0.522076)
(0.314242, 0.529228)
(0.31627, 0.539896)
(0.318297, 0.548509)
(0.320324, 0.561108)
(0.322352, 0.569295)
(0.324379, 0.577429)
(0.326407, 0.581798)
(0.328434, 0.580969)
(0.330461, 0.579926)
(0.332489, 0.592181)
(0.334516, 0.596402)
(0.336543, 0.598734)
(0.338571, 0.604943)
(0.340598, 0.611596)
(0.342625, 0.614478)
(0.344653, 0.614928)
(0.34668, 0.614788)
(0.348708, 0.617065)
(0.350735, 0.617576)
(0.352762, 0.617431)
(0.35479, 0.615707)
(0.356817, 0.615198)
(0.358844, 0.626247)
(0.360872, 0.623066)
(0.362899, 0.626832)
(0.364927, 0.617563)
(0.366954, 0.608584)
(0.368981, 0.595726)
(0.371009, 0.59052)
(0.373036, 0.58699)
(0.375063, 0.582998)
(0.377091, 0.577)
(0.379118, 0.57347)
(0.381145, 0.569723)
(0.383173, 0.56427)
(0.3852, 0.558613)
(0.387228, 0.553027)
(0.389255, 0.5192)
(0.391282, 0.488606)
(0.39331, 0.421256)
(0.395337, 0.375705)
(0.397364, 0.323283)
(0.399392, 0.27494)
(0.401419, 0.245545)
(0.403447, 0.216396)
(0.405474, 0.20855)
(0.407501, 0.196627)
(0.409529, 0.205725)
(0.411556, 0.202103)
(0.413583, 0.206198)
(0.415611, 0.213774)
(0.417638, 0.212883)
(0.419666, 0.216638)
(0.421693, 0.226807)
(0.42372, 0.235587)
(0.425748, 0.261282)
(0.427775, 0.287619)
(0.429802, 0.301348)
(0.43183, 0.317163)
(0.433857, 0.337651)
(0.435884, 0.365633)
(0.437912, 0.390369)
(0.439939, 0.420335)
(0.441967, 0.437359)
(0.443994, 0.441135)
(0.446021, 0.450155)
(0.448049, 0.471529)
(0.450076, 0.488617)
(0.452103, 0.501422)
(0.454131, 0.516639)
(0.456158, 0.526612)
(0.458185, 0.541136)
(0.460213, 0.550411)
(0.46224, 0.558972)
(0.464268, 0.557617)
(0.466295, 0.56366)
(0.468322, 0.568547)
(0.47035, 0.576678)
(0.472377, 0.588824)
(0.474404, 0.599636)
(0.476432, 0.610645)
(0.478459, 0.619334)
(0.480487, 0.621969)
(0.482514, 0.624461)
(0.484541, 0.627887)
(0.486569, 0.632592)
(0.488596, 0.634106)
(0.490623, 0.6312)
(0.492651, 0.630503)
(0.494678, 0.630698)
(0.496706, 0.631186)
(0.498733, 0.630119)
(0.50076, 0.628957)
(0.502788, 0.629183)
(0.504815, 0.628485)
(0.506842, 0.629062)
(0.50887, 0.626415)
(0.510897, 0.604171)
(0.512924, 0.590024)
(0.514952, 0.575681)
(0.516979, 0.568816)
(0.519007, 0.55702)
(0.521034, 0.539342)
(0.523061, 0.526205)
(0.525089, 0.513521)
(0.527116, 0.504984)
(0.529143, 0.500787)
(0.531171, 0.497661)
(0.533198, 0.50044)
(0.535226, 0.50087)
(0.537253, 0.504426)
(0.53928, 0.502526)
(0.541308, 0.49893)
(0.543335, 0.493018)
(0.545362, 0.491081)
(0.54739, 0.490949)
(0.549417, 0.490341)
(0.551444, 0.489927)
(0.553472, 0.494891)
(0.555499, 0.495461)
(0.557527, 0.499473)
(0.559554, 0.504566)
(0.561581, 0.509656)
(0.563609, 0.512825)
(0.565636, 0.512264)
(0.567663, 0.513622)
(0.569691, 0.513116)
(0.571718, 0.513879)
(0.573746, 0.513525)
(0.575773, 0.51352)
(0.5778, 0.514086)
(0.579828, 0.514033)
(0.581855, 0.514233)
(0.583882, 0.510894)
(0.58591, 0.512164)
(0.587937, 0.512913)
(0.589965, 0.513496)
(0.591992, 0.510413)
(0.594019, 0.509538)
(0.596047, 0.508795)
(0.598074, 0.508577)
(0.600101, 0.508879)
(0.602129, 0.495174)
(0.604156, 0.490376)
(0.606184, 0.494491)
(0.608211, 0.490915)
(0.610238, 0.487129)
(0.612266, 0.484633)
(0.614293, 0.484123)
(0.61632, 0.480767)
(0.618348, 0.479441)
(0.620375, 0.478948)
(0.622402, 0.475018)
(0.62443, 0.470749)
(0.626457, 0.468638)
(0.628485, 0.467811)
(0.630512, 0.464894)
(0.632539, 0.461674)
(0.634567, 0.462015)
(0.636594, 0.46233)
(0.638621, 0.461744)
(0.640649, 0.459311)
(0.642676, 0.457933)
(0.644704, 0.454815)
(0.646731, 0.451971)
(0.648758, 0.449688)
(0.650786, 0.446879)
(0.652813, 0.431405)
(0.65484, 0.424391)
(0.656868, 0.41575)
(0.658895, 0.406483)
(0.660922, 0.400601)
(0.66295, 0.398494)
(0.664977, 0.397411)
(0.667005, 0.396902)
(0.669032, 0.398514)
(0.671059, 0.398427)
(0.673087, 0.397404)
(0.675114, 0.395572)
(0.677141, 0.392574)
(0.679169, 0.389117)
(0.681196, 0.381666)
(0.683224, 0.374611)
(0.685251, 0.369487)
(0.687278, 0.364671)
(0.689306, 0.361312)
(0.691333, 0.363956)
(0.69336, 0.36022)
(0.695388, 0.357309)
(0.697415, 0.363216)
(0.699443, 0.364119)
(0.70147, 0.363663)
(0.703497, 0.351886)
(0.705525, 0.343673)
(0.707552, 0.340889)
(0.709579, 0.337006)
(0.711607, 0.339042)
(0.713634, 0.341276)
(0.715661, 0.347587)
(0.717689, 0.345547)
(0.719716, 0.351842)
(0.721744, 0.356217)
(0.723771, 0.36015)
(0.725798, 0.361653)
(0.727826, 0.363326)
(0.729853, 0.364623)
(0.73188, 0.368353)
(0.733908, 0.368838)
(0.735935, 0.366791)
(0.737962, 0.375383)
(0.73999, 0.378488)
(0.742017, 0.395964)
(0.744045, 0.404431)
(0.746072, 0.409131)
(0.748099, 0.417252)
(0.750127, 0.428311)
(0.752154, 0.426456)
(0.754181, 0.415889)
(0.756209, 0.406454)
(0.758236, 0.373282)
(0.760264, 0.355897)
(0.762291, 0.323055)
(0.764318, 0.310292)
(0.766346, 0.285542)
(0.768373, 0.271671)
(0.7704, 0.265736)
(0.772428, 0.261662)
(0.774455, 0.256901)
(0.776483, 0.24688)
(0.77851, 0.236862)
(0.780537, 0.229683)
(0.782565, 0.227656)
(0.784592, 0.237005)
(0.786619, 0.249336)
(0.788647, 0.257938)
(0.790674, 0.26588)
(0.792701, 0.281916)
(0.794729, 0.294363)
(0.796756, 0.307233)
(0.798784, 0.326063)
(0.800811, 0.34211)
(0.802838, 0.359679)
(0.804866, 0.378594)
(0.806893, 0.388621)
(0.80892, 0.40442)
(0.810948, 0.414657)
(0.812975, 0.412139)
(0.815003, 0.420334)
(0.81703, 0.437527)
(0.819057, 0.460918)
(0.821085, 0.476799)
(0.823112, 0.493875)
(0.825139, 0.506183)
(0.827167, 0.519236)
(0.829194, 0.534974)
(0.831222, 0.54308)
(0.833249, 0.549313)
(0.835276, 0.557589)
(0.837304, 0.563763)
(0.839331, 0.569419)
(0.841358, 0.579113)
(0.843386, 0.593817)
(0.845413, 0.600552)
(0.84744, 0.616684)
(0.849468, 0.629222)
(0.851495, 0.636772)
(0.853523, 0.644464)
(0.85555, 0.64943)
(0.857577, 0.65635)
(0.859605, 0.657194)
(0.861632, 0.656091)
(0.863659, 0.659033)
(0.865687, 0.659628)
(0.867714, 0.661108)
(0.869741, 0.662049)
(0.871769, 0.664745)
(0.873796, 0.665135)
(0.875824, 0.66581)
(0.877851, 0.664435)
(0.879878, 0.665339)
(0.881906, 0.65784)
(0.883933, 0.650897)
(0.885961, 0.636819)
(0.887988, 0.627022)
(0.890015, 0.616047)
(0.892043, 0.609886)
(0.89407, 0.60815)
(0.896097, 0.604597)
(0.898125, 0.597575)
(0.900152, 0.59646)
(0.902179, 0.601825)
(0.904207, 0.605427)
(0.906234, 0.614258)
(0.908262, 0.616884)
(0.910289, 0.615053)
(0.912316, 0.613175)
(0.914344, 0.609874)
(0.916371, 0.607766)
(0.918398, 0.606905)
(0.920426, 0.605669)
(0.922453, 0.603971)
(0.92448, 0.599788)
(0.926508, 0.596279)
(0.928535, 0.59023)
(0.930563, 0.58655)
(0.93259, 0.582942)
(0.934617, 0.580185)
(0.936645, 0.577335)
(0.938672, 0.575889)
(0.940699, 0.571356)
(0.942727, 0.559837)
(0.944754, 0.548946)
(0.946782, 0.540501)
(0.948809, 0.532357)
(0.950836, 0.523995)
(0.952864, 0.514864)
(0.954891, 0.511186)
(0.956918, 0.506779)
(0.958946, 0.500207)
(0.960973, 0.494788)
(0.963001, 0.49203)
(0.965028, 0.49382)
(0.967055, 0.493467)
(0.969083, 0.491022)
(0.97111, 0.489673)
(0.973137, 0.491748)
(0.975165, 0.494213)
(0.977192, 0.493941)
(0.979219, 0.48667)
(0.981247, 0.487259)
(0.983274, 0.493195)
(0.985302, 0.493737)
(0.987329, 0.493635)
(0.989356, 0.494766)
(0.991384, 0.495893)
(0.993411, 0.502649)
(0.995438, 0.505634)
(0.997466, 0.507147)
(0.999493, 0.508484)
(1.0, 0)
};

==> exp_plots/disturb_rej__tmaf_vs_da/z_des.tex <==
\addplot[
    fill=none,draw = desclr,
    line width= \linew +0.2 pt,
    dashed
    ]
 %%
coordinates {
(0, 0.5)
(1,0.5)
};

==> exp_plots/disturb_rej__tmaf_vs_da/z_tmaf.tex <==
\addplot[
    fill=white!60!clr4,draw = clr4,opacity=\opacty,
    line width= \linew pt,
    forget plot
    ]
 %%
coordinates {
(0, 0)
(0, 0.534432)
(0.00202737, 0.532226)
(0.00405474, 0.52958)
(0.00608211, 0.524937)
(0.00810948, 0.520879)
(0.0101368, 0.518495)
(0.0121642, 0.51736)
(0.0141916, 0.515877)
(0.016219, 0.517038)
(0.0182463, 0.517156)
(0.0202737, 0.518119)
(0.0223011, 0.51849)
(0.0243284, 0.512876)
(0.0263558, 0.502944)
(0.0283832, 0.500813)
(0.0304105, 0.494727)
(0.0324379, 0.492001)
(0.0344653, 0.489395)
(0.0364927, 0.48831)
(0.03852, 0.486388)
(0.0405474, 0.483601)
(0.0425748, 0.476227)
(0.0446021, 0.465726)
(0.0466295, 0.46626)
(0.0486569, 0.467451)
(0.0506842, 0.466772)
(0.0527116, 0.466353)
(0.054739, 0.466215)
(0.0567663, 0.463538)
(0.0587937, 0.462033)
(0.0608211, 0.460509)
(0.0628485, 0.46006)
(0.0648758, 0.45997)
(0.0669032, 0.461419)
(0.0689306, 0.460643)
(0.0709579, 0.460441)
(0.0729853, 0.459269)
(0.0750127, 0.45829)
(0.07704, 0.459849)
(0.0790674, 0.463268)
(0.0810948, 0.466325)
(0.0831221, 0.468403)
(0.0851495, 0.469353)
(0.0871769, 0.469825)
(0.0892043, 0.469068)
(0.0912316, 0.469339)
(0.093259, 0.468531)
(0.0952864, 0.468861)
(0.0973137, 0.46929)
(0.0993411, 0.471729)
(0.101368, 0.478081)
(0.103396, 0.483562)
(0.105423, 0.489466)
(0.107451, 0.492055)
(0.109478, 0.488326)
(0.111505, 0.488836)
(0.113533, 0.49031)
(0.11556, 0.491397)
(0.117587, 0.493124)
(0.119615, 0.495545)
(0.121642, 0.495981)
(0.12367, 0.497164)
(0.125697, 0.498326)
(0.127724, 0.502486)
(0.129752, 0.501725)
(0.131779, 0.498868)
(0.133806, 0.492272)
(0.135834, 0.487446)
(0.137861, 0.482178)
(0.139888, 0.490009)
(0.141916, 0.488419)
(0.143943, 0.488531)
(0.145971, 0.486843)
(0.147998, 0.485679)
(0.150025, 0.482552)
(0.152053, 0.481151)
(0.15408, 0.477635)
(0.156107, 0.486967)
(0.158135, 0.487965)
(0.160162, 0.488896)
(0.16219, 0.490796)
(0.164217, 0.495117)
(0.166244, 0.49775)
(0.168272, 0.501253)
(0.170299, 0.510447)
(0.172326, 0.523668)
(0.174354, 0.529849)
(0.176381, 0.527231)
(0.178409, 0.529477)
(0.180436, 0.520891)
(0.182463, 0.518009)
(0.184491, 0.519028)
(0.186518, 0.521091)
(0.188545, 0.520282)
(0.190573, 0.520342)
(0.1926, 0.523264)
(0.194627, 0.525874)
(0.196655, 0.525854)
(0.198682, 0.524772)
(0.20071, 0.516965)
(0.202737, 0.508052)
(0.204764, 0.503431)
(0.206792, 0.496716)
(0.208819, 0.475015)
(0.210846, 0.455172)
(0.212874, 0.44967)
(0.214901, 0.453457)
(0.216929, 0.457017)
(0.218956, 0.480337)
(0.220983, 0.488619)
(0.223011, 0.492166)
(0.225038, 0.492848)
(0.227065, 0.489643)
(0.229093, 0.486238)
(0.23112, 0.483847)
(0.233147, 0.478443)
(0.235175, 0.478078)
(0.237202, 0.478324)
(0.23923, 0.483632)
(0.241257, 0.487198)
(0.243284, 0.490986)
(0.245312, 0.490602)
(0.247339, 0.49066)
(0.249366, 0.499245)
(0.251394, 0.503354)
(0.253421, 0.506893)
(0.255449, 0.509125)
(0.257476, 0.508666)
(0.259503, 0.508919)
(0.261531, 0.510285)
(0.263558, 0.511704)
(0.265585, 0.512157)
(0.267613, 0.511646)
(0.26964, 0.510925)
(0.271668, 0.511572)
(0.273695, 0.51481)
(0.275722, 0.516214)
(0.27775, 0.514962)
(0.279777, 0.515129)
(0.281804, 0.512286)
(0.283832, 0.507925)
(0.285859, 0.50454)
(0.287886, 0.497568)
(0.289914, 0.493261)
(0.291941, 0.489405)
(0.293969, 0.488458)
(0.295996, 0.482023)
(0.298023, 0.481759)
(0.300051, 0.481027)
(0.302078, 0.476196)
(0.304105, 0.474785)
(0.306133, 0.474814)
(0.30816, 0.47314)
(0.310188, 0.475001)
(0.312215, 0.480132)
(0.314242, 0.481564)
(0.31627, 0.484873)
(0.318297, 0.490171)
(0.320324, 0.490491)
(0.322352, 0.491679)
(0.324379, 0.490747)
(0.326407, 0.497084)
(0.328434, 0.499079)
(0.330461, 0.498352)
(0.332489, 0.497246)
(0.334516, 0.499727)
(0.336543, 0.500697)
(0.338571, 0.500375)
(0.340598, 0.500447)
(0.342625, 0.500838)
(0.344653, 0.502557)
(0.34668, 0.502378)
(0.348708, 0.502245)
(0.350735, 0.50261)
(0.352762, 0.501994)
(0.35479, 0.501877)
(0.356817, 0.500244)
(0.358844, 0.503982)
(0.360872, 0.506761)
(0.362899, 0.509388)
(0.364927, 0.508595)
(0.366954, 0.505552)
(0.368981, 0.509326)
(0.371009, 0.51013)
(0.373036, 0.511099)
(0.375063, 0.506767)
(0.377091, 0.499979)
(0.379118, 0.494395)
(0.381145, 0.455016)
(0.383173, 0.434612)
(0.3852, 0.426874)
(0.387228, 0.431887)
(0.389255, 0.432165)
(0.391282, 0.436991)
(0.39331, 0.466687)
(0.395337, 0.479233)
(0.397364, 0.497461)
(0.399392, 0.506174)
(0.401419, 0.52054)
(0.403447, 0.528127)
(0.405474, 0.528618)
(0.407501, 0.530836)
(0.409529, 0.539122)
(0.411556, 0.542897)
(0.413583, 0.540786)
(0.415611, 0.543948)
(0.417638, 0.543927)
(0.419666, 0.545521)
(0.421693, 0.546289)
(0.42372, 0.553361)
(0.425748, 0.559891)
(0.427775, 0.56041)
(0.429802, 0.562277)
(0.43183, 0.563008)
(0.433857, 0.560682)
(0.435884, 0.560312)
(0.437912, 0.557736)
(0.439939, 0.556757)
(0.441967, 0.555445)
(0.443994, 0.561555)
(0.446021, 0.570269)
(0.448049, 0.571485)
(0.450076, 0.567388)
(0.452103, 0.566502)
(0.454131, 0.566216)
(0.456158, 0.563057)
(0.458185, 0.557315)
(0.460213, 0.555792)
(0.46224, 0.558205)
(0.464268, 0.556957)
(0.466295, 0.553243)
(0.468322, 0.552873)
(0.47035, 0.552324)
(0.472377, 0.551019)
(0.474404, 0.545848)
(0.476432, 0.542258)
(0.478459, 0.540794)
(0.480487, 0.538693)
(0.482514, 0.524654)
(0.484541, 0.518141)
(0.486569, 0.514935)
(0.488596, 0.513933)
(0.490623, 0.509611)
(0.492651, 0.513638)
(0.494678, 0.478415)
(0.496706, 0.467883)
(0.498733, 0.453444)
(0.50076, 0.447132)
(0.502788, 0.431719)
(0.504815, 0.421286)
(0.506842, 0.417784)
(0.50887, 0.423994)
(0.510897, 0.431663)
(0.512924, 0.449956)
(0.514952, 0.451546)
(0.516979, 0.460426)
(0.519007, 0.463266)
(0.521034, 0.472771)
(0.523061, 0.485288)
(0.525089, 0.491358)
(0.527116, 0.505935)
(0.529143, 0.512174)
(0.531171, 0.514234)
(0.533198, 0.515515)
(0.535226, 0.51692)
(0.537253, 0.521511)
(0.53928, 0.522401)
(0.541308, 0.521393)
(0.543335, 0.524033)
(0.545362, 0.528272)
(0.54739, 0.527402)
(0.549417, 0.524079)
(0.551444, 0.529216)
(0.553472, 0.532397)
(0.555499, 0.533886)
(0.557527, 0.532776)
(0.559554, 0.531192)
(0.561581, 0.522138)
(0.563609, 0.516352)
(0.565636, 0.512825)
(0.567663, 0.504882)
(0.569691, 0.492819)
(0.571718, 0.485283)
(0.573746, 0.476794)
(0.575773, 0.476897)
(0.5778, 0.479951)
(0.579828, 0.477104)
(0.581855, 0.471393)
(0.583882, 0.465801)
(0.58591, 0.464249)
(0.587937, 0.468113)
(0.589965, 0.464838)
(0.591992, 0.46305)
(0.594019, 0.461602)
(0.596047, 0.460431)
(0.598074, 0.460773)
(0.600101, 0.462086)
(0.602129, 0.46569)
(0.604156, 0.467676)
(0.606184, 0.471291)
(0.608211, 0.475306)
(0.610238, 0.477422)
(0.612266, 0.478356)
(0.614293, 0.480969)
(0.61632, 0.48319)
(0.618348, 0.487769)
(0.620375, 0.489653)
(0.622402, 0.491142)
(0.62443, 0.492397)
(0.626457, 0.494935)
(0.628485, 0.49433)
(0.630512, 0.494325)
(0.632539, 0.494423)
(0.634567, 0.490546)
(0.636594, 0.49173)
(0.638621, 0.492321)
(0.640649, 0.493002)
(0.642676, 0.493465)
(0.644704, 0.493039)
(0.646731, 0.492176)
(0.648758, 0.492159)
(0.650786, 0.488928)
(0.652813, 0.480884)
(0.65484, 0.477176)
(0.656868, 0.475852)
(0.658895, 0.475491)
(0.660922, 0.476961)
(0.66295, 0.478305)
(0.664977, 0.479513)
(0.667005, 0.482095)
(0.669032, 0.483112)
(0.671059, 0.485843)
(0.673087, 0.48776)
(0.675114, 0.48849)
(0.677141, 0.490488)
(0.679169, 0.491192)
(0.681196, 0.491643)
(0.683224, 0.487361)
(0.685251, 0.484953)
(0.687278, 0.475353)
(0.689306, 0.471434)
(0.691333, 0.470774)
(0.69336, 0.469688)
(0.695388, 0.470461)
(0.697415, 0.469523)
(0.699443, 0.470484)
(0.70147, 0.472942)
(0.703497, 0.474343)
(0.705525, 0.476639)
(0.707552, 0.472109)
(0.709579, 0.47517)
(0.711607, 0.473217)
(0.713634, 0.473442)
(0.715661, 0.472907)
(0.717689, 0.471957)
(0.719716, 0.472718)
(0.721744, 0.476875)
(0.723771, 0.479203)
(0.725798, 0.479124)
(0.727826, 0.478787)
(0.729853, 0.476699)
(0.73188, 0.475724)
(0.733908, 0.475327)
(0.735935, 0.47568)
(0.737962, 0.47304)
(0.73999, 0.471763)
(0.742017, 0.473993)
(0.744045, 0.47201)
(0.746072, 0.468802)
(0.748099, 0.46914)
(0.750127, 0.477852)
(0.752154, 0.500569)
(0.754181, 0.507633)
(0.756209, 0.512337)
(0.758236, 0.513804)
(0.760264, 0.514019)
(0.762291, 0.514804)
(0.764318, 0.516531)
(0.766346, 0.517828)
(0.768373, 0.515547)
(0.7704, 0.51807)
(0.772428, 0.515763)
(0.774455, 0.516103)
(0.776483, 0.517289)
(0.77851, 0.524349)
(0.780537, 0.525271)
(0.782565, 0.530154)
(0.784592, 0.531634)
(0.786619, 0.535275)
(0.788647, 0.537018)
(0.790674, 0.539058)
(0.792701, 0.540318)
(0.794729, 0.540685)
(0.796756, 0.538197)
(0.798784, 0.538074)
(0.800811, 0.537933)
(0.802838, 0.536267)
(0.804866, 0.536166)
(0.806893, 0.538461)
(0.80892, 0.538462)
(0.810948, 0.54118)
(0.812975, 0.54787)
(0.815003, 0.548481)
(0.81703, 0.546532)
(0.819057, 0.547608)
(0.821085, 0.547633)
(0.823112, 0.546609)
(0.825139, 0.544564)
(0.827167, 0.542439)
(0.829194, 0.543103)
(0.831222, 0.54096)
(0.833249, 0.543411)
(0.835276, 0.543918)
(0.837304, 0.544689)
(0.839331, 0.541247)
(0.841358, 0.539304)
(0.843386, 0.53365)
(0.845413, 0.528295)
(0.84744, 0.522844)
(0.849468, 0.51822)
(0.851495, 0.508044)
(0.853523, 0.504721)
(0.85555, 0.500365)
(0.857577, 0.497117)
(0.859605, 0.491381)
(0.861632, 0.486884)
(0.863659, 0.477443)
(0.865687, 0.474329)
(0.867714, 0.473258)
(0.869741, 0.470766)
(0.871769, 0.471274)
(0.873796, 0.469193)
(0.875824, 0.470219)
(0.877851, 0.470575)
(0.879878, 0.477734)
(0.881906, 0.480299)
(0.883933, 0.484144)
(0.885961, 0.487734)
(0.887988, 0.491562)
(0.890015, 0.494148)
(0.892043, 0.500988)
(0.89407, 0.506423)
(0.896097, 0.510329)
(0.898125, 0.512152)
(0.900152, 0.509844)
(0.902179, 0.501145)
(0.904207, 0.500629)
(0.906234, 0.492007)
(0.908262, 0.489758)
(0.910289, 0.48266)
(0.912316, 0.478717)
(0.914344, 0.463457)
(0.916371, 0.456967)
(0.918398, 0.456672)
(0.920426, 0.454412)
(0.922453, 0.454457)
(0.92448, 0.450697)
(0.926508, 0.448015)
(0.928535, 0.449145)
(0.930563, 0.450682)
(0.93259, 0.450955)
(0.934617, 0.449361)
(0.936645, 0.446892)
(0.938672, 0.443893)
(0.940699, 0.439563)
(0.942727, 0.433724)
(0.944754, 0.423481)
(0.946782, 0.412568)
(0.948809, 0.404632)
(0.950836, 0.398901)
(0.952864, 0.398171)
(0.954891, 0.407334)
(0.956918, 0.414482)
(0.958946, 0.421043)
(0.960973, 0.426282)
(0.963001, 0.430202)
(0.965028, 0.430028)
(0.967055, 0.423243)
(0.969083, 0.419865)
(0.97111, 0.417259)
(0.973137, 0.41624)
(0.975165, 0.412795)
(0.977192, 0.41149)
(0.979219, 0.407391)
(0.981247, 0.418109)
(0.983274, 0.432047)
(0.985302, 0.439588)
(0.987329, 0.452017)
(0.989356, 0.456596)
(0.991384, 0.463401)
(0.993411, 0.470534)
(0.995438, 0.476849)
(0.997466, 0.481091)
(0.999493, 0.484595)
(1.0, 0)
};

==> exp_plots/hover_dyanmic_payload/az.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0.00586733)
(0.2, 0.0082358)
(0.4, 0.0046987)
(0.6, -0.00233035)
(0.8, -0.0103146)
(1, -0.0097921)
(1.2, 0.0118744)
(1.4, 0.0240839)
(1.6, 0.0274357)
(1.8, 0.0287435)
(2, 0.0281571)
(2.2, 0.0152023)
(2.4, -0.00165968)
(2.6, 0.068379)
(2.8, 0.182961)
(3, 0.162903)
(3.2, 0.133635)
(3.4, -0.0545466)
(3.6, -0.0199356)
(3.8, 0.0387907)
(4, 0.00495385)
(4.2, -0.00348105)
(4.4, 0.0282165)
(4.6, 0.0212752)
(4.8, 0.0579598)
(5, 0.00661382)
(5.2, 0.0214939)
(5.4, 0.0340077)
(5.6, -0.0250624)
(5.8, 0.0369287)
(6, 0.012858)
(6.2, -0.0781202)
(6.4, -0.0904475)
(6.6, -0.223665)
(6.8, -0.0561876)
(7, -0.0552077)
(7.2, -0.0710227)
(7.4, -0.0120047)
(7.6, -0.0250502)
(7.8, -0.0804287)
(8, -0.098669)
(8.2, 0.0881763)
(8.4, 0.0169219)
(8.6, -0.0661667)
(8.8, -0.0458939)
(9, -0.036647)
(9.2, -0.0612121)
(9.4, -0.0430978)
(9.6, 0.0311082)
(9.8, 0.03197)
(10, 0.131078)
(10.2, 0.0473505)
(10.4, -0.0125198)
(10.6, 0.0566319)
(10.8, -0.0360754)
(11, -0.0781757)
(11.2, 0.0378269)
(11.4, 0.0700071)
(11.6, 0.041138)
(11.8, 0.0946939)
(12, 0.0231415)
(12.2, -0.0541649)
(12.4, -0.0224027)
(12.6, -0.0235399)
(12.8, -0.131806)
(13, -0.104131)
(13.2, -0.112222)
(13.4, -0.122023)
(13.6, -0.0532888)
(13.8, 0.000105664)
(14, -0.00222671)
(14.2, 0.0375558)
(14.4, 0.0169348)
(14.6, -0.0225252)
(14.8, -0.00435424)
(15, 0.0276428)
(15.2, -0.0286211)
(15.4, -0.0924428)
(15.6, 0.0486867)
(15.8, -0.041691)
(16, -0.00745186)
(16.2, 0.00305331)
(16.4, 0.0546327)
(16.6, 0.0953988)
(16.8, 0.0318794)
(17, 0.073148)
(17.2, 0.0310125)
(17.4, -0.0602616)
(17.6, -0.0735421)
(17.8, -0.0738429)
(18, -0.0931471)
(18.2, -0.0167973)
(18.4, 0.0772586)
(18.6, 0.0555575)
(18.8, -0.0208225)
(19, 0.034136)
(19.2, 0.0419775)
(19.4, 0.0109851)
(19.6, 0.0449682)
(19.8, 0.0573804)
(20, -0.00777174)
(20.2, -0.0912899)
(20.4, -0.0591064)
(20.6, -0.045857)
(20.8, -0.00887294)
(21, 0.0242291)
(21.2, -0.018447)
(21.4, 0.0546987)
(21.6, 0.0524584)
(21.8, 0.110099)
(22, 0.116694)
(22.2, -0.0128512)
(22.4, 0.0202795)
(22.6, 0.0337499)
(22.8, -0.01358)
(23, 0.0256905)
(23.2, 0.0570143)
(23.4, 0.0151201)
(23.6, -0.00175694)
(23.8, 0.0618312)
(24, 0.0466709)
(24.2, 0.0459531)
(24.4, 0.106949)
(24.6, 0.128411)
(24.8, 0.0558381)
(25, -0.0057552)
(25.2, -0.0240339)
(25.4, -0.0427953)
(25.6, -0.0603681)
(25.8, -0.000460256)
(26, -0.0330031)
(26.2, -0.0117955)
(26.4, -0.0110657)
(26.6, -0.0422272)
(26.8, -0.0176432)
(27, -0.0040378)
(27.2, -0.0116215)
(27.4, -0.00663616)
(27.6, 0.00635972)
(27.8, 0.066343)
(28, 0.0379484)
(28.2, 0.044843)
(28.4, -0.0196268)
(28.6, -0.0329911)
(28.8, 0.129656)
(29, 0.133747)
(29.2, -0.0116861)
(29.4, 0.0521671)
(29.6, -0.0668975)
(29.8, -0.0562814)
(30, -0.0929357)
(30.2, -0.0575966)
(30.4, 0.0517948)
(30.6, 0.100966)
(30.8, 0.0380362)
(31, 0.0601748)
(31.2, 0.106229)
(31.4, 0.0810562)
(31.6, 0.000614159)
(31.8, -0.137727)
(32, -0.110977)
(32.2, -0.0834072)
(32.4, -0.113578)
(32.6, -0.029818)
(32.8, -0.0218883)
(33, -0.00467191)
(33.2, 0.0881981)
(33.4, 0.0576003)
(33.6, 0.0410322)
(33.8, 0.0445963)
(34, 0.00778833)
(34.2, 0.0439499)
(34.4, 0.0244668)
(34.6, -0.117106)
(34.8, -0.18462)
(35, -0.0859239)
(35.2, -0.069487)
(35.4, -0.0387098)
(35.6, 0.0187204)
(35.8, 0.0188521)
(36, 0.012824)
(36.2, 0.0520301)
(36.4, 0.0582812)
(36.6, 0.14465)
(36.8, 0.037285)
(37, -0.246769)
(37.2, -0.108942)
(37.4, -0.00359837)
(37.6, -0.0403852)
(37.8, 0.0107493)
(38, 0.0958091)
(38.2, 0.0668947)
(38.4, 0.190893)
(38.6, 0.337451)
(38.8, 0.121146)
(39, 0.056436)
(39.2, -0.0908975)
(39.4, -0.217064)
(39.6, -0.133002)
(39.8, -0.201599)
(40, -0.290931)
(40.2, -0.169261)
(40.4, -0.00370503)
(40.6, 0.05655)
(40.8, -0.0422717)
(41, 0.00319479)
(41.2, 0.134021)
(41.4, 0.245915)
(41.6, 0.11953)
(41.8, 0.0909699)
(42, 0.0589159)
(42.2, -0.242823)
(42.4, -0.137912)
(42.6, 0.0436227)
(42.8, 0.0120839)
(43, -0.105414)
(43.2, -0.0310076)
(43.4, 0.0828165)
(43.6, 0.105478)
(43.8, 0.0543974)
(44, -0.00807903)
(44.2, 0.0517919)
(44.4, 0.0442587)
(44.6, -0.0976942)
(44.8, -0.0830804)
(45, 0.0190617)
(45.2, -0.019038)
(45.4, -0.0270339)
(45.6, -0.0373782)
(45.8, -0.00918626)
(46, -0.0331214)
(46.2, 0.107874)
(46.4, 0.158089)
(46.6, 0.0204496)
(46.8, -0.0482582)
(47, -0.0578866)
(47.2, -0.155993)
(47.4, -0.125832)
(47.6, -0.0431526)
(47.8, -0.108172)
(48, -0.0372057)
(48.2, 0.0355384)
(48.4, -0.0273482)
(48.6, -0.00937838)
(48.8, 0.017099)
(49, 0.043267)
(49.2, 0.0713219)
(49.4, 0.0319862)
(49.6, 0.00306931)
(49.8, 0.0341878)
(50, 0.0590112)
(50.2, 0.014202)
(50.4, 0.0643045)
(50.6, 0.231555)
(50.8, 0.0712788)
(51, 0.00149417)
(51.2, 0.00401292)
(51.4, -0.140864)
(51.6, -0.213717)
(51.8, -0.0743131)
(52, -0.0124359)
(52.2, 0.0780877)
(52.4, 0.0825615)
(52.6, 0.116518)
(52.8, 0.0753684)
(53, 0.0648564)
(53.2, 0.00176533)
(53.4, -0.0514256)
(53.6, -0.0283091)
(53.8, 0.0671422)
(54, -0.00631826)
(54.2, -0.00539479)
(54.4, 0.0412452)
(54.6, -0.0272027)
(54.8, -0.0130776)
(55, 0.00481651)
(55.2, -0.132145)
(55.4, -0.0253123)
(55.6, -0.0197568)
(55.8, -0.0714049)
(56, -0.0142086)
(56.2, 0.015782)
(56.4, 0.0213146)
(56.6, 0.132643)
(56.8, 0.157483)
(57, 0.130619)
(57.2, 0.0560796)
(57.4, 0.0390642)
(57.6, 0.00571816)
(57.8, -0.0482438)
(58, -0.0880932)
(58.2, -0.0807287)
(58.4, -0.187518)
(58.6, -0.104934)
(58.8, 0.0089789)
(59, 0.0201856)
(59.2, 0.0704043)
(59.4, 0.0867343)
(59.6, 0.0320912)
(59.8, -0.0339673)
(60, 0.0102206)
(60.2, 0.0305986)
(60.4, -0.0233591)
(60.6, 0.0653676)
(60.8, 0.0615073)
(61, 0.00400548)
(61.2, -0.0240544)
(61.4, 0.0635985)
(61.6, 0.180701)
(61.8, -0.0258445)
(62, -0.10485)
(62.2, -0.0728216)
(62.4, 0.0708836)
(62.6, -0.0158077)
(62.8, -0.00167488)
(63, 0.0437286)
(63.2, 0.0803335)
(63.4, 0.000431582)
(63.6, -0.16019)
(63.8, -0.135733)
(64, -0.068465)
(64.2, -0.0423841)
(64.4, -0.0088481)
(64.6, 0.0255557)
(64.8, 0.0219962)
(65, 0.0142668)
(65.2, 0.039084)
(65.4, 0.0739849)
(65.6, 0.0809418)
(65.8, -0.199161)
(66, -0.184748)
(66.2, -0.102379)
(66.4, -0.214295)
(66.6, -0.174617)
(66.8, 0.0540395)
(67, 0.160966)
(67.2, 0.261054)
(67.4, 0.135367)
(67.6, -0.00477995)
(67.8, -0.0433069)
(68, -0.0175939)
(68.2, 0.0711565)
(68.4, -0.0165764)
(68.6, 0.00204361)
(68.8, 0.0895925)
(69, 0.0419862)
(69.2, -0.0550501)
(69.4, -0.136159)
(69.6, -0.0228437)
(69.8, 0.0238747)
(70, 0.0190471)
(70.2, 0.0489191)
(70.4, 0.0577793)
(70.6, -0.0265349)
(70.8, -0.0596714)
(71, 0.0183265)
(71.2, -0.00813786)
(71.4, -0.0837481)
(71.6, -0.0464462)
(71.8, 0.0280803)
(72, 0.0340719)
(72.2, 0.0211687)
(72.4, -0.0290434)
(72.6, 0.0271931)
(72.8, -0.0524462)
(73, -0.103796)
(73.2, -0.0227037)
(73.4, 0.193081)
(73.6, 0.152406)
(73.8, -0.062664)
(74, -0.147153)
(74.2, -0.06254)
(74.4, 0.0442134)
(74.6, 0.0827438)
(74.8, 0.0633503)
(75, 0.00440696)
(75.2, -0.0352747)
(75.4, -0.0220569)
(75.6, -0.000141954)
(75.8, 0.0154577)
(76, 0.0212541)
(76.2, 0.0198788)
(76.4, 0.00630731)
(76.6, 0.00514747)
(76.8, 0.00931018)
(77, 0.000197111)
(77.2, -0.0107946)
(77.4, -0.0102706)
(77.6, -0.00168129)
(77.8, 0.00485814)
(78, 0.00481911)
(78.2, 0.00529367)
(78.4, 0.0304967)
(78.6, 0.0390208)
(78.8, 0.0342001)
(79, 0.0216297)
(79.2, 0.00343875)
(79.4, -0.00511161)
(79.6, -0.0273426)
(79.8, -0.0277859)
(80, -0.0200164)
(80.2, -0.00447679)
(80.4, 0.00207797)
(80.6, -0.00638374)
(80.8, -0.0136913)
(81, -0.00448651)
(81.2, 0.000784595)
(81.4, -0.00624055)
(81.6, 0.00918237)
(81.8, 0.0126227)
(82, 0.00990969)
(82.2, 0.017361)
(82.4, 0.0217957)
};

==> exp_plots/hover_dyanmic_payload/az_des.tex <==
\addplot[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates{
(0, -0.122727)
(0.2, -0.104796)
(0.4, -0.0698137)
(0.6, -0.0452978)
(0.8, -0.000347479)
(1, 0.0188682)
(1.2, 0.148826)
(1.4, 0.256516)
(1.6, 0.342745)
(1.8, 0.406442)
(2, 0.433647)
(2.2, 0.448952)
(2.4, 0.453537)
(2.6, 0.452934)
(2.8, 0.393642)
(3, 0.315438)
(3.2, 0.123594)
(3.4, 0.0848096)
(3.6, 0.101634)
(3.8, 0.0943878)
(4, 0.0586471)
(4.2, 0.0492534)
(4.4, 0.0202514)
(4.6, 0.0359762)
(4.8, 0.0373963)
(5, 0.0851912)
(5.2, 0.100055)
(5.4, 0.0454263)
(5.6, 0.0486458)
(5.8, 0.0411964)
(6, 0.0369309)
(6.2, -0.0643621)
(6.4, -0.156986)
(6.6, -0.0393465)
(6.8, -0.0514695)
(7, -0.0389234)
(7.2, -0.00786067)
(7.4, -0.00943029)
(7.6, -0.0480869)
(7.8, -0.0718565)
(8, -0.00754413)
(8.2, 0.00795958)
(8.4, 0.031234)
(8.6, 0.0425909)
(8.8, 0.0478737)
(9, 0.0107727)
(9.2, 0.00311654)
(9.4, 0.0395592)
(9.6, 0.0651211)
(9.8, 0.0810875)
(10, 0.0982481)
(10.2, 0.045239)
(10.4, 0.060966)
(10.6, 0.0052767)
(10.8, -0.00831968)
(11, -0.00417036)
(11.2, 0.0208305)
(11.4, 0.0133738)
(11.6, 0.0448335)
(11.8, 0.0536035)
(12, 0.0267245)
(12.2, 0.0445712)
(12.4, 0.0634775)
(12.6, -0.0253975)
(12.8, -0.0702155)
(13, -0.0896156)
(13.2, -0.104758)
(13.4, -0.0660686)
(13.6, -0.0389168)
(13.8, -0.00497071)
(14, 0.0427107)
(14.2, 0.0314798)
(14.4, 0.039412)
(14.6, 0.0858079)
(14.8, 0.0784032)
(15, -0.0376616)
(15.2, -0.0618983)
(15.4, -0.0232699)
(15.6, -0.0451602)
(15.8, -0.0357751)
(16, 0.0233257)
(16.2, 0.032383)
(16.4, 0.0420809)
(16.6, 0.0541334)
(16.8, 0.07456)
(17, 0.0374314)
(17.2, -0.0210573)
(17.4, -0.0303851)
(17.6, -0.0391733)
(17.8, -0.0412669)
(18, -0.0159209)
(18.2, 0.0730106)
(18.4, 0.0761703)
(18.6, 0.0231838)
(18.8, 0.0304182)
(19, 0.0325706)
(19.2, 0.0241119)
(19.4, 0.0249936)
(19.6, 0.0221775)
(19.8, -0.068189)
(20, -0.0963398)
(20.2, -0.0784762)
(20.4, -0.0586262)
(20.6, 0.0104406)
(20.8, -0.00868177)
(21, 0.0138406)
(21.2, 0.02711)
(21.4, 0.0499197)
(21.6, 0.0891376)
(21.8, 0.0858575)
(22, 0.0137003)
(22.2, -0.00854166)
(22.4, 0.0396841)
(22.6, 0.0190568)
(22.8, 0.016446)
(23, 0.0127121)
(23.2, -0.0101286)
(23.4, -0.0270802)
(23.6, 0.0229955)
(23.8, 0.0239812)
(24, 0.0424876)
(24.2, 0.111285)
(24.4, 0.058439)
(24.6, 0.00395115)
(24.8, -0.0341432)
(25, -0.0607209)
(25.2, -0.0432302)
(25.4, -0.0352399)
(25.6, -0.00811383)
(25.8, -0.00449136)
(26, 0.00427314)
(26.2, -0.01463)
(26.4, -0.0210248)
(26.6, -0.000746395)
(26.8, 0.0191628)
(27, 0.0219371)
(27.2, 0.0197307)
(27.4, 0.0249101)
(27.6, 0.0489506)
(27.8, 0.043585)
(28, 0.0564452)
(28.2, -0.000992522)
(28.4, -0.00537609)
(28.6, 0.105921)
(28.8, 0.069016)
(29, -0.0028348)
(29.2, -0.00389808)
(29.4, -0.111838)
(29.6, -0.100123)
(29.8, -0.0757422)
(30, -0.0706196)
(30.2, 0.00677161)
(30.4, 0.035571)
(30.6, -0.00267543)
(30.8, 0.0242458)
(31, 0.0702937)
(31.2, 0.07647)
(31.4, 0.049315)
(31.6, -0.0327244)
(31.8, -0.0465348)
(32, -0.0479418)
(32.2, -0.0584796)
(32.4, -0.0121028)
(32.6, -0.0113811)
(32.8, 0.0456632)
(33, 0.116728)
(33.2, 0.0771661)
(33.4, 0.0822112)
(33.6, 0.0618007)
(33.8, 0.0491447)
(34, 0.0612117)
(34.2, 0.0230309)
(34.4, -0.147304)
(34.6, -0.134632)
(34.8, -0.094444)
(35, -0.0806338)
(35.2, -0.0301462)
(35.4, 0.0077513)
(35.6, 0.00440107)
(35.8, 0.0136463)
(36, 0.0390043)
(36.2, 0.0378995)
(36.4, 0.0610301)
(36.6, -0.0264811)
(36.8, -0.140104)
(37, -0.0787389)
(37.2, -0.0291273)
(37.4, -0.00921258)
(37.6, 0.0326715)
(37.8, 0.071372)
(38, 0.10272)
(38.2, 0.269963)
(38.4, 0.28398)
(38.6, 0.152778)
(38.8, 0.0766279)
(39, -0.0572245)
(39.2, -0.144838)
(39.4, -0.170582)
(39.6, -0.258222)
(39.8, -0.258113)
(40, -0.200256)
(40.2, -0.0682375)
(40.4, 0.0261689)
(40.6, -0.0103925)
(40.8, 0.00300416)
(41, 0.0705805)
(41.2, 0.106218)
(41.4, 0.0765385)
(41.6, 0.0698697)
(41.8, -0.070072)
(42, -0.178219)
(42.2, -0.139735)
(42.4, -0.049027)
(42.6, -0.0553358)
(42.8, -0.0513017)
(43, -0.0152232)
(43.2, 0.0834758)
(43.4, 0.0808982)
(43.6, 0.0677582)
(43.8, 0.0487677)
(44, 0.0727891)
(44.2, 0.0314915)
(44.4, -0.0350135)
(44.6, -0.0330136)
(44.8, -0.00620419)
(45, -0.00148963)
(45.2, 0.0042968)
(45.4, -0.015133)
(45.6, -0.00724914)
(45.8, -0.00818295)
(46, 0.0985514)
(46.2, 0.0909689)
(46.4, 0.0456008)
(46.6, -0.0191978)
(46.8, -0.0541387)
(47, -0.140167)
(47.2, -0.108304)
(47.4, -0.105211)
(47.6, -0.133604)
(47.8, -0.0868311)
(48, -0.054924)
(48.2, -0.0128098)
(48.4, -0.00127814)
(48.6, 0.00168995)
(48.8, 0.0701995)
(49, 0.0761117)
(49.2, 0.0411175)
(49.4, 0.0246172)
(49.6, 0.0649677)
(49.8, 0.0656974)
(50, 0.0258354)
(50.2, 0.169636)
(50.4, 0.176023)
(50.6, 0.100077)
(50.8, 0.0492656)
(51, -0.00119847)
(51.2, -0.14038)
(51.4, -0.15675)
(51.6, -0.147579)
(51.8, -0.0590164)
(52, 0.00154416)
(52.2, 0.0734799)
(52.4, 0.0981554)
(52.6, 0.0950673)
(52.8, 0.0779533)
(53, 0.0188137)
(53.2, -0.0454743)
(53.4, -0.0182165)
(53.6, -0.0189762)
(53.8, -0.0207158)
(54, 0.00268157)
(54.2, 0.00888308)
(54.4, -0.00158838)
(54.6, 0.00896834)
(54.8, 0.0150502)
(55, -0.0292042)
(55.2, -0.0266671)
(55.4, -0.0358705)
(55.6, -0.0486183)
(55.8, -0.0204613)
(56, 0.0037546)
(56.2, 0.0586757)
(56.4, 0.0944488)
(56.6, 0.116987)
(56.8, 0.0906159)
(57, 0.00178555)
(57.2, 0.0381589)
(57.4, 0.0247028)
(57.6, -0.0124237)
(57.8, -0.0662463)
(58, -0.0863004)
(58.2, -0.125102)
(58.4, -0.0776934)
(58.6, -0.0173752)
(58.8, 0.0315693)
(59, 0.0537247)
(59.2, 0.0396135)
(59.4, 0.0693687)
(59.6, 0.0148485)
(59.8, 0.0508928)
(60, 0.0388915)
(60.2, -0.00729053)
(60.4, 0.0070332)
(60.6, 0.00729812)
(60.8, -0.011669)
(61, -0.0731245)
(61.2, 0.0640447)
(61.4, 0.178924)
(61.6, 0.0308139)
(61.8, -0.0302561)
(62, 0.0409485)
(62.2, 0.0513191)
(62.4, -0.000595354)
(62.6, 0.0154471)
(62.8, 0.0141777)
(63, 0.0664004)
(63.2, 0.0263837)
(63.4, -0.105699)
(63.6, -0.148699)
(63.8, -0.0779528)
(64, -0.0357505)
(64.2, -0.0255392)
(64.4, 0.00776736)
(64.6, 0.0106468)
(64.8, 0.0350456)
(65, 0.0332422)
(65.2, 0.0411045)
(65.4, 0.0225843)
(65.6, -0.134441)
(65.8, -0.13189)
(66, -0.125849)
(66.2, -0.201352)
(66.4, -0.164458)
(66.6, -0.0964491)
(66.8, 0.129551)
(67, 0.210957)
(67.2, 0.193223)
(67.4, 0.0441356)
(67.6, -0.00970028)
(67.8, -0.0728434)
(68, -0.0336303)
(68.2, -0.045149)
(68.4, -0.0231248)
(68.6, 0.0161867)
(68.8, 0.017581)
(69, -0.0264039)
(69.2, -0.0842193)
(69.4, -0.0454987)
(69.6, -0.017131)
(69.8, -0.0187053)
(70, -0.0152634)
(70.2, -0.0334348)
(70.4, -0.0529784)
(70.6, -0.060907)
(70.8, -0.0212371)
(71, -0.0251759)
(71.2, -0.0545405)
(71.4, -0.0460437)
(71.6, -0.0285836)
(71.8, -0.0180786)
(72, -0.00812702)
(72.2, -0.0112977)
(72.4, 0.0114798)
(72.6, -0.0320958)
(72.8, -0.0254515)
(73, -0.0069391)
(73.2, 0.11948)
(73.4, 0.0980164)
(73.6, 0.0223607)
(73.8, -0.135756)
(74, -0.183138)
(74.2, -0.159706)
(74.4, -0.171321)
(74.6, -0.135484)
(74.8, -0.135965)
(75, -0.178425)
(75.2, -0.175693)
(75.4, -0.193221)
(75.6, -0.22753)
(75.8, -0.221638)
(76, -0.218606)
(76.2, -0.246156)
(76.4, -0.255331)
(76.6, -0.275613)
(76.8, -0.278589)
(77, -0.269757)
(77.2, -0.261149)
(77.4, -0.270735)
(77.6, -0.276248)
(77.8, -0.268051)
(78, -0.277834)
(78.2, -0.284597)
(78.4, -0.305546)
(78.6, -0.318758)
(78.8, -0.332215)
(79, -0.340867)
(79.2, -0.330054)
(79.4, -0.330634)
(79.6, -0.336357)
(79.8, -0.343852)
(80, -0.346015)
(80.2, -0.374139)
(80.4, -0.368589)
(80.6, -0.334984)
(80.8, -0.338657)
(81, -0.353399)
(81.2, -0.348928)
(81.4, -0.356427)
(81.6, -0.369124)
(81.8, -0.392787)
(82, -0.394941)
(82.2, -0.396926)
(82.4, -0.399277)
};

==> exp_plots/hover_dyanmic_payload/plot_1.tex <==
%%    
\begin{figure}[t]
\centering

\begin{tikzpicture}


\FPeval{\xshfta}{0}
\FPeval{\xshftb}{0}
\FPeval{\xshftc}{0}
\FPeval{\xshftd}{0}
\FPeval{\xshfte}{0}
\FPeval{\xshftf}{0}



\FPeval{\yshfta}{0-0}
\FPeval{\yshftb}{0-9}
\FPeval{\yshftc}{0-18}
\FPeval{\yshftd}{0-27.1}
\FPeval{\yshfte}{0-36.3}
\FPeval{\yshftf}{0-46.3}


\FPeval{\pltw}{110}
\FPeval{\plth}{24}

\FPeval{\scal}{0.5}


\FPeval{\mrksize}{0.3}

%
\colorlet{desclr}{white!0!magenta}
\colorlet{currclr}{blue!60!green}

\colorlet{gridclr}{white!85!black}
\colorlet{dlegendclr}{white!80!black}
\colorlet{axisclr}{white!75!black}
\colorlet{axisbgclr}{white!99!black}

\colorlet{dlegendclr}{white!80!black}
\colorlet{legendclr}{white!100!black}






\FPeval{\lscale}{0.6}
\FPeval{\limscale}{0.5}
\FPeval{\lxshft}{95.5}
\FPeval{\lyshft}{9.0}

  
\FPeval{\titlescale}{0.7}
\FPeval{\titlexshift}{21.0}
\FPeval{\titleyshift}{13.7}

\colorlet{gpudclr}{white!80!black}
\colorlet{gpuclr}{white!90!black}
\colorlet{gputxtclr}{white!0!black}

\FPeval{\labelscale}{1.0}
\FPeval{\ticklabelscale}{0.9}

\FPeval{\xlabelxshift}{0+15}
\FPeval{\xlabelyshift}{0+0.5}
\FPeval{\ylabelxshift}{0+4.0}
\FPeval{\ylabelyshift}{0+6.2}


\FPeval{\linew}{1.0}
\FPeval{\dashon}{5.0}
\FPeval{\dashoff}{3.0}

\FPeval{\xshfttakeoff}{0-16}
\FPeval{\xshfthover}{0}
\FPeval{\xshftland}{16}
%
%
\node (a) [xshift = \xshfta ex, yshift=\yshfta ex, scale=\scal]{
\tikz{
%
\pgfplotsset{width=\pltw ex, height=\plth ex}
\begin{axis}[
   axis background style={fill=axisbgclr},
    title={},
    xlabel={},
    ylabel={ X (m)},
    xmin=0, xmax=80,
    ymin=-1.5, ymax=1.5,
    xtick={0, 10, 20, 30, 40, 50,  60, 70,  80},
    ytick={-1,  1},
    xticklabels={$0$, $10$, $20$, $30$, $40$, $50$, $60$, $70$, $80$},
    yticklabels={$-1$, $1$},
    extra y ticks={0},
    extra y tick labels={},
     axis line style={axisclr},
    legend image post style={scale =\limscale},
    legend style={at={(\lxshft ex,\lyshft ex)},anchor=south, legend columns = 1, draw = {dlegendclr}, fill={legendclr}, nodes={scale=\lscale}},
    ymajorgrids=true, 
    xmajorgrids=true,
    grid style={dashed, gridclr},
    major tick length=1ex,
    x label style={at={(\xlabelxshift ex, \xlabelyshift ex)},scale=\labelscale},
    y label style={at={(\ylabelxshift ex, \ylabelyshift ex)},scale=\labelscale},
    xticklabel style={scale=\ticklabelscale},
    yticklabel style={scale=\ticklabelscale},
%    ybar,
%    bar width = 4pt,
]
%
%
\input{exp_plots/hover_dyanmic_payload/x_des}
%
\input{exp_plots/hover_dyanmic_payload/x}
%
%
%%   
  \legend{Ref, SLAM}
  %
\end{axis}
%
% \node [draw=gpudclr,fill=gpuclr,rounded corners=0.2ex, minimum width=10.0ex, xshift=\titlexshift ex, yshift=\titleyshift ex, scale=\titlescale]{\textcolor{gputxtclr}{\textbf{Step-X}}};
}};
%
%    
%
%
\node (b) [xshift = \xshftb ex, yshift=\yshftb ex, scale=\scal]{
\tikz{
%
\pgfplotsset{width=\pltw ex, height=\plth ex}
\begin{axis}[
   axis background style={fill=axisbgclr},
    title={},
    xlabel={},
    ylabel={ Y (m)},
    xmin=0, xmax=80,
    ymin=-1.5, ymax=1.5,
    xtick={0, 10, 20, 30, 40, 50,  60, 70,  80},
    ytick={-1,  1},
    xticklabels={$0$, $10$, $20$, $30$, $40$, $50$, $60$, $70$, $80$},
    yticklabels={$-1$, $1$},
    extra y ticks={0},
    extra y tick labels={},
     axis line style={axisclr},
    legend image post style={scale =\limscale},
    legend style={at={(\lxshft ex,\lyshft ex)},anchor=south, legend columns = 1, draw = {dlegendclr}, fill={legendclr}, nodes={scale=\lscale}},
    ymajorgrids=true, 
    xmajorgrids=true,
    grid style={dashed, gridclr},
    major tick length=1ex,
    x label style={at={(\xlabelxshift ex, \xlabelyshift ex)},scale=\labelscale},
    y label style={at={(\ylabelxshift ex, \ylabelyshift ex)},scale=\labelscale},
    xticklabel style={scale=\ticklabelscale},
    yticklabel style={scale=\ticklabelscale},
%    ybar,
%    bar width = 4pt,
]
%
\input{exp_plots/hover_dyanmic_payload/y}
%
%
\input{exp_plots/hover_dyanmic_payload/y_des}
%
%% 
  \legend{Ref, SLAM}
  %
\end{axis}
%
% \node [draw=gpudclr,fill=gpuclr,rounded corners=0.2ex, minimum width=10.0ex, xshift=\titlexshift ex, yshift=\titleyshift ex, scale=\titlescale]{\textcolor{gputxtclr}{\textbf{Step-X}}};
}};
%
% 
%
\node (c) [xshift = \xshftc ex, yshift=\yshftc ex, scale=\scal]{
\tikz{
%
\pgfplotsset{width=\pltw ex, height=\plth ex}
\begin{axis}[
   axis background style={fill=axisbgclr},
    title={},
    xlabel={},
    ylabel={ Z (m)},
    xmin=0, xmax=80,
    ymin=-1.5, ymax=1.5,
    xtick={0, 10, 20, 30, 40, 50,  60, 70,  80},
    ytick={-1,  1},
    xticklabels={$0$, $10$, $20$, $30$, $40$, $50$, $60$, $70$, $80$},
    yticklabels={$-1$, $1$},
    extra y ticks={0},
    extra y tick labels={},
     axis line style={axisclr},
    legend image post style={scale =\limscale},
    legend style={at={(\lxshft ex,\lyshft ex)},anchor=south, legend columns = 1, draw = {dlegendclr}, fill={legendclr}, nodes={scale=\lscale}},
    ymajorgrids=true, 
    xmajorgrids=true,
    grid style={dashed, gridclr},
    major tick length=1ex,
    x label style={at={(\xlabelxshift ex, \xlabelyshift ex)},scale=\labelscale},
    y label style={at={(\ylabelxshift ex, \ylabelyshift ex)},scale=\labelscale},
    xticklabel style={scale=\ticklabelscale},
    yticklabel style={scale=\ticklabelscale},
%    ybar,
%    bar width = 4pt,
]
%
\input{exp_plots/hover_dyanmic_payload/z}
%
%
\input{exp_plots/hover_dyanmic_payload/z_des}
%
%% 
  \legend{Ref, SLAM}
  %
\end{axis}
%
% \node [draw=gpudclr,fill=gpuclr,rounded corners=0.2ex, minimum width=10.0ex, xshift=\titlexshift ex, yshift=\titleyshift ex, scale=\titlescale]{\textcolor{gputxtclr}{\textbf{Step-X}}};
}};
%
% 
%
\node (d) [xshift = \xshftd ex, yshift=\yshftd ex, scale=\scal]{
\tikz{
%
\pgfplotsset{width=\pltw ex, height=\plth ex}
\begin{axis}[
   axis background style={fill=axisbgclr},
    title={},
    xlabel={},
    ylabel={ Yaw ($^\text{o}$)},
    xmin=0, xmax=80,
    ymin=-30, ymax=30,
    xtick={0, 10, 20, 30, 40, 50,  60, 70,  80},
    ytick={0},
    xticklabels={$0$, $10$, $20$, $30$, $40$, $50$, $60$, $70$, $80$},
    yticklabels={},
    extra y ticks={-20, 20},
    extra y tick labels={$-20$, $20$},
     axis line style={axisclr},
    legend image post style={scale =\limscale},
    legend style={at={(\lxshft ex,\lyshft ex)},anchor=south, legend columns = 1, draw = {dlegendclr}, fill={legendclr}, nodes={scale=\lscale}},
    ymajorgrids=true, 
    xmajorgrids=true,
    grid style={dashed, gridclr},
    major tick length=1ex,
    x label style={at={(\xlabelxshift ex, \xlabelyshift ex)},scale=\labelscale},
    y label style={at={(\ylabelxshift ex, \ylabelyshift ex)},scale=\labelscale},
    xticklabel style={scale=\ticklabelscale},
    yticklabel style={scale=\ticklabelscale},
%    ybar,
%    bar width = 4pt,
]
%
\input{exp_plots/hover_dyanmic_payload/yaw}
%
%
%
\input{exp_plots/hover_dyanmic_payload/yaw_des}
%
%% 
  \legend{Ref, SLAM}
  %
\end{axis}
%
% \node [draw=gpudclr,fill=gpuclr,rounded corners=0.2ex, minimum width=10.0ex, xshift=\titlexshift ex, yshift=\titleyshift ex, scale=\titlescale]{\textcolor{gputxtclr}{\textbf{Step-X}}};
}};
%
% 
%
\node (e) [xshift = \xshfte ex, yshift=\yshfte ex, scale=\scal]{
\tikz{
%
\pgfplotsset{width=\pltw ex, height=\plth ex }
\begin{axis}[
   axis background style={fill=axisbgclr},
    title={},
    xlabel={},
    ylabel={ $a_z$ (m/s$^2$)},
    xmin=0, xmax=80,
    ymin=-1.5, ymax=1.5,
    xtick={0, 10, 20, 30, 40, 50,  60, 70,  80},
    ytick={0},
    xticklabels={$0$, $10$, $20$, $30$, $40$, $50$, $60$, $70$, $80$},
        yticklabels={},
    extra y ticks={-1, 1},
    extra y tick labels={$-1$, $1$},
    axis line style={axisclr},
    legend image post style={scale =\limscale},
    legend style={at={(\lxshft ex,\lyshft ex)},anchor=south, legend columns = 1, draw = {dlegendclr}, fill={legendclr}, nodes={scale=\lscale}},
    ymajorgrids=true, 
    xmajorgrids=true,
    grid style={dashed, gridclr},
    major tick length=1ex,
    x label style={at={(\xlabelxshift ex, \xlabelyshift ex)},scale=\labelscale},
    y label style={at={(\ylabelxshift ex, \ylabelyshift ex)},scale=\labelscale},
    xticklabel style={scale=\ticklabelscale},
    yticklabel style={scale=\ticklabelscale},
%    ybar,
%    bar width = 4pt,
]
%
\input{exp_plots/hover_dyanmic_payload/az}
%
%
\input{exp_plots/hover_dyanmic_payload/az_des}
%
%
%
%% 
  \legend{Ref, SLAM}
  %
\end{axis}
%
% \node [draw=gpudclr,fill=gpuclr,rounded corners=0.2ex, minimum width=10.0ex, xshift=\titlexshift ex, yshift=\titleyshift ex, scale=\titlescale]{\textcolor{gputxtclr}{\textbf{Step-X}}};
}};
%
%
\node (f) [xshift = \xshftf ex, yshift=\yshftf ex, scale=\scal]{
\tikz{
%
\pgfplotsset{width=\pltw ex, height=\plth ex}
\begin{axis}[
   axis background style={fill=axisbgclr},
    title={},
    xlabel={Time (s)},
    ylabel={ Thrust ($\%$)},
    xmin=0, xmax=80,
    ymin=0, ymax=100,
    xtick={0, 10, 20, 30, 40, 50,  60, 70,  80},
    ytick={50},
    xticklabels={$0$, $10$, $20$, $30$, $40$, $50$, $60$, $70$, $80$},
    yticklabels={},
    extra y ticks={20, 80},
    extra y tick labels={$20$, $80$},
    axis line style={axisclr},
    legend image post style={scale =\limscale},
    legend style={at={(\lxshft ex,\lyshft ex)},anchor=south, legend columns = 1, draw = {dlegendclr}, fill={legendclr}, nodes={scale=\lscale}},
    ymajorgrids=true, 
    xmajorgrids=true,
    grid style={dashed, gridclr},
    major tick length=1ex,
    x label style={at={(\xlabelxshift ex, \xlabelyshift ex)},scale=\labelscale},
    y label style={at={(\ylabelxshift ex, \ylabelyshift ex)},scale=\labelscale},
    xticklabel style={scale=\ticklabelscale},
    yticklabel style={scale=\ticklabelscale},
%    ybar,
%    bar width = 4pt,
]
%
\input{exp_plots/hover_dyanmic_payload/thrust}
%
%
%% 
  \legend{Thrust}
  %
\end{axis}
%
% \node [draw=gpudclr,fill=gpuclr,rounded corners=0.2ex, minimum width=10.0ex, xshift=\titlexshift ex, yshift=\titleyshift ex, scale=\titlescale]{\textcolor{gputxtclr}{\textbf{Step-X}}};
}};
%
%
%
%
\FPeval{\imw}{12}
\FPeval{\imh}{8}
%
%
\node (im1) [xshift=-17.6ex, yshift=10ex]{\includegraphics[width=\imw ex, height = \imh ex]{images/no_load.png}};
\node (im2) [xshift=-4.95ex, yshift=10ex]{\includegraphics[width=\imw ex, height = \imh ex]{images/center_load.png}};
\node (im3) [xshift=7.75ex, yshift=10ex]{\includegraphics[width=\imw ex, height = \imh ex]{images/off_center_load.png}};
\node (im4) [xshift=20.4ex, yshift=10ex]{\includegraphics[width=\imw ex, height = \imh ex]{images/no_load.png}};
%%
%
\node (im1) [xshift=-17.6ex, yshift=15ex]{\scriptsize No payload};
\node (im2) [xshift=-4.95ex, yshift=15ex]{\scriptsize Center payload};
\node (im3) [xshift=7.75ex, yshift=15ex]{\scriptsize Off-Center payload};
\node (im4) [xshift=20.4ex, yshift=15ex]{\scriptsize No payload};
 
\end{tikzpicture}
%
%
\caption{Hover performance with dynamic payload.}
%
\label{fig:hoverdynamicpayload}
%
%\vspace{-3ex}
\end{figure}
%
%
%
%%


==> exp_plots/hover_dyanmic_payload/thrust.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 10)
(0.2, 10.1345)
(0.4, 10.7821)
(0.6, 10.8152)
(0.8, 11.4611)
(1, 11.6848)
(1.2, 17.1867)
(1.4, 20.7069)
(1.6, 24.3966)
(1.8, 29.1277)
(2, 32.6912)
(2.2, 37.2823)
(2.4, 42.3338)
(2.6, 45.7042)
(2.8, 44.3325)
(3, 45.5408)
(3.2, 41.5613)
(3.4, 45.2254)
(3.6, 47.3967)
(3.8, 45.7932)
(4, 46.366)
(4.2, 46.5569)
(4.4, 46.6195)
(4.6, 47.8797)
(4.8, 46.6758)
(5, 48.7704)
(5.2, 49.2457)
(5.4, 47.014)
(5.6, 48.0928)
(5.8, 48.4592)
(6, 46.7193)
(6.2, 47.5833)
(6.4, 45.9)
(6.6, 49.379)
(6.8, 48.5797)
(7, 46.6728)
(7.2, 49.4153)
(7.4, 48.5475)
(7.6, 47.3037)
(7.8, 47.4529)
(8, 50.7477)
(8.2, 48.5865)
(8.4, 47.618)
(8.6, 50.2105)
(8.8, 49.8108)
(9, 48.2807)
(9.2, 48.352)
(9.4, 51.2872)
(9.6, 49.9911)
(9.8, 50.4823)
(10, 48.8463)
(10.2, 46.9621)
(10.4, 51.3952)
(10.6, 47.5984)
(10.8, 48.1479)
(11, 51.4397)
(11.2, 49.5941)
(11.4, 48.6499)
(11.6, 50.2241)
(11.8, 49.6099)
(12, 48.2272)
(12.2, 48.7642)
(12.4, 50.4181)
(12.6, 46.5537)
(12.8, 48.5416)
(13, 48.5139)
(13.2, 47.9296)
(13.4, 49.0592)
(13.6, 49.864)
(13.8, 50.2755)
(14, 49.5226)
(14.2, 49.9453)
(14.4, 49.0426)
(14.6, 51.8431)
(14.8, 51.6929)
(15, 50.6426)
(15.2, 49.6614)
(15.4, 53.752)
(15.6, 49.8424)
(15.8, 50.0308)
(16, 51.8506)
(16.2, 51.8265)
(16.4, 51.1029)
(16.6, 49.4)
(16.8, 52.3958)
(17, 51.6142)
(17.2, 50.164)
(17.4, 50.7051)
(17.6, 52.2415)
(17.8, 50.4744)
(18, 52.0751)
(18.2, 52.7835)
(18.4, 51.5379)
(18.6, 49.7677)
(18.8, 52.0836)
(19, 52.4923)
(19.2, 50.6365)
(19.4, 51.2138)
(19.6, 50.7477)
(19.8, 50.8122)
(20, 48.8862)
(20.2, 51.8812)
(20.4, 52.0662)
(20.6, 51.7111)
(20.8, 52.2271)
(21, 51.6998)
(21.2, 53.4188)
(21.4, 52.4837)
(21.6, 52.25)
(21.8, 51.9106)
(22, 48.839)
(22.2, 50.9888)
(22.4, 51.3481)
(22.6, 50.5937)
(22.8, 50.7764)
(23, 51.6508)
(23.2, 50.4127)
(23.4, 49.7647)
(23.6, 53.1359)
(23.8, 51.0722)
(24, 50.7336)
(24.2, 53.5433)
(24.4, 50.7132)
(24.6, 48.7494)
(24.8, 48.1544)
(25, 49.9372)
(25.2, 50.2805)
(25.4, 50.1942)
(25.6, 50.6813)
(25.8, 50.3361)
(26, 50.6968)
(26.2, 50.3255)
(26.4, 50.48)
(26.6, 51.3722)
(26.8, 51.5802)
(27, 50.3097)
(27.2, 50.6633)
(27.4, 50.8918)
(27.6, 51.7286)
(27.8, 51.3407)
(28, 51.1072)
(28.2, 50.8155)
(28.4, 49.3145)
(28.6, 53.1622)
(28.8, 50.7144)
(29, 46.4874)
(29.2, 50.4781)
(29.4, 48.8724)
(29.6, 48.7429)
(29.8, 49.5696)
(30, 49.3447)
(30.2, 52.2628)
(30.4, 51.5297)
(30.6, 49.3636)
(30.8, 50.6365)
(31, 52.0741)
(31.2, 50.1438)
(31.4, 49.1704)
(31.6, 50.066)
(31.8, 52.608)
(32, 53.6721)
(32.2, 50.9124)
(32.4, 52.9894)
(32.6, 52.4581)
(32.8, 52.7112)
(33, 54.3167)
(33.2, 52.9291)
(33.4, 52.5323)
(33.6, 54.431)
(33.8, 53.0743)
(34, 54.9348)
(34.2, 53.5125)
(34.4, 50.3249)
(34.6, 51.1722)
(34.8, 56.0203)
(35, 53.3636)
(35.2, 52.4304)
(35.4, 54.4748)
(35.6, 53.5874)
(35.8, 53.0613)
(36, 54.902)
(36.2, 53.4009)
(36.4, 54.548)
(36.6, 52.8843)
(36.8, 46.5309)
(37, 55.3479)
(37.2, 55.8691)
(37.4, 52.633)
(37.6, 53.1033)
(37.8, 55.2779)
(38, 54.0942)
(38.2, 56.0473)
(38.4, 58.2034)
(38.6, 51.056)
(38.8, 51.7592)
(39, 52.8164)
(39.2, 49.6489)
(39.4, 53.1173)
(39.6, 48.5929)
(39.8, 47.2449)
(40, 51.9062)
(40.2, 53.5327)
(40.4, 52.1217)
(40.6, 48.6536)
(40.8, 51.2472)
(41, 53.7865)
(41.2, 54.2275)
(41.4, 48.2797)
(41.6, 51.3632)
(41.8, 51.9414)
(42, 46.5665)
(42.2, 52.1713)
(42.4, 54.6377)
(42.6, 50.5722)
(42.8, 48.9717)
(43, 52.4159)
(43.2, 54.337)
(43.4, 52.5794)
(43.6, 49.5126)
(43.8, 51.0138)
(44, 54.0931)
(44.2, 52.9439)
(44.4, 48.1621)
(44.6, 51.9124)
(44.8, 54.0745)
(45, 52.2986)
(45.2, 51.2208)
(45.4, 51.4581)
(45.6, 52.7408)
(45.8, 51.4067)
(46, 54.9472)
(46.2, 53.2748)
(46.4, 49.9867)
(46.6, 50.3124)
(46.8, 52.2871)
(47, 48.4377)
(47.2, 51.4492)
(47.4, 52.1941)
(47.6, 50.2053)
(47.8, 51.1135)
(48, 52.0719)
(48.2, 50.4154)
(48.4, 50.0682)
(48.6, 52.328)
(48.8, 52.0483)
(49, 52.1805)
(49.2, 50.3063)
(49.4, 51.1632)
(49.6, 52.5611)
(49.8, 52.2886)
(50, 50.8702)
(50.2, 51.9277)
(50.4, 55.3266)
(50.6, 48.7423)
(50.8, 49.2707)
(51, 52.0407)
(51.2, 49.9022)
(51.4, 49.3769)
(51.6, 53.6098)
(51.8, 53.8117)
(52, 52.6392)
(52.2, 50.9608)
(52.4, 52.3388)
(52.6, 51.9365)
(52.8, 51.6428)
(53, 50.655)
(53.2, 50.7917)
(53.4, 52.1252)
(53.6, 52.3095)
(53.8, 49.7343)
(54, 50.4424)
(54.2, 52.7193)
(54.4, 49.7607)
(54.6, 51.2564)
(54.8, 51.5263)
(55, 48.2501)
(55.2, 51.6551)
(55.4, 51.8877)
(55.6, 49.936)
(55.8, 52.5878)
(56, 52.8295)
(56.2, 50.7952)
(56.4, 53.7573)
(56.6, 52.2832)
(56.8, 50.7264)
(57, 49.1467)
(57.2, 50.941)
(57.4, 51.449)
(57.6, 49.4333)
(57.8, 50.3695)
(58, 50.2981)
(58.2, 49.9711)
(58.4, 52.5219)
(58.6, 53.972)
(58.8, 51.4241)
(59, 51.7979)
(59.2, 52.2835)
(59.4, 51.2134)
(59.6, 50.849)
(59.8, 53.086)
(60, 52.6466)
(60.2, 49.9158)
(60.4, 53.1168)
(60.6, 51.8568)
(60.8, 50.5042)
(61, 50.1887)
(61.2, 52.3624)
(61.4, 54.7845)
(61.6, 48.3142)
(61.8, 48.0837)
(62, 53.6826)
(62.2, 55.192)
(62.4, 49.8384)
(62.6, 50.7696)
(62.8, 53.4861)
(63, 52.6448)
(63.2, 51.5547)
(63.4, 48.2927)
(63.6, 52.8412)
(63.8, 53.5274)
(64, 51.6516)
(64.2, 51.2057)
(64.4, 51.4229)
(64.6, 52.0842)
(64.8, 52.0326)
(65, 52.3413)
(65.2, 52.6055)
(65.4, 51.9899)
(65.6, 46.8167)
(65.8, 50.5881)
(66, 53.1616)
(66.2, 48.1105)
(66.4, 49.8293)
(66.6, 54.5321)
(66.8, 53.1655)
(67, 54.4264)
(67.2, 50.9919)
(67.4, 49.9664)
(67.6, 52.4535)
(67.8, 52.4424)
(68, 52.2046)
(68.2, 49.5998)
(68.4, 51.5215)
(68.6, 54.1491)
(68.8, 50.7044)
(69, 48.4728)
(69.2, 47.773)
(69.4, 53.3482)
(69.6, 51.1036)
(69.8, 49.6801)
(70, 49.8841)
(70.2, 49.5124)
(70.4, 47.723)
(70.6, 48.4759)
(70.8, 50.7545)
(71, 48.7022)
(71.2, 47.726)
(71.4, 49.1585)
(71.6, 50.0484)
(71.8, 48.2147)
(72, 47.3436)
(72.2, 48.4402)
(72.4, 49.4667)
(72.6, 47.1742)
(72.8, 47.0179)
(73, 49.8374)
(73.2, 50.5)
(73.4, 48.449)
(73.6, 44.5198)
(73.8, 46.6517)
(74, 47.0632)
(74.2, 46.1219)
(74.4, 42.6708)
(74.6, 42.9799)
(74.8, 41.1126)
(75, 39.9647)
(75.2, 38.6764)
(75.4, 36.9335)
(75.6, 34.3952)
(75.8, 32.3558)
(76, 30.2335)
(76.2, 27.4142)
(76.4, 24.2403)
(76.6, 21.9957)
(76.8, 19.3746)
(77, 17.0476)
(77.2, 14.9424)
(77.4, 12.1689)
(77.6, 10)
(77.8, 10)
(78, 10)
(78.2, 10)
(78.4, 10)
(78.6, 10)
(78.8, 10)
(79, 10)
(79.2, 10)
(79.4, 10)
(79.6, 10)
(79.8, 10)
(80, 10)
(80.2, 10)
(80.4, 10)
(80.6, 10)
(80.8, 10)
(81, 10)
(81.2, 10)
(81.4, 10)
(81.6, 10)
(81.8, 10)
(82, 10)
(82.2, 10)
(82.4, 10)
};

==> exp_plots/hover_dyanmic_payload/thrust_center.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(18, 51.1818)
(18.2, 51.3592)
(18.4, 51.3658)
(18.6, 51.2517)
(18.8, 51.351)
(19, 51.4635)
(19.2, 51.3973)
(19.4, 51.3978)
(19.6, 51.3636)
(19.8, 51.2941)
(20, 51.0524)
(20.2, 51.1218)
(20.4, 51.196)
(20.6, 51.2183)
(20.8, 51.3144)
(21, 51.338)
(21.2, 51.5309)
(21.4, 51.6527)
(21.6, 51.7644)
(21.8, 51.8059)
(22, 51.5456)
(22.2, 51.5206)
(22.4, 51.5184)
(22.6, 51.4433)
(22.8, 51.3796)
(23, 51.4122)
(23.2, 51.2764)
(23.4, 51.0814)
(23.6, 51.2292)
(23.8, 51.1742)
(24, 51.0998)
(24.2, 51.2926)
(24.4, 51.234)
(24.6, 50.9962)
(24.8, 50.7153)
(25, 50.6456)
(25.2, 50.5762)
(25.4, 50.4994)
(25.6, 50.4842)
(25.8, 50.4346)
(26, 50.4165)
(26.2, 50.383)
(26.4, 50.3702)
(26.6, 50.4122)
(26.8, 50.5155)
(27, 50.5016)
(27.2, 50.502)
(27.4, 50.5751)
(27.6, 50.747)
(27.8, 50.8671)
(28, 50.9252)
(28.2, 50.9429)
(28.4, 50.8082)
(28.6, 51.0418)
(28.8, 51.034)
};

==> exp_plots/hover_dyanmic_payload/thrust_offcenter.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(31, 50.2754)
(31.2, 50.2769)
(31.4, 50.1999)
(31.6, 50.1723)
(31.8, 50.4406)
(32, 50.8487)
(32.2, 50.9135)
(32.4, 51.1908)
(32.6, 51.3952)
(32.8, 51.5932)
(33, 51.9316)
(33.2, 52.086)
(33.4, 52.2087)
(33.6, 52.5285)
(33.8, 52.6756)
(34, 52.9748)
(34.2, 53.1411)
(34.4, 52.9754)
(34.6, 52.8521)
(34.8, 53.159)
(35, 53.1907)
(35.2, 53.1575)
(35.4, 53.2878)
(35.6, 53.3323)
(35.8, 53.315)
(36, 53.46)
(36.2, 53.4761)
(36.4, 53.6029)
(36.6, 53.5413)
(36.8, 52.8763)
(37, 53.0649)
(37.2, 53.3321)
(37.4, 53.3082)
(37.6, 53.2968)
(37.8, 53.4404)
(38, 53.512)
(38.2, 53.7809)
(38.4, 54.2315)
(38.6, 53.9892)
(38.8, 53.8176)
(39, 53.7289)
(39.2, 53.3529)
(39.4, 53.3096)
(39.6, 52.8475)
(39.8, 52.3064)
(40, 52.1011)
(40.2, 52.0807)
(40.4, 51.9817)
(40.6, 51.5449)
(40.8, 51.3603)
(41, 51.4697)
(41.2, 51.6294)
(41.4, 51.2281)
(41.6, 51.2507)
(41.8, 51.3227)
(42, 50.863)
(42.2, 50.9976)
(42.4, 51.3335)
(42.6, 51.3219)
(42.8, 51.1397)
};

==> exp_plots/hover_dyanmic_payload/x.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0.046363)
(0.2, 0.0629639)
(0.4, 0.0624878)
(0.6, 0.0615439)
(0.8, 0.0637038)
(1, 0.0596236)
(1.2, 0.0642756)
(1.4, 0.0648243)
(1.6, 0.0644671)
(1.8, 0.0659488)
(2, 0.065535)
(2.2, 0.0647658)
(2.4, 0.0672382)
(2.6, 0.0686695)
(2.8, 0.068943)
(3, 0.0774559)
(3.2, 0.101426)
(3.4, 0.129103)
(3.6, 0.138995)
(3.8, 0.12135)
(4, 0.0871543)
(4.2, 0.0567019)
(4.4, 0.0299762)
(4.6, 0.011302)
(4.8, -0.0132501)
(5, -0.0280696)
(5.2, -0.042964)
(5.4, -0.0552543)
(5.6, -0.0511331)
(5.8, -0.0461272)
(6, -0.0440016)
(6.2, -0.0376502)
(6.4, -0.0281489)
(6.6, -0.0137652)
(6.8, -0.00693898)
(7, 0.00147335)
(7.2, 0.002477)
(7.4, 0.00845313)
(7.6, 0.0101122)
(7.8, 0.0129457)
(8, 0.015254)
(8.2, 0.00650616)
(8.4, 0.000466453)
(8.6, -0.00571609)
(8.8, -0.0147886)
(9, -0.0245086)
(9.2, -0.0351122)
(9.4, -0.0444108)
(9.6, -0.0495191)
(9.8, -0.0482717)
(10, -0.0425941)
(10.2, -0.0347176)
(10.4, -0.0250423)
(10.6, -0.0169126)
(10.8, -0.015499)
(11, -0.0109456)
(11.2, -0.00537899)
(11.4, -0.00080353)
(11.6, 0.0035897)
(11.8, 0.00523239)
(12, 0.00164423)
(12.2, -0.00315534)
(12.4, -0.0198186)
(12.6, -0.0319891)
(12.8, -0.0381239)
(13, -0.0328602)
(13.2, -0.0102276)
(13.4, -0.00270534)
(13.6, -0.00413353)
(13.8, -0.00819361)
(14, -0.00308231)
(14.2, -0.00336824)
(14.4, 0.00403517)
(14.6, 0.0195433)
(14.8, 0.0224342)
(15, 0.0224455)
(15.2, 0.0148648)
(15.4, 0.0102379)
(15.6, 0.00536424)
(15.8, 0.00347366)
(16, -0.000537581)
(16.2, -0.00329161)
(16.4, -0.00269038)
(16.6, 0.00411474)
(16.8, -0.0024198)
(17, -0.00431871)
(17.2, 0.000226298)
(17.4, 0.000239511)
(17.6, -0.000619364)
(17.8, -0.00194011)
(18, -0.00280014)
(18.2, -0.000576671)
(18.4, -0.00136203)
(18.6, 0.00560488)
(18.8, 0.0166911)
(19, 0.0143924)
(19.2, 0.0244762)
(19.4, 0.0329941)
(19.6, 0.0387727)
(19.8, 0.0387061)
(20, 0.0380681)
(20.2, 0.043416)
(20.4, 0.0316024)
(20.6, 0.0224652)
(20.8, 0.014291)
(21, 0.00481291)
(21.2, 0.00270934)
(21.4, -0.00953894)
(21.6, -0.0166146)
(21.8, -0.00832935)
(22, 0.0102972)
(22.2, 0.0201949)
(22.4, 0.029892)
(22.6, 0.0341279)
(22.8, 0.0393035)
(23, 0.0342164)
(23.2, 0.0268474)
(23.4, 0.0190102)
(23.6, 0.0125001)
(23.8, 0.0123049)
(24, 0.0190869)
(24.2, 0.0287763)
(24.4, 0.0191944)
(24.6, 0.0131468)
(24.8, 0.0127814)
(25, 0.0130445)
(25.2, 0.0191169)
(25.4, 0.02662)
(25.6, 0.0396069)
(25.8, 0.0529501)
(26, 0.0663623)
(26.2, 0.0749505)
(26.4, 0.0708353)
(26.6, 0.057366)
(26.8, 0.0388675)
(27, 0.0218818)
(27.2, 0.00563251)
(27.4, -0.00136751)
(27.6, -0.00160839)
(27.8, -0.0125719)
(28, -0.0165812)
(28.2, -0.00765566)
(28.4, -0.00350383)
(28.6, 0.00252329)
(28.8, 0.00427154)
(29, 0.00177157)
(29.2, 0.0063747)
(29.4, 0.00227725)
(29.6, 0.00553313)
(29.8, 0.0137658)
(30, 0.0214978)
(30.2, 0.0316901)
(30.4, 0.0346614)
(30.6, 0.0368297)
(30.8, 0.0348275)
(31, 0.0279932)
(31.2, 0.0138129)
(31.4, 0.000572898)
(31.6, -0.00904131)
(31.8, 0.00384938)
(32, 0.0367815)
(32.2, 0.0816398)
(32.4, 0.108928)
(32.6, 0.147205)
(32.8, 0.162797)
(33, 0.172796)
(33.2, 0.159271)
(33.4, 0.128702)
(33.6, 0.0908441)
(33.8, 0.0463406)
(34, 0.0129669)
(34.2, -0.000712942)
(34.4, -0.0212607)
(34.6, -0.0322265)
(34.8, -0.0492456)
(35, -0.0664895)
(35.2, -0.0709504)
(35.4, -0.0648082)
(35.6, -0.0553132)
(35.8, -0.039119)
(36, -0.0261444)
(36.2, -0.00887137)
(36.4, 0.000993366)
(36.6, 0.0157117)
(36.8, 0.0234527)
(37, 0.016633)
(37.2, 0.000813632)
(37.4, -0.0101895)
(37.6, -0.000648821)
(37.8, 0.00521955)
(38, 0.00176868)
(38.2, 0.00553075)
(38.4, 0.0244467)
(38.6, 0.0324918)
(38.8, 0.0406098)
(39, 0.0380216)
(39.2, 0.0264638)
(39.4, -0.00896169)
(39.6, -0.048388)
(39.8, -0.0935534)
(40, -0.137349)
(40.2, -0.16648)
(40.4, -0.172561)
(40.6, -0.157618)
(40.8, -0.124654)
(41, -0.0831709)
(41.2, -0.0381353)
(41.4, -0.00950391)
(41.6, 0.0050839)
(41.8, 0.0183796)
(42, 0.0194956)
(42.2, 0.0156208)
(42.4, 0.0167184)
(42.6, 0.0158742)
(42.8, 0.0208519)
(43, 0.0125668)
(43.2, 0.00347616)
(43.4, 0.00144871)
(43.6, 0.00998126)
(43.8, 0.012084)
(44, 0.0105321)
(44.2, 0.0109915)
(44.4, 0.0123233)
(44.6, 0.0144505)
(44.8, 0.016377)
(45, 0.0198541)
(45.2, 0.0242059)
(45.4, 0.0202003)
(45.6, 0.00894446)
(45.8, -0.00416762)
(46, -0.0203036)
(46.2, -0.0202732)
(46.4, -0.0239294)
(46.6, -0.0168053)
(46.8, -0.00943323)
(47, 0.00454434)
(47.2, 0.0107401)
(47.4, 0.0104889)
(47.6, -0.00233283)
(47.8, 0.00915515)
(48, 0.00381087)
(48.2, 0.000613082)
(48.4, 0.00715617)
(48.6, 0.00803056)
(48.8, 0.00945096)
(49, 0.00720212)
(49.2, 0.0148756)
(49.4, 0.0145572)
(49.6, 0.0157012)
(49.8, 0.0142871)
(50, 0.00944119)
(50.2, 0.013453)
(50.4, 0.0170338)
(50.6, 0.00198531)
(50.8, -0.00168315)
(51, -0.00223529)
(51.2, -0.00415466)
(51.4, -0.00702978)
(51.6, -0.00854397)
(51.8, -0.00968837)
(52, -0.01838)
(52.2, -0.0193506)
(52.4, -0.0141929)
(52.6, -0.00687602)
(52.8, 0.00919471)
(53, 0.0245251)
(53.2, 0.0360289)
(53.4, 0.0401855)
(53.6, 0.0379873)
(53.8, 0.0291557)
(54, 0.0109408)
(54.2, 0.00687927)
(54.4, 0.00523207)
(54.6, 0.00326578)
(54.8, 0.0043832)
(55, 0.00338787)
(55.2, -0.00121926)
(55.4, -0.00326973)
(55.6, 0.00608601)
(55.8, 0.0147127)
(56, 0.0181489)
(56.2, 0.0272275)
(56.4, 0.0261869)
(56.6, 0.0223097)
(56.8, 0.0166234)
(57, 0.0175877)
(57.2, 0.00910383)
(57.4, -0.00216956)
(57.6, -0.00977974)
(57.8, -0.0100654)
(58, -0.00314093)
(58.2, -0.00332253)
(58.4, 0.012969)
(58.6, 0.0233381)
(58.8, 0.0342077)
(59, 0.0486082)
(59.2, 0.0517185)
(59.4, 0.0467131)
(59.6, 0.0378222)
(59.8, 0.0426862)
(60, 0.0407969)
(60.2, 0.0483146)
(60.4, 0.0518756)
(60.6, 0.0436325)
(60.8, 0.0363148)
(61, 0.0281738)
(61.2, 0.0165904)
(61.4, -0.0113083)
(61.6, -0.0193373)
(61.8, -0.0212956)
(62, -0.0293618)
(62.2, -0.041414)
(62.4, -0.0432116)
(62.6, -0.0349157)
(62.8, -0.0102425)
(63, 0.0158183)
(63.2, 0.0337672)
(63.4, 0.0486669)
(63.6, 0.0628233)
(63.8, 0.0509681)
(64, 0.0362966)
(64.2, 0.0348617)
(64.4, 0.0317568)
(64.6, 0.0191026)
(64.8, 0.00799001)
(65, 0.00947267)
(65.2, 0.0135547)
(65.4, 0.0123151)
(65.6, 0.00996338)
(65.8, 0.0102833)
(66, 0.00339882)
(66.2, -0.00755733)
(66.4, -0.0109983)
(66.6, -0.0110948)
(66.8, -0.00800823)
(67, -0.00651753)
(67.2, 0.00152103)
(67.4, 0.00718879)
(67.6, 0.0163421)
(67.8, 0.0219385)
(68, 0.0347196)
(68.2, 0.0352811)
(68.4, 0.0439028)
(68.6, 0.0464607)
(68.8, 0.0445949)
(69, 0.0372895)
(69.2, 0.00693789)
(69.4, -0.00945331)
(69.6, -0.0201164)
(69.8, -0.0193487)
(70, -0.0100989)
(70.2, -0.00535263)
(70.4, 0.00140981)
(70.6, 0.00334157)
(70.8, 0.00107301)
(71, -0.000647308)
(71.2, 0.00596996)
(71.4, 0.0197912)
(71.6, 0.028816)
(71.8, 0.0273464)
(72, 0.0301027)
(72.2, 0.01945)
(72.4, -0.00316143)
(72.6, -0.0141375)
(72.8, -0.00588233)
(73, 0.00134223)
(73.2, 0.0120627)
(73.4, 0.0266696)
(73.6, 0.0349769)
(73.8, 0.0334082)
(74, 0.0292632)
(74.2, 0.0115529)
(74.4, 0.0180622)
(74.6, 0.0247665)
(74.8, 0.0272748)
(75, 0.0293176)
(75.2, 0.0242636)
(75.4, 0.0268526)
(75.6, 0.028215)
(75.8, 0.0288303)
(76, 0.0282033)
(76.2, 0.0274528)
(76.4, 0.0242541)
(76.6, 0.0205251)
(76.8, 0.0225581)
(77, 0.0192803)
(77.2, 0.0249077)
(77.4, 0.0262778)
(77.6, 0.0279809)
(77.8, 0.0254219)
(78, 0.0238116)
(78.2, 0.0241507)
(78.4, 0.0228343)
(78.6, 0.0224155)
(78.8, 0.0238159)
(79, 0.0219918)
(79.2, 0.024869)
(79.4, 0.0234772)
(79.6, 0.0233623)
(79.8, 0.0244855)
(80, 0.0222035)
(80.2, 0.0264522)
(80.4, 0.0238285)
(80.6, 0.0235583)
(80.8, 0.024321)
(81, 0.0232838)
(81.2, 0.0257316)
(81.4, 0.0269953)
(81.6, 0.024339)
(81.8, 0.0248235)
(82, 0.0210837)
(82.2, 0.0240371)
(82.4, 0.0230982)
};

==> exp_plots/hover_dyanmic_payload/x_des.tex <==
\addplot[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates {
(8, 0)
(8.2, 0)
(8.4, 0)
(8.6, 0)
(8.8, 0)
(9, 0)
(9.2, 0)
(9.4, 0)
(9.6, 0)
(9.8, 0)
(10, 0)
(10.2, 0)
(10.4, 0)
(10.6, 0)
(10.8, 0)
(11, 0)
(11.2, 0)
(11.4, 0)
(11.6, 0)
(11.8, 0)
(12, 0)
(12.2, 0)
(12.4, 0)
(12.6, 0)
(12.8, 0)
(13, 0)
(13.2, 0)
(13.4, 0)
(13.6, 0)
(13.8, 0)
(14, 0)
(14.2, 0)
(14.4, 0)
(14.6, 0)
(14.8, 0)
(15, 0)
(15.2, 0)
(15.4, 0)
(15.6, 0)
(15.8, 0)
(16, 0)
(16.2, 0)
(16.4, 0)
(16.6, 0)
(16.8, 0)
(17, 0)
(17.2, 0)
(17.4, 0)
(17.6, 0)
(17.8, 0)
(18, 0)
(18.2, 0)
(18.4, 0)
(18.6, 0)
(18.8, 0)
(19, 0)
(19.2, 0)
(19.4, 0)
(19.6, 0)
(19.8, 0)
(20, 0)
(20.2, 0)
(20.4, 0)
(20.6, 0)
(20.8, 0)
(21, 0)
(21.2, 0)
(21.4, 0)
(21.6, 0)
(21.8, 0)
(22, 0)
(22.2, 0)
(22.4, 0)
(22.6, 0)
(22.8, 0)
(23, 0)
(23.2, 0)
(23.4, 0)
(23.6, 0)
(23.8, 0)
(24, 0)
(24.2, 0)
(24.4, 0)
(24.6, 0)
(24.8, 0)
(25, 0)
(25.2, 0)
(25.4, 0)
(25.6, 0)
(25.8, 0)
(26, 0)
(26.2, 0)
(26.4, 0)
(26.6, 0)
(26.8, 0)
(27, 0)
(27.2, 0)
(27.4, 0)
(27.6, 0)
(27.8, 0)
(28, 0)
(28.2, 0)
(28.4, 0)
(28.6, 0)
(28.8, 0)
(29, 0)
(29.2, 0)
(29.4, 0)
(29.6, 0)
(29.8, 0)
(30, 0)
(30.2, 0)
(30.4, 0)
(30.6, 0)
(30.8, 0)
(31, 0)
(31.2, 0)
(31.4, 0)
(31.6, 0)
(31.8, 0)
(32, 0)
(32.2, 0)
(32.4, 0)
(32.6, 0)
(32.8, 0)
(33, 0)
(33.2, 0)
(33.4, 0)
(33.6, 0)
(33.8, 0)
(34, 0)
(34.2, 0)
(34.4, 0)
(34.6, 0)
(34.8, 0)
(35, 0)
(35.2, 0)
(35.4, 0)
(35.6, 0)
(35.8, 0)
(36, 0)
(36.2, 0)
(36.4, 0)
(36.6, 0)
(36.8, 0)
(37, 0)
(37.2, 0)
(37.4, 0)
(37.6, 0)
(37.8, 0)
(38, 0)
(38.2, 0)
(38.4, 0)
(38.6, 0)
(38.8, 0)
(39, 0)
(39.2, 0)
(39.4, 0)
(39.6, 0)
(39.8, 0)
(40, 0)
(40.2, 0)
(40.4, 0)
(40.6, 0)
(40.8, 0)
(41, 0)
(41.2, 0)
(41.4, 0)
(41.6, 0)
(41.8, 0)
(42, 0)
(42.2, 0)
(42.4, 0)
(42.6, 0)
(42.8, 0)
(43, 0)
(43.2, 0)
(43.4, 0)
(43.6, 0)
(43.8, 0)
(44, 0)
};

==> exp_plots/hover_dyanmic_payload/y.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, -0.133355)
(0.2, -0.00318656)
(0.4, -0.00750739)
(0.6, -0.00462392)
(0.8, -0.00234201)
(1, -0.00489901)
(1.2, 0.00175474)
(1.4, 0.0030477)
(1.6, 0.00278073)
(1.8, 0.000984163)
(2, 0.00058343)
(2.2, 0.000899888)
(2.4, -0.000561135)
(2.6, -0.00152213)
(2.8, 0.00163562)
(3, -0.0131056)
(3.2, -0.0368787)
(3.4, -0.0669228)
(3.6, -0.0846253)
(3.8, -0.102367)
(4, -0.114971)
(4.2, -0.126236)
(4.4, -0.137774)
(4.6, -0.146673)
(4.8, -0.146429)
(5, -0.142374)
(5.2, -0.132978)
(5.4, -0.104303)
(5.6, -0.0899282)
(5.8, -0.0733823)
(6, -0.0446271)
(6.2, -0.0160344)
(6.4, -0.00718077)
(6.6, -0.0139065)
(6.8, -0.0256678)
(7, -0.0271528)
(7.2, -0.0298448)
(7.4, -0.0346356)
(7.6, -0.0513285)
(7.8, -0.0665561)
(8, -0.0711325)
(8.2, -0.0716175)
(8.4, -0.0659178)
(8.6, -0.0690101)
(8.8, -0.0757794)
(9, -0.0675313)
(9.2, -0.0599443)
(9.4, -0.0514688)
(9.6, -0.0355586)
(9.8, -0.027765)
(10, -0.00625147)
(10.2, 0.0159924)
(10.4, 0.0111112)
(10.6, 0.0012419)
(10.8, -0.00396397)
(11, -0.0187536)
(11.2, -0.0175006)
(11.4, -0.0245798)
(11.6, -0.0403283)
(11.8, -0.0707917)
(12, -0.0983665)
(12.2, -0.103742)
(12.4, -0.0930303)
(12.6, -0.0914152)
(12.8, -0.0900715)
(13, -0.0947008)
(13.2, -0.0716241)
(13.4, -0.0607755)
(13.6, -0.0500552)
(13.8, -0.0226526)
(14, -0.00973653)
(14.2, -0.00982379)
(14.4, -0.0130676)
(14.6, -0.0194261)
(14.8, -0.0234929)
(15, -0.0415747)
(15.2, -0.062273)
(15.4, -0.068098)
(15.6, -0.0674265)
(15.8, -0.07802)
(16, -0.0938508)
(16.2, -0.0997409)
(16.4, -0.106522)
(16.6, -0.111039)
(16.8, -0.110852)
(17, -0.111112)
(17.2, -0.111179)
(17.4, -0.110069)
(17.6, -0.0803855)
(17.8, -0.0771448)
(18, -0.0765185)
(18.2, -0.0532386)
(18.4, -0.0214945)
(18.6, -0.00657167)
(18.8, -0.00968411)
(19, -0.00535649)
(19.2, -0.00105882)
(19.4, -0.0028334)
(19.6, -0.00462721)
(19.8, -0.012928)
(20, -0.0235278)
(20.2, -0.0347621)
(20.4, -0.0480867)
(20.6, -0.0583225)
(20.8, -0.0722933)
(21, -0.0905166)
(21.2, -0.103481)
(21.4, -0.108171)
(21.6, -0.108298)
(21.8, -0.0976648)
(22, -0.0543324)
(22.2, -0.00813121)
(22.4, 0.0100933)
(22.6, 0.0127765)
(22.8, 0.0128298)
(23, 0.0131399)
(23.2, 0.010114)
(23.4, 0.0100028)
(23.6, -0.0296381)
(23.8, -0.0524061)
(24, -0.0588828)
(24.2, -0.0747612)
(24.4, -0.0753031)
(24.6, -0.0829881)
(24.8, -0.0880643)
(25, -0.0978689)
(25.2, -0.103446)
(25.4, -0.104654)
(25.6, -0.104493)
(25.8, -0.0860901)
(26, -0.0753224)
(26.2, -0.0749301)
(26.4, -0.0793507)
(26.6, -0.0822356)
(26.8, -0.0824408)
(27, -0.0822609)
(27.2, -0.0750506)
(27.4, -0.0711309)
(27.6, -0.0619634)
(27.8, -0.057087)
(28, -0.0433417)
(28.2, -0.0328288)
(28.4, -0.0289966)
(28.6, -0.0288156)
(28.8, -0.0246411)
(29, -0.0241649)
(29.2, -0.0275538)
(29.4, -0.0325547)
(29.6, -0.0393671)
(29.8, -0.0458482)
(30, -0.0505125)
(30.2, -0.0574436)
(30.4, -0.0529894)
(30.6, -0.0489948)
(30.8, -0.0489561)
(31, -0.0516455)
(31.2, -0.0459338)
(31.4, -0.0387277)
(31.6, -0.0145307)
(31.8, 0.0231633)
(32, 0.0542475)
(32.2, 0.0575413)
(32.4, 0.0574356)
(32.6, 0.0278111)
(32.8, -0.0346781)
(33, -0.0708162)
(33.2, -0.114592)
(33.4, -0.134974)
(33.6, -0.153386)
(33.8, -0.153585)
(34, -0.147835)
(34.2, -0.134349)
(34.4, -0.110102)
(34.6, -0.0761093)
(34.8, -0.0212663)
(35, 0.00299098)
(35.2, -0.00435214)
(35.4, -0.0158058)
(35.6, -0.038531)
(35.8, -0.0459059)
(36, -0.0668722)
(36.2, -0.0813187)
(36.4, -0.0867542)
(36.6, -0.0975994)
(36.8, -0.114497)
(37, -0.118309)
(37.2, -0.115424)
(37.4, -0.114708)
(37.6, -0.117035)
(37.8, -0.113981)
(38, -0.0998343)
(38.2, -0.0689395)
(38.4, -0.0442605)
(38.6, -0.0328993)
(38.8, -0.0306735)
(39, -0.0281874)
(39.2, -0.0208007)
(39.4, -0.0370533)
(39.6, -0.0488437)
(39.8, -0.062736)
(40, -0.0870846)
(40.2, -0.110395)
(40.4, -0.116333)
(40.6, -0.107127)
(40.8, -0.096182)
(41, -0.0782063)
(41.2, -0.0632772)
(41.4, -0.0662948)
(41.6, -0.0613332)
(41.8, -0.0649406)
(42, -0.0674782)
(42.2, -0.0697463)
(42.4, -0.0743526)
(42.6, -0.0745724)
(42.8, -0.0811528)
(43, -0.0814386)
(43.2, -0.084063)
(43.4, -0.0863779)
(43.6, -0.0831215)
(43.8, -0.0618801)
(44, -0.0358065)
(44.2, -0.00819956)
(44.4, 0.00291566)
(44.6, 0.00525539)
(44.8, -0.000561334)
(45, -0.00580946)
(45.2, -0.0163039)
(45.4, -0.05087)
(45.6, -0.0724191)
(45.8, -0.0862386)
(46, -0.0867577)
(46.2, -0.0900118)
(46.4, -0.105746)
(46.6, -0.118419)
(46.8, -0.124836)
(47, -0.130719)
(47.2, -0.127509)
(47.4, -0.115568)
(47.6, -0.0853378)
(47.8, -0.0734193)
(48, -0.0448712)
(48.2, -0.0269822)
(48.4, -0.0226715)
(48.6, -0.00884822)
(48.8, -0.014465)
(49, -0.0148282)
(49.2, -0.0387294)
(49.4, -0.049031)
(49.6, -0.0670388)
(49.8, -0.0765208)
(50, -0.111111)
(50.2, -0.139004)
(50.4, -0.153939)
(50.6, -0.146448)
(50.8, -0.151974)
(51, -0.148664)
(51.2, -0.151236)
(51.4, -0.12862)
(51.6, -0.114027)
(51.8, -0.06702)
(52, -0.0406151)
(52.2, -0.0315249)
(52.4, -0.0340497)
(52.6, -0.0393067)
(52.8, -0.0451652)
(53, -0.0420648)
(53.2, -0.0423133)
(53.4, -0.0501962)
(53.6, -0.0538936)
(53.8, -0.0496726)
(54, -0.0574287)
(54.2, -0.0589144)
(54.4, -0.0642378)
(54.6, -0.0602947)
(54.8, -0.0572837)
(55, -0.0481259)
(55.2, -0.0402992)
(55.4, -0.0347047)
(55.6, -0.0344917)
(55.8, -0.0383028)
(56, -0.0378227)
(56.2, -0.0412078)
(56.4, -0.0391124)
(56.6, -0.034169)
(56.8, -0.0298066)
(57, -0.0221083)
(57.2, -0.02309)
(57.4, -0.018791)
(57.6, -0.00505676)
(57.8, 0.0107804)
(58, 0.0174012)
(58.2, 0.0116235)
(58.4, -0.0104236)
(58.6, -0.0416439)
(58.8, -0.0658206)
(59, -0.0916846)
(59.2, -0.105175)
(59.4, -0.114586)
(59.6, -0.11673)
(59.8, -0.125232)
(60, -0.123338)
(60.2, -0.123745)
(60.4, -0.124105)
(60.6, -0.120963)
(60.8, -0.120574)
(61, -0.124739)
(61.2, -0.115244)
(61.4, -0.0816289)
(61.6, -0.0700839)
(61.8, -0.0605412)
(62, -0.0402121)
(62.2, -0.0337724)
(62.4, -0.0379128)
(62.6, -0.0503709)
(62.8, -0.0551686)
(63, -0.0623862)
(63.2, -0.0678571)
(63.4, -0.0726993)
(63.6, -0.0684822)
(63.8, -0.0577489)
(64, -0.034818)
(64.2, -0.0223412)
(64.4, -0.0262389)
(64.6, -0.0234615)
(64.8, -0.0350377)
(65, -0.044881)
(65.2, -0.0583541)
(65.4, -0.0743293)
(65.6, -0.0982198)
(65.8, -0.121338)
(66, -0.123627)
(66.2, -0.118488)
(66.4, -0.115331)
(66.6, -0.111507)
(66.8, -0.084919)
(67, -0.0593278)
(67.2, -0.0371308)
(67.4, -0.0151457)
(67.6, -0.0168451)
(67.8, -0.0174327)
(68, -0.0219224)
(68.2, -0.0242814)
(68.4, -0.0383978)
(68.6, -0.051553)
(68.8, -0.0632398)
(69, -0.0691926)
(69.2, -0.0422531)
(69.4, -0.0386219)
(69.6, -0.0362611)
(69.8, -0.0434199)
(70, -0.0359604)
(70.2, -0.0288588)
(70.4, -0.0218547)
(70.6, -0.0152935)
(70.8, -0.000731713)
(71, 0.00723094)
(71.2, -0.000248258)
(71.4, -0.0263151)
(71.6, -0.0514681)
(71.8, -0.0768127)
(72, -0.0708621)
(72.2, -0.0688336)
(72.4, -0.0858067)
(72.6, -0.105561)
(72.8, -0.114097)
(73, -0.115457)
(73.2, -0.125012)
(73.4, -0.13961)
(73.6, -0.135134)
(73.8, -0.122032)
(74, -0.113745)
(74.2, -0.0827927)
(74.4, -0.0700787)
(74.6, -0.0623599)
(74.8, -0.0626855)
(75, -0.0712162)
(75.2, -0.0703607)
(75.4, -0.0694382)
(75.6, -0.0702349)
(75.8, -0.0692932)
(76, -0.0695317)
(76.2, -0.0672616)
(76.4, -0.0658583)
(76.6, -0.0712959)
(76.8, -0.0677879)
(77, -0.0648054)
(77.2, -0.0631)
(77.4, -0.0641183)
(77.6, -0.068275)
(77.8, -0.0656966)
(78, -0.0657989)
(78.2, -0.0654251)
(78.4, -0.0676543)
(78.6, -0.0672779)
(78.8, -0.0672663)
(79, -0.0680327)
(79.2, -0.0651044)
(79.4, -0.0648503)
(79.6, -0.0676241)
(79.8, -0.0618004)
(80, -0.0651954)
(80.2, -0.0662679)
(80.4, -0.0679609)
(80.6, -0.065877)
(80.8, -0.0640626)
(81, -0.0648817)
(81.2, -0.0686249)
(81.4, -0.0655102)
(81.6, -0.0636432)
(81.8, -0.0612701)
(82, -0.0660984)
(82.2, -0.0642669)
(82.4, -0.062347)
};

==> exp_plots/hover_dyanmic_payload/y_des.tex <==
\addplot[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates {
(0, 0)
(0.2, 0)
(0.4, 0)
(0.6, 0)
(0.8, 0)
(1, 0)
(1.2, 0)
(1.4, 0)
(1.6, 0)
(1.8, 0)
(2, 0)
(2.2, 0)
(2.4, 0)
(2.6, 0)
(2.8, 0)
(3, 0)
(3.2, 0)
(3.4, 0)
(3.6, 0)
(3.8, 0)
(4, 0)
(4.2, 0)
(4.4, 0)
(4.6, 0)
(4.8, 0)
(5, 0)
(5.2, 0)
(5.4, 0)
(5.6, 0)
(5.8, 0)
(6, 0)
(6.2, 0)
(6.4, 0)
(6.6, 0)
(6.8, 0)
(7, 0)
(7.2, 0)
(7.4, 0)
(7.6, 0)
(7.8, 0)
(8, 0)
(8.2, 0)
(8.4, 0)
(8.6, 0)
(8.8, 0)
(9, 0)
(9.2, 0)
(9.4, 0)
(9.6, 0)
(9.8, 0)
(10, 0)
(10.2, 0)
(10.4, 0)
(10.6, 0)
(10.8, 0)
(11, 0)
(11.2, 0)
(11.4, 0)
(11.6, 0)
(11.8, 0)
(12, 0)
(12.2, 0)
(12.4, 0)
(12.6, 0)
(12.8, 0)
(13, 0)
(13.2, 0)
(13.4, 0)
(13.6, 0)
(13.8, 0)
(14, 0)
(14.2, 0)
(14.4, 0)
(14.6, 0)
(14.8, 0)
(15, 0)
(15.2, 0)
(15.4, 0)
(15.6, 0)
(15.8, 0)
(16, 0)
(16.2, 0)
(16.4, 0)
(16.6, 0)
(16.8, 0)
(17, 0)
(17.2, 0)
(17.4, 0)
(17.6, 0)
(17.8, 0)
(18, 0)
(18.2, 0)
(18.4, 0)
(18.6, 0)
(18.8, 0)
(19, 0)
(19.2, 0)
(19.4, 0)
(19.6, 0)
(19.8, 0)
(20, 0)
(20.2, 0)
(20.4, 0)
(20.6, 0)
(20.8, 0)
(21, 0)
(21.2, 0)
(21.4, 0)
(21.6, 0)
(21.8, 0)
(22, 0)
(22.2, 0)
(22.4, 0)
(22.6, 0)
(22.8, 0)
(23, 0)
(23.2, 0)
(23.4, 0)
(23.6, 0)
(23.8, 0)
(24, 0)
(24.2, 0)
(24.4, 0)
(24.6, 0)
(24.8, 0)
(25, 0)
(25.2, 0)
(25.4, 0)
(25.6, 0)
(25.8, 0)
(26, 0)
(26.2, 0)
(26.4, 0)
(26.6, 0)
(26.8, 0)
(27, 0)
(27.2, 0)
(27.4, 0)
(27.6, 0)
(27.8, 0)
(28, 0)
(28.2, 0)
(28.4, 0)
(28.6, 0)
(28.8, 0)
(29, 0)
(29.2, 0)
(29.4, 0)
(29.6, 0)
(29.8, 0)
(30, 0)
(30.2, 0)
(30.4, 0)
(30.6, 0)
(30.8, 0)
(31, 0)
(31.2, 0)
(31.4, 0)
(31.6, 0)
(31.8, 0)
(32, 0)
(32.2, 0)
(32.4, 0)
(32.6, 0)
(32.8, 0)
(33, 0)
(33.2, 0)
(33.4, 0)
(33.6, 0)
(33.8, 0)
(34, 0)
(34.2, 0)
(34.4, 0)
(34.6, 0)
(34.8, 0)
(35, 0)
(35.2, 0)
(35.4, 0)
(35.6, 0)
(35.8, 0)
(36, 0)
(36.2, 0)
(36.4, 0)
(36.6, 0)
(36.8, 0)
(37, 0)
(37.2, 0)
(37.4, 0)
(37.6, 0)
(37.8, 0)
(38, 0)
(38.2, 0)
(38.4, 0)
(38.6, 0)
(38.8, 0)
(39, 0)
(39.2, 0)
(39.4, 0)
(39.6, 0)
(39.8, 0)
(40, 0)
(40.2, 0)
(40.4, 0)
(40.6, 0)
(40.8, 0)
(41, 0)
(41.2, 0)
(41.4, 0)
(41.6, 0)
(41.8, 0)
(42, 0)
(42.2, 0)
(42.4, 0)
(42.6, 0)
(42.8, 0)
(43, 0)
(43.2, 0)
(43.4, 0)
(43.6, 0)
(43.8, 0)
(44, 0)
(44.2, 0)
(44.4, 0)
(44.6, 0)
(44.8, 0)
(45, 0)
(45.2, 0)
(45.4, 0)
(45.6, 0)
(45.8, 0)
(46, 0)
(46.2, 0)
(46.4, 0)
(46.6, 0)
(46.8, 0)
(47, 0)
(47.2, 0)
(47.4, 0)
(47.6, 0)
(47.8, 0)
(48, 0)
(48.2, 0)
(48.4, 0)
(48.6, 0)
(48.8, 0)
(49, 0)
(49.2, 0)
(49.4, 0)
(49.6, 0)
(49.8, 0)
(50, 0)
(50.2, 0)
(50.4, 0)
(50.6, 0)
(50.8, 0)
(51, 0)
(51.2, 0)
(51.4, 0)
(51.6, 0)
(51.8, 0)
(52, 0)
(52.2, 0)
(52.4, 0)
(52.6, 0)
(52.8, 0)
(53, 0)
(53.2, 0)
(53.4, 0)
(53.6, 0)
(53.8, 0)
(54, 0)
(54.2, 0)
(54.4, 0)
(54.6, 0)
(54.8, 0)
(55, 0)
(55.2, 0)
(55.4, 0)
(55.6, 0)
(55.8, 0)
(56, 0)
(56.2, 0)
(56.4, 0)
(56.6, 0)
(56.8, 0)
(57, 0)
(57.2, 0)
(57.4, 0)
(57.6, 0)
(57.8, 0)
(58, 0)
(58.2, 0)
(58.4, 0)
(58.6, 0)
(58.8, 0)
(59, 0)
(59.2, 0)
(59.4, 0)
(59.6, 0)
(59.8, 0)
(60, 0)
(60.2, 0)
(60.4, 0)
(60.6, 0)
(60.8, 0)
(61, 0)
(61.2, 0)
(61.4, 0)
(61.6, 0)
(61.8, 0)
(62, 0)
(62.2, 0)
(62.4, 0)
(62.6, 0)
(62.8, 0)
(63, 0)
(63.2, 0)
(63.4, 0)
(63.6, 0)
(63.8, 0)
(64, 0)
(64.2, 0)
(64.4, 0)
(64.6, 0)
(64.8, 0)
(65, 0)
(65.2, 0)
(65.4, 0)
(65.6, 0)
(65.8, 0)
(66, 0)
(66.2, 0)
(66.4, 0)
(66.6, 0)
(66.8, 0)
(67, 0)
(67.2, 0)
(67.4, 0)
(67.6, 0)
(67.8, 0)
(68, 0)
(68.2, 0)
(68.4, 0)
(68.6, 0)
(68.8, 0)
(69, 0)
(69.2, 0)
(69.4, 0)
(69.6, 0)
(69.8, 0)
(70, 0)
(70.2, 0)
(70.4, 0)
(70.6, 0)
(70.8, 0)
(71, 0)
(71.2, 0)
(71.4, 0)
(71.6, 0)
(71.8, 0)
(72, 0)
(72.2, 0)
(72.4, 0)
(72.6, 0)
(72.8, 0)
(73, 0)
(73.2, 0)
(73.4, 0)
(73.6, 0)
(73.8, 0)
(74, 0)
(74.2, 0)
(74.4, 0)
(74.6, 0)
(74.8, 0)
(75, 0)
(75.2, 0)
(75.4, 0)
(75.6, 0)
(75.8, 0)
(76, 0)
(76.2, 0)
(76.4, 0)
(76.6, 0)
(76.8, 0)
(77, 0)
(77.2, 0)
(77.4, 0)
(77.6, 0)
(77.8, 0)
(78, 0)
(78.2, 0)
(78.4, 0)
(78.6, 0)
(78.8, 0)
(79, 0)
(79.2, 0)
(79.4, 0)
(79.6, 0)
(79.8, 0)
(80, 0)
(80.2, 0)
(80.4, 0)
(80.6, 0)
(80.8, 0)
(81, 0)
(81.2, 0)
(81.4, 0)
(81.6, 0)
(81.8, 0)
(82, 0)
(82.2, 0)
(82.4, 0)
};

==> exp_plots/hover_dyanmic_payload/yaw.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 1.31268)
(0.2, -0.341074)
(0.4, -0.30526)
(0.6, -0.286435)
(0.8, -0.334684)
(1, -0.290144)
(1.2, -0.396506)
(1.4, -0.383933)
(1.6, -0.359834)
(1.8, -0.330932)
(2, -0.367579)
(2.2, -0.353879)
(2.4, -0.332065)
(2.6, 0.129473)
(2.8, 0.896639)
(3, 1.95937)
(3.2, 2.61769)
(3.4, 2.2888)
(3.6, 1.48744)
(3.8, 0.850953)
(4, 0.50776)
(4.2, 0.160687)
(4.4, -0.0946667)
(4.6, -0.29167)
(4.8, -0.234401)
(5, -0.12371)
(5.2, 0.0303377)
(5.4, -0.132645)
(5.6, -0.0618936)
(5.8, -0.134776)
(6, -0.193158)
(6.2, -0.34187)
(6.4, -0.113428)
(6.6, 0.29105)
(6.8, 0.410444)
(7, 0.448961)
(7.2, 0.303346)
(7.4, -0.0929355)
(7.6, -0.401991)
(7.8, -0.602618)
(8, -0.595116)
(8.2, -0.306411)
(8.4, 0.209822)
(8.6, 0.536485)
(8.8, 0.905613)
(9, 1.14496)
(9.2, 1.27832)
(9.4, 1.18218)
(9.6, 0.790707)
(9.8, 0.292458)
(10, -0.575807)
(10.2, -1.06687)
(10.4, -1.28647)
(10.6, -1.4045)
(10.8, -1.29686)
(11, -0.827531)
(11.2, -0.814054)
(11.4, -0.629297)
(11.6, -0.580408)
(11.8, -0.522689)
(12, -0.224367)
(12.2, -0.300133)
(12.4, -0.362631)
(12.6, -0.276666)
(12.8, -0.104279)
(13, 0.174684)
(13.2, 0.112377)
(13.4, 0.671274)
(13.6, 1.04326)
(13.8, 0.625392)
(14, 0.258043)
(14.2, -0.25833)
(14.4, -0.849065)
(14.6, -1.57959)
(14.8, -1.88101)
(15, -0.867989)
(15.2, -0.777095)
(15.4, -0.540434)
(15.6, -0.402792)
(15.8, 0.112344)
(16, 0.557674)
(16.2, 0.901108)
(16.4, 1.15665)
(16.6, 1.23544)
(16.8, 0.799736)
(17, 0.45745)
(17.2, 0.0396212)
(17.4, -0.458688)
(17.6, -0.803903)
(17.8, -0.875013)
(18, -0.937441)
(18.2, -0.795126)
(18.4, -0.36359)
(18.6, 0.254804)
(18.8, 0.645834)
(19, 0.713051)
(19.2, 0.491203)
(19.4, -0.13243)
(19.6, -1.23925)
(19.8, -1.89036)
(20, -2.4492)
(20.2, -2.38812)
(20.4, -1.6547)
(20.6, -0.861042)
(20.8, 0.314861)
(21, 1.12595)
(21.2, 1.19335)
(21.4, 0.870537)
(21.6, 0.430307)
(21.8, 0.308313)
(22, -0.193003)
(22.2, -0.762259)
(22.4, -1.29784)
(22.6, -1.15144)
(22.8, -1.16443)
(23, -0.871393)
(23.2, -0.223576)
(23.4, 0.121131)
(23.6, 0.785203)
(23.8, 0.625124)
(24, 0.163562)
(24.2, -0.249272)
(24.4, -0.627436)
(24.6, -0.467918)
(24.8, -0.162163)
(25, 0.371663)
(25.2, 0.587335)
(25.4, 0.755705)
(25.6, 0.699735)
(25.8, 0.566879)
(26, 0.426678)
(26.2, 0.329809)
(26.4, 0.324922)
(26.6, 0.28078)
(26.8, 0.333319)
(27, 0.859974)
(27.2, 1.50274)
(27.4, 1.9685)
(27.6, 1.82858)
(27.8, 0.980309)
(28, 0.108495)
(28.2, -0.778121)
(28.4, -1.37275)
(28.6, -1.87579)
(28.8, -2.09986)
(29, -1.53905)
(29.2, -0.759022)
(29.4, 0.515561)
(29.6, 2.1467)
(29.8, 3.22769)
(30, 3.34283)
(30.2, 2.49721)
(30.4, 1.23385)
(30.6, -0.0820471)
(30.8, -0.426787)
(31, -0.880388)
(31.2, -1.03935)
(31.4, -1.16764)
(31.6, -2.3327)
(31.8, -4.09101)
(32, -4.41566)
(32.2, -2.84508)
(32.4, -0.782161)
(32.6, 1.19613)
(32.8, 2.63487)
(33, 3.83891)
(33.2, 4.05103)
(33.4, 3.5906)
(33.6, 2.513)
(33.8, 0.481965)
(34, -1.57467)
(34.2, -3.70967)
(34.4, -4.55353)
(34.6, -4.16617)
(34.8, -2.98315)
(35, -0.722567)
(35.2, 2.38289)
(35.4, 3.89527)
(35.6, 4.12941)
(35.8, 3.50372)
(36, 1.38564)
(36.2, -0.410589)
(36.4, -2.22598)
(36.6, -3.87084)
(36.8, -3.96175)
(37, -2.99015)
(37.2, -1.99278)
(37.4, -0.657789)
(37.6, 0.777418)
(37.8, 1.86314)
(38, 1.99534)
(38.2, 1.78158)
(38.4, 0.790133)
(38.6, 0.202375)
(38.8, 0.415161)
(39, 0.668924)
(39.2, 0.955169)
(39.4, 1.43959)
(39.6, 1.97568)
(39.8, 2.41564)
(40, 3.42413)
(40.2, 4.14816)
(40.4, 4.29767)
(40.6, 3.58536)
(40.8, 2.10901)
(41, 0.403178)
(41.2, -0.615131)
(41.4, -1.03453)
(41.6, -1.36117)
(41.8, -0.649667)
(42, -0.110332)
(42.2, 0.375062)
(42.4, 0.612565)
(42.6, 0.762781)
(42.8, 0.884164)
(43, 0.487338)
(43.2, 0.117567)
(43.4, -0.8487)
(43.6, -1.62392)
(43.8, -2.08349)
(44, -2.31846)
(44.2, -2.08316)
(44.4, -1.6949)
(44.6, -1.17398)
(44.8, -0.415627)
(45, -0.0979305)
(45.2, 0.170531)
(45.4, 0.418675)
(45.6, 0.230933)
(45.8, -0.520788)
(46, -1.19673)
(46.2, -1.42186)
(46.4, -1.28357)
(46.6, -0.722545)
(46.8, 0.0141912)
(47, 0.815028)
(47.2, 1.55265)
(47.4, 1.65743)
(47.6, 1.80607)
(47.8, 2.03856)
(48, 1.65044)
(48.2, 1.26466)
(48.4, 0.892126)
(48.6, 0.881646)
(48.8, 0.792336)
(49, 0.706674)
(49.2, 0.818529)
(49.4, 1.0756)
(49.6, 1.31039)
(49.8, 1.343)
(50, 1.58022)
(50.2, 0.901073)
(50.4, 0.493087)
(50.6, 0.1253)
(50.8, -0.118697)
(51, -0.594794)
(51.2, -0.871377)
(51.4, -1.04825)
(51.6, -0.818511)
(51.8, -0.710431)
(52, -0.48797)
(52.2, -0.231709)
(52.4, -0.0893321)
(52.6, -0.2126)
(52.8, -0.472715)
(53, -0.940722)
(53.2, -1.73591)
(53.4, -2.31846)
(53.6, -2.61637)
(53.8, -2.51095)
(54, -2.05982)
(54.2, -1.67406)
(54.4, -1.30701)
(54.6, -1.30258)
(54.8, -1.23617)
(55, -1.13333)
(55.2, -0.738663)
(55.4, -0.107733)
(55.6, 1.0118)
(55.8, 1.69058)
(56, 1.94923)
(56.2, 1.92159)
(56.4, 1.28591)
(56.6, 0.454064)
(56.8, -0.311731)
(57, -0.60274)
(57.2, -0.669023)
(57.4, -0.817535)
(57.6, -0.625051)
(57.8, 0.0290417)
(58, 0.928701)
(58.2, 1.91685)
(58.4, 2.6888)
(58.6, 2.85404)
(58.8, 2.2681)
(59, 1.46152)
(59.2, 0.101932)
(59.4, -1.66865)
(59.6, -1.75334)
(59.8, -1.64535)
(60, -0.934036)
(60.2, 0.0254693)
(60.4, 1.00754)
(60.6, 1.42958)
(60.8, 1.11427)
(61, -0.037389)
(61.2, -0.894264)
(61.4, -1.51294)
(61.6, -1.88069)
(61.8, -1.69501)
(62, -1.71322)
(62.2, -0.871986)
(62.4, -0.289477)
(62.6, 0.162007)
(62.8, 0.351344)
(63, 0.32004)
(63.2, -0.318233)
(63.4, -1.04308)
(63.6, -1.85962)
(63.8, -2.50809)
(64, -2.72314)
(64.2, -1.88693)
(64.4, -0.408935)
(64.6, 0.501193)
(64.8, 1.15661)
(65, 1.20343)
(65.2, 0.876553)
(65.4, 0.322832)
(65.6, -0.24967)
(65.8, -0.644403)
(66, -0.747641)
(66.2, -0.448876)
(66.4, -0.00571933)
(66.6, 0.33242)
(66.8, 0.0840385)
(67, -0.0458423)
(67.2, 0.0760664)
(67.4, 0.330556)
(67.6, 0.316085)
(67.8, -0.0177023)
(68, -0.51112)
(68.2, -0.829229)
(68.4, -0.56348)
(68.6, -0.293241)
(68.8, -0.189288)
(69, -0.021947)
(69.2, 0.683747)
(69.4, 1.70969)
(69.6, 2.53409)
(69.8, 2.98036)
(70, 2.91067)
(70.2, 2.35886)
(70.4, 1.15047)
(70.6, -0.168289)
(70.8, -1.07909)
(71, -1.32915)
(71.2, -1.28457)
(71.4, -1.08902)
(71.6, -1.14486)
(71.8, -1.11441)
(72, -1.77931)
(72.2, -1.80173)
(72.4, -1.36547)
(72.6, -1.02909)
(72.8, -0.891222)
(73, -0.674048)
(73.2, -0.14171)
(73.4, 0.38251)
(73.6, 0.413648)
(73.8, 0.141002)
(74, 0.323682)
(74.2, 0.424412)
(74.4, 0.445958)
(74.6, 1.16585)
(74.8, 1.70794)
(75, 1.91957)
(75.2, 1.90254)
(75.4, 1.7958)
(75.6, 1.82899)
(75.8, 1.69609)
(76, 1.73673)
(76.2, 1.73121)
(76.4, 1.76227)
(76.6, 1.86254)
(76.8, 1.7667)
(77, 1.74463)
(77.2, 1.76821)
(77.4, 1.77639)
(77.6, 1.80503)
(77.8, 1.77784)
(78, 1.76796)
(78.2, 1.76084)
(78.4, 1.80053)
(78.6, 1.78244)
(78.8, 1.79714)
(79, 1.75099)
(79.2, 1.75213)
(79.4, 1.77409)
(79.6, 1.80022)
(79.8, 1.74723)
(80, 1.76167)
(80.2, 1.79896)
(80.4, 1.78507)
(80.6, 1.75771)
(80.8, 1.73459)
(81, 1.72196)
(81.2, 1.80171)
(81.4, 1.78112)
(81.6, 1.74164)
(81.8, 1.67243)
(82, 1.75808)
(82.2, 1.75184)
(82.4, 1.71465)
};

==> exp_plots/hover_dyanmic_payload/yaw_des.tex <==
\addplot[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates {
(0, 0)
(0.2, 0)
(0.4, 0)
(0.6, 0)
(0.8, 0)
(1, 0)
(1.2, 0)
(1.4, 0)
(1.6, 0)
(1.8, 0)
(2, 0)
(2.2, 0)
(2.4, 0)
(2.6, 0)
(2.8, 0)
(3, 0)
(3.2, 0)
(3.4, 0)
(3.6, 0)
(3.8, 0)
(4, 0)
(4.2, 0)
(4.4, 0)
(4.6, 0)
(4.8, 0)
(5, 0)
(5.2, 0)
(5.4, 0)
(5.6, 0)
(5.8, 0)
(6, 0)
(6.2, 0)
(6.4, 0)
(6.6, 0)
(6.8, 0)
(7, 0)
(7.2, 0)
(7.4, 0)
(7.6, 0)
(7.8, 0)
(8, 0)
(8.2, 0)
(8.4, 0)
(8.6, 0)
(8.8, 0)
(9, 0)
(9.2, 0)
(9.4, 0)
(9.6, 0)
(9.8, 0)
(10, 0)
(10.2, 0)
(10.4, 0)
(10.6, 0)
(10.8, 0)
(11, 0)
(11.2, 0)
(11.4, 0)
(11.6, 0)
(11.8, 0)
(12, 0)
(12.2, 0)
(12.4, 0)
(12.6, 0)
(12.8, 0)
(13, 0)
(13.2, 0)
(13.4, 0)
(13.6, 0)
(13.8, 0)
(14, 0)
(14.2, 0)
(14.4, 0)
(14.6, 0)
(14.8, 0)
(15, 0)
(15.2, 0)
(15.4, 0)
(15.6, 0)
(15.8, 0)
(16, 0)
(16.2, 0)
(16.4, 0)
(16.6, 0)
(16.8, 0)
(17, 0)
(17.2, 0)
(17.4, 0)
(17.6, 0)
(17.8, 0)
(18, 0)
(18.2, 0)
(18.4, 0)
(18.6, 0)
(18.8, 0)
(19, 0)
(19.2, 0)
(19.4, 0)
(19.6, 0)
(19.8, 0)
(20, 0)
(20.2, 0)
(20.4, 0)
(20.6, 0)
(20.8, 0)
(21, 0)
(21.2, 0)
(21.4, 0)
(21.6, 0)
(21.8, 0)
(22, 0)
(22.2, 0)
(22.4, 0)
(22.6, 0)
(22.8, 0)
(23, 0)
(23.2, 0)
(23.4, 0)
(23.6, 0)
(23.8, 0)
(24, 0)
(24.2, 0)
(24.4, 0)
(24.6, 0)
(24.8, 0)
(25, 0)
(25.2, 0)
(25.4, 0)
(25.6, 0)
(25.8, 0)
(26, 0)
(26.2, 0)
(26.4, 0)
(26.6, 0)
(26.8, 0)
(27, 0)
(27.2, 0)
(27.4, 0)
(27.6, 0)
(27.8, 0)
(28, 0)
(28.2, 0)
(28.4, 0)
(28.6, 0)
(28.8, 0)
(29, 0)
(29.2, 0)
(29.4, 0)
(29.6, 0)
(29.8, 0)
(30, 0)
(30.2, 0)
(30.4, 0)
(30.6, 0)
(30.8, 0)
(31, 0)
(31.2, 0)
(31.4, 0)
(31.6, 0)
(31.8, 0)
(32, 0)
(32.2, 0)
(32.4, 0)
(32.6, 0)
(32.8, 0)
(33, 0)
(33.2, 0)
(33.4, 0)
(33.6, 0)
(33.8, 0)
(34, 0)
(34.2, 0)
(34.4, 0)
(34.6, 0)
(34.8, 0)
(35, 0)
(35.2, 0)
(35.4, 0)
(35.6, 0)
(35.8, 0)
(36, 0)
(36.2, 0)
(36.4, 0)
(36.6, 0)
(36.8, 0)
(37, 0)
(37.2, 0)
(37.4, 0)
(37.6, 0)
(37.8, 0)
(38, 0)
(38.2, 0)
(38.4, 0)
(38.6, 0)
(38.8, 0)
(39, 0)
(39.2, 0)
(39.4, 0)
(39.6, 0)
(39.8, 0)
(40, 0)
(40.2, 0)
(40.4, 0)
(40.6, 0)
(40.8, 0)
(41, 0)
(41.2, 0)
(41.4, 0)
(41.6, 0)
(41.8, 0)
(42, 0)
(42.2, 0)
(42.4, 0)
(42.6, 0)
(42.8, 0)
(43, 0)
(43.2, 0)
(43.4, 0)
(43.6, 0)
(43.8, 0)
(44, 0)
(44.2, 0)
(44.4, 0)
(44.6, 0)
(44.8, 0)
(45, 0)
(45.2, 0)
(45.4, 0)
(45.6, 0)
(45.8, 0)
(46, 0)
(46.2, 0)
(46.4, 0)
(46.6, 0)
(46.8, 0)
(47, 0)
(47.2, 0)
(47.4, 0)
(47.6, 0)
(47.8, 0)
(48, 0)
(48.2, 0)
(48.4, 0)
(48.6, 0)
(48.8, 0)
(49, 0)
(49.2, 0)
(49.4, 0)
(49.6, 0)
(49.8, 0)
(50, 0)
(50.2, 0)
(50.4, 0)
(50.6, 0)
(50.8, 0)
(51, 0)
(51.2, 0)
(51.4, 0)
(51.6, 0)
(51.8, 0)
(52, 0)
(52.2, 0)
(52.4, 0)
(52.6, 0)
(52.8, 0)
(53, 0)
(53.2, 0)
(53.4, 0)
(53.6, 0)
(53.8, 0)
(54, 0)
(54.2, 0)
(54.4, 0)
(54.6, 0)
(54.8, 0)
(55, 0)
(55.2, 0)
(55.4, 0)
(55.6, 0)
(55.8, 0)
(56, 0)
(56.2, 0)
(56.4, 0)
(56.6, 0)
(56.8, 0)
(57, 0)
(57.2, 0)
(57.4, 0)
(57.6, 0)
(57.8, 0)
(58, 0)
(58.2, 0)
(58.4, 0)
(58.6, 0)
(58.8, 0)
(59, 0)
(59.2, 0)
(59.4, 0)
(59.6, 0)
(59.8, 0)
(60, 0)
(60.2, 0)
(60.4, 0)
(60.6, 0)
(60.8, 0)
(61, 0)
(61.2, 0)
(61.4, 0)
(61.6, 0)
(61.8, 0)
(62, 0)
(62.2, 0)
(62.4, 0)
(62.6, 0)
(62.8, 0)
(63, 0)
(63.2, 0)
(63.4, 0)
(63.6, 0)
(63.8, 0)
(64, 0)
(64.2, 0)
(64.4, 0)
(64.6, 0)
(64.8, 0)
(65, 0)
(65.2, 0)
(65.4, 0)
(65.6, 0)
(65.8, 0)
(66, 0)
(66.2, 0)
(66.4, 0)
(66.6, 0)
(66.8, 0)
(67, 0)
(67.2, 0)
(67.4, 0)
(67.6, 0)
(67.8, 0)
(68, 0)
(68.2, 0)
(68.4, 0)
(68.6, 0)
(68.8, 0)
(69, 0)
(69.2, 0)
(69.4, 0)
(69.6, 0)
(69.8, 0)
(70, 0)
(70.2, 0)
(70.4, 0)
(70.6, 0)
(70.8, 0)
(71, 0)
(71.2, 0)
(71.4, 0)
(71.6, 0)
(71.8, 0)
(72, 0)
(72.2, 0)
(72.4, 0)
(72.6, 0)
(72.8, 0)
(73, 0)
(73.2, 0)
(73.4, 0)
(73.6, 0)
(73.8, 0)
(74, 0)
(74.2, 0)
(74.4, 0)
(74.6, 0)
(74.8, 0)
(75, 0)
(75.2, 0)
(75.4, 0)
(75.6, 0)
(75.8, 0)
(76, 0)
(76.2, 0)
(76.4, 0)
(76.6, 0)
(76.8, 0)
(77, 0)
(77.2, 0)
(77.4, 0)
(77.6, 0)
(77.8, 0)
(78, 0)
(78.2, 0)
(78.4, 0)
(78.6, 0)
(78.8, 0)
(79, 0)
(79.2, 0)
(79.4, 0)
(79.6, 0)
(79.8, 0)
(80, 0)
(80.2, 0)
(80.4, 0)
(80.6, 0)
(80.8, 0)
(81, 0)
(81.2, 0)
(81.4, 0)
(81.6, 0)
(81.8, 0)
(82, 0)
(82.2, 0)
(82.4, 0)
};

==> exp_plots/hover_dyanmic_payload/z.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0.00686926)
(0.2, 0.00402774)
(0.4, 0.0035991)
(0.6, 0.00493695)
(0.8, 0.0031073)
(1, 0.00452138)
(1.2, 0.00590937)
(1.4, 0.00597772)
(1.6, 0.0058419)
(1.8, 0.00620064)
(2, 0.00606105)
(2.2, 0.00572019)
(2.4, 0.00616294)
(2.6, 0.00683015)
(2.8, 0.0175008)
(3, 0.0366102)
(3.2, 0.0948671)
(3.4, 0.141426)
(3.6, 0.150046)
(3.8, 0.157026)
(4, 0.178565)
(4.2, 0.205291)
(4.4, 0.230037)
(4.6, 0.250321)
(4.8, 0.274309)
(5, 0.290356)
(5.2, 0.313184)
(5.4, 0.356838)
(5.6, 0.373047)
(5.8, 0.398763)
(6, 0.423764)
(6.2, 0.466592)
(6.4, 0.490198)
(6.6, 0.495255)
(6.8, 0.507232)
(7, 0.508404)
(7.2, 0.512806)
(7.4, 0.509312)
(7.6, 0.518367)
(7.8, 0.523534)
(8, 0.506704)
(8.2, 0.500445)
(8.4, 0.500587)
(8.6, 0.505497)
(8.8, 0.495007)
(9, 0.497191)
(9.2, 0.497658)
(9.4, 0.486828)
(9.6, 0.472724)
(9.8, 0.462854)
(10, 0.455692)
(10.2, 0.469367)
(10.4, 0.475834)
(10.6, 0.486875)
(10.8, 0.491664)
(11, 0.490835)
(11.2, 0.481879)
(11.4, 0.482545)
(11.6, 0.474556)
(11.8, 0.477276)
(12, 0.485186)
(12.2, 0.500464)
(12.4, 0.494691)
(12.6, 0.525809)
(12.8, 0.543929)
(13, 0.547635)
(13.2, 0.548053)
(13.4, 0.542265)
(13.6, 0.537424)
(13.8, 0.520717)
(14, 0.510636)
(14.2, 0.513936)
(14.4, 0.507693)
(14.6, 0.491717)
(14.8, 0.485198)
(15, 0.491744)
(15.2, 0.496072)
(15.4, 0.484913)
(15.6, 0.490708)
(15.8, 0.495328)
(16, 0.487359)
(16.2, 0.480633)
(16.4, 0.476663)
(16.6, 0.473567)
(16.8, 0.474172)
(17, 0.479917)
(17.2, 0.487851)
(17.4, 0.498254)
(17.6, 0.504389)
(17.8, 0.515402)
(18, 0.512365)
(18.2, 0.494532)
(18.4, 0.491446)
(18.6, 0.503296)
(18.8, 0.498)
(19, 0.491974)
(19.2, 0.486382)
(19.4, 0.488779)
(19.6, 0.488801)
(19.8, 0.511463)
(20, 0.521451)
(20.2, 0.523376)
(20.4, 0.523705)
(20.6, 0.506875)
(20.8, 0.513492)
(21, 0.503831)
(21.2, 0.497768)
(21.4, 0.482499)
(21.6, 0.467759)
(21.8, 0.46745)
(22, 0.483523)
(22.2, 0.496719)
(22.4, 0.493914)
(22.6, 0.493636)
(22.8, 0.495367)
(23, 0.497806)
(23.2, 0.497369)
(23.4, 0.501178)
(23.6, 0.483444)
(23.8, 0.478337)
(24, 0.466259)
(24.2, 0.458831)
(24.4, 0.462211)
(24.6, 0.473358)
(24.8, 0.486555)
(25, 0.492845)
(25.2, 0.490255)
(25.4, 0.492909)
(25.6, 0.493182)
(25.8, 0.498896)
(26, 0.497206)
(26.2, 0.498311)
(26.4, 0.505255)
(26.6, 0.501364)
(26.8, 0.500188)
(27, 0.499202)
(27.2, 0.500604)
(27.4, 0.496749)
(27.6, 0.486934)
(27.8, 0.481086)
(28, 0.471542)
(28.2, 0.479916)
(28.4, 0.48678)
(28.6, 0.470239)
(28.8, 0.466808)
(29, 0.480146)
(29.2, 0.48446)
(29.4, 0.499723)
(29.6, 0.499578)
(29.8, 0.512218)
(30, 0.517163)
(30.2, 0.495908)
(30.4, 0.480691)
(30.6, 0.478304)
(30.8, 0.4754)
(31, 0.463184)
(31.2, 0.461535)
(31.4, 0.466591)
(31.6, 0.481736)
(31.8, 0.492702)
(32, 0.492615)
(32.2, 0.504105)
(32.4, 0.504399)
(32.6, 0.502256)
(32.8, 0.488416)
(33, 0.467786)
(33.2, 0.47173)
(33.4, 0.466636)
(33.6, 0.469566)
(33.8, 0.469969)
(34, 0.464158)
(34.2, 0.469007)
(34.4, 0.502606)
(34.6, 0.511067)
(34.8, 0.50909)
(35, 0.510437)
(35.2, 0.508597)
(35.4, 0.507465)
(35.6, 0.500536)
(35.8, 0.495854)
(36, 0.485282)
(36.2, 0.480281)
(36.4, 0.469992)
(36.6, 0.479272)
(36.8, 0.525392)
(37, 0.52431)
(37.2, 0.507236)
(37.4, 0.491146)
(37.6, 0.488307)
(37.8, 0.479721)
(38, 0.459728)
(38.2, 0.432763)
(38.4, 0.406591)
(38.6, 0.430563)
(38.8, 0.449719)
(39, 0.50351)
(39.2, 0.532792)
(39.4, 0.559688)
(39.6, 0.583478)
(39.8, 0.599668)
(40, 0.59581)
(40.2, 0.567365)
(40.4, 0.541605)
(40.6, 0.555192)
(40.8, 0.551124)
(41, 0.513272)
(41.2, 0.484462)
(41.4, 0.482335)
(41.6, 0.487389)
(41.8, 0.503997)
(42, 0.536314)
(42.2, 0.5348)
(42.4, 0.523736)
(42.6, 0.520088)
(42.8, 0.528333)
(43, 0.527919)
(43.2, 0.507145)
(43.4, 0.494906)
(43.6, 0.493861)
(43.8, 0.496498)
(44, 0.488102)
(44.2, 0.493899)
(44.4, 0.507291)
(44.6, 0.512511)
(44.8, 0.504012)
(45, 0.49448)
(45.2, 0.499207)
(45.4, 0.513587)
(45.6, 0.506938)
(45.8, 0.504709)
(46, 0.476396)
(46.2, 0.470038)
(46.4, 0.477186)
(46.6, 0.498538)
(46.8, 0.513798)
(47, 0.537017)
(47.2, 0.538815)
(47.4, 0.539792)
(47.6, 0.549447)
(47.8, 0.547024)
(48, 0.547203)
(48.2, 0.534501)
(48.4, 0.534178)
(48.6, 0.529226)
(48.8, 0.510681)
(49, 0.501257)
(49.2, 0.501818)
(49.4, 0.50606)
(49.6, 0.488679)
(49.8, 0.486212)
(50, 0.487751)
(50.2, 0.470856)
(50.4, 0.453263)
(50.6, 0.456902)
(50.8, 0.473967)
(51, 0.483116)
(51.2, 0.517081)
(51.4, 0.533094)
(51.6, 0.543028)
(51.8, 0.513658)
(52, 0.503826)
(52.2, 0.492068)
(52.4, 0.475818)
(52.6, 0.468409)
(52.8, 0.471874)
(53, 0.48631)
(53.2, 0.48929)
(53.4, 0.487662)
(53.6, 0.491547)
(53.8, 0.492659)
(54, 0.487241)
(54.2, 0.487199)
(54.4, 0.487056)
(54.6, 0.487825)
(54.8, 0.496381)
(55, 0.513787)
(55.2, 0.517097)
(55.4, 0.518032)
(55.6, 0.518891)
(55.8, 0.515386)
(56, 0.507692)
(56.2, 0.48805)
(56.4, 0.477721)
(56.6, 0.460399)
(56.8, 0.455796)
(57, 0.470144)
(57.2, 0.46664)
(57.4, 0.466745)
(57.6, 0.481812)
(57.8, 0.502945)
(58, 0.514708)
(58.2, 0.527179)
(58.4, 0.516473)
(58.6, 0.511342)
(58.8, 0.492792)
(59, 0.487532)
(59.2, 0.493823)
(59.4, 0.490464)
(59.6, 0.506224)
(59.8, 0.495822)
(60, 0.495116)
(60.2, 0.51141)
(60.4, 0.507817)
(60.6, 0.508053)
(60.8, 0.509899)
(61, 0.529473)
(61.2, 0.516794)
(61.4, 0.47701)
(61.6, 0.501769)
(61.8, 0.522516)
(62, 0.518301)
(62.2, 0.505094)
(62.4, 0.498581)
(62.6, 0.497493)
(62.8, 0.503834)
(63, 0.496269)
(63.2, 0.500442)
(63.4, 0.541665)
(63.6, 0.55593)
(63.8, 0.546197)
(64, 0.533029)
(64.2, 0.537796)
(64.4, 0.532628)
(64.6, 0.5257)
(64.8, 0.50954)
(65, 0.508401)
(65.2, 0.497657)
(65.4, 0.494765)
(65.6, 0.506565)
(65.8, 0.518233)
(66, 0.52175)
(66.2, 0.538145)
(66.4, 0.53861)
(66.6, 0.525939)
(66.8, 0.463562)
(67, 0.393259)
(67.2, 0.379676)
(67.4, 0.391469)
(67.6, 0.392708)
(67.8, 0.381453)
(68, 0.361318)
(68.2, 0.358713)
(68.4, 0.344803)
(68.6, 0.321718)
(68.8, 0.303991)
(69, 0.307439)
(69.2, 0.336165)
(69.4, 0.309234)
(69.6, 0.287951)
(69.8, 0.27165)
(70, 0.263453)
(70.2, 0.256655)
(70.4, 0.244757)
(70.6, 0.23639)
(70.8, 0.21572)
(71, 0.200064)
(71.2, 0.202836)
(71.4, 0.200843)
(71.6, 0.17843)
(71.8, 0.156894)
(72, 0.143317)
(72.2, 0.135562)
(72.4, 0.117196)
(72.6, 0.118154)
(72.8, 0.109)
(73, 0.0992175)
(73.2, 0.0635816)
(73.4, 0.0401416)
(73.6, 0.0395072)
(73.8, 0.0550448)
(74, 0.0488963)
(74.2, 0.0333411)
(74.4, 0.0267655)
(74.6, 0.0253723)
(74.8, 0.0212078)
(75, 0.0223097)
(75.2, 0.0218822)
(75.4, 0.0207316)
(75.6, 0.021914)
(75.8, 0.0208469)
(76, 0.0180341)
(76.2, 0.0237558)
(76.4, 0.0235941)
(76.6, 0.0240489)
(76.8, 0.0210566)
(77, 0.0212984)
(77.2, 0.0206365)
(77.4, 0.0204335)
(77.6, 0.0187889)
(77.8, 0.0151071)
(78, 0.0146875)
(78.2, 0.0158539)
(78.4, 0.0182625)
(78.6, 0.0166398)
(78.8, 0.0175551)
(79, 0.017481)
(79.2, 0.0157965)
(79.4, 0.0165038)
(79.6, 0.0179126)
(79.8, 0.018317)
(80, 0.0174094)
(80.2, 0.0202402)
(80.4, 0.0178889)
(80.6, 0.010437)
(80.8, 0.0106821)
(81, 0.0150963)
(81.2, 0.0138096)
(81.4, 0.0170429)
(81.6, 0.0173526)
(81.8, 0.0182848)
(82, 0.0154669)
(82.2, 0.0135716)
(82.4, 0.0156203)
};

==> exp_plots/hover_dyanmic_payload/z_des.tex <==
\addplot[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates {
(0, 0)
(0.2, 0)
(0.4, 0)
(0.6, 0)
(0.8, 0)
(1, 0)
(1.2, 0)
(1.4, 0)
(1.6, 0)
(1.8, 0)
(2, 0)
(2.2, 0)
(2.4, 0)
(2.6, 0)
(2.8, 0)
(3, 0)
(3.2, 0)
(3.4, 0)
(3.6, 0)
(3.8, 0)
(4, 0)
(4.2, 0)
(4.4, 0)
(4.6, 0)
(4.8, 0)
(5, 0)
(5.2, 0)
(5.4, 0)
(5.6, 0)
(5.8, 0)
(6, 0)
(6.2, 0.5)
(6.4, 0.5)
(6.6, 0.5)
(6.8, 0.5)
(7, 0.5)
(7.2, 0.5)
(7.4, 0.5)
(7.6, 0.5)
(7.8, 0.5)
(8, 0.5)
(8.2, 0.5)
(8.4, 0.5)
(8.6, 0.5)
(8.8, 0.5)
(9, 0.5)
(9.2, 0.5)
(9.4, 0.5)
(9.6, 0.5)
(9.8, 0.5)
(10, 0.5)
(10.2, 0.5)
(10.4, 0.5)
(10.6, 0.5)
(10.8, 0.5)
(11, 0.5)
(11.2, 0.5)
(11.4, 0.5)
(11.6, 0.5)
(11.8, 0.5)
(12, 0.5)
(12.2, 0.5)
(12.4, 0.5)
(12.6, 0.5)
(12.8, 0.5)
(13, 0.5)
(13.2, 0.5)
(13.4, 0.5)
(13.6, 0.5)
(13.8, 0.5)
(14, 0.5)
(14.2, 0.5)
(14.4, 0.5)
(14.6, 0.5)
(14.8, 0.5)
(15, 0.5)
(15.2, 0.5)
(15.4, 0.5)
(15.6, 0.5)
(15.8, 0.5)
(16, 0.5)
(16.2, 0.5)
(16.4, 0.5)
(16.6, 0.5)
(16.8, 0.5)
(17, 0.5)
(17.2, 0.5)
(17.4, 0.5)
(17.6, 0.5)
(17.8, 0.5)
(18, 0.5)
(18.2, 0.5)
(18.4, 0.5)
(18.6, 0.5)
(18.8, 0.5)
(19, 0.5)
(19.2, 0.5)
(19.4, 0.5)
(19.6, 0.5)
(19.8, 0.5)
(20, 0.5)
(20.2, 0.5)
(20.4, 0.5)
(20.6, 0.5)
(20.8, 0.5)
(21, 0.5)
(21.2, 0.5)
(21.4, 0.5)
(21.6, 0.5)
(21.8, 0.5)
(22, 0.5)
(22.2, 0.5)
(22.4, 0.5)
(22.6, 0.5)
(22.8, 0.5)
(23, 0.5)
(23.2, 0.5)
(23.4, 0.5)
(23.6, 0.5)
(23.8, 0.5)
(24, 0.5)
(24.2, 0.5)
(24.4, 0.5)
(24.6, 0.5)
(24.8, 0.5)
(25, 0.5)
(25.2, 0.5)
(25.4, 0.5)
(25.6, 0.5)
(25.8, 0.5)
(26, 0.5)
(26.2, 0.5)
(26.4, 0.5)
(26.6, 0.5)
(26.8, 0.5)
(27, 0.5)
(27.2, 0.5)
(27.4, 0.5)
(27.6, 0.5)
(27.8, 0.5)
(28, 0.5)
(28.2, 0.5)
(28.4, 0.5)
(28.6, 0.5)
(28.8, 0.5)
(29, 0.5)
(29.2, 0.5)
(29.4, 0.5)
(29.6, 0.5)
(29.8, 0.5)
(30, 0.5)
(30.2, 0.5)
(30.4, 0.5)
(30.6, 0.5)
(30.8, 0.5)
(31, 0.5)
(31.2, 0.5)
(31.4, 0.5)
(31.6, 0.5)
(31.8, 0.5)
(32, 0.5)
(32.2, 0.5)
(32.4, 0.5)
(32.6, 0.5)
(32.8, 0.5)
(33, 0.5)
(33.2, 0.5)
(33.4, 0.5)
(33.6, 0.5)
(33.8, 0.5)
(34, 0.5)
(34.2, 0.5)
(34.4, 0.5)
(34.6, 0.5)
(34.8, 0.5)
(35, 0.5)
(35.2, 0.5)
(35.4, 0.5)
(35.6, 0.5)
(35.8, 0.5)
(36, 0.5)
(36.2, 0.5)
(36.4, 0.5)
(36.6, 0.5)
(36.8, 0.5)
(37, 0.5)
(37.2, 0.5)
(37.4, 0.5)
(37.6, 0.5)
(37.8, 0.5)
(38, 0.5)
(38.2, 0.5)
(38.4, 0.5)
(38.6, 0.5)
(38.8, 0.5)
(39, 0.5)
(39.2, 0.5)
(39.4, 0.5)
(39.6, 0.5)
(39.8, 0.5)
(40, 0.5)
(40.2, 0.5)
(40.4, 0.5)
(40.6, 0.5)
(40.8, 0.5)
(41, 0.5)
(41.2, 0.5)
(41.4, 0.5)
(41.6, 0.5)
(41.8, 0.5)
(42, 0.5)
(42.2, 0.5)
(42.4, 0.5)
(42.6, 0.5)
(42.8, 0.5)
(43, 0.5)
(43.2, 0.5)
(43.4, 0.5)
(43.6, 0.5)
(43.8, 0.5)
(44, 0.5)
(44.2, 0.5)
(44.4, 0.5)
(44.6, 0.5)
(44.8, 0.5)
(45, 0.5)
(45.2, 0.5)
(45.4, 0.5)
(45.6, 0.5)
(45.8, 0.5)
(46, 0.5)
(46.2, 0.5)
(46.4, 0.5)
(46.6, 0.5)
(46.8, 0.5)
(47, 0.5)
(47.2, 0.5)
(47.4, 0.5)
(47.6, 0.5)
(47.8, 0.5)
(48, 0.5)
(48.2, 0.5)
(48.4, 0.5)
(48.6, 0.5)
(48.8, 0.5)
(49, 0.5)
(49.2, 0.5)
(49.4, 0.5)
(49.6, 0.5)
(49.8, 0.5)
(50, 0.5)
(50.2, 0.5)
(50.4, 0.5)
(50.6, 0.5)
(50.8, 0.5)
(51, 0.5)
(51.2, 0.5)
(51.4, 0.5)
(51.6, 0.5)
(51.8, 0.5)
(52, 0.5)
(52.2, 0.5)
(52.4, 0.5)
(52.6, 0.5)
(52.8, 0.5)
(53, 0.5)
(53.2, 0.5)
(53.4, 0.5)
(53.6, 0.5)
(53.8, 0.5)
(54, 0.5)
(54.2, 0.5)
(54.4, 0.5)
(54.6, 0.5)
(54.8, 0.5)
(55, 0.5)
(55.2, 0.5)
(55.4, 0.5)
(55.6, 0.5)
(55.8, 0.5)
(56, 0.5)
(56.2, 0.5)
(56.4, 0.5)
(56.6, 0.5)
(56.8, 0.5)
(57, 0.5)
(57.2, 0.5)
(57.4, 0.5)
(57.6, 0.5)
(57.8, 0.5)
(58, 0.5)
(58.2, 0.5)
(58.4, 0.5)
(58.6, 0.5)
(58.8, 0.5)
(59, 0.5)
(59.2, 0.5)
(59.4, 0.5)
(59.6, 0.5)
(59.8, 0.5)
(60, 0.5)
(60.2, 0.5)
(60.4, 0.5)
(60.6, 0.5)
(60.8, 0.5)
(61, 0.5)
(61.2, 0.5)
(61.4, 0.5)
(61.6, 0.5)
(61.8, 0.5)
(62, 0.5)
(62.2, 0.5)
(62.4, 0.5)
(62.6, 0.5)
(62.8, 0.5)
(63, 0.5)
(63.2, 0.5)
(63.4, 0.5)
(63.6, 0.5)
(63.8, 0.5)
(64, 0.5)
(64.2, 0.5)
(64.4, 0.5)
(64.6, 0.5)
(64.8, 0.5)
(65, 0.5)
(65.2, 0.5)
(65.4, 0.5)
(65.6, 0)
(65.8, 0)
(66, 0)
(66.2, 0)
(66.4, 0)
(66.6, 0)
(66.8, 0)
(67, 0)
(67.2, 0)
(67.4, 0)
(67.6, 0)
(67.8, 0)
(68, 0)
(68.2, 0)
(68.4, 0)
(68.6, 0)
(68.8, 0)
(69, 0)
(69.2, 0)
(69.4, 0)
(69.6, 0)
(69.8, 0)
(70, 0)
(70.2, 0)
(70.4, 0)
(70.6, 0)
(70.8, 0)
(71, 0)
(71.2, 0)
(71.4, 0)
(71.6, 0)
(71.8, 0)
(72, 0)
(72.2, 0)
(72.4, 0)
(72.6, 0)
(72.8, 0)
(73, 0)
(73.2, 0)
(73.4, 0)
(73.6, 0)
(73.8, 0)
(74, 0)
(74.2, 0)
(74.4, 0)
(74.6, 0)
(74.8, 0)
(75, 0)
(75.2, 0)
(75.4, 0)
(75.6, 0)
(75.8, 0)
(76, 0)
(76.2, 0)
(76.4, 0)
(76.6, 0)
(76.8, 0)
(77, 0)
(77.2, 0)
(77.4, 0)
(77.6, 0)
(77.8, 0)
(78, 0)
(78.2, 0)
(78.4, 0)
(78.6, 0)
(78.8, 0)
(79, 0)
(79.2, 0)
(79.4, 0)
(79.6, 0)
(79.8, 0)
(80, 0)
(80.2, 0)
(80.4, 0)
(80.6, 0)
(80.8, 0)
(81, 0)
(81.2, 0)
(81.4, 0)
(81.6, 0)
(81.8, 0)
(82, 0)
(82.2, 0)
(82.4, 0)
};

==> exp_plots/open_ws/az.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0)
(0.075, -0.00686153)
(0.15, -0.00839824)
(0.225, -0.00901854)
(0.3, -0.000244247)
(0.375, -0.00955035)
(0.45, -0.0180641)
(0.525, -0.0267543)
(0.6, -0.0364856)
(0.675, -0.0333468)
(0.75, -0.0363413)
(0.825, -0.0517192)
(0.9, -0.0549254)
(0.975, -0.0373362)
(1.05, -0.00083217)
(1.125, 0.00539405)
(1.2, 0.0156349)
(1.275, 0.0101594)
(1.35, -0.0119724)
(1.425, -0.012951)
(1.5, -0.0110835)
(1.575, -0.0101042)
(1.65, -0.0102478)
(1.725, -0.0114761)
(1.8, -0.0285245)
(1.875, -0.0278118)
(1.95, -0.0239541)
(2.025, -0.0181531)
(2.1, -0.00145749)
(2.175, -0.0219044)
(2.25, -0.0496721)
(2.325, -0.0584789)
(2.4, -0.0375193)
(2.475, -0.0703836)
(2.55, -0.0390401)
(2.625, 0.0714803)
(2.7, 0.207413)
(2.775, 0.372108)
(2.85, 0.469267)
(2.925, 0.409938)
(3, 0.276439)
(3.075, 0.121685)
(3.15, 0.0817632)
(3.225, 0.143682)
(3.3, 0.291651)
(3.375, 0.344499)
(3.45, 0.262338)
(3.525, 0.00371698)
(3.6, -0.307354)
(3.675, -0.505893)
(3.75, -0.464308)
(3.825, -0.257446)
(3.9, 0.0643847)
(3.975, 0.259415)
(4.05, 0.197046)
(4.125, -0.05036)
(4.2, -0.298789)
(4.275, -0.368508)
(4.35, -0.23235)
(4.425, -0.040153)
(4.5, 0.102402)
(4.575, 0.15001)
(4.65, 0.136529)
(4.725, 0.0666467)
(4.8, 0.0163621)
(4.875, 0.0179657)
(4.95, 0.0673421)
(5.025, 0.0941721)
(5.1, 0.0715522)
(5.175, 0.00186608)
(5.25, -0.0365366)
(5.325, -0.0263013)
(5.4, -0.00666796)
(5.475, -0.0555342)
(5.55, -0.122488)
(5.625, -0.12163)
(5.7, -0.0454957)
(5.775, 0.104645)
(5.85, 0.236198)
(5.925, 0.263065)
(6, 0.182046)
(6.075, 0.0343119)
(6.15, -0.101645)
(6.225, -0.138131)
(6.3, -0.0900558)
(6.375, -0.00626066)
(6.45, 0.0163013)
(6.525, -0.0185265)
(6.6, -0.128862)
(6.675, -0.237495)
(6.75, -0.301686)
(6.825, -0.272903)
(6.9, -0.16007)
(6.975, -0.0174118)
(7.05, 0.0755098)
(7.125, 0.116561)
(7.2, 0.10467)
(7.275, 0.061032)
(7.35, -0.00288317)
(7.425, -0.0736163)
(7.5, -0.134853)
(7.575, -0.204533)
(7.65, -0.233428)
(7.725, -0.194862)
(7.8, -0.166494)
(7.875, -0.0933614)
(7.95, 0.0197499)
(8.025, 0.0739288)
(8.1, 0.070914)
(8.175, 0.0342924)
(8.25, -0.0552322)
(8.325, -0.0725537)
(8.4, 0.029957)
(8.475, 0.183002)
(8.55, 0.297006)
(8.625, 0.334469)
(8.7, 0.309773)
(8.775, 0.223212)
(8.85, 0.11897)
(8.925, 0.00445619)
(9, -0.150298)
(9.075, -0.235906)
(9.15, -0.211698)
(9.225, -0.0921956)
(9.3, 0.0424167)
(9.375, 0.067856)
(9.45, -0.00487543)
(9.525, -0.141124)
(9.6, -0.239008)
(9.675, -0.225565)
(9.75, -0.148479)
(9.825, -0.038617)
(9.9, 0.0111539)
(9.975, 0.00138357)
(10.05, -0.0284335)
(10.125, -0.00815476)
(10.2, 0.0406642)
(10.275, 0.102249)
(10.35, 0.123143)
(10.425, 0.128396)
(10.5, 0.128665)
(10.575, 0.0692928)
(10.65, -0.0190121)
(10.725, -0.0918859)
(10.8, -0.0886276)
(10.875, -0.0573497)
(10.95, 0.00288304)
(11.025, 0.0748072)
(11.1, 0.118818)
(11.175, 0.1061)
(11.25, -0.00219771)
(11.325, -0.087712)
(11.4, -0.103454)
(11.475, -0.095384)
(11.55, -0.0369892)
(11.625, 0.087703)
(11.7, 0.179609)
(11.775, 0.209003)
(11.85, 0.119249)
(11.925, -0.00418176)
(12, -0.142545)
(12.075, -0.197931)
(12.15, -0.139482)
(12.225, 0.036743)
(12.3, 0.214222)
(12.375, 0.251619)
(12.45, 0.102587)
(12.525, -0.1144)
(12.6, -0.274306)
(12.675, -0.263248)
(12.75, -0.143566)
(12.825, 0.0173809)
(12.9, 0.165328)
(12.975, 0.183852)
(13.05, 0.148163)
(13.125, 0.13815)
(13.2, 0.119783)
(13.275, 0.0881381)
(13.35, 0.0727729)
(13.425, 0.0293825)
(13.5, 0.0287883)
(13.575, 0.0651766)
(13.65, 0.0677125)
(13.725, 0.0155172)
(13.8, -0.0918213)
(13.875, -0.170839)
(13.95, -0.211432)
(14.025, -0.17907)
(14.1, -0.152259)
(14.175, -0.138584)
(14.25, -0.121531)
(14.325, -0.0995028)
(14.4, -0.0440208)
(14.475, 0.0261982)
(14.55, 0.0821542)
(14.625, 0.114892)
(14.7, 0.0693567)
(14.775, -0.0439203)
(14.85, -0.16707)
(14.925, -0.216001)
(15, -0.146277)
(15.075, -0.0219229)
(15.15, 0.09444)
(15.225, 0.144243)
(15.3, 0.109118)
(15.375, 0.0225447)
(15.45, -0.0192407)
(15.525, 0.0217638)
(15.6, 0.111387)
(15.675, 0.148827)
(15.75, 0.117045)
(15.825, 0.0767642)
(15.9, 0.0332181)
(15.975, -0.00064667)
(16.05, -0.0159398)
(16.125, -0.0960162)
(16.2, -0.173648)
(16.275, -0.214938)
(16.35, -0.131677)
(16.425, -0.0114964)
(16.5, 0.0614173)
(16.575, 0.0248847)
(16.65, -0.0974539)
(16.725, -0.18938)
(16.8, -0.153179)
(16.875, -0.046715)
(16.95, 0.0065468)
(17.025, 0.00234059)
(17.1, -0.030599)
(17.175, -0.0590237)
(17.25, -0.0315265)
(17.325, 0.013835)
(17.4, 0.0731004)
(17.475, 0.128511)
(17.55, 0.109451)
(17.625, 0.054339)
(17.7, 0.0117455)
(17.775, -0.0241236)
(17.85, -0.0405688)
(17.925, -0.0500547)
(18, -0.0709676)
(18.075, -0.0828561)
(18.15, -0.0676104)
(18.225, -0.0196713)
(18.3, 0.00671214)
(18.375, 0.0407856)
(18.45, 0.0879075)
(18.525, 0.111786)
(18.6, 0.0960264)
(18.675, 0.0614149)
(18.75, 0.0058543)
(18.825, -0.0454361)
(18.9, -0.148933)
(18.975, -0.224761)
(19.05, -0.230269)
(19.125, -0.164154)
(19.2, 0.00877232)
(19.275, 0.145339)
(19.35, 0.168663)
(19.425, 0.132795)
(19.5, 0.058618)
(19.575, 0.00562783)
(19.65, 0.0146417)
(19.725, 0.0360932)
(19.8, 0.0634599)
(19.875, 0.0542972)
(19.95, -0.0381166)
(20.025, -0.155095)
(20.1, -0.224882)
(20.175, -0.140905)
(20.25, 0.0938095)
(20.325, 0.332461)
(20.4, 0.47195)
(20.475, 0.433483)
(20.55, 0.19881)
(20.625, -0.120668)
(20.7, -0.346632)
(20.775, -0.349415)
(20.85, -0.2043)
(20.925, -0.00290368)
(21, 0.167296)
(21.075, 0.210518)
(21.15, 0.104691)
(21.225, -0.0547888)
(21.3, -0.146743)
(21.375, -0.185324)
(21.45, -0.166394)
(21.525, -0.0555089)
(21.6, 0.0534941)
(21.675, 0.112808)
(21.75, 0.101644)
(21.825, 0.0457477)
(21.9, -0.00971133)
(21.975, -0.0138411)
(22.05, 0.032663)
(22.125, 0.0574059)
(22.2, 0.0464536)
(22.275, 0.0253597)
(22.35, -0.00663271)
(22.425, -0.0395725)
(22.5, -0.060049)
(22.575, -0.0781038)
(22.65, -0.0724756)
(22.725, -0.0552675)
(22.8, -0.027345)
(22.875, 0.0412091)
(22.95, 0.0687357)
(23.025, 0.0358923)
(23.1, -0.0255603)
(23.175, -0.0839971)
(23.25, -0.0765663)
(23.325, 0.103173)
(23.4, 0.253911)
(23.475, 0.240025)
(23.55, 0.122225)
(23.625, -0.0157594)
(23.7, -0.0960007)
(23.775, -0.134706)
(23.85, -0.14336)
(23.925, -0.0574899)
(24, 0.0643185)
(24.075, 0.146307)
(24.15, 0.0921561)
(24.225, -0.0227453)
(24.3, -0.0684366)
(24.375, -0.0165581)
(24.45, 0.0429232)
(24.525, 0.0151323)
(24.6, 0.000213269)
(24.675, -0.00200153)
(24.75, -0.016445)
(24.825, -0.0184826)
(24.9, -3.47202e-05)
(24.975, 0.0167021)
(25.05, 0.0174255)
(25.125, 0.0114954)
(25.2, -0.0209439)
(25.275, -0.0100104)
(25.35, -0.0002883)
(25.425, -0.00705691)
(25.5, -0.0146868)
(25.575, -0.037724)
(25.65, -0.0279944)
(25.725, -0.00221441)
(25.8, 0.0184188)
(25.875, 0.000313643)
(25.95, -0.00357404)
(26.025, -0.0147849)
(26.1, -0.0109746)
(26.175, -0.00161955)
(26.25, 0.0173966)
(26.325, 0.0177488)
(26.4, 0.0131816)
(26.475, -0.00592135)
(26.55, -0.00251732)
(26.625, 0.00792841)
(26.7, 0.0223298)
(26.775, 0.0229017)
(26.85, 0.00336781)
(26.925, 0.0107468)
(27, 0.0218352)
(27.075, 0.0161473)
(27.15, 0.0302778)
(27.225, 0.035161)
(27.3, 0.0321354)
(27.375, 0.0357094)
(27.45, 0.0411918)
(27.525, 0.035545)
(27.6, 0.0450848)
(27.675, 0.0279532)
(27.75, -0.00329385)
(27.825, -0.0192341)
(27.9, -0.0117366)
(27.975, -0.00886163)
(28.05, 0.0106799)
(28.125, 0.0261627)
(28.2, 0.0167464)
(28.275, -0.000180827)
(28.35, -0.0121143)
(28.425, -0.0198783)
(28.5, -0.00303746)
(28.575, -0.000171996)
(28.65, 0.0152673)
(28.725, 0.0151742)
(28.8, 0.0184166)
(28.875, 0.00561607)
(28.95, 0.0153629)
(29.025, 0.025194)
(29.1, 0.0337905)
(29.175, 0.0270366)
(29.25, 0.00862205)
(29.325, 0.0119188)
(29.4, 0.0272011)
(29.475, 0.0398933)
(29.55, 0.0349306)
(29.625, 0.0246715)
(29.7, 0.0162152)
(29.775, 0.0031902)
(29.85, 0.00412193)
(29.925, 0.00585473)
(30, 0.0145957)
(30.075, 0.0148355)
(30.15, 0.0176432)
(30.225, 0.024417)
(30.3, 0.0250077)
(30.375, 0.0297917)
(30.45, 0.0152826)
(30.525, 0.0206477)
(30.6, 0.0148121)
(30.675, 0.00676032)
(30.75, 0.00699255)
(30.825, -0.00319955)
(30.9, -0.00477298)
(30.975, 0.00414291)
(31.05, 5.57029e-05)
(31.125, 0.00508524)
(31.2, 0.0047915)
(31.275, 0.00399155)
(31.35, 0.00203286)
(31.425, -0.00585957)
(31.5, -0.00540637)
(31.575, 0.00665774)
(31.65, 0.0182786)
(31.725, 0.0291752)
(31.8, 0.0493156)
(31.875, 0.0580385)
(31.95, 0.0556723)
(32.025, 0.0351852)
(32.1, 0.014436)
(32.175, 0.00543189)
(32.25, -2.05098e-05)
};

==> exp_plots/open_ws/az_des.tex <==
\addplot[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates {
(0, 0)
(0.075, 0.00402167)
(0.15, 0.00650516)
(0.225, 0.00797283)
(0.3, 0.00632454)
(0.375, 0.00484)
(0.45, 0.00688737)
(0.525, 0.00667093)
(0.6, 0.00585235)
(0.675, 0.00646181)
(0.75, 0.00636577)
(0.825, 0.00826256)
(0.9, 0.0129057)
(0.975, 0.0140273)
(1.05, 0.258118)
(1.125, 0.429472)
(1.2, 0.493487)
(1.275, 0.506537)
(1.35, 0.480642)
(1.425, 0.444447)
(1.5, 0.430805)
(1.575, 0.431857)
(1.65, 0.433021)
(1.725, 0.432803)
(1.8, 0.434686)
(1.875, 0.434666)
(1.95, 0.43976)
(2.025, 0.440984)
(2.1, 0.445485)
(2.175, 0.447052)
(2.25, 0.451673)
(2.325, 0.462597)
(2.4, 0.462804)
(2.475, 0.434956)
(2.55, 0.430881)
(2.625, 0.435361)
(2.7, 0.431862)
(2.775, 0.415173)
(2.85, 0.358795)
(2.925, 0.291156)
(3, 0.27244)
(3.075, 0.260185)
(3.15, 0.299772)
(3.225, 0.286073)
(3.3, 0.189477)
(3.375, 0.00655064)
(3.45, -0.129679)
(3.525, -0.163272)
(3.6, -0.115717)
(3.675, 0.0821454)
(3.75, 0.0721308)
(3.825, -0.0168115)
(3.9, -0.094254)
(3.975, -0.148512)
(4.05, -0.162944)
(4.125, -0.122563)
(4.2, -0.0879838)
(4.275, -0.0458226)
(4.35, -0.0089663)
(4.425, 0.0104323)
(4.5, 0.0711955)
(4.575, 0.120921)
(4.65, 0.127293)
(4.725, 0.12392)
(4.8, 0.114255)
(4.875, 0.116362)
(4.95, 0.0450262)
(5.025, -0.0111707)
(5.1, -0.0314357)
(5.175, -0.0542208)
(5.25, -0.0552628)
(5.325, -0.0396529)
(5.4, -0.00356274)
(5.475, 0.0230185)
(5.55, 0.0364326)
(5.625, 0.0715453)
(5.7, 0.0907269)
(5.775, 0.101982)
(5.85, 0.0959109)
(5.925, 0.0589564)
(6, 0.0317933)
(6.075, 0.0317602)
(6.15, -0.0624535)
(6.225, -0.142181)
(6.3, -0.158541)
(6.375, -0.14607)
(6.45, -0.164014)
(6.525, -0.173769)
(6.6, -0.147779)
(6.675, -0.106498)
(6.75, -0.054857)
(6.825, -0.0115087)
(6.9, 0.0120754)
(6.975, 0.0438937)
(7.05, 0.0518734)
(7.125, 0.0288604)
(7.2, -0.0165425)
(7.275, -0.0764391)
(7.35, -0.146112)
(7.425, -0.173366)
(7.5, -0.161186)
(7.575, -0.113725)
(7.65, -0.0540203)
(7.725, -0.0196584)
(7.8, -0.00757709)
(7.875, -0.0147872)
(7.95, -0.0351114)
(8.025, -0.0380634)
(8.1, -0.0361774)
(8.175, 0.107122)
(8.25, 0.218495)
(8.325, 0.233074)
(8.4, 0.229562)
(8.475, 0.238247)
(8.55, 0.172237)
(8.625, 0.0763268)
(8.7, 0.00821595)
(8.775, -0.0299293)
(8.85, -0.0353289)
(8.925, -0.0379763)
(9, -0.0440093)
(9.075, -0.0463452)
(9.15, -0.0407427)
(9.225, -0.094528)
(9.3, -0.115285)
(9.375, -0.11478)
(9.45, -0.106646)
(9.525, -0.0945871)
(9.6, -0.0753821)
(9.675, -0.0707211)
(9.75, -0.0455179)
(9.825, -0.0208072)
(9.9, 0.0046466)
(9.975, 0.0129784)
(10.05, 0.024314)
(10.125, 0.0245908)
(10.2, 0.0135508)
(10.275, 0.0815047)
(10.35, 0.100686)
(10.425, 0.10338)
(10.5, 0.0751379)
(10.575, 0.00326049)
(10.65, -0.0460207)
(10.725, -0.0225987)
(10.8, 0.010362)
(10.875, 0.00199519)
(10.95, 0.0163389)
(11.025, 0.00549561)
(11.1, -0.0824929)
(11.175, -0.100537)
(11.25, -0.0690107)
(11.325, -0.0369329)
(11.4, 0.0613604)
(11.475, 0.121093)
(11.55, 0.125995)
(11.625, 0.0886615)
(11.7, 0.0326971)
(11.775, -0.0133344)
(11.85, -0.0340345)
(11.925, -0.0228809)
(12, 0.0398791)
(12.075, 0.107572)
(12.15, 0.125919)
(12.225, 0.0692012)
(12.3, -0.00962869)
(12.375, -0.0511596)
(12.45, -0.0594628)
(12.525, -0.0367898)
(12.6, 0.0182274)
(12.675, 0.0584686)
(12.75, 0.0359334)
(12.825, -0.00152057)
(12.9, 0.0447479)
(12.975, 0.0367429)
(13.05, 0.053537)
(13.125, 0.0524722)
(13.2, 0.0857138)
(13.275, 0.102318)
(13.35, 0.0807987)
(13.425, 0.0486061)
(13.5, -0.0327591)
(13.575, -0.0917441)
(13.65, -0.125927)
(13.725, -0.158222)
(13.8, -0.163528)
(13.875, -0.160027)
(13.95, -0.146511)
(14.025, -0.128334)
(14.1, -0.0888109)
(14.175, -0.0594173)
(14.25, -0.0126966)
(14.325, 0.0228477)
(14.4, 0.0417979)
(14.475, 0.0153548)
(14.55, -0.0186017)
(14.625, -0.0607371)
(14.7, -0.0876468)
(14.775, -0.0795005)
(14.85, -0.0325195)
(14.925, 0.0148199)
(15, 0.0604188)
(15.075, 0.0726981)
(15.15, 0.0268602)
(15.225, -0.021115)
(15.3, -0.0455416)
(15.375, 0.0438805)
(15.45, 0.109928)
(15.525, 0.132067)
(15.6, 0.103872)
(15.675, 0.0464664)
(15.75, -0.0125571)
(15.825, -0.0296911)
(15.9, -0.0346286)
(15.975, -0.121555)
(16.05, -0.147249)
(16.125, -0.106429)
(16.2, -0.0552403)
(16.275, -0.0220777)
(16.35, -0.01724)
(16.425, -0.0425031)
(16.5, -0.120881)
(16.575, -0.143323)
(16.65, -0.0878678)
(16.725, -0.0495194)
(16.8, -0.0320929)
(16.875, -0.0383117)
(16.95, -0.0603119)
(17.025, -0.0604939)
(17.1, -0.0395343)
(17.175, -0.0310995)
(17.25, 0.0454632)
(17.325, 0.0959683)
(17.4, 0.0690455)
(17.475, 0.0926994)
(17.55, 0.020827)
(17.625, -0.0320929)
(17.7, -0.0233735)
(17.775, -0.00899344)
(17.85, -0.00956566)
(17.925, -0.00225126)
(18, -0.00533614)
(18.075, -0.0215679)
(18.15, -0.01055)
(18.225, 0.0237054)
(18.3, 0.0412084)
(18.375, 0.0374568)
(18.45, 0.00804108)
(18.525, -0.01398)
(18.6, -0.0342507)
(18.675, -0.126875)
(18.75, -0.187007)
(18.825, -0.156199)
(18.9, -0.113551)
(18.975, -0.035664)
(19.05, 0.0275286)
(19.125, 0.0468222)
(19.2, 0.0700558)
(19.275, 0.0847898)
(19.35, 0.0771401)
(19.425, 0.0551523)
(19.5, 0.0403147)
(19.575, 0.0240567)
(19.65, 0.0295742)
(19.725, -0.0573961)
(19.8, -0.133785)
(19.875, -0.148671)
(19.95, -0.0972597)
(20.025, 0.102944)
(20.1, 0.209136)
(20.175, 0.252996)
(20.25, 0.243575)
(20.325, 0.138857)
(20.4, 0.026472)
(20.475, -0.0502687)
(20.55, -0.1211)
(20.625, -0.131102)
(20.7, -0.0985901)
(20.775, -0.0424626)
(20.85, -0.0207357)
(20.925, -0.0291635)
(21, -0.0734579)
(21.075, -0.102021)
(21.15, -0.105724)
(21.225, -0.083029)
(21.3, -0.0512898)
(21.375, -0.0215412)
(21.45, -0.0117105)
(21.525, -0.0215644)
(21.6, -0.0427447)
(21.675, -0.0466182)
(21.75, -0.0306115)
(21.825, 0.0151061)
(21.9, 0.0394218)
(21.975, 0.0292674)
(22.05, -0.00840979)
(22.125, -0.0476927)
(22.2, -0.0743088)
(22.275, -0.0810256)
(22.35, -0.0786243)
(22.425, -0.0730393)
(22.5, -0.056721)
(22.575, -0.0450864)
(22.65, -0.0315701)
(22.725, -0.020341)
(22.8, -0.024513)
(22.875, -0.0456297)
(22.95, -0.0431151)
(23.025, -0.0337164)
(23.1, 0.00177775)
(23.175, 0.136802)
(23.25, 0.172251)
(23.325, 0.120075)
(23.4, 0.102966)
(23.475, 0.0333353)
(23.55, -0.0211961)
(23.625, -0.0358693)
(23.7, -0.0307371)
(23.775, -0.0322501)
(23.85, -0.02919)
(23.925, -0.0318989)
(24, -0.0481584)
(24.075, -0.136397)
(24.15, -0.172983)
(24.225, -0.206672)
(24.3, -0.203477)
(24.375, -0.180888)
(24.45, -0.174289)
(24.525, -0.184272)
(24.6, -0.183323)
(24.675, -0.185959)
(24.75, -0.19396)
(24.825, -0.195056)
(24.9, -0.190496)
(24.975, -0.191325)
(25.05, -0.197935)
(25.125, -0.191001)
(25.2, -0.180581)
(25.275, -0.173051)
(25.35, -0.169877)
(25.425, -0.176156)
(25.5, -0.197685)
(25.575, -0.212252)
(25.65, -0.223465)
(25.725, -0.232278)
(25.8, -0.238373)
(25.875, -0.2425)
(25.95, -0.241653)
(26.025, -0.244739)
(26.1, -0.247196)
(26.175, -0.24416)
(26.25, -0.244864)
(26.325, -0.249916)
(26.4, -0.256125)
(26.475, -0.262389)
(26.55, -0.264726)
(26.625, -0.264448)
(26.7, -0.267419)
(26.775, -0.269176)
(26.85, -0.267457)
(26.925, -0.265219)
(27, -0.267027)
(27.075, -0.271347)
(27.15, -0.275934)
(27.225, -0.281506)
(27.3, -0.285602)
(27.375, -0.28701)
(27.45, -0.28966)
(27.525, -0.292115)
(27.6, -0.291586)
(27.675, -0.29517)
(27.75, -0.296154)
(27.825, -0.293173)
(27.9, -0.291188)
(27.975, -0.292157)
(28.05, -0.294093)
(28.125, -0.297575)
(28.2, -0.301377)
(28.275, -0.299816)
(28.35, -0.298139)
(28.425, -0.298161)
(28.5, -0.298488)
(28.575, -0.303201)
(28.65, -0.306816)
(28.725, -0.310928)
(28.8, -0.315678)
(28.875, -0.321099)
(28.95, -0.322545)
(29.025, -0.325657)
(29.1, -0.329212)
(29.175, -0.331396)
(29.25, -0.331408)
(29.325, -0.325971)
(29.4, -0.321851)
(29.475, -0.3215)
(29.55, -0.325206)
(29.625, -0.32715)
(29.7, -0.323923)
(29.775, -0.326769)
(29.85, -0.328375)
(29.925, -0.331763)
(30, -0.337788)
(30.075, -0.341972)
(30.15, -0.343041)
(30.225, -0.348576)
(30.3, -0.359937)
(30.375, -0.365527)
(30.45, -0.369314)
(30.525, -0.370903)
(30.6, -0.363569)
(30.675, -0.357734)
(30.75, -0.353747)
(30.825, -0.355263)
(30.9, -0.353563)
(30.975, -0.354977)
(31.05, -0.360214)
(31.125, -0.362642)
(31.2, -0.369515)
(31.275, -0.372312)
(31.35, -0.371371)
(31.425, -0.362187)
(31.5, -0.35833)
(31.575, -0.367014)
(31.65, -0.385745)
(31.725, -0.375107)
(31.8, -0.388086)
(31.875, -0.408478)
(31.95, -0.42284)
(32.025, -0.438443)
(32.1, -0.449838)
(32.175, -0.449404)
(32.25, -0.44033)
};

==> exp_plots/open_ws/plot.tex <==
%%    
\begin{figure}[t]
\centering

\begin{tikzpicture}


\FPeval{\xshfta}{0}
\FPeval{\xshftb}{0}
\FPeval{\xshftc}{0}
\FPeval{\xshftd}{0}



\FPeval{\yshfta}{0-0}
\FPeval{\yshftb}{0-9}
\FPeval{\yshftc}{0-18}
\FPeval{\yshftd}{0-27.9}


\FPeval{\pltw}{110}
\FPeval{\plth}{24}

\FPeval{\scal}{0.5}


\FPeval{\mrksize}{0.3}

%
\colorlet{desclr}{white!0!magenta}
\colorlet{currclr}{blue!60!green}

\colorlet{gridclr}{white!85!black}
\colorlet{dlegendclr}{white!80!black}
\colorlet{axisclr}{white!75!black}
\colorlet{axisbgclr}{white!99!black}

\colorlet{dlegendclr}{white!80!black}
\colorlet{legendclr}{white!100!black}






\FPeval{\lscale}{0.6}
\FPeval{\limscale}{0.5}
\FPeval{\lxshft}{95.5}
\FPeval{\lyshft}{9.0}

  
\FPeval{\titlescale}{0.7}
\FPeval{\titlexshift}{21.0}
\FPeval{\titleyshift}{13.7}

\colorlet{gpudclr}{white!80!black}
\colorlet{gpuclr}{white!90!black}
\colorlet{gputxtclr}{white!0!black}

\FPeval{\labelscale}{1.0}
\FPeval{\ticklabelscale}{0.9}

\FPeval{\xlabelxshift}{0+15}
\FPeval{\xlabelyshift}{0+0.5}
\FPeval{\ylabelxshift}{0+4.0}
\FPeval{\ylabelyshift}{0+6.2}


\FPeval{\linew}{1.5}
\FPeval{\dashon}{5.0}
\FPeval{\dashoff}{3.0}

\FPeval{\xshfttakeoff}{0-16}
\FPeval{\xshfthover}{0}
\FPeval{\xshftland}{16}
%
%
\node (a) [xshift = \xshfta ex, yshift=\yshfta ex, scale=\scal]{
\tikz{
%
\pgfplotsset{width=\pltw ex, height=\plth ex}
\begin{axis}[
   axis background style={fill=axisbgclr},
    title={},
    xlabel={},
    ylabel={ X (m)},
    xmin=0, xmax=28,
    ymin=-1, ymax=1,
    xtick={0, 15, 30, 45, 60},
    ytick={-1, 0, 1},
    xticklabels={$0$, $15$, $30$, $45$, $60$},
    yticklabels={$-1$, $0$, $0$},
     axis line style={axisclr},
    legend image post style={scale =\limscale},
    legend style={at={(\lxshft ex,\lyshft ex)},anchor=south, legend columns = 1, draw = {dlegendclr}, fill={legendclr}, nodes={scale=\lscale}},
    ymajorgrids=true, 
    xmajorgrids=true,
    grid style={dashed, gridclr},
    major tick length=1ex,
    x label style={at={(\xlabelxshift ex, \xlabelyshift ex)},scale=\labelscale},
    y label style={at={(\ylabelxshift ex, \ylabelyshift ex)},scale=\labelscale},
    xticklabel style={scale=\ticklabelscale},
    yticklabel style={scale=\ticklabelscale},
%    ybar,
%    bar width = 4pt,
]
%
%
\input{exp_plots/open_ws/x_des}
%
\input{exp_plots/open_ws/x}
%
%
%%   
  \legend{Ref, SLAM}
  %
\end{axis}
%
% \node [draw=gpudclr,fill=gpuclr,rounded corners=0.2ex, minimum width=10.0ex, xshift=\titlexshift ex, yshift=\titleyshift ex, scale=\titlescale]{\textcolor{gputxtclr}{\textbf{Step-X}}};
}};
%
%    
%
%
\node (b) [xshift = \xshftb ex, yshift=\yshftb ex, scale=\scal]{
\tikz{
%
\pgfplotsset{width=\pltw ex, height=\plth ex}
\begin{axis}[
   axis background style={fill=axisbgclr},
    title={},
    xlabel={},
    ylabel={ Y (m)},
    xmin=0, xmax=28,
    ymin=-1, ymax=1,
    xtick={0, 15, 30, 45, 60},
    ytick={-1, 0, 1},
    xticklabels={$0$, $15$, $30$, $45$, $60$},
    yticklabels={$-1$, $0$, $0$},
     axis line style={axisclr},
    legend image post style={scale =\limscale},
    legend style={at={(\lxshft ex,\lyshft ex)},anchor=south, legend columns = 1, draw = {dlegendclr}, fill={legendclr}, nodes={scale=\lscale}},
    ymajorgrids=true, 
    xmajorgrids=true,
    grid style={dashed, gridclr},
    major tick length=1ex,
    x label style={at={(\xlabelxshift ex, \xlabelyshift ex)},scale=\labelscale},
    y label style={at={(\ylabelxshift ex, \ylabelyshift ex)},scale=\labelscale},
    xticklabel style={scale=\ticklabelscale},
    yticklabel style={scale=\ticklabelscale},
%    ybar,
%    bar width = 4pt,
]
%
\input{exp_plots/open_ws/y}
%
%
\input{exp_plots/open_ws/y_des}
%
%% 
  \legend{Ref, SLAM}
  %
\end{axis}
%
% \node [draw=gpudclr,fill=gpuclr,rounded corners=0.2ex, minimum width=10.0ex, xshift=\titlexshift ex, yshift=\titleyshift ex, scale=\titlescale]{\textcolor{gputxtclr}{\textbf{Step-X}}};
}};
%
% 
%
\node (c) [xshift = \xshftc ex, yshift=\yshftc ex, scale=\scal]{
\tikz{
%
\pgfplotsset{width=\pltw ex, height=\plth ex}
\begin{axis}[
   axis background style={fill=axisbgclr},
    title={},
    xlabel={},
    ylabel={ Z (m)},
    xmin=0, xmax=28,
    ymin=-1, ymax=1,
    xtick={0, 15, 30, 45, 60},
    ytick={-1, 0, 1},
    xticklabels={$0$, $15$, $30$, $45$, $60$},
    yticklabels={$-1$, $0$, $0$},
     axis line style={axisclr},
    legend image post style={scale =\limscale},
    legend style={at={(\lxshft ex,\lyshft ex)},anchor=south, legend columns = 1, draw = {dlegendclr}, fill={legendclr}, nodes={scale=\lscale}},
    ymajorgrids=true, 
    xmajorgrids=true,
    grid style={dashed, gridclr},
    major tick length=1ex,
    x label style={at={(\xlabelxshift ex, \xlabelyshift ex)},scale=\labelscale},
    y label style={at={(\ylabelxshift ex, \ylabelyshift ex)},scale=\labelscale},
    xticklabel style={scale=\ticklabelscale},
    yticklabel style={scale=\ticklabelscale},
%    ybar,
%    bar width = 4pt,
]
%
\input{exp_plots/open_ws/z}
%
%
\input{exp_plots/open_ws/z_des}
%
%% 
  \legend{Ref, SLAM}
  %
\end{axis}
%
% \node [draw=gpudclr,fill=gpuclr,rounded corners=0.2ex, minimum width=10.0ex, xshift=\titlexshift ex, yshift=\titleyshift ex, scale=\titlescale]{\textcolor{gputxtclr}{\textbf{Step-X}}};
}};
%
% 
%
\node (d) [xshift = \xshftd ex, yshift=\yshftd ex, scale=\scal]{
\tikz{
%
\pgfplotsset{width=\pltw ex, height=\plth ex}
\begin{axis}[
   axis background style={fill=axisbgclr},
    title={},
    xlabel={Time (s)},
    ylabel={ Yaw ($^\text{o}$)},
    xmin=0, xmax=28,
    ymin=-40, ymax=40,
    xtick={0, 7, 14, 21, 28},
    ytick={-40, -20, 0, 20, 40},
    xticklabels={$0$, $7$, $14$, $28$, $28$},
    yticklabels={$-40$, $-20$, $0$, $20$, $40$},
     axis line style={axisclr},
    legend image post style={scale =\limscale},
    legend style={at={(\lxshft ex,\lyshft ex)},anchor=south, legend columns = 1, draw = {dlegendclr}, fill={legendclr}, nodes={scale=\lscale}},
    ymajorgrids=true, 
    xmajorgrids=true,
    grid style={dashed, gridclr},
    major tick length=1ex,
    x label style={at={(\xlabelxshift ex, \xlabelyshift ex)},scale=\labelscale},
    y label style={at={(\ylabelxshift ex, \ylabelyshift ex)},scale=\labelscale},
    xticklabel style={scale=\ticklabelscale},
    yticklabel style={scale=\ticklabelscale},
%    ybar,
%    bar width = 4pt,
]
%
\input{exp_plots/open_ws/yaw}
%
%
%
\input{exp_plots/open_ws/yaw_des}
%
%% 
  \legend{Ref, SLAM}
  %
\end{axis}
%
% \node [draw=gpudclr,fill=gpuclr,rounded corners=0.2ex, minimum width=10.0ex, xshift=\titlexshift ex, yshift=\titleyshift ex, scale=\titlescale]{\textcolor{gputxtclr}{\textbf{Step-X}}};
}};
%
% 
%
%
\node (t) [xshift=\xshfttakeoff ex, yshift=5 ex]{\scriptsize Takeoff};
\node (h) [xshift=\xshfthover ex, yshift=5 ex]{\scriptsize Hover};
\node (l) [xshift=\xshftland ex, yshift=5 ex]{\scriptsize Land};
%%
%
 
\end{tikzpicture}
%
%
\caption{Takeoff-Hover-Land performance in open workspace.}
%
\label{fig:openwsTHL}
%
%\vspace{-3ex}
\end{figure}
%
%
%
%%


==> exp_plots/open_ws/thrust.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0)
(0.075, 10.1017)
(0.15, 10.1714)
(0.225, 10.2688)
(0.3, 10.1457)
(0.375, 10.3145)
(0.45, 10.4469)
(0.525, 10.633)
(0.6, 10.7706)
(0.675, 10.8494)
(0.75, 10.937)
(0.825, 11.3323)
(0.9, 11.6793)
(0.975, 11.7099)
(1.05, 12.2938)
(1.125, 15.6016)
(1.2, 17.1169)
(1.275, 18.5373)
(1.35, 20.3268)
(1.425, 21.4869)
(1.5, 23.2633)
(1.575, 24.8204)
(1.65, 26.4653)
(1.725, 27.8284)
(1.8, 29.5934)
(1.875, 31.2649)
(1.95, 32.8615)
(2.025, 34.2309)
(2.1, 35.9996)
(2.175, 37.8221)
(2.25, 39.809)
(2.325, 41.6861)
(2.4, 43.4356)
(2.475, 45.1285)
(2.55, 46.4438)
(2.625, 47.045)
(2.7, 46.9551)
(2.775, 45.9396)
(2.85, 44.9895)
(2.925, 45.0701)
(3, 46.0487)
(3.075, 47.6734)
(3.15, 48.7622)
(3.225, 48.0364)
(3.3, 45.6021)
(3.375, 43.0897)
(3.45, 42.0659)
(3.525, 43.6201)
(3.6, 46.825)
(3.675, 50.1226)
(3.75, 51.8003)
(3.825, 49.5788)
(3.9, 46.3617)
(3.975, 44.0641)
(4.05, 44.2549)
(4.125, 46.3543)
(4.2, 48.4198)
(4.275, 49.7046)
(4.35, 49.131)
(4.425, 48.2806)
(4.5, 47.9353)
(4.575, 48.405)
(4.65, 48.6227)
(4.725, 49.0746)
(4.8, 49.5387)
(4.875, 49.8487)
(4.95, 49.0365)
(5.025, 47.8258)
(5.1, 47.8783)
(5.175, 48.4583)
(5.25, 48.5261)
(5.325, 48.1513)
(5.4, 47.9162)
(5.475, 48.8876)
(5.55, 50.1161)
(5.625, 50.8841)
(5.7, 50.7289)
(5.775, 49.4946)
(5.85, 48.1027)
(5.925, 47.4685)
(6, 47.735)
(6.075, 48.8041)
(6.15, 49.8465)
(6.225, 49.224)
(6.3, 48.4751)
(6.375, 47.5006)
(6.45, 47.0615)
(6.525, 46.8108)
(6.6, 47.5829)
(6.675, 48.8092)
(6.75, 50.1662)
(6.825, 50.8717)
(6.9, 50.5087)
(6.975, 50.1414)
(7.05, 49.8414)
(7.125, 49.2971)
(7.2, 48.6557)
(7.275, 48.1839)
(7.35, 47.6325)
(7.425, 47.6669)
(7.5, 48.0995)
(7.575, 49.066)
(7.65, 50.174)
(7.725, 50.4222)
(7.8, 50.6821)
(7.875, 50.5363)
(7.95, 49.3724)
(8.025, 48.7598)
(8.1, 48.8212)
(8.175, 50.2934)
(8.25, 52.6107)
(8.325, 53.214)
(8.4, 52.6546)
(8.475, 52.1217)
(8.55, 50.6144)
(8.625, 49.5028)
(8.7, 48.3104)
(8.775, 48.0123)
(8.85, 48.2438)
(8.925, 48.5711)
(9, 49.6146)
(9.075, 50.5438)
(9.15, 50.6839)
(9.225, 49.3173)
(9.3, 47.6852)
(9.375, 47.3277)
(9.45, 48.0128)
(9.525, 49.1886)
(9.6, 50.2952)
(9.675, 50.2243)
(9.75, 50.0483)
(9.825, 49.7149)
(9.9, 49.4895)
(9.975, 49.9984)
(10.05, 50.5038)
(10.125, 50.3422)
(10.2, 49.5796)
(10.275, 50.0637)
(10.35, 50.2051)
(10.425, 49.941)
(10.5, 49.4477)
(10.575, 48.8292)
(10.65, 49.3185)
(10.725, 50.5444)
(10.8, 50.8938)
(10.875, 50.545)
(10.95, 50.3645)
(11.025, 49.8913)
(11.1, 48.347)
(11.175, 47.4168)
(11.25, 48.6132)
(11.325, 49.9749)
(11.4, 50.7791)
(11.475, 51.5212)
(11.55, 51.495)
(11.625, 50.4548)
(11.7, 49.0564)
(11.775, 48.049)
(11.85, 48.3517)
(11.925, 49.475)
(12, 51.2008)
(12.075, 52.7228)
(12.15, 52.8484)
(12.225, 50.8472)
(12.3, 48.4385)
(12.375, 47.3495)
(12.45, 48.5739)
(12.525, 50.3692)
(12.6, 52.4361)
(12.675, 53.104)
(12.75, 52.3728)
(12.825, 51.2282)
(12.9, 50.7928)
(12.975, 50.347)
(13.05, 50.6479)
(13.125, 50.1748)
(13.2, 49.9846)
(13.275, 50.4815)
(13.35, 50.2906)
(13.425, 50.4397)
(13.5, 49.759)
(13.575, 48.4117)
(13.65, 47.7867)
(13.725, 47.628)
(13.8, 48.3229)
(13.875, 48.7683)
(13.95, 49.0706)
(14.025, 48.8078)
(14.1, 49.1958)
(14.175, 49.7509)
(14.25, 50.2371)
(14.325, 50.7184)
(14.4, 50.7085)
(14.475, 49.8496)
(14.55, 49.036)
(14.625, 48.4042)
(14.7, 48.0488)
(14.775, 48.897)
(14.85, 50.49)
(14.925, 51.4233)
(15, 51.5629)
(15.075, 50.8384)
(15.15, 49.4248)
(15.225, 48.7745)
(15.3, 48.705)
(15.375, 50.7099)
(15.45, 51.5561)
(15.525, 51.3599)
(15.6, 50.082)
(15.675, 49.1261)
(15.75, 49.2385)
(15.825, 49.1224)
(15.9, 49.1024)
(15.975, 47.9871)
(16.05, 47.2612)
(16.125, 48.5152)
(16.2, 49.6837)
(16.275, 50.5481)
(16.35, 49.816)
(16.425, 48.5347)
(16.5, 47.5674)
(16.575, 47.3777)
(16.65, 49.0939)
(16.725, 50.4229)
(16.8, 50.181)
(16.875, 48.8413)
(16.95, 48.3105)
(17.025, 48.8997)
(17.1, 49.22)
(17.175, 49.4267)
(17.25, 49.8878)
(17.325, 50.2573)
(17.4, 49.4359)
(17.475, 49.1356)
(17.55, 48.8895)
(17.625, 48.6278)
(17.7, 49.0451)
(17.775, 49.3401)
(17.85, 49.4067)
(17.925, 49.5374)
(18, 49.8611)
(18.075, 50.1548)
(18.15, 50.3021)
(18.225, 50.1734)
(18.3, 50.4008)
(18.375, 50.1411)
(18.45, 49.3255)
(18.525, 48.5621)
(18.6, 48.3005)
(18.675, 47.7312)
(18.75, 46.9641)
(18.825, 47.0965)
(18.9, 48.4959)
(18.975, 50.1016)
(19.05, 50.7198)
(19.125, 51.001)
(19.2, 50.1434)
(19.275, 49.1065)
(19.35, 49.2676)
(19.425, 49.3335)
(19.5, 49.6072)
(19.575, 49.7437)
(19.65, 49.5105)
(19.725, 49.075)
(19.8, 47.4943)
(19.875, 46.7982)
(19.95, 48.1539)
(20.025, 51.4051)
(20.1, 53.6063)
(20.175, 54.0999)
(20.25, 52.3317)
(20.325, 49.823)
(20.4, 47.3636)
(20.475, 46.1107)
(20.55, 46.6303)
(20.625, 48.4243)
(20.7, 50.739)
(20.775, 51.5356)
(20.85, 50.7768)
(20.925, 49.4084)
(21, 47.6021)
(21.075, 46.3578)
(21.15, 46.5703)
(21.225, 48.0813)
(21.3, 48.5281)
(21.375, 49.1142)
(21.45, 49.4444)
(21.525, 48.7682)
(21.6, 47.8704)
(21.675, 47.0996)
(21.75, 47.1113)
(21.825, 48.1049)
(21.9, 48.516)
(21.975, 48.3402)
(22.05, 47.5256)
(22.125, 46.6544)
(22.2, 46.4292)
(22.275, 46.3536)
(22.35, 46.3282)
(22.425, 46.3034)
(22.5, 46.484)
(22.575, 46.8457)
(22.65, 47.0368)
(22.725, 46.9998)
(22.8, 46.7521)
(22.875, 45.9567)
(22.95, 45.3294)
(23.025, 45.6511)
(23.1, 46.509)
(23.175, 49.1892)
(23.25, 49.4199)
(23.325, 47.2254)
(23.4, 45.5036)
(23.475, 45.149)
(23.55, 45.6269)
(23.625, 46.3897)
(23.7, 46.9224)
(23.775, 46.893)
(23.85, 47.3948)
(23.925, 46.9241)
(24, 45.1846)
(24.075, 42.8534)
(24.15, 42.866)
(24.225, 43.3863)
(24.3, 43.3027)
(24.375, 42.4192)
(24.45, 40.7537)
(24.525, 40.4342)
(24.6, 40.0892)
(24.675, 39.1521)
(24.75, 38.525)
(24.825, 37.9338)
(24.9, 37.2699)
(24.975, 36.0641)
(25.05, 35.3965)
(25.125, 34.8316)
(25.2, 34.6882)
(25.275, 33.9498)
(25.35, 33.2618)
(25.425, 32.7985)
(25.5, 32.1794)
(25.575, 31.5634)
(25.65, 30.6614)
(25.725, 29.603)
(25.8, 28.413)
(25.875, 27.7256)
(25.95, 27.1792)
(26.025, 26.1342)
(26.1, 25.2045)
(26.175, 24.3237)
(26.25, 23.3981)
(26.325, 22.434)
(26.4, 21.4231)
(26.475, 20.6024)
(26.55, 19.6149)
(26.625, 18.7008)
(26.7, 17.5295)
(26.775, 16.4632)
(26.85, 15.7627)
(26.925, 14.911)
(27, 13.6875)
(27.075, 12.6927)
(27.15, 11.397)
(27.225, 10.4467)
(27.3, 10)
(27.375, 10)
(27.45, 10)
(27.525, 10)
(27.6, 10)
(27.675, 10)
(27.75, 10)
(27.825, 10)
(27.9, 10)
(27.975, 10)
(28.05, 10)
(28.125, 10)
(28.2, 10)
(28.275, 10)
(28.35, 10)
(28.425, 10)
(28.5, 10)
(28.575, 10)
(28.65, 10)
(28.725, 10)
(28.8, 10)
(28.875, 10)
(28.95, 10)
(29.025, 10)
(29.1, 10)
(29.175, 10)
(29.25, 10)
(29.325, 10)
(29.4, 10)
(29.475, 10)
(29.55, 10)
(29.625, 10)
(29.7, 10)
(29.775, 10)
(29.85, 10)
(29.925, 10)
(30, 10)
(30.075, 10)
(30.15, 10)
(30.225, 10)
(30.3, 10)
(30.375, 10)
(30.45, 10)
(30.525, 10)
(30.6, 10)
(30.675, 10)
(30.75, 10)
(30.825, 10)
(30.9, 10)
(30.975, 10)
(31.05, 10)
(31.125, 10)
(31.2, 10)
(31.275, 10)
(31.35, 10)
(31.425, 10)
(31.5, 10)
(31.575, 10)
(31.65, 10)
(31.725, 10)
(31.8, 10)
(31.875, 10)
(31.95, 10)
(32.025, 10)
(32.1, 10)
(32.175, 10)
(32.25, 10)
};

==> exp_plots/open_ws/x.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0)
(0.075, -0.000232231)
(0.15, -0.000147224)
(0.225, -0.000111155)
(0.3, -0.000134689)
(0.375, -0.000299059)
(0.45, -0.0008052)
(0.525, -0.000719813)
(0.6, -0.000100276)
(0.675, -5.33175e-05)
(0.75, -1.01951e-05)
(0.825, -2.52832e-05)
(0.9, 8.35417e-05)
(0.975, -8.18745e-05)
(1.05, 0.000565434)
(1.125, 0.0006346)
(1.2, 0.000196947)
(1.275, 2.76619e-05)
(1.35, -0.000242227)
(1.425, -0.000351283)
(1.5, -0.000623219)
(1.575, -0.000244865)
(1.65, 0.000428987)
(1.725, 0.00125241)
(1.8, 0.00680675)
(1.875, 0.00450234)
(1.95, 0.00207065)
(2.025, 0.0014552)
(2.1, 0.00124474)
(2.175, 0.000991978)
(2.25, 0.000390956)
(2.325, -0.00093483)
(2.4, -0.00154202)
(2.475, -0.00106423)
(2.55, -0.00151563)
(2.625, -0.00162886)
(2.7, 0.000285025)
(2.775, 0.0028949)
(2.85, 0.00156788)
(2.925, -0.00601675)
(3, -0.019017)
(3.075, -0.0391964)
(3.15, -0.0525151)
(3.225, -0.0772903)
(3.3, -0.0976081)
(3.375, -0.116326)
(3.45, -0.130184)
(3.525, -0.141917)
(3.6, -0.149163)
(3.675, -0.153119)
(3.75, -0.161602)
(3.825, -0.161302)
(3.9, -0.1617)
(3.975, -0.148782)
(4.05, -0.141997)
(4.125, -0.132757)
(4.2, -0.121207)
(4.275, -0.108499)
(4.35, -0.0967254)
(4.425, -0.0825261)
(4.5, -0.0718147)
(4.575, -0.0555485)
(4.65, -0.0382413)
(4.725, -0.0285425)
(4.8, -0.0199634)
(4.875, -0.00748337)
(4.95, 0.00175985)
(5.025, 0.00597322)
(5.1, 0.0157552)
(5.175, 0.0260796)
(5.25, 0.0323844)
(5.325, 0.0367716)
(5.4, 0.0401962)
(5.475, 0.0432059)
(5.55, 0.0443984)
(5.625, 0.0437338)
(5.7, 0.0423996)
(5.775, 0.0359393)
(5.85, 0.0321127)
(5.925, 0.0271676)
(6, 0.0228686)
(6.075, 0.0195836)
(6.15, 0.0184927)
(6.225, 0.015972)
(6.3, 0.0163575)
(6.375, 0.0132646)
(6.45, 0.00703638)
(6.525, 0.00628587)
(6.6, 0.00721686)
(6.675, 0.00424664)
(6.75, 0.000427268)
(6.825, -0.00617588)
(6.9, -0.0180877)
(6.975, -0.0247262)
(7.05, -0.030198)
(7.125, -0.0322229)
(7.2, -0.0337992)
(7.275, -0.0351098)
(7.35, -0.0328481)
(7.425, -0.0352332)
(7.5, -0.0350428)
(7.575, -0.0424388)
(7.65, -0.044513)
(7.725, -0.0463657)
(7.8, -0.0514143)
(7.875, -0.0503317)
(7.95, -0.0535017)
(8.025, -0.0526314)
(8.1, -0.0526112)
(8.175, -0.0552182)
(8.25, -0.0575419)
(8.325, -0.0589428)
(8.4, -0.060001)
(8.475, -0.0588853)
(8.55, -0.0594879)
(8.625, -0.0617182)
(8.7, -0.056622)
(8.775, -0.052828)
(8.85, -0.0502232)
(8.925, -0.0555409)
(9, -0.0527565)
(9.075, -0.0523528)
(9.15, -0.0506145)
(9.225, -0.0498358)
(9.3, -0.0408524)
(9.375, -0.0344497)
(9.45, -0.0288459)
(9.525, -0.0241329)
(9.6, -0.0183032)
(9.675, -0.0116454)
(9.75, 0.00176415)
(9.825, 0.0105024)
(9.9, 0.01808)
(9.975, 0.0234432)
(10.05, 0.0210734)
(10.125, 0.013724)
(10.2, 0.0127603)
(10.275, 0.0144949)
(10.35, 0.00974275)
(10.425, 0.00820441)
(10.5, 0.000943937)
(10.575, -0.00435241)
(10.65, -0.00746757)
(10.725, -0.00999954)
(10.8, -0.0132109)
(10.875, -0.014806)
(10.95, -0.0179621)
(11.025, -0.0209885)
(11.1, -0.0246744)
(11.175, -0.0278722)
(11.25, -0.0319496)
(11.325, -0.0351066)
(11.4, -0.0428984)
(11.475, -0.0453208)
(11.55, -0.0476215)
(11.625, -0.0456517)
(11.7, -0.0448452)
(11.775, -0.0426866)
(11.85, -0.0410476)
(11.925, -0.0397173)
(12, -0.0333387)
(12.075, -0.0304672)
(12.15, -0.0327568)
(12.225, -0.0331113)
(12.3, -0.0368379)
(12.375, -0.0392845)
(12.45, -0.0387674)
(12.525, -0.0385936)
(12.6, -0.0386971)
(12.675, -0.0374936)
(12.75, -0.0389059)
(12.825, -0.0356123)
(12.9, -0.0355454)
(12.975, -0.0368329)
(13.05, -0.0366771)
(13.125, -0.0346741)
(13.2, -0.0329033)
(13.275, -0.0276525)
(13.35, -0.0314898)
(13.425, -0.0295137)
(13.5, -0.0330389)
(13.575, -0.0343762)
(13.65, -0.036439)
(13.725, -0.0363662)
(13.8, -0.0361724)
(13.875, -0.0357844)
(13.95, -0.0340747)
(14.025, -0.0351951)
(14.1, -0.0367518)
(14.175, -0.0368361)
(14.25, -0.0330296)
(14.325, -0.0308002)
(14.4, -0.0274978)
(14.475, -0.0228097)
(14.55, -0.0180031)
(14.625, -0.0216922)
(14.7, -0.0188809)
(14.775, -0.0171037)
(14.85, -0.0161526)
(14.925, -0.0187817)
(15, -0.017169)
(15.075, -0.0145489)
(15.15, -0.0150267)
(15.225, -0.0161443)
(15.3, -0.0169301)
(15.375, -0.0246372)
(15.45, -0.0259153)
(15.525, -0.0250768)
(15.6, -0.0254823)
(15.675, -0.0224298)
(15.75, -0.0200012)
(15.825, -0.0237364)
(15.9, -0.0210679)
(15.975, -0.0273585)
(16.05, -0.0268496)
(16.125, -0.0317093)
(16.2, -0.0352168)
(16.275, -0.0314166)
(16.35, -0.0335681)
(16.425, -0.0354033)
(16.5, -0.0354375)
(16.575, -0.0317057)
(16.65, -0.0297214)
(16.725, -0.0261761)
(16.8, -0.0268929)
(16.875, -0.0267942)
(16.95, -0.024955)
(17.025, -0.026834)
(17.1, -0.025537)
(17.175, -0.0263799)
(17.25, -0.0244753)
(17.325, -0.0252858)
(17.4, -0.0229606)
(17.475, -0.0207626)
(17.55, -0.019624)
(17.625, -0.014909)
(17.7, -0.010244)
(17.775, -0.0117175)
(17.85, -0.0129393)
(17.925, -0.013112)
(18, -0.0153472)
(18.075, -0.0163941)
(18.15, -0.0161331)
(18.225, -0.0160171)
(18.3, -0.0240566)
(18.375, -0.0259002)
(18.45, -0.0344535)
(18.525, -0.0394441)
(18.6, -0.0401379)
(18.675, -0.0430788)
(18.75, -0.041445)
(18.825, -0.0412446)
(18.9, -0.04209)
(18.975, -0.0417061)
(19.05, -0.043059)
(19.125, -0.0443662)
(19.2, -0.0447359)
(19.275, -0.0467168)
(19.35, -0.0457949)
(19.425, -0.0442605)
(19.5, -0.0407618)
(19.575, -0.0363011)
(19.65, -0.029519)
(19.725, -0.0253346)
(19.8, -0.0203511)
(19.875, -0.0206259)
(19.95, -0.0190602)
(20.025, -0.0127512)
(20.1, -0.0138058)
(20.175, -0.00958774)
(20.25, -0.0111713)
(20.325, -0.015061)
(20.4, -0.016746)
(20.475, -0.01484)
(20.55, -0.016931)
(20.625, -0.0193431)
(20.7, -0.0185352)
(20.775, -0.0231752)
(20.85, -0.0256486)
(20.925, -0.0250839)
(21, -0.0246261)
(21.075, -0.0262975)
(21.15, -0.0264602)
(21.225, -0.026379)
(21.3, -0.0270786)
(21.375, -0.0238826)
(21.45, -0.024894)
(21.525, -0.0249249)
(21.6, -0.0317249)
(21.675, -0.0320855)
(21.75, -0.0344927)
(21.825, -0.0349538)
(21.9, -0.0387143)
(21.975, -0.0410164)
(22.05, -0.043455)
(22.125, -0.0476429)
(22.2, -0.0452286)
(22.275, -0.0535914)
(22.35, -0.0571925)
(22.425, -0.0567453)
(22.5, -0.0617319)
(22.575, -0.0620694)
(22.65, -0.0634106)
(22.725, -0.0652761)
(22.8, -0.0654743)
(22.875, -0.0714338)
(22.95, -0.0722957)
(23.025, -0.0730257)
(23.1, -0.0723071)
(23.175, -0.0755469)
(23.25, -0.0800326)
(23.325, -0.0787363)
(23.4, -0.0769331)
(23.475, -0.0781211)
(23.55, -0.0676796)
(23.625, -0.062211)
(23.7, -0.058115)
(23.775, -0.0518246)
(23.85, -0.0452621)
(23.925, -0.0302387)
(24, -0.0217737)
(24.075, -0.0138844)
(24.15, -0.00686587)
(24.225, -0.00332754)
(24.3, 0.00524162)
(24.375, 0.0131432)
(24.45, 0.0155395)
(24.525, 0.0187944)
(24.6, 0.0197542)
(24.675, 0.0152506)
(24.75, 0.0159078)
(24.825, 0.0153117)
(24.9, 0.0154214)
(24.975, 0.015875)
(25.05, 0.0183283)
(25.125, 0.0207745)
(25.2, 0.022721)
(25.275, 0.0250748)
(25.35, 0.026712)
(25.425, 0.0274892)
(25.5, 0.0274284)
(25.575, 0.0278384)
(25.65, 0.0277191)
(25.725, 0.0279864)
(25.8, 0.0262939)
(25.875, 0.0256917)
(25.95, 0.0250816)
(26.025, 0.0254001)
(26.1, 0.0245293)
(26.175, 0.0235394)
(26.25, 0.0234674)
(26.325, 0.0239639)
(26.4, 0.0247307)
(26.475, 0.0247585)
(26.55, 0.024397)
(26.625, 0.0237509)
(26.7, 0.0236955)
(26.775, 0.0237013)
(26.85, 0.0246042)
(26.925, 0.0253858)
(27, 0.0224812)
(27.075, 0.0214287)
(27.15, 0.0193014)
(27.225, 0.0182967)
(27.3, 0.018033)
(27.375, 0.0182197)
(27.45, 0.0185028)
(27.525, 0.0184609)
(27.6, 0.018584)
(27.675, 0.0199773)
(27.75, 0.0205353)
(27.825, 0.0207533)
(27.9, 0.0210609)
(27.975, 0.0209937)
(28.05, 0.0208413)
(28.125, 0.0199975)
(28.2, 0.0193395)
(28.275, 0.0183431)
(28.35, 0.0187755)
(28.425, 0.0188821)
(28.5, 0.0187719)
(28.575, 0.0187729)
(28.65, 0.0187147)
(28.725, 0.0189947)
(28.8, 0.0191071)
(28.875, 0.0191759)
(28.95, 0.0193537)
(29.025, 0.0190883)
(29.1, 0.0190877)
(29.175, 0.0191797)
(29.25, 0.019329)
(29.325, 0.0193249)
(29.4, 0.0185695)
(29.475, 0.0175552)
(29.55, 0.0180105)
(29.625, 0.0178174)
(29.7, 0.0180568)
(29.775, 0.0179225)
(29.85, 0.0188666)
(29.925, 0.0207566)
(30, 0.0216274)
(30.075, 0.0218611)
(30.15, 0.0207779)
(30.225, 0.0198622)
(30.3, 0.019849)
(30.375, 0.0195998)
(30.45, 0.0202134)
(30.525, 0.0184648)
(30.6, 0.0172026)
(30.675, 0.016497)
(30.75, 0.0152229)
(30.825, 0.0156485)
(30.9, 0.0167801)
(30.975, 0.016106)
(31.05, 0.0155172)
(31.125, 0.016235)
(31.2, 0.0169433)
(31.275, 0.0163399)
(31.35, 0.0146773)
(31.425, 0.0152466)
(31.5, 0.0155516)
(31.575, 0.0141157)
(31.65, 0.0167131)
(31.725, 0.0176258)
(31.8, 0.0147392)
(31.875, 0.0118216)
(31.95, 0.0109058)
(32.025, 0.0111787)
(32.1, 0.0104394)
(32.175, 0.0112631)
(32.25, 0.0125788)
};

==> exp_plots/open_ws/x_des.tex <==
\addplot[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates {
(0, 0)
(0.075, 0)
(0.15, 0)
(0.225, 0)
(0.3, 0)
(0.375, 0)
(0.45, 0)
(0.525, 0)
(0.6, 0)
(0.675, 0)
(0.75, 0)
(0.825, 0)
(0.9, 0)
(0.975, 0)
(1.05, 0)
(1.125, 0)
(1.2, 0)
(1.275, 0)
(1.35, 0)
(1.425, 0)
(1.5, 0)
(1.575, 0)
(1.65, 0)
(1.725, 0)
(1.8, 0)
(1.875, 0)
(1.95, 0)
(2.025, 0)
(2.1, 0)
(2.175, 0)
(2.25, 0)
(2.325, 0)
(2.4, 0)
(2.475, 0)
(2.55, 0)
(2.625, 0)
(2.7, 0)
(2.775, 0)
(2.85, 0)
(2.925, 0)
(3, 0)
(3.075, 0)
(3.15, 0)
(3.225, 0)
(3.3, 0)
(3.375, 0)
(3.45, 0)
(3.525, 0)
(3.6, 0)
(3.675, 0)
(3.75, 0)
(3.825, 0)
(3.9, 0)
(3.975, 0)
(4.05, 0)
(4.125, 0)
(4.2, 0)
(4.275, 0)
(4.35, 0)
(4.425, 0)
(4.5, 0)
(4.575, 0)
(4.65, 0)
(4.725, 0)
(4.8, 0)
(4.875, 0)
(4.95, 0)
(5.025, 0)
(5.1, 0)
(5.175, 0)
(5.25, 0)
(5.325, 0)
(5.4, 0)
(5.475, 0)
(5.55, 0)
(5.625, 0)
(5.7, 0)
(5.775, 0)
(5.85, 0)
(5.925, 0)
(6, 0)
(6.075, 0)
(6.15, 0)
(6.225, 0)
(6.3, 0)
(6.375, 0)
(6.45, 0)
(6.525, 0)
(6.6, 0)
(6.675, 0)
(6.75, 0)
(6.825, 0)
(6.9, 0)
(6.975, 0)
(7.05, 0)
(7.125, 0)
(7.2, 0)
(7.275, 0)
(7.35, 0)
(7.425, 0)
(7.5, 0)
(7.575, 0)
(7.65, 0)
(7.725, 0)
(7.8, 0)
(7.875, 0)
(7.95, 0)
(8.025, 0)
(8.1, 0)
(8.175, 0)
(8.25, 0)
(8.325, 0)
(8.4, 0)
(8.475, 0)
(8.55, 0)
(8.625, 0)
(8.7, 0)
(8.775, 0)
(8.85, 0)
(8.925, 0)
(9, 0)
(9.075, 0)
(9.15, 0)
(9.225, 0)
(9.3, 0)
(9.375, 0)
(9.45, 0)
(9.525, 0)
(9.6, 0)
(9.675, 0)
(9.75, 0)
(9.825, 0)
(9.9, 0)
(9.975, 0)
(10.05, 0)
(10.125, 0)
(10.2, 0)
(10.275, 0)
(10.35, 0)
(10.425, 0)
(10.5, 0)
(10.575, 0)
(10.65, 0)
(10.725, 0)
(10.8, 0)
(10.875, 0)
(10.95, 0)
(11.025, 0)
(11.1, 0)
(11.175, 0)
(11.25, 0)
(11.325, 0)
(11.4, 0)
(11.475, 0)
(11.55, 0)
(11.625, 0)
(11.7, 0)
(11.775, 0)
(11.85, 0)
(11.925, 0)
(12, 0)
(12.075, 0)
(12.15, 0)
(12.225, 0)
(12.3, 0)
(12.375, 0)
(12.45, 0)
(12.525, 0)
(12.6, 0)
(12.675, 0)
(12.75, 0)
(12.825, 0)
(12.9, 0)
(12.975, 0)
(13.05, 0)
(13.125, 0)
(13.2, 0)
(13.275, 0)
(13.35, 0)
(13.425, 0)
(13.5, 0)
(13.575, 0)
(13.65, 0)
(13.725, 0)
(13.8, 0)
(13.875, 0)
(13.95, 0)
(14.025, 0)
(14.1, 0)
(14.175, 0)
(14.25, 0)
(14.325, 0)
(14.4, 0)
(14.475, 0)
(14.55, 0)
(14.625, 0)
(14.7, 0)
(14.775, 0)
(14.85, 0)
(14.925, 0)
(15, 0)
(15.075, 0)
(15.15, 0)
(15.225, 0)
(15.3, 0)
(15.375, 0)
(15.45, 0)
(15.525, 0)
(15.6, 0)
(15.675, 0)
(15.75, 0)
(15.825, 0)
(15.9, 0)
(15.975, 0)
(16.05, 0)
(16.125, 0)
(16.2, 0)
(16.275, 0)
(16.35, 0)
(16.425, 0)
(16.5, 0)
(16.575, 0)
(16.65, 0)
(16.725, 0)
(16.8, 0)
(16.875, 0)
(16.95, 0)
(17.025, 0)
(17.1, 0)
(17.175, 0)
(17.25, 0)
(17.325, 0)
(17.4, 0)
(17.475, 0)
(17.55, 0)
(17.625, 0)
(17.7, 0)
(17.775, 0)
(17.85, 0)
(17.925, 0)
(18, 0)
(18.075, 0)
(18.15, 0)
(18.225, 0)
(18.3, 0)
(18.375, 0)
(18.45, 0)
(18.525, 0)
(18.6, 0)
(18.675, 0)
(18.75, 0)
(18.825, 0)
(18.9, 0)
(18.975, 0)
(19.05, 0)
(19.125, 0)
(19.2, 0)
(19.275, 0)
(19.35, 0)
(19.425, 0)
(19.5, 0)
(19.575, 0)
(19.65, 0)
(19.725, 0)
(19.8, 0)
(19.875, 0)
(19.95, 0)
(20.025, 0)
(20.1, 0)
(20.175, 0)
(20.25, 0)
(20.325, 0)
(20.4, 0)
(20.475, 0)
(20.55, 0)
(20.625, 0)
(20.7, 0)
(20.775, 0)
(20.85, 0)
(20.925, 0)
(21, 0)
(21.075, 0)
(21.15, 0)
(21.225, 0)
(21.3, 0)
(21.375, 0)
(21.45, 0)
(21.525, 0)
(21.6, 0)
(21.675, 0)
(21.75, 0)
(21.825, 0)
(21.9, 0)
(21.975, 0)
(22.05, 0)
(22.125, 0)
(22.2, 0)
(22.275, 0)
(22.35, 0)
(22.425, 0)
(22.5, 0)
(22.575, 0)
(22.65, 0)
(22.725, 0)
(22.8, 0)
(22.875, 0)
(22.95, 0)
(23.025, 0)
(23.1, 0)
(23.175, 0)
(23.25, 0)
(23.325, 0)
(23.4, 0)
(23.475, 0)
(23.55, 0)
(23.625, 0)
(23.7, 0)
(23.775, 0)
(23.85, 0)
(23.925, 0)
(24, 0)
(24.075, 0)
(24.15, 0)
(24.225, 0)
(24.3, 0)
(24.375, 0)
(24.45, 0)
(24.525, 0)
(24.6, 0)
(24.675, 0)
(24.75, 0)
(24.825, 0)
(24.9, 0)
(24.975, 0)
(25.05, 0)
(25.125, 0)
(25.2, 0)
(25.275, 0)
(25.35, 0)
(25.425, 0)
(25.5, 0)
(25.575, 0)
(25.65, 0)
(25.725, 0)
(25.8, 0)
(25.875, 0)
(25.95, 0)
(26.025, 0)
(26.1, 0)
(26.175, 0)
(26.25, 0)
(26.325, 0)
(26.4, 0)
(26.475, 0)
(26.55, 0)
(26.625, 0)
(26.7, 0)
(26.775, 0)
(26.85, 0)
(26.925, 0)
(27, 0)
(27.075, 0)
(27.15, 0)
(27.225, 0)
(27.3, 0)
(27.375, 0)
(27.45, 0)
(27.525, 0)
(27.6, 0)
(27.675, 0)
(27.75, 0)
(27.825, 0)
(27.9, 0)
(27.975, 0)
(28.05, 0)
(28.125, 0)
(28.2, 0)
(28.275, 0)
(28.35, 0)
(28.425, 0)
(28.5, 0)
(28.575, 0)
(28.65, 0)
(28.725, 0)
(28.8, 0)
(28.875, 0)
(28.95, 0)
(29.025, 0)
(29.1, 0)
(29.175, 0)
(29.25, 0)
(29.325, 0)
(29.4, 0)
(29.475, 0)
(29.55, 0)
(29.625, 0)
(29.7, 0)
(29.775, 0)
(29.85, 0)
(29.925, 0)
(30, 0)
(30.075, 0)
(30.15, 0)
(30.225, 0)
(30.3, 0)
(30.375, 0)
(30.45, 0)
(30.525, 0)
(30.6, 0)
(30.675, 0)
(30.75, 0)
(30.825, 0)
(30.9, 0)
(30.975, 0)
(31.05, 0)
(31.125, 0)
(31.2, 0)
(31.275, 0)
(31.35, 0)
(31.425, 0)
(31.5, 0)
(31.575, 0)
(31.65, 0)
(31.725, 0)
(31.8, 0)
(31.875, 0)
(31.95, 0)
(32.025, 0)
(32.1, 0)
(32.175, 0)
(32.25, 0)
};

==> exp_plots/open_ws/y.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0)
(0.075, 0.00026747)
(0.15, -2.79423e-05)
(0.225, -9.09982e-05)
(0.3, -7.85262e-06)
(0.375, 0.000257844)
(0.45, 0.000571022)
(0.525, 0.000547639)
(0.6, 0.000145799)
(0.675, 4.06254e-05)
(0.75, -2.07488e-05)
(0.825, -3.02709e-05)
(0.9, -8.94509e-06)
(0.975, 0.000190459)
(1.05, 4.13183e-05)
(1.125, 0.00012247)
(1.2, 0.000298806)
(1.275, 0.000251259)
(1.35, 0.000274625)
(1.425, 0.000142985)
(1.5, 0.000768588)
(1.575, 0.0011802)
(1.65, 0.00213617)
(1.725, 0.0132722)
(1.8, 0.0103901)
(1.875, 0.00601559)
(1.95, 0.00298693)
(2.025, 0.0025946)
(2.1, 0.00224644)
(2.175, 0.00174152)
(2.25, 0.00192548)
(2.325, 0.00214138)
(2.4, 0.0033079)
(2.475, 0.00153468)
(2.55, 0.00411577)
(2.625, 0.00324568)
(2.7, 0.00329783)
(2.775, 0.00114544)
(2.85, -0.00443715)
(2.925, -0.0100774)
(3, -0.0106379)
(3.075, -0.0148068)
(3.15, -0.0242861)
(3.225, -0.0259392)
(3.3, -0.0346793)
(3.375, -0.0426356)
(3.45, -0.053731)
(3.525, -0.0663541)
(3.6, -0.0776526)
(3.675, -0.0825253)
(3.75, -0.088869)
(3.825, -0.0875809)
(3.9, -0.0941835)
(3.975, -0.10075)
(4.05, -0.103633)
(4.125, -0.106757)
(4.2, -0.110648)
(4.275, -0.113842)
(4.35, -0.115824)
(4.425, -0.11692)
(4.5, -0.11511)
(4.575, -0.111297)
(4.65, -0.106566)
(4.725, -0.105741)
(4.8, -0.107035)
(4.875, -0.105267)
(4.95, -0.0976068)
(5.025, -0.0921952)
(5.1, -0.0882385)
(5.175, -0.0818052)
(5.25, -0.0758653)
(5.325, -0.0662331)
(5.4, -0.0559155)
(5.475, -0.0508032)
(5.55, -0.0451643)
(5.625, -0.0432828)
(5.7, -0.0383373)
(5.775, -0.0245494)
(5.85, -0.0190784)
(5.925, -0.0147184)
(6, -0.00920835)
(6.075, 0.000230828)
(6.15, 0.000665032)
(6.225, -0.000766363)
(6.3, -0.00262746)
(6.375, -0.00322423)
(6.45, -0.00368037)
(6.525, -0.00544858)
(6.6, -0.00788669)
(6.675, -0.00944197)
(6.75, -0.00758536)
(6.825, -0.00871069)
(6.9, -0.00820639)
(6.975, -0.0087354)
(7.05, -0.0138516)
(7.125, -0.0122813)
(7.2, -0.0159757)
(7.275, -0.0185495)
(7.35, -0.0136684)
(7.425, -0.0131616)
(7.5, -0.0119864)
(7.575, -0.00559141)
(7.65, -0.00602818)
(7.725, -0.00581172)
(7.8, -0.00352393)
(7.875, -0.00643042)
(7.95, -0.00704477)
(8.025, -0.00746818)
(8.1, -0.00460963)
(8.175, -0.00686745)
(8.25, -0.00980053)
(8.325, -0.0153637)
(8.4, -0.0163371)
(8.475, -0.0215675)
(8.55, -0.0240421)
(8.625, -0.0232228)
(8.7, -0.0218952)
(8.775, -0.0209936)
(8.85, -0.0211009)
(8.925, -0.0269851)
(9, -0.033527)
(9.075, -0.0397625)
(9.15, -0.0566156)
(9.225, -0.0678539)
(9.3, -0.0749046)
(9.375, -0.0798385)
(9.45, -0.0880727)
(9.525, -0.0918859)
(9.6, -0.0940172)
(9.675, -0.0938826)
(9.75, -0.0984991)
(9.825, -0.103945)
(9.9, -0.105087)
(9.975, -0.106635)
(10.05, -0.102781)
(10.125, -0.0943092)
(10.2, -0.094067)
(10.275, -0.0949346)
(10.35, -0.0900327)
(10.425, -0.082807)
(10.5, -0.07179)
(10.575, -0.0670689)
(10.65, -0.0642018)
(10.725, -0.0536342)
(10.8, -0.0429707)
(10.875, -0.0384006)
(10.95, -0.0351252)
(11.025, -0.0308856)
(11.1, -0.0296381)
(11.175, -0.0273117)
(11.25, -0.0225103)
(11.325, -0.0195385)
(11.4, -0.0150876)
(11.475, -0.0122071)
(11.55, -0.0112839)
(11.625, -0.010594)
(11.7, -0.01204)
(11.775, -0.0137831)
(11.85, -0.014594)
(11.925, -0.0214623)
(12, -0.0294257)
(12.075, -0.0347946)
(12.15, -0.0342198)
(12.225, -0.0305403)
(12.3, -0.0284998)
(12.375, -0.0260633)
(12.45, -0.0279403)
(12.525, -0.028534)
(12.6, -0.0255691)
(12.675, -0.0250457)
(12.75, -0.0259105)
(12.825, -0.03283)
(12.9, -0.0363879)
(12.975, -0.0361516)
(13.05, -0.0472861)
(13.125, -0.0587258)
(13.2, -0.0621324)
(13.275, -0.0638975)
(13.35, -0.0635591)
(13.425, -0.0641706)
(13.5, -0.0679698)
(13.575, -0.0699907)
(13.65, -0.0715192)
(13.725, -0.0750558)
(13.8, -0.0764402)
(13.875, -0.0792123)
(13.95, -0.0793287)
(14.025, -0.0783309)
(14.1, -0.0786674)
(14.175, -0.0776814)
(14.25, -0.0774242)
(14.325, -0.0777379)
(14.4, -0.0779209)
(14.475, -0.0813324)
(14.55, -0.0838097)
(14.625, -0.0771222)
(14.7, -0.0688356)
(14.775, -0.0661278)
(14.85, -0.061299)
(14.925, -0.0503413)
(15, -0.0462362)
(15.075, -0.0399117)
(15.15, -0.0329949)
(15.225, -0.0278219)
(15.3, -0.027091)
(15.375, -0.0212763)
(15.45, -0.0203878)
(15.525, -0.0219869)
(15.6, -0.0198786)
(15.675, -0.0195552)
(15.75, -0.0207018)
(15.825, -0.0195108)
(15.9, -0.0177798)
(15.975, -0.0152763)
(16.05, -0.0158321)
(16.125, -0.0196304)
(16.2, -0.0183753)
(16.275, -0.022486)
(16.35, -0.0236875)
(16.425, -0.0294322)
(16.5, -0.0317711)
(16.575, -0.0358985)
(16.65, -0.0487137)
(16.725, -0.0592033)
(16.8, -0.0655852)
(16.875, -0.0694049)
(16.95, -0.0724256)
(17.025, -0.0727362)
(17.1, -0.0715447)
(17.175, -0.0692877)
(17.25, -0.0688151)
(17.325, -0.0671272)
(17.4, -0.0665866)
(17.475, -0.0650994)
(17.55, -0.0634314)
(17.625, -0.0595158)
(17.7, -0.0587064)
(17.775, -0.0574208)
(17.85, -0.0526362)
(17.925, -0.0478613)
(18, -0.0430799)
(18.075, -0.0425354)
(18.15, -0.0414778)
(18.225, -0.0379676)
(18.3, -0.0375165)
(18.375, -0.0349304)
(18.45, -0.0295334)
(18.525, -0.029963)
(18.6, -0.0318223)
(18.675, -0.0345304)
(18.75, -0.0326438)
(18.825, -0.0348021)
(18.9, -0.0331834)
(18.975, -0.0301718)
(19.05, -0.0279793)
(19.125, -0.0248297)
(19.2, -0.0193797)
(19.275, -0.0127016)
(19.35, -0.00962954)
(19.425, -0.00904135)
(19.5, -0.00335822)
(19.575, 0.00192678)
(19.65, 0.00464596)
(19.725, 0.0040466)
(19.8, 0.00531918)
(19.875, 0.0041229)
(19.95, 0.00328653)
(20.025, -0.00817089)
(20.1, -0.0116362)
(20.175, -0.0229252)
(20.25, -0.030401)
(20.325, -0.0398252)
(20.4, -0.0518444)
(20.475, -0.0546814)
(20.55, -0.0563468)
(20.625, -0.0609133)
(20.7, -0.0617321)
(20.775, -0.0692626)
(20.85, -0.0737349)
(20.925, -0.0681031)
(21, -0.0648729)
(21.075, -0.0625444)
(21.15, -0.0625831)
(21.225, -0.062241)
(21.3, -0.0635072)
(21.375, -0.0639058)
(21.45, -0.0629767)
(21.525, -0.0607607)
(21.6, -0.0545491)
(21.675, -0.0473618)
(21.75, -0.0439769)
(21.825, -0.0396875)
(21.9, -0.0293221)
(21.975, -0.0258335)
(22.05, -0.0257597)
(22.125, -0.0252787)
(22.2, -0.0258633)
(22.275, -0.0266692)
(22.35, -0.0257738)
(22.425, -0.0244809)
(22.5, -0.0208557)
(22.575, -0.0210871)
(22.65, -0.023161)
(22.725, -0.0236119)
(22.8, -0.0261021)
(22.875, -0.0274171)
(22.95, -0.0323572)
(23.025, -0.0358106)
(23.1, -0.0418163)
(23.175, -0.0437006)
(23.25, -0.0454617)
(23.325, -0.0472515)
(23.4, -0.0507876)
(23.475, -0.0572975)
(23.55, -0.061902)
(23.625, -0.0636114)
(23.7, -0.0670747)
(23.775, -0.0764408)
(23.85, -0.0784829)
(23.925, -0.0786224)
(24, -0.078872)
(24.075, -0.0845158)
(24.15, -0.0821522)
(24.225, -0.0818229)
(24.3, -0.0757025)
(24.375, -0.0717917)
(24.45, -0.0699043)
(24.525, -0.0697436)
(24.6, -0.0704239)
(24.675, -0.0706863)
(24.75, -0.0681231)
(24.825, -0.0710364)
(24.9, -0.070337)
(24.975, -0.0719737)
(25.05, -0.0751825)
(25.125, -0.07798)
(25.2, -0.0785801)
(25.275, -0.078952)
(25.35, -0.0795158)
(25.425, -0.0800986)
(25.5, -0.0801888)
(25.575, -0.0805901)
(25.65, -0.0808567)
(25.725, -0.0808768)
(25.8, -0.0796697)
(25.875, -0.0797213)
(25.95, -0.0794729)
(26.025, -0.0797382)
(26.1, -0.0794723)
(26.175, -0.0790755)
(26.25, -0.079283)
(26.325, -0.0798641)
(26.4, -0.0804905)
(26.475, -0.0805427)
(26.55, -0.0803726)
(26.625, -0.0800126)
(26.7, -0.0800316)
(26.775, -0.080073)
(26.85, -0.0806479)
(26.925, -0.0811739)
(27, -0.0827771)
(27.075, -0.0835671)
(27.15, -0.0832757)
(27.225, -0.0831023)
(27.3, -0.0833239)
(27.375, -0.0830043)
(27.45, -0.0826985)
(27.525, -0.0824672)
(27.6, -0.0824029)
(27.675, -0.0830753)
(27.75, -0.0834797)
(27.825, -0.0837939)
(27.9, -0.0841546)
(27.975, -0.0842359)
(28.05, -0.0841977)
(28.125, -0.083873)
(28.2, -0.0836578)
(28.275, -0.0828912)
(28.35, -0.0831185)
(28.425, -0.0831344)
(28.5, -0.082935)
(28.575, -0.0827878)
(28.65, -0.0826647)
(28.725, -0.0828992)
(28.8, -0.0830556)
(28.875, -0.0831227)
(28.95, -0.0832565)
(29.025, -0.0831039)
(29.1, -0.0831735)
(29.175, -0.0832869)
(29.25, -0.0834836)
(29.325, -0.0835626)
(29.4, -0.0837049)
(29.475, -0.0833247)
(29.55, -0.0834066)
(29.625, -0.0833947)
(29.7, -0.0829492)
(29.775, -0.0828928)
(29.85, -0.0830275)
(29.925, -0.0816672)
(30, -0.0810446)
(30.075, -0.0808241)
(30.15, -0.0808632)
(30.225, -0.0802316)
(30.3, -0.080518)
(30.375, -0.0803788)
(30.45, -0.0800703)
(30.525, -0.0799554)
(30.6, -0.0796214)
(30.675, -0.0789713)
(30.75, -0.0784609)
(30.825, -0.0775609)
(30.9, -0.0767356)
(30.975, -0.0762018)
(31.05, -0.0758461)
(31.125, -0.0754456)
(31.2, -0.0755025)
(31.275, -0.0749839)
(31.35, -0.0746306)
(31.425, -0.0761999)
(31.5, -0.0762385)
(31.575, -0.0736955)
(31.65, -0.0754237)
(31.725, -0.0771171)
(31.8, -0.0773005)
(31.875, -0.0765676)
(31.95, -0.0762508)
(32.025, -0.0753033)
(32.1, -0.0766665)
(32.175, -0.0766031)
(32.25, -0.0770284)
};

==> exp_plots/open_ws/y_des.tex <==
\addplot[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates {
(0, 0)
(0.075, 0)
(0.15, 0)
(0.225, 0)
(0.3, 0)
(0.375, 0)
(0.45, 0)
(0.525, 0)
(0.6, 0)
(0.675, 0)
(0.75, 0)
(0.825, 0)
(0.9, 0)
(0.975, 0)
(1.05, 0)
(1.125, 0)
(1.2, 0)
(1.275, 0)
(1.35, 0)
(1.425, 0)
(1.5, 0)
(1.575, 0)
(1.65, 0)
(1.725, 0)
(1.8, 0)
(1.875, 0)
(1.95, 0)
(2.025, 0)
(2.1, 0)
(2.175, 0)
(2.25, 0)
(2.325, 0)
(2.4, 0)
(2.475, 0)
(2.55, 0)
(2.625, 0)
(2.7, 0)
(2.775, 0)
(2.85, 0)
(2.925, 0)
(3, 0)
(3.075, 0)
(3.15, 0)
(3.225, 0)
(3.3, 0)
(3.375, 0)
(3.45, 0)
(3.525, 0)
(3.6, 0)
(3.675, 0)
(3.75, 0)
(3.825, 0)
(3.9, 0)
(3.975, 0)
(4.05, 0)
(4.125, 0)
(4.2, 0)
(4.275, 0)
(4.35, 0)
(4.425, 0)
(4.5, 0)
(4.575, 0)
(4.65, 0)
(4.725, 0)
(4.8, 0)
(4.875, 0)
(4.95, 0)
(5.025, 0)
(5.1, 0)
(5.175, 0)
(5.25, 0)
(5.325, 0)
(5.4, 0)
(5.475, 0)
(5.55, 0)
(5.625, 0)
(5.7, 0)
(5.775, 0)
(5.85, 0)
(5.925, 0)
(6, 0)
(6.075, 0)
(6.15, 0)
(6.225, 0)
(6.3, 0)
(6.375, 0)
(6.45, 0)
(6.525, 0)
(6.6, 0)
(6.675, 0)
(6.75, 0)
(6.825, 0)
(6.9, 0)
(6.975, 0)
(7.05, 0)
(7.125, 0)
(7.2, 0)
(7.275, 0)
(7.35, 0)
(7.425, 0)
(7.5, 0)
(7.575, 0)
(7.65, 0)
(7.725, 0)
(7.8, 0)
(7.875, 0)
(7.95, 0)
(8.025, 0)
(8.1, 0)
(8.175, 0)
(8.25, 0)
(8.325, 0)
(8.4, 0)
(8.475, 0)
(8.55, 0)
(8.625, 0)
(8.7, 0)
(8.775, 0)
(8.85, 0)
(8.925, 0)
(9, 0)
(9.075, 0)
(9.15, 0)
(9.225, 0)
(9.3, 0)
(9.375, 0)
(9.45, 0)
(9.525, 0)
(9.6, 0)
(9.675, 0)
(9.75, 0)
(9.825, 0)
(9.9, 0)
(9.975, 0)
(10.05, 0)
(10.125, 0)
(10.2, 0)
(10.275, 0)
(10.35, 0)
(10.425, 0)
(10.5, 0)
(10.575, 0)
(10.65, 0)
(10.725, 0)
(10.8, 0)
(10.875, 0)
(10.95, 0)
(11.025, 0)
(11.1, 0)
(11.175, 0)
(11.25, 0)
(11.325, 0)
(11.4, 0)
(11.475, 0)
(11.55, 0)
(11.625, 0)
(11.7, 0)
(11.775, 0)
(11.85, 0)
(11.925, 0)
(12, 0)
(12.075, 0)
(12.15, 0)
(12.225, 0)
(12.3, 0)
(12.375, 0)
(12.45, 0)
(12.525, 0)
(12.6, 0)
(12.675, 0)
(12.75, 0)
(12.825, 0)
(12.9, 0)
(12.975, 0)
(13.05, 0)
(13.125, 0)
(13.2, 0)
(13.275, 0)
(13.35, 0)
(13.425, 0)
(13.5, 0)
(13.575, 0)
(13.65, 0)
(13.725, 0)
(13.8, 0)
(13.875, 0)
(13.95, 0)
(14.025, 0)
(14.1, 0)
(14.175, 0)
(14.25, 0)
(14.325, 0)
(14.4, 0)
(14.475, 0)
(14.55, 0)
(14.625, 0)
(14.7, 0)
(14.775, 0)
(14.85, 0)
(14.925, 0)
(15, 0)
(15.075, 0)
(15.15, 0)
(15.225, 0)
(15.3, 0)
(15.375, 0)
(15.45, 0)
(15.525, 0)
(15.6, 0)
(15.675, 0)
(15.75, 0)
(15.825, 0)
(15.9, 0)
(15.975, 0)
(16.05, 0)
(16.125, 0)
(16.2, 0)
(16.275, 0)
(16.35, 0)
(16.425, 0)
(16.5, 0)
(16.575, 0)
(16.65, 0)
(16.725, 0)
(16.8, 0)
(16.875, 0)
(16.95, 0)
(17.025, 0)
(17.1, 0)
(17.175, 0)
(17.25, 0)
(17.325, 0)
(17.4, 0)
(17.475, 0)
(17.55, 0)
(17.625, 0)
(17.7, 0)
(17.775, 0)
(17.85, 0)
(17.925, 0)
(18, 0)
(18.075, 0)
(18.15, 0)
(18.225, 0)
(18.3, 0)
(18.375, 0)
(18.45, 0)
(18.525, 0)
(18.6, 0)
(18.675, 0)
(18.75, 0)
(18.825, 0)
(18.9, 0)
(18.975, 0)
(19.05, 0)
(19.125, 0)
(19.2, 0)
(19.275, 0)
(19.35, 0)
(19.425, 0)
(19.5, 0)
(19.575, 0)
(19.65, 0)
(19.725, 0)
(19.8, 0)
(19.875, 0)
(19.95, 0)
(20.025, 0)
(20.1, 0)
(20.175, 0)
(20.25, 0)
(20.325, 0)
(20.4, 0)
(20.475, 0)
(20.55, 0)
(20.625, 0)
(20.7, 0)
(20.775, 0)
(20.85, 0)
(20.925, 0)
(21, 0)
(21.075, 0)
(21.15, 0)
(21.225, 0)
(21.3, 0)
(21.375, 0)
(21.45, 0)
(21.525, 0)
(21.6, 0)
(21.675, 0)
(21.75, 0)
(21.825, 0)
(21.9, 0)
(21.975, 0)
(22.05, 0)
(22.125, 0)
(22.2, 0)
(22.275, 0)
(22.35, 0)
(22.425, 0)
(22.5, 0)
(22.575, 0)
(22.65, 0)
(22.725, 0)
(22.8, 0)
(22.875, 0)
(22.95, 0)
(23.025, 0)
(23.1, 0)
(23.175, 0)
(23.25, 0)
(23.325, 0)
(23.4, 0)
(23.475, 0)
(23.55, 0)
(23.625, 0)
(23.7, 0)
(23.775, 0)
(23.85, 0)
(23.925, 0)
(24, 0)
(24.075, 0)
(24.15, 0)
(24.225, 0)
(24.3, 0)
(24.375, 0)
(24.45, 0)
(24.525, 0)
(24.6, 0)
(24.675, 0)
(24.75, 0)
(24.825, 0)
(24.9, 0)
(24.975, 0)
(25.05, 0)
(25.125, 0)
(25.2, 0)
(25.275, 0)
(25.35, 0)
(25.425, 0)
(25.5, 0)
(25.575, 0)
(25.65, 0)
(25.725, 0)
(25.8, 0)
(25.875, 0)
(25.95, 0)
(26.025, 0)
(26.1, 0)
(26.175, 0)
(26.25, 0)
(26.325, 0)
(26.4, 0)
(26.475, 0)
(26.55, 0)
(26.625, 0)
(26.7, 0)
(26.775, 0)
(26.85, 0)
(26.925, 0)
(27, 0)
(27.075, 0)
(27.15, 0)
(27.225, 0)
(27.3, 0)
(27.375, 0)
(27.45, 0)
(27.525, 0)
(27.6, 0)
(27.675, 0)
(27.75, 0)
(27.825, 0)
(27.9, 0)
(27.975, 0)
(28.05, 0)
(28.125, 0)
(28.2, 0)
(28.275, 0)
(28.35, 0)
(28.425, 0)
(28.5, 0)
(28.575, 0)
(28.65, 0)
(28.725, 0)
(28.8, 0)
(28.875, 0)
(28.95, 0)
(29.025, 0)
(29.1, 0)
(29.175, 0)
(29.25, 0)
(29.325, 0)
(29.4, 0)
(29.475, 0)
(29.55, 0)
(29.625, 0)
(29.7, 0)
(29.775, 0)
(29.85, 0)
(29.925, 0)
(30, 0)
(30.075, 0)
(30.15, 0)
(30.225, 0)
(30.3, 0)
(30.375, 0)
(30.45, 0)
(30.525, 0)
(30.6, 0)
(30.675, 0)
(30.75, 0)
(30.825, 0)
(30.9, 0)
(30.975, 0)
(31.05, 0)
(31.125, 0)
(31.2, 0)
(31.275, 0)
(31.35, 0)
(31.425, 0)
(31.5, 0)
(31.575, 0)
(31.65, 0)
(31.725, 0)
(31.8, 0)
(31.875, 0)
(31.95, 0)
(32.025, 0)
(32.1, 0)
(32.175, 0)
(32.25, 0)
};

==> exp_plots/open_ws/z.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0)
(0.075, -0.000272623)
(0.15, -0.000193634)
(0.225, -0.000239496)
(0.3, -0.000243331)
(0.375, -0.000251413)
(0.45, -0.00029784)
(0.525, -0.00028403)
(0.6, -0.000185342)
(0.675, -0.000181609)
(0.75, -0.000170196)
(0.825, -0.000264804)
(0.9, -0.000333505)
(0.975, -0.000394285)
(1.05, -0.000205456)
(1.125, -0.000101696)
(1.2, -0.000121792)
(1.275, -7.78004e-05)
(1.35, -0.000417838)
(1.425, -0.000910992)
(1.5, -0.000296646)
(1.575, -0.000917724)
(1.65, -0.000339967)
(1.725, -0.000671945)
(1.8, -4.60972e-05)
(1.875, 0.000983511)
(1.95, 0.000950679)
(2.025, 0.00130747)
(2.1, 0.00166114)
(2.175, 0.00205566)
(2.25, 0.00230609)
(2.325, 0.00214219)
(2.4, 0.00505518)
(2.475, 0.00869135)
(2.55, 0.0103196)
(2.625, 0.00748645)
(2.7, 0.00785034)
(2.775, 0.00729156)
(2.85, 0.0137537)
(2.925, 0.0191972)
(3, 0.022609)
(3.075, 0.0305502)
(3.15, 0.0284312)
(3.225, 0.0417275)
(3.3, 0.0596068)
(3.375, 0.0794128)
(3.45, 0.0926263)
(3.525, 0.106846)
(3.6, 0.119162)
(3.675, 0.117385)
(3.75, 0.156433)
(3.825, 0.175294)
(3.9, 0.195017)
(3.975, 0.207006)
(4.05, 0.223141)
(4.125, 0.238364)
(4.2, 0.255005)
(4.275, 0.266627)
(4.35, 0.275521)
(4.425, 0.280827)
(4.5, 0.281783)
(4.575, 0.286562)
(4.65, 0.292625)
(4.725, 0.297786)
(4.8, 0.30177)
(4.875, 0.308517)
(4.95, 0.323417)
(5.025, 0.335169)
(5.1, 0.343807)
(5.175, 0.358011)
(5.25, 0.372732)
(5.325, 0.384531)
(5.4, 0.3955)
(5.475, 0.4054)
(5.55, 0.416091)
(5.625, 0.421396)
(5.7, 0.425262)
(5.775, 0.429482)
(5.85, 0.434393)
(5.925, 0.445426)
(6, 0.449596)
(6.075, 0.460192)
(6.15, 0.466781)
(6.225, 0.479987)
(6.3, 0.483635)
(6.375, 0.485499)
(6.45, 0.501516)
(6.525, 0.508389)
(6.6, 0.511094)
(6.675, 0.512316)
(6.75, 0.512641)
(6.825, 0.512786)
(6.9, 0.50991)
(6.975, 0.504696)
(7.05, 0.503543)
(7.125, 0.505836)
(7.2, 0.515814)
(7.275, 0.528041)
(7.35, 0.535073)
(7.425, 0.540595)
(7.5, 0.543067)
(7.575, 0.538115)
(7.65, 0.538352)
(7.725, 0.538158)
(7.8, 0.537031)
(7.875, 0.538559)
(7.95, 0.537724)
(8.025, 0.534003)
(8.1, 0.522977)
(8.175, 0.511793)
(8.25, 0.503567)
(8.325, 0.497885)
(8.4, 0.481867)
(8.475, 0.477572)
(8.55, 0.475808)
(8.625, 0.478144)
(8.7, 0.478882)
(8.775, 0.479555)
(8.85, 0.479776)
(8.925, 0.485783)
(9, 0.493724)
(9.075, 0.496635)
(9.15, 0.502319)
(9.225, 0.51031)
(9.3, 0.511693)
(9.375, 0.513043)
(9.45, 0.520573)
(9.525, 0.523646)
(9.6, 0.528657)
(9.675, 0.531932)
(9.75, 0.530264)
(9.825, 0.529922)
(9.9, 0.522877)
(9.975, 0.522457)
(10.05, 0.520224)
(10.125, 0.518323)
(10.2, 0.512762)
(10.275, 0.505531)
(10.35, 0.502992)
(10.425, 0.498491)
(10.5, 0.50201)
(10.575, 0.504448)
(10.65, 0.503526)
(10.725, 0.499149)
(10.8, 0.496549)
(10.875, 0.499068)
(10.95, 0.493177)
(11.025, 0.496893)
(11.1, 0.506858)
(11.175, 0.5043)
(11.25, 0.502222)
(11.325, 0.504024)
(11.4, 0.49534)
(11.475, 0.492925)
(11.55, 0.492499)
(11.625, 0.491562)
(11.7, 0.492563)
(11.775, 0.493685)
(11.85, 0.493254)
(11.925, 0.489333)
(12, 0.481365)
(12.075, 0.476379)
(12.15, 0.479538)
(12.225, 0.485103)
(12.3, 0.488626)
(12.375, 0.488645)
(12.45, 0.490105)
(12.525, 0.489852)
(12.6, 0.487364)
(12.675, 0.486745)
(12.75, 0.488174)
(12.825, 0.483866)
(12.9, 0.48196)
(12.975, 0.483016)
(13.05, 0.481325)
(13.125, 0.482503)
(13.2, 0.476821)
(13.275, 0.473329)
(13.35, 0.475719)
(13.425, 0.480275)
(13.5, 0.488898)
(13.575, 0.49521)
(13.65, 0.502144)
(13.725, 0.507965)
(13.8, 0.515198)
(13.875, 0.528093)
(13.95, 0.531958)
(14.025, 0.535157)
(14.1, 0.534597)
(14.175, 0.534082)
(14.25, 0.53162)
(14.325, 0.527759)
(14.4, 0.524011)
(14.475, 0.52612)
(14.55, 0.526836)
(14.625, 0.533778)
(14.7, 0.532693)
(14.775, 0.531349)
(14.85, 0.527804)
(14.925, 0.521487)
(15, 0.516228)
(15.075, 0.515215)
(15.15, 0.516095)
(15.225, 0.516445)
(15.3, 0.515924)
(15.375, 0.49962)
(15.45, 0.494964)
(15.525, 0.493718)
(15.6, 0.496641)
(15.675, 0.49567)
(15.75, 0.50219)
(15.825, 0.500361)
(15.9, 0.503147)
(15.975, 0.505246)
(16.05, 0.502157)
(16.125, 0.498841)
(16.2, 0.496323)
(16.275, 0.495896)
(16.35, 0.49337)
(16.425, 0.496194)
(16.5, 0.498968)
(16.575, 0.494761)
(16.65, 0.485375)
(16.725, 0.486016)
(16.8, 0.4851)
(16.875, 0.485229)
(16.95, 0.479711)
(17.025, 0.47384)
(17.1, 0.468904)
(17.175, 0.4663)
(17.25, 0.45368)
(17.325, 0.448773)
(17.4, 0.448223)
(17.475, 0.442852)
(17.55, 0.445029)
(17.625, 0.441252)
(17.7, 0.429637)
(17.775, 0.426487)
(17.85, 0.423552)
(17.925, 0.41902)
(18, 0.415332)
(18.075, 0.414242)
(18.15, 0.401419)
(18.225, 0.38923)
(18.3, 0.381239)
(18.375, 0.379308)
(18.45, 0.374189)
(18.525, 0.365821)
(18.6, 0.362279)
(18.675, 0.369233)
(18.75, 0.37171)
(18.825, 0.363817)
(18.9, 0.36199)
(18.975, 0.355052)
(19.05, 0.349236)
(19.125, 0.335879)
(19.2, 0.316787)
(19.275, 0.304825)
(19.35, 0.296462)
(19.425, 0.2929)
(19.5, 0.286696)
(19.575, 0.281634)
(19.65, 0.268323)
(19.725, 0.271049)
(19.8, 0.269156)
(19.875, 0.264323)
(19.95, 0.26157)
(20.025, 0.235548)
(20.1, 0.227452)
(20.175, 0.207775)
(20.25, 0.198266)
(20.325, 0.189475)
(20.4, 0.187299)
(20.475, 0.18291)
(20.55, 0.185999)
(20.625, 0.188536)
(20.7, 0.188274)
(20.775, 0.182712)
(20.85, 0.181007)
(20.925, 0.182917)
(21, 0.184711)
(21.075, 0.181877)
(21.15, 0.179323)
(21.225, 0.176897)
(21.3, 0.173931)
(21.375, 0.167793)
(21.45, 0.165354)
(21.525, 0.1632)
(21.6, 0.160421)
(21.675, 0.144347)
(21.75, 0.135824)
(21.825, 0.126436)
(21.9, 0.122485)
(21.975, 0.118399)
(22.05, 0.118945)
(22.125, 0.120428)
(22.2, 0.118725)
(22.275, 0.116791)
(22.35, 0.116488)
(22.425, 0.115252)
(22.5, 0.11109)
(22.575, 0.108967)
(22.65, 0.105157)
(22.725, 0.0991396)
(22.8, 0.0951328)
(22.875, 0.091869)
(22.95, 0.0873765)
(23.025, 0.080199)
(23.1, 0.0660819)
(23.175, 0.0587564)
(23.25, 0.0567094)
(23.325, 0.051879)
(23.4, 0.0438298)
(23.475, 0.0434305)
(23.55, 0.0399723)
(23.625, 0.0395184)
(23.7, 0.0394639)
(23.775, 0.0350983)
(23.85, 0.0327506)
(23.925, 0.0262697)
(24, 0.0229258)
(24.075, 0.0245054)
(24.15, 0.0211266)
(24.225, 0.0220822)
(24.3, 0.0192952)
(24.375, 0.0174197)
(24.45, 0.0163939)
(24.525, 0.0162303)
(24.6, 0.0153009)
(24.675, 0.0151916)
(24.75, 0.0170756)
(24.825, 0.01527)
(24.9, 0.0140184)
(24.975, 0.0135334)
(25.05, 0.0114427)
(25.125, 0.0088583)
(25.2, 0.00790091)
(25.275, 0.00642716)
(25.35, 0.00474068)
(25.425, 0.0044329)
(25.5, 0.00493217)
(25.575, 0.00527473)
(25.65, 0.00564002)
(25.725, 0.00577953)
(25.8, 0.00557887)
(25.875, 0.0056893)
(25.95, 0.00552)
(26.025, 0.00567498)
(26.1, 0.00569595)
(26.175, 0.00549715)
(26.25, 0.00546813)
(26.325, 0.00570235)
(26.4, 0.00633174)
(26.475, 0.00664724)
(26.55, 0.0065893)
(26.625, 0.00630433)
(26.7, 0.00636678)
(26.775, 0.00640979)
(26.85, 0.00632047)
(26.925, 0.00617701)
(27, 0.00625239)
(27.075, 0.00636026)
(27.15, 0.00608156)
(27.225, 0.00605849)
(27.3, 0.00614397)
(27.375, 0.00622476)
(27.45, 0.00619431)
(27.525, 0.00621996)
(27.6, 0.00621384)
(27.675, 0.00656032)
(27.75, 0.00666776)
(27.825, 0.00663158)
(27.9, 0.00658258)
(27.975, 0.00656342)
(28.05, 0.00655493)
(28.125, 0.00638118)
(28.2, 0.00640448)
(28.275, 0.00605522)
(28.35, 0.00601729)
(28.425, 0.00593751)
(28.5, 0.00575719)
(28.575, 0.00585075)
(28.65, 0.00583107)
(28.725, 0.00595328)
(28.8, 0.00601168)
(28.875, 0.00616897)
(28.95, 0.0061128)
(29.025, 0.00610148)
(29.1, 0.00607253)
(29.175, 0.00607176)
(29.25, 0.00609501)
(29.325, 0.00596463)
(29.4, 0.00542322)
(29.475, 0.00507799)
(29.55, 0.00494702)
(29.625, 0.00426548)
(29.7, 0.00325878)
(29.775, 0.00353064)
(29.85, 0.00270316)
(29.925, 0.00259247)
(30, 0.00254503)
(30.075, 0.00233233)
(30.15, 0.00212346)
(30.225, 0.00339011)
(30.3, 0.00377121)
(30.375, 0.00409482)
(30.45, 0.00421516)
(30.525, 0.00397525)
(30.6, 0.00366513)
(30.675, 0.0030183)
(30.75, 0.0026584)
(30.825, 0.00248695)
(30.9, 0.00231129)
(30.975, 0.00213501)
(31.05, 0.00229047)
(31.125, 0.00204577)
(31.2, 0.00245138)
(31.275, 0.00211042)
(31.35, 0.000387986)
(31.425, -0.000627064)
(31.5, -0.000519963)
(31.575, -0.000409709)
(31.65, -0.00221209)
(31.725, -0.00282159)
(31.8, -0.00266276)
(31.875, -0.0015612)
(31.95, 0.000180104)
(32.025, 0.00246244)
(32.1, 0.00291653)
(32.175, 0.00304532)
(32.25, 0.00267613)
};

==> exp_plots/open_ws/z_des.tex <==
\addplot[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates {
(0, 0)
(0.075, 0)
(0.15, 0)
(0.225, 0)
(0.3, 0)
(0.375, 0)
(0.45, 0)
(0.525, 0)
(0.6, 0)
(0.675, 0)
(0.75, 0)
(0.825, 0)
(0.9, 0)
(0.975, 0)
(1.05, 0)
(1.125, 0)
(1.2, 0)
(1.275, 0)
(1.35, 0)
(1.425, 0)
(1.5, 0)
(1.575, 0)
(1.65, 0)
(1.725, 0)
(1.8, 0)
(1.875, 0)
(1.95, 0)
(2.025, 0)
(2.1, 0)
(2.175, 0)
(2.25, 0)
(2.325, 0)
(2.4, 0)
(2.475, 0)
(2.55, 0)
(2.625, 0)
(2.7, 0)
(2.775, 0)
(2.85, 0)
(2.925, 0)
(3, 0)
(3.075, 0)
(3.15, 0)
(3.225, 0)
(3.3, 0)
(3.375, 0)
(3.45, 0)
(3.525, 0)
(3.6, 0)
(3.675, 0)
(3.75, 0)
(3.825, 0)
(3.9, 0)
(3.975, 0)
(4.05, 0)
(4.125, 0)
(4.2, 0)
(4.275, 0)
(4.35, 0)
(4.425, 0)
(4.5, 0)
(4.575, 0)
(4.65, 0)
(4.725, 0)
(4.8, 0)
(4.875, 0)
(4.95, 0)
(5.025, 0)
(5.1, 0)
(5.175, 0)
(5.25, 0)
(5.325, 0)
(5.4, 0)
(5.475, 0)
(5.55, 0)
(5.625, 0)
(5.7, 0)
(5.775, 0)
(5.85, 0)
(5.925, 0)
(6, 0)
(6.075, 0)
(6.15, 0.5)
(6.225, 0.5)
(6.3, 0.5)
(6.375, 0.5)
(6.45, 0.5)
(6.525, 0.5)
(6.6, 0.5)
(6.675, 0.5)
(6.75, 0.5)
(6.825, 0.5)
(6.9, 0.5)
(6.975, 0.5)
(7.05, 0.5)
(7.125, 0.5)
(7.2, 0.5)
(7.275, 0.5)
(7.35, 0.5)
(7.425, 0.5)
(7.5, 0.5)
(7.575, 0.5)
(7.65, 0.5)
(7.725, 0.5)
(7.8, 0.5)
(7.875, 0.5)
(7.95, 0.5)
(8.025, 0.5)
(8.1, 0.5)
(8.175, 0.5)
(8.25, 0.5)
(8.325, 0.5)
(8.4, 0.5)
(8.475, 0.5)
(8.55, 0.5)
(8.625, 0.5)
(8.7, 0.5)
(8.775, 0.5)
(8.85, 0.5)
(8.925, 0.5)
(9, 0.5)
(9.075, 0.5)
(9.15, 0.5)
(9.225, 0.5)
(9.3, 0.5)
(9.375, 0.5)
(9.45, 0.5)
(9.525, 0.5)
(9.6, 0.5)
(9.675, 0.5)
(9.75, 0.5)
(9.825, 0.5)
(9.9, 0.5)
(9.975, 0.5)
(10.05, 0.5)
(10.125, 0.5)
(10.2, 0.5)
(10.275, 0.5)
(10.35, 0.5)
(10.425, 0.5)
(10.5, 0.5)
(10.575, 0.5)
(10.65, 0.5)
(10.725, 0.5)
(10.8, 0.5)
(10.875, 0.5)
(10.95, 0.5)
(11.025, 0.5)
(11.1, 0.5)
(11.175, 0.5)
(11.25, 0.5)
(11.325, 0.5)
(11.4, 0.5)
(11.475, 0.5)
(11.55, 0.5)
(11.625, 0.5)
(11.7, 0.5)
(11.775, 0.5)
(11.85, 0.5)
(11.925, 0.5)
(12, 0.5)
(12.075, 0.5)
(12.15, 0.5)
(12.225, 0.5)
(12.3, 0.5)
(12.375, 0.5)
(12.45, 0.5)
(12.525, 0.5)
(12.6, 0.5)
(12.675, 0.5)
(12.75, 0.5)
(12.825, 0.5)
(12.9, 0.5)
(12.975, 0.5)
(13.05, 0.5)
(13.125, 0.5)
(13.2, 0.5)
(13.275, 0.5)
(13.35, 0.5)
(13.425, 0.5)
(13.5, 0.5)
(13.575, 0.5)
(13.65, 0.5)
(13.725, 0.5)
(13.8, 0.5)
(13.875, 0.5)
(13.95, 0.5)
(14.025, 0.5)
(14.1, 0.5)
(14.175, 0.5)
(14.25, 0.5)
(14.325, 0.5)
(14.4, 0.5)
(14.475, 0.5)
(14.55, 0.5)
(14.625, 0.5)
(14.7, 0.5)
(14.775, 0.5)
(14.85, 0.5)
(14.925, 0.5)
(15, 0.5)
(15.075, 0.5)
(15.15, 0.5)
(15.225, 0.5)
(15.3, 0.5)
(15.375, 0.5)
(15.45, 0.5)
(15.525, 0.5)
(15.6, 0.5)
(15.675, 0.5)
(15.75, 0.5)
(15.825, 0.5)
(15.9, 0.5)
(15.975, 0)
(16.05, 0)
(16.125, 0)
(16.2, 0)
(16.275, 0)
(16.35, 0)
(16.425, 0)
(16.5, 0)
(16.575, 0)
(16.65, 0)
(16.725, 0)
(16.8, 0)
(16.875, 0)
(16.95, 0)
(17.025, 0)
(17.1, 0)
(17.175, 0)
(17.25, 0)
(17.325, 0)
(17.4, 0)
(17.475, 0)
(17.55, 0)
(17.625, 0)
(17.7, 0)
(17.775, 0)
(17.85, 0)
(17.925, 0)
(18, 0)
(18.075, 0)
(18.15, 0)
(18.225, 0)
(18.3, 0)
(18.375, 0)
(18.45, 0)
(18.525, 0)
(18.6, 0)
(18.675, 0)
(18.75, 0)
(18.825, 0)
(18.9, 0)
(18.975, 0)
(19.05, 0)
(19.125, 0)
(19.2, 0)
(19.275, 0)
(19.35, 0)
(19.425, 0)
(19.5, 0)
(19.575, 0)
(19.65, 0)
(19.725, 0)
(19.8, 0)
(19.875, 0)
(19.95, 0)
(20.025, 0)
(20.1, 0)
(20.175, 0)
(20.25, 0)
(20.325, 0)
(20.4, 0)
(20.475, 0)
(20.55, 0)
(20.625, 0)
(20.7, 0)
(20.775, 0)
(20.85, 0)
(20.925, 0)
(21, 0)
(21.075, 0)
(21.15, 0)
(21.225, 0)
(21.3, 0)
(21.375, 0)
(21.45, 0)
(21.525, 0)
(21.6, 0)
(21.675, 0)
(21.75, 0)
(21.825, 0)
(21.9, 0)
(21.975, 0)
(22.05, 0)
(22.125, 0)
(22.2, 0)
(22.275, 0)
(22.35, 0)
(22.425, 0)
(22.5, 0)
(22.575, 0)
(22.65, 0)
(22.725, 0)
(22.8, 0)
(22.875, 0)
(22.95, 0)
(23.025, 0)
(23.1, 0)
(23.175, 0)
(23.25, 0)
(23.325, 0)
(23.4, 0)
(23.475, 0)
(23.55, 0)
(23.625, 0)
(23.7, 0)
(23.775, 0)
(23.85, 0)
(23.925, 0)
(24, 0)
(24.075, 0)
(24.15, 0)
(24.225, 0)
(24.3, 0)
(24.375, 0)
(24.45, 0)
(24.525, 0)
(24.6, 0)
(24.675, 0)
(24.75, 0)
(24.825, 0)
(24.9, 0)
(24.975, 0)
(25.05, 0)
(25.125, 0)
(25.2, 0)
(25.275, 0)
(25.35, 0)
(25.425, 0)
(25.5, 0)
(25.575, 0)
(25.65, 0)
(25.725, 0)
(25.8, 0)
(25.875, 0)
(25.95, 0)
(26.025, 0)
(26.1, 0)
(26.175, 0)
(26.25, 0)
(26.325, 0)
(26.4, 0)
(26.475, 0)
(26.55, 0)
(26.625, 0)
(26.7, 0)
(26.775, 0)
(26.85, 0)
(26.925, 0)
(27, 0)
(27.075, 0)
(27.15, 0)
(27.225, 0)
(27.3, 0)
(27.375, 0)
(27.45, 0)
(27.525, 0)
(27.6, 0)
(27.675, 0)
(27.75, 0)
(27.825, 0)
(27.9, 0)
(27.975, 0)
(28.05, 0)
(28.125, 0)
(28.2, 0)
(28.275, 0)
(28.35, 0)
(28.425, 0)
(28.5, 0)
(28.575, 0)
(28.65, 0)
(28.725, 0)
(28.8, 0)
(28.875, 0)
(28.95, 0)
(29.025, 0)
(29.1, 0)
(29.175, 0)
(29.25, 0)
(29.325, 0)
(29.4, 0)
(29.475, 0)
(29.55, 0)
(29.625, 0)
(29.7, 0)
(29.775, 0)
(29.85, 0)
(29.925, 0)
(30, 0)
(30.075, 0)
(30.15, 0)
(30.225, 0)
(30.3, 0)
(30.375, 0)
(30.45, 0)
(30.525, 0)
(30.6, 0)
(30.675, 0)
(30.75, 0)
(30.825, 0)
(30.9, 0)
(30.975, 0)
(31.05, 0)
(31.125, 0)
(31.2, 0)
(31.275, 0)
(31.35, 0)
(31.425, 0)
(31.5, 0)
(31.575, 0)
(31.65, 0)
(31.725, 0)
(31.8, 0)
(31.875, 0)
(31.95, 0)
(32.025, 0)
(32.1, 0)
(32.175, 0)
(32.25, 0)
};

==> exp_plots/open_ws_gripper/az.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0)
(0.075, 0.015476)
(0.15, 0.0272082)
(0.225, 0.0366179)
(0.3, 0.0482529)
(0.375, 0.0338257)
(0.45, 0.0227764)
(0.525, 0.010967)
(0.6, 0.00116339)
(0.675, -0.000847049)
(0.75, -0.00240812)
(0.825, 0.013521)
(0.9, 0.0167115)
(0.975, 0.00385037)
(1.05, -0.00540122)
(1.125, -0.00999473)
(1.2, -0.0180826)
(1.275, -0.0125605)
(1.35, -0.00835811)
(1.425, 0.00324954)
(1.5, 0.0132035)
(1.575, 0.0342669)
(1.65, 0.0482897)
(1.725, 0.0331413)
(1.8, 0.021464)
(1.875, 0.0267617)
(1.95, 0.0111119)
(2.025, 0.00797589)
(2.1, 0.00623048)
(2.175, -0.0263943)
(2.25, -0.0188877)
(2.325, -0.0185171)
(2.4, -0.0222162)
(2.475, -0.0382636)
(2.55, -0.0445121)
(2.625, -0.0437645)
(2.7, -0.0262791)
(2.775, 0.0493977)
(2.85, 0.208437)
(2.925, 0.421136)
(3, 0.556316)
(3.075, 0.50679)
(3.15, 0.325347)
(3.225, 0.12049)
(3.3, -0.0562816)
(3.375, -0.204205)
(3.45, -0.230822)
(3.525, -0.160578)
(3.6, -0.0884387)
(3.675, 0.00503027)
(3.75, 0.092977)
(3.825, 0.12832)
(3.9, 0.116162)
(3.975, 0.0758661)
(4.05, 0.0114608)
(4.125, -0.0570757)
(4.2, -0.0873225)
(4.275, -0.0957689)
(4.35, -0.0765672)
(4.425, 0.0226839)
(4.5, 0.172176)
(4.575, 0.305612)
(4.65, 0.311146)
(4.725, 0.167463)
(4.8, -0.0395241)
(4.875, -0.190122)
(4.95, -0.173415)
(5.025, 0.00294664)
(5.1, 0.1801)
(5.175, 0.304066)
(5.25, 0.290621)
(5.325, 0.146376)
(5.4, 0.00542149)
(5.475, -0.0578976)
(5.55, -0.0160893)
(5.625, 0.1273)
(5.7, 0.17749)
(5.775, 0.0859272)
(5.85, -0.0613487)
(5.925, -0.200594)
(6, -0.264805)
(6.075, -0.16059)
(6.15, 0.0176488)
(6.225, 0.172094)
(6.3, 0.211338)
(6.375, 0.175011)
(6.45, 0.0562176)
(6.525, -0.0481393)
(6.6, -0.0856537)
(6.675, -0.11345)
(6.75, -0.0951621)
(6.825, -0.00964122)
(6.9, 0.105317)
(6.975, 0.227278)
(7.05, 0.256644)
(7.125, 0.187391)
(7.2, 0.0981604)
(7.275, 0.0193419)
(7.35, 0.0129693)
(7.425, 0.0754822)
(7.5, 0.127642)
(7.575, 0.0983991)
(7.65, 0.0323806)
(7.725, -0.0176406)
(7.8, -0.0261747)
(7.875, -0.028434)
(7.95, -0.035325)
(8.025, -0.156972)
(8.1, -0.310365)
(8.175, -0.392502)
(8.25, -0.338314)
(8.325, -0.210624)
(8.4, -0.0471014)
(8.475, 0.12939)
(8.55, 0.240411)
(8.625, 0.2221)
(8.7, 0.0713513)
(8.775, -0.083448)
(8.85, -0.168484)
(8.925, -0.153164)
(9, -0.0548763)
(9.075, 0.0284687)
(9.15, 0.0307235)
(9.225, -0.00614062)
(9.3, -0.060244)
(9.375, -0.0828829)
(9.45, -0.0664747)
(9.525, -0.0359215)
(9.6, 0.0117586)
(9.675, 0.0383052)
(9.75, 0.0569456)
(9.825, 0.0647983)
(9.9, 0.0227365)
(9.975, -0.00261686)
(10.05, -0.00925622)
(10.125, 0.00448846)
(10.2, -0.00890725)
(10.275, -0.0141716)
(10.35, -0.0273572)
(10.425, -0.0106416)
(10.5, 0.041816)
(10.575, 0.062627)
(10.65, 0.0501465)
(10.725, -0.0144384)
(10.8, -0.0985677)
(10.875, -0.145011)
(10.95, -0.104542)
(11.025, -0.00511846)
(11.1, 0.082943)
(11.175, 0.171052)
(11.25, 0.232144)
(11.325, 0.233679)
(11.4, 0.178334)
(11.475, 0.107914)
(11.55, 0.0354653)
(11.625, -0.0802843)
(11.7, -0.200265)
(11.775, -0.22477)
(11.85, -0.166969)
(11.925, -0.0446733)
(12, 0.0196439)
(12.075, 0.0217511)
(12.15, -0.00875256)
(12.225, 0.0430668)
(12.3, 0.0875833)
(12.375, 0.0783651)
(12.45, 0.0340896)
(12.525, -0.0248089)
(12.6, -0.0667014)
(12.675, -0.0675843)
(12.75, -0.0443978)
(12.825, 0.020633)
(12.9, 0.0756256)
(12.975, 0.12282)
(13.05, 0.0905664)
(13.125, -0.0267498)
(13.2, -0.154646)
(13.275, -0.217942)
(13.35, -0.194612)
(13.425, -0.127649)
(13.5, -0.115797)
(13.575, -0.123722)
(13.65, -0.0963574)
(13.725, -0.0176362)
(13.8, 0.0821228)
(13.875, 0.192477)
(13.95, 0.214027)
(14.025, 0.136002)
(14.1, -0.0233797)
(14.175, -0.149514)
(14.25, -0.199848)
(14.325, -0.173827)
(14.4, -0.0850625)
(14.475, -0.026101)
(14.55, 0.00295212)
(14.625, -0.0143954)
(14.7, -0.0453555)
(14.775, -0.0944915)
(14.85, -0.137831)
(14.925, -0.183681)
(15, -0.16576)
(15.075, -0.0724827)
(15.15, 0.0459102)
(15.225, 0.12748)
(15.3, 0.163094)
(15.375, 0.140378)
(15.45, 0.100821)
(15.525, 0.0541838)
(15.6, 0.0203624)
(15.675, -0.0215931)
(15.75, -0.0626426)
(15.825, -0.111585)
(15.9, -0.0855779)
(15.975, 0.0134125)
(16.05, 0.132462)
(16.125, 0.208186)
(16.2, 0.197442)
(16.275, 0.125527)
(16.35, -0.0102485)
(16.425, -0.14623)
(16.5, -0.210111)
(16.575, -0.204798)
(16.65, -0.139729)
(16.725, -0.0837574)
(16.8, -0.0817005)
(16.875, -0.0831)
(16.95, -0.0606771)
(17.025, -0.0332869)
(17.1, 0.0174159)
(17.175, 0.0752773)
(17.25, 0.0519909)
(17.325, -0.00879176)
(17.4, -0.0604485)
(17.475, -0.05944)
(17.55, -0.0732707)
(17.625, -0.0807952)
(17.7, -0.0252525)
(17.775, 0.0714792)
(17.85, 0.156097)
(17.925, 0.163034)
(18, 0.0689307)
(18.075, -0.0683785)
(18.15, -0.170645)
(18.225, -0.201479)
(18.3, -0.192903)
(18.375, -0.168063)
(18.45, -0.13519)
(18.525, -0.0849323)
(18.6, -0.0275234)
(18.675, -0.00313632)
(18.75, -0.0287916)
(18.825, -0.00840956)
(18.9, 0.0917334)
(18.975, 0.211682)
(19.05, 0.248464)
(19.125, 0.204905)
(19.2, 0.0989068)
(19.275, 0.00837249)
(19.35, -0.0342699)
(19.425, -0.0195636)
(19.5, 0.0293592)
(19.575, 0.0730922)
(19.65, 0.0552504)
(19.725, -0.0420194)
(19.8, -0.135332)
(19.875, -0.14446)
(19.95, -0.0757634)
(20.025, -0.00732609)
(20.1, 0.0159602)
(20.175, 0.0159673)
(20.25, -0.00750569)
(20.325, -0.0108747)
(20.4, 0.0544383)
(20.475, 0.146454)
(20.55, 0.199104)
(20.625, 0.184002)
(20.7, 0.137829)
(20.775, 0.0356744)
(20.85, -0.111114)
(20.925, -0.189913)
(21, -0.181198)
(21.075, -0.106276)
(21.15, 0.0307952)
(21.225, 0.13336)
(21.3, 0.143087)
(21.375, 0.059439)
(21.45, -0.0471613)
(21.525, -0.0788815)
(21.6, -0.033709)
(21.675, 0.0245675)
(21.75, 0.0534207)
(21.825, 0.0319236)
(21.9, 0.00844)
(21.975, 0.00748531)
(22.05, -0.00995547)
(22.125, -0.0224019)
(22.2, -0.0426414)
(22.275, -0.0390545)
(22.35, -0.0424921)
(22.425, -0.0411325)
(22.5, -0.0297728)
(22.575, -0.000937121)
(22.65, 0.0348932)
(22.725, 0.0691487)
(22.8, 0.101751)
(22.875, 0.107668)
(22.95, 0.0605805)
(23.025, -0.00953691)
(23.1, -0.0333759)
(23.175, -0.0290531)
(23.25, -0.0347729)
(23.325, -0.0362804)
(23.4, -0.0341708)
(23.475, -0.0843237)
(23.55, -0.15016)
(23.625, -0.181438)
(23.7, -0.171836)
(23.775, -0.0161711)
(23.85, 0.160916)
(23.925, 0.216732)
(24, 0.117941)
(24.075, -0.0050446)
(24.15, -0.133766)
(24.225, -0.13763)
(24.3, -0.0536858)
(24.375, 0.0078625)
(24.45, 0.0580368)
(24.525, 0.0630428)
(24.6, 0.0207318)
(24.675, -0.0118384)
(24.75, -0.065947)
(24.825, -0.154796)
(24.9, -0.231178)
(24.975, -0.181849)
(25.05, -0.0924419)
(25.125, 0.000284258)
(25.2, 0.0526238)
(25.275, 0.04858)
(25.35, 0.0332416)
(25.425, 0.0223649)
(25.5, 0.0467651)
(25.575, 0.0856669)
(25.65, 0.113304)
(25.725, 0.135274)
(25.8, 0.121968)
(25.875, 0.0206172)
(25.95, -0.0947032)
(26.025, -0.202417)
(26.1, -0.279952)
(26.175, -0.302044)
(26.25, -0.241122)
(26.325, -0.123153)
(26.4, 0.0203442)
(26.475, 0.249701)
(26.55, 0.33659)
(26.625, 0.256308)
(26.7, 0.0255492)
(26.775, -0.202407)
(26.85, -0.297296)
(26.925, -0.203324)
(27, -0.0870797)
(27.075, 0.0424375)
(27.15, 0.138594)
(27.225, 0.156539)
(27.3, 0.056861)
(27.375, -0.0352347)
(27.45, -0.104294)
(27.525, -0.125999)
(27.6, -0.0169019)
(27.675, 0.0311337)
(27.75, 0.028112)
(27.825, 0.0378512)
(27.9, 0.0196639)
(27.975, 0.00559702)
(28.05, 0.00756563)
(28.125, 0.00300042)
(28.2, 0.00934177)
(28.275, 0.00706897)
(28.35, 0.00165376)
(28.425, 0.0104217)
(28.5, 0.016246)
(28.575, 0.0251599)
(28.65, 0.0426048)
(28.725, 0.0533027)
(28.8, 0.0563249)
(28.875, 0.0495719)
(28.95, 0.0360775)
(29.025, 0.0122212)
(29.1, 0.00973468)
(29.175, 0.010774)
(29.25, 0.0265137)
(29.325, 0.040006)
(29.4, 0.0447869)
(29.475, 0.0426956)
(29.55, 0.021908)
(29.625, 0.0126841)
(29.7, 0.0105089)
(29.775, 0.0236498)
(29.85, 0.0266515)
(29.925, 0.0138432)
(30, 0.00645932)
(30.075, 0.00397287)
(30.15, 0.00480968)
(30.225, 0.00857745)
(30.3, 0.0219487)
(30.375, 0.00257568)
(30.45, 0.00983001)
(30.525, 0.00962813)
(30.6, 0.00101099)
(30.675, 0.00975356)
(30.75, 0.0169053)
(30.825, 0.0246422)
(30.9, 0.0384008)
(30.975, 0.0336652)
(31.05, 0.0190746)
(31.125, 0.016084)
(31.2, -0.0123631)
(31.275, -0.0112111)
(31.35, -0.00145584)
(31.425, 0.0077451)
(31.5, 0.00930426)
(31.575, 0.0179528)
(31.65, 0.0100856)
(31.725, 0.0377265)
(31.8, 0.0462796)
(31.875, 0.0459946)
(31.95, 0.0314336)
(32.025, -0.00176868)
(32.1, -0.0231129)
(32.175, -0.0268389)
(32.25, -0.0225846)
(32.325, -0.00751189)
(32.4, 0.00775729)
(32.475, 0.0374906)
(32.55, 0.0278165)
(32.625, 0.0151263)
(32.7, 0.00672589)
(32.775, 0.00104254)
(32.85, -0.00219939)
(32.925, 0.00476213)
(33, 0.0121441)
(33.075, 0.0277943)
(33.15, 0.0377925)
(33.225, 0.0361592)
(33.3, 0.0245129)
(33.375, 0.0194712)
(33.45, 0.0127191)
(33.525, 0.019773)
(33.6, 0.0300703)
(33.675, 0.0257292)
(33.75, 0.0040678)
(33.825, -0.0227692)
(33.9, -0.0417558)
(33.975, -0.0444275)
(34.05, -0.0335243)
(34.125, -0.0210903)
(34.2, -0.0272095)
(34.275, -0.0220437)
(34.35, -0.0114237)
(34.425, -0.00298391)
(34.5, 0.00461499)
(34.575, 0.0105313)
(34.65, 0.0129507)
};

==> exp_plots/open_ws_gripper/az_des.tex <==
\addplot[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates {
(0, 0)
(0.075, -0.00645138)
(0.15, -0.0152539)
(0.225, -0.0208424)
(0.3, -0.0236733)
(0.375, -0.0256191)
(0.45, -0.0190408)
(0.525, -0.0138296)
(0.6, -0.00925081)
(0.675, 0.000293884)
(0.75, 0.00486172)
(0.825, 0.00295449)
(0.9, -0.000315318)
(0.975, -0.00134013)
(1.05, 0.242956)
(1.125, 0.424688)
(1.2, 0.49459)
(1.275, 0.509012)
(1.35, 0.480237)
(1.425, 0.436564)
(1.5, 0.420487)
(1.575, 0.419725)
(1.65, 0.417103)
(1.725, 0.408962)
(1.8, 0.390415)
(1.875, 0.386606)
(1.95, 0.388592)
(2.025, 0.394317)
(2.1, 0.394071)
(2.175, 0.392189)
(2.25, 0.398893)
(2.325, 0.416366)
(2.4, 0.435015)
(2.475, 0.452922)
(2.55, 0.469401)
(2.625, 0.483032)
(2.7, 0.501129)
(2.775, 0.506174)
(2.85, 0.496366)
(2.925, 0.457086)
(3, 0.382965)
(3.075, 0.290485)
(3.15, 0.110882)
(3.225, -0.00595704)
(3.3, -0.0770169)
(3.375, -0.116098)
(3.45, -0.0557586)
(3.525, 0.0203162)
(3.6, 0.0628008)
(3.675, 0.0938703)
(3.75, 0.120878)
(3.825, 0.114396)
(3.9, 0.0689414)
(3.975, 0.0247926)
(4.05, -0.00663092)
(4.125, -0.0114322)
(4.2, 0.019467)
(4.275, 0.0796048)
(4.35, 0.151668)
(4.425, 0.184703)
(4.5, 0.17369)
(4.575, 0.1082)
(4.65, 0.0511021)
(4.725, 0.048228)
(4.8, 0.0564866)
(4.875, 0.0676469)
(4.95, 0.110128)
(5.025, 0.11951)
(5.1, 0.117959)
(5.175, 0.0950517)
(5.25, 0.0905154)
(5.325, 0.108895)
(5.4, 0.156486)
(5.475, 0.192674)
(5.55, 0.0408094)
(5.625, -0.0503753)
(5.7, -0.0700631)
(5.775, -0.0482951)
(5.85, 0.00303195)
(5.925, 0.0541292)
(6, 0.0878499)
(6.075, 0.0586074)
(6.15, 0.0434279)
(6.225, 0.0442468)
(6.3, 0.0416979)
(6.375, 0.0631199)
(6.45, -0.0122193)
(6.525, -0.0661469)
(6.6, -0.0494122)
(6.675, -0.0297568)
(6.75, 0.0286826)
(6.825, 0.100549)
(6.9, 0.133347)
(6.975, 0.151229)
(7.05, 0.174812)
(7.125, 0.186798)
(7.2, 0.162988)
(7.275, 0.142366)
(7.35, 0.0445838)
(7.425, -0.00767924)
(7.5, -0.0136449)
(7.575, -0.0171485)
(7.65, -0.00217444)
(7.725, -0.0146433)
(7.8, -0.045519)
(7.875, -0.171998)
(7.95, -0.169524)
(8.025, -0.128206)
(8.1, -0.0899287)
(8.175, -0.0493557)
(8.25, -0.00362373)
(8.325, 0.00614096)
(8.4, 0.0264537)
(8.475, 0.0201091)
(8.55, -0.00422958)
(8.625, -0.0445894)
(8.7, -0.0464445)
(8.775, -0.0057729)
(8.85, 0.0269739)
(8.925, 0.0419634)
(9, 0.0124647)
(9.075, -0.0529578)
(9.15, -0.103842)
(9.225, -0.114642)
(9.3, -0.083952)
(9.375, -0.0393673)
(9.45, -0.00377712)
(9.525, 0.020069)
(9.6, 0.0336717)
(9.675, 0.0207639)
(9.75, 0.0138422)
(9.825, 0.0371022)
(9.9, 0.0247401)
(9.975, 0.0111368)
(10.05, -0.00699246)
(10.125, -0.0119168)
(10.2, -0.00392529)
(10.275, 0.0121358)
(10.35, 0.004658)
(10.425, -0.000861671)
(10.5, -0.00887053)
(10.575, -0.0175951)
(10.65, -0.0280925)
(10.725, -0.0271964)
(10.8, -0.0115694)
(10.875, 0.0141694)
(10.95, 0.0519713)
(11.025, 0.114836)
(11.1, 0.151921)
(11.175, 0.125779)
(11.25, 0.0844035)
(11.325, 0.0396494)
(11.4, 0.00268201)
(11.475, -0.0466089)
(11.55, -0.0534753)
(11.625, -0.0691778)
(11.7, -0.0583747)
(11.775, -0.0234738)
(11.85, 0.00300803)
(11.925, 0.0212861)
(12, 0.00631385)
(12.075, -0.000607244)
(12.15, 0.0187021)
(12.225, 0.0255738)
(12.3, 0.00982716)
(12.375, -0.0091905)
(12.45, -0.0175948)
(12.525, -0.0450786)
(12.6, -0.01258)
(12.675, 0.0301457)
(12.75, 0.0417497)
(12.825, 0.0398423)
(12.9, 0.0063641)
(12.975, -0.0583535)
(13.05, -0.0812505)
(13.125, -0.0848328)
(13.2, -0.0936982)
(13.275, -0.130044)
(13.35, -0.131915)
(13.425, -0.103034)
(13.5, -0.0191202)
(13.575, 0.0505686)
(13.65, 0.0842882)
(13.725, 0.0981551)
(13.8, 0.0690314)
(13.875, 0.0121496)
(13.95, -0.0707886)
(14.025, -0.0823224)
(14.1, -0.0602185)
(14.175, -0.0337365)
(14.25, -0.0353444)
(14.325, -0.0335371)
(14.4, -0.0356193)
(14.475, -0.0421523)
(14.55, -0.0470466)
(14.625, -0.0650656)
(14.7, -0.0875497)
(14.775, -0.118286)
(14.85, -0.0785023)
(14.925, 0.0145317)
(15, 0.0593757)
(15.075, 0.0866444)
(15.15, 0.10351)
(15.225, 0.102499)
(15.3, 0.0807687)
(15.375, 0.0561539)
(15.45, 0.0157443)
(15.525, 0.00787867)
(15.6, 0.0207196)
(15.675, 0.0338718)
(15.75, 0.0452972)
(15.825, 0.0780145)
(15.9, 0.12488)
(15.975, 0.139205)
(16.05, 0.0748834)
(16.125, -0.0243492)
(16.2, -0.095777)
(16.275, -0.130482)
(16.35, -0.13284)
(16.425, -0.108216)
(16.5, -0.0792759)
(16.575, -0.0618681)
(16.65, -0.0494793)
(16.725, -0.0419739)
(16.8, -0.0518518)
(16.875, -0.0585959)
(16.95, -0.0605453)
(17.025, -0.0680194)
(17.1, -0.103038)
(17.175, -0.119834)
(17.25, -0.104696)
(17.325, -0.0893441)
(17.4, -0.0453191)
(17.475, 0.00643237)
(17.55, 0.0655531)
(17.625, 0.0962182)
(17.7, 0.0812283)
(17.775, 0.0294564)
(17.85, -0.0164447)
(17.925, -0.0621785)
(18, -0.117287)
(18.075, -0.138072)
(18.15, -0.144562)
(18.225, -0.152338)
(18.3, -0.141475)
(18.375, -0.126498)
(18.45, -0.11356)
(18.525, -0.0754089)
(18.6, -0.0461393)
(18.675, 0.0984327)
(18.75, 0.195171)
(18.825, 0.140563)
(18.9, 0.102783)
(18.975, 0.0665798)
(19.05, 0.00542571)
(19.125, 0.00788239)
(19.2, 0.0115151)
(19.275, 0.0154145)
(19.35, 0.018706)
(19.425, -0.00406016)
(19.5, -0.0346525)
(19.575, -0.0513139)
(19.65, -0.0581617)
(19.725, -0.0596505)
(19.8, -0.0515246)
(19.875, -0.039137)
(19.95, -0.0103081)
(20.025, 0.0253036)
(20.1, 0.059205)
(20.175, 0.104299)
(20.25, 0.104686)
(20.325, 0.0989903)
(20.4, 0.0962762)
(20.475, 0.105301)
(20.55, 0.0560595)
(20.625, -0.0187157)
(20.7, -0.068724)
(20.775, -0.102019)
(20.85, -0.0792462)
(20.925, -0.0305427)
(21, 0.016234)
(21.075, 0.0345817)
(21.15, 0.0229284)
(21.225, -0.00556039)
(21.3, -0.0280954)
(21.375, 0.00468324)
(21.45, 0.0285598)
(21.525, 0.032371)
(21.6, 0.0149994)
(21.675, 0.000449894)
(21.75, 0.00830843)
(21.825, 0.00966947)
(21.9, 0.000258388)
(21.975, 0.0158101)
(22.05, 0.0124893)
(22.125, 0.00206805)
(22.2, -0.0317622)
(22.275, -0.0550248)
(22.35, -0.0128505)
(22.425, 0.0070191)
(22.5, 0.0228417)
(22.575, 0.0325735)
(22.65, 0.0383127)
(22.725, 0.0206486)
(22.8, -0.0451115)
(22.875, -0.097865)
(22.95, -0.114469)
(23.025, -0.0963877)
(23.1, -0.0707972)
(23.175, -0.0504466)
(23.25, -0.0513024)
(23.325, -0.061621)
(23.4, -0.0520255)
(23.475, -0.0326904)
(23.55, 0.00380048)
(23.625, 0.0336067)
(23.7, 0.029596)
(23.775, -0.0139179)
(23.85, -0.0236791)
(23.925, -0.0356842)
(24, -0.0410595)
(24.075, -0.0403728)
(24.15, -0.0450645)
(24.225, -0.0514653)
(24.3, -0.060773)
(24.375, -0.0817785)
(24.45, -0.0520504)
(24.525, -0.0691634)
(24.6, -0.0967889)
(24.675, -0.11891)
(24.75, -0.120839)
(24.825, -0.110427)
(24.9, -0.084913)
(24.975, -0.0603573)
(25.05, -0.0619833)
(25.125, -0.0764225)
(25.2, -0.0849071)
(25.275, -0.046497)
(25.35, -0.0214923)
(25.425, 0.071851)
(25.5, 0.126882)
(25.575, 0.114011)
(25.65, 0.0851033)
(25.725, 0.0426426)
(25.8, -0.00913798)
(25.875, -0.0847608)
(25.95, -0.13426)
(26.025, -0.140953)
(26.1, -0.130129)
(26.175, -0.103709)
(26.25, -0.104448)
(26.325, -0.02997)
(26.4, 0.00949349)
(26.475, 0.00497355)
(26.55, -0.0477563)
(26.625, -0.0969504)
(26.7, -0.17557)
(26.775, -0.192277)
(26.85, -0.198232)
(26.925, -0.156319)
(27, -0.139168)
(27.075, -0.119476)
(27.15, -0.13182)
(27.225, -0.160091)
(27.3, -0.169932)
(27.375, -0.174768)
(27.45, -0.163498)
(27.525, -0.161057)
(27.6, -0.181793)
(27.675, -0.205951)
(27.75, -0.196366)
(27.825, -0.182538)
(27.9, -0.184547)
(27.975, -0.195866)
(28.05, -0.229644)
(28.125, -0.255755)
(28.2, -0.263566)
(28.275, -0.254842)
(28.35, -0.24495)
(28.425, -0.2424)
(28.5, -0.239128)
(28.575, -0.231237)
(28.65, -0.225164)
(28.725, -0.229161)
(28.8, -0.236168)
(28.875, -0.240086)
(28.95, -0.240409)
(29.025, -0.242548)
(29.1, -0.250081)
(29.175, -0.258283)
(29.25, -0.276572)
(29.325, -0.287696)
(29.4, -0.291292)
(29.475, -0.290838)
(29.55, -0.278491)
(29.625, -0.268234)
(29.7, -0.266155)
(29.775, -0.269876)
(29.85, -0.275322)
(29.925, -0.289661)
(30, -0.297658)
(30.075, -0.299873)
(30.15, -0.305113)
(30.225, -0.272113)
(30.3, -0.254467)
(30.375, -0.255949)
(30.45, -0.25616)
(30.525, -0.26701)
(30.6, -0.278883)
(30.675, -0.285073)
(30.75, -0.29461)
(30.825, -0.302879)
(30.9, -0.31052)
(30.975, -0.32514)
(31.05, -0.332127)
(31.125, -0.339662)
(31.2, -0.335629)
(31.275, -0.324534)
(31.35, -0.310332)
(31.425, -0.305487)
(31.5, -0.30784)
(31.575, -0.315488)
(31.65, -0.339911)
(31.725, -0.348498)
(31.8, -0.352524)
(31.875, -0.352459)
(31.95, -0.351322)
(32.025, -0.331353)
(32.1, -0.31883)
(32.175, -0.304823)
(32.25, -0.286721)
(32.325, -0.283567)
(32.4, -0.291931)
(32.475, -0.309155)
(32.55, -0.359274)
(32.625, -0.368503)
(32.7, -0.362142)
(32.775, -0.343995)
(32.85, -0.328657)
(32.925, -0.357338)
(33, -0.37618)
(33.075, -0.38201)
(33.15, -0.400431)
(33.225, -0.410916)
(33.3, -0.409892)
(33.375, -0.408389)
(33.45, -0.400912)
(33.525, -0.394497)
(33.6, -0.392702)
(33.675, -0.386824)
(33.75, -0.383571)
(33.825, -0.37769)
(33.9, -0.377796)
(33.975, -0.376671)
(34.05, -0.375393)
(34.125, -0.376325)
(34.2, -0.37754)
(34.275, -0.37964)
(34.35, -0.381549)
(34.425, -0.383872)
(34.5, -0.385836)
(34.575, -0.388174)
(34.65, -0.390753)
};

==> exp_plots/open_ws_gripper/plot.tex <==
%%    
\begin{figure}[t]
\centering

\begin{tikzpicture}


\FPeval{\xshfta}{0}
\FPeval{\xshftb}{0}
\FPeval{\xshftc}{0}
\FPeval{\xshftd}{0}



\FPeval{\yshfta}{0-0}
\FPeval{\yshftb}{0-9}
\FPeval{\yshftc}{0-18}
\FPeval{\yshftd}{0-27.9}


\FPeval{\pltw}{110}
\FPeval{\plth}{24}

\FPeval{\scal}{0.5}


\FPeval{\mrksize}{0.3}

%
\colorlet{desclr}{white!0!magenta}
\colorlet{currclr}{blue!60!green}

\colorlet{gridclr}{white!85!black}
\colorlet{dlegendclr}{white!80!black}
\colorlet{axisclr}{white!75!black}
\colorlet{axisbgclr}{white!99!black}

\colorlet{dlegendclr}{white!80!black}
\colorlet{legendclr}{white!100!black}






\FPeval{\lscale}{0.6}
\FPeval{\limscale}{0.5}
\FPeval{\lxshft}{95.5}
\FPeval{\lyshft}{9.0}

  
\FPeval{\titlescale}{0.7}
\FPeval{\titlexshift}{21.0}
\FPeval{\titleyshift}{13.7}

\colorlet{gpudclr}{white!80!black}
\colorlet{gpuclr}{white!90!black}
\colorlet{gputxtclr}{white!0!black}

\FPeval{\labelscale}{1.0}
\FPeval{\ticklabelscale}{0.9}

\FPeval{\xlabelxshift}{0+15}
\FPeval{\xlabelyshift}{0+0.5}
\FPeval{\ylabelxshift}{0+4.0}
\FPeval{\ylabelyshift}{0+6.2}


\FPeval{\linew}{1.5}
\FPeval{\dashon}{5.0}
\FPeval{\dashoff}{3.0}

\FPeval{\xshfttakeoff}{0-16}
\FPeval{\xshfthover}{0}
\FPeval{\xshftland}{16}
%
%
\node (a) [xshift = \xshfta ex, yshift=\yshfta ex, scale=\scal]{
\tikz{
%
\pgfplotsset{width=\pltw ex, height=\plth ex}
\begin{axis}[
   axis background style={fill=axisbgclr},
    title={},
    xlabel={},
    ylabel={ X (m)},
    xmin=0, xmax=30,
    ymin=-1, ymax=1,
    xtick={0, 15, 30, 45, 60},
    ytick={-1, 0, 1},
    xticklabels={$0$, $15$, $30$, $45$, $60$},
    yticklabels={$-1$, $0$, $0$},
     axis line style={axisclr},
    legend image post style={scale =\limscale},
    legend style={at={(\lxshft ex,\lyshft ex)},anchor=south, legend columns = 1, draw = {dlegendclr}, fill={legendclr}, nodes={scale=\lscale}},
    ymajorgrids=true, 
    xmajorgrids=true,
    grid style={dashed, gridclr},
    major tick length=1ex,
    x label style={at={(\xlabelxshift ex, \xlabelyshift ex)},scale=\labelscale},
    y label style={at={(\ylabelxshift ex, \ylabelyshift ex)},scale=\labelscale},
    xticklabel style={scale=\ticklabelscale},
    yticklabel style={scale=\ticklabelscale},
%    ybar,
%    bar width = 4pt,
]
%
%
\input{exp_plots/open_ws_gripper/x_des}
%
\input{exp_plots/open_ws_gripper/x}
%
%
%%   
  \legend{Ref, SLAM}
  %
\end{axis}
%
% \node [draw=gpudclr,fill=gpuclr,rounded corners=0.2ex, minimum width=10.0ex, xshift=\titlexshift ex, yshift=\titleyshift ex, scale=\titlescale]{\textcolor{gputxtclr}{\textbf{Step-X}}};
}};
%
%    
%
%
\node (b) [xshift = \xshftb ex, yshift=\yshftb ex, scale=\scal]{
\tikz{
%
\pgfplotsset{width=\pltw ex, height=\plth ex}
\begin{axis}[
   axis background style={fill=axisbgclr},
    title={},
    xlabel={},
    ylabel={ Y (m)},
    xmin=0, xmax=30,
    ymin=-1, ymax=1,
    xtick={0, 15, 30, 45, 60},
    ytick={-1, 0, 1},
    xticklabels={$0$, $15$, $30$, $45$, $60$},
    yticklabels={$-1$, $0$, $0$},
     axis line style={axisclr},
    legend image post style={scale =\limscale},
    legend style={at={(\lxshft ex,\lyshft ex)},anchor=south, legend columns = 1, draw = {dlegendclr}, fill={legendclr}, nodes={scale=\lscale}},
    ymajorgrids=true, 
    xmajorgrids=true,
    grid style={dashed, gridclr},
    major tick length=1ex,
    x label style={at={(\xlabelxshift ex, \xlabelyshift ex)},scale=\labelscale},
    y label style={at={(\ylabelxshift ex, \ylabelyshift ex)},scale=\labelscale},
    xticklabel style={scale=\ticklabelscale},
    yticklabel style={scale=\ticklabelscale},
%    ybar,
%    bar width = 4pt,
]
%
\input{exp_plots/open_ws_gripper/y}
%
%
\input{exp_plots/open_ws_gripper/y_des}
%
%% 
  \legend{Ref, SLAM}
  %
\end{axis}
%
% \node [draw=gpudclr,fill=gpuclr,rounded corners=0.2ex, minimum width=10.0ex, xshift=\titlexshift ex, yshift=\titleyshift ex, scale=\titlescale]{\textcolor{gputxtclr}{\textbf{Step-X}}};
}};
%
% 
%
\node (c) [xshift = \xshftc ex, yshift=\yshftc ex, scale=\scal]{
\tikz{
%
\pgfplotsset{width=\pltw ex, height=\plth ex}
\begin{axis}[
   axis background style={fill=axisbgclr},
    title={},
    xlabel={},
    ylabel={ Z (m)},
    xmin=0, xmax=30,
    ymin=-1, ymax=1,
    xtick={0, 15, 30, 45, 60},
    ytick={-1, 0, 1},
    xticklabels={$0$, $15$, $30$, $45$, $60$},
    yticklabels={$-1$, $0$, $0$},
     axis line style={axisclr},
    legend image post style={scale =\limscale},
    legend style={at={(\lxshft ex,\lyshft ex)},anchor=south, legend columns = 1, draw = {dlegendclr}, fill={legendclr}, nodes={scale=\lscale}},
    ymajorgrids=true, 
    xmajorgrids=true,
    grid style={dashed, gridclr},
    major tick length=1ex,
    x label style={at={(\xlabelxshift ex, \xlabelyshift ex)},scale=\labelscale},
    y label style={at={(\ylabelxshift ex, \ylabelyshift ex)},scale=\labelscale},
    xticklabel style={scale=\ticklabelscale},
    yticklabel style={scale=\ticklabelscale},
%    ybar,
%    bar width = 4pt,
]
%
\input{exp_plots/open_ws_gripper/z}
%
%
\input{exp_plots/open_ws_gripper/z_des}
%
%% 
  \legend{Ref, SLAM}
  %
\end{axis}
%
% \node [draw=gpudclr,fill=gpuclr,rounded corners=0.2ex, minimum width=10.0ex, xshift=\titlexshift ex, yshift=\titleyshift ex, scale=\titlescale]{\textcolor{gputxtclr}{\textbf{Step-X}}};
}};
%
% 
%
\node (d) [xshift = \xshftd ex, yshift=\yshftd ex, scale=\scal]{
\tikz{
%
\pgfplotsset{width=\pltw ex, height=\plth ex}
\begin{axis}[
   axis background style={fill=axisbgclr},
    title={},
    xlabel={Time (s)},
    ylabel={ Yaw ($^\text{o}$)},
    xmin=0, xmax=30,
    ymin=-40, ymax=40,
    xtick={0, 15, 30, 45, 60},
    ytick={-1, 0, 1},
    xticklabels={$0$, $15$, $30$, $45$, $60$},
    yticklabels={$-1$, $0$, $0$},
     axis line style={axisclr},
    legend image post style={scale =\limscale},
    legend style={at={(\lxshft ex,\lyshft ex)},anchor=south, legend columns = 1, draw = {dlegendclr}, fill={legendclr}, nodes={scale=\lscale}},
    ymajorgrids=true, 
    xmajorgrids=true,
    grid style={dashed, gridclr},
    major tick length=1ex,
    x label style={at={(\xlabelxshift ex, \xlabelyshift ex)},scale=\labelscale},
    y label style={at={(\ylabelxshift ex, \ylabelyshift ex)},scale=\labelscale},
    xticklabel style={scale=\ticklabelscale},
    yticklabel style={scale=\ticklabelscale},
%    ybar,
%    bar width = 4pt,
]
%
\input{exp_plots/open_ws_gripper/yaw}
%
%
%
\input{exp_plots/open_ws_gripper/yaw_des}
%
%% 
  \legend{Ref, SLAM}
  %
\end{axis}
%
% \node [draw=gpudclr,fill=gpuclr,rounded corners=0.2ex, minimum width=10.0ex, xshift=\titlexshift ex, yshift=\titleyshift ex, scale=\titlescale]{\textcolor{gputxtclr}{\textbf{Step-X}}};
}};
%
% 
%
%
\node (t) [xshift=\xshfttakeoff ex, yshift=5 ex]{\scriptsize Takeoff};
\node (h) [xshift=\xshfthover ex, yshift=5 ex]{\scriptsize Hover};
\node (l) [xshift=\xshftland ex, yshift=5 ex]{\scriptsize Land};
%%
%
 
\end{tikzpicture}
%
%
\caption{Takeoff-Hover-Land performance in open workspace with gripper.}
%
\label{fig:openwsTHLgripper}
%
%\vspace{-3ex}
\end{figure}
%
%
%
%%


==> exp_plots/open_ws_gripper/thrust.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0)
(0.075, 10)
(0.15, 10)
(0.225, 10)
(0.3, 10)
(0.375, 10)
(0.45, 10)
(0.525, 10)
(0.6, 10)
(0.675, 10)
(0.75, 10)
(0.825, 10)
(0.9, 10)
(0.975, 10)
(1.05, 10)
(1.125, 13.1718)
(1.2, 14.7861)
(1.275, 16.1875)
(1.35, 17.4493)
(1.425, 18.9569)
(1.5, 20.3361)
(1.575, 21.6155)
(1.65, 22.669)
(1.725, 24.0654)
(1.8, 25.2895)
(1.875, 26.5321)
(1.95, 27.7828)
(2.025, 29.2446)
(2.1, 30.6701)
(2.175, 32.3288)
(2.25, 33.5776)
(2.325, 35.174)
(2.4, 36.9212)
(2.475, 38.8859)
(2.55, 40.672)
(2.625, 42.4765)
(2.7, 44.4585)
(2.775, 45.5951)
(2.85, 45.6106)
(2.925, 44.1611)
(3, 42.2842)
(3.075, 41.6643)
(3.15, 42.1885)
(3.225, 42.1681)
(3.3, 42.5223)
(3.375, 43.4795)
(3.45, 44.2557)
(3.525, 44.674)
(3.6, 44.8668)
(3.675, 44.8617)
(3.75, 44.7139)
(3.825, 44.5841)
(3.9, 43.9734)
(3.975, 43.8462)
(4.05, 43.983)
(4.125, 44.6334)
(4.2, 45.5156)
(4.275, 46.4364)
(4.35, 47.3569)
(4.425, 47.3496)
(4.5, 45.9746)
(4.575, 43.9974)
(4.65, 43.3346)
(4.725, 44.2496)
(4.8, 46.3341)
(4.875, 47.7879)
(4.95, 48.5637)
(5.025, 47.2701)
(5.1, 46.2062)
(5.175, 44.9702)
(5.25, 44.8209)
(5.325, 45.8061)
(5.4, 47.5758)
(5.475, 48.7402)
(5.55, 46.8124)
(5.625, 44.6287)
(5.7, 43.9592)
(5.775, 44.9341)
(5.85, 46.69)
(5.925, 48.0381)
(6, 49.4519)
(6.075, 49.1981)
(6.15, 47.6671)
(6.225, 46.5778)
(6.3, 46.4117)
(6.375, 46.4951)
(6.45, 46.5607)
(6.525, 46.5496)
(6.6, 46.8774)
(6.675, 47.6591)
(6.75, 48.4024)
(6.825, 48.5453)
(6.9, 48.0198)
(6.975, 47.1363)
(7.05, 47.1824)
(7.125, 47.9657)
(7.2, 48.4988)
(7.275, 48.9726)
(7.35, 48.2798)
(7.425, 47.2775)
(7.5, 46.7581)
(7.575, 47.0695)
(7.65, 47.2735)
(7.725, 47.5312)
(7.8, 47.1155)
(7.875, 44.6434)
(7.95, 43.5335)
(8.025, 45.5055)
(8.1, 47.7453)
(8.175, 49.2397)
(8.25, 49.8665)
(8.325, 49.5787)
(8.4, 49.2559)
(8.475, 47.8815)
(8.55, 46.5173)
(8.625, 45.6056)
(8.7, 46.8066)
(8.775, 48.3251)
(8.85, 49.2144)
(8.925, 49.4878)
(9, 48.6795)
(9.075, 47.6527)
(9.15, 47.3238)
(9.225, 47.4431)
(9.3, 47.9632)
(9.375, 48.4342)
(9.45, 48.5404)
(9.525, 48.5275)
(9.6, 48.5125)
(9.675, 48.2604)
(9.75, 47.9493)
(9.825, 48.002)
(9.9, 48.3413)
(9.975, 48.4108)
(10.05, 48.1842)
(10.125, 47.8932)
(10.2, 48.3664)
(10.275, 48.5765)
(10.35, 48.8392)
(10.425, 48.5991)
(10.5, 48.0181)
(10.575, 47.5276)
(10.65, 47.4764)
(10.725, 47.9348)
(10.8, 48.7196)
(10.875, 49.6216)
(10.95, 50.1616)
(11.025, 50.2646)
(11.1, 50.3172)
(11.175, 49.4884)
(11.25, 48.4309)
(11.325, 47.878)
(11.4, 47.5174)
(11.475, 46.8203)
(11.55, 46.737)
(11.625, 47.3433)
(11.7, 48.7936)
(11.775, 49.7233)
(11.85, 49.6389)
(11.925, 48.9425)
(12, 48.7441)
(12.075, 49.0217)
(12.15, 49.9656)
(12.225, 49.2346)
(12.3, 48.1458)
(12.375, 47.8588)
(12.45, 48.1739)
(12.525, 48.3072)
(12.6, 48.6846)
(12.675, 49.1778)
(12.75, 49.4293)
(12.825, 48.8775)
(12.9, 48.2526)
(12.975, 46.7839)
(13.05, 46.4212)
(13.125, 47.3193)
(13.2, 48.3076)
(13.275, 48.3219)
(13.35, 47.9766)
(13.425, 47.7346)
(13.5, 48.5764)
(13.575, 49.9818)
(13.65, 50.2864)
(13.725, 50.0714)
(13.8, 49.2412)
(13.875, 47.5753)
(13.95, 46.0622)
(14.025, 46.1994)
(14.1, 47.6061)
(14.175, 48.7427)
(14.25, 49.2168)
(14.325, 49.1629)
(14.4, 48.6476)
(14.475, 48.4369)
(14.55, 48.1558)
(14.625, 48.0503)
(14.7, 48.128)
(14.775, 48.0602)
(14.85, 48.4134)
(14.925, 50.1045)
(15, 50.8476)
(15.075, 50.7288)
(15.15, 50.0894)
(15.225, 49.804)
(15.3, 49.588)
(15.375, 49.2077)
(15.45, 48.8673)
(15.525, 49.0177)
(15.6, 49.2683)
(15.675, 49.6204)
(15.75, 50.1168)
(15.825, 51.4703)
(15.9, 52.4398)
(15.975, 51.8421)
(16.05, 50.2662)
(16.125, 48.6068)
(16.2, 47.6449)
(16.275, 47.4346)
(16.35, 47.7782)
(16.425, 48.8281)
(16.5, 49.5772)
(16.575, 49.8154)
(16.65, 49.5755)
(16.725, 49.4012)
(16.8, 49.8184)
(16.875, 49.9928)
(16.95, 49.8145)
(17.025, 49.4216)
(17.1, 48.5414)
(17.175, 47.4796)
(17.25, 47.4807)
(17.325, 47.7803)
(17.4, 48.346)
(17.475, 48.4508)
(17.55, 49.3663)
(17.625, 50.3836)
(17.7, 50.3059)
(17.775, 48.8548)
(17.85, 47.5899)
(17.925, 46.6688)
(18, 46.8382)
(18.075, 47.3337)
(18.15, 47.8626)
(18.225, 48.0193)
(18.3, 48.1469)
(18.375, 48.2464)
(18.45, 48.4062)
(18.525, 48.5516)
(18.6, 48.0225)
(18.675, 48.9409)
(18.75, 50.9417)
(18.825, 50.902)
(18.9, 49.3421)
(18.975, 47.9587)
(19.05, 47.1362)
(19.125, 47.2803)
(19.2, 47.8474)
(19.275, 48.113)
(19.35, 48.4162)
(19.425, 47.8633)
(19.5, 47.2069)
(19.575, 46.4142)
(19.65, 46.1646)
(19.725, 46.943)
(19.8, 47.9366)
(19.875, 48.1885)
(19.95, 47.6746)
(20.025, 47.6048)
(20.1, 48.2895)
(20.175, 48.7778)
(20.25, 49.3949)
(20.325, 49.6219)
(20.4, 49.1987)
(20.475, 48.4522)
(20.55, 47.9454)
(20.625, 46.8447)
(20.7, 46.3026)
(20.775, 46.2851)
(20.85, 47.6292)
(20.925, 48.9496)
(21, 49.4486)
(21.075, 49.3572)
(21.15, 48.3574)
(21.225, 47.1693)
(21.3, 46.7318)
(21.375, 47.704)
(21.45, 48.6284)
(21.525, 48.8249)
(21.6, 48.1563)
(21.675, 47.6376)
(21.75, 47.7234)
(21.825, 48.1391)
(21.9, 48.2198)
(21.975, 48.0871)
(22.05, 48.2279)
(22.125, 48.3699)
(22.2, 48.1219)
(22.275, 47.8366)
(22.35, 48.1555)
(22.425, 48.6186)
(22.5, 48.9187)
(22.575, 48.7144)
(22.65, 48.5281)
(22.725, 48.1063)
(22.8, 47.083)
(22.875, 45.9698)
(22.95, 45.8522)
(23.025, 46.3458)
(23.1, 46.4002)
(23.175, 46.0916)
(23.25, 45.9382)
(23.325, 45.8823)
(23.4, 45.8442)
(23.475, 46.4607)
(23.55, 47.6642)
(23.625, 48.5874)
(23.7, 48.7804)
(23.775, 47.3633)
(23.85, 45.3633)
(23.925, 44.6059)
(24, 45.323)
(24.075, 46.0617)
(24.15, 46.8083)
(24.225, 46.7941)
(24.3, 45.6976)
(24.375, 45.0076)
(24.45, 44.7965)
(24.525, 44.5912)
(24.6, 44.294)
(24.675, 43.788)
(24.75, 44.0551)
(24.825, 44.7482)
(24.9, 45.94)
(24.975, 45.9291)
(25.05, 44.9641)
(25.125, 44.437)
(25.2, 43.7921)
(25.275, 44.3589)
(25.35, 44.455)
(25.425, 45.5144)
(25.5, 45.6997)
(25.575, 45.0699)
(25.65, 44.746)
(25.725, 43.7699)
(25.8, 43.2808)
(25.875, 42.9667)
(25.95, 43.4259)
(26.025, 44.3597)
(26.1, 44.98)
(26.175, 45.9387)
(26.25, 45.7511)
(26.325, 46.0701)
(26.4, 45.7205)
(26.475, 43.3064)
(26.55, 41.1672)
(26.625, 40.671)
(26.7, 41.1497)
(26.775, 42.3532)
(26.85, 42.8649)
(26.925, 42.1992)
(27, 41.2158)
(27.075, 40.4485)
(27.15, 38.9754)
(27.225, 37.4796)
(27.3, 37.5795)
(27.375, 37.6784)
(27.45, 37.9756)
(27.525, 37.639)
(27.6, 36.0453)
(27.675, 34.5931)
(27.75, 34.4177)
(27.825, 33.7837)
(27.9, 33.1024)
(27.975, 32.051)
(28.05, 31.1905)
(28.125, 30.1968)
(28.2, 29.2212)
(28.275, 28.4732)
(28.35, 27.7723)
(28.425, 26.8891)
(28.5, 25.8403)
(28.575, 24.9619)
(28.65, 24.0473)
(28.725, 23.0154)
(28.8, 21.7508)
(28.875, 21.0904)
(28.95, 20.0976)
(29.025, 19.2922)
(29.1, 18.3342)
(29.175, 17.2117)
(29.25, 16.0981)
(29.325, 14.7727)
(29.4, 13.6491)
(29.475, 12.5082)
(29.55, 11.8677)
(29.625, 10.9041)
(29.7, 10)
(29.775, 10)
(29.85, 10)
(29.925, 10)
(30, 10)
(30.075, 10)
(30.15, 10)
(30.225, 10)
(30.3, 10)
(30.375, 10)
(30.45, 10)
(30.525, 10)
(30.6, 10)
(30.675, 10)
(30.75, 10)
(30.825, 10)
(30.9, 10)
(30.975, 10)
(31.05, 10)
(31.125, 10)
(31.2, 10)
(31.275, 10)
(31.35, 10)
(31.425, 10)
(31.5, 10)
(31.575, 10)
(31.65, 10)
(31.725, 10)
(31.8, 10)
(31.875, 10)
(31.95, 10)
(32.025, 10)
(32.1, 10)
(32.175, 10)
(32.25, 10)
(32.325, 10)
(32.4, 10)
(32.475, 10)
(32.55, 10)
(32.625, 10)
(32.7, 10)
(32.775, 10)
(32.85, 10)
(32.925, 10)
(33, 10)
(33.075, 10)
(33.15, 10)
(33.225, 10)
(33.3, 10)
(33.375, 10)
(33.45, 10)
(33.525, 10)
(33.6, 10)
(33.675, 10)
(33.75, 10)
(33.825, 10)
(33.9, 10)
(33.975, 10)
(34.05, 10)
(34.125, 10)
(34.2, 10)
(34.275, 10)
(34.35, 10)
(34.425, 10)
(34.5, 10)
(34.575, 10)
(34.65, 10)
};

==> exp_plots/open_ws_gripper/x.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0)
(0.075, 0.000554018)
(0.15, 0.000779225)
(0.225, 0.000861512)
(0.3, 0.000404807)
(0.375, 0.000496276)
(0.45, 0.00115234)
(0.525, 0.00233792)
(0.6, 0.00176396)
(0.675, 0.00193702)
(0.75, 0.00131305)
(0.825, 0.00104044)
(0.9, 0.000803532)
(0.975, 0.00110581)
(1.05, 0.000979935)
(1.125, 0.0014516)
(1.2, 0.00115697)
(1.275, 0.000262169)
(1.35, 0.00150724)
(1.425, 0.00276654)
(1.5, 0.00159077)
(1.575, 0.00229235)
(1.65, 0.00340356)
(1.725, 0.00434308)
(1.8, 0.00264508)
(1.875, 0.0022118)
(1.95, 0.00434075)
(2.025, 0.00268052)
(2.1, 0.00193235)
(2.175, 0.00104827)
(2.25, 0.00100195)
(2.325, -5.08883e-05)
(2.4, 7.53523e-05)
(2.475, 0.00022959)
(2.55, 0.000517393)
(2.625, 0.0041032)
(2.7, 0.00521977)
(2.775, 0.00501146)
(2.85, 0.00583973)
(2.925, 0.00502578)
(3, 0.0107301)
(3.075, 0.0176717)
(3.15, 0.0327198)
(3.225, 0.0478235)
(3.3, 0.0638142)
(3.375, 0.0796589)
(3.45, 0.0984356)
(3.525, 0.110807)
(3.6, 0.122963)
(3.675, 0.128613)
(3.75, 0.137833)
(3.825, 0.146934)
(3.9, 0.155941)
(3.975, 0.158495)
(4.05, 0.158086)
(4.125, 0.153542)
(4.2, 0.146337)
(4.275, 0.137935)
(4.35, 0.123657)
(4.425, 0.106812)
(4.5, 0.0915209)
(4.575, 0.0771158)
(4.65, 0.0688592)
(4.725, 0.0605314)
(4.8, 0.0506299)
(4.875, 0.0445974)
(4.95, 0.0375763)
(5.025, 0.0256875)
(5.1, 0.0194882)
(5.175, 0.0167458)
(5.25, -0.00134864)
(5.325, -0.00756659)
(5.4, -0.0172906)
(5.475, -0.0286014)
(5.55, -0.0361474)
(5.625, -0.0404233)
(5.7, -0.0475498)
(5.775, -0.0560513)
(5.85, -0.0614541)
(5.925, -0.0635602)
(6, -0.0623553)
(6.075, -0.0640561)
(6.15, -0.0614057)
(6.225, -0.05951)
(6.3, -0.0584225)
(6.375, -0.0575255)
(6.45, -0.0498307)
(6.525, -0.0472488)
(6.6, -0.0413182)
(6.675, -0.0368781)
(6.75, -0.0368141)
(6.825, -0.034038)
(6.9, -0.0346097)
(6.975, -0.0349162)
(7.05, -0.0378231)
(7.125, -0.0364905)
(7.2, -0.0335351)
(7.275, -0.0335981)
(7.35, -0.0346339)
(7.425, -0.0342451)
(7.5, -0.0297232)
(7.575, -0.0215527)
(7.65, -0.0200939)
(7.725, -0.0141728)
(7.8, -0.00840155)
(7.875, -0.00855581)
(7.95, -0.0117226)
(8.025, -0.0101568)
(8.1, -0.00853836)
(8.175, -0.00862744)
(8.25, -0.00753765)
(8.325, -0.00579787)
(8.4, -0.0018639)
(8.475, -0.00585705)
(8.55, -0.0125301)
(8.625, -0.0164312)
(8.7, -0.0176279)
(8.775, -0.019134)
(8.85, -0.0206544)
(8.925, -0.0199634)
(9, -0.018324)
(9.075, -0.0150515)
(9.15, -0.00958679)
(9.225, -0.00829419)
(9.3, -0.00844236)
(9.375, -0.00822793)
(9.45, -0.00831298)
(9.525, -0.006126)
(9.6, -0.00879971)
(9.675, -0.0140872)
(9.75, -0.0095471)
(9.825, -0.0106222)
(9.9, -0.0122424)
(9.975, -0.0125319)
(10.05, -0.0174833)
(10.125, -0.0197516)
(10.2, -0.0216334)
(10.275, -0.0222173)
(10.35, -0.0225827)
(10.425, -0.0234503)
(10.5, -0.0271861)
(10.575, -0.0285)
(10.65, -0.0327912)
(10.725, -0.0334833)
(10.8, -0.0363923)
(10.875, -0.0401123)
(10.95, -0.037866)
(11.025, -0.0375058)
(11.1, -0.0344041)
(11.175, -0.0362516)
(11.25, -0.0302976)
(11.325, -0.0292096)
(11.4, -0.0302688)
(11.475, -0.0278974)
(11.55, -0.0229135)
(11.625, -0.0215835)
(11.7, -0.0189952)
(11.775, -0.0173026)
(11.85, -0.0158495)
(11.925, -0.00804087)
(12, -0.00517906)
(12.075, -0.00499115)
(12.15, -0.00315117)
(12.225, 0.00445896)
(12.3, 0.00764974)
(12.375, 0.00836928)
(12.45, 0.00748516)
(12.525, 0.0102824)
(12.6, 0.0120647)
(12.675, 0.0151348)
(12.75, 0.0148776)
(12.825, 0.0157952)
(12.9, 0.00791349)
(12.975, 0.00567959)
(13.05, 0.00450364)
(13.125, 0.00174308)
(13.2, -0.00243757)
(13.275, -0.00693288)
(13.35, -0.0119051)
(13.425, -0.0148413)
(13.5, -0.0182739)
(13.575, -0.0214667)
(13.65, -0.0245038)
(13.725, -0.0246269)
(13.8, -0.0220574)
(13.875, -0.0237351)
(13.95, -0.0257658)
(14.025, -0.0267427)
(14.1, -0.0248836)
(14.175, -0.0259738)
(14.25, -0.0237997)
(14.325, -0.0260808)
(14.4, -0.0267493)
(14.475, -0.0282971)
(14.55, -0.0266395)
(14.625, -0.0225359)
(14.7, -0.019741)
(14.775, -0.0153136)
(14.85, -0.0173627)
(14.925, -0.0154603)
(15, -0.0133478)
(15.075, -0.0137583)
(15.15, -0.00893374)
(15.225, -0.00131235)
(15.3, 0.00788985)
(15.375, 0.00806834)
(15.45, 0.0100658)
(15.525, 0.0115542)
(15.6, 0.0122374)
(15.675, 0.0122986)
(15.75, 0.00922048)
(15.825, 0.0133939)
(15.9, 0.0169405)
(15.975, 0.0182504)
(16.05, 0.0203469)
(16.125, 0.0207485)
(16.2, 0.0245578)
(16.275, 0.0264018)
(16.35, 0.0280521)
(16.425, 0.0290994)
(16.5, 0.0297389)
(16.575, 0.0296445)
(16.65, 0.0287632)
(16.725, 0.0211289)
(16.8, 0.0158742)
(16.875, 0.0111463)
(16.95, 0.0127291)
(17.025, 0.0120966)
(17.1, 0.00891824)
(17.175, 0.0115137)
(17.25, 0.00878495)
(17.325, 0.00574336)
(17.4, 0.00776893)
(17.475, 0.00279092)
(17.55, -0.00109319)
(17.625, -0.00423497)
(17.7, -0.00839321)
(17.775, -0.0151076)
(17.85, -0.0175934)
(17.925, -0.019621)
(18, -0.0208476)
(18.075, -0.0230453)
(18.15, -0.0287938)
(18.225, -0.0327415)
(18.3, -0.0341123)
(18.375, -0.0363309)
(18.45, -0.0375618)
(18.525, -0.0386759)
(18.6, -0.037475)
(18.675, -0.0353241)
(18.75, -0.0359037)
(18.825, -0.0339972)
(18.9, -0.0256087)
(18.975, -0.0249039)
(19.05, -0.0282254)
(19.125, -0.0244728)
(19.2, -0.0243137)
(19.275, -0.0231927)
(19.35, -0.022817)
(19.425, -0.0233118)
(19.5, -0.0214786)
(19.575, -0.0188217)
(19.65, -0.0157503)
(19.725, -0.0131802)
(19.8, -0.0135369)
(19.875, -0.0149633)
(19.95, -0.0173947)
(20.025, -0.0172619)
(20.1, -0.0186498)
(20.175, -0.0214838)
(20.25, -0.024327)
(20.325, -0.027158)
(20.4, -0.0285175)
(20.475, -0.0290213)
(20.55, -0.0283161)
(20.625, -0.0293267)
(20.7, -0.0217435)
(20.775, -0.0168108)
(20.85, -0.0143914)
(20.925, -0.00672754)
(21, -0.00261992)
(21.075, 0.00112248)
(21.15, 0.00483914)
(21.225, 0.00778347)
(21.3, 0.0133873)
(21.375, 0.0147767)
(21.45, 0.0195624)
(21.525, 0.0191675)
(21.6, 0.0175962)
(21.675, 0.0139849)
(21.75, 0.00852554)
(21.825, 0.00438784)
(21.9, 0.000667744)
(21.975, -0.000955274)
(22.05, 6.71252e-05)
(22.125, -0.000944607)
(22.2, 0.000187445)
(22.275, 0.000502989)
(22.35, 4.00339e-05)
(22.425, -0.0013995)
(22.5, -0.00192704)
(22.575, -0.00137129)
(22.65, -0.00282343)
(22.725, -0.00600122)
(22.8, -0.00827862)
(22.875, -0.0113216)
(22.95, -0.0139042)
(23.025, -0.014688)
(23.1, -0.0184117)
(23.175, -0.0224588)
(23.25, -0.02922)
(23.325, -0.0310798)
(23.4, -0.0329382)
(23.475, -0.0371609)
(23.55, -0.0351594)
(23.625, -0.0345691)
(23.7, -0.0308612)
(23.775, -0.0324646)
(23.85, -0.0222242)
(23.925, -0.0184093)
(24, -0.0124693)
(24.075, -0.0114885)
(24.15, -0.00982035)
(24.225, -0.0134776)
(24.3, -0.0158022)
(24.375, -0.0121211)
(24.45, -0.00509741)
(24.525, -0.00763965)
(24.6, -0.0128239)
(24.675, -0.0140628)
(24.75, -0.00826155)
(24.825, -0.00509353)
(24.9, -0.0041866)
(24.975, -0.00321386)
(25.05, -0.000640421)
(25.125, -0.00207387)
(25.2, 0.0019284)
(25.275, 0.00835324)
(25.35, 0.00783718)
(25.425, 0.00903939)
(25.5, 6.52096e-05)
(25.575, -0.00819147)
(25.65, -0.0126171)
(25.725, -0.0102892)
(25.8, -0.0163776)
(25.875, -0.0147464)
(25.95, -0.0167262)
(26.025, -0.0177218)
(26.1, -0.0159464)
(26.175, -0.0172537)
(26.25, -0.0149522)
(26.325, 0.00208436)
(26.4, 0.0112592)
(26.475, 0.0243666)
(26.55, 0.0283494)
(26.625, 0.0363045)
(26.7, 0.0416603)
(26.775, 0.0495281)
(26.85, 0.0516285)
(26.925, 0.0498385)
(27, 0.0500894)
(27.075, 0.0538747)
(27.15, 0.0531343)
(27.225, 0.0549779)
(27.3, 0.0531166)
(27.375, 0.0543984)
(27.45, 0.053426)
(27.525, 0.0490756)
(27.6, 0.0495777)
(27.675, 0.050221)
(27.75, 0.0489848)
(27.825, 0.0503888)
(27.9, 0.0522982)
(27.975, 0.0515996)
(28.05, 0.0463215)
(28.125, 0.0455902)
(28.2, 0.0453842)
(28.275, 0.0482136)
(28.35, 0.0496402)
(28.425, 0.0481964)
(28.5, 0.0494879)
(28.575, 0.0509819)
(28.65, 0.050946)
(28.725, 0.0517374)
(28.8, 0.0503873)
(28.875, 0.0490674)
(28.95, 0.0490571)
(29.025, 0.0489385)
(29.1, 0.0464908)
(29.175, 0.0469003)
(29.25, 0.0495533)
(29.325, 0.0498448)
(29.4, 0.04873)
(29.475, 0.0468473)
(29.55, 0.0467417)
(29.625, 0.0469218)
(29.7, 0.0482357)
(29.775, 0.0485979)
(29.85, 0.0486006)
(29.925, 0.050256)
(30, 0.0538584)
(30.075, 0.0548813)
(30.15, 0.0544638)
(30.225, 0.0536085)
(30.3, 0.0528518)
(30.375, 0.0523936)
(30.45, 0.0515061)
(30.525, 0.0507818)
(30.6, 0.0509018)
(30.675, 0.049808)
(30.75, 0.0504747)
(30.825, 0.0526015)
(30.9, 0.0527967)
(30.975, 0.0515972)
(31.05, 0.048922)
(31.125, 0.0480373)
(31.2, 0.0478501)
(31.275, 0.0477054)
(31.35, 0.0476407)
(31.425, 0.04764)
(31.5, 0.0486121)
(31.575, 0.0523413)
(31.65, 0.0525413)
(31.725, 0.0513094)
(31.8, 0.0506903)
(31.875, 0.0497733)
(31.95, 0.0503021)
(32.025, 0.0540202)
(32.1, 0.0552954)
(32.175, 0.0534725)
(32.25, 0.0529075)
(32.325, 0.0488852)
(32.4, 0.0472934)
(32.475, 0.0464244)
(32.55, 0.0459447)
(32.625, 0.0473981)
(32.7, 0.04621)
(32.775, 0.0471197)
(32.85, 0.0467462)
(32.925, 0.0468818)
(33, 0.0470616)
(33.075, 0.0478208)
(33.15, 0.0479998)
(33.225, 0.0471879)
(33.3, 0.0477175)
(33.375, 0.048081)
(33.45, 0.0478711)
(33.525, 0.0473227)
(33.6, 0.0478211)
(33.675, 0.0482607)
(33.75, 0.0473697)
(33.825, 0.0468473)
(33.9, 0.0481274)
(33.975, 0.0475653)
(34.05, 0.0461293)
(34.125, 0.0457985)
(34.2, 0.0463182)
(34.275, 0.0462637)
(34.35, 0.0458688)
(34.425, 0.0452524)
(34.5, 0.0456753)
(34.575, 0.0461002)
(34.65, 0.0463545)
};

==> exp_plots/open_ws_gripper/x_des.tex <==
\addplot[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates {
(0, 0)
(0.075, 0)
(0.15, 0)
(0.225, 0)
(0.3, 0)
(0.375, 0)
(0.45, 0)
(0.525, 0)
(0.6, 0)
(0.675, 0)
(0.75, 0)
(0.825, 0)
(0.9, 0)
(0.975, 0)
(1.05, 0)
(1.125, 0)
(1.2, 0)
(1.275, 0)
(1.35, 0)
(1.425, 0)
(1.5, 0)
(1.575, 0)
(1.65, 0)
(1.725, 0)
(1.8, 0)
(1.875, 0)
(1.95, 0)
(2.025, 0)
(2.1, 0)
(2.175, 0)
(2.25, 0)
(2.325, 0)
(2.4, 0)
(2.475, 0)
(2.55, 0)
(2.625, 0)
(2.7, 0)
(2.775, 0)
(2.85, 0)
(2.925, 0)
(3, 0)
(3.075, 0)
(3.15, 0)
(3.225, 0)
(3.3, 0)
(3.375, 0)
(3.45, 0)
(3.525, 0)
(3.6, 0)
(3.675, 0)
(3.75, 0)
(3.825, 0)
(3.9, 0)
(3.975, 0)
(4.05, 0)
(4.125, 0)
(4.2, 0)
(4.275, 0)
(4.35, 0)
(4.425, 0)
(4.5, 0)
(4.575, 0)
(4.65, 0)
(4.725, 0)
(4.8, 0)
(4.875, 0)
(4.95, 0)
(5.025, 0)
(5.1, 0)
(5.175, 0)
(5.25, 0)
(5.325, 0)
(5.4, 0)
(5.475, 0)
(5.55, 0)
(5.625, 0)
(5.7, 0)
(5.775, 0)
(5.85, 0)
(5.925, 0)
(6, 0)
(6.075, 0)
(6.15, 0)
(6.225, 0)
(6.3, 0)
(6.375, 0)
(6.45, 0)
(6.525, 0)
(6.6, 0)
(6.675, 0)
(6.75, 0)
(6.825, 0)
(6.9, 0)
(6.975, 0)
(7.05, 0)
(7.125, 0)
(7.2, 0)
(7.275, 0)
(7.35, 0)
(7.425, 0)
(7.5, 0)
(7.575, 0)
(7.65, 0)
(7.725, 0)
(7.8, 0)
(7.875, 0)
(7.95, 0)
(8.025, 0)
(8.1, 0)
(8.175, 0)
(8.25, 0)
(8.325, 0)
(8.4, 0)
(8.475, 0)
(8.55, 0)
(8.625, 0)
(8.7, 0)
(8.775, 0)
(8.85, 0)
(8.925, 0)
(9, 0)
(9.075, 0)
(9.15, 0)
(9.225, 0)
(9.3, 0)
(9.375, 0)
(9.45, 0)
(9.525, 0)
(9.6, 0)
(9.675, 0)
(9.75, 0)
(9.825, 0)
(9.9, 0)
(9.975, 0)
(10.05, 0)
(10.125, 0)
(10.2, 0)
(10.275, 0)
(10.35, 0)
(10.425, 0)
(10.5, 0)
(10.575, 0)
(10.65, 0)
(10.725, 0)
(10.8, 0)
(10.875, 0)
(10.95, 0)
(11.025, 0)
(11.1, 0)
(11.175, 0)
(11.25, 0)
(11.325, 0)
(11.4, 0)
(11.475, 0)
(11.55, 0)
(11.625, 0)
(11.7, 0)
(11.775, 0)
(11.85, 0)
(11.925, 0)
(12, 0)
(12.075, 0)
(12.15, 0)
(12.225, 0)
(12.3, 0)
(12.375, 0)
(12.45, 0)
(12.525, 0)
(12.6, 0)
(12.675, 0)
(12.75, 0)
(12.825, 0)
(12.9, 0)
(12.975, 0)
(13.05, 0)
(13.125, 0)
(13.2, 0)
(13.275, 0)
(13.35, 0)
(13.425, 0)
(13.5, 0)
(13.575, 0)
(13.65, 0)
(13.725, 0)
(13.8, 0)
(13.875, 0)
(13.95, 0)
(14.025, 0)
(14.1, 0)
(14.175, 0)
(14.25, 0)
(14.325, 0)
(14.4, 0)
(14.475, 0)
(14.55, 0)
(14.625, 0)
(14.7, 0)
(14.775, 0)
(14.85, 0)
(14.925, 0)
(15, 0)
(15.075, 0)
(15.15, 0)
(15.225, 0)
(15.3, 0)
(15.375, 0)
(15.45, 0)
(15.525, 0)
(15.6, 0)
(15.675, 0)
(15.75, 0)
(15.825, 0)
(15.9, 0)
(15.975, 0)
(16.05, 0)
(16.125, 0)
(16.2, 0)
(16.275, 0)
(16.35, 0)
(16.425, 0)
(16.5, 0)
(16.575, 0)
(16.65, 0)
(16.725, 0)
(16.8, 0)
(16.875, 0)
(16.95, 0)
(17.025, 0)
(17.1, 0)
(17.175, 0)
(17.25, 0)
(17.325, 0)
(17.4, 0)
(17.475, 0)
(17.55, 0)
(17.625, 0)
(17.7, 0)
(17.775, 0)
(17.85, 0)
(17.925, 0)
(18, 0)
(18.075, 0)
(18.15, 0)
(18.225, 0)
(18.3, 0)
(18.375, 0)
(18.45, 0)
(18.525, 0)
(18.6, 0)
(18.675, 0)
(18.75, 0)
(18.825, 0)
(18.9, 0)
(18.975, 0)
(19.05, 0)
(19.125, 0)
(19.2, 0)
(19.275, 0)
(19.35, 0)
(19.425, 0)
(19.5, 0)
(19.575, 0)
(19.65, 0)
(19.725, 0)
(19.8, 0)
(19.875, 0)
(19.95, 0)
(20.025, 0)
(20.1, 0)
(20.175, 0)
(20.25, 0)
(20.325, 0)
(20.4, 0)
(20.475, 0)
(20.55, 0)
(20.625, 0)
(20.7, 0)
(20.775, 0)
(20.85, 0)
(20.925, 0)
(21, 0)
(21.075, 0)
(21.15, 0)
(21.225, 0)
(21.3, 0)
(21.375, 0)
(21.45, 0)
(21.525, 0)
(21.6, 0)
(21.675, 0)
(21.75, 0)
(21.825, 0)
(21.9, 0)
(21.975, 0)
(22.05, 0)
(22.125, 0)
(22.2, 0)
(22.275, 0)
(22.35, 0)
(22.425, 0)
(22.5, 0)
(22.575, 0)
(22.65, 0)
(22.725, 0)
(22.8, 0)
(22.875, 0)
(22.95, 0)
(23.025, 0)
(23.1, 0)
(23.175, 0)
(23.25, 0)
(23.325, 0)
(23.4, 0)
(23.475, 0)
(23.55, 0)
(23.625, 0)
(23.7, 0)
(23.775, 0)
(23.85, 0)
(23.925, 0)
(24, 0)
(24.075, 0)
(24.15, 0)
(24.225, 0)
(24.3, 0)
(24.375, 0)
(24.45, 0)
(24.525, 0)
(24.6, 0)
(24.675, 0)
(24.75, 0)
(24.825, 0)
(24.9, 0)
(24.975, 0)
(25.05, 0)
(25.125, 0)
(25.2, 0)
(25.275, 0)
(25.35, 0)
(25.425, 0)
(25.5, 0)
(25.575, 0)
(25.65, 0)
(25.725, 0)
(25.8, 0)
(25.875, 0)
(25.95, 0)
(26.025, 0)
(26.1, 0)
(26.175, 0)
(26.25, 0)
(26.325, 0)
(26.4, 0)
(26.475, 0)
(26.55, 0)
(26.625, 0)
(26.7, 0)
(26.775, 0)
(26.85, 0)
(26.925, 0)
(27, 0)
(27.075, 0)
(27.15, 0)
(27.225, 0)
(27.3, 0)
(27.375, 0)
(27.45, 0)
(27.525, 0)
(27.6, 0)
(27.675, 0)
(27.75, 0)
(27.825, 0)
(27.9, 0)
(27.975, 0)
(28.05, 0)
(28.125, 0)
(28.2, 0)
(28.275, 0)
(28.35, 0)
(28.425, 0)
(28.5, 0)
(28.575, 0)
(28.65, 0)
(28.725, 0)
(28.8, 0)
(28.875, 0)
(28.95, 0)
(29.025, 0)
(29.1, 0)
(29.175, 0)
(29.25, 0)
(29.325, 0)
(29.4, 0)
(29.475, 0)
(29.55, 0)
(29.625, 0)
(29.7, 0)
(29.775, 0)
(29.85, 0)
(29.925, 0)
(30, 0)
(30.075, 0)
(30.15, 0)
(30.225, 0)
(30.3, 0)
(30.375, 0)
(30.45, 0)
(30.525, 0)
(30.6, 0)
(30.675, 0)
(30.75, 0)
(30.825, 0)
(30.9, 0)
(30.975, 0)
(31.05, 0)
(31.125, 0)
(31.2, 0)
(31.275, 0)
(31.35, 0)
(31.425, 0)
(31.5, 0)
(31.575, 0)
(31.65, 0)
(31.725, 0)
(31.8, 0)
(31.875, 0)
(31.95, 0)
(32.025, 0)
(32.1, 0)
(32.175, 0)
(32.25, 0)
(32.325, 0)
(32.4, 0)
(32.475, 0)
(32.55, 0)
(32.625, 0)
(32.7, 0)
(32.775, 0)
(32.85, 0)
(32.925, 0)
(33, 0)
(33.075, 0)
(33.15, 0)
(33.225, 0)
(33.3, 0)
(33.375, 0)
(33.45, 0)
(33.525, 0)
(33.6, 0)
(33.675, 0)
(33.75, 0)
(33.825, 0)
(33.9, 0)
(33.975, 0)
(34.05, 0)
(34.125, 0)
(34.2, 0)
(34.275, 0)
(34.35, 0)
(34.425, 0)
(34.5, 0)
(34.575, 0)
(34.65, 0)
};

==> exp_plots/open_ws_gripper/y.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0)
(0.075, 0.000297458)
(0.15, 0.000800959)
(0.225, 0.000322847)
(0.3, 0.000623961)
(0.375, 0.000724407)
(0.45, 0.000880074)
(0.525, 0.000906284)
(0.6, 0.000564541)
(0.675, -0.000284384)
(0.75, -0.00111749)
(0.825, -0.00039867)
(0.9, -0.000395071)
(0.975, -0.000479336)
(1.05, -4.07157e-05)
(1.125, -1.99362e-06)
(1.2, 2.24315e-05)
(1.275, -0.000242759)
(1.35, -0.000295011)
(1.425, -0.000584562)
(1.5, -0.000443049)
(1.575, -0.000445021)
(1.65, -0.000124537)
(1.725, 0.000766653)
(1.8, 0.00071294)
(1.875, 0.00020884)
(1.95, -0.000575727)
(2.025, -0.00100366)
(2.1, -0.000192503)
(2.175, 0.00122068)
(2.25, 0.00211368)
(2.325, 0.00261279)
(2.4, 0.00251597)
(2.475, 0.00253814)
(2.55, 0.00295495)
(2.625, 0.00195571)
(2.7, 0.00166665)
(2.775, 0.00137782)
(2.85, 0.00116135)
(2.925, -0.000245728)
(3, -0.00221241)
(3.075, -0.0054873)
(3.15, -0.0145522)
(3.225, -0.024731)
(3.3, -0.0316022)
(3.375, -0.0405209)
(3.45, -0.0451039)
(3.525, -0.0471027)
(3.6, -0.0492398)
(3.675, -0.049693)
(3.75, -0.0524113)
(3.825, -0.0646239)
(3.9, -0.0746475)
(3.975, -0.083479)
(4.05, -0.0921101)
(4.125, -0.102784)
(4.2, -0.108555)
(4.275, -0.112318)
(4.35, -0.116091)
(4.425, -0.117955)
(4.5, -0.121675)
(4.575, -0.123975)
(4.65, -0.122138)
(4.725, -0.118832)
(4.8, -0.128914)
(4.875, -0.131257)
(4.95, -0.13322)
(5.025, -0.137559)
(5.1, -0.139899)
(5.175, -0.141628)
(5.25, -0.135522)
(5.325, -0.133263)
(5.4, -0.132204)
(5.475, -0.12873)
(5.55, -0.121388)
(5.625, -0.118178)
(5.7, -0.117977)
(5.775, -0.113089)
(5.85, -0.109058)
(5.925, -0.103087)
(6, -0.094428)
(6.075, -0.0829638)
(6.15, -0.070206)
(6.225, -0.0625093)
(6.3, -0.0565608)
(6.375, -0.0554584)
(6.45, -0.0557253)
(6.525, -0.0518319)
(6.6, -0.0500898)
(6.675, -0.0433795)
(6.75, -0.0413341)
(6.825, -0.0419321)
(6.9, -0.0397191)
(6.975, -0.038558)
(7.05, -0.0402029)
(7.125, -0.0411314)
(7.2, -0.0435643)
(7.275, -0.0434597)
(7.35, -0.0447058)
(7.425, -0.0453727)
(7.5, -0.0480404)
(7.575, -0.0466861)
(7.65, -0.0463868)
(7.725, -0.0507328)
(7.8, -0.0517631)
(7.875, -0.0505241)
(7.95, -0.0498767)
(8.025, -0.0526059)
(8.1, -0.0549353)
(8.175, -0.0594997)
(8.25, -0.0581235)
(8.325, -0.0580017)
(8.4, -0.0590851)
(8.475, -0.0573995)
(8.55, -0.0573585)
(8.625, -0.058916)
(8.7, -0.0595299)
(8.775, -0.0597532)
(8.85, -0.0609645)
(8.925, -0.0615941)
(9, -0.0631375)
(9.075, -0.0642209)
(9.15, -0.0653901)
(9.225, -0.0654144)
(9.3, -0.0568825)
(9.375, -0.0529541)
(9.45, -0.049623)
(9.525, -0.0454156)
(9.6, -0.042049)
(9.675, -0.0368626)
(9.75, -0.026622)
(9.825, -0.0165756)
(9.9, -0.010165)
(9.975, -0.00798073)
(10.05, -0.00803742)
(10.125, -0.00665769)
(10.2, -0.00616646)
(10.275, -0.00646442)
(10.35, -0.00667877)
(10.425, -0.00671282)
(10.5, -0.00674314)
(10.575, -0.00883202)
(10.65, -0.0104242)
(10.725, -0.0117397)
(10.8, -0.0225032)
(10.875, -0.0255647)
(10.95, -0.0345351)
(11.025, -0.0479916)
(11.1, -0.0596244)
(11.175, -0.0671532)
(11.25, -0.0746467)
(11.325, -0.0763648)
(11.4, -0.0772834)
(11.475, -0.0799491)
(11.55, -0.0818459)
(11.625, -0.0844848)
(11.7, -0.0850432)
(11.775, -0.085526)
(11.85, -0.0863245)
(11.925, -0.0902861)
(12, -0.0896093)
(12.075, -0.0907068)
(12.15, -0.0904658)
(12.225, -0.0939857)
(12.3, -0.0961189)
(12.375, -0.0969744)
(12.45, -0.097218)
(12.525, -0.0970357)
(12.6, -0.0924938)
(12.675, -0.0924392)
(12.75, -0.0915898)
(12.825, -0.0901929)
(12.9, -0.0888282)
(12.975, -0.0881243)
(13.05, -0.0830849)
(13.125, -0.0709068)
(13.2, -0.0542801)
(13.275, -0.0401072)
(13.35, -0.0319912)
(13.425, -0.0220801)
(13.5, -0.014012)
(13.575, -0.00903659)
(13.65, 0.00234513)
(13.725, 0.00933415)
(13.8, 0.0069121)
(13.875, 0.00836485)
(13.95, 0.00862417)
(14.025, 0.0086799)
(14.1, 0.00558125)
(14.175, -0.0027454)
(14.25, -0.00793596)
(14.325, -0.0113533)
(14.4, -0.0167)
(14.475, -0.0219638)
(14.55, -0.0256383)
(14.625, -0.0304962)
(14.7, -0.036537)
(14.775, -0.0441451)
(14.85, -0.0489101)
(14.925, -0.0547234)
(15, -0.0623317)
(15.075, -0.0664792)
(15.15, -0.0662207)
(15.225, -0.0734024)
(15.3, -0.0761348)
(15.375, -0.0802217)
(15.45, -0.0821226)
(15.525, -0.083469)
(15.6, -0.0848938)
(15.675, -0.0843068)
(15.75, -0.0847075)
(15.825, -0.0885691)
(15.9, -0.0909348)
(15.975, -0.0931272)
(16.05, -0.0942531)
(16.125, -0.0939118)
(16.2, -0.0926621)
(16.275, -0.0915181)
(16.35, -0.0903662)
(16.425, -0.0893646)
(16.5, -0.0871355)
(16.575, -0.0858098)
(16.65, -0.0856762)
(16.725, -0.0829438)
(16.8, -0.0767074)
(16.875, -0.0744414)
(16.95, -0.0709464)
(17.025, -0.0697381)
(17.1, -0.0667966)
(17.175, -0.0635891)
(17.25, -0.062417)
(17.325, -0.0594722)
(17.4, -0.0594953)
(17.475, -0.0614336)
(17.55, -0.0584168)
(17.625, -0.0576485)
(17.7, -0.0569504)
(17.775, -0.058193)
(17.85, -0.0588014)
(17.925, -0.0577341)
(18, -0.0599394)
(18.075, -0.0612719)
(18.15, -0.0584171)
(18.225, -0.0558213)
(18.3, -0.0579288)
(18.375, -0.0584513)
(18.45, -0.0597894)
(18.525, -0.0606959)
(18.6, -0.064256)
(18.675, -0.0681127)
(18.75, -0.0706766)
(18.825, -0.0717997)
(18.9, -0.0666538)
(18.975, -0.0650545)
(19.05, -0.0567346)
(19.125, -0.0555186)
(19.2, -0.0517979)
(19.275, -0.0451469)
(19.35, -0.0395684)
(19.425, -0.0370154)
(19.5, -0.0348405)
(19.575, -0.0326397)
(19.65, -0.0312419)
(19.725, -0.0318816)
(19.8, -0.0326311)
(19.875, -0.029721)
(19.95, -0.027392)
(20.025, -0.0248899)
(20.1, -0.0241221)
(20.175, -0.0223828)
(20.25, -0.0220548)
(20.325, -0.024082)
(20.4, -0.0309073)
(20.475, -0.0344338)
(20.55, -0.0395005)
(20.625, -0.0453294)
(20.7, -0.0589996)
(20.775, -0.0669108)
(20.85, -0.072841)
(20.925, -0.0769968)
(21, -0.0814705)
(21.075, -0.083611)
(21.15, -0.0847927)
(21.225, -0.0855583)
(21.3, -0.0888266)
(21.375, -0.0987946)
(21.45, -0.103431)
(21.525, -0.106381)
(21.6, -0.109641)
(21.675, -0.115543)
(21.75, -0.115777)
(21.825, -0.121139)
(21.9, -0.126485)
(21.975, -0.134395)
(22.05, -0.138673)
(22.125, -0.1436)
(22.2, -0.149449)
(22.275, -0.156132)
(22.35, -0.159038)
(22.425, -0.160183)
(22.5, -0.161522)
(22.575, -0.159997)
(22.65, -0.157949)
(22.725, -0.157302)
(22.8, -0.156151)
(22.875, -0.154504)
(22.95, -0.155081)
(23.025, -0.153162)
(23.1, -0.151212)
(23.175, -0.140203)
(23.25, -0.132013)
(23.325, -0.119653)
(23.4, -0.10622)
(23.475, -0.0934333)
(23.55, -0.0832441)
(23.625, -0.0752742)
(23.7, -0.074309)
(23.775, -0.0569451)
(23.85, -0.0396708)
(23.925, -0.0231792)
(24, -0.00571329)
(24.075, 0.00904367)
(24.15, 0.022258)
(24.225, 0.0308126)
(24.3, 0.0354399)
(24.375, 0.0334212)
(24.45, 0.0354429)
(24.525, 0.0358258)
(24.6, 0.0312416)
(24.675, 0.034053)
(24.75, 0.0310609)
(24.825, 0.0318128)
(24.9, 0.0326608)
(24.975, 0.0324836)
(25.05, 0.032081)
(25.125, 0.0308185)
(25.2, 0.019557)
(25.275, 0.00342586)
(25.35, -0.00776427)
(25.425, -0.0224887)
(25.5, -0.0355107)
(25.575, -0.0440424)
(25.65, -0.0559367)
(25.725, -0.0688741)
(25.8, -0.0811967)
(25.875, -0.0960123)
(25.95, -0.105663)
(26.025, -0.106478)
(26.1, -0.107755)
(26.175, -0.110036)
(26.25, -0.110446)
(26.325, -0.11945)
(26.4, -0.124725)
(26.475, -0.129615)
(26.55, -0.127041)
(26.625, -0.129949)
(26.7, -0.132251)
(26.775, -0.131234)
(26.85, -0.124767)
(26.925, -0.113512)
(27, -0.112819)
(27.075, -0.114261)
(27.15, -0.116744)
(27.225, -0.119986)
(27.3, -0.11992)
(27.375, -0.119577)
(27.45, -0.120251)
(27.525, -0.11869)
(27.6, -0.121159)
(27.675, -0.125644)
(27.75, -0.128515)
(27.825, -0.127664)
(27.9, -0.128605)
(27.975, -0.130163)
(28.05, -0.12552)
(28.125, -0.123251)
(28.2, -0.121448)
(28.275, -0.12376)
(28.35, -0.125046)
(28.425, -0.126845)
(28.5, -0.128521)
(28.575, -0.130366)
(28.65, -0.131545)
(28.725, -0.132122)
(28.8, -0.128881)
(28.875, -0.124733)
(28.95, -0.122958)
(29.025, -0.124256)
(29.1, -0.126147)
(29.175, -0.125652)
(29.25, -0.122802)
(29.325, -0.122589)
(29.4, -0.124252)
(29.475, -0.124745)
(29.55, -0.124847)
(29.625, -0.127735)
(29.7, -0.131651)
(29.775, -0.132781)
(29.85, -0.133143)
(29.925, -0.132839)
(30, -0.131811)
(30.075, -0.131576)
(30.15, -0.130167)
(30.225, -0.130041)
(30.3, -0.13186)
(30.375, -0.130359)
(30.45, -0.130452)
(30.525, -0.132375)
(30.6, -0.132926)
(30.675, -0.132868)
(30.75, -0.132797)
(30.825, -0.132692)
(30.9, -0.131923)
(30.975, -0.131034)
(31.05, -0.131217)
(31.125, -0.131028)
(31.2, -0.131289)
(31.275, -0.132242)
(31.35, -0.132897)
(31.425, -0.133188)
(31.5, -0.133339)
(31.575, -0.132495)
(31.65, -0.131706)
(31.725, -0.129858)
(31.8, -0.131847)
(31.875, -0.132582)
(31.95, -0.129924)
(32.025, -0.129293)
(32.1, -0.129351)
(32.175, -0.130046)
(32.25, -0.130899)
(32.325, -0.132578)
(32.4, -0.132075)
(32.475, -0.132672)
(32.55, -0.129971)
(32.625, -0.131106)
(32.7, -0.13203)
(32.775, -0.134264)
(32.85, -0.133098)
(32.925, -0.131571)
(33, -0.130083)
(33.075, -0.131618)
(33.15, -0.132836)
(33.225, -0.132706)
(33.3, -0.134152)
(33.375, -0.134861)
(33.45, -0.135512)
(33.525, -0.136016)
(33.6, -0.135537)
(33.675, -0.134853)
(33.75, -0.13514)
(33.825, -0.135435)
(33.9, -0.13254)
(33.975, -0.131834)
(34.05, -0.131799)
(34.125, -0.132151)
(34.2, -0.132282)
(34.275, -0.132277)
(34.35, -0.132367)
(34.425, -0.132086)
(34.5, -0.132583)
(34.575, -0.133246)
(34.65, -0.133398)
};

==> exp_plots/open_ws_gripper/y_des.tex <==
\addplot[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates {
(0, 0)
(0.075, 0)
(0.15, 0)
(0.225, 0)
(0.3, 0)
(0.375, 0)
(0.45, 0)
(0.525, 0)
(0.6, 0)
(0.675, 0)
(0.75, 0)
(0.825, 0)
(0.9, 0)
(0.975, 0)
(1.05, 0)
(1.125, 0)
(1.2, 0)
(1.275, 0)
(1.35, 0)
(1.425, 0)
(1.5, 0)
(1.575, 0)
(1.65, 0)
(1.725, 0)
(1.8, 0)
(1.875, 0)
(1.95, 0)
(2.025, 0)
(2.1, 0)
(2.175, 0)
(2.25, 0)
(2.325, 0)
(2.4, 0)
(2.475, 0)
(2.55, 0)
(2.625, 0)
(2.7, 0)
(2.775, 0)
(2.85, 0)
(2.925, 0)
(3, 0)
(3.075, 0)
(3.15, 0)
(3.225, 0)
(3.3, 0)
(3.375, 0)
(3.45, 0)
(3.525, 0)
(3.6, 0)
(3.675, 0)
(3.75, 0)
(3.825, 0)
(3.9, 0)
(3.975, 0)
(4.05, 0)
(4.125, 0)
(4.2, 0)
(4.275, 0)
(4.35, 0)
(4.425, 0)
(4.5, 0)
(4.575, 0)
(4.65, 0)
(4.725, 0)
(4.8, 0)
(4.875, 0)
(4.95, 0)
(5.025, 0)
(5.1, 0)
(5.175, 0)
(5.25, 0)
(5.325, 0)
(5.4, 0)
(5.475, 0)
(5.55, 0)
(5.625, 0)
(5.7, 0)
(5.775, 0)
(5.85, 0)
(5.925, 0)
(6, 0)
(6.075, 0)
(6.15, 0)
(6.225, 0)
(6.3, 0)
(6.375, 0)
(6.45, 0)
(6.525, 0)
(6.6, 0)
(6.675, 0)
(6.75, 0)
(6.825, 0)
(6.9, 0)
(6.975, 0)
(7.05, 0)
(7.125, 0)
(7.2, 0)
(7.275, 0)
(7.35, 0)
(7.425, 0)
(7.5, 0)
(7.575, 0)
(7.65, 0)
(7.725, 0)
(7.8, 0)
(7.875, 0)
(7.95, 0)
(8.025, 0)
(8.1, 0)
(8.175, 0)
(8.25, 0)
(8.325, 0)
(8.4, 0)
(8.475, 0)
(8.55, 0)
(8.625, 0)
(8.7, 0)
(8.775, 0)
(8.85, 0)
(8.925, 0)
(9, 0)
(9.075, 0)
(9.15, 0)
(9.225, 0)
(9.3, 0)
(9.375, 0)
(9.45, 0)
(9.525, 0)
(9.6, 0)
(9.675, 0)
(9.75, 0)
(9.825, 0)
(9.9, 0)
(9.975, 0)
(10.05, 0)
(10.125, 0)
(10.2, 0)
(10.275, 0)
(10.35, 0)
(10.425, 0)
(10.5, 0)
(10.575, 0)
(10.65, 0)
(10.725, 0)
(10.8, 0)
(10.875, 0)
(10.95, 0)
(11.025, 0)
(11.1, 0)
(11.175, 0)
(11.25, 0)
(11.325, 0)
(11.4, 0)
(11.475, 0)
(11.55, 0)
(11.625, 0)
(11.7, 0)
(11.775, 0)
(11.85, 0)
(11.925, 0)
(12, 0)
(12.075, 0)
(12.15, 0)
(12.225, 0)
(12.3, 0)
(12.375, 0)
(12.45, 0)
(12.525, 0)
(12.6, 0)
(12.675, 0)
(12.75, 0)
(12.825, 0)
(12.9, 0)
(12.975, 0)
(13.05, 0)
(13.125, 0)
(13.2, 0)
(13.275, 0)
(13.35, 0)
(13.425, 0)
(13.5, 0)
(13.575, 0)
(13.65, 0)
(13.725, 0)
(13.8, 0)
(13.875, 0)
(13.95, 0)
(14.025, 0)
(14.1, 0)
(14.175, 0)
(14.25, 0)
(14.325, 0)
(14.4, 0)
(14.475, 0)
(14.55, 0)
(14.625, 0)
(14.7, 0)
(14.775, 0)
(14.85, 0)
(14.925, 0)
(15, 0)
(15.075, 0)
(15.15, 0)
(15.225, 0)
(15.3, 0)
(15.375, 0)
(15.45, 0)
(15.525, 0)
(15.6, 0)
(15.675, 0)
(15.75, 0)
(15.825, 0)
(15.9, 0)
(15.975, 0)
(16.05, 0)
(16.125, 0)
(16.2, 0)
(16.275, 0)
(16.35, 0)
(16.425, 0)
(16.5, 0)
(16.575, 0)
(16.65, 0)
(16.725, 0)
(16.8, 0)
(16.875, 0)
(16.95, 0)
(17.025, 0)
(17.1, 0)
(17.175, 0)
(17.25, 0)
(17.325, 0)
(17.4, 0)
(17.475, 0)
(17.55, 0)
(17.625, 0)
(17.7, 0)
(17.775, 0)
(17.85, 0)
(17.925, 0)
(18, 0)
(18.075, 0)
(18.15, 0)
(18.225, 0)
(18.3, 0)
(18.375, 0)
(18.45, 0)
(18.525, 0)
(18.6, 0)
(18.675, 0)
(18.75, 0)
(18.825, 0)
(18.9, 0)
(18.975, 0)
(19.05, 0)
(19.125, 0)
(19.2, 0)
(19.275, 0)
(19.35, 0)
(19.425, 0)
(19.5, 0)
(19.575, 0)
(19.65, 0)
(19.725, 0)
(19.8, 0)
(19.875, 0)
(19.95, 0)
(20.025, 0)
(20.1, 0)
(20.175, 0)
(20.25, 0)
(20.325, 0)
(20.4, 0)
(20.475, 0)
(20.55, 0)
(20.625, 0)
(20.7, 0)
(20.775, 0)
(20.85, 0)
(20.925, 0)
(21, 0)
(21.075, 0)
(21.15, 0)
(21.225, 0)
(21.3, 0)
(21.375, 0)
(21.45, 0)
(21.525, 0)
(21.6, 0)
(21.675, 0)
(21.75, 0)
(21.825, 0)
(21.9, 0)
(21.975, 0)
(22.05, 0)
(22.125, 0)
(22.2, 0)
(22.275, 0)
(22.35, 0)
(22.425, 0)
(22.5, 0)
(22.575, 0)
(22.65, 0)
(22.725, 0)
(22.8, 0)
(22.875, 0)
(22.95, 0)
(23.025, 0)
(23.1, 0)
(23.175, 0)
(23.25, 0)
(23.325, 0)
(23.4, 0)
(23.475, 0)
(23.55, 0)
(23.625, 0)
(23.7, 0)
(23.775, 0)
(23.85, 0)
(23.925, 0)
(24, 0)
(24.075, 0)
(24.15, 0)
(24.225, 0)
(24.3, 0)
(24.375, 0)
(24.45, 0)
(24.525, 0)
(24.6, 0)
(24.675, 0)
(24.75, 0)
(24.825, 0)
(24.9, 0)
(24.975, 0)
(25.05, 0)
(25.125, 0)
(25.2, 0)
(25.275, 0)
(25.35, 0)
(25.425, 0)
(25.5, 0)
(25.575, 0)
(25.65, 0)
(25.725, 0)
(25.8, 0)
(25.875, 0)
(25.95, 0)
(26.025, 0)
(26.1, 0)
(26.175, 0)
(26.25, 0)
(26.325, 0)
(26.4, 0)
(26.475, 0)
(26.55, 0)
(26.625, 0)
(26.7, 0)
(26.775, 0)
(26.85, 0)
(26.925, 0)
(27, 0)
(27.075, 0)
(27.15, 0)
(27.225, 0)
(27.3, 0)
(27.375, 0)
(27.45, 0)
(27.525, 0)
(27.6, 0)
(27.675, 0)
(27.75, 0)
(27.825, 0)
(27.9, 0)
(27.975, 0)
(28.05, 0)
(28.125, 0)
(28.2, 0)
(28.275, 0)
(28.35, 0)
(28.425, 0)
(28.5, 0)
(28.575, 0)
(28.65, 0)
(28.725, 0)
(28.8, 0)
(28.875, 0)
(28.95, 0)
(29.025, 0)
(29.1, 0)
(29.175, 0)
(29.25, 0)
(29.325, 0)
(29.4, 0)
(29.475, 0)
(29.55, 0)
(29.625, 0)
(29.7, 0)
(29.775, 0)
(29.85, 0)
(29.925, 0)
(30, 0)
(30.075, 0)
(30.15, 0)
(30.225, 0)
(30.3, 0)
(30.375, 0)
(30.45, 0)
(30.525, 0)
(30.6, 0)
(30.675, 0)
(30.75, 0)
(30.825, 0)
(30.9, 0)
(30.975, 0)
(31.05, 0)
(31.125, 0)
(31.2, 0)
(31.275, 0)
(31.35, 0)
(31.425, 0)
(31.5, 0)
(31.575, 0)
(31.65, 0)
(31.725, 0)
(31.8, 0)
(31.875, 0)
(31.95, 0)
(32.025, 0)
(32.1, 0)
(32.175, 0)
(32.25, 0)
(32.325, 0)
(32.4, 0)
(32.475, 0)
(32.55, 0)
(32.625, 0)
(32.7, 0)
(32.775, 0)
(32.85, 0)
(32.925, 0)
(33, 0)
(33.075, 0)
(33.15, 0)
(33.225, 0)
(33.3, 0)
(33.375, 0)
(33.45, 0)
(33.525, 0)
(33.6, 0)
(33.675, 0)
(33.75, 0)
(33.825, 0)
(33.9, 0)
(33.975, 0)
(34.05, 0)
(34.125, 0)
(34.2, 0)
(34.275, 0)
(34.35, 0)
(34.425, 0)
(34.5, 0)
(34.575, 0)
(34.65, 0)
};

==> exp_plots/open_ws_gripper/z.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0)
(0.075, 0.00082429)
(0.15, 0.00151438)
(0.225, 0.00127709)
(0.3, 0.00175761)
(0.375, 0.00129922)
(0.45, 0.00166101)
(0.525, 0.00167014)
(0.6, 0.00129414)
(0.675, 0.000877374)
(0.75, 0.000847586)
(0.825, 0.0012543)
(0.9, 0.000857161)
(0.975, 0.00056161)
(1.05, 0.00105445)
(1.125, 0.000742255)
(1.2, 0.000627403)
(1.275, 0.000763905)
(1.35, 0.000666443)
(1.425, 0.000804264)
(1.5, 0.000435871)
(1.575, 0.000571135)
(1.65, 0.00133739)
(1.725, 0.00215645)
(1.8, 0.00325639)
(1.875, 0.0038573)
(1.95, 0.00448751)
(2.025, 0.00563383)
(2.1, 0.00744551)
(2.175, 0.00910049)
(2.25, 0.00981385)
(2.325, 0.00971618)
(2.4, 0.00948775)
(2.475, 0.00919677)
(2.55, 0.00908934)
(2.625, 0.0066456)
(2.7, 0.00489849)
(2.775, 0.00396435)
(2.85, 0.00161531)
(2.925, 0.00330772)
(3, 0.00743188)
(3.075, 0.0163617)
(3.15, 0.0340653)
(3.225, 0.0480998)
(3.3, 0.0643859)
(3.375, 0.085159)
(3.45, 0.0967342)
(3.525, 0.102594)
(3.6, 0.107437)
(3.675, 0.109476)
(3.75, 0.10759)
(3.825, 0.117578)
(3.9, 0.125245)
(3.975, 0.138495)
(4.05, 0.148012)
(4.125, 0.156372)
(4.2, 0.158718)
(4.275, 0.159338)
(4.35, 0.160918)
(4.425, 0.164315)
(4.5, 0.169998)
(4.575, 0.180438)
(4.65, 0.187898)
(4.725, 0.194833)
(4.8, 0.213018)
(4.875, 0.218703)
(4.95, 0.225586)
(5.025, 0.23025)
(5.1, 0.231269)
(5.175, 0.238727)
(5.25, 0.24196)
(5.325, 0.243487)
(5.4, 0.24233)
(5.475, 0.248457)
(5.55, 0.268947)
(5.625, 0.27632)
(5.7, 0.279135)
(5.775, 0.285353)
(5.85, 0.294426)
(5.925, 0.303947)
(6, 0.310262)
(6.075, 0.318381)
(6.15, 0.324199)
(6.225, 0.32767)
(6.3, 0.332374)
(6.375, 0.333392)
(6.45, 0.349423)
(6.525, 0.361451)
(6.6, 0.37036)
(6.675, 0.38076)
(6.75, 0.383582)
(6.825, 0.38175)
(6.9, 0.384737)
(6.975, 0.385643)
(7.05, 0.384175)
(7.125, 0.384397)
(7.2, 0.392739)
(7.275, 0.397427)
(7.35, 0.411024)
(7.425, 0.417916)
(7.5, 0.425718)
(7.575, 0.437834)
(7.65, 0.445145)
(7.725, 0.463713)
(7.8, 0.477408)
(7.875, 0.48769)
(7.95, 0.495252)
(8.025, 0.497681)
(8.1, 0.502778)
(8.175, 0.504791)
(8.25, 0.505023)
(8.325, 0.505004)
(8.4, 0.503392)
(8.475, 0.503161)
(8.55, 0.508415)
(8.625, 0.508478)
(8.7, 0.505251)
(8.775, 0.503133)
(8.85, 0.503081)
(8.925, 0.50367)
(9, 0.512539)
(9.075, 0.521097)
(9.15, 0.523908)
(9.225, 0.525834)
(9.3, 0.523598)
(9.375, 0.523004)
(9.45, 0.520275)
(9.525, 0.514743)
(9.6, 0.513883)
(9.675, 0.514748)
(9.75, 0.509065)
(9.825, 0.507298)
(9.9, 0.507362)
(9.975, 0.508451)
(10.05, 0.508898)
(10.125, 0.506946)
(10.2, 0.50365)
(10.275, 0.503303)
(10.35, 0.504705)
(10.425, 0.504461)
(10.5, 0.504334)
(10.575, 0.504138)
(10.65, 0.505541)
(10.725, 0.505626)
(10.8, 0.503791)
(10.875, 0.502466)
(10.95, 0.493422)
(11.025, 0.48422)
(11.1, 0.47168)
(11.175, 0.478708)
(11.25, 0.476122)
(11.325, 0.474084)
(11.4, 0.480467)
(11.475, 0.481189)
(11.55, 0.48358)
(11.625, 0.487967)
(11.7, 0.487241)
(11.775, 0.488642)
(11.85, 0.488105)
(11.925, 0.488636)
(12, 0.488045)
(12.075, 0.485999)
(12.15, 0.485225)
(12.225, 0.485949)
(12.3, 0.488406)
(12.375, 0.490319)
(12.45, 0.490078)
(12.525, 0.494626)
(12.6, 0.492189)
(12.675, 0.489695)
(12.75, 0.490089)
(12.825, 0.48972)
(12.9, 0.500602)
(12.975, 0.505294)
(13.05, 0.506435)
(13.125, 0.508707)
(13.2, 0.519609)
(13.275, 0.525969)
(13.35, 0.530657)
(13.425, 0.529813)
(13.5, 0.525646)
(13.575, 0.523528)
(13.65, 0.521932)
(13.725, 0.519709)
(13.8, 0.522274)
(13.875, 0.526678)
(13.95, 0.530546)
(14.025, 0.527163)
(14.1, 0.526541)
(14.175, 0.529588)
(14.25, 0.533036)
(14.325, 0.532655)
(14.4, 0.531701)
(14.475, 0.533957)
(14.55, 0.535389)
(14.625, 0.536879)
(14.7, 0.539275)
(14.775, 0.545305)
(14.85, 0.54242)
(14.925, 0.537229)
(15, 0.535803)
(15.075, 0.527289)
(15.15, 0.521775)
(15.225, 0.514122)
(15.3, 0.513461)
(15.375, 0.516806)
(15.45, 0.514065)
(15.525, 0.510239)
(15.6, 0.506771)
(15.675, 0.504031)
(15.75, 0.503163)
(15.825, 0.495497)
(15.9, 0.493329)
(15.975, 0.489267)
(16.05, 0.496926)
(16.125, 0.501784)
(16.2, 0.506732)
(16.275, 0.510398)
(16.35, 0.516217)
(16.425, 0.519684)
(16.5, 0.522282)
(16.575, 0.524329)
(16.65, 0.524361)
(16.725, 0.525971)
(16.8, 0.529783)
(16.875, 0.531226)
(16.95, 0.532048)
(17.025, 0.534205)
(17.1, 0.538821)
(17.175, 0.538396)
(17.25, 0.539797)
(17.325, 0.538959)
(17.4, 0.534376)
(17.475, 0.523798)
(17.55, 0.515002)
(17.625, 0.511121)
(17.7, 0.512187)
(17.775, 0.507392)
(17.85, 0.503776)
(17.925, 0.503369)
(18, 0.507661)
(18.075, 0.508943)
(18.15, 0.513893)
(18.225, 0.520143)
(18.3, 0.522064)
(18.375, 0.522694)
(18.45, 0.516824)
(18.525, 0.510543)
(18.6, 0.497775)
(18.675, 0.484227)
(18.75, 0.47239)
(18.825, 0.467426)
(18.9, 0.44593)
(18.975, 0.439075)
(19.05, 0.430615)
(19.125, 0.425116)
(19.2, 0.420655)
(19.275, 0.415873)
(19.35, 0.409575)
(19.425, 0.412011)
(19.5, 0.411827)
(19.575, 0.406097)
(19.65, 0.402825)
(19.725, 0.401782)
(19.8, 0.400556)
(19.875, 0.397045)
(19.95, 0.39018)
(20.025, 0.378445)
(20.1, 0.367746)
(20.175, 0.354074)
(20.25, 0.348177)
(20.325, 0.340088)
(20.4, 0.322485)
(20.475, 0.310135)
(20.55, 0.305064)
(20.625, 0.306046)
(20.7, 0.311745)
(20.775, 0.309776)
(20.85, 0.304225)
(20.925, 0.297931)
(21, 0.288945)
(21.075, 0.283301)
(21.15, 0.279087)
(21.225, 0.273791)
(21.3, 0.265962)
(21.375, 0.255237)
(21.45, 0.250233)
(21.525, 0.246257)
(21.6, 0.244332)
(21.675, 0.236803)
(21.75, 0.229048)
(21.825, 0.223241)
(21.9, 0.222436)
(21.975, 0.211851)
(22.05, 0.209274)
(22.125, 0.206371)
(22.2, 0.206413)
(22.275, 0.206478)
(22.35, 0.199509)
(22.425, 0.195256)
(22.5, 0.188119)
(22.575, 0.181944)
(22.65, 0.173289)
(22.725, 0.169342)
(22.8, 0.169199)
(22.875, 0.171105)
(22.95, 0.170701)
(23.025, 0.167793)
(23.1, 0.165624)
(23.175, 0.163316)
(23.25, 0.163044)
(23.325, 0.158037)
(23.4, 0.152876)
(23.475, 0.148089)
(23.55, 0.14092)
(23.625, 0.135456)
(23.7, 0.136807)
(23.775, 0.135658)
(23.85, 0.127064)
(23.925, 0.121598)
(24, 0.119937)
(24.075, 0.118574)
(24.15, 0.120577)
(24.225, 0.119923)
(24.3, 0.119739)
(24.375, 0.119281)
(24.45, 0.110519)
(24.525, 0.112069)
(24.6, 0.115697)
(24.675, 0.116788)
(24.75, 0.116398)
(24.825, 0.115113)
(24.9, 0.113868)
(24.975, 0.111668)
(25.05, 0.11144)
(25.125, 0.110454)
(25.2, 0.0937244)
(25.275, 0.0844902)
(25.35, 0.0779386)
(25.425, 0.0655487)
(25.5, 0.0579741)
(25.575, 0.0526582)
(25.65, 0.0496851)
(25.725, 0.0407983)
(25.8, 0.0419103)
(25.875, 0.0457819)
(25.95, 0.0480142)
(26.025, 0.0462618)
(26.1, 0.0450175)
(26.175, 0.0437154)
(26.25, 0.0447434)
(26.325, 0.0344372)
(26.4, 0.0284586)
(26.475, 0.0245648)
(26.55, 0.0219638)
(26.625, 0.0229852)
(26.7, 0.0267629)
(26.775, 0.0265824)
(26.85, 0.0286065)
(26.925, 0.0216889)
(27, 0.0218682)
(27.075, 0.019387)
(27.15, 0.0182502)
(27.225, 0.0177024)
(27.3, 0.0148936)
(27.375, 0.0154673)
(27.45, 0.0136212)
(27.525, 0.0148808)
(27.6, 0.0169897)
(27.675, 0.0143777)
(27.75, 0.0115556)
(27.825, 0.0106516)
(27.9, 0.0115035)
(27.975, 0.011289)
(28.05, 0.0138455)
(28.125, 0.0147805)
(28.2, 0.0144876)
(28.275, 0.0138475)
(28.35, 0.013439)
(28.425, 0.0140537)
(28.5, 0.0130348)
(28.575, 0.0106349)
(28.65, 0.00961368)
(28.725, 0.00953647)
(28.8, 0.0093427)
(28.875, 0.00911219)
(28.95, 0.00785121)
(29.025, 0.00813964)
(29.1, 0.00949768)
(29.175, 0.0105739)
(29.25, 0.0114493)
(29.325, 0.0111633)
(29.4, 0.0105565)
(29.475, 0.0111022)
(29.55, 0.0096504)
(29.625, 0.00903924)
(29.7, 0.0092174)
(29.775, 0.00930707)
(29.85, 0.00938057)
(29.925, 0.00986875)
(30, 0.0104727)
(30.075, 0.0109172)
(30.15, 0.011726)
(30.225, 0.00919734)
(30.3, 0.00892955)
(30.375, 0.00888846)
(30.45, 0.00851654)
(30.525, 0.00864645)
(30.6, 0.00875599)
(30.675, 0.00885716)
(30.75, 0.00941536)
(30.825, 0.0100687)
(30.9, 0.010429)
(30.975, 0.0114034)
(31.05, 0.0116755)
(31.125, 0.0116023)
(31.2, 0.0116261)
(31.275, 0.0104204)
(31.35, 0.00940084)
(31.425, 0.00914955)
(31.5, 0.00933564)
(31.575, 0.0104205)
(31.65, 0.0109021)
(31.725, 0.0116361)
(31.8, 0.0118196)
(31.875, 0.0115971)
(31.95, 0.0121363)
(32.025, 0.0107346)
(32.1, 0.0102743)
(32.175, 0.0085903)
(32.25, 0.00848157)
(32.325, 0.00671061)
(32.4, 0.0067947)
(32.475, 0.00693677)
(32.55, 0.00870324)
(32.625, 0.00593747)
(32.7, 0.00614987)
(32.775, 0.00328403)
(32.85, 0.00361397)
(32.925, 0.00465113)
(33, 0.0050264)
(33.075, 0.00463019)
(33.15, 0.00549538)
(33.225, 0.0069523)
(33.3, 0.00761428)
(33.375, 0.00806809)
(33.45, 0.00806083)
(33.525, 0.00788708)
(33.6, 0.00794685)
(33.675, 0.00794061)
(33.75, 0.0078968)
(33.825, 0.00773788)
(33.9, 0.00755067)
(33.975, 0.00741151)
(34.05, 0.00700519)
(34.125, 0.00705266)
(34.2, 0.00712861)
(34.275, 0.00725314)
(34.35, 0.00713348)
(34.425, 0.00695936)
(34.5, 0.00693729)
(34.575, 0.00689775)
(34.65, 0.00688254)
};

==> exp_plots/open_ws_gripper/z_des.tex <==
\addplot[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates {
(0, 0)
(0.075, 0)
(0.15, 0)
(0.225, 0)
(0.3, 0)
(0.375, 0)
(0.45, 0)
(0.525, 0)
(0.6, 0)
(0.675, 0)
(0.75, 0)
(0.825, 0)
(0.9, 0)
(0.975, 0)
(1.05, 0)
(1.125, 0)
(1.2, 0)
(1.275, 0)
(1.35, 0)
(1.425, 0)
(1.5, 0)
(1.575, 0)
(1.65, 0)
(1.725, 0)
(1.8, 0)
(1.875, 0)
(1.95, 0)
(2.025, 0)
(2.1, 0)
(2.175, 0)
(2.25, 0)
(2.325, 0)
(2.4, 0)
(2.475, 0)
(2.55, 0)
(2.625, 0)
(2.7, 0)
(2.775, 0)
(2.85, 0)
(2.925, 0)
(3, 0)
(3.075, 0)
(3.15, 0)
(3.225, 0)
(3.3, 0)
(3.375, 0)
(3.45, 0)
(3.525, 0)
(3.6, 0)
(3.675, 0)
(3.75, 0)
(3.825, 0)
(3.9, 0)
(3.975, 0)
(4.05, 0)
(4.125, 0)
(4.2, 0)
(4.275, 0)
(4.35, 0)
(4.425, 0)
(4.5, 0)
(4.575, 0)
(4.65, 0)
(4.725, 0)
(4.8, 0)
(4.875, 0)
(4.95, 0)
(5.025, 0)
(5.1, 0)
(5.175, 0)
(5.25, 0)
(5.325, 0)
(5.4, 0)
(5.475, 0)
(5.55, 0)
(5.625, 0)
(5.7, 0)
(5.775, 0)
(5.85, 0)
(5.925, 0)
(6, 0)
(6.075, 0)
(6.15, 0)
(6.225, 0)
(6.3, 0)
(6.375, 0)
(6.45, 0)
(6.525, 0)
(6.6, 0)
(6.675, 0)
(6.75, 0)
(6.825, 0)
(6.9, 0)
(6.975, 0)
(7.05, 0)
(7.125, 0)
(7.2, 0)
(7.275, 0)
(7.35, 0)
(7.425, 0)
(7.5, 0)
(7.575, 0)
(7.65, 0)
(7.725, 0)
(7.8, 0.5)
(7.875, 0.5)
(7.95, 0.5)
(8.025, 0.5)
(8.1, 0.5)
(8.175, 0.5)
(8.25, 0.5)
(8.325, 0.5)
(8.4, 0.5)
(8.475, 0.5)
(8.55, 0.5)
(8.625, 0.5)
(8.7, 0.5)
(8.775, 0.5)
(8.85, 0.5)
(8.925, 0.5)
(9, 0.5)
(9.075, 0.5)
(9.15, 0.5)
(9.225, 0.5)
(9.3, 0.5)
(9.375, 0.5)
(9.45, 0.5)
(9.525, 0.5)
(9.6, 0.5)
(9.675, 0.5)
(9.75, 0.5)
(9.825, 0.5)
(9.9, 0.5)
(9.975, 0.5)
(10.05, 0.5)
(10.125, 0.5)
(10.2, 0.5)
(10.275, 0.5)
(10.35, 0.5)
(10.425, 0.5)
(10.5, 0.5)
(10.575, 0.5)
(10.65, 0.5)
(10.725, 0.5)
(10.8, 0.5)
(10.875, 0.5)
(10.95, 0.5)
(11.025, 0.5)
(11.1, 0.5)
(11.175, 0.5)
(11.25, 0.5)
(11.325, 0.5)
(11.4, 0.5)
(11.475, 0.5)
(11.55, 0.5)
(11.625, 0.5)
(11.7, 0.5)
(11.775, 0.5)
(11.85, 0.5)
(11.925, 0.5)
(12, 0.5)
(12.075, 0.5)
(12.15, 0.5)
(12.225, 0.5)
(12.3, 0.5)
(12.375, 0.5)
(12.45, 0.5)
(12.525, 0.5)
(12.6, 0.5)
(12.675, 0.5)
(12.75, 0.5)
(12.825, 0.5)
(12.9, 0.5)
(12.975, 0.5)
(13.05, 0.5)
(13.125, 0.5)
(13.2, 0.5)
(13.275, 0.5)
(13.35, 0.5)
(13.425, 0.5)
(13.5, 0.5)
(13.575, 0.5)
(13.65, 0.5)
(13.725, 0.5)
(13.8, 0.5)
(13.875, 0.5)
(13.95, 0.5)
(14.025, 0.5)
(14.1, 0.5)
(14.175, 0.5)
(14.25, 0.5)
(14.325, 0.5)
(14.4, 0.5)
(14.475, 0.5)
(14.55, 0.5)
(14.625, 0.5)
(14.7, 0.5)
(14.775, 0.5)
(14.85, 0.5)
(14.925, 0.5)
(15, 0.5)
(15.075, 0.5)
(15.15, 0.5)
(15.225, 0.5)
(15.3, 0.5)
(15.375, 0.5)
(15.45, 0.5)
(15.525, 0.5)
(15.6, 0.5)
(15.675, 0.5)
(15.75, 0.5)
(15.825, 0.5)
(15.9, 0.5)
(15.975, 0.5)
(16.05, 0.5)
(16.125, 0.5)
(16.2, 0.5)
(16.275, 0.5)
(16.35, 0.5)
(16.425, 0.5)
(16.5, 0.5)
(16.575, 0.5)
(16.65, 0.5)
(16.725, 0.5)
(16.8, 0.5)
(16.875, 0.5)
(16.95, 0.5)
(17.025, 0.5)
(17.1, 0.5)
(17.175, 0.5)
(17.25, 0.5)
(17.325, 0.5)
(17.4, 0.5)
(17.475, 0.5)
(17.55, 0.5)
(17.625, 0.5)
(17.7, 0)
(17.775, 0)
(17.85, 0)
(17.925, 0)
(18, 0)
(18.075, 0)
(18.15, 0)
(18.225, 0)
(18.3, 0)
(18.375, 0)
(18.45, 0)
(18.525, 0)
(18.6, 0)
(18.675, 0)
(18.75, 0)
(18.825, 0)
(18.9, 0)
(18.975, 0)
(19.05, 0)
(19.125, 0)
(19.2, 0)
(19.275, 0)
(19.35, 0)
(19.425, 0)
(19.5, 0)
(19.575, 0)
(19.65, 0)
(19.725, 0)
(19.8, 0)
(19.875, 0)
(19.95, 0)
(20.025, 0)
(20.1, 0)
(20.175, 0)
(20.25, 0)
(20.325, 0)
(20.4, 0)
(20.475, 0)
(20.55, 0)
(20.625, 0)
(20.7, 0)
(20.775, 0)
(20.85, 0)
(20.925, 0)
(21, 0)
(21.075, 0)
(21.15, 0)
(21.225, 0)
(21.3, 0)
(21.375, 0)
(21.45, 0)
(21.525, 0)
(21.6, 0)
(21.675, 0)
(21.75, 0)
(21.825, 0)
(21.9, 0)
(21.975, 0)
(22.05, 0)
(22.125, 0)
(22.2, 0)
(22.275, 0)
(22.35, 0)
(22.425, 0)
(22.5, 0)
(22.575, 0)
(22.65, 0)
(22.725, 0)
(22.8, 0)
(22.875, 0)
(22.95, 0)
(23.025, 0)
(23.1, 0)
(23.175, 0)
(23.25, 0)
(23.325, 0)
(23.4, 0)
(23.475, 0)
(23.55, 0)
(23.625, 0)
(23.7, 0)
(23.775, 0)
(23.85, 0)
(23.925, 0)
(24, 0)
(24.075, 0)
(24.15, 0)
(24.225, 0)
(24.3, 0)
(24.375, 0)
(24.45, 0)
(24.525, 0)
(24.6, 0)
(24.675, 0)
(24.75, 0)
(24.825, 0)
(24.9, 0)
(24.975, 0)
(25.05, 0)
(25.125, 0)
(25.2, 0)
(25.275, 0)
(25.35, 0)
(25.425, 0)
(25.5, 0)
(25.575, 0)
(25.65, 0)
(25.725, 0)
(25.8, 0)
(25.875, 0)
(25.95, 0)
(26.025, 0)
(26.1, 0)
(26.175, 0)
(26.25, 0)
(26.325, 0)
(26.4, 0)
(26.475, 0)
(26.55, 0)
(26.625, 0)
(26.7, 0)
(26.775, 0)
(26.85, 0)
(26.925, 0)
(27, 0)
(27.075, 0)
(27.15, 0)
(27.225, 0)
(27.3, 0)
(27.375, 0)
(27.45, 0)
(27.525, 0)
(27.6, 0)
(27.675, 0)
(27.75, 0)
(27.825, 0)
(27.9, 0)
(27.975, 0)
(28.05, 0)
(28.125, 0)
(28.2, 0)
(28.275, 0)
(28.35, 0)
(28.425, 0)
(28.5, 0)
(28.575, 0)
(28.65, 0)
(28.725, 0)
(28.8, 0)
(28.875, 0)
(28.95, 0)
(29.025, 0)
(29.1, 0)
(29.175, 0)
(29.25, 0)
(29.325, 0)
(29.4, 0)
(29.475, 0)
(29.55, 0)
(29.625, 0)
(29.7, 0)
(29.775, 0)
(29.85, 0)
(29.925, 0)
(30, 0)
(30.075, 0)
(30.15, 0)
(30.225, 0)
(30.3, 0)
(30.375, 0)
(30.45, 0)
(30.525, 0)
(30.6, 0)
(30.675, 0)
(30.75, 0)
(30.825, 0)
(30.9, 0)
(30.975, 0)
(31.05, 0)
(31.125, 0)
(31.2, 0)
(31.275, 0)
(31.35, 0)
(31.425, 0)
(31.5, 0)
(31.575, 0)
(31.65, 0)
(31.725, 0)
(31.8, 0)
(31.875, 0)
(31.95, 0)
(32.025, 0)
(32.1, 0)
(32.175, 0)
(32.25, 0)
(32.325, 0)
(32.4, 0)
(32.475, 0)
(32.55, 0)
(32.625, 0)
(32.7, 0)
(32.775, 0)
(32.85, 0)
(32.925, 0)
(33, 0)
(33.075, 0)
(33.15, 0)
(33.225, 0)
(33.3, 0)
(33.375, 0)
(33.45, 0)
(33.525, 0)
(33.6, 0)
(33.675, 0)
(33.75, 0)
(33.825, 0)
(33.9, 0)
(33.975, 0)
(34.05, 0)
(34.125, 0)
(34.2, 0)
(34.275, 0)
(34.35, 0)
(34.425, 0)
(34.5, 0)
(34.575, 0)
(34.65, 0)
};

==> exp_plots/open_ws_wind/az.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0)
(0.1, 0.00906026)
(0.2, 0.00786329)
(0.3, -0.00614316)
(0.4, -0.0112824)
(0.5, -0.0103994)
(0.6, -0.0165858)
(0.7, -0.00386357)
(0.8, 0.0041621)
(0.9, 0.00689768)
(1, 0.00980543)
(1.1, -0.00459731)
(1.2, -0.00780367)
(1.3, -0.00885787)
(1.4, -0.00124282)
(1.5, -0.0220852)
(1.6, -0.0378413)
(1.7, -0.0417555)
(1.8, -0.0380299)
(1.9, -0.0146258)
(2, 0.00396254)
(2.1, -0.0191515)
(2.2, -0.0127005)
(2.3, -0.00588708)
(2.4, -0.0153284)
(2.5, -0.0180946)
(2.6, 0.0046746)
(2.7, 0.0592588)
(2.8, 0.202879)
(2.9, 0.326535)
(3, 0.374515)
(3.1, 0.307181)
(3.2, 0.198772)
(3.3, 0.137034)
(3.4, 0.153967)
(3.5, 0.189028)
(3.6, 0.187519)
(3.7, 0.208793)
(3.8, 0.14203)
(3.9, -0.0676591)
(4, -0.257565)
(4.1, -0.314775)
(4.2, -0.150575)
(4.3, 0.0376796)
(4.4, 0.0602682)
(4.5, -0.0884169)
(4.6, -0.206185)
(4.7, -0.117012)
(4.8, 0.121648)
(4.9, 0.263842)
(5, 0.166322)
(5.1, -0.0416491)
(5.2, -0.203299)
(5.3, -0.198257)
(5.4, -0.0677923)
(5.5, 0.0735387)
(5.6, 0.122862)
(5.7, 0.0871456)
(5.8, 0.05653)
(5.9, 0.0728361)
(6, 0.0568014)
(6.1, -0.00121576)
(6.2, -0.0862912)
(6.3, -0.0754888)
(6.4, 0.0813238)
(6.5, 0.179707)
(6.6, 0.0792877)
(6.7, -0.157822)
(6.8, -0.22555)
(6.9, -0.0689492)
(7, 0.0950122)
(7.1, 0.069192)
(7.2, -0.096502)
(7.3, -0.277197)
(7.4, -0.275234)
(7.5, -0.143144)
(7.6, -0.0801111)
(7.7, -0.140228)
(7.8, -0.208717)
(7.9, -0.125767)
(8, 0.0417556)
(8.1, 0.318094)
(8.2, 0.377183)
(8.3, 0.17735)
(8.4, -0.0931941)
(8.5, -0.217981)
(8.6, -0.205758)
(8.7, -0.0962784)
(8.8, -0.00200766)
(8.9, 0.142449)
(9, 0.279659)
(9.1, 0.311118)
(9.2, 0.266499)
(9.3, 0.184452)
(9.4, 0.0665213)
(9.5, -0.00594077)
(9.6, -0.0504043)
(9.7, -0.0332407)
(9.8, 0.0288223)
(9.9, 0.0732978)
(10, 0.0326064)
(10.1, -0.0292085)
(10.2, -0.0998404)
(10.3, -0.199052)
(10.4, -0.198035)
(10.5, -0.0841674)
(10.6, 0.0577043)
(10.7, 0.139028)
(10.8, 0.169622)
(10.9, 0.187518)
(11, 0.179578)
(11.1, 0.0782354)
(11.2, 0.026703)
(11.3, 0.0342224)
(11.4, 0.028869)
(11.5, 0.0309057)
(11.6, 0.00148871)
(11.7, -0.0443274)
(11.8, -0.0562845)
(11.9, -0.0319038)
(12, 0.00942064)
(12.1, -0.00637751)
(12.2, -0.0624604)
(12.3, -0.119404)
(12.4, -0.116519)
(12.5, -0.150108)
(12.6, -0.200539)
(12.7, -0.175648)
(12.8, -0.152506)
(12.9, -0.0883396)
(13, -0.0187152)
(13.1, 0.0401482)
(13.2, 0.0745019)
(13.3, 0.105321)
(13.4, 0.0709263)
(13.5, -0.0584843)
(13.6, -0.105323)
(13.7, -0.0172537)
(13.8, 0.112718)
(13.9, 0.12869)
(14, 0.0259137)
(14.1, -0.088271)
(14.2, -0.0852872)
(14.3, 0.0116075)
(14.4, 0.146383)
(14.5, 0.204402)
(14.6, 0.138191)
(14.7, -0.0360606)
(14.8, -0.169412)
(14.9, -0.160442)
(15, -0.0249371)
(15.1, 0.0931368)
(15.2, 0.103624)
(15.3, -0.0351204)
(15.4, -0.267337)
(15.5, -0.415689)
(15.6, -0.257712)
(15.7, 0.0881813)
(15.8, 0.361855)
(15.9, 0.295638)
(16, 0.0491871)
(16.1, -0.177803)
(16.2, -0.240527)
(16.3, -0.0338663)
(16.4, 0.223191)
(16.5, 0.316576)
(16.6, 0.215248)
(16.7, -0.00939131)
(16.8, -0.173051)
(16.9, -0.213062)
(17, -0.185047)
(17.1, -0.123054)
(17.2, -0.0410578)
(17.3, 0.0145527)
(17.4, 0.0258761)
(17.5, 0.00184166)
(17.6, -0.0615432)
(17.7, -0.0568011)
(17.8, -0.0396399)
(17.9, -0.0758843)
(18, -0.0391089)
(18.1, 0.0474887)
(18.2, 0.11774)
(18.3, 0.170799)
(18.4, 0.118567)
(18.5, 0.0190126)
(18.6, 0.0199134)
(18.7, 0.0623675)
(18.8, 0.112419)
(18.9, 0.0830737)
(19, -0.013082)
(19.1, -0.0279014)
(19.2, -0.00445344)
(19.3, 0.0246845)
(19.4, 0.0363803)
(19.5, 0.0176226)
(19.6, 0.0207139)
(19.7, 0.0662034)
(19.8, 0.109427)
(19.9, 0.0931592)
(20, -0.0340308)
(20.1, -0.170646)
(20.2, -0.228438)
(20.3, -0.153316)
(20.4, -0.0521098)
(20.5, 0.0423557)
(20.6, 0.137175)
(20.7, 0.17863)
(20.8, 0.167675)
(20.9, 0.0921268)
(21, -0.0201067)
(21.1, -0.172917)
(21.2, -0.245711)
(21.3, -0.199311)
(21.4, -0.0289308)
(21.5, 0.0242032)
(21.6, -0.0685036)
(21.7, -0.182561)
(21.8, -0.160055)
(21.9, -0.0071352)
(22, 0.123706)
(22.1, 0.113671)
(22.2, 0.0337729)
(22.3, -0.0755413)
(22.4, -0.0963373)
(22.5, -0.035933)
(22.6, 0.0176002)
(22.7, 0.114478)
(22.8, 0.133185)
(22.9, 0.0834329)
(23, 0.0216986)
(23.1, -0.0730704)
(23.2, -0.108485)
(23.3, -0.0325511)
(23.4, 0.141557)
(23.5, 0.288619)
(23.6, 0.389088)
(23.7, 0.336396)
(23.8, 0.112786)
(23.9, -0.178671)
(24, -0.280867)
(24.1, -0.187553)
(24.2, -0.0810547)
(24.3, -0.00655059)
(24.4, 0.005941)
(24.5, -0.0230987)
(24.6, -0.00361815)
(24.7, 0.0715023)
(24.8, 0.218519)
(24.9, 0.297198)
(25, 0.202407)
(25.1, 0.0641661)
(25.2, -0.0459531)
(25.3, -0.0836494)
(25.4, -0.0335356)
(25.5, 0.0426345)
(25.6, 0.0531337)
(25.7, 0.0342331)
(25.8, 0.0409789)
(25.9, 0.00345965)
(26, -0.0440402)
(26.1, 0.025781)
(26.2, 0.108496)
(26.3, 0.120937)
(26.4, 0.0164768)
(26.5, -0.0353294)
(26.6, -0.0750562)
(26.7, -0.156144)
(26.8, -0.213818)
(26.9, -0.207805)
(27, -0.15264)
(27.1, -0.128373)
(27.2, -0.107901)
(27.3, -0.0363292)
(27.4, -0.0031166)
(27.5, 0.0234262)
(27.6, -0.0485936)
(27.7, -0.0774661)
(27.8, -0.0217672)
(27.9, 0.110324)
(28, 0.089587)
(28.1, -0.0361849)
(28.2, -0.0969309)
(28.3, -0.117886)
(28.4, -0.0289877)
(28.5, 0.136032)
(28.6, 0.248746)
(28.7, 0.200708)
(28.8, -0.0199218)
(28.9, -0.238221)
(29, -0.179418)
(29.1, 0.0948494)
(29.2, 0.343995)
(29.3, 0.316057)
(29.4, 0.0932711)
(29.5, -0.123038)
(29.6, -0.159541)
(29.7, -0.051374)
(29.8, 0.00857641)
(29.9, -0.0818775)
(30, -0.179397)
(30.1, -0.130879)
(30.2, 0.0443885)
(30.3, 0.146374)
(30.4, 0.11845)
(30.5, 0.0660011)
(30.6, -0.0368708)
(30.7, -0.0802726)
(30.8, -0.0360518)
(30.9, 0.0824702)
(31, 0.146983)
(31.1, 0.0261611)
(31.2, -0.108005)
(31.3, -0.0984853)
(31.4, 0.00348373)
(31.5, 0.111998)
(31.6, 0.0781941)
(31.7, -0.0206089)
(31.8, -0.0482775)
(31.9, 0.0417003)
(32, 0.0802444)
(32.1, -0.0043063)
(32.2, -0.110307)
(32.3, -0.155625)
(32.4, -0.0994461)
(32.5, 0.0372038)
(32.6, 0.0950722)
(32.7, 0.0840259)
(32.8, 0.0289365)
(32.9, 0.00520113)
(33, 0.0217286)
(33.1, 0.0164267)
(33.2, -0.0295947)
(33.3, -0.0847142)
(33.4, -0.119489)
(33.5, -0.0876076)
(33.6, 0.00710252)
(33.7, 0.0148921)
(33.8, -0.0777201)
(33.9, -0.068731)
(34, 0.144328)
(34.1, 0.260739)
(34.2, 0.0410462)
(34.3, -0.0302495)
(34.4, 0.00380591)
(34.5, -0.0534261)
(34.6, -0.0283421)
(34.7, -0.00564179)
(34.8, -0.0297657)
(34.9, -0.0153822)
(35, -0.0197915)
(35.1, -0.0141277)
(35.2, 0.00268288)
(35.3, 0.0109441)
(35.4, 0.0116329)
(35.5, 0.0173852)
(35.6, 0.0139799)
(35.7, 0.0185881)
(35.8, 0.026327)
(35.9, 0.0320585)
(36, 0.0351056)
(36.1, 0.0253756)
(36.2, 0.0245644)
(36.3, 0.00735104)
(36.4, -0.0162199)
(36.5, -0.0146948)
(36.6, -0.00756134)
(36.7, -0.0081671)
(36.8, -0.00245193)
(36.9, 0.00491718)
(37, 0.0089213)
(37.1, 0.00681479)
(37.2, 0.0131451)
(37.3, -0.000992954)
(37.4, -0.0030298)
(37.5, -0.00888482)
(37.6, -0.0183508)
(37.7, -0.0283497)
(37.8, -0.0155163)
(37.9, -0.00225201)
(38, 0.0175445)
(38.1, 0.0178762)
(38.2, 0.0127512)
(38.3, 0.00801146)
(38.4, 0.00267882)
(38.5, 0.00851204)
(38.6, 0.00557646)
(38.7, 0.00111099)
(38.8, 0.00990307)
(38.9, 0.0212726)
(39, 0.00728909)
(39.1, -0.00880659)
(39.2, -0.0167168)
(39.3, -0.0227168)
(39.4, -0.00268218)
(39.5, 0.00931874)
(39.6, 0.0136145)
(39.7, 0.00787726)
(39.8, -0.0184741)
(39.9, -0.0338982)
(40, -0.0212001)
(40.1, -0.0225734)
(40.2, -0.0084727)
(40.3, 0.0067056)
(40.4, 0.00714718)
(40.5, 0.00549962)
(40.6, 0.00403076)
(40.7, -0.000155488)
(40.8, -0.0202035)
(40.9, -0.0298756)
(41, -0.0230333)
(41.1, -0.0195588)
(41.2, -0.0224573)
(41.3, -0.0188865)
(41.4, -0.00625643)
(41.5, -0.00605883)
(41.6, -0.00372373)
(41.7, -0.0235616)
(41.8, -0.0165891)
(41.9, 0.000565569)
(42, 0.00168519)
(42.1, -0.000140637)
(42.2, -0.00542662)
};

==> exp_plots/open_ws_wind/az_des.tex <==
\addplot[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates {
(0, 0)
(0.1, -0.00388304)
(0.2, -0.00418727)
(0.3, -0.00180161)
(0.4, 0.00269348)
(0.5, 0.00449757)
(0.6, 0.00535406)
(0.7, 0.00481591)
(0.8, 0.00087807)
(0.9, -0.00146997)
(1, -0.00172123)
(1.1, 0.230578)
(1.2, 0.344537)
(1.3, 0.417619)
(1.4, 0.449854)
(1.5, 0.440261)
(1.6, 0.425008)
(1.7, 0.430175)
(1.8, 0.436292)
(1.9, 0.442467)
(2, 0.448508)
(2.1, 0.449055)
(2.2, 0.45734)
(2.3, 0.459668)
(2.4, 0.465496)
(2.5, 0.472734)
(2.6, 0.475926)
(2.7, 0.458832)
(2.8, 0.427488)
(2.9, 0.360605)
(3, 0.276991)
(3.1, 0.246077)
(3.2, 0.250267)
(3.3, 0.251162)
(3.4, 0.235183)
(3.5, 0.236596)
(3.6, 0.198558)
(3.7, 0.0213626)
(3.8, -0.138734)
(3.9, -0.160781)
(4, -0.10058)
(4.1, -0.00550449)
(4.2, 0.0181821)
(4.3, -0.0233591)
(4.4, 0.0358831)
(4.5, 0.069855)
(4.6, 0.0736719)
(4.7, 0.0823778)
(4.8, 0.0116148)
(4.9, -0.041028)
(5, -0.0452671)
(5.1, -0.0615575)
(5.2, -0.0420291)
(5.3, 0.0104552)
(5.4, 0.0768796)
(5.5, 0.0528139)
(5.6, 0.0501834)
(5.7, 0.0700767)
(5.8, 0.0147483)
(5.9, -0.0564109)
(6, -0.0709525)
(6.1, -0.0407348)
(6.2, 0.0399724)
(6.3, 0.0873519)
(6.4, -0.0337307)
(6.5, -0.181772)
(6.6, -0.173287)
(6.7, -0.0912546)
(6.8, -0.0685229)
(6.9, -0.0885877)
(7, -0.115103)
(7.1, -0.139191)
(7.2, -0.117635)
(7.3, -0.0515716)
(7.4, -0.0510848)
(7.5, -0.120815)
(7.6, -0.143835)
(7.7, -0.0966127)
(7.8, 0.0249487)
(7.9, 0.218016)
(8, 0.295178)
(8.1, 0.20125)
(8.2, 0.0769973)
(8.3, -0.0423209)
(8.4, -0.107158)
(8.5, -0.100287)
(8.6, -0.0679988)
(8.7, -0.053264)
(8.8, 0.0416627)
(8.9, 0.184489)
(9, 0.219482)
(9.1, 0.185558)
(9.2, 0.138615)
(9.3, 0.0756563)
(9.4, -0.0195776)
(9.5, -0.0398319)
(9.6, 0.072484)
(9.7, 0.0931275)
(9.8, 0.0953963)
(9.9, -0.0107954)
(10, -0.0726788)
(10.1, -0.133091)
(10.2, -0.135263)
(10.3, -0.069553)
(10.4, -0.0143664)
(10.5, 0.0079739)
(10.6, 0.0846188)
(10.7, 0.104778)
(10.8, 0.0815826)
(10.9, 0.0556138)
(11, 0.028202)
(11.1, 0.0667805)
(11.2, 0.0738514)
(11.3, 0.050402)
(11.4, 0.0209656)
(11.5, 0.00237871)
(11.6, -0.0206199)
(11.7, -0.0255119)
(11.8, -0.0199926)
(11.9, -0.037568)
(12, -0.0841666)
(12.1, -0.0939065)
(12.2, -0.0948481)
(12.3, -0.114549)
(12.4, -0.13582)
(12.5, -0.141519)
(12.6, -0.136984)
(12.7, -0.112823)
(12.8, -0.0743612)
(12.9, -0.0362862)
(13, 0.0200622)
(13.1, 0.0435849)
(13.2, 0.0433359)
(13.3, -0.0126698)
(13.4, -0.0190048)
(13.5, 0.0178365)
(13.6, 0.0587204)
(13.7, 0.060682)
(13.8, 0.041274)
(13.9, 0.0431353)
(14, 0.0582409)
(14.1, 0.0664616)
(14.2, 0.107855)
(14.3, 0.0943008)
(14.4, 0.0761109)
(14.5, 0.00822466)
(14.6, -0.0465021)
(14.7, -0.0191615)
(14.8, -0.0320444)
(14.9, -0.0408179)
(15, -0.0327997)
(15.1, -0.0347011)
(15.2, -0.0769879)
(15.3, -0.139437)
(15.4, -0.117601)
(15.5, 0.0135115)
(15.6, 0.106237)
(15.7, 0.0886624)
(15.8, 0.0320641)
(15.9, 7.96142e-05)
(16, 0.00868363)
(16.1, 0.042401)
(16.2, 0.0622193)
(16.3, 0.00575065)
(16.4, 0.00680092)
(16.5, -0.0011813)
(16.6, -0.00701527)
(16.7, -0.0778193)
(16.8, -0.120234)
(16.9, -0.131057)
(17, -0.131809)
(17.1, -0.0988721)
(17.2, -0.0702857)
(17.3, -0.0510566)
(17.4, -0.00629248)
(17.5, -0.0253239)
(17.6, -0.0272484)
(17.7, -0.0116401)
(17.8, -0.00073707)
(17.9, 0.0219286)
(18, 0.0435465)
(18.1, 0.0802679)
(18.2, 0.109458)
(18.3, 0.0787229)
(18.4, 0.066739)
(18.5, 0.0725498)
(18.6, 0.0762162)
(18.7, 0.063314)
(18.8, 0.05509)
(18.9, 0.0304792)
(19, 0.0142641)
(19.1, 0.00455616)
(19.2, -0.0133715)
(19.3, -0.0321476)
(19.4, 0.0927197)
(19.5, 0.122367)
(19.6, 0.0674148)
(19.7, 0.050674)
(19.8, -0.0494734)
(19.9, -0.146179)
(20, -0.147047)
(20.1, -0.0626596)
(20.2, 0.0124415)
(20.3, 0.0935981)
(20.4, 0.131813)
(20.5, 0.110365)
(20.6, 0.0538265)
(20.7, -0.00010086)
(20.8, -0.0437482)
(20.9, -0.140444)
(21, -0.163837)
(21.1, -0.103093)
(21.2, -0.061255)
(21.3, -0.060818)
(21.4, -0.0771767)
(21.5, -0.1003)
(21.6, -0.0693319)
(21.7, -0.0150985)
(21.8, 0.0315003)
(21.9, 0.0303865)
(22, -0.0259023)
(22.1, -0.0404035)
(22.2, -0.0536814)
(22.3, -0.0388451)
(22.4, 0.00258118)
(22.5, 0.0276205)
(22.6, 0.086631)
(22.7, 0.0790974)
(22.8, 0.0536821)
(22.9, 0.036878)
(23, 0.0355412)
(23.1, 0.0506899)
(23.2, 0.120846)
(23.3, 0.194318)
(23.4, 0.178519)
(23.5, 0.168013)
(23.6, 0.106911)
(23.7, -0.0638718)
(23.8, -0.1104)
(23.9, -0.0934392)
(24, -0.126894)
(24.1, -0.125849)
(24.2, -0.0810573)
(24.3, -0.00466862)
(24.4, 0.0166068)
(24.5, 0.0577807)
(24.6, 0.107424)
(24.7, 0.171778)
(24.8, 0.168321)
(24.9, 0.114244)
(25, 0.0503885)
(25.1, 0.0409865)
(25.2, 0.0473863)
(25.3, 0.0472122)
(25.4, 0.050656)
(25.5, 0.056768)
(25.6, 0.0825588)
(25.7, 0.0593321)
(25.8, 0.0512912)
(25.9, 0.0450931)
(26, 0.0268681)
(26.1, 0.0137453)
(26.2, -0.00990776)
(26.3, -0.0199167)
(26.4, -0.0863249)
(26.5, -0.100521)
(26.6, -0.156903)
(26.7, -0.169269)
(26.8, -0.154327)
(26.9, -0.127992)
(27, -0.109489)
(27.1, -0.0675668)
(27.2, -0.0746315)
(27.3, 0.000563562)
(27.4, -0.000551406)
(27.5, 0.0186203)
(27.6, -0.00416528)
(27.7, -0.0564111)
(27.8, -0.0678642)
(27.9, -0.0784265)
(28, -0.0919606)
(28.1, -0.0520356)
(28.2, 0.0163983)
(28.3, 0.0540617)
(28.4, 0.0885502)
(28.5, 0.0600803)
(28.6, 0.00961756)
(28.7, -0.0530778)
(28.8, 0.00929794)
(28.9, 0.158214)
(29, 0.251582)
(29.1, 0.198583)
(29.2, 0.112493)
(29.3, 0.0526622)
(29.4, -0.0229958)
(29.5, -0.048515)
(29.6, -0.0613556)
(29.7, -0.112074)
(29.8, -0.137884)
(29.9, -0.09785)
(30, -0.014682)
(30.1, 0.0274879)
(30.2, 0.0264086)
(30.3, 0.0147824)
(30.4, -0.00946402)
(30.5, -0.0214045)
(30.6, 0.00164282)
(30.7, 0.0327593)
(30.8, 0.0379121)
(30.9, 0.0105748)
(31, -0.0438998)
(31.1, -0.0689525)
(31.2, -0.0441801)
(31.3, -0.00732599)
(31.4, 0.0287142)
(31.5, 0.0398457)
(31.6, 0.0336692)
(31.7, 0.0300769)
(31.8, -0.00955727)
(31.9, -0.103819)
(32, -0.117537)
(32.1, -0.101215)
(32.2, -0.073942)
(32.3, -0.0330386)
(32.4, -0.0131193)
(32.5, -0.0146286)
(32.6, -0.00506915)
(32.7, -0.00718671)
(32.8, 0.0179626)
(32.9, 0.00620508)
(33, -0.0300429)
(33.1, -0.076214)
(33.2, -0.100734)
(33.3, -0.0731501)
(33.4, -0.0267613)
(33.5, 0.00698433)
(33.6, -0.00851846)
(33.7, -0.0493083)
(33.8, -0.0499054)
(33.9, 0.0651572)
(34, 0.0444038)
(34.1, -0.0736278)
(34.2, -0.161873)
(34.3, -0.184508)
(34.4, -0.218331)
(34.5, -0.250585)
(34.6, -0.221112)
(34.7, -0.131308)
(34.8, -0.11334)
(34.9, -0.147702)
(35, -0.165946)
(35.1, -0.185071)
(35.2, -0.216531)
(35.3, -0.244603)
(35.4, -0.254976)
(35.5, -0.256006)
(35.6, -0.225658)
(35.7, -0.212915)
(35.8, -0.213175)
(35.9, -0.223439)
(36, -0.235525)
(36.1, -0.244539)
(36.2, -0.251178)
(36.3, -0.241375)
(36.4, -0.238131)
(36.5, -0.236692)
(36.6, -0.222693)
(36.7, -0.221174)
(36.8, -0.240742)
(36.9, -0.277909)
(37, -0.283995)
(37.1, -0.286941)
(37.2, -0.283992)
(37.3, -0.2736)
(37.4, -0.270216)
(37.5, -0.267727)
(37.6, -0.269393)
(37.7, -0.270735)
(37.8, -0.273843)
(37.9, -0.280065)
(38, -0.288529)
(38.1, -0.297587)
(38.2, -0.305498)
(38.3, -0.307668)
(38.4, -0.306814)
(38.5, -0.308286)
(38.6, -0.309187)
(38.7, -0.30739)
(38.8, -0.311339)
(38.9, -0.323945)
(39, -0.330345)
(39.1, -0.328817)
(39.2, -0.326992)
(39.3, -0.324788)
(39.4, -0.322197)
(39.5, -0.302642)
(39.6, -0.29118)
(39.7, -0.293941)
(39.8, -0.300196)
(39.9, -0.303065)
(40, -0.307308)
(40.1, -0.314293)
(40.2, -0.319242)
(40.3, -0.328257)
(40.4, -0.339062)
(40.5, -0.348628)
(40.6, -0.356388)
(40.7, -0.363375)
(40.8, -0.361817)
(40.9, -0.356254)
(41, -0.350425)
(41.1, -0.350328)
(41.2, -0.352265)
(41.3, -0.352322)
(41.4, -0.357446)
(41.5, -0.364264)
(41.6, -0.369223)
(41.7, -0.376272)
(41.8, -0.378701)
(41.9, -0.382457)
(42, -0.389115)
(42.1, -0.331596)
(42.2, -0.313029)
};

==> exp_plots/open_ws_wind/plot.tex <==
%%    
\begin{figure}[t]
\centering

\begin{tikzpicture}


\FPeval{\xshfta}{0}
\FPeval{\xshftb}{0}
\FPeval{\xshftc}{0}
\FPeval{\xshftd}{0}



\FPeval{\yshfta}{0-0}
\FPeval{\yshftb}{0-9}
\FPeval{\yshftc}{0-18}
\FPeval{\yshftd}{0-27.9}


\FPeval{\pltw}{110}
\FPeval{\plth}{24}

\FPeval{\scal}{0.5}


\FPeval{\mrksize}{0.3}

%
\colorlet{desclr}{white!0!magenta}
\colorlet{currclr}{blue!60!green}

\colorlet{gridclr}{white!85!black}
\colorlet{dlegendclr}{white!80!black}
\colorlet{axisclr}{white!75!black}
\colorlet{axisbgclr}{white!99!black}

\colorlet{dlegendclr}{white!80!black}
\colorlet{legendclr}{white!100!black}






\FPeval{\lscale}{0.6}
\FPeval{\limscale}{0.5}
\FPeval{\lxshft}{95.5}
\FPeval{\lyshft}{9.0}

  
\FPeval{\titlescale}{0.7}
\FPeval{\titlexshift}{21.0}
\FPeval{\titleyshift}{13.7}

\colorlet{gpudclr}{white!80!black}
\colorlet{gpuclr}{white!90!black}
\colorlet{gputxtclr}{white!0!black}

\FPeval{\labelscale}{1.0}
\FPeval{\ticklabelscale}{0.9}

\FPeval{\xlabelxshift}{0+15}
\FPeval{\xlabelyshift}{0+0.5}
\FPeval{\ylabelxshift}{0+4.0}
\FPeval{\ylabelyshift}{0+6.2}


\FPeval{\linew}{1.5}
\FPeval{\dashon}{5.0}
\FPeval{\dashoff}{3.0}

\FPeval{\xshfttakeoff}{0-16}
\FPeval{\xshfthover}{0}
\FPeval{\xshftland}{16}
%
%
\node (a) [xshift = \xshfta ex, yshift=\yshfta ex, scale=\scal]{
\tikz{
%
\pgfplotsset{width=\pltw ex, height=\plth ex}
\begin{axis}[
   axis background style={fill=axisbgclr},
    title={},
    xlabel={},
    ylabel={ X (m)},
    xmin=0, xmax=42,
    ymin=-1, ymax=1,
    xtick={0, 15, 30, 45, 60},
    ytick={-1, 0, 1},
    xticklabels={$0$, $15$, $30$, $45$, $60$},
    yticklabels={$-1$, $0$, $0$},
     axis line style={axisclr},
    legend image post style={scale =\limscale},
    legend style={at={(\lxshft ex,\lyshft ex)},anchor=south, legend columns = 1, draw = {dlegendclr}, fill={legendclr}, nodes={scale=\lscale}},
    ymajorgrids=true, 
    xmajorgrids=true,
    grid style={dashed, gridclr},
    major tick length=1ex,
    x label style={at={(\xlabelxshift ex, \xlabelyshift ex)},scale=\labelscale},
    y label style={at={(\ylabelxshift ex, \ylabelyshift ex)},scale=\labelscale},
    xticklabel style={scale=\ticklabelscale},
    yticklabel style={scale=\ticklabelscale},
%    ybar,
%    bar width = 4pt,
]
%
%
\input{exp_plots/open_ws_wind/x_des}
%
\input{exp_plots/open_ws_wind/x}
%
%
%%   
  \legend{Ref, SLAM}
  %
\end{axis}
%
% \node [draw=gpudclr,fill=gpuclr,rounded corners=0.2ex, minimum width=10.0ex, xshift=\titlexshift ex, yshift=\titleyshift ex, scale=\titlescale]{\textcolor{gputxtclr}{\textbf{Step-X}}};
}};
%
%    
%
%
\node (b) [xshift = \xshftb ex, yshift=\yshftb ex, scale=\scal]{
\tikz{
%
\pgfplotsset{width=\pltw ex, height=\plth ex}
\begin{axis}[
   axis background style={fill=axisbgclr},
    title={},
    xlabel={},
    ylabel={ Y (m)},
    xmin=0, xmax=42,
    ymin=-1, ymax=1,
    xtick={0, 15, 30, 45, 60},
    ytick={-1, 0, 1},
    xticklabels={$0$, $15$, $30$, $45$, $60$},
    yticklabels={$-1$, $0$, $0$},
     axis line style={axisclr},
    legend image post style={scale =\limscale},
    legend style={at={(\lxshft ex,\lyshft ex)},anchor=south, legend columns = 1, draw = {dlegendclr}, fill={legendclr}, nodes={scale=\lscale}},
    ymajorgrids=true, 
    xmajorgrids=true,
    grid style={dashed, gridclr},
    major tick length=1ex,
    x label style={at={(\xlabelxshift ex, \xlabelyshift ex)},scale=\labelscale},
    y label style={at={(\ylabelxshift ex, \ylabelyshift ex)},scale=\labelscale},
    xticklabel style={scale=\ticklabelscale},
    yticklabel style={scale=\ticklabelscale},
%    ybar,
%    bar width = 4pt,
]
%
\input{exp_plots/open_ws_wind/y}
%
%
\input{exp_plots/open_ws_wind/y_des}
%
%% 
  \legend{Ref, SLAM}
  %
\end{axis}
%
% \node [draw=gpudclr,fill=gpuclr,rounded corners=0.2ex, minimum width=10.0ex, xshift=\titlexshift ex, yshift=\titleyshift ex, scale=\titlescale]{\textcolor{gputxtclr}{\textbf{Step-X}}};
}};
%
% 
%
\node (c) [xshift = \xshftc ex, yshift=\yshftc ex, scale=\scal]{
\tikz{
%
\pgfplotsset{width=\pltw ex, height=\plth ex}
\begin{axis}[
   axis background style={fill=axisbgclr},
    title={},
    xlabel={},
    ylabel={ Z (m)},
    xmin=0, xmax=42,
    ymin=-1, ymax=1,
    xtick={0, 15, 30, 45, 60},
    ytick={-1, 0, 1},
    xticklabels={$0$, $15$, $30$, $45$, $60$},
    yticklabels={$-1$, $0$, $0$},
     axis line style={axisclr},
    legend image post style={scale =\limscale},
    legend style={at={(\lxshft ex,\lyshft ex)},anchor=south, legend columns = 1, draw = {dlegendclr}, fill={legendclr}, nodes={scale=\lscale}},
    ymajorgrids=true, 
    xmajorgrids=true,
    grid style={dashed, gridclr},
    major tick length=1ex,
    x label style={at={(\xlabelxshift ex, \xlabelyshift ex)},scale=\labelscale},
    y label style={at={(\ylabelxshift ex, \ylabelyshift ex)},scale=\labelscale},
    xticklabel style={scale=\ticklabelscale},
    yticklabel style={scale=\ticklabelscale},
%    ybar,
%    bar width = 4pt,
]
%
\input{exp_plots/open_ws_wind/z}
%
%
\input{exp_plots/open_ws_wind/z_des}
%
%% 
  \legend{Ref, SLAM}
  %
\end{axis}
%
% \node [draw=gpudclr,fill=gpuclr,rounded corners=0.2ex, minimum width=10.0ex, xshift=\titlexshift ex, yshift=\titleyshift ex, scale=\titlescale]{\textcolor{gputxtclr}{\textbf{Step-X}}};
}};
%
% 
%
\node (d) [xshift = \xshftd ex, yshift=\yshftd ex, scale=\scal]{
\tikz{
%
\pgfplotsset{width=\pltw ex, height=\plth ex}
\begin{axis}[
   axis background style={fill=axisbgclr},
    title={},
    xlabel={Time (s)},
    ylabel={ Yaw ($^\text{o}$)},
    xmin=0, xmax=42,
    ymin=-40, ymax=40,
    xtick={0, 15, 30, 45, 60},
    ytick={-1, 0, 1},
    xticklabels={$0$, $15$, $30$, $45$, $60$},
    yticklabels={$-1$, $0$, $0$},
     axis line style={axisclr},
    legend image post style={scale =\limscale},
    legend style={at={(\lxshft ex,\lyshft ex)},anchor=south, legend columns = 1, draw = {dlegendclr}, fill={legendclr}, nodes={scale=\lscale}},
    ymajorgrids=true, 
    xmajorgrids=true,
    grid style={dashed, gridclr},
    major tick length=1ex,
    x label style={at={(\xlabelxshift ex, \xlabelyshift ex)},scale=\labelscale},
    y label style={at={(\ylabelxshift ex, \ylabelyshift ex)},scale=\labelscale},
    xticklabel style={scale=\ticklabelscale},
    yticklabel style={scale=\ticklabelscale},
%    ybar,
%    bar width = 4pt,
]
%
\input{exp_plots/open_ws_wind/yaw}
%
%
%
\input{exp_plots/open_ws_wind/yaw_des}
%
%% 
  \legend{Ref, SLAM}
  %
\end{axis}
%
% \node [draw=gpudclr,fill=gpuclr,rounded corners=0.2ex, minimum width=10.0ex, xshift=\titlexshift ex, yshift=\titleyshift ex, scale=\titlescale]{\textcolor{gputxtclr}{\textbf{Step-X}}};
}};
%
% 
%
%
\node (t) [xshift=\xshfttakeoff ex, yshift=5 ex]{\scriptsize Takeoff};
\node (h) [xshift=\xshfthover ex, yshift=5 ex]{\scriptsize Hover};
\node (l) [xshift=\xshftland ex, yshift=5 ex]{\scriptsize Land};
%%
%
 
\end{tikzpicture}
%
%
\caption{Takeoff-Hover-Land performance in open workspace with external wind.}
%
\label{fig:openwsTHLwind}
%
%\vspace{-3ex}
\end{figure}
%
%
%
%%


==> exp_plots/open_ws_wind/thrust.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0)
(0.1, 10)
(0.2, 10)
(0.3, 10)
(0.4, 10.0716)
(0.5, 10)
(0.6, 10.2493)
(0.7, 10.2908)
(0.8, 10.115)
(0.9, 10.1098)
(1, 10.0561)
(1.1, 13.6827)
(1.2, 16.016)
(1.3, 18.0967)
(1.4, 19.6386)
(1.5, 21.9803)
(1.6, 24.2337)
(1.7, 26.4323)
(1.8, 28.5707)
(1.9, 30.6633)
(2, 33.1109)
(2.1, 35.5606)
(2.2, 38.2091)
(2.3, 39.8743)
(2.4, 42.2108)
(2.5, 44.7396)
(2.6, 46.6882)
(2.7, 47.8235)
(2.8, 47.7507)
(2.9, 46.4392)
(3, 45.4621)
(3.1, 45.9414)
(3.2, 48.155)
(3.3, 48.9722)
(3.4, 48.6416)
(3.5, 48.3488)
(3.6, 48.4084)
(3.7, 46.2085)
(3.8, 44.0501)
(3.9, 45.964)
(4, 49.5558)
(4.1, 51.3373)
(4.2, 49.6517)
(4.3, 46.817)
(4.4, 46.9935)
(4.5, 50.5415)
(4.6, 53.0246)
(4.7, 52.2226)
(4.8, 49.1645)
(4.9, 45.9753)
(5, 47.0851)
(5.1, 49.388)
(5.2, 51.2522)
(5.3, 51.6763)
(5.4, 51.297)
(5.5, 49.8726)
(5.6, 49.2896)
(5.7, 50.4207)
(5.8, 50.5257)
(5.9, 48.9375)
(6, 48.4486)
(6.1, 49.4666)
(6.2, 51.8549)
(6.3, 52.4546)
(6.4, 50.0969)
(6.5, 45.8022)
(6.6, 46.7299)
(6.7, 51.2123)
(6.8, 52.1175)
(6.9, 49.1446)
(7, 45.8554)
(7.1, 45.9373)
(7.2, 48.4711)
(7.3, 51.374)
(7.4, 51.4529)
(7.5, 48.456)
(7.6, 48.2125)
(7.7, 50.2599)
(7.8, 53.0514)
(7.9, 53.9746)
(8, 53.8384)
(8.1, 49.9202)
(8.2, 47.7398)
(8.3, 48.3728)
(8.4, 50.8141)
(8.5, 51.6618)
(8.6, 51.5083)
(8.7, 50.564)
(8.8, 51.6567)
(8.9, 52.7622)
(9, 51.3117)
(9.1, 50.1055)
(9.2, 49.713)
(9.3, 50.0854)
(9.4, 49.8076)
(9.5, 50.148)
(9.6, 52.1039)
(9.7, 52.916)
(9.8, 52.0678)
(9.9, 51.121)
(10, 50.4271)
(10.1, 50.47)
(10.2, 50.7468)
(10.3, 52.7019)
(10.4, 53.6647)
(10.5, 52.8029)
(10.6, 51.793)
(10.7, 51.8441)
(10.8, 51.1265)
(10.9, 50.4471)
(11, 49.3546)
(11.1, 50.9093)
(11.2, 51.9031)
(11.3, 51.1034)
(11.4, 50.6466)
(11.5, 50.5524)
(11.6, 50.7356)
(11.7, 51.147)
(11.8, 51.4348)
(11.9, 50.9031)
(12, 49.3748)
(12.1, 49.0959)
(12.2, 49.7058)
(12.3, 50.3775)
(12.4, 49.4807)
(12.5, 49.4472)
(12.6, 50.3716)
(12.7, 50.6696)
(12.8, 50.8777)
(12.9, 50.8277)
(13, 50.8975)
(13.1, 50.8763)
(13.2, 50.526)
(13.3, 49.8366)
(13.4, 49.218)
(13.5, 51.4726)
(13.6, 52.8303)
(13.7, 51.7035)
(13.8, 49.322)
(13.9, 49.4132)
(14, 51.4173)
(14.1, 53.3451)
(14.2, 54.121)
(14.3, 52.8458)
(14.4, 51.3976)
(14.5, 49.8555)
(14.6, 49.2798)
(14.7, 51.4095)
(14.8, 53.1614)
(14.9, 52.6624)
(15, 50.8807)
(15.1, 49.4876)
(15.2, 48.5856)
(15.3, 48.603)
(15.4, 51.4205)
(15.5, 55.5687)
(15.6, 56.3856)
(15.7, 52.5031)
(15.8, 48.1544)
(15.9, 48.0569)
(16, 51.4386)
(16.1, 54.1174)
(16.2, 55.4799)
(16.3, 53.21)
(16.4, 49.416)
(16.5, 48.2075)
(16.6, 48.6963)
(16.7, 50.0308)
(16.8, 50.8778)
(16.9, 51.0852)
(17, 50.945)
(17.1, 51.1792)
(17.2, 50.5885)
(17.3, 50.153)
(17.4, 50.6563)
(17.5, 50.2791)
(17.6, 50.9358)
(17.7, 51.0259)
(17.8, 51.0726)
(17.9, 52.108)
(18, 52.7603)
(18.1, 52.4449)
(18.2, 51.9063)
(18.3, 50.7506)
(18.4, 51.0266)
(18.5, 52.3492)
(18.6, 52.6056)
(18.7, 51.6517)
(18.8, 50.9335)
(18.9, 51.1149)
(19, 52.3013)
(19.1, 52.5827)
(19.2, 51.7977)
(19.3, 50.9151)
(19.4, 52.7998)
(19.5, 53.9769)
(19.6, 52.5798)
(19.7, 51.8968)
(19.8, 50.8129)
(19.9, 48.9034)
(20, 49.5905)
(20.1, 52.1254)
(20.2, 53.6476)
(20.3, 53.8321)
(20.4, 53.8185)
(20.5, 53.5571)
(20.6, 51.943)
(20.7, 50.7849)
(20.8, 49.618)
(20.9, 48.8011)
(21, 48.8877)
(21.1, 51.0642)
(21.2, 52.7965)
(21.3, 52.4573)
(21.4, 50.1805)
(21.5, 48.885)
(21.6, 50.816)
(21.7, 53.7941)
(21.8, 54.3348)
(21.9, 52.247)
(22, 49.8766)
(22.1, 50.307)
(22.2, 50.9874)
(22.3, 51.9347)
(22.4, 52.5913)
(22.5, 52.2192)
(22.6, 52.7738)
(22.7, 51.8815)
(22.8, 51.2653)
(22.9, 51.2271)
(23, 52.1333)
(23.1, 53.4216)
(23.2, 55.2291)
(23.3, 56.2024)
(23.4, 54.4067)
(23.5, 52.8923)
(23.6, 50.6993)
(23.7, 47.7569)
(23.8, 48.7131)
(23.9, 52.1423)
(24, 53.2175)
(24.1, 51.5478)
(24.2, 51.033)
(24.3, 51.7766)
(24.4, 52.3346)
(24.5, 52.9192)
(24.6, 53.4724)
(24.7, 54.0641)
(24.8, 52.5954)
(24.9, 50.1311)
(25, 49.8214)
(25.1, 51.5565)
(25.2, 52.8067)
(25.3, 52.9851)
(25.4, 52.656)
(25.5, 51.8421)
(25.6, 52.5204)
(25.7, 52.9931)
(25.8, 52.6397)
(25.9, 52.8302)
(26, 53.5483)
(26.1, 53.1353)
(26.2, 51.6085)
(26.3, 50.7818)
(26.4, 50.8285)
(26.5, 51.3864)
(26.6, 49.9153)
(26.7, 50.421)
(26.8, 51.3835)
(26.9, 51.7195)
(27, 51.4324)
(27.1, 51.6541)
(27.2, 51.6695)
(27.3, 52.6273)
(27.4, 52.1151)
(27.5, 51.8626)
(27.6, 52.6657)
(27.7, 52.7144)
(27.8, 51.8154)
(27.9, 49.8277)
(28, 48.8489)
(28.1, 50.9994)
(28.2, 52.8519)
(28.3, 53.4046)
(28.4, 52.9637)
(28.5, 51.3868)
(28.6, 48.9575)
(28.7, 47.6933)
(28.8, 49.6116)
(28.9, 54.5691)
(29, 56.0682)
(29.1, 52.6564)
(29.2, 48.3786)
(29.3, 48.2629)
(29.4, 50.3881)
(29.5, 52.0715)
(29.6, 51.4699)
(29.7, 49.5375)
(29.8, 47.8489)
(29.9, 49.8349)
(30, 52.9254)
(30.1, 52.7304)
(30.2, 50.1315)
(30.3, 48.617)
(30.4, 48.9938)
(30.5, 49.5334)
(30.6, 50.3515)
(30.7, 51.1115)
(30.8, 50.7305)
(30.9, 48.9718)
(31, 47.3505)
(31.1, 48.4233)
(31.2, 50.4881)
(31.3, 50.7937)
(31.4, 49.5699)
(31.5, 48.1099)
(31.6, 48.243)
(31.7, 49.855)
(31.8, 49.7647)
(31.9, 47.13)
(32, 45.4494)
(32.1, 46.7203)
(32.2, 48.5588)
(32.3, 49.1651)
(32.4, 48.8718)
(32.5, 47.0451)
(32.6, 46.579)
(32.7, 46.624)
(32.8, 47.5492)
(32.9, 47.1502)
(33, 46.4689)
(33.1, 45.5021)
(33.2, 45.5202)
(33.3, 46.8529)
(33.4, 47.9179)
(33.5, 47.7585)
(33.6, 46.3994)
(33.7, 45.3193)
(33.8, 46.7124)
(33.9, 49.4412)
(34, 45.5492)
(34.1, 41.1028)
(34.2, 42.0664)
(34.3, 43.479)
(34.4, 39.9666)
(34.5, 39.6718)
(34.6, 38.5306)
(34.7, 39.3199)
(34.8, 39.1082)
(34.9, 37.4553)
(35, 36.4908)
(35.1, 35.9211)
(35.2, 34.7081)
(35.3, 33.1911)
(35.4, 31.8686)
(35.5, 30.6246)
(35.6, 30.2638)
(35.7, 29.1407)
(35.8, 27.6635)
(35.9, 26.4362)
(36, 25.1804)
(36.1, 24.1174)
(36.2, 22.9173)
(36.3, 21.8803)
(36.4, 21.053)
(36.5, 20.0525)
(36.6, 18.604)
(36.7, 17.5982)
(36.8, 16.2659)
(36.9, 14.552)
(37, 13.2891)
(37.1, 11.914)
(37.2, 10.694)
(37.3, 10)
(37.4, 10)
(37.5, 10)
(37.6, 10)
(37.7, 10)
(37.8, 10)
(37.9, 10)
(38, 10)
(38.1, 10)
(38.2, 10)
(38.3, 10)
(38.4, 10)
(38.5, 10)
(38.6, 10)
(38.7, 10)
(38.8, 10)
(38.9, 10)
(39, 10)
(39.1, 10)
(39.2, 10)
(39.3, 10)
(39.4, 10)
(39.5, 10)
(39.6, 10)
(39.7, 10)
(39.8, 10)
(39.9, 10)
(40, 10)
(40.1, 10)
(40.2, 10)
(40.3, 10)
(40.4, 10)
(40.5, 10)
(40.6, 10)
(40.7, 10)
(40.8, 10)
(40.9, 10)
(41, 10)
(41.1, 10)
(41.2, 10)
(41.3, 10)
(41.4, 10)
(41.5, 10)
(41.6, 10)
(41.7, 10)
(41.8, 10)
(41.9, 10)
(42, 10)
(42.1, 10)
(42.2, 10)
};

==> exp_plots/open_ws_wind/x.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0)
(0.1, 0.000221347)
(0.2, 0.000447361)
(0.3, 0.000360303)
(0.4, -0.000209872)
(0.5, -0.000360893)
(0.6, -0.000350996)
(0.7, 0.000350545)
(0.8, 0.000195218)
(0.9, 0.000844339)
(1, -6.92679e-05)
(1.1, 0.000300319)
(1.2, 0.000663431)
(1.3, 9.17822e-05)
(1.4, -0.000112637)
(1.5, 0.000410106)
(1.6, -0.000570047)
(1.7, -0.00062025)
(1.8, -0.000296019)
(1.9, -0.000453673)
(2, -0.00090974)
(2.1, 0.000197325)
(2.2, 0.00176055)
(2.3, 0.00329139)
(2.4, 0.00306661)
(2.5, 0.00139094)
(2.6, 0.00358267)
(2.7, 0.0036177)
(2.8, 0.0052357)
(2.9, 5.1929e-05)
(3, 0.00084893)
(3.1, 0.00447599)
(3.2, 0.00580796)
(3.3, -0.00729125)
(3.4, -0.0170489)
(3.5, -0.0234725)
(3.6, -0.0405113)
(3.7, -0.0584068)
(3.8, -0.0718175)
(3.9, -0.081227)
(4, -0.0880052)
(4.1, -0.085406)
(4.2, -0.0842568)
(4.3, -0.0838322)
(4.4, -0.074128)
(4.5, -0.0768401)
(4.6, -0.0677688)
(4.7, -0.0646063)
(4.8, -0.0573181)
(4.9, -0.0498756)
(5, -0.0337478)
(5.1, -0.0276716)
(5.2, -0.0219297)
(5.3, -0.0144618)
(5.4, -0.0125954)
(5.5, -0.0100799)
(5.6, -0.00632503)
(5.7, -0.001655)
(5.8, 0.0100543)
(5.9, 0.0164468)
(6, 0.0228757)
(6.1, 0.0241063)
(6.2, 0.0271779)
(6.3, 0.0280529)
(6.4, 0.0257599)
(6.5, 0.0174394)
(6.6, 0.019309)
(6.7, 0.0131621)
(6.8, 0.0112468)
(6.9, 0.00560489)
(7, 0.00280303)
(7.1, 0.00242298)
(7.2, 0.00193535)
(7.3, -0.00317244)
(7.4, 0.000230489)
(7.5, 0.0011429)
(7.6, 0.0010217)
(7.7, -0.0081719)
(7.8, -0.018959)
(7.9, -0.0316398)
(8, -0.0330671)
(8.1, -0.0382175)
(8.2, -0.0415005)
(8.3, -0.0416473)
(8.4, -0.0373898)
(8.5, -0.034481)
(8.6, -0.0343859)
(8.7, -0.0337357)
(8.8, -0.0214794)
(8.9, -0.00903131)
(9, 0.00360266)
(9.1, 0.0133444)
(9.2, 0.0153377)
(9.3, 0.011507)
(9.4, 0.0041366)
(9.5, -0.00303265)
(9.6, 0.00226416)
(9.7, 0.000398235)
(9.8, 0.000351161)
(9.9, -0.000990164)
(10, -0.00389997)
(10.1, -0.0148039)
(10.2, -0.0225746)
(10.3, -0.027308)
(10.4, -0.0314491)
(10.5, -0.0302133)
(10.6, -0.0266167)
(10.7, -0.0210042)
(10.8, -0.0174414)
(10.9, -0.0154101)
(11, -0.00844176)
(11.1, -0.00132786)
(11.2, 0.00353087)
(11.3, 0.00790222)
(11.4, 0.0111596)
(11.5, 0.000391129)
(11.6, -0.0100747)
(11.7, -0.0179884)
(11.8, -0.0299546)
(11.9, -0.039274)
(12, -0.0456306)
(12.1, -0.0507125)
(12.2, -0.0551402)
(12.3, -0.0607257)
(12.4, -0.0606787)
(12.5, -0.0567319)
(12.6, -0.0585015)
(12.7, -0.0521935)
(12.8, -0.0479844)
(12.9, -0.0399526)
(13, -0.0329761)
(13.1, -0.0210992)
(13.2, -0.0196376)
(13.3, -0.0155881)
(13.4, -0.00810813)
(13.5, -0.00246257)
(13.6, -0.00183882)
(13.7, 0.0100943)
(13.8, 0.0200389)
(13.9, 0.0214855)
(14, 0.0252713)
(14.1, 0.0277329)
(14.2, 0.0273511)
(14.3, 0.0283142)
(14.4, 0.0286255)
(14.5, 0.0307816)
(14.6, 0.0300841)
(14.7, 0.0310468)
(14.8, 0.0247416)
(14.9, 0.0197296)
(15, 0.0202983)
(15.1, 0.0267813)
(15.2, 0.0255089)
(15.3, 0.0236108)
(15.4, 0.0191376)
(15.5, 0.0168834)
(15.6, 0.0143099)
(15.7, 0.00465172)
(15.8, 0.00187744)
(15.9, 0.00267875)
(16, 0.00215694)
(16.1, 0.00117142)
(16.2, 0.00256653)
(16.3, 0.00306212)
(16.4, 0.00839244)
(16.5, 0.00915828)
(16.6, 0.0098123)
(16.7, 0.00922734)
(16.8, 0.00623945)
(16.9, 0.00778384)
(17, 0.00345195)
(17.1, -0.0082772)
(17.2, -0.0171885)
(17.3, -0.0244171)
(17.4, -0.0240094)
(17.5, -0.0277856)
(17.6, -0.0298569)
(17.7, -0.0306901)
(17.8, -0.0414613)
(17.9, -0.046998)
(18, -0.052894)
(18.1, -0.0506598)
(18.2, -0.0460956)
(18.3, -0.0401648)
(18.4, -0.0341359)
(18.5, -0.0304417)
(18.6, -0.0243468)
(18.7, -0.0166898)
(18.8, -0.0158517)
(18.9, -0.0101569)
(19, -0.0051008)
(19.1, -0.00589447)
(19.2, -0.00797363)
(19.3, -0.000296007)
(19.4, 0.00255274)
(19.5, 0.00913378)
(19.6, 0.0130395)
(19.7, 0.0126023)
(19.8, 0.0147591)
(19.9, 0.0205055)
(20, 0.0230341)
(20.1, 0.01785)
(20.2, 0.0154528)
(20.3, 0.0116063)
(20.4, 0.00709252)
(20.5, 0.00377352)
(20.6, 0.00291614)
(20.7, 0.00458731)
(20.8, 0.00800986)
(20.9, 0.00829354)
(21, 0.00974409)
(21.1, 0.0105894)
(21.2, 0.0099884)
(21.3, 0.00143606)
(21.4, -0.00296403)
(21.5, -0.00618972)
(21.6, -0.00576503)
(21.7, -0.00552892)
(21.8, -0.00619083)
(21.9, -0.00807801)
(22, -0.0116837)
(22.1, -0.0110366)
(22.2, -0.00894795)
(22.3, -0.00604452)
(22.4, -0.00326676)
(22.5, -0.00262195)
(22.6, -0.00302453)
(22.7, 0.00474039)
(22.8, 0.0081246)
(22.9, 0.00604888)
(23, -0.00135581)
(23.1, -0.0105757)
(23.2, -0.0160365)
(23.3, -0.017708)
(23.4, -0.0330792)
(23.5, -0.0387306)
(23.6, -0.0445475)
(23.7, -0.0377896)
(23.8, -0.0330755)
(23.9, -0.0298893)
(24, -0.0322363)
(24.1, -0.0277395)
(24.2, -0.0280184)
(24.3, -0.0258127)
(24.4, -0.0294839)
(24.5, -0.0221721)
(24.6, -0.0106236)
(24.7, -0.00363273)
(24.8, 0.00324239)
(24.9, 0.0078282)
(25, 0.0131968)
(25.1, 0.0168626)
(25.2, 0.020985)
(25.3, 0.0241037)
(25.4, 0.0262171)
(25.5, 0.0294382)
(25.6, 0.0327132)
(25.7, 0.0321823)
(25.8, 0.0354774)
(25.9, 0.0393769)
(26, 0.0415617)
(26.1, 0.0428608)
(26.2, 0.0456679)
(26.3, 0.0467785)
(26.4, 0.042284)
(26.5, 0.0372928)
(26.6, 0.0317106)
(26.7, 0.0266618)
(26.8, 0.0233783)
(26.9, 0.0132719)
(27, 0.00114174)
(27.1, -0.00819125)
(27.2, -0.0174508)
(27.3, -0.021893)
(27.4, -0.0300577)
(27.5, -0.0355654)
(27.6, -0.0416772)
(27.7, -0.0455917)
(27.8, -0.0495294)
(27.9, -0.0515229)
(28, -0.0503311)
(28.1, -0.0471232)
(28.2, -0.0486724)
(28.3, -0.0433738)
(28.4, -0.0404118)
(28.5, -0.0380154)
(28.6, -0.0338614)
(28.7, -0.0250718)
(28.8, -0.014228)
(28.9, -0.00443992)
(29, 0.000673901)
(29.1, -0.000553937)
(29.2, -0.000782392)
(29.3, 0.000138149)
(29.4, 0.00681375)
(29.5, 0.00504377)
(29.6, 0.00724052)
(29.7, 0.00338689)
(29.8, 0.000959687)
(29.9, -0.000269941)
(30, 0.00138563)
(30.1, -0.000865183)
(30.2, 0.00332459)
(30.3, 0.00717478)
(30.4, 0.0114891)
(30.5, 0.0214019)
(30.6, 0.0256477)
(30.7, 0.0266215)
(30.8, 0.0253105)
(30.9, 0.0265037)
(31, 0.026986)
(31.1, 0.0302306)
(31.2, 0.0399974)
(31.3, 0.0395326)
(31.4, 0.0420235)
(31.5, 0.0418087)
(31.6, 0.0401689)
(31.7, 0.0406127)
(31.8, 0.0374204)
(31.9, 0.036047)
(32, 0.0383817)
(32.1, 0.0315293)
(32.2, 0.0201064)
(32.3, 0.0101403)
(32.4, -0.00377219)
(32.5, -0.0157552)
(32.6, -0.0250035)
(32.7, -0.0317533)
(32.8, -0.033963)
(32.9, -0.033788)
(33, -0.0365634)
(33.1, -0.0400469)
(33.2, -0.0380571)
(33.3, -0.0335187)
(33.4, -0.0305909)
(33.5, -0.0254512)
(33.6, -0.0258438)
(33.7, -0.0248074)
(33.8, -0.0225689)
(33.9, -0.0246688)
(34, -0.0252843)
(34.1, -0.0310836)
(34.2, -0.0344138)
(34.3, -0.0408259)
(34.4, -0.0407787)
(34.5, -0.0380109)
(34.6, -0.0360984)
(34.7, -0.0328039)
(34.8, -0.0334339)
(34.9, -0.0412765)
(35, -0.0458911)
(35.1, -0.0454807)
(35.2, -0.0462612)
(35.3, -0.0445854)
(35.4, -0.045787)
(35.5, -0.0439177)
(35.6, -0.0415597)
(35.7, -0.040285)
(35.8, -0.0403699)
(35.9, -0.0414241)
(36, -0.0436901)
(36.1, -0.0431748)
(36.2, -0.0409423)
(36.3, -0.035975)
(36.4, -0.0317945)
(36.5, -0.0315739)
(36.6, -0.0362717)
(36.7, -0.0347683)
(36.8, -0.0337489)
(36.9, -0.0319703)
(37, -0.0318717)
(37.1, -0.0310445)
(37.2, -0.0325591)
(37.3, -0.0332639)
(37.4, -0.0341209)
(37.5, -0.0350167)
(37.6, -0.034606)
(37.7, -0.0343442)
(37.8, -0.0349873)
(37.9, -0.0388004)
(38, -0.036501)
(38.1, -0.0366945)
(38.2, -0.0363649)
(38.3, -0.0369434)
(38.4, -0.0365494)
(38.5, -0.0365337)
(38.6, -0.0369518)
(38.7, -0.0379505)
(38.8, -0.0372723)
(38.9, -0.0367232)
(39, -0.035823)
(39.1, -0.0358908)
(39.2, -0.0349144)
(39.3, -0.0343819)
(39.4, -0.0357297)
(39.5, -0.0390355)
(39.6, -0.039932)
(39.7, -0.0411602)
(39.8, -0.0420051)
(39.9, -0.0430124)
(40, -0.039409)
(40.1, -0.0385307)
(40.2, -0.03864)
(40.3, -0.0385684)
(40.4, -0.038693)
(40.5, -0.0380804)
(40.6, -0.0370065)
(40.7, -0.0372662)
(40.8, -0.0372907)
(40.9, -0.03908)
(41, -0.0392672)
(41.1, -0.0386274)
(41.2, -0.0388788)
(41.3, -0.038085)
(41.4, -0.0385797)
(41.5, -0.0381285)
(41.6, -0.0382542)
(41.7, -0.0393955)
(41.8, -0.0402566)
(41.9, -0.03981)
(42, -0.0398538)
(42.1, -0.038855)
(42.2, -0.0388138)
};

==> exp_plots/open_ws_wind/x_des.tex <==
\addplot[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates {
(0, 0)
(0.1, 0)
(0.2, 0)
(0.3, 0)
(0.4, 0)
(0.5, 0)
(0.6, 0)
(0.7, 0)
(0.8, 0)
(0.9, 0)
(1, 0)
(1.1, 0)
(1.2, 0)
(1.3, 0)
(1.4, 0)
(1.5, 0)
(1.6, 0)
(1.7, 0)
(1.8, 0)
(1.9, 0)
(2, 0)
(2.1, 0)
(2.2, 0)
(2.3, 0)
(2.4, 0)
(2.5, 0)
(2.6, 0)
(2.7, 0)
(2.8, 0)
(2.9, 0)
(3, 0)
(3.1, 0)
(3.2, 0)
(3.3, 0)
(3.4, 0)
(3.5, 0)
(3.6, 0)
(3.7, 0)
(3.8, 0)
(3.9, 0)
(4, 0)
(4.1, 0)
(4.2, 0)
(4.3, 0)
(4.4, 0)
(4.5, 0)
(4.6, 0)
(4.7, 0)
(4.8, 0)
(4.9, 0)
(5, 0)
(5.1, 0)
(5.2, 0)
(5.3, 0)
(5.4, 0)
(5.5, 0)
(5.6, 0)
(5.7, 0)
(5.8, 0)
(5.9, 0)
(6, 0)
(6.1, 0)
(6.2, 0)
(6.3, 0)
(6.4, 0)
(6.5, 0)
(6.6, 0)
(6.7, 0)
(6.8, 0)
(6.9, 0)
(7, 0)
(7.1, 0)
(7.2, 0)
(7.3, 0)
(7.4, 0)
(7.5, 0)
(7.6, 0)
(7.7, 0)
(7.8, 0)
(7.9, 0)
(8, 0)
(8.1, 0)
(8.2, 0)
(8.3, 0)
(8.4, 0)
(8.5, 0)
(8.6, 0)
(8.7, 0)
(8.8, 0)
(8.9, 0)
(9, 0)
(9.1, 0)
(9.2, 0)
(9.3, 0)
(9.4, 0)
(9.5, 0)
(9.6, 0)
(9.7, 0)
(9.8, 0)
(9.9, 0)
(10, 0)
(10.1, 0)
(10.2, 0)
(10.3, 0)
(10.4, 0)
(10.5, 0)
(10.6, 0)
(10.7, 0)
(10.8, 0)
(10.9, 0)
(11, 0)
(11.1, 0)
(11.2, 0)
(11.3, 0)
(11.4, 0)
(11.5, 0)
(11.6, 0)
(11.7, 0)
(11.8, 0)
(11.9, 0)
(12, 0)
(12.1, 0)
(12.2, 0)
(12.3, 0)
(12.4, 0)
(12.5, 0)
(12.6, 0)
(12.7, 0)
(12.8, 0)
(12.9, 0)
(13, 0)
(13.1, 0)
(13.2, 0)
(13.3, 0)
(13.4, 0)
(13.5, 0)
(13.6, 0)
(13.7, 0)
(13.8, 0)
(13.9, 0)
(14, 0)
(14.1, 0)
(14.2, 0)
(14.3, 0)
(14.4, 0)
(14.5, 0)
(14.6, 0)
(14.7, 0)
(14.8, 0)
(14.9, 0)
(15, 0)
(15.1, 0)
(15.2, 0)
(15.3, 0)
(15.4, 0)
(15.5, 0)
(15.6, 0)
(15.7, 0)
(15.8, 0)
(15.9, 0)
(16, 0)
(16.1, 0)
(16.2, 0)
(16.3, 0)
(16.4, 0)
(16.5, 0)
(16.6, 0)
(16.7, 0)
(16.8, 0)
(16.9, 0)
(17, 0)
(17.1, 0)
(17.2, 0)
(17.3, 0)
(17.4, 0)
(17.5, 0)
(17.6, 0)
(17.7, 0)
(17.8, 0)
(17.9, 0)
(18, 0)
(18.1, 0)
(18.2, 0)
(18.3, 0)
(18.4, 0)
(18.5, 0)
(18.6, 0)
(18.7, 0)
(18.8, 0)
(18.9, 0)
(19, 0)
(19.1, 0)
(19.2, 0)
(19.3, 0)
(19.4, 0)
(19.5, 0)
(19.6, 0)
(19.7, 0)
(19.8, 0)
(19.9, 0)
(20, 0)
(20.1, 0)
(20.2, 0)
(20.3, 0)
(20.4, 0)
(20.5, 0)
(20.6, 0)
(20.7, 0)
(20.8, 0)
(20.9, 0)
(21, 0)
(21.1, 0)
(21.2, 0)
(21.3, 0)
(21.4, 0)
(21.5, 0)
(21.6, 0)
(21.7, 0)
(21.8, 0)
(21.9, 0)
(22, 0)
(22.1, 0)
(22.2, 0)
(22.3, 0)
(22.4, 0)
(22.5, 0)
(22.6, 0)
(22.7, 0)
(22.8, 0)
(22.9, 0)
(23, 0)
(23.1, 0)
(23.2, 0)
(23.3, 0)
(23.4, 0)
(23.5, 0)
(23.6, 0)
(23.7, 0)
(23.8, 0)
(23.9, 0)
(24, 0)
(24.1, 0)
(24.2, 0)
(24.3, 0)
(24.4, 0)
(24.5, 0)
(24.6, 0)
(24.7, 0)
(24.8, 0)
(24.9, 0)
(25, 0)
(25.1, 0)
(25.2, 0)
(25.3, 0)
(25.4, 0)
(25.5, 0)
(25.6, 0)
(25.7, 0)
(25.8, 0)
(25.9, 0)
(26, 0)
(26.1, 0)
(26.2, 0)
(26.3, 0)
(26.4, 0)
(26.5, 0)
(26.6, 0)
(26.7, 0)
(26.8, 0)
(26.9, 0)
(27, 0)
(27.1, 0)
(27.2, 0)
(27.3, 0)
(27.4, 0)
(27.5, 0)
(27.6, 0)
(27.7, 0)
(27.8, 0)
(27.9, 0)
(28, 0)
(28.1, 0)
(28.2, 0)
(28.3, 0)
(28.4, 0)
(28.5, 0)
(28.6, 0)
(28.7, 0)
(28.8, 0)
(28.9, 0)
(29, 0)
(29.1, 0)
(29.2, 0)
(29.3, 0)
(29.4, 0)
(29.5, 0)
(29.6, 0)
(29.7, 0)
(29.8, 0)
(29.9, 0)
(30, 0)
(30.1, 0)
(30.2, 0)
(30.3, 0)
(30.4, 0)
(30.5, 0)
(30.6, 0)
(30.7, 0)
(30.8, 0)
(30.9, 0)
(31, 0)
(31.1, 0)
(31.2, 0)
(31.3, 0)
(31.4, 0)
(31.5, 0)
(31.6, 0)
(31.7, 0)
(31.8, 0)
(31.9, 0)
(32, 0)
(32.1, 0)
(32.2, 0)
(32.3, 0)
(32.4, 0)
(32.5, 0)
(32.6, 0)
(32.7, 0)
(32.8, 0)
(32.9, 0)
(33, 0)
(33.1, 0)
(33.2, 0)
(33.3, 0)
(33.4, 0)
(33.5, 0)
(33.6, 0)
(33.7, 0)
(33.8, 0)
(33.9, 0)
(34, 0)
(34.1, 0)
(34.2, 0)
(34.3, 0)
(34.4, 0)
(34.5, 0)
(34.6, 0)
(34.7, 0)
(34.8, 0)
(34.9, 0)
(35, 0)
(35.1, 0)
(35.2, 0)
(35.3, 0)
(35.4, 0)
(35.5, 0)
(35.6, 0)
(35.7, 0)
(35.8, 0)
(35.9, 0)
(36, 0)
(36.1, 0)
(36.2, 0)
(36.3, 0)
(36.4, 0)
(36.5, 0)
(36.6, 0)
(36.7, 0)
(36.8, 0)
(36.9, 0)
(37, 0)
(37.1, 0)
(37.2, 0)
(37.3, 0)
(37.4, 0)
(37.5, 0)
(37.6, 0)
(37.7, 0)
(37.8, 0)
(37.9, 0)
(38, 0)
(38.1, 0)
(38.2, 0)
(38.3, 0)
(38.4, 0)
(38.5, 0)
(38.6, 0)
(38.7, 0)
(38.8, 0)
(38.9, 0)
(39, 0)
(39.1, 0)
(39.2, 0)
(39.3, 0)
(39.4, 0)
(39.5, 0)
(39.6, 0)
(39.7, 0)
(39.8, 0)
(39.9, 0)
(40, 0)
(40.1, 0)
(40.2, 0)
(40.3, 0)
(40.4, 0)
(40.5, 0)
(40.6, 0)
(40.7, 0)
(40.8, 0)
(40.9, 0)
(41, 0)
(41.1, 0)
(41.2, 0)
(41.3, 0)
(41.4, 0)
(41.5, 0)
(41.6, 0)
(41.7, 0)
(41.8, 0)
(41.9, 0)
(42, 0)
(42.1, 0)
(42.2, 0)
};

==> exp_plots/open_ws_wind/y.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0)
(0.1, 0.000125241)
(0.2, 0.000309161)
(0.3, 0.000350872)
(0.4, 0.000112302)
(0.5, 0.000150228)
(0.6, 8.48212e-05)
(0.7, 0.000360292)
(0.8, 0.000252877)
(0.9, 0.000580401)
(1, 0.0003348)
(1.1, 0.000329271)
(1.2, 0.000573098)
(1.3, 0.00058061)
(1.4, 0.00048454)
(1.5, 0.000757851)
(1.6, 0.000415351)
(1.7, 0.000194517)
(1.8, 0.000114748)
(1.9, 0.000553482)
(2, -0.00010915)
(2.1, -0.000727513)
(2.2, -0.000104453)
(2.3, -5.19195e-05)
(2.4, 0.000582032)
(2.5, 0.000817344)
(2.6, 0.00051503)
(2.7, -0.000193091)
(2.8, -0.00270099)
(2.9, -0.00327276)
(3, -0.00675006)
(3.1, -0.00886706)
(3.2, -0.00399101)
(3.3, -0.00430089)
(3.4, -0.00178391)
(3.5, -0.00155217)
(3.6, 0.0025606)
(3.7, -0.00703728)
(3.8, -0.00862624)
(3.9, -0.00804298)
(4, -0.00852741)
(4.1, -0.0103455)
(4.2, -0.0125862)
(4.3, -0.0152317)
(4.4, -0.0131744)
(4.5, -0.0184229)
(4.6, -0.0184017)
(4.7, -0.0172271)
(4.8, -0.017183)
(4.9, -0.0171971)
(5, -0.0191305)
(5.1, -0.0176302)
(5.2, -0.0228677)
(5.3, -0.0263634)
(5.4, -0.0269734)
(5.5, -0.0263071)
(5.6, -0.0247746)
(5.7, -0.0235815)
(5.8, -0.0247933)
(5.9, -0.0313063)
(6, -0.0311796)
(6.1, -0.0344877)
(6.2, -0.0362061)
(6.3, -0.0370495)
(6.4, -0.0403826)
(6.5, -0.0437836)
(6.6, -0.0425978)
(6.7, -0.0422003)
(6.8, -0.0456368)
(6.9, -0.0515124)
(7, -0.0569228)
(7.1, -0.0621783)
(7.2, -0.0706735)
(7.3, -0.0713185)
(7.4, -0.0707839)
(7.5, -0.0676383)
(7.6, -0.0654838)
(7.7, -0.0591152)
(7.8, -0.0643986)
(7.9, -0.0642257)
(8, -0.0672966)
(8.1, -0.0678058)
(8.2, -0.0686862)
(8.3, -0.0726494)
(8.4, -0.07433)
(8.5, -0.0774894)
(8.6, -0.0786262)
(8.7, -0.080558)
(8.8, -0.0807881)
(8.9, -0.0790485)
(9, -0.0748068)
(9.1, -0.0633469)
(9.2, -0.0602368)
(9.3, -0.0578183)
(9.4, -0.0535305)
(9.5, -0.0429781)
(9.6, -0.0515943)
(9.7, -0.0426524)
(9.8, -0.0301898)
(9.9, -0.0233052)
(10, -0.0179749)
(10.1, -0.013445)
(10.2, -0.0133225)
(10.3, -0.0110711)
(10.4, -0.0125049)
(10.5, -0.0185408)
(10.6, -0.0260969)
(10.7, -0.0277632)
(10.8, -0.0391269)
(10.9, -0.0481473)
(11, -0.0551464)
(11.1, -0.0598405)
(11.2, -0.0638347)
(11.3, -0.0634476)
(11.4, -0.064254)
(11.5, -0.0551341)
(11.6, -0.0477821)
(11.7, -0.04716)
(11.8, -0.0507497)
(11.9, -0.0572875)
(12, -0.0624349)
(12.1, -0.0629586)
(12.2, -0.0685208)
(12.3, -0.0641305)
(12.4, -0.067078)
(12.5, -0.0713006)
(12.6, -0.0753293)
(12.7, -0.0769957)
(12.8, -0.0750534)
(12.9, -0.0782723)
(13, -0.0743591)
(13.1, -0.0731566)
(13.2, -0.0713382)
(13.3, -0.0682861)
(13.4, -0.0616364)
(13.5, -0.059168)
(13.6, -0.0584024)
(13.7, -0.0435291)
(13.8, -0.0291159)
(13.9, -0.021739)
(14, -0.0170063)
(14.1, -7.73776e-05)
(14.2, 0.023666)
(14.3, 0.034307)
(14.4, 0.038748)
(14.5, 0.0554602)
(14.6, 0.0568626)
(14.7, 0.0578108)
(14.8, 0.0469584)
(14.9, 0.0418585)
(15, 0.0263818)
(15.1, 0.0120915)
(15.2, 0.000973683)
(15.3, -0.0170749)
(15.4, -0.0316715)
(15.5, -0.0387179)
(15.6, -0.0435863)
(15.7, -0.0493301)
(15.8, -0.0635196)
(15.9, -0.0735456)
(16, -0.0878111)
(16.1, -0.0998309)
(16.2, -0.111637)
(16.3, -0.116361)
(16.4, -0.116347)
(16.5, -0.115816)
(16.6, -0.117948)
(16.7, -0.125818)
(16.8, -0.124081)
(16.9, -0.123054)
(17, -0.119046)
(17.1, -0.112038)
(17.2, -0.106854)
(17.3, -0.09365)
(17.4, -0.0850123)
(17.5, -0.0761585)
(17.6, -0.0684645)
(17.7, -0.0608383)
(17.8, -0.0468011)
(17.9, -0.0357549)
(18, -0.0261263)
(18.1, -0.0162689)
(18.2, -0.00830453)
(18.3, 0.001483)
(18.4, 0.00966989)
(18.5, 0.0200189)
(18.6, 0.0275388)
(18.7, 0.0303363)
(18.8, 0.0351094)
(18.9, 0.0304584)
(19, 0.0277472)
(19.1, 0.0212693)
(19.2, 0.0202765)
(19.3, 0.0144424)
(19.4, -7.63586e-05)
(19.5, -0.035289)
(19.6, -0.0620057)
(19.7, -0.0837817)
(19.8, -0.101867)
(19.9, -0.123317)
(20, -0.130675)
(20.1, -0.134282)
(20.2, -0.136113)
(20.3, -0.140142)
(20.4, -0.1432)
(20.5, -0.143731)
(20.6, -0.141323)
(20.7, -0.141207)
(20.8, -0.139448)
(20.9, -0.12374)
(21, -0.110069)
(21.1, -0.0972869)
(21.2, -0.0852666)
(21.3, -0.0719558)
(21.4, -0.0689725)
(21.5, -0.0555079)
(21.6, -0.0366944)
(21.7, -0.0242369)
(21.8, 0.000602964)
(21.9, 0.0195497)
(22, 0.0252998)
(22.1, 0.0263878)
(22.2, 0.0289696)
(22.3, 0.0239913)
(22.4, 0.0114441)
(22.5, 0.00926787)
(22.6, 0.00297375)
(22.7, -0.00102404)
(22.8, -0.00446332)
(22.9, -0.0102096)
(23, -0.0146597)
(23.1, -0.0205687)
(23.2, -0.0720422)
(23.3, -0.123631)
(23.4, -0.151842)
(23.5, -0.169549)
(23.6, -0.174913)
(23.7, -0.183293)
(23.8, -0.187334)
(23.9, -0.188251)
(24, -0.171289)
(24.1, -0.158477)
(24.2, -0.153684)
(24.3, -0.142888)
(24.4, -0.129639)
(24.5, -0.128832)
(24.6, -0.118361)
(24.7, -0.117642)
(24.8, -0.11562)
(24.9, -0.108005)
(25, -0.0946177)
(25.1, -0.0814473)
(25.2, -0.0645716)
(25.3, -0.0390921)
(25.4, -0.0206928)
(25.5, -0.00231467)
(25.6, 0.0134353)
(25.7, 0.0198681)
(25.8, 0.0260988)
(25.9, 0.0342281)
(26, 0.041486)
(26.1, 0.0447928)
(26.2, 0.0469468)
(26.3, 0.0442126)
(26.4, 0.0401835)
(26.5, 0.0355272)
(26.6, 0.0122845)
(26.7, -0.00244087)
(26.8, -0.0261222)
(26.9, -0.0358985)
(27, -0.0369248)
(27.1, -0.0454222)
(27.2, -0.0476089)
(27.3, -0.0603197)
(27.4, -0.0642811)
(27.5, -0.0668637)
(27.6, -0.0735257)
(27.7, -0.0693163)
(27.8, -0.0652359)
(27.9, -0.0636261)
(28, -0.062396)
(28.1, -0.0610258)
(28.2, -0.0604788)
(28.3, -0.0556885)
(28.4, -0.0534955)
(28.5, -0.04838)
(28.6, -0.0444498)
(28.7, -0.0428293)
(28.8, -0.0472341)
(28.9, -0.0555903)
(29, -0.0607406)
(29.1, -0.0606336)
(29.2, -0.0625396)
(29.3, -0.0644968)
(29.4, -0.0625327)
(29.5, -0.0630497)
(29.6, -0.061937)
(29.7, -0.0590065)
(29.8, -0.0524985)
(29.9, -0.0476655)
(30, -0.0396662)
(30.1, -0.0334573)
(30.2, -0.0254915)
(30.3, -0.0158035)
(30.4, -0.00976389)
(30.5, -0.00366996)
(30.6, 0.002194)
(30.7, 0.00197138)
(30.8, 0.000777984)
(30.9, -0.000992443)
(31, -0.00253781)
(31.1, -0.00471888)
(31.2, -0.00185426)
(31.3, -0.00182735)
(31.4, -0.00401974)
(31.5, -0.0136422)
(31.6, -0.0221288)
(31.7, -0.0316958)
(31.8, -0.0448997)
(31.9, -0.049326)
(32, -0.0525085)
(32.1, -0.0551919)
(32.2, -0.0586783)
(32.3, -0.0621827)
(32.4, -0.0680327)
(32.5, -0.0718968)
(32.6, -0.0763368)
(32.7, -0.0739455)
(32.8, -0.0765213)
(32.9, -0.0768112)
(33, -0.0770502)
(33.1, -0.0746136)
(33.2, -0.0720322)
(33.3, -0.0707044)
(33.4, -0.0618049)
(33.5, -0.055182)
(33.6, -0.0514668)
(33.7, -0.0504949)
(33.8, -0.0487772)
(33.9, -0.0463317)
(34, -0.0423302)
(34.1, -0.0431195)
(34.2, -0.0447757)
(34.3, -0.0475929)
(34.4, -0.0505749)
(34.5, -0.0572785)
(34.6, -0.0603135)
(34.7, -0.0600759)
(34.8, -0.0618203)
(34.9, -0.0609796)
(35, -0.0598571)
(35.1, -0.058786)
(35.2, -0.054697)
(35.3, -0.0541895)
(35.4, -0.0528409)
(35.5, -0.053091)
(35.6, -0.0543828)
(35.7, -0.0549213)
(35.8, -0.0549916)
(35.9, -0.0550471)
(36, -0.0552769)
(36.1, -0.0551915)
(36.2, -0.0549915)
(36.3, -0.0560375)
(36.4, -0.0576161)
(36.5, -0.0595738)
(36.6, -0.0571194)
(36.7, -0.0554268)
(36.8, -0.0566962)
(36.9, -0.0580192)
(37, -0.0578029)
(37.1, -0.057911)
(37.2, -0.0572975)
(37.3, -0.0570735)
(37.4, -0.0565559)
(37.5, -0.0565386)
(37.6, -0.0563458)
(37.7, -0.0565658)
(37.8, -0.0568439)
(37.9, -0.0543685)
(38, -0.0549641)
(38.1, -0.0549501)
(38.2, -0.0553648)
(38.3, -0.054583)
(38.4, -0.0547377)
(38.5, -0.0548034)
(38.6, -0.054575)
(38.7, -0.0541513)
(38.8, -0.0544303)
(38.9, -0.0547018)
(39, -0.0551673)
(39.1, -0.0553182)
(39.2, -0.0561607)
(39.3, -0.056821)
(39.4, -0.0562033)
(39.5, -0.0575839)
(39.6, -0.0566268)
(39.7, -0.0571883)
(39.8, -0.0572356)
(39.9, -0.0580611)
(40, -0.0581573)
(40.1, -0.0584856)
(40.2, -0.0583668)
(40.3, -0.0580269)
(40.4, -0.0577833)
(40.5, -0.0577325)
(40.6, -0.0577293)
(40.7, -0.0577718)
(40.8, -0.0578747)
(40.9, -0.0580343)
(41, -0.0580871)
(41.1, -0.0582575)
(41.2, -0.0585002)
(41.3, -0.0577925)
(41.4, -0.0578873)
(41.5, -0.0577623)
(41.6, -0.0577364)
(41.7, -0.0579551)
(41.8, -0.0578725)
(41.9, -0.0574838)
(42, -0.0574635)
(42.1, -0.0567517)
(42.2, -0.0565331)
};

==> exp_plots/open_ws_wind/y_des.tex <==
\addplot[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates {
(0, 0)
(0.1, 0)
(0.2, 0)
(0.3, 0)
(0.4, 0)
(0.5, 0)
(0.6, 0)
(0.7, 0)
(0.8, 0)
(0.9, 0)
(1, 0)
(1.1, 0)
(1.2, 0)
(1.3, 0)
(1.4, 0)
(1.5, 0)
(1.6, 0)
(1.7, 0)
(1.8, 0)
(1.9, 0)
(2, 0)
(2.1, 0)
(2.2, 0)
(2.3, 0)
(2.4, 0)
(2.5, 0)
(2.6, 0)
(2.7, 0)
(2.8, 0)
(2.9, 0)
(3, 0)
(3.1, 0)
(3.2, 0)
(3.3, 0)
(3.4, 0)
(3.5, 0)
(3.6, 0)
(3.7, 0)
(3.8, 0)
(3.9, 0)
(4, 0)
(4.1, 0)
(4.2, 0)
(4.3, 0)
(4.4, 0)
(4.5, 0)
(4.6, 0)
(4.7, 0)
(4.8, 0)
(4.9, 0)
(5, 0)
(5.1, 0)
(5.2, 0)
(5.3, 0)
(5.4, 0)
(5.5, 0)
(5.6, 0)
(5.7, 0)
(5.8, 0)
(5.9, 0)
(6, 0)
(6.1, 0)
(6.2, 0)
(6.3, 0)
(6.4, 0)
(6.5, 0)
(6.6, 0)
(6.7, 0)
(6.8, 0)
(6.9, 0)
(7, 0)
(7.1, 0)
(7.2, 0)
(7.3, 0)
(7.4, 0)
(7.5, 0)
(7.6, 0)
(7.7, 0)
(7.8, 0)
(7.9, 0)
(8, 0)
(8.1, 0)
(8.2, 0)
(8.3, 0)
(8.4, 0)
(8.5, 0)
(8.6, 0)
(8.7, 0)
(8.8, 0)
(8.9, 0)
(9, 0)
(9.1, 0)
(9.2, 0)
(9.3, 0)
(9.4, 0)
(9.5, 0)
(9.6, 0)
(9.7, 0)
(9.8, 0)
(9.9, 0)
(10, 0)
(10.1, 0)
(10.2, 0)
(10.3, 0)
(10.4, 0)
(10.5, 0)
(10.6, 0)
(10.7, 0)
(10.8, 0)
(10.9, 0)
(11, 0)
(11.1, 0)
(11.2, 0)
(11.3, 0)
(11.4, 0)
(11.5, 0)
(11.6, 0)
(11.7, 0)
(11.8, 0)
(11.9, 0)
(12, 0)
(12.1, 0)
(12.2, 0)
(12.3, 0)
(12.4, 0)
(12.5, 0)
(12.6, 0)
(12.7, 0)
(12.8, 0)
(12.9, 0)
(13, 0)
(13.1, 0)
(13.2, 0)
(13.3, 0)
(13.4, 0)
(13.5, 0)
(13.6, 0)
(13.7, 0)
(13.8, 0)
(13.9, 0)
(14, 0)
(14.1, 0)
(14.2, 0)
(14.3, 0)
(14.4, 0)
(14.5, 0)
(14.6, 0)
(14.7, 0)
(14.8, 0)
(14.9, 0)
(15, 0)
(15.1, 0)
(15.2, 0)
(15.3, 0)
(15.4, 0)
(15.5, 0)
(15.6, 0)
(15.7, 0)
(15.8, 0)
(15.9, 0)
(16, 0)
(16.1, 0)
(16.2, 0)
(16.3, 0)
(16.4, 0)
(16.5, 0)
(16.6, 0)
(16.7, 0)
(16.8, 0)
(16.9, 0)
(17, 0)
(17.1, 0)
(17.2, 0)
(17.3, 0)
(17.4, 0)
(17.5, 0)
(17.6, 0)
(17.7, 0)
(17.8, 0)
(17.9, 0)
(18, 0)
(18.1, 0)
(18.2, 0)
(18.3, 0)
(18.4, 0)
(18.5, 0)
(18.6, 0)
(18.7, 0)
(18.8, 0)
(18.9, 0)
(19, 0)
(19.1, 0)
(19.2, 0)
(19.3, 0)
(19.4, 0)
(19.5, 0)
(19.6, 0)
(19.7, 0)
(19.8, 0)
(19.9, 0)
(20, 0)
(20.1, 0)
(20.2, 0)
(20.3, 0)
(20.4, 0)
(20.5, 0)
(20.6, 0)
(20.7, 0)
(20.8, 0)
(20.9, 0)
(21, 0)
(21.1, 0)
(21.2, 0)
(21.3, 0)
(21.4, 0)
(21.5, 0)
(21.6, 0)
(21.7, 0)
(21.8, 0)
(21.9, 0)
(22, 0)
(22.1, 0)
(22.2, 0)
(22.3, 0)
(22.4, 0)
(22.5, 0)
(22.6, 0)
(22.7, 0)
(22.8, 0)
(22.9, 0)
(23, 0)
(23.1, 0)
(23.2, 0)
(23.3, 0)
(23.4, 0)
(23.5, 0)
(23.6, 0)
(23.7, 0)
(23.8, 0)
(23.9, 0)
(24, 0)
(24.1, 0)
(24.2, 0)
(24.3, 0)
(24.4, 0)
(24.5, 0)
(24.6, 0)
(24.7, 0)
(24.8, 0)
(24.9, 0)
(25, 0)
(25.1, 0)
(25.2, 0)
(25.3, 0)
(25.4, 0)
(25.5, 0)
(25.6, 0)
(25.7, 0)
(25.8, 0)
(25.9, 0)
(26, 0)
(26.1, 0)
(26.2, 0)
(26.3, 0)
(26.4, 0)
(26.5, 0)
(26.6, 0)
(26.7, 0)
(26.8, 0)
(26.9, 0)
(27, 0)
(27.1, 0)
(27.2, 0)
(27.3, 0)
(27.4, 0)
(27.5, 0)
(27.6, 0)
(27.7, 0)
(27.8, 0)
(27.9, 0)
(28, 0)
(28.1, 0)
(28.2, 0)
(28.3, 0)
(28.4, 0)
(28.5, 0)
(28.6, 0)
(28.7, 0)
(28.8, 0)
(28.9, 0)
(29, 0)
(29.1, 0)
(29.2, 0)
(29.3, 0)
(29.4, 0)
(29.5, 0)
(29.6, 0)
(29.7, 0)
(29.8, 0)
(29.9, 0)
(30, 0)
(30.1, 0)
(30.2, 0)
(30.3, 0)
(30.4, 0)
(30.5, 0)
(30.6, 0)
(30.7, 0)
(30.8, 0)
(30.9, 0)
(31, 0)
(31.1, 0)
(31.2, 0)
(31.3, 0)
(31.4, 0)
(31.5, 0)
(31.6, 0)
(31.7, 0)
(31.8, 0)
(31.9, 0)
(32, 0)
(32.1, 0)
(32.2, 0)
(32.3, 0)
(32.4, 0)
(32.5, 0)
(32.6, 0)
(32.7, 0)
(32.8, 0)
(32.9, 0)
(33, 0)
(33.1, 0)
(33.2, 0)
(33.3, 0)
(33.4, 0)
(33.5, 0)
(33.6, 0)
(33.7, 0)
(33.8, 0)
(33.9, 0)
(34, 0)
(34.1, 0)
(34.2, 0)
(34.3, 0)
(34.4, 0)
(34.5, 0)
(34.6, 0)
(34.7, 0)
(34.8, 0)
(34.9, 0)
(35, 0)
(35.1, 0)
(35.2, 0)
(35.3, 0)
(35.4, 0)
(35.5, 0)
(35.6, 0)
(35.7, 0)
(35.8, 0)
(35.9, 0)
(36, 0)
(36.1, 0)
(36.2, 0)
(36.3, 0)
(36.4, 0)
(36.5, 0)
(36.6, 0)
(36.7, 0)
(36.8, 0)
(36.9, 0)
(37, 0)
(37.1, 0)
(37.2, 0)
(37.3, 0)
(37.4, 0)
(37.5, 0)
(37.6, 0)
(37.7, 0)
(37.8, 0)
(37.9, 0)
(38, 0)
(38.1, 0)
(38.2, 0)
(38.3, 0)
(38.4, 0)
(38.5, 0)
(38.6, 0)
(38.7, 0)
(38.8, 0)
(38.9, 0)
(39, 0)
(39.1, 0)
(39.2, 0)
(39.3, 0)
(39.4, 0)
(39.5, 0)
(39.6, 0)
(39.7, 0)
(39.8, 0)
(39.9, 0)
(40, 0)
(40.1, 0)
(40.2, 0)
(40.3, 0)
(40.4, 0)
(40.5, 0)
(40.6, 0)
(40.7, 0)
(40.8, 0)
(40.9, 0)
(41, 0)
(41.1, 0)
(41.2, 0)
(41.3, 0)
(41.4, 0)
(41.5, 0)
(41.6, 0)
(41.7, 0)
(41.8, 0)
(41.9, 0)
(42, 0)
(42.1, 0)
(42.2, 0)
};

==> exp_plots/open_ws_wind/z.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0, 0)
(0.1, 0.000208607)
(0.2, 0.000158086)
(0.3, 6.43437e-05)
(0.4, -0.000152614)
(0.5, -0.000174939)
(0.6, -0.00016292)
(0.7, -0.00011383)
(0.8, -3.98563e-05)
(0.9, 0.000184377)
(1, 9.9769e-06)
(1.1, 6.99964e-05)
(1.2, -7.02186e-05)
(1.3, -0.000222427)
(1.4, -9.43467e-05)
(1.5, 5.02199e-05)
(1.6, -0.000215479)
(1.7, -0.000327188)
(1.8, -0.00021782)
(1.9, -0.000225335)
(2, -0.00041813)
(2.1, 8.20969e-05)
(2.2, 0.00021452)
(2.3, 0.000360816)
(2.4, 9.16191e-05)
(2.5, 4.40255e-05)
(2.6, -0.000319196)
(2.7, 0.00112426)
(2.8, 0.00278836)
(2.9, 0.00996607)
(3, 0.0203906)
(3.1, 0.026754)
(3.2, 0.034069)
(3.3, 0.0472354)
(3.4, 0.0564735)
(3.5, 0.064197)
(3.6, 0.07536)
(3.7, 0.107074)
(3.8, 0.141795)
(3.9, 0.158939)
(4, 0.162604)
(4.1, 0.168994)
(4.2, 0.186969)
(4.3, 0.210732)
(4.4, 0.217828)
(4.5, 0.230336)
(4.6, 0.24536)
(4.7, 0.251485)
(4.8, 0.265323)
(4.9, 0.276643)
(5, 0.288273)
(5.1, 0.321044)
(5.2, 0.337067)
(5.3, 0.343965)
(5.4, 0.350858)
(5.5, 0.367473)
(5.6, 0.374125)
(5.7, 0.380076)
(5.8, 0.401119)
(5.9, 0.422674)
(6, 0.437193)
(6.1, 0.444758)
(6.2, 0.445774)
(6.3, 0.45595)
(6.4, 0.471866)
(6.5, 0.48762)
(6.6, 0.486831)
(6.7, 0.489653)
(6.8, 0.503454)
(6.9, 0.511525)
(7, 0.516389)
(7.1, 0.521943)
(7.2, 0.52004)
(7.3, 0.523535)
(7.4, 0.529779)
(7.5, 0.538836)
(7.6, 0.543184)
(7.7, 0.53978)
(7.8, 0.526705)
(7.9, 0.501546)
(8, 0.492298)
(8.1, 0.497986)
(8.2, 0.505279)
(8.3, 0.509753)
(8.4, 0.523037)
(8.5, 0.525252)
(8.6, 0.526638)
(8.7, 0.514452)
(8.8, 0.485914)
(8.9, 0.466906)
(9, 0.460105)
(9.1, 0.457884)
(9.2, 0.45585)
(9.3, 0.459016)
(9.4, 0.465099)
(9.5, 0.468335)
(9.6, 0.455509)
(9.7, 0.461307)
(9.8, 0.462314)
(9.9, 0.469035)
(10, 0.473801)
(10.1, 0.483464)
(10.2, 0.488113)
(10.3, 0.487358)
(10.4, 0.49047)
(10.5, 0.490399)
(10.6, 0.482599)
(10.7, 0.479319)
(10.8, 0.479585)
(10.9, 0.481235)
(11, 0.479837)
(11.1, 0.468986)
(11.2, 0.470081)
(11.3, 0.476349)
(11.4, 0.480044)
(11.5, 0.481148)
(11.6, 0.487885)
(11.7, 0.489059)
(11.8, 0.492953)
(11.9, 0.50062)
(12, 0.508432)
(12.1, 0.509121)
(12.2, 0.510318)
(12.3, 0.530057)
(12.4, 0.540116)
(12.5, 0.544767)
(12.6, 0.553324)
(12.7, 0.553658)
(12.8, 0.549337)
(12.9, 0.546514)
(13, 0.530009)
(13.1, 0.526903)
(13.2, 0.522857)
(13.3, 0.523652)
(13.4, 0.520264)
(13.5, 0.510878)
(13.6, 0.506695)
(13.7, 0.50814)
(13.8, 0.504428)
(13.9, 0.497531)
(14, 0.491767)
(14.1, 0.485795)
(14.2, 0.47667)
(14.3, 0.475208)
(14.4, 0.471198)
(14.5, 0.479548)
(14.6, 0.485378)
(14.7, 0.485376)
(14.8, 0.497835)
(14.9, 0.501552)
(15, 0.498787)
(15.1, 0.497898)
(15.2, 0.506634)
(15.3, 0.518118)
(15.4, 0.5154)
(15.5, 0.504081)
(15.6, 0.498863)
(15.7, 0.499688)
(15.8, 0.499861)
(15.9, 0.496059)
(16, 0.496985)
(16.1, 0.492141)
(16.2, 0.499038)
(16.3, 0.504077)
(16.4, 0.498557)
(16.5, 0.49567)
(16.6, 0.49848)
(16.7, 0.509332)
(16.8, 0.520909)
(16.9, 0.526244)
(17, 0.528089)
(17.1, 0.529358)
(17.2, 0.529068)
(17.3, 0.52197)
(17.4, 0.52592)
(17.5, 0.529036)
(17.6, 0.530723)
(17.7, 0.524358)
(17.8, 0.520718)
(17.9, 0.515519)
(18, 0.511761)
(18.1, 0.497502)
(18.2, 0.489334)
(18.3, 0.488895)
(18.4, 0.485894)
(18.5, 0.477729)
(18.6, 0.479119)
(18.7, 0.477071)
(18.8, 0.477022)
(18.9, 0.479487)
(19, 0.480253)
(19.1, 0.484955)
(19.2, 0.488088)
(19.3, 0.488167)
(19.4, 0.473882)
(19.5, 0.483761)
(19.6, 0.487622)
(19.7, 0.486588)
(19.8, 0.494335)
(19.9, 0.511685)
(20, 0.515026)
(20.1, 0.512834)
(20.2, 0.510665)
(20.3, 0.504786)
(20.4, 0.495571)
(20.5, 0.500974)
(20.6, 0.504002)
(20.7, 0.505651)
(20.8, 0.509053)
(20.9, 0.528688)
(21, 0.535688)
(21.1, 0.534502)
(21.2, 0.537204)
(21.3, 0.543901)
(21.4, 0.547956)
(21.5, 0.54867)
(21.6, 0.543082)
(21.7, 0.538908)
(21.8, 0.534974)
(21.9, 0.537223)
(22, 0.541806)
(22.1, 0.538326)
(22.2, 0.539858)
(22.3, 0.538061)
(22.4, 0.531121)
(22.5, 0.524903)
(22.6, 0.513264)
(22.7, 0.508144)
(22.8, 0.506289)
(22.9, 0.501143)
(23, 0.496729)
(23.1, 0.495698)
(23.2, 0.478383)
(23.3, 0.461013)
(23.4, 0.461768)
(23.5, 0.447971)
(23.6, 0.4488)
(23.7, 0.467992)
(23.8, 0.475416)
(23.9, 0.48195)
(24, 0.494404)
(24.1, 0.494778)
(24.2, 0.491659)
(24.3, 0.486736)
(24.4, 0.491329)
(24.5, 0.484788)
(24.6, 0.460575)
(24.7, 0.452753)
(24.8, 0.448937)
(24.9, 0.449715)
(25, 0.451216)
(25.1, 0.450315)
(25.2, 0.452238)
(25.3, 0.455003)
(25.4, 0.455368)
(25.5, 0.450324)
(25.6, 0.44363)
(25.7, 0.44644)
(25.8, 0.447648)
(25.9, 0.451092)
(26, 0.455875)
(26.1, 0.460795)
(26.2, 0.461833)
(26.3, 0.458537)
(26.4, 0.456244)
(26.5, 0.458152)
(26.6, 0.467245)
(26.7, 0.473216)
(26.8, 0.476489)
(26.9, 0.476927)
(27, 0.470209)
(27.1, 0.463941)
(27.2, 0.463411)
(27.3, 0.449858)
(27.4, 0.443942)
(27.5, 0.434759)
(27.6, 0.431985)
(27.7, 0.434584)
(27.8, 0.429383)
(27.9, 0.425785)
(28, 0.423325)
(28.1, 0.416291)
(28.2, 0.404636)
(28.3, 0.38745)
(28.4, 0.374749)
(28.5, 0.369631)
(28.6, 0.366997)
(28.7, 0.365938)
(28.8, 0.355835)
(28.9, 0.325)
(29, 0.302646)
(29.1, 0.295125)
(29.2, 0.287113)
(29.3, 0.27758)
(29.4, 0.276824)
(29.5, 0.278783)
(29.6, 0.277846)
(29.7, 0.278601)
(29.8, 0.277126)
(29.9, 0.271871)
(30, 0.262892)
(30.1, 0.255068)
(30.2, 0.24808)
(30.3, 0.235147)
(30.4, 0.22903)
(30.5, 0.224183)
(30.6, 0.211608)
(30.7, 0.200279)
(30.8, 0.1981)
(30.9, 0.194045)
(31, 0.192773)
(31.1, 0.190211)
(31.2, 0.180591)
(31.3, 0.17426)
(31.4, 0.163651)
(31.5, 0.151853)
(31.6, 0.143143)
(31.7, 0.138281)
(31.8, 0.148064)
(31.9, 0.153009)
(32, 0.149393)
(32.1, 0.145313)
(32.2, 0.143424)
(32.3, 0.138653)
(32.4, 0.13164)
(32.5, 0.122874)
(32.6, 0.109291)
(32.7, 0.101602)
(32.8, 0.0926089)
(32.9, 0.0889206)
(33, 0.0876909)
(33.1, 0.0869716)
(33.2, 0.0817592)
(33.3, 0.0720499)
(33.4, 0.0626842)
(33.5, 0.0556754)
(33.6, 0.0531743)
(33.7, 0.0525333)
(33.8, 0.0360285)
(33.9, 0.0193182)
(34, 0.0174488)
(34.1, 0.0139569)
(34.2, 0.0184338)
(34.3, 0.0165843)
(34.4, 0.0154313)
(34.5, 0.020238)
(34.6, 0.0154445)
(34.7, 0.00880587)
(34.8, 0.00825125)
(34.9, 0.0121531)
(35, 0.0131086)
(35.1, 0.0110072)
(35.2, 0.014103)
(35.3, 0.0170208)
(35.4, 0.0172321)
(35.5, 0.016239)
(35.6, 0.013681)
(35.7, 0.0133141)
(35.8, 0.0135389)
(35.9, 0.0138735)
(36, 0.0138732)
(36.1, 0.0143776)
(36.2, 0.0140887)
(36.3, 0.0128506)
(36.4, 0.0127668)
(36.5, 0.0129144)
(36.6, 0.00860263)
(36.7, 0.00748029)
(36.8, 0.00917146)
(36.9, 0.0122767)
(37, 0.0115172)
(37.1, 0.0112872)
(37.2, 0.0119158)
(37.3, 0.0112815)
(37.4, 0.0111702)
(37.5, 0.010519)
(37.6, 0.0102472)
(37.7, 0.0100473)
(37.8, 0.00994227)
(37.9, 0.00998753)
(38, 0.0101901)
(38.1, 0.0107413)
(38.2, 0.0113801)
(38.3, 0.0109884)
(38.4, 0.010608)
(38.5, 0.0109859)
(38.6, 0.0114164)
(38.7, 0.0106108)
(38.8, 0.0110429)
(38.9, 0.0115082)
(39, 0.0111983)
(39.1, 0.0109976)
(39.2, 0.0108784)
(39.3, 0.0110298)
(39.4, 0.0108848)
(39.5, 0.00487853)
(39.6, 0.00347074)
(39.7, 0.00255157)
(39.8, 0.00247938)
(39.9, 0.00170662)
(40, 0.000692448)
(40.1, 0.00017571)
(40.2, 3.9413e-05)
(40.3, 0.000164616)
(40.4, 0.000379309)
(40.5, 0.000663532)
(40.6, 0.00122889)
(40.7, 0.00130763)
(40.8, 0.00132436)
(40.9, 0.000717395)
(41, 9.02013e-05)
(41.1, -0.000140815)
(41.2, -0.000211766)
(41.3, -0.000545166)
(41.4, -0.000194763)
(41.5, -7.69738e-05)
(41.6, 3.91056e-07)
(41.7, 0.000324018)
(41.8, 0.000389952)
(41.9, 0.00044041)
(42, 0.000680826)
(42.1, -0.003635)
(42.2, -0.003252)
};

==> exp_plots/open_ws_wind/z_des.tex <==
\addplot[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates {
(0, 0)
(0.1, 0)
(0.2, 0)
(0.3, 0)
(0.4, 0)
(0.5, 0)
(0.6, 0)
(0.7, 0)
(0.8, 0)
(0.9, 0)
(1, 0)
(1.1, 0)
(1.2, 0)
(1.3, 0)
(1.4, 0)
(1.5, 0)
(1.6, 0)
(1.7, 0)
(1.8, 0)
(1.9, 0)
(2, 0)
(2.1, 0)
(2.2, 0)
(2.3, 0)
(2.4, 0)
(2.5, 0)
(2.6, 0)
(2.7, 0)
(2.8, 0)
(2.9, 0)
(3, 0)
(3.1, 0)
(3.2, 0)
(3.3, 0)
(3.4, 0)
(3.5, 0)
(3.6, 0)
(3.7, 0)
(3.8, 0)
(3.9, 0)
(4, 0)
(4.1, 0)
(4.2, 0)
(4.3, 0)
(4.4, 0)
(4.5, 0)
(4.6, 0)
(4.7, 0)
(4.8, 0)
(4.9, 0)
(5, 0)
(5.1, 0)
(5.2, 0)
(5.3, 0)
(5.4, 0)
(5.5, 0)
(5.6, 0)
(5.7, 0)
(5.8, 0)
(5.9, 0)
(6, 0)
(6.1, 0)
(6.2, 0)
(6.3, 0)
(6.4, 0.5)
(6.5, 0.5)
(6.6, 0.5)
(6.7, 0.5)
(6.8, 0.5)
(6.9, 0.5)
(7, 0.5)
(7.1, 0.5)
(7.2, 0.5)
(7.3, 0.5)
(7.4, 0.5)
(7.5, 0.5)
(7.6, 0.5)
(7.7, 0.5)
(7.8, 0.5)
(7.9, 0.5)
(8, 0.5)
(8.1, 0.5)
(8.2, 0.5)
(8.3, 0.5)
(8.4, 0.5)
(8.5, 0.5)
(8.6, 0.5)
(8.7, 0.5)
(8.8, 0.5)
(8.9, 0.5)
(9, 0.5)
(9.1, 0.5)
(9.2, 0.5)
(9.3, 0.5)
(9.4, 0.5)
(9.5, 0.5)
(9.6, 0.5)
(9.7, 0.5)
(9.8, 0.5)
(9.9, 0.5)
(10, 0.5)
(10.1, 0.5)
(10.2, 0.5)
(10.3, 0.5)
(10.4, 0.5)
(10.5, 0.5)
(10.6, 0.5)
(10.7, 0.5)
(10.8, 0.5)
(10.9, 0.5)
(11, 0.5)
(11.1, 0.5)
(11.2, 0.5)
(11.3, 0.5)
(11.4, 0.5)
(11.5, 0.5)
(11.6, 0.5)
(11.7, 0.5)
(11.8, 0.5)
(11.9, 0.5)
(12, 0.5)
(12.1, 0.5)
(12.2, 0.5)
(12.3, 0.5)
(12.4, 0.5)
(12.5, 0.5)
(12.6, 0.5)
(12.7, 0.5)
(12.8, 0.5)
(12.9, 0.5)
(13, 0.5)
(13.1, 0.5)
(13.2, 0.5)
(13.3, 0.5)
(13.4, 0.5)
(13.5, 0.5)
(13.6, 0.5)
(13.7, 0.5)
(13.8, 0.5)
(13.9, 0.5)
(14, 0.5)
(14.1, 0.5)
(14.2, 0.5)
(14.3, 0.5)
(14.4, 0.5)
(14.5, 0.5)
(14.6, 0.5)
(14.7, 0.5)
(14.8, 0.5)
(14.9, 0.5)
(15, 0.5)
(15.1, 0.5)
(15.2, 0.5)
(15.3, 0.5)
(15.4, 0.5)
(15.5, 0.5)
(15.6, 0.5)
(15.7, 0.5)
(15.8, 0.5)
(15.9, 0.5)
(16, 0.5)
(16.1, 0.5)
(16.2, 0.5)
(16.3, 0.5)
(16.4, 0.5)
(16.5, 0.5)
(16.6, 0.5)
(16.7, 0.5)
(16.8, 0.5)
(16.9, 0.5)
(17, 0.5)
(17.1, 0.5)
(17.2, 0.5)
(17.3, 0.5)
(17.4, 0.5)
(17.5, 0.5)
(17.6, 0.5)
(17.7, 0.5)
(17.8, 0.5)
(17.9, 0.5)
(18, 0.5)
(18.1, 0.5)
(18.2, 0.5)
(18.3, 0.5)
(18.4, 0.5)
(18.5, 0.5)
(18.6, 0.5)
(18.7, 0.5)
(18.8, 0.5)
(18.9, 0.5)
(19, 0.5)
(19.1, 0.5)
(19.2, 0.5)
(19.3, 0.5)
(19.4, 0.5)
(19.5, 0.5)
(19.6, 0.5)
(19.7, 0.5)
(19.8, 0.5)
(19.9, 0.5)
(20, 0.5)
(20.1, 0.5)
(20.2, 0.5)
(20.3, 0.5)
(20.4, 0.5)
(20.5, 0.5)
(20.6, 0.5)
(20.7, 0.5)
(20.8, 0.5)
(20.9, 0.5)
(21, 0.5)
(21.1, 0.5)
(21.2, 0.5)
(21.3, 0.5)
(21.4, 0.5)
(21.5, 0.5)
(21.6, 0.5)
(21.7, 0.5)
(21.8, 0.5)
(21.9, 0.5)
(22, 0.5)
(22.1, 0.5)
(22.2, 0.5)
(22.3, 0.5)
(22.4, 0.5)
(22.5, 0.5)
(22.6, 0.5)
(22.7, 0.5)
(22.8, 0.5)
(22.9, 0.5)
(23, 0.5)
(23.1, 0.5)
(23.2, 0.5)
(23.3, 0.5)
(23.4, 0.5)
(23.5, 0.5)
(23.6, 0.5)
(23.7, 0.5)
(23.8, 0.5)
(23.9, 0.5)
(24, 0.5)
(24.1, 0.5)
(24.2, 0.5)
(24.3, 0.5)
(24.4, 0.5)
(24.5, 0.5)
(24.6, 0.5)
(24.7, 0.5)
(24.8, 0.5)
(24.9, 0.5)
(25, 0.5)
(25.1, 0.5)
(25.2, 0.5)
(25.3, 0.5)
(25.4, 0.5)
(25.5, 0.5)
(25.6, 0.5)
(25.7, 0.5)
(25.8, 0.5)
(25.9, 0.5)
(26, 0.5)
(26.1, 0.5)
(26.2, 0.5)
(26.3, 0.5)
(26.4, 0)
(26.5, 0)
(26.6, 0)
(26.7, 0)
(26.8, 0)
(26.9, 0)
(27, 0)
(27.1, 0)
(27.2, 0)
(27.3, 0)
(27.4, 0)
(27.5, 0)
(27.6, 0)
(27.7, 0)
(27.8, 0)
(27.9, 0)
(28, 0)
(28.1, 0)
(28.2, 0)
(28.3, 0)
(28.4, 0)
(28.5, 0)
(28.6, 0)
(28.7, 0)
(28.8, 0)
(28.9, 0)
(29, 0)
(29.1, 0)
(29.2, 0)
(29.3, 0)
(29.4, 0)
(29.5, 0)
(29.6, 0)
(29.7, 0)
(29.8, 0)
(29.9, 0)
(30, 0)
(30.1, 0)
(30.2, 0)
(30.3, 0)
(30.4, 0)
(30.5, 0)
(30.6, 0)
(30.7, 0)
(30.8, 0)
(30.9, 0)
(31, 0)
(31.1, 0)
(31.2, 0)
(31.3, 0)
(31.4, 0)
(31.5, 0)
(31.6, 0)
(31.7, 0)
(31.8, 0)
(31.9, 0)
(32, 0)
(32.1, 0)
(32.2, 0)
(32.3, 0)
(32.4, 0)
(32.5, 0)
(32.6, 0)
(32.7, 0)
(32.8, 0)
(32.9, 0)
(33, 0)
(33.1, 0)
(33.2, 0)
(33.3, 0)
(33.4, 0)
(33.5, 0)
(33.6, 0)
(33.7, 0)
(33.8, 0)
(33.9, 0)
(34, 0)
(34.1, 0)
(34.2, 0)
(34.3, 0)
(34.4, 0)
(34.5, 0)
(34.6, 0)
(34.7, 0)
(34.8, 0)
(34.9, 0)
(35, 0)
(35.1, 0)
(35.2, 0)
(35.3, 0)
(35.4, 0)
(35.5, 0)
(35.6, 0)
(35.7, 0)
(35.8, 0)
(35.9, 0)
(36, 0)
(36.1, 0)
(36.2, 0)
(36.3, 0)
(36.4, 0)
(36.5, 0)
(36.6, 0)
(36.7, 0)
(36.8, 0)
(36.9, 0)
(37, 0)
(37.1, 0)
(37.2, 0)
(37.3, 0)
(37.4, 0)
(37.5, 0)
(37.6, 0)
(37.7, 0)
(37.8, 0)
(37.9, 0)
(38, 0)
(38.1, 0)
(38.2, 0)
(38.3, 0)
(38.4, 0)
(38.5, 0)
(38.6, 0)
(38.7, 0)
(38.8, 0)
(38.9, 0)
(39, 0)
(39.1, 0)
(39.2, 0)
(39.3, 0)
(39.4, 0)
(39.5, 0)
(39.6, 0)
(39.7, 0)
(39.8, 0)
(39.9, 0)
(40, 0)
(40.1, 0)
(40.2, 0)
(40.3, 0)
(40.4, 0)
(40.5, 0)
(40.6, 0)
(40.7, 0)
(40.8, 0)
(40.9, 0)
(41, 0)
(41.1, 0)
(41.2, 0)
(41.3, 0)
(41.4, 0)
(41.5, 0)
(41.6, 0)
(41.7, 0)
(41.8, 0)
(41.9, 0)
(42, 0)
(42.1, 0)
(42.2, 0)
};

==> exp_plots/payload_comparison/th_da.tex <==
\addplot[
    fill=white!60!clr1,draw = clr1,opacity=\opacty,
    line width= \linew pt,
    forget plot
    ]
 %%
coordinates {
(0,0)
(0, 50.817)
(0.00240249, 49.8785)
(0.00480497, 49.2196)
(0.00720746, 50.4277)
(0.00960995, 51.1479)
(0.0120124, 50.8579)
(0.0144149, 51.391)
(0.0168174, 52.7728)
(0.0192199, 52.735)
(0.0216224, 53.8893)
(0.0240249, 53.862)
(0.0264274, 54.8011)
(0.0288298, 54.0926)
(0.0312323, 53.9778)
(0.0336348, 55.3252)
(0.0360373, 55.7092)
(0.0384398, 54.2923)
(0.0408423, 53.6594)
(0.0432448, 54.327)
(0.0456473, 54.3652)
(0.0480497, 53.6502)
(0.0504522, 53.7682)
(0.0528547, 54.7825)
(0.0552572, 54.2573)
(0.0576597, 53.9406)
(0.0600622, 54.3773)
(0.0624647, 53.76)
(0.0648672, 52.7569)
(0.0672696, 53.8472)
(0.0696721, 53.3546)
(0.0720746, 53.0093)
(0.0744771, 53.1487)
(0.0768796, 52.8214)
(0.0792821, 53.1229)
(0.0816846, 53.3211)
(0.0840871, 52.1602)
(0.0864895, 51.2047)
(0.088892, 51.2498)
(0.0912945, 52.8795)
(0.093697, 52.0624)
(0.0960995, 52.3694)
(0.098502, 51.3591)
(0.100904, 51.7798)
(0.103307, 52.3737)
(0.105709, 50.7122)
(0.108112, 52.1789)
(0.110514, 51.8146)
(0.112917, 51.7408)
(0.115319, 51.5536)
(0.117722, 51.0967)
(0.120124, 51.7504)
(0.122527, 51.7644)
(0.124929, 54.1239)
(0.127332, 52.8352)
(0.129734, 52.5327)
(0.132137, 54.6659)
(0.134539, 53.6313)
(0.136942, 53.3761)
(0.139344, 52.9541)
(0.141747, 53.3891)
(0.144149, 52.2848)
(0.146552, 51.7934)
(0.148954, 51.8272)
(0.151357, 52.9012)
(0.153759, 54.2535)
(0.156162, 54.1025)
(0.158564, 54.0349)
(0.160967, 56.3852)
(0.163369, 54.906)
(0.165772, 57.1672)
(0.168174, 55.0451)
(0.170577, 54.9892)
(0.172979, 55.1833)
(0.175382, 56.0011)
(0.177784, 54.6875)
(0.180187, 53.9984)
(0.182589, 54.1126)
(0.184992, 54.0508)
(0.187394, 54.2784)
(0.189796, 53.6437)
(0.192199, 54.683)
(0.194601, 54.0025)
(0.197004, 54.5952)
(0.199406, 54.4953)
(0.201809, 54.9186)
(0.204211, 56.6575)
(0.206614, 55.844)
(0.209016, 56.1863)
(0.211419, 56.8831)
(0.213821, 56.3262)
(0.216224, 55.3038)
(0.218626, 55.0177)
(0.221029, 55.6052)
(0.223431, 56.4995)
(0.225834, 55.4526)
(0.228236, 55.2796)
(0.230639, 54.817)
(0.233041, 55.364)
(0.235444, 55.1142)
(0.237846, 55.2587)
(0.240249, 55.2189)
(0.242651, 54.1437)
(0.245054, 52.9872)
(0.247456, 52.6507)
(0.249859, 53.91)
(0.252261, 53.0779)
(0.254664, 49.9907)
(0.257066, 54.1164)
(0.259469, 53.8463)
(0.261871, 50.5569)
(0.264274, 49.6006)
(0.266676, 51.4325)
(0.269079, 51.9031)
(0.271481, 52.7205)
(0.273884, 52.886)
(0.276286, 53.7071)
(0.278689, 51.887)
(0.281091, 51.9865)
(0.283493, 53.9679)
(0.285896, 53.3491)
(0.288298, 53.0756)
(0.290701, 52.8854)
(0.293103, 52.8312)
(0.295506, 53.457)
(0.297908, 53.7952)
(0.300311, 53.4034)
(0.302713, 53.1838)
(0.305116, 53.2309)
(0.307518, 53.3982)
(0.309921, 52.166)
(0.312323, 52.1001)
(0.314726, 52.9763)
(0.317128, 52.7816)
(0.319531, 51.8799)
(0.321933, 50.7035)
(0.324336, 50.6519)
(0.326738, 52.2816)
(0.329141, 52.3354)
(0.331543, 52.5069)
(0.333946, 52.7863)
(0.336348, 52.7046)
(0.338751, 52.106)
(0.341153, 52.0735)
(0.343556, 52.5132)
(0.345958, 53.2113)
(0.348361, 54.3199)
(0.350763, 55.4481)
(0.353166, 57.8406)
(0.355568, 56.4792)
(0.357971, 55.5226)
(0.360373, 55.3965)
(0.362776, 55.0202)
(0.365178, 54.6238)
(0.367581, 53.1067)
(0.369983, 53.8361)
(0.372386, 52.2619)
(0.374788, 51.7385)
(0.37719, 52.3598)
(0.379593, 53.2113)
(0.381995, 52.791)
(0.384398, 53.15)
(0.3868, 53.7784)
(0.389203, 53.3454)
(0.391605, 53.3586)
(0.394008, 54.3482)
(0.39641, 54.4115)
(0.398813, 54.4332)
(0.401215, 54.6086)
(0.403618, 54.2629)
(0.40602, 55.4395)
(0.408423, 54.4341)
(0.410825, 54.8126)
(0.413228, 55.0006)
(0.41563, 54.0336)
(0.418033, 53.956)
(0.420435, 53.8421)
(0.422838, 53.166)
(0.42524, 51.4719)
(0.427643, 53.1798)
(0.430045, 51.1631)
(0.432448, 52.6687)
(0.43485, 52.8979)
(0.437253, 51.6808)
(0.439655, 52.5335)
(0.442058, 51.5967)
(0.44446, 52.1812)
(0.446863, 52.1684)
(0.449265, 52.827)
(0.451668, 52.7019)
(0.45407, 53.1087)
(0.456473, 54.667)
(0.458875, 55.6155)
(0.461278, 54.8591)
(0.46368, 54.2727)
(0.466083, 54.1417)
(0.468485, 53.4936)
(0.470887, 54.9565)
(0.47329, 54.0594)
(0.475692, 54.3598)
(0.478095, 54.6182)
(0.480497, 55.4987)
(0.4829, 55.3744)
(0.485302, 54.7568)
(0.487705, 55.507)
(0.490107, 55.267)
(0.49251, 55.3898)
(0.494912, 54.4106)
(0.497315, 54.5606)
(0.499717, 54.3988)
(0.50212, 54.6425)
(0.504522, 54.9485)
(0.506925, 55.0834)
(0.509327, 55.2854)
(0.51173, 56.385)
(0.514132, 57.012)
(0.516535, 57.244)
(0.518937, 57.6249)
(0.52134, 57.3885)
(0.523742, 56.9752)
(0.526145, 56.8716)
(0.528547, 56.27)
(0.53095, 55.0087)
(0.533352, 55.6115)
(0.535755, 56.4756)
(0.538157, 55.8232)
(0.54056, 56.3478)
(0.542962, 57.0028)
(0.545365, 56.202)
(0.547767, 56.249)
(0.55017, 56.0911)
(0.552572, 56.4754)
(0.554975, 56.6244)
(0.557377, 56.3324)
(0.55978, 56.3123)
(0.562182, 55.6431)
(0.564584, 56.0113)
(0.566987, 55.5299)
(0.569389, 55.7712)
(0.571792, 53.2299)
(0.574194, 55.0123)
(0.576597, 55.7478)
(0.578999, 55.2605)
(0.581402, 53.4798)
(0.583804, 52.5908)
(0.586207, 53.7761)
(0.588609, 53.1793)
(0.591012, 51.8242)
(0.593414, 53.2121)
(0.595817, 52.7432)
(0.598219, 52.8926)
(0.600622, 52.6999)
(0.603024, 52.0458)
(0.605427, 51.6695)
(0.607829, 50.7796)
(0.610232, 51.6508)
(0.612634, 51.9156)
(0.615037, 51.8125)
(0.617439, 52.9024)
(0.619842, 52.3479)
(0.622244, 52.957)
(0.624647, 57.0759)
(0.627049, 54.302)
(0.629452, 56.5825)
(0.631854, 55.537)
(0.634257, 55.1987)
(0.636659, 55.2872)
(0.639062, 55.0077)
(0.641464, 55.2112)
(0.643867, 54.6582)
(0.646269, 55.4981)
(0.648672, 53.9936)
(0.651074, 54.3183)
(0.653477, 54.0541)
(0.655879, 52.7564)
(0.658282, 52.6545)
(0.660684, 52.4157)
(0.663086, 52.9387)
(0.665489, 53.5741)
(0.667891, 53.6038)
(0.670294, 53.4613)
(0.672696, 54.0385)
(0.675099, 53.0067)
(0.677501, 52.9701)
(0.679904, 52.4529)
(0.682306, 51.9506)
(0.684709, 52.2015)
(0.687111, 51.134)
(0.689514, 52.3609)
(0.691916, 52.9931)
(0.694319, 53.5505)
(0.696721, 53.9292)
(0.699124, 55.5823)
(0.701526, 53.7648)
(0.703929, 53.3672)
(0.706331, 54.5661)
(0.708734, 53.6829)
(0.711136, 53.1579)
(0.713539, 53.9195)
(0.715941, 53.5475)
(0.718344, 53.4106)
(0.720746, 53.0292)
(0.723149, 53.0835)
(0.725551, 51.563)
(0.727954, 52.4892)
(0.730356, 52.4012)
(0.732759, 51.1453)
(0.735161, 50.569)
(0.737564, 51.1441)
(0.739966, 51.426)
(0.742369, 52.2706)
(0.744771, 53.0943)
(0.747173, 52.0464)
(0.749576, 54.753)
(0.751978, 54.6539)
(0.754381, 52.8061)
(0.756783, 53.5233)
(0.759186, 52.7256)
(0.761588, 52.9817)
(0.763991, 53.4137)
(0.766393, 53.0209)
(0.768796, 53.4145)
(0.771198, 53.7206)
(0.773601, 53.9439)
(0.776003, 54.0871)
(0.778406, 53.6312)
(0.780808, 53.4159)
(0.783211, 52.911)
(0.785613, 53.4137)
(0.788016, 52.9157)
(0.790418, 53.1411)
(0.792821, 52.027)
(0.795223, 52.7136)
(0.797626, 50.2111)
(0.800028, 52.6417)
(0.802431, 51.8418)
(0.804833, 50.4237)
(0.807236, 51.1208)
(0.809638, 52.1229)
(0.812041, 52.4042)
(0.814443, 51.8879)
(0.816846, 52.8071)
(0.819248, 52.1462)
(0.821651, 52.7071)
(0.824053, 52.7338)
(0.826456, 53.281)
(0.828858, 51.9714)
(0.831261, 52.1646)
(0.833663, 52.2521)
(0.836066, 54.1155)
(0.838468, 54.2944)
(0.840871, 54.3928)
(0.843273, 54.1329)
(0.845675, 54.4759)
(0.848078, 53.8136)
(0.85048, 54.5783)
(0.852883, 54.3834)
(0.855285, 53.0142)
(0.857688, 52.5977)
(0.86009, 52.4864)
(0.862493, 52.6224)
(0.864895, 51.4766)
(0.867298, 51.8197)
(0.8697, 52.2827)
(0.872103, 52.1993)
(0.874505, 52.5381)
(0.876908, 52.0597)
(0.87931, 51.9872)
(0.881713, 52.241)
(0.884115, 52.9631)
(0.886518, 52.6876)
(0.88892, 54.5283)
(0.891323, 54.3782)
(0.893725, 52.8215)
(0.896128, 53.1921)
(0.89853, 52.2839)
(0.900933, 52.8544)
(0.903335, 53.2336)
(0.905738, 53.2557)
(0.90814, 53.4611)
(0.910543, 53.5582)
(0.912945, 53.1023)
(0.915348, 53.3357)
(0.91775, 54.1126)
(0.920153, 54.7829)
(0.922555, 54.1364)
(0.924958, 53.745)
(0.92736, 53.9846)
(0.929763, 53.6307)
(0.932165, 53.6616)
(0.934568, 53.5522)
(0.93697, 53.418)
(0.939372, 53.0132)
(0.941775, 53.3917)
(0.944178, 54.1194)
(0.94658, 52.3014)
(0.948982, 52.4401)
(0.951385, 51.9568)
(0.953787, 51.8498)
(0.95619, 51.5853)
(0.958592, 51.8137)
(0.960995, 51.4196)
(0.963397, 51.6495)
(0.9658, 51.6967)
(0.968202, 51.9059)
(0.970605, 51.5685)
(0.973007, 51.7232)
(0.97541, 52.1536)
(0.977812, 52.5397)
(0.980215, 52.1365)
(0.982617, 52.2437)
(0.98502, 53.0395)
(0.987422, 53.0201)
(0.989825, 53.5561)
(0.992227, 52.0756)
(0.99463, 51.5694)
(0.997032, 51.2252)
(0.999435, 51.4666)
(1, 0)
};

==> exp_plots/payload_comparison/th_da_no_fill.tex <==
\addplot[
    fill=none,draw = clr1,opacity=1.0,
    line width= \linew pt
    ]
 %%
coordinates {
(0, 0)
(0, 50.817)
(0.00240249, 49.8785)
(0.00480497, 49.2196)
(0.00720746, 50.4277)
(0.00960995, 51.1479)
(0.0120124, 50.8579)
(0.0144149, 51.391)
(0.0168174, 52.7728)
(0.0192199, 52.735)
(0.0216224, 53.8893)
(0.0240249, 53.862)
(0.0264274, 54.8011)
(0.0288298, 54.0926)
(0.0312323, 53.9778)
(0.0336348, 55.3252)
(0.0360373, 55.7092)
(0.0384398, 54.2923)
(0.0408423, 53.6594)
(0.0432448, 54.327)
(0.0456473, 54.3652)
(0.0480497, 53.6502)
(0.0504522, 53.7682)
(0.0528547, 54.7825)
(0.0552572, 54.2573)
(0.0576597, 53.9406)
(0.0600622, 54.3773)
(0.0624647, 53.76)
(0.0648672, 52.7569)
(0.0672696, 53.8472)
(0.0696721, 53.3546)
(0.0720746, 53.0093)
(0.0744771, 53.1487)
(0.0768796, 52.8214)
(0.0792821, 53.1229)
(0.0816846, 53.3211)
(0.0840871, 52.1602)
(0.0864895, 51.2047)
(0.088892, 51.2498)
(0.0912945, 52.8795)
(0.093697, 52.0624)
(0.0960995, 52.3694)
(0.098502, 51.3591)
(0.100904, 51.7798)
(0.103307, 52.3737)
(0.105709, 50.7122)
(0.108112, 52.1789)
(0.110514, 51.8146)
(0.112917, 51.7408)
(0.115319, 51.5536)
(0.117722, 51.0967)
(0.120124, 51.7504)
(0.122527, 51.7644)
(0.124929, 54.1239)
(0.127332, 52.8352)
(0.129734, 52.5327)
(0.132137, 54.6659)
(0.134539, 53.6313)
(0.136942, 53.3761)
(0.139344, 52.9541)
(0.141747, 53.3891)
(0.144149, 52.2848)
(0.146552, 51.7934)
(0.148954, 51.8272)
(0.151357, 52.9012)
(0.153759, 54.2535)
(0.156162, 54.1025)
(0.158564, 54.0349)
(0.160967, 56.3852)
(0.163369, 54.906)
(0.165772, 57.1672)
(0.168174, 55.0451)
(0.170577, 54.9892)
(0.172979, 55.1833)
(0.175382, 56.0011)
(0.177784, 54.6875)
(0.180187, 53.9984)
(0.182589, 54.1126)
(0.184992, 54.0508)
(0.187394, 54.2784)
(0.189796, 53.6437)
(0.192199, 54.683)
(0.194601, 54.0025)
(0.197004, 54.5952)
(0.199406, 54.4953)
(0.201809, 54.9186)
(0.204211, 56.6575)
(0.206614, 55.844)
(0.209016, 56.1863)
(0.211419, 56.8831)
(0.213821, 56.3262)
(0.216224, 55.3038)
(0.218626, 55.0177)
(0.221029, 55.6052)
(0.223431, 56.4995)
(0.225834, 55.4526)
(0.228236, 55.2796)
(0.230639, 54.817)
(0.233041, 55.364)
(0.235444, 55.1142)
(0.237846, 55.2587)
(0.240249, 55.2189)
(0.242651, 54.1437)
(0.245054, 52.9872)
(0.247456, 52.6507)
(0.249859, 53.91)
(0.252261, 53.0779)
(0.254664, 49.9907)
(0.257066, 54.1164)
(0.259469, 53.8463)
(0.261871, 50.5569)
(0.264274, 49.6006)
(0.266676, 51.4325)
(0.269079, 51.9031)
(0.271481, 52.7205)
(0.273884, 52.886)
(0.276286, 53.7071)
(0.278689, 51.887)
(0.281091, 51.9865)
(0.283493, 53.9679)
(0.285896, 53.3491)
(0.288298, 53.0756)
(0.290701, 52.8854)
(0.293103, 52.8312)
(0.295506, 53.457)
(0.297908, 53.7952)
(0.300311, 53.4034)
(0.302713, 53.1838)
(0.305116, 53.2309)
(0.307518, 53.3982)
(0.309921, 52.166)
(0.312323, 52.1001)
(0.314726, 52.9763)
(0.317128, 52.7816)
(0.319531, 51.8799)
(0.321933, 50.7035)
(0.324336, 50.6519)
(0.326738, 52.2816)
(0.329141, 52.3354)
(0.331543, 52.5069)
(0.333946, 52.7863)
(0.336348, 52.7046)
(0.338751, 52.106)
(0.341153, 52.0735)
(0.343556, 52.5132)
(0.345958, 53.2113)
(0.348361, 54.3199)
(0.350763, 55.4481)
(0.353166, 57.8406)
(0.355568, 56.4792)
(0.357971, 55.5226)
(0.360373, 55.3965)
(0.362776, 55.0202)
(0.365178, 54.6238)
(0.367581, 53.1067)
(0.369983, 53.8361)
(0.372386, 52.2619)
(0.374788, 51.7385)
(0.37719, 52.3598)
(0.379593, 53.2113)
(0.381995, 52.791)
(0.384398, 53.15)
(0.3868, 53.7784)
(0.389203, 53.3454)
(0.391605, 53.3586)
(0.394008, 54.3482)
(0.39641, 54.4115)
(0.398813, 54.4332)
(0.401215, 54.6086)
(0.403618, 54.2629)
(0.40602, 55.4395)
(0.408423, 54.4341)
(0.410825, 54.8126)
(0.413228, 55.0006)
(0.41563, 54.0336)
(0.418033, 53.956)
(0.420435, 53.8421)
(0.422838, 53.166)
(0.42524, 51.4719)
(0.427643, 53.1798)
(0.430045, 51.1631)
(0.432448, 52.6687)
(0.43485, 52.8979)
(0.437253, 51.6808)
(0.439655, 52.5335)
(0.442058, 51.5967)
(0.44446, 52.1812)
(0.446863, 52.1684)
(0.449265, 52.827)
(0.451668, 52.7019)
(0.45407, 53.1087)
(0.456473, 54.667)
(0.458875, 55.6155)
(0.461278, 54.8591)
(0.46368, 54.2727)
(0.466083, 54.1417)
(0.468485, 53.4936)
(0.470887, 54.9565)
(0.47329, 54.0594)
(0.475692, 54.3598)
(0.478095, 54.6182)
(0.480497, 55.4987)
(0.4829, 55.3744)
(0.485302, 54.7568)
(0.487705, 55.507)
(0.490107, 55.267)
(0.49251, 55.3898)
(0.494912, 54.4106)
(0.497315, 54.5606)
(0.499717, 54.3988)
(0.50212, 54.6425)
(0.504522, 54.9485)
(0.506925, 55.0834)
(0.509327, 55.2854)
(0.51173, 56.385)
(0.514132, 57.012)
(0.516535, 57.244)
(0.518937, 57.6249)
(0.52134, 57.3885)
(0.523742, 56.9752)
(0.526145, 56.8716)
(0.528547, 56.27)
(0.53095, 55.0087)
(0.533352, 55.6115)
(0.535755, 56.4756)
(0.538157, 55.8232)
(0.54056, 56.3478)
(0.542962, 57.0028)
(0.545365, 56.202)
(0.547767, 56.249)
(0.55017, 56.0911)
(0.552572, 56.4754)
(0.554975, 56.6244)
(0.557377, 56.3324)
(0.55978, 56.3123)
(0.562182, 55.6431)
(0.564584, 56.0113)
(0.566987, 55.5299)
(0.569389, 55.7712)
(0.571792, 53.2299)
(0.574194, 55.0123)
(0.576597, 55.7478)
(0.578999, 55.2605)
(0.581402, 53.4798)
(0.583804, 52.5908)
(0.586207, 53.7761)
(0.588609, 53.1793)
(0.591012, 51.8242)
(0.593414, 53.2121)
(0.595817, 52.7432)
(0.598219, 52.8926)
(0.600622, 52.6999)
(0.603024, 52.0458)
(0.605427, 51.6695)
(0.607829, 50.7796)
(0.610232, 51.6508)
(0.612634, 51.9156)
(0.615037, 51.8125)
(0.617439, 52.9024)
(0.619842, 52.3479)
(0.622244, 52.957)
(0.624647, 57.0759)
(0.627049, 54.302)
(0.629452, 56.5825)
(0.631854, 55.537)
(0.634257, 55.1987)
(0.636659, 55.2872)
(0.639062, 55.0077)
(0.641464, 55.2112)
(0.643867, 54.6582)
(0.646269, 55.4981)
(0.648672, 53.9936)
(0.651074, 54.3183)
(0.653477, 54.0541)
(0.655879, 52.7564)
(0.658282, 52.6545)
(0.660684, 52.4157)
(0.663086, 52.9387)
(0.665489, 53.5741)
(0.667891, 53.6038)
(0.670294, 53.4613)
(0.672696, 54.0385)
(0.675099, 53.0067)
(0.677501, 52.9701)
(0.679904, 52.4529)
(0.682306, 51.9506)
(0.684709, 52.2015)
(0.687111, 51.134)
(0.689514, 52.3609)
(0.691916, 52.9931)
(0.694319, 53.5505)
(0.696721, 53.9292)
(0.699124, 55.5823)
(0.701526, 53.7648)
(0.703929, 53.3672)
(0.706331, 54.5661)
(0.708734, 53.6829)
(0.711136, 53.1579)
(0.713539, 53.9195)
(0.715941, 53.5475)
(0.718344, 53.4106)
(0.720746, 53.0292)
(0.723149, 53.0835)
(0.725551, 51.563)
(0.727954, 52.4892)
(0.730356, 52.4012)
(0.732759, 51.1453)
(0.735161, 50.569)
(0.737564, 51.1441)
(0.739966, 51.426)
(0.742369, 52.2706)
(0.744771, 53.0943)
(0.747173, 52.0464)
(0.749576, 54.753)
(0.751978, 54.6539)
(0.754381, 52.8061)
(0.756783, 53.5233)
(0.759186, 52.7256)
(0.761588, 52.9817)
(0.763991, 53.4137)
(0.766393, 53.0209)
(0.768796, 53.4145)
(0.771198, 53.7206)
(0.773601, 53.9439)
(0.776003, 54.0871)
(0.778406, 53.6312)
(0.780808, 53.4159)
(0.783211, 52.911)
(0.785613, 53.4137)
(0.788016, 52.9157)
(0.790418, 53.1411)
(0.792821, 52.027)
(0.795223, 52.7136)
(0.797626, 50.2111)
(0.800028, 52.6417)
(0.802431, 51.8418)
(0.804833, 50.4237)
(0.807236, 51.1208)
(0.809638, 52.1229)
(0.812041, 52.4042)
(0.814443, 51.8879)
(0.816846, 52.8071)
(0.819248, 52.1462)
(0.821651, 52.7071)
(0.824053, 52.7338)
(0.826456, 53.281)
(0.828858, 51.9714)
(0.831261, 52.1646)
(0.833663, 52.2521)
(0.836066, 54.1155)
(0.838468, 54.2944)
(0.840871, 54.3928)
(0.843273, 54.1329)
(0.845675, 54.4759)
(0.848078, 53.8136)
(0.85048, 54.5783)
(0.852883, 54.3834)
(0.855285, 53.0142)
(0.857688, 52.5977)
(0.86009, 52.4864)
(0.862493, 52.6224)
(0.864895, 51.4766)
(0.867298, 51.8197)
(0.8697, 52.2827)
(0.872103, 52.1993)
(0.874505, 52.5381)
(0.876908, 52.0597)
(0.87931, 51.9872)
(0.881713, 52.241)
(0.884115, 52.9631)
(0.886518, 52.6876)
(0.88892, 54.5283)
(0.891323, 54.3782)
(0.893725, 52.8215)
(0.896128, 53.1921)
(0.89853, 52.2839)
(0.900933, 52.8544)
(0.903335, 53.2336)
(0.905738, 53.2557)
(0.90814, 53.4611)
(0.910543, 53.5582)
(0.912945, 53.1023)
(0.915348, 53.3357)
(0.91775, 54.1126)
(0.920153, 54.7829)
(0.922555, 54.1364)
(0.924958, 53.745)
(0.92736, 53.9846)
(0.929763, 53.6307)
(0.932165, 53.6616)
(0.934568, 53.5522)
(0.93697, 53.418)
(0.939372, 53.0132)
(0.941775, 53.3917)
(0.944178, 54.1194)
(0.94658, 52.3014)
(0.948982, 52.4401)
(0.951385, 51.9568)
(0.953787, 51.8498)
(0.95619, 51.5853)
(0.958592, 51.8137)
(0.960995, 51.4196)
(0.963397, 51.6495)
(0.9658, 51.6967)
(0.968202, 51.9059)
(0.970605, 51.5685)
(0.973007, 51.7232)
(0.97541, 52.1536)
(0.977812, 52.5397)
(0.980215, 52.1365)
(0.982617, 52.2437)
(0.98502, 53.0395)
(0.987422, 53.0201)
(0.989825, 53.5561)
(0.992227, 52.0756)
(0.99463, 51.5694)
(0.997032, 51.2252)
(0.999435, 51.4666)
(1,0)
};

==> exp_plots/payload_comparison/th_tmdc.tex <==
\addplot[
    fill=white!60!clr3,draw = clr3,opacity=\opacty,
    line width= \linew pt,
    forget plot
    ]
 %%
coordinates {
(0,0)
(0, 49.9052)
(0.00240215, 47.1886)
(0.0048043, 49.5342)
(0.00720644, 50.4022)
(0.00960859, 46.911)
(0.0120107, 44.9446)
(0.0144129, 50.8655)
(0.016815, 54.1427)
(0.0192172, 54.6702)
(0.0216193, 48.8426)
(0.0240215, 50.6598)
(0.0264236, 49.7009)
(0.0288258, 48.1427)
(0.0312279, 48.6926)
(0.0336301, 49.8479)
(0.0360322, 51.7714)
(0.0384344, 50.9043)
(0.0408365, 49.6778)
(0.0432387, 49.7084)
(0.0456408, 51.4177)
(0.048043, 50.4673)
(0.0504451, 50.8468)
(0.0528472, 50.0102)
(0.0552494, 50.4687)
(0.0576515, 50.162)
(0.0600537, 49.3042)
(0.0624558, 51.9184)
(0.064858, 50.3742)
(0.0672601, 48.2087)
(0.0696623, 52.013)
(0.0720644, 50.8563)
(0.0744666, 49.7673)
(0.0768687, 53.1569)
(0.0792709, 50.1827)
(0.081673, 50.1136)
(0.0840752, 49.2603)
(0.0864773, 51.1869)
(0.0888795, 48.6631)
(0.0912816, 49.8069)
(0.0936838, 51.7899)
(0.0960859, 51.4799)
(0.0984881, 50.9363)
(0.10089, 51.9366)
(0.103292, 51.9285)
(0.105694, 51.5557)
(0.108097, 49.1932)
(0.110499, 53.2841)
(0.112901, 56.7868)
(0.115303, 53.931)
(0.117705, 49.2225)
(0.120107, 50.3293)
(0.12251, 51.6992)
(0.124912, 52.4509)
(0.127314, 51.7064)
(0.129716, 51.433)
(0.132118, 53.0676)
(0.13452, 50.6708)
(0.136922, 49.4102)
(0.139325, 50.7201)
(0.141727, 52.619)
(0.144129, 51.5981)
(0.146531, 51.897)
(0.148933, 53.0202)
(0.151335, 52.6689)
(0.153737, 52.8211)
(0.15614, 57.7843)
(0.158542, 56.5379)
(0.160944, 54.3764)
(0.163346, 53.6651)
(0.165748, 52.4707)
(0.16815, 53.6717)
(0.170552, 55.0021)
(0.172955, 52.4022)
(0.175357, 53.9709)
(0.177759, 54.6251)
(0.180161, 52.4077)
(0.182563, 55.1016)
(0.184965, 55.7821)
(0.187368, 49.7302)
(0.18977, 56.1061)
(0.192172, 55.4036)
(0.194574, 53.4486)
(0.196976, 56.5278)
(0.199378, 56.699)
(0.20178, 56.7764)
(0.204183, 56.6102)
(0.206585, 55.5755)
(0.208987, 53.4619)
(0.211389, 51.6307)
(0.213791, 51.9419)
(0.216193, 56.7039)
(0.218595, 51.6107)
(0.220998, 52.9449)
(0.2234, 54.9573)
(0.225802, 56.229)
(0.228204, 54.1834)
(0.230606, 55.637)
(0.233008, 57.2454)
(0.23541, 52.9588)
(0.237813, 54.5191)
(0.240215, 55.8831)
(0.242617, 52.5487)
(0.245019, 52.5935)
(0.247421, 53.9587)
(0.249823, 51.2113)
(0.252225, 50.4182)
(0.254628, 52.188)
(0.25703, 49.6909)
(0.259432, 51.825)
(0.261834, 54.6032)
(0.264236, 52.7169)
(0.266638, 55.3006)
(0.269041, 54.74)
(0.271443, 52.0824)
(0.273845, 53.4097)
(0.276247, 52.7873)
(0.278649, 54.108)
(0.281051, 53.131)
(0.283453, 53.6786)
(0.285856, 56.2472)
(0.288258, 58.6878)
(0.29066, 54.8405)
(0.293062, 56.5156)
(0.295464, 58.1549)
(0.297866, 55.7281)
(0.300268, 53.5108)
(0.302671, 54.0096)
(0.305073, 54.3996)
(0.307475, 52.5783)
(0.309877, 56.9482)
(0.312279, 54.4286)
(0.314681, 52.4437)
(0.317084, 55.2932)
(0.319486, 54.6293)
(0.321888, 55.5012)
(0.32429, 57.2134)
(0.326692, 55.0685)
(0.329094, 56.2418)
(0.331496, 53.5427)
(0.333899, 56.2893)
(0.336301, 53.2706)
(0.338703, 54.3591)
(0.341105, 57.3843)
(0.343507, 55.2857)
(0.345909, 51.9254)
(0.348311, 52.0121)
(0.350714, 52.6931)
(0.353116, 54.76)
(0.355518, 57.6649)
(0.35792, 52.4027)
(0.360322, 51.9168)
(0.362724, 54.1371)
(0.365126, 52.8559)
(0.367529, 50.3337)
(0.369931, 51.9135)
(0.372333, 53.272)
(0.374735, 53.6787)
(0.377137, 53.5062)
(0.379539, 53.1626)
(0.381941, 55.9723)
(0.384344, 54.0866)
(0.386746, 54.0259)
(0.389148, 56.2711)
(0.39155, 54.2317)
(0.393952, 54.8013)
(0.396354, 55.0772)
(0.398757, 53.0086)
(0.401159, 56.1554)
(0.403561, 55.2902)
(0.405963, 50.8604)
(0.408365, 51.8722)
(0.410767, 52.2792)
(0.413169, 52.2876)
(0.415572, 52.6732)
(0.417974, 52.8515)
(0.420376, 51.3052)
(0.422778, 53.5075)
(0.42518, 52.319)
(0.427582, 55.3455)
(0.429984, 55.978)
(0.432387, 54.1951)
(0.434789, 55.7176)
(0.437191, 55.0533)
(0.439593, 50.4866)
(0.441995, 52.811)
(0.444397, 54.7847)
(0.446799, 51.4916)
(0.449202, 55.2131)
(0.451604, 53.0977)
(0.454006, 57.1349)
(0.456408, 58.9234)
(0.45881, 53.5976)
(0.461212, 57.35)
(0.463615, 58.3924)
(0.466017, 57.1316)
(0.468419, 55.2849)
(0.470821, 52.1034)
(0.473223, 57.6365)
(0.475625, 55.0552)
(0.478027, 58.6589)
(0.48043, 58.2041)
(0.482832, 56.0404)
(0.485234, 54.57)
(0.487636, 55.0527)
(0.490038, 58.7567)
(0.49244, 55.9503)
(0.494842, 54.453)
(0.497245, 55.5327)
(0.499647, 58.5272)
(0.502049, 55.5477)
(0.504451, 54.5168)
(0.506853, 57.9421)
(0.509255, 54.6261)
(0.511657, 57.1336)
(0.51406, 58.3497)
(0.516462, 56.0805)
(0.518864, 54.75)
(0.521266, 53.8679)
(0.523668, 56.9214)
(0.52607, 56.0514)
(0.528472, 51.9097)
(0.530875, 53.2527)
(0.533277, 52.881)
(0.535679, 52.7941)
(0.538081, 55.5226)
(0.540483, 54.711)
(0.542885, 54.8635)
(0.545288, 54.4223)
(0.54769, 54.2897)
(0.550092, 54.8695)
(0.552494, 54.9527)
(0.554896, 52.4353)
(0.557298, 50.3269)
(0.5597, 54.5561)
(0.562103, 51.8837)
(0.564505, 54.5153)
(0.566907, 56.0713)
(0.569309, 53.5474)
(0.571711, 52.8781)
(0.574113, 56.8626)
(0.576515, 55.2853)
(0.578918, 55.4482)
(0.58132, 53.115)
(0.583722, 52.9948)
(0.586124, 49.9414)
(0.588526, 52.6606)
(0.590928, 54.7171)
(0.593331, 54.5456)
(0.595733, 57.6415)
(0.598135, 53.9727)
(0.600537, 52.6913)
(0.602939, 53.811)
(0.605341, 53.5177)
(0.607743, 54.2369)
(0.610146, 54.2117)
(0.612548, 54.8644)
(0.61495, 53.3457)
(0.617352, 54.6526)
(0.619754, 54.073)
(0.622156, 53.6522)
(0.624558, 53.9001)
(0.626961, 53.0437)
(0.629363, 54.2884)
(0.631765, 53.5815)
(0.634167, 54.8438)
(0.636569, 57.2515)
(0.638971, 53.4435)
(0.641373, 55.4479)
(0.643776, 54.3602)
(0.646178, 56.38)
(0.64858, 55.5356)
(0.650982, 54.8265)
(0.653384, 56.9196)
(0.655786, 61.1597)
(0.658189, 55.7003)
(0.660591, 54.2596)
(0.662993, 55.9811)
(0.665395, 54.7993)
(0.667797, 57.1495)
(0.670199, 54.7919)
(0.672601, 56.0525)
(0.675004, 57.9241)
(0.677406, 58.1529)
(0.679808, 55.8935)
(0.68221, 56.6292)
(0.684612, 58.4559)
(0.687014, 56.8936)
(0.689416, 55.1404)
(0.691819, 57.8997)
(0.694221, 57.2346)
(0.696623, 56.0863)
(0.699025, 55.2336)
(0.701427, 53.6567)
(0.703829, 51.9912)
(0.706231, 52.9539)
(0.708634, 53.0652)
(0.711036, 53.2484)
(0.713438, 52.8112)
(0.71584, 53.8529)
(0.718242, 53.8937)
(0.720644, 55.5823)
(0.723046, 53.6149)
(0.725449, 53.0031)
(0.727851, 54.2792)
(0.730253, 52.9673)
(0.732655, 55.062)
(0.735057, 53.2383)
(0.737459, 55.2151)
(0.739861, 51.4048)
(0.742264, 49.2404)
(0.744666, 54.1013)
(0.747068, 55.1173)
(0.74947, 51.9537)
(0.751872, 53.567)
(0.754274, 54.305)
(0.756677, 52.8448)
(0.759079, 51.4686)
(0.761481, 53.3564)
(0.763883, 55.2169)
(0.766285, 55.4504)
(0.768687, 54.2341)
(0.771089, 54.0115)
(0.773492, 54.4491)
(0.775894, 54.7969)
(0.778296, 55.5464)
(0.780698, 51.7949)
(0.7831, 55.4067)
(0.785502, 53.6066)
(0.787905, 55.0773)
(0.790307, 56.1029)
(0.792709, 54.4461)
(0.795111, 56.0885)
(0.797513, 54.7568)
(0.799915, 55.1573)
(0.802317, 53.798)
(0.804719, 55.2344)
(0.807122, 54.9522)
(0.809524, 54.3267)
(0.811926, 55.7423)
(0.814328, 54.8755)
(0.81673, 58.0205)
(0.819132, 57.3011)
(0.821535, 56.9876)
(0.823937, 59.2286)
(0.826339, 58.8836)
(0.828741, 58.2791)
(0.831143, 57.6628)
(0.833545, 58.8832)
(0.835947, 55.8703)
(0.83835, 56.4064)
(0.840752, 57.1848)
(0.843154, 57.5196)
(0.845556, 58.3373)
(0.847958, 56.5632)
(0.85036, 57.7965)
(0.852762, 56.8527)
(0.855165, 58.7422)
(0.857567, 60.0941)
(0.859969, 59.5127)
(0.862371, 57.1779)
(0.864773, 55.6674)
(0.867175, 56.6715)
(0.869577, 58.7005)
(0.87198, 57.3372)
(0.874382, 55.458)
(0.876784, 56.1057)
(0.879186, 55.3137)
(0.881588, 55.4812)
(0.88399, 56.6157)
(0.886393, 55.1585)
(0.888795, 55.013)
(0.891197, 58.764)
(0.893599, 55.1063)
(0.896001, 57.6435)
(0.898403, 57.7655)
(0.900805, 53.9649)
(0.903208, 53.5509)
(0.90561, 55.4454)
(0.908012, 55.0821)
(0.910414, 52.9836)
(0.912816, 56.2294)
(0.915218, 55.5179)
(0.91762, 53.097)
(0.920023, 56.4038)
(0.922425, 54.592)
(0.924827, 55.337)
(0.927229, 56.2744)
(0.929631, 55.0436)
(0.932033, 55.9583)
(0.934435, 52.5839)
(0.936838, 52.5276)
(0.93924, 54.6502)
(0.941642, 54.5541)
(0.944044, 53.536)
(0.946446, 54.4725)
(0.948848, 54.2213)
(0.951251, 53.9104)
(0.953653, 54.9621)
(0.956055, 54.3752)
(0.958457, 55.2616)
(0.960859, 54.5771)
(0.963261, 52.6299)
(0.965663, 53.5998)
(0.968066, 56.0166)
(0.970468, 55.0426)
(0.97287, 52.4684)
(0.975272, 51.6205)
(0.977674, 52.9954)
(0.980076, 52.9953)
(0.982478, 54.759)
(0.984881, 54.4547)
(0.987283, 53.6688)
(0.989685, 52.6857)
(0.992087, 54.4275)
(0.994489, 53.624)
(0.996891, 53.3735)
(0.999293, 55.217)
(1,0)
};

==> exp_plots/payload_comparison/th_tmdc_gt.tex <==
\addplot[
    fill=white!60!clr2,draw = clr2,opacity=\opacty,
    line width= \linew pt,
    forget plot
    ]
 %%
coordinates {
(0,0)
(0, 51.4543)
(0.00240657, 49.7298)
(0.00481314, 51.9851)
(0.00721971, 51.1396)
(0.00962627, 52.5784)
(0.0120328, 51.3777)
(0.0144394, 51.7488)
(0.016846, 56.2084)
(0.0192525, 51.5272)
(0.0216591, 52.8702)
(0.0240657, 53.6455)
(0.0264723, 51.8087)
(0.0288788, 51.873)
(0.0312854, 55.556)
(0.033692, 52.7396)
(0.0360985, 52.6292)
(0.0385051, 54.2659)
(0.0409117, 51.7279)
(0.0433182, 54.1971)
(0.0457248, 53.5545)
(0.0481314, 51.8562)
(0.0505379, 53.6245)
(0.0529445, 54.055)
(0.0553511, 53.2664)
(0.0577576, 53.6201)
(0.0601642, 52.9496)
(0.0625708, 53.4837)
(0.0649773, 54.0793)
(0.0673839, 52.8859)
(0.0697905, 53.693)
(0.0721971, 51.6559)
(0.0746036, 55.8098)
(0.0770102, 54.941)
(0.0794168, 52.9171)
(0.0818233, 51.3613)
(0.0842299, 52.4284)
(0.0866365, 53.773)
(0.089043, 51.0737)
(0.0914496, 51.21)
(0.0938562, 52.8743)
(0.0962627, 55.2325)
(0.0986693, 53.2981)
(0.101076, 53.137)
(0.103482, 52.9772)
(0.105889, 51.9131)
(0.108296, 56.8611)
(0.110702, 53.0069)
(0.113109, 51.6613)
(0.115515, 52.9591)
(0.117922, 53.6525)
(0.120328, 53.0186)
(0.122735, 54.4014)
(0.125142, 53.415)
(0.127548, 51.3196)
(0.129955, 50.1754)
(0.132361, 54.4318)
(0.134768, 54.7365)
(0.137174, 51.059)
(0.139581, 55.2463)
(0.141988, 53.1343)
(0.144394, 52.4863)
(0.146801, 53.686)
(0.149207, 55.1485)
(0.151614, 57.6116)
(0.15402, 55.3243)
(0.156427, 55.372)
(0.158834, 56.1047)
(0.16124, 54.9048)
(0.163647, 53.5319)
(0.166053, 56.6921)
(0.16846, 56.2645)
(0.170866, 57.4693)
(0.173273, 56.0032)
(0.17568, 54.8289)
(0.178086, 59.5142)
(0.180493, 57.646)
(0.182899, 55.7386)
(0.185306, 57.3341)
(0.187712, 58.5306)
(0.190119, 56.3836)
(0.192525, 56.4453)
(0.194932, 57.0169)
(0.197339, 53.987)
(0.199745, 58.0954)
(0.202152, 56.4321)
(0.204558, 57.6857)
(0.206965, 57.5596)
(0.209371, 53.9257)
(0.211778, 56.2045)
(0.214185, 56.9466)
(0.216591, 54.1399)
(0.218998, 56.4965)
(0.221404, 55.5691)
(0.223811, 56.4649)
(0.226217, 57.4815)
(0.228624, 52.9449)
(0.231031, 53.1187)
(0.233437, 56.4575)
(0.235844, 53.5156)
(0.23825, 57.7932)
(0.240657, 53.8886)
(0.243063, 52.3837)
(0.24547, 57.1387)
(0.247877, 55.3017)
(0.250283, 54.3067)
(0.25269, 55.325)
(0.255096, 54.9308)
(0.257503, 56.3251)
(0.259909, 57.7393)
(0.262316, 58.2118)
(0.264723, 58.9147)
(0.267129, 58.4764)
(0.269536, 57.8773)
(0.271942, 57.6777)
(0.274349, 55.2726)
(0.276755, 56.4635)
(0.279162, 56.933)
(0.281568, 56.7674)
(0.283975, 55.3443)
(0.286382, 56.4862)
(0.288788, 56.0951)
(0.291195, 56.0049)
(0.293601, 55.694)
(0.296008, 56.725)
(0.298414, 58.381)
(0.300821, 57.1193)
(0.303228, 58.773)
(0.305634, 58.8454)
(0.308041, 56.4962)
(0.310447, 56.6182)
(0.312854, 58.0924)
(0.31526, 57.2105)
(0.317667, 57.4098)
(0.320074, 58.0528)
(0.32248, 57.9005)
(0.324887, 57.0899)
(0.327293, 59.8201)
(0.3297, 59.7017)
(0.332106, 58.1506)
(0.334513, 55.741)
(0.33692, 56.5086)
(0.339326, 55.7624)
(0.341733, 57.3266)
(0.344139, 57.9514)
(0.346546, 57.5673)
(0.348952, 55.2243)
(0.351359, 55.0169)
(0.353766, 55.6107)
(0.356172, 55.7054)
(0.358579, 54.1651)
(0.360985, 55.6563)
(0.363392, 57.8999)
(0.365798, 54.6227)
(0.368205, 58.1191)
(0.370612, 58.206)
(0.373018, 53.2514)
(0.375425, 53.6239)
(0.377831, 54.3088)
(0.380238, 54.8669)
(0.382644, 53.4528)
(0.385051, 53.2618)
(0.387458, 59.1493)
(0.389864, 49.6106)
(0.392271, 53.1399)
(0.394677, 61.8743)
(0.397084, 56.434)
(0.39949, 59.8679)
(0.401897, 61.6205)
(0.404304, 54.8842)
(0.40671, 56.3156)
(0.409117, 59.1501)
(0.411523, 57.7281)
(0.41393, 58.0768)
(0.416336, 56.2958)
(0.418743, 55.7489)
(0.421149, 59.7929)
(0.423556, 58.2325)
(0.425963, 56.4963)
(0.428369, 59.2568)
(0.430776, 60.3627)
(0.433182, 56.9226)
(0.435589, 59.3516)
(0.437995, 57.5475)
(0.440402, 57.1255)
(0.442809, 57.9152)
(0.445215, 64.3253)
(0.447622, 58.3507)
(0.450028, 57.2067)
(0.452435, 56.4207)
(0.454841, 58.8551)
(0.457248, 56.9329)
(0.459655, 57.9117)
(0.462061, 58.4542)
(0.464468, 57.0296)
(0.466874, 59.6924)
(0.469281, 58.7876)
(0.471687, 59.157)
(0.474094, 58.2423)
(0.476501, 55.8263)
(0.478907, 56.1091)
(0.481314, 56.1651)
(0.48372, 58.9018)
(0.486127, 54.5929)
(0.488533, 56.2312)
(0.49094, 57.1226)
(0.493347, 53.0353)
(0.495753, 59.3818)
(0.49816, 57.8415)
(0.500566, 57.2723)
(0.502973, 55.6017)
(0.505379, 54.7323)
(0.507786, 56.8569)
(0.510193, 53.8376)
(0.512599, 54.8672)
(0.515006, 56.0566)
(0.517412, 54.5883)
(0.519819, 55.9032)
(0.522225, 58.9335)
(0.524632, 60.4143)
(0.527039, 59.5418)
(0.529445, 59.7358)
(0.531852, 57.1174)
(0.534258, 58.5055)
(0.536665, 58.6059)
(0.539071, 56.4335)
(0.541478, 59.548)
(0.543884, 56.2502)
(0.546291, 55.5579)
(0.548698, 57.7964)
(0.551104, 58.5832)
(0.553511, 56.4145)
(0.555917, 55.6263)
(0.558324, 56.3563)
(0.56073, 58.6497)
(0.563137, 58.297)
(0.565544, 56.5756)
(0.56795, 57.3174)
(0.570357, 58.0932)
(0.572763, 55.8944)
(0.57517, 56.7717)
(0.577576, 58.0188)
(0.579983, 58.1144)
(0.58239, 56.4083)
(0.584796, 55.7961)
(0.587203, 57.7081)
(0.589609, 59.1695)
(0.592016, 55.4627)
(0.594422, 55.3594)
(0.596829, 55.6715)
(0.599236, 55.204)
(0.601642, 54.2981)
(0.604049, 54.227)
(0.606455, 53.2289)
(0.608862, 56.7552)
(0.611268, 53.9719)
(0.613675, 57.8768)
(0.616082, 56.5056)
(0.618488, 55.14)
(0.620895, 57.0365)
(0.623301, 56.6168)
(0.625708, 53.1137)
(0.628114, 53.5943)
(0.630521, 54.8563)
(0.632927, 52.0649)
(0.635334, 53.7631)
(0.637741, 53.5791)
(0.640147, 57.3522)
(0.642554, 53.4845)
(0.64496, 54.7195)
(0.647367, 57.2694)
(0.649774, 53.7562)
(0.65218, 53.5455)
(0.654587, 57.9813)
(0.656993, 56.9423)
(0.6594, 55.0945)
(0.661806, 57.3025)
(0.664213, 59.0057)
(0.666619, 56.1716)
(0.669026, 58.0014)
(0.671433, 58.7352)
(0.673839, 60.8217)
(0.676246, 58.02)
(0.678652, 57.6089)
(0.681059, 58.6463)
(0.683465, 57.5765)
(0.685872, 56.4343)
(0.688279, 57.6291)
(0.690685, 59.3744)
(0.693092, 55.592)
(0.695498, 57.0829)
(0.697905, 59.6902)
(0.700311, 58.7641)
(0.702718, 60.2477)
(0.705125, 59.4184)
(0.707531, 63.3267)
(0.709938, 62.4834)
(0.712344, 59.2931)
(0.714751, 62.8214)
(0.717157, 64.9174)
(0.719564, 59.0972)
(0.72197, 62.0726)
(0.724377, 61.4332)
(0.726784, 60.05)
(0.72919, 60.01)
(0.731597, 62.2036)
(0.734003, 62.863)
(0.73641, 61.4659)
(0.738817, 61.4102)
(0.741223, 56.696)
(0.74363, 59.9883)
(0.746036, 58.506)
(0.748443, 59.4186)
(0.750849, 59.7325)
(0.753256, 60.8009)
(0.755662, 63.636)
(0.758069, 59.1678)
(0.760476, 54.8234)
(0.762882, 55.7527)
(0.765289, 57.2349)
(0.767695, 60.6603)
(0.770102, 59.4997)
(0.772509, 56.1546)
(0.774915, 57.2481)
(0.777322, 58.9547)
(0.779728, 56.6949)
(0.782135, 58.6117)
(0.784541, 56.8731)
(0.786948, 59.7976)
(0.789355, 56.077)
(0.791761, 58.1935)
(0.794168, 57.5235)
(0.796574, 55.6588)
(0.798981, 57.0241)
(0.801387, 56.2967)
(0.803794, 54.7551)
(0.8062, 58.6103)
(0.808607, 60.3398)
(0.811014, 54.2471)
(0.81342, 55.2191)
(0.815827, 56.862)
(0.818233, 54.9722)
(0.82064, 57.2097)
(0.823046, 55.5252)
(0.825453, 61.3756)
(0.82786, 59.7809)
(0.830266, 59.7506)
(0.832673, 57.3455)
(0.835079, 59.3334)
(0.837486, 58.1791)
(0.839892, 55.8906)
(0.842299, 57.8149)
(0.844706, 58.5077)
(0.847112, 56.2388)
(0.849519, 57.9352)
(0.851925, 58.158)
(0.854332, 57.0136)
(0.856738, 57.3932)
(0.859145, 56.7495)
(0.861552, 56.4813)
(0.863958, 58.1085)
(0.866365, 58.289)
(0.868771, 58.5548)
(0.871178, 57.4188)
(0.873584, 57.3693)
(0.875991, 55.7068)
(0.878397, 55.4085)
(0.880804, 51.7287)
(0.883211, 54.1151)
(0.885617, 59.0882)
(0.888024, 58.5877)
(0.89043, 55.9288)
(0.892837, 55.2138)
(0.895243, 56.6851)
(0.89765, 54.8302)
(0.900057, 55.8342)
(0.902463, 58.0051)
(0.90487, 54.8052)
(0.907276, 55.4515)
(0.909683, 56.1904)
(0.912089, 54.2948)
(0.914496, 55.373)
(0.916903, 56.2313)
(0.919309, 56.3927)
(0.921716, 56.9567)
(0.924122, 55.1823)
(0.926529, 58.5016)
(0.928935, 57.6081)
(0.931342, 55.0793)
(0.933749, 56.5227)
(0.936155, 57.5486)
(0.938562, 55.8832)
(0.940968, 54.3885)
(0.943375, 53.621)
(0.945781, 55.6494)
(0.948188, 56.3204)
(0.950595, 53.4905)
(0.953001, 54.5125)
(0.955408, 56.6864)
(0.957814, 55.5488)
(0.960221, 54.984)
(0.962627, 56.9935)
(0.965034, 56.7467)
(0.967441, 54.8903)
(0.969847, 55.4889)
(0.972254, 53.9584)
(0.97466, 55.5164)
(0.977067, 57.6698)
(0.979473, 54.4381)
(0.98188, 55.5123)
(0.984286, 57.6989)
(0.986693, 57.7266)
(0.9891, 51.9255)
(0.991506, 57.2269)
(0.993913, 57.8323)
(0.996319, 56.1001)
(0.998726, 56.761)
(1,0)
};

==> exp_plots/payload_comparison/th_tmdc_gt_no_fill.tex <==
\addplot[
    fill=none,draw = clr2,opacity=1.0,
    line width= \linew pt
    ]
 %%
coordinates {
(0, 0)
(0, 51.4543)
(0.00240657, 49.7298)
(0.00481314, 51.9851)
(0.00721971, 51.1396)
(0.00962627, 52.5784)
(0.0120328, 51.3777)
(0.0144394, 51.7488)
(0.016846, 56.2084)
(0.0192525, 51.5272)
(0.0216591, 52.8702)
(0.0240657, 53.6455)
(0.0264723, 51.8087)
(0.0288788, 51.873)
(0.0312854, 55.556)
(0.033692, 52.7396)
(0.0360985, 52.6292)
(0.0385051, 54.2659)
(0.0409117, 51.7279)
(0.0433182, 54.1971)
(0.0457248, 53.5545)
(0.0481314, 51.8562)
(0.0505379, 53.6245)
(0.0529445, 54.055)
(0.0553511, 53.2664)
(0.0577576, 53.6201)
(0.0601642, 52.9496)
(0.0625708, 53.4837)
(0.0649773, 54.0793)
(0.0673839, 52.8859)
(0.0697905, 53.693)
(0.0721971, 51.6559)
(0.0746036, 55.8098)
(0.0770102, 54.941)
(0.0794168, 52.9171)
(0.0818233, 51.3613)
(0.0842299, 52.4284)
(0.0866365, 53.773)
(0.089043, 51.0737)
(0.0914496, 51.21)
(0.0938562, 52.8743)
(0.0962627, 55.2325)
(0.0986693, 53.2981)
(0.101076, 53.137)
(0.103482, 52.9772)
(0.105889, 51.9131)
(0.108296, 56.8611)
(0.110702, 53.0069)
(0.113109, 51.6613)
(0.115515, 52.9591)
(0.117922, 53.6525)
(0.120328, 53.0186)
(0.122735, 54.4014)
(0.125142, 53.415)
(0.127548, 51.3196)
(0.129955, 50.1754)
(0.132361, 54.4318)
(0.134768, 54.7365)
(0.137174, 51.059)
(0.139581, 55.2463)
(0.141988, 53.1343)
(0.144394, 52.4863)
(0.146801, 53.686)
(0.149207, 55.1485)
(0.151614, 57.6116)
(0.15402, 55.3243)
(0.156427, 55.372)
(0.158834, 56.1047)
(0.16124, 54.9048)
(0.163647, 53.5319)
(0.166053, 56.6921)
(0.16846, 56.2645)
(0.170866, 57.4693)
(0.173273, 56.0032)
(0.17568, 54.8289)
(0.178086, 59.5142)
(0.180493, 57.646)
(0.182899, 55.7386)
(0.185306, 57.3341)
(0.187712, 58.5306)
(0.190119, 56.3836)
(0.192525, 56.4453)
(0.194932, 57.0169)
(0.197339, 53.987)
(0.199745, 58.0954)
(0.202152, 56.4321)
(0.204558, 57.6857)
(0.206965, 57.5596)
(0.209371, 53.9257)
(0.211778, 56.2045)
(0.214185, 56.9466)
(0.216591, 54.1399)
(0.218998, 56.4965)
(0.221404, 55.5691)
(0.223811, 56.4649)
(0.226217, 57.4815)
(0.228624, 52.9449)
(0.231031, 53.1187)
(0.233437, 56.4575)
(0.235844, 53.5156)
(0.23825, 57.7932)
(0.240657, 53.8886)
(0.243063, 52.3837)
(0.24547, 57.1387)
(0.247877, 55.3017)
(0.250283, 54.3067)
(0.25269, 55.325)
(0.255096, 54.9308)
(0.257503, 56.3251)
(0.259909, 57.7393)
(0.262316, 58.2118)
(0.264723, 58.9147)
(0.267129, 58.4764)
(0.269536, 57.8773)
(0.271942, 57.6777)
(0.274349, 55.2726)
(0.276755, 56.4635)
(0.279162, 56.933)
(0.281568, 56.7674)
(0.283975, 55.3443)
(0.286382, 56.4862)
(0.288788, 56.0951)
(0.291195, 56.0049)
(0.293601, 55.694)
(0.296008, 56.725)
(0.298414, 58.381)
(0.300821, 57.1193)
(0.303228, 58.773)
(0.305634, 58.8454)
(0.308041, 56.4962)
(0.310447, 56.6182)
(0.312854, 58.0924)
(0.31526, 57.2105)
(0.317667, 57.4098)
(0.320074, 58.0528)
(0.32248, 57.9005)
(0.324887, 57.0899)
(0.327293, 59.8201)
(0.3297, 59.7017)
(0.332106, 58.1506)
(0.334513, 55.741)
(0.33692, 56.5086)
(0.339326, 55.7624)
(0.341733, 57.3266)
(0.344139, 57.9514)
(0.346546, 57.5673)
(0.348952, 55.2243)
(0.351359, 55.0169)
(0.353766, 55.6107)
(0.356172, 55.7054)
(0.358579, 54.1651)
(0.360985, 55.6563)
(0.363392, 57.8999)
(0.365798, 54.6227)
(0.368205, 58.1191)
(0.370612, 58.206)
(0.373018, 53.2514)
(0.375425, 53.6239)
(0.377831, 54.3088)
(0.380238, 54.8669)
(0.382644, 53.4528)
(0.385051, 53.2618)
(0.387458, 59.1493)
(0.389864, 49.6106)
(0.392271, 53.1399)
(0.394677, 61.8743)
(0.397084, 56.434)
(0.39949, 59.8679)
(0.401897, 61.6205)
(0.404304, 54.8842)
(0.40671, 56.3156)
(0.409117, 59.1501)
(0.411523, 57.7281)
(0.41393, 58.0768)
(0.416336, 56.2958)
(0.418743, 55.7489)
(0.421149, 59.7929)
(0.423556, 58.2325)
(0.425963, 56.4963)
(0.428369, 59.2568)
(0.430776, 60.3627)
(0.433182, 56.9226)
(0.435589, 59.3516)
(0.437995, 57.5475)
(0.440402, 57.1255)
(0.442809, 57.9152)
(0.445215, 64.3253)
(0.447622, 58.3507)
(0.450028, 57.2067)
(0.452435, 56.4207)
(0.454841, 58.8551)
(0.457248, 56.9329)
(0.459655, 57.9117)
(0.462061, 58.4542)
(0.464468, 57.0296)
(0.466874, 59.6924)
(0.469281, 58.7876)
(0.471687, 59.157)
(0.474094, 58.2423)
(0.476501, 55.8263)
(0.478907, 56.1091)
(0.481314, 56.1651)
(0.48372, 58.9018)
(0.486127, 54.5929)
(0.488533, 56.2312)
(0.49094, 57.1226)
(0.493347, 53.0353)
(0.495753, 59.3818)
(0.49816, 57.8415)
(0.500566, 57.2723)
(0.502973, 55.6017)
(0.505379, 54.7323)
(0.507786, 56.8569)
(0.510193, 53.8376)
(0.512599, 54.8672)
(0.515006, 56.0566)
(0.517412, 54.5883)
(0.519819, 55.9032)
(0.522225, 58.9335)
(0.524632, 60.4143)
(0.527039, 59.5418)
(0.529445, 59.7358)
(0.531852, 57.1174)
(0.534258, 58.5055)
(0.536665, 58.6059)
(0.539071, 56.4335)
(0.541478, 59.548)
(0.543884, 56.2502)
(0.546291, 55.5579)
(0.548698, 57.7964)
(0.551104, 58.5832)
(0.553511, 56.4145)
(0.555917, 55.6263)
(0.558324, 56.3563)
(0.56073, 58.6497)
(0.563137, 58.297)
(0.565544, 56.5756)
(0.56795, 57.3174)
(0.570357, 58.0932)
(0.572763, 55.8944)
(0.57517, 56.7717)
(0.577576, 58.0188)
(0.579983, 58.1144)
(0.58239, 56.4083)
(0.584796, 55.7961)
(0.587203, 57.7081)
(0.589609, 59.1695)
(0.592016, 55.4627)
(0.594422, 55.3594)
(0.596829, 55.6715)
(0.599236, 55.204)
(0.601642, 54.2981)
(0.604049, 54.227)
(0.606455, 53.2289)
(0.608862, 56.7552)
(0.611268, 53.9719)
(0.613675, 57.8768)
(0.616082, 56.5056)
(0.618488, 55.14)
(0.620895, 57.0365)
(0.623301, 56.6168)
(0.625708, 53.1137)
(0.628114, 53.5943)
(0.630521, 54.8563)
(0.632927, 52.0649)
(0.635334, 53.7631)
(0.637741, 53.5791)
(0.640147, 57.3522)
(0.642554, 53.4845)
(0.64496, 54.7195)
(0.647367, 57.2694)
(0.649774, 53.7562)
(0.65218, 53.5455)
(0.654587, 57.9813)
(0.656993, 56.9423)
(0.6594, 55.0945)
(0.661806, 57.3025)
(0.664213, 59.0057)
(0.666619, 56.1716)
(0.669026, 58.0014)
(0.671433, 58.7352)
(0.673839, 60.8217)
(0.676246, 58.02)
(0.678652, 57.6089)
(0.681059, 58.6463)
(0.683465, 57.5765)
(0.685872, 56.4343)
(0.688279, 57.6291)
(0.690685, 59.3744)
(0.693092, 55.592)
(0.695498, 57.0829)
(0.697905, 59.6902)
(0.700311, 58.7641)
(0.702718, 60.2477)
(0.705125, 59.4184)
(0.707531, 63.3267)
(0.709938, 62.4834)
(0.712344, 59.2931)
(0.714751, 62.8214)
(0.717157, 64.9174)
(0.719564, 59.0972)
(0.72197, 62.0726)
(0.724377, 61.4332)
(0.726784, 60.05)
(0.72919, 60.01)
(0.731597, 62.2036)
(0.734003, 62.863)
(0.73641, 61.4659)
(0.738817, 61.4102)
(0.741223, 56.696)
(0.74363, 59.9883)
(0.746036, 58.506)
(0.748443, 59.4186)
(0.750849, 59.7325)
(0.753256, 60.8009)
(0.755662, 63.636)
(0.758069, 59.1678)
(0.760476, 54.8234)
(0.762882, 55.7527)
(0.765289, 57.2349)
(0.767695, 60.6603)
(0.770102, 59.4997)
(0.772509, 56.1546)
(0.774915, 57.2481)
(0.777322, 58.9547)
(0.779728, 56.6949)
(0.782135, 58.6117)
(0.784541, 56.8731)
(0.786948, 59.7976)
(0.789355, 56.077)
(0.791761, 58.1935)
(0.794168, 57.5235)
(0.796574, 55.6588)
(0.798981, 57.0241)
(0.801387, 56.2967)
(0.803794, 54.7551)
(0.8062, 58.6103)
(0.808607, 60.3398)
(0.811014, 54.2471)
(0.81342, 55.2191)
(0.815827, 56.862)
(0.818233, 54.9722)
(0.82064, 57.2097)
(0.823046, 55.5252)
(0.825453, 61.3756)
(0.82786, 59.7809)
(0.830266, 59.7506)
(0.832673, 57.3455)
(0.835079, 59.3334)
(0.837486, 58.1791)
(0.839892, 55.8906)
(0.842299, 57.8149)
(0.844706, 58.5077)
(0.847112, 56.2388)
(0.849519, 57.9352)
(0.851925, 58.158)
(0.854332, 57.0136)
(0.856738, 57.3932)
(0.859145, 56.7495)
(0.861552, 56.4813)
(0.863958, 58.1085)
(0.866365, 58.289)
(0.868771, 58.5548)
(0.871178, 57.4188)
(0.873584, 57.3693)
(0.875991, 55.7068)
(0.878397, 55.4085)
(0.880804, 51.7287)
(0.883211, 54.1151)
(0.885617, 59.0882)
(0.888024, 58.5877)
(0.89043, 55.9288)
(0.892837, 55.2138)
(0.895243, 56.6851)
(0.89765, 54.8302)
(0.900057, 55.8342)
(0.902463, 58.0051)
(0.90487, 54.8052)
(0.907276, 55.4515)
(0.909683, 56.1904)
(0.912089, 54.2948)
(0.914496, 55.373)
(0.916903, 56.2313)
(0.919309, 56.3927)
(0.921716, 56.9567)
(0.924122, 55.1823)
(0.926529, 58.5016)
(0.928935, 57.6081)
(0.931342, 55.0793)
(0.933749, 56.5227)
(0.936155, 57.5486)
(0.938562, 55.8832)
(0.940968, 54.3885)
(0.943375, 53.621)
(0.945781, 55.6494)
(0.948188, 56.3204)
(0.950595, 53.4905)
(0.953001, 54.5125)
(0.955408, 56.6864)
(0.957814, 55.5488)
(0.960221, 54.984)
(0.962627, 56.9935)
(0.965034, 56.7467)
(0.967441, 54.8903)
(0.969847, 55.4889)
(0.972254, 53.9584)
(0.97466, 55.5164)
(0.977067, 57.6698)
(0.979473, 54.4381)
(0.98188, 55.5123)
(0.984286, 57.6989)
(0.986693, 57.7266)
(0.9891, 51.9255)
(0.991506, 57.2269)
(0.993913, 57.8323)
(0.996319, 56.1001)
(0.998726, 56.761)
(1,0)
};

==> exp_plots/payload_comparison/th_tmdc_no_fill.tex <==
\addplot[
    fill=none,draw = clr3,opacity=1.0,
    line width= \linew pt
    ]
 %%
coordinates {
(0, 0)
(0, 49.9052)
(0.00240215, 47.1886)
(0.0048043, 49.5342)
(0.00720644, 50.4022)
(0.00960859, 46.911)
(0.0120107, 44.9446)
(0.0144129, 50.8655)
(0.016815, 54.1427)
(0.0192172, 54.6702)
(0.0216193, 48.8426)
(0.0240215, 50.6598)
(0.0264236, 49.7009)
(0.0288258, 48.1427)
(0.0312279, 48.6926)
(0.0336301, 49.8479)
(0.0360322, 51.7714)
(0.0384344, 50.9043)
(0.0408365, 49.6778)
(0.0432387, 49.7084)
(0.0456408, 51.4177)
(0.048043, 50.4673)
(0.0504451, 50.8468)
(0.0528472, 50.0102)
(0.0552494, 50.4687)
(0.0576515, 50.162)
(0.0600537, 49.3042)
(0.0624558, 51.9184)
(0.064858, 50.3742)
(0.0672601, 48.2087)
(0.0696623, 52.013)
(0.0720644, 50.8563)
(0.0744666, 49.7673)
(0.0768687, 53.1569)
(0.0792709, 50.1827)
(0.081673, 50.1136)
(0.0840752, 49.2603)
(0.0864773, 51.1869)
(0.0888795, 48.6631)
(0.0912816, 49.8069)
(0.0936838, 51.7899)
(0.0960859, 51.4799)
(0.0984881, 50.9363)
(0.10089, 51.9366)
(0.103292, 51.9285)
(0.105694, 51.5557)
(0.108097, 49.1932)
(0.110499, 53.2841)
(0.112901, 56.7868)
(0.115303, 53.931)
(0.117705, 49.2225)
(0.120107, 50.3293)
(0.12251, 51.6992)
(0.124912, 52.4509)
(0.127314, 51.7064)
(0.129716, 51.433)
(0.132118, 53.0676)
(0.13452, 50.6708)
(0.136922, 49.4102)
(0.139325, 50.7201)
(0.141727, 52.619)
(0.144129, 51.5981)
(0.146531, 51.897)
(0.148933, 53.0202)
(0.151335, 52.6689)
(0.153737, 52.8211)
(0.15614, 57.7843)
(0.158542, 56.5379)
(0.160944, 54.3764)
(0.163346, 53.6651)
(0.165748, 52.4707)
(0.16815, 53.6717)
(0.170552, 55.0021)
(0.172955, 52.4022)
(0.175357, 53.9709)
(0.177759, 54.6251)
(0.180161, 52.4077)
(0.182563, 55.1016)
(0.184965, 55.7821)
(0.187368, 49.7302)
(0.18977, 56.1061)
(0.192172, 55.4036)
(0.194574, 53.4486)
(0.196976, 56.5278)
(0.199378, 56.699)
(0.20178, 56.7764)
(0.204183, 56.6102)
(0.206585, 55.5755)
(0.208987, 53.4619)
(0.211389, 51.6307)
(0.213791, 51.9419)
(0.216193, 56.7039)
(0.218595, 51.6107)
(0.220998, 52.9449)
(0.2234, 54.9573)
(0.225802, 56.229)
(0.228204, 54.1834)
(0.230606, 55.637)
(0.233008, 57.2454)
(0.23541, 52.9588)
(0.237813, 54.5191)
(0.240215, 55.8831)
(0.242617, 52.5487)
(0.245019, 52.5935)
(0.247421, 53.9587)
(0.249823, 51.2113)
(0.252225, 50.4182)
(0.254628, 52.188)
(0.25703, 49.6909)
(0.259432, 51.825)
(0.261834, 54.6032)
(0.264236, 52.7169)
(0.266638, 55.3006)
(0.269041, 54.74)
(0.271443, 52.0824)
(0.273845, 53.4097)
(0.276247, 52.7873)
(0.278649, 54.108)
(0.281051, 53.131)
(0.283453, 53.6786)
(0.285856, 56.2472)
(0.288258, 58.6878)
(0.29066, 54.8405)
(0.293062, 56.5156)
(0.295464, 58.1549)
(0.297866, 55.7281)
(0.300268, 53.5108)
(0.302671, 54.0096)
(0.305073, 54.3996)
(0.307475, 52.5783)
(0.309877, 56.9482)
(0.312279, 54.4286)
(0.314681, 52.4437)
(0.317084, 55.2932)
(0.319486, 54.6293)
(0.321888, 55.5012)
(0.32429, 57.2134)
(0.326692, 55.0685)
(0.329094, 56.2418)
(0.331496, 53.5427)
(0.333899, 56.2893)
(0.336301, 53.2706)
(0.338703, 54.3591)
(0.341105, 57.3843)
(0.343507, 55.2857)
(0.345909, 51.9254)
(0.348311, 52.0121)
(0.350714, 52.6931)
(0.353116, 54.76)
(0.355518, 57.6649)
(0.35792, 52.4027)
(0.360322, 51.9168)
(0.362724, 54.1371)
(0.365126, 52.8559)
(0.367529, 50.3337)
(0.369931, 51.9135)
(0.372333, 53.272)
(0.374735, 53.6787)
(0.377137, 53.5062)
(0.379539, 53.1626)
(0.381941, 55.9723)
(0.384344, 54.0866)
(0.386746, 54.0259)
(0.389148, 56.2711)
(0.39155, 54.2317)
(0.393952, 54.8013)
(0.396354, 55.0772)
(0.398757, 53.0086)
(0.401159, 56.1554)
(0.403561, 55.2902)
(0.405963, 50.8604)
(0.408365, 51.8722)
(0.410767, 52.2792)
(0.413169, 52.2876)
(0.415572, 52.6732)
(0.417974, 52.8515)
(0.420376, 51.3052)
(0.422778, 53.5075)
(0.42518, 52.319)
(0.427582, 55.3455)
(0.429984, 55.978)
(0.432387, 54.1951)
(0.434789, 55.7176)
(0.437191, 55.0533)
(0.439593, 50.4866)
(0.441995, 52.811)
(0.444397, 54.7847)
(0.446799, 51.4916)
(0.449202, 55.2131)
(0.451604, 53.0977)
(0.454006, 57.1349)
(0.456408, 58.9234)
(0.45881, 53.5976)
(0.461212, 57.35)
(0.463615, 58.3924)
(0.466017, 57.1316)
(0.468419, 55.2849)
(0.470821, 52.1034)
(0.473223, 57.6365)
(0.475625, 55.0552)
(0.478027, 58.6589)
(0.48043, 58.2041)
(0.482832, 56.0404)
(0.485234, 54.57)
(0.487636, 55.0527)
(0.490038, 58.7567)
(0.49244, 55.9503)
(0.494842, 54.453)
(0.497245, 55.5327)
(0.499647, 58.5272)
(0.502049, 55.5477)
(0.504451, 54.5168)
(0.506853, 57.9421)
(0.509255, 54.6261)
(0.511657, 57.1336)
(0.51406, 58.3497)
(0.516462, 56.0805)
(0.518864, 54.75)
(0.521266, 53.8679)
(0.523668, 56.9214)
(0.52607, 56.0514)
(0.528472, 51.9097)
(0.530875, 53.2527)
(0.533277, 52.881)
(0.535679, 52.7941)
(0.538081, 55.5226)
(0.540483, 54.711)
(0.542885, 54.8635)
(0.545288, 54.4223)
(0.54769, 54.2897)
(0.550092, 54.8695)
(0.552494, 54.9527)
(0.554896, 52.4353)
(0.557298, 50.3269)
(0.5597, 54.5561)
(0.562103, 51.8837)
(0.564505, 54.5153)
(0.566907, 56.0713)
(0.569309, 53.5474)
(0.571711, 52.8781)
(0.574113, 56.8626)
(0.576515, 55.2853)
(0.578918, 55.4482)
(0.58132, 53.115)
(0.583722, 52.9948)
(0.586124, 49.9414)
(0.588526, 52.6606)
(0.590928, 54.7171)
(0.593331, 54.5456)
(0.595733, 57.6415)
(0.598135, 53.9727)
(0.600537, 52.6913)
(0.602939, 53.811)
(0.605341, 53.5177)
(0.607743, 54.2369)
(0.610146, 54.2117)
(0.612548, 54.8644)
(0.61495, 53.3457)
(0.617352, 54.6526)
(0.619754, 54.073)
(0.622156, 53.6522)
(0.624558, 53.9001)
(0.626961, 53.0437)
(0.629363, 54.2884)
(0.631765, 53.5815)
(0.634167, 54.8438)
(0.636569, 57.2515)
(0.638971, 53.4435)
(0.641373, 55.4479)
(0.643776, 54.3602)
(0.646178, 56.38)
(0.64858, 55.5356)
(0.650982, 54.8265)
(0.653384, 56.9196)
(0.655786, 61.1597)
(0.658189, 55.7003)
(0.660591, 54.2596)
(0.662993, 55.9811)
(0.665395, 54.7993)
(0.667797, 57.1495)
(0.670199, 54.7919)
(0.672601, 56.0525)
(0.675004, 57.9241)
(0.677406, 58.1529)
(0.679808, 55.8935)
(0.68221, 56.6292)
(0.684612, 58.4559)
(0.687014, 56.8936)
(0.689416, 55.1404)
(0.691819, 57.8997)
(0.694221, 57.2346)
(0.696623, 56.0863)
(0.699025, 55.2336)
(0.701427, 53.6567)
(0.703829, 51.9912)
(0.706231, 52.9539)
(0.708634, 53.0652)
(0.711036, 53.2484)
(0.713438, 52.8112)
(0.71584, 53.8529)
(0.718242, 53.8937)
(0.720644, 55.5823)
(0.723046, 53.6149)
(0.725449, 53.0031)
(0.727851, 54.2792)
(0.730253, 52.9673)
(0.732655, 55.062)
(0.735057, 53.2383)
(0.737459, 55.2151)
(0.739861, 51.4048)
(0.742264, 49.2404)
(0.744666, 54.1013)
(0.747068, 55.1173)
(0.74947, 51.9537)
(0.751872, 53.567)
(0.754274, 54.305)
(0.756677, 52.8448)
(0.759079, 51.4686)
(0.761481, 53.3564)
(0.763883, 55.2169)
(0.766285, 55.4504)
(0.768687, 54.2341)
(0.771089, 54.0115)
(0.773492, 54.4491)
(0.775894, 54.7969)
(0.778296, 55.5464)
(0.780698, 51.7949)
(0.7831, 55.4067)
(0.785502, 53.6066)
(0.787905, 55.0773)
(0.790307, 56.1029)
(0.792709, 54.4461)
(0.795111, 56.0885)
(0.797513, 54.7568)
(0.799915, 55.1573)
(0.802317, 53.798)
(0.804719, 55.2344)
(0.807122, 54.9522)
(0.809524, 54.3267)
(0.811926, 55.7423)
(0.814328, 54.8755)
(0.81673, 58.0205)
(0.819132, 57.3011)
(0.821535, 56.9876)
(0.823937, 59.2286)
(0.826339, 58.8836)
(0.828741, 58.2791)
(0.831143, 57.6628)
(0.833545, 58.8832)
(0.835947, 55.8703)
(0.83835, 56.4064)
(0.840752, 57.1848)
(0.843154, 57.5196)
(0.845556, 58.3373)
(0.847958, 56.5632)
(0.85036, 57.7965)
(0.852762, 56.8527)
(0.855165, 58.7422)
(0.857567, 60.0941)
(0.859969, 59.5127)
(0.862371, 57.1779)
(0.864773, 55.6674)
(0.867175, 56.6715)
(0.869577, 58.7005)
(0.87198, 57.3372)
(0.874382, 55.458)
(0.876784, 56.1057)
(0.879186, 55.3137)
(0.881588, 55.4812)
(0.88399, 56.6157)
(0.886393, 55.1585)
(0.888795, 55.013)
(0.891197, 58.764)
(0.893599, 55.1063)
(0.896001, 57.6435)
(0.898403, 57.7655)
(0.900805, 53.9649)
(0.903208, 53.5509)
(0.90561, 55.4454)
(0.908012, 55.0821)
(0.910414, 52.9836)
(0.912816, 56.2294)
(0.915218, 55.5179)
(0.91762, 53.097)
(0.920023, 56.4038)
(0.922425, 54.592)
(0.924827, 55.337)
(0.927229, 56.2744)
(0.929631, 55.0436)
(0.932033, 55.9583)
(0.934435, 52.5839)
(0.936838, 52.5276)
(0.93924, 54.6502)
(0.941642, 54.5541)
(0.944044, 53.536)
(0.946446, 54.4725)
(0.948848, 54.2213)
(0.951251, 53.9104)
(0.953653, 54.9621)
(0.956055, 54.3752)
(0.958457, 55.2616)
(0.960859, 54.5771)
(0.963261, 52.6299)
(0.965663, 53.5998)
(0.968066, 56.0166)
(0.970468, 55.0426)
(0.97287, 52.4684)
(0.975272, 51.6205)
(0.977674, 52.9954)
(0.980076, 52.9953)
(0.982478, 54.759)
(0.984881, 54.4547)
(0.987283, 53.6688)
(0.989685, 52.6857)
(0.992087, 54.4275)
(0.994489, 53.624)
(0.996891, 53.3735)
(0.999293, 55.217)
(1,0)
};

==> exp_plots/payload_comparison/x_da_no_fill.tex <==
\addplot[
    fill=none,draw = clr1,opacity=1.0,
    line width= \linew pt
    ]
 %%
coordinates {
(0,   -0)
(0,   -0.0126766)
(0.00240249,   -0.0048115)
(0.00480497,   0.00156844)
(0.00720746,   0.014353)
(0.00960995,   0.0202765)
(0.0120124,   0.0326366)
(0.0144149,   0.0452058)
(0.0168174,   0.0515179)
(0.0192199,   0.0450583)
(0.0216224,   0.0566123)
(0.0240249,   0.0793038)
(0.0264274,   0.0854172)
(0.0288298,   0.0709533)
(0.0312323,   0.0564784)
(0.0336348,   0.0453178)
(0.0360373,   0.0279483)
(0.0384398,   0.0137973)
(0.0408423,   -0.00213128)
(0.0432448,   -0.0304456)
(0.0456473,   -0.0370141)
(0.0480497,   -0.037904)
(0.0504522,   -0.0177952)
(0.0528547,   -0.00900266)
(0.0552572,   0.00327449)
(0.0576597,   0.020908)
(0.0600622,   0.0424856)
(0.0624647,   0.0623221)
(0.0648672,   0.0758426)
(0.0672696,   0.058495)
(0.0696721,   0.0423714)
(0.0720746,   0.0295179)
(0.0744771,   0.0184845)
(0.0768796,   0.00916259)
(0.0792821,   -0.00197849)
(0.0816846,   -0.00709943)
(0.0840871,   -0.0273847)
(0.0864895,   -0.0673321)
(0.088892,   -0.0969621)
(0.0912945,   -0.110943)
(0.093697,   -0.101174)
(0.0960995,   -0.0707528)
(0.098502,   -0.0330115)
(0.100904,   0.00972873)
(0.103307,   0.0130458)
(0.105709,   0.0185805)
(0.108112,   0.0217137)
(0.110514,   0.0325372)
(0.112917,   0.0409135)
(0.115319,   0.0388255)
(0.117722,   0.0365225)
(0.120124,   0.0272191)
(0.122527,   0.0239245)
(0.124929,   0.0235844)
(0.127332,   0.0121627)
(0.129734,   0.00510986)
(0.132137,   -0.0109654)
(0.134539,   -0.0187555)
(0.136942,   -0.0249309)
(0.139344,   -0.02677)
(0.141747,   -0.0269767)
(0.144149,   -0.0200423)
(0.146552,   -0.0127133)
(0.148954,   -0.00699074)
(0.151357,   -0.00668484)
(0.153759,   -0.0142644)
(0.156162,   -0.0557011)
(0.158564,   -0.113599)
(0.160967,   -0.150152)
(0.163369,   -0.148107)
(0.165772,   -0.149422)
(0.168174,   -0.14327)
(0.170577,   -0.12902)
(0.172979,   -0.113118)
(0.175382,   -0.0616879)
(0.177784,   -0.00815782)
(0.180187,   0.026461)
(0.182589,   0.0506221)
(0.184992,   0.0668923)
(0.187394,   0.0844981)
(0.189796,   0.101139)
(0.192199,   0.112545)
(0.194601,   0.10116)
(0.197004,   0.0849998)
(0.199406,   0.0634512)
(0.201809,   0.0567518)
(0.204211,   0.0279081)
(0.206614,   -0.00147154)
(0.209016,   -0.00572285)
(0.211419,   0.00336651)
(0.213821,   0.00684668)
(0.216224,   0.000755011)
(0.218626,   -0.0210776)
(0.221029,   -0.0197518)
(0.223431,   -0.0154037)
(0.225834,   -0.00917149)
(0.228236,   -0.0071431)
(0.230639,   0.00706858)
(0.233041,   0.0146828)
(0.235444,   0.0332219)
(0.237846,   0.069345)
(0.240249,   0.106689)
(0.242651,   0.152878)
(0.245054,   0.183497)
(0.247456,   0.195067)
(0.249859,   0.193342)
(0.252261,   0.15926)
(0.254664,   0.106805)
(0.257066,   0.0721862)
(0.259469,   0.0452937)
(0.261871,   0.028699)
(0.264274,   -0.00400546)
(0.266676,   -0.0273718)
(0.269079,   -0.0409442)
(0.271481,   -0.0470024)
(0.273884,   -0.0314994)
(0.276286,   -0.0212601)
(0.278689,   -0.0252814)
(0.281091,   -0.0300749)
(0.283493,   -0.0295602)
(0.285896,   -0.0188497)
(0.288298,   -0.0106143)
(0.290701,   -0.000683047)
(0.293103,   -0.000294015)
(0.295506,   0.00443752)
(0.297908,   -0.00241523)
(0.300311,   -0.0265359)
(0.302713,   -0.034159)
(0.305116,   -0.032838)
(0.307518,   -0.0214708)
(0.309921,   -0.0154038)
(0.312323,   -0.00198447)
(0.314726,   0.00736688)
(0.317128,   0.0139378)
(0.319531,   0.0259809)
(0.321933,   0.0312351)
(0.324336,   0.0262142)
(0.326738,   0.0198289)
(0.329141,   0.0223925)
(0.331543,   0.00477104)
(0.333946,   -0.0126522)
(0.336348,   -0.0316448)
(0.338751,   -0.0255637)
(0.341153,   -0.0306973)
(0.343556,   -0.0351391)
(0.345958,   -0.059048)
(0.348361,   -0.117501)
(0.350763,   -0.162605)
(0.353166,   -0.179007)
(0.355568,   -0.179895)
(0.357971,   -0.153806)
(0.360373,   -0.126873)
(0.362776,   -0.109494)
(0.365178,   -0.0395464)
(0.367581,   0.0166175)
(0.369983,   0.0586439)
(0.372386,   0.0808604)
(0.374788,   0.102389)
(0.37719,   0.112387)
(0.379593,   0.109597)
(0.381995,   0.102592)
(0.384398,   0.0815654)
(0.3868,   0.0526281)
(0.389203,   0.036594)
(0.391605,   0.0113168)
(0.394008,   -0.0228571)
(0.39641,   -0.0420278)
(0.398813,   -0.0561634)
(0.401215,   -0.0580238)
(0.403618,   -0.0546477)
(0.40602,   -0.043505)
(0.408423,   -0.0253356)
(0.410825,   0.000943886)
(0.413228,   0.0468728)
(0.41563,   0.0897714)
(0.418033,   0.13598)
(0.420435,   0.16757)
(0.422838,   0.176239)
(0.42524,   0.155721)
(0.427643,   0.11589)
(0.430045,   0.0913556)
(0.432448,   0.0656359)
(0.43485,   0.0430435)
(0.437253,   0.006657)
(0.439655,   -0.0206205)
(0.442058,   -0.0326677)
(0.44446,   -0.0413326)
(0.446863,   -0.0568667)
(0.449265,   -0.0704143)
(0.451668,   -0.0689537)
(0.45407,   -0.0582185)
(0.456473,   -0.0397975)
(0.458875,   -0.020627)
(0.461278,   -0.0124896)
(0.46368,   -0.0229978)
(0.466083,   -0.0214235)
(0.468485,   0.0113959)
(0.470887,   0.0438582)
(0.47329,   0.0638496)
(0.475692,   0.0708136)
(0.478095,   0.0699573)
(0.480497,   0.0588823)
(0.4829,   0.0483656)
(0.485302,   0.0373667)
(0.487705,   0.0212578)
(0.490107,   0.00905345)
(0.49251,   -0.00495926)
(0.494912,   -0.0150737)
(0.497315,   -0.00879962)
(0.499717,   -0.00760307)
(0.50212,   -0.0046877)
(0.504522,   -0.00155915)
(0.506925,   -0.00222068)
(0.509327,   -0.000317778)
(0.51173,   0.0124698)
(0.514132,   0.0143419)
(0.516535,   0.0246943)
(0.518937,   0.0300302)
(0.52134,   0.0256461)
(0.523742,   0.0303254)
(0.526145,   0.0360495)
(0.528547,   0.0232739)
(0.53095,   0.0126154)
(0.533352,   0.0227987)
(0.535755,   0.0171653)
(0.538157,   0.00505374)
(0.54056,   -0.0116887)
(0.542962,   -0.00540935)
(0.545365,   0.000415904)
(0.547767,   -0.00429946)
(0.55017,   -0.0195416)
(0.552572,   -0.0359814)
(0.554975,   -0.034523)
(0.557377,   -0.038439)
(0.55978,   -0.0374879)
(0.562182,   -0.0418089)
(0.564584,   -0.0307544)
(0.566987,   -0.0231864)
(0.569389,   -0.0319057)
(0.571792,   -0.0507559)
(0.574194,   -0.0607159)
(0.576597,   -0.0864308)
(0.578999,   -0.0918876)
(0.581402,   -0.0841786)
(0.583804,   -0.0708025)
(0.586207,   -0.0597121)
(0.588609,   -0.0362764)
(0.591012,   -0.0127479)
(0.593414,   -0.00333964)
(0.595817,   0.00884019)
(0.598219,   0.0124118)
(0.600622,   0.00143894)
(0.603024,   0.00240808)
(0.605427,   -0.00606177)
(0.607829,   -0.000825324)
(0.610232,   0.00473817)
(0.612634,   0.000553135)
(0.615037,   -0.00202234)
(0.617439,   -0.0160437)
(0.619842,   -0.0346071)
(0.622244,   -0.0471986)
(0.624647,   -0.0566543)
(0.627049,   -0.054681)
(0.629452,   -0.0555394)
(0.631854,   -0.0471982)
(0.634257,   -0.0561347)
(0.636659,   -0.0455797)
(0.639062,   -0.00713373)
(0.641464,   0.0398666)
(0.643867,   0.0770626)
(0.646269,   0.0879872)
(0.648672,   0.0916916)
(0.651074,   0.093293)
(0.653477,   0.0882264)
(0.655879,   0.0836549)
(0.658282,   0.0760954)
(0.660684,   0.0606208)
(0.663086,   0.0382414)
(0.665489,   0.0192674)
(0.667891,   0.00916236)
(0.670294,   0.00522711)
(0.672696,   0.0154236)
(0.675099,   0.0181321)
(0.677501,   0.0196367)
(0.679904,   0.018535)
(0.682306,   0.0270239)
(0.684709,   0.038446)
(0.687111,   0.0443121)
(0.689514,   0.033155)
(0.691916,   0.0221062)
(0.694319,   0.0119773)
(0.696721,   0.0020285)
(0.699124,   -0.0318103)
(0.701526,   -0.0376137)
(0.703929,   -0.0332397)
(0.706331,   -0.0201503)
(0.708734,   -0.00735376)
(0.711136,   0.00678589)
(0.713539,   0.0123316)
(0.715941,   0.0181601)
(0.718344,   0.0345852)
(0.720746,   0.0429085)
(0.723149,   0.0394525)
(0.725551,   0.0293443)
(0.727954,   0.0311971)
(0.730356,   0.0345645)
(0.732759,   0.0409396)
(0.735161,   0.036531)
(0.737564,   0.0320611)
(0.739966,   0.0319562)
(0.742369,   0.0294599)
(0.744771,   0.0218363)
(0.747173,   0.0141996)
(0.749576,   0.000180571)
(0.751978,   -0.0117764)
(0.754381,   -0.022266)
(0.756783,   -0.0396535)
(0.759186,   -0.0456039)
(0.761588,   -0.0386677)
(0.763991,   -0.0326316)
(0.766393,   -0.0201047)
(0.768796,   -0.0193018)
(0.771198,   -0.0212223)
(0.773601,   -0.0294362)
(0.776003,   -0.0225093)
(0.778406,   -0.0091405)
(0.780808,   0.00139953)
(0.783211,   0.00455176)
(0.785613,   -0.00107461)
(0.788016,   0.00238924)
(0.790418,   0.0111362)
(0.792821,   0.031045)
(0.795223,   0.0480213)
(0.797626,   0.0572191)
(0.800028,   0.0532146)
(0.802431,   0.0531635)
(0.804833,   0.0393519)
(0.807236,   0.0238666)
(0.809638,   0.000138908)
(0.812041,   -0.0246017)
(0.814443,   -0.0381188)
(0.816846,   -0.0433071)
(0.819248,   -0.0432433)
(0.821651,   -0.0434648)
(0.824053,   -0.0358154)
(0.826456,   -0.0268622)
(0.828858,   -0.0151039)
(0.831261,   -0.00981526)
(0.833663,   -0.00311706)
(0.836066,   -0.00394284)
(0.838468,   -0.0119973)
(0.840871,   -0.00181643)
(0.843273,   0.012648)
(0.845675,   0.0191333)
(0.848078,   0.0129164)
(0.85048,   0.0098369)
(0.852883,   0.00663017)
(0.855285,   -0.00132025)
(0.857688,   -0.00113539)
(0.86009,   0.00147965)
(0.862493,   0.00643326)
(0.864895,   0.0217302)
(0.867298,   0.0243128)
(0.8697,   0.0273896)
(0.872103,   0.0404377)
(0.874505,   0.0404788)
(0.876908,   0.0362862)
(0.87931,   0.0389949)
(0.881713,   0.034261)
(0.884115,   0.0247273)
(0.886518,   0.0216138)
(0.88892,   0.0196456)
(0.891323,   0.0195067)
(0.893725,   0.010517)
(0.896128,   -0.00832618)
(0.89853,   -0.0177445)
(0.900933,   -0.0203917)
(0.903335,   -0.0259181)
(0.905738,   -0.0189226)
(0.90814,   -0.0176079)
(0.910543,   -0.00751574)
(0.912945,   -0.00277189)
(0.915348,   0.0104854)
(0.91775,   0.0219473)
(0.920153,   0.0175394)
(0.922555,   0.0106165)
(0.924958,   -0.00387582)
(0.92736,   -0.0220564)
(0.929763,   -0.0386606)
(0.932165,   -0.0284198)
(0.934568,   -0.0111154)
(0.93697,   0.00481812)
(0.939372,   0.0055566)
(0.941775,   0.00721862)
(0.944178,   0.0193495)
(0.94658,   0.0294241)
(0.948982,   0.0301952)
(0.951385,   0.0269353)
(0.953787,   0.0293308)
(0.95619,   0.0392793)
(0.958592,   0.0416819)
(0.960995,   0.0323538)
(0.963397,   0.0177336)
(0.9658,   0.0104427)
(0.968202,   0.00425026)
(0.970605,   -0.00870931)
(0.973007,   -0.0112174)
(0.97541,   -0.0337879)
(0.977812,   -0.074445)
(0.980215,   -0.0838964)
(0.982617,   -0.0796161)
(0.98502,   -0.0686126)
(0.987422,   -0.05595)
(0.989825,   -0.04385)
(0.992227,   -0.0224646)
(0.99463,   -0.000255233)
(0.997032,   0.0189684)
(0.999435,   0.030989)
(1.0,   -0)
};

==> exp_plots/payload_comparison/x_tmdc_gt_no_fill.tex <==
\addplot[
    fill=none,draw = clr2,opacity=1.0,
    line width= \linew pt
    ]
 %%
coordinates {
(0,   -0)
(0,   0.0713527)
(0.00240657,   0.0732646)
(0.00481314,   0.0636901)
(0.00721971,   0.0446121)
(0.00962627,   0.0290541)
(0.0120328,   0.0137468)
(0.0144394,   -0.0255472)
(0.016846,   -0.0408085)
(0.0192525,   -0.0307712)
(0.0216591,   -0.0284789)
(0.0240657,   -0.0158882)
(0.0264723,   -0.00588056)
(0.0288788,   -0.000946365)
(0.0312854,   0.00697322)
(0.033692,   0.0162282)
(0.0360985,   0.0140592)
(0.0385051,   0.0197017)
(0.0409117,   0.0161316)
(0.0433182,   0.015291)
(0.0457248,   0.0190674)
(0.0481314,   0.0370886)
(0.0505379,   0.0267763)
(0.0529445,   0.0155326)
(0.0553511,   -0.0110273)
(0.0577576,   -0.0202413)
(0.0601642,   -0.0285594)
(0.0625708,   -0.0305519)
(0.0649773,   -0.0251129)
(0.0673839,   -0.0146771)
(0.0697905,   -0.00316963)
(0.0721971,   0.00562048)
(0.0746036,   0.00613746)
(0.0770102,   0.0158417)
(0.0794168,   0.0215314)
(0.0818233,   0.0224343)
(0.0842299,   0.0190796)
(0.0866365,   0.0219209)
(0.089043,   0.0233288)
(0.0914496,   0.0188155)
(0.0938562,   0.00869107)
(0.0962627,   -0.00511115)
(0.0986693,   -0.00935128)
(0.101076,   -0.0200463)
(0.103482,   -0.0336797)
(0.105889,   -0.0387709)
(0.108296,   -0.0320821)
(0.110702,   -0.0219624)
(0.113109,   -0.0136619)
(0.115515,   -0.00829819)
(0.117922,   -0.0120878)
(0.120328,   -0.0119688)
(0.122735,   -0.000752535)
(0.125142,   0.0051081)
(0.127548,   0.00954423)
(0.129955,   0.0085712)
(0.132361,   -0.0016001)
(0.134768,   -0.00426932)
(0.137174,   -0.0052302)
(0.139581,   -0.0115404)
(0.141988,   -0.00610432)
(0.144394,   -0.0141677)
(0.146801,   -0.0205462)
(0.149207,   -0.0229709)
(0.151614,   -0.0222625)
(0.15402,   -0.000609206)
(0.156427,   0.0387714)
(0.158834,   0.0572316)
(0.16124,   0.0529262)
(0.163647,   0.0417835)
(0.166053,   0.0394441)
(0.16846,   0.0299708)
(0.170866,   0.021667)
(0.173273,   -0.00377335)
(0.17568,   -0.0169926)
(0.178086,   -0.0293867)
(0.180493,   -0.0180698)
(0.182899,   -0.0140023)
(0.185306,   -0.0222286)
(0.187712,   -0.0402783)
(0.190119,   -0.0575673)
(0.192525,   -0.0587436)
(0.194932,   -0.041714)
(0.197339,   -0.0146689)
(0.199745,   -0.00239297)
(0.202152,   0.0173158)
(0.204558,   0.0341038)
(0.206965,   0.0473813)
(0.209371,   0.0396897)
(0.211778,   0.0305084)
(0.214185,   0.0173048)
(0.216591,   -0.0112905)
(0.218998,   -0.0693929)
(0.221404,   -0.0801365)
(0.223811,   -0.068269)
(0.226217,   -0.0373456)
(0.228624,   -0.025072)
(0.231031,   -0.0167304)
(0.233437,   -0.00618314)
(0.235844,   0.0108668)
(0.23825,   0.00699117)
(0.240657,   -0.00302877)
(0.243063,   -0.00262663)
(0.24547,   -0.00462217)
(0.247877,   0.00665729)
(0.250283,   0.0159379)
(0.25269,   0.00617215)
(0.255096,   -0.00530479)
(0.257503,   -0.00383883)
(0.259909,   0.000724871)
(0.262316,   -0.000646408)
(0.264723,   -0.00835324)
(0.267129,   0.00432537)
(0.269536,   0.0264831)
(0.271942,   0.046402)
(0.274349,   0.0410151)
(0.276755,   0.0428893)
(0.279162,   0.0413562)
(0.281568,   0.041511)
(0.283975,   0.0347268)
(0.286382,   0.0326381)
(0.288788,   0.0212937)
(0.291195,   -0.00303447)
(0.293601,   -0.0274925)
(0.296008,   -0.037214)
(0.298414,   -0.0443001)
(0.300821,   -0.0481057)
(0.303228,   -0.0504939)
(0.305634,   -0.0641137)
(0.308041,   -0.0666545)
(0.310447,   -0.0678062)
(0.312854,   -0.0523159)
(0.31526,   -0.0267385)
(0.317667,   -0.00917657)
(0.320074, 6.59162e-05)
(0.32248,   -0.00616845)
(0.324887,   -0.0134303)
(0.327293,   -0.0139566)
(0.3297,   -0.0173003)
(0.332106,   -0.0287361)
(0.334513,   -0.0330132)
(0.33692,   -0.0471931)
(0.339326,   -0.0581993)
(0.341733,   -0.0813774)
(0.344139,   -0.0965589)
(0.346546,   -0.0892906)
(0.348952,   -0.0778624)
(0.351359,   -0.0662489)
(0.353766,   -0.0507313)
(0.356172,   -0.0187851)
(0.358579,   0.0146343)
(0.360985,   0.0290217)
(0.363392,   0.037465)
(0.365798,   0.0377096)
(0.368205,   0.037726)
(0.370612,   0.0356593)
(0.373018,   0.0227662)
(0.375425,   0.00603642)
(0.377831,   0.00477432)
(0.380238,   -0.00127685)
(0.382644,   -0.00556811)
(0.385051,   -0.0138686)
(0.387458,   -0.0217981)
(0.389864,   -0.0212153)
(0.392271,   -0.0100747)
(0.394677,   -0.00751982)
(0.397084,   -0.0123136)
(0.39949,   -0.0492427)
(0.401897,   -0.114995)
(0.404304,   -0.206454)
(0.40671,   -0.280367)
(0.409117,   -0.304404)
(0.411523,   -0.276707)
(0.41393,   -0.221082)
(0.416336,   -0.143334)
(0.418743,   -0.0644893)
(0.421149,   0.00461109)
(0.423556,   0.0316368)
(0.425963,   0.0419988)
(0.428369,   0.0509346)
(0.430776,   0.0723285)
(0.433182,   0.0873914)
(0.435589,   0.0752491)
(0.437995,   0.0378528)
(0.440402,   0.0241555)
(0.442809,   0.0288717)
(0.445215,   0.0291807)
(0.447622,   0.0309464)
(0.450028,   0.0277588)
(0.452435,   0.016235)
(0.454841,   0.0128217)
(0.457248,   0.030738)
(0.459655,   0.0265495)
(0.462061,   0.0245657)
(0.464468,   0.0245701)
(0.466874,   0.0230916)
(0.469281,   0.0351803)
(0.471687,   0.0273886)
(0.474094,   0.0247522)
(0.476501,   0.0262558)
(0.478907,   0.049949)
(0.481314,   0.0940027)
(0.48372,   0.163613)
(0.486127,   0.187106)
(0.488533,   0.164318)
(0.49094,   0.135319)
(0.493347,   0.111887)
(0.495753,   0.0784962)
(0.49816,   0.0503707)
(0.500566,   0.0208175)
(0.502973,   -0.00989307)
(0.505379,   -0.0353739)
(0.507786,   -0.0503079)
(0.510193,   -0.0608317)
(0.512599,   -0.0568346)
(0.515006,   -0.0337851)
(0.517412,   -0.0179961)
(0.519819,   -0.0152007)
(0.522225,   -0.00537549)
(0.524632,   -0.00666887)
(0.527039,   -0.0313236)
(0.529445,   -0.0731494)
(0.531852,   -0.137453)
(0.534258,   -0.182412)
(0.536665,   -0.182815)
(0.539071,   -0.159076)
(0.541478,   -0.129175)
(0.543884,   -0.102143)
(0.546291,   -0.0612094)
(0.548698,   -0.0143964)
(0.551104,   0.0194183)
(0.553511,   0.0343561)
(0.555917,   0.0283162)
(0.558324,   0.0369176)
(0.56073,   0.0560148)
(0.563137,   0.067631)
(0.565544,   0.0696358)
(0.56795,   0.0441824)
(0.570357,   0.00843087)
(0.572763,   -0.0220427)
(0.57517,   -0.0388383)
(0.577576,   -0.0453227)
(0.579983,   -0.0506279)
(0.58239,   -0.0417258)
(0.584796,   -0.0316493)
(0.587203,   -0.00984505)
(0.589609,   0.0132362)
(0.592016,   0.0168631)
(0.594422,   0.0124718)
(0.596829,   0.0146968)
(0.599236,   0.0470912)
(0.601642,   0.107844)
(0.604049,   0.159297)
(0.606455,   0.19554)
(0.608862,   0.183884)
(0.611268,   0.146114)
(0.613675,   0.101402)
(0.616082,   0.036347)
(0.618488,   -0.0187266)
(0.620895,   -0.0516065)
(0.623301,   -0.0685285)
(0.625708,   -0.0697407)
(0.628114,   -0.0791669)
(0.630521,   -0.0736588)
(0.632927,   -0.0612155)
(0.635334,   -0.0687162)
(0.637741,   -0.059145)
(0.640147,   -0.0497675)
(0.642554,   -0.0365155)
(0.64496,   -0.0111638)
(0.647367,   0.00536632)
(0.649774,   0.00842714)
(0.65218,   -0.0173125)
(0.654587,   -0.0387722)
(0.656993,   -0.041612)
(0.6594,   -0.0315677)
(0.661806,   -0.0155579)
(0.664213,   -0.00831608)
(0.666619,   -0.00268307)
(0.669026,   0.0174109)
(0.671433,   0.0262393)
(0.673839,   0.0203129)
(0.676246,   0.0112803)
(0.678652,   0.00143667)
(0.681059,   -0.0106858)
(0.683465,   -0.0170274)
(0.685872,   -0.0306474)
(0.688279,   -0.044683)
(0.690685,   -0.0537458)
(0.693092,   -0.0681523)
(0.695498,   -0.0761216)
(0.697905,   -0.0621855)
(0.700311,   -0.0422427)
(0.702718,   -0.038078)
(0.705125,   -0.030978)
(0.707531,   -0.0185048)
(0.709938,   0.00751676)
(0.712344,   0.0152729)
(0.714751,   0.0425958)
(0.717157,   0.0433756)
(0.719564,   0.0408383)
(0.72197,   0.0233655)
(0.724377,   0.0336547)
(0.726784,   0.0332208)
(0.72919,   0.0230352)
(0.731597,   0.00924157)
(0.734003,   -0.0137135)
(0.73641,   -0.0369242)
(0.738817,   -0.0431148)
(0.741223,   -0.0497895)
(0.74363,   -0.059239)
(0.746036,   -0.0658539)
(0.748443,   -0.0804291)
(0.750849,   -0.0760546)
(0.753256,   -0.0586388)
(0.755662,   -0.0375113)
(0.758069,   -0.0118588)
(0.760476,   -0.00812123)
(0.762882,   -0.0293699)
(0.765289,   -0.0501662)
(0.767695,   -0.0519279)
(0.770102,   -0.045761)
(0.772509,   -0.0482341)
(0.774915,   -0.0656491)
(0.777322,   -0.0645746)
(0.779728,   -0.0598516)
(0.782135,   -0.0675388)
(0.784541,   -0.0678784)
(0.786948,   -0.0606105)
(0.789355,   -0.0412106)
(0.791761,   -0.0117479)
(0.794168,   0.0318333)
(0.796574,   0.0568779)
(0.798981,   0.0524914)
(0.801387,   0.0455592)
(0.803794,   0.0374842)
(0.8062,   0.0332535)
(0.808607,   0.0249594)
(0.811014,   0.0113447)
(0.81342,   -0.000909316)
(0.815827,   -0.0116644)
(0.818233,   -0.0130539)
(0.82064,   -0.0112128)
(0.823046,   -0.00847729)
(0.825453,   -0.0070149)
(0.82786,   -0.0121407)
(0.830266,   -0.022868)
(0.832673,   -0.0289796)
(0.835079,   -0.03123)
(0.837486,   -0.0199179)
(0.839892,   -0.0209344)
(0.842299,   -0.0191728)
(0.844706,   -0.0212426)
(0.847112,   -0.0150385)
(0.849519,   0.00386399)
(0.851925,   0.0219532)
(0.854332,   0.0293118)
(0.856738,   0.027733)
(0.859145,   0.0172057)
(0.861552,   0.0214231)
(0.863958,   0.0354476)
(0.866365,   0.0355923)
(0.868771,   0.028881)
(0.871178,   0.0262947)
(0.873584,   0.0131647)
(0.875991,   -0.00857268)
(0.878397,   0.00466232)
(0.880804,   0.0424436)
(0.883211,   0.0565022)
(0.885617,   0.050601)
(0.888024,   0.032503)
(0.89043,   0.0228387)
(0.892837,   0.0204868)
(0.895243,   0.0186473)
(0.89765,   0.0118493)
(0.900057,   -0.00672749)
(0.902463,   -0.0293391)
(0.90487,   -0.0454843)
(0.907276,   -0.0416277)
(0.909683,   -0.0594235)
(0.912089,   -0.0657557)
(0.914496,   -0.0520984)
(0.916903,   -0.0139478)
(0.919309,   0.0102875)
(0.921716,   0.0249605)
(0.924122,   0.0483219)
(0.926529,   0.07332)
(0.928935,   0.067967)
(0.931342,   0.0413759)
(0.933749,   0.00894102)
(0.936155,   -0.00198729)
(0.938562,   -0.00616678)
(0.940968,   -0.00383807)
(0.943375,   -0.00234355)
(0.945781,   0.00596126)
(0.948188,   0.0114645)
(0.950595,   0.0106389)
(0.953001,   0.00809421)
(0.955408,   0.00456988)
(0.957814,   0.00633371)
(0.960221,   0.00395973)
(0.962627,   0.0046056)
(0.965034,   0.00811975)
(0.967441,   0.00492029)
(0.969847,   -0.0121668)
(0.972254,   -0.0250213)
(0.97466,   -0.0274329)
(0.977067,   -0.0245025)
(0.979473,   -0.0220268)
(0.98188,   -0.0133786)
(0.984286,   -0.0142918)
(0.986693,   -0.0189619)
(0.9891,   -0.022767)
(0.991506,   -0.0267466)
(0.993913,   -0.0128402)
(0.996319,   0.00386711)
(0.998726,   0.0127711)
(1.0,   -0)
};

==> exp_plots/payload_comparison/x_tmdc_no_fill.tex <==
\addplot[
    fill=none,draw = clr3,opacity=1.0,
    line width= \linew pt
    ]
 %%
coordinates {
(0,   -0)
(0,   0.0641287)
(0.00240215,   0.050748)
(0.0048043,   0.0323166)
(0.00720644,   0.0202602)
(0.00960859,   0.00837656)
(0.0120107,   0.00206367)
(0.0144129,   -0.000882384)
(0.016815,   0.0119145)
(0.0192172,   0.0283124)
(0.0216193,   0.0284283)
(0.0240215,   0.0176502)
(0.0264236,   0.0195539)
(0.0288258,   0.0203036)
(0.0312279,   0.0269342)
(0.0336301,   0.0295052)
(0.0360322,   0.0368012)
(0.0384344,   0.0427486)
(0.0408365,   0.0382847)
(0.0432387,   0.0285315)
(0.0456408,   0.0218075)
(0.048043,   0.0281974)
(0.0504451,   0.0274834)
(0.0528472,   0.0212107)
(0.0552494,   0.0213345)
(0.0576515,   0.0210256)
(0.0600537,   0.0137224)
(0.0624558,   0.0156312)
(0.064858,   0.0144663)
(0.0672601,   0.005138)
(0.0696623,   0.00720639)
(0.0720644,   0.0148354)
(0.0744666,   0.0239065)
(0.0768687,   0.0325038)
(0.0792709,   0.036846)
(0.081673,   0.0283136)
(0.0840752,   0.0223637)
(0.0864773,   0.0216915)
(0.0888795,   0.0233571)
(0.0912816,   0.0248438)
(0.0936838,   0.0269934)
(0.0960859,   0.0324273)
(0.0984881,   0.0256548)
(0.10089,   0.0226937)
(0.103292,   0.0214125)
(0.105694,   0.0122421)
(0.108097,   0.0105139)
(0.110499,   0.0131361)
(0.112901,   0.0199673)
(0.115303,   0.0145239)
(0.117705,   0.0143777)
(0.120107,   0.0200787)
(0.12251,   0.0221173)
(0.124912,   0.0129046)
(0.127314,   0.00424113)
(0.129716,   0.0020597)
(0.132118,   0.00975467)
(0.13452,   0.0100689)
(0.136922,   0.0103531)
(0.139325,   0.00762862)
(0.141727,   0.0160092)
(0.144129,   0.0270432)
(0.146531,   0.0317493)
(0.148933,   0.034464)
(0.151335,   0.0278259)
(0.153737,   0.0178971)
(0.15614,   0.011366)
(0.158542,   0.0181139)
(0.160944,   0.0243298)
(0.163346,   0.0357243)
(0.165748,   0.0535249)
(0.16815,   0.0742872)
(0.170552,   0.0948189)
(0.172955,   0.0902031)
(0.175357,   0.0651828)
(0.177759,   0.0487924)
(0.180161,   0.044846)
(0.182563,   0.0461815)
(0.184965,   0.0469682)
(0.187368,   0.0491119)
(0.18977,   0.0390159)
(0.192172,   0.0396767)
(0.194574,   0.0402474)
(0.196976,   0.0158033)
(0.199378,   -0.0165469)
(0.20178,   -0.0360282)
(0.204183,   -0.0590113)
(0.206585,   -0.0630756)
(0.208987,   -0.044284)
(0.211389,   -0.0158522)
(0.213791,   0.0138245)
(0.216193,   0.0449407)
(0.218595,   0.0609352)
(0.220998,   0.0603875)
(0.2234,   0.064112)
(0.225802,   0.0510658)
(0.228204,   0.0452266)
(0.230606,   0.0385083)
(0.233008,   0.0256786)
(0.23541,   0.0119659)
(0.237813,   -0.0090411)
(0.240215,   -0.0172165)
(0.242617,   -0.0361783)
(0.245019,   -0.0444838)
(0.247421,   -0.0576011)
(0.249823,   -0.057427)
(0.252225,   -0.051484)
(0.254628,   -0.0428684)
(0.25703,   -0.0425575)
(0.259432,   -0.0298751)
(0.261834,   -0.0124682)
(0.264236,   -0.00157022)
(0.266638,   -0.00476529)
(0.269041,   0.0107144)
(0.271443,   0.0235862)
(0.273845,   0.00602711)
(0.276247,   -0.0242244)
(0.278649,   -0.0298044)
(0.281051,   -0.0219841)
(0.283453,   -0.0134793)
(0.285856,   -0.000211073)
(0.288258,   0.0111507)
(0.29066,   0.0177847)
(0.293062,   0.0264997)
(0.295464,   0.0208011)
(0.297866,   0.0258331)
(0.300268,   0.0266531)
(0.302671,   0.0320279)
(0.305073,   0.0286322)
(0.307475,   0.0315934)
(0.309877,   0.0253835)
(0.312279,   0.0343867)
(0.314681,   0.042962)
(0.317084,   0.0509879)
(0.319486,   0.0375074)
(0.321888,   0.00852685)
(0.32429,   -0.0035257)
(0.326692,   -0.0111712)
(0.329094,   -0.0180814)
(0.331496,   -0.0294495)
(0.333899,   -0.0381714)
(0.336301,   -0.0279424)
(0.338703,   -0.0175053)
(0.341105,   -0.00724196)
(0.343507,   0.00494957)
(0.345909,   0.00669435)
(0.348311,   -0.00551067)
(0.350714,   -0.0387003)
(0.353116,   -0.0503214)
(0.355518,   -0.0469712)
(0.35792,   -0.0434352)
(0.360322,   -0.0441814)
(0.362724,   -0.029543)
(0.365126,   -0.0159066)
(0.367529,   -0.00418504)
(0.369931,   -0.00464595)
(0.372333,   0.0115155)
(0.374735,   0.0403353)
(0.377137,   0.0605633)
(0.379539,   0.0583662)
(0.381941,   0.0580187)
(0.384344,   0.0532892)
(0.386746,   0.0388079)
(0.389148,   0.0189532)
(0.39155,   -0.000419812)
(0.393952,   -0.00813907)
(0.396354,   -0.0190734)
(0.398757,   -0.0170067)
(0.401159,   -0.0237962)
(0.403561,   -0.0215129)
(0.405963,   -0.0153335)
(0.408365,   0.0111156)
(0.410767,   0.0337586)
(0.413169,   0.0445805)
(0.415572,   0.0600617)
(0.417974,   0.0757967)
(0.420376,   0.0692298)
(0.422778,   0.052218)
(0.42518,   0.0377406)
(0.427582,   0.0315184)
(0.429984,   0.0261729)
(0.432387,   0.0187938)
(0.434789,   0.0166933)
(0.437191,   0.0117024)
(0.439593,   0.013563)
(0.441995,   0.0103845)
(0.444397,   0.00773464)
(0.446799,   0.0135363)
(0.449202,   0.0329037)
(0.451604,   0.0258593)
(0.454006,   0.0148215)
(0.456408,   -0.0356851)
(0.45881,   -0.0994471)
(0.461212,   -0.15858)
(0.463615,   -0.176584)
(0.466017,   -0.156817)
(0.468419,   -0.10805)
(0.470821,   -0.0749718)
(0.473223,   -0.0517313)
(0.475625,   -0.0189408)
(0.478027,   0.0168624)
(0.48043,   0.0419214)
(0.482832,   0.0465191)
(0.485234,   0.0275635)
(0.487636,   0.0106798)
(0.490038,   0.0169756)
(0.49244,   0.0318639)
(0.494842,   0.0376063)
(0.497245,   0.0377685)
(0.499647,   0.0398033)
(0.502049,   0.0444467)
(0.504451,   0.03463)
(0.506853,   0.0240064)
(0.509255,   0.0268835)
(0.511657,   0.0379893)
(0.51406,   0.0463919)
(0.516462,   0.0540777)
(0.518864,   0.0380936)
(0.521266,   0.0180483)
(0.523668,   0.0098306)
(0.52607,   0.0110971)
(0.528472,   0.0149541)
(0.530875,   0.022911)
(0.533277,   0.0627524)
(0.535679,   0.103228)
(0.538081,   0.134947)
(0.540483,   0.155572)
(0.542885,   0.150187)
(0.545288,   0.119999)
(0.54769,   0.0967875)
(0.550092,   0.0384268)
(0.552494,   -0.0242907)
(0.554896,   -0.0627659)
(0.557298,   -0.0758227)
(0.5597,   -0.0791083)
(0.562103,   -0.0679267)
(0.564505,   -0.0475382)
(0.566907,   -0.03378)
(0.569309,   -0.000279845)
(0.571711,   0.0288691)
(0.574113,   0.0281498)
(0.576515,   0.0180981)
(0.578918,   0.0072732)
(0.58132,   -0.0103426)
(0.583722,   -0.0282956)
(0.586124,   -0.0415281)
(0.588526,   -0.0644373)
(0.590928,   -0.0559547)
(0.593331,   -0.0317602)
(0.595733,   -0.00962813)
(0.598135,   -0.00558731)
(0.600537,   -0.00586583)
(0.602939,   -0.00928438)
(0.605341,   -0.00820272)
(0.607743,   -0.00502428)
(0.610146,   0.00133882)
(0.612548,   -0.000191864)
(0.61495,   0.00361614)
(0.617352,   0.0025418)
(0.619754,   0.000146888)
(0.622156,   -0.0184528)
(0.624558,   -0.0323512)
(0.626961,   -0.0494162)
(0.629363,   -0.066188)
(0.631765,   -0.0526837)
(0.634167,   -0.0413889)
(0.636569,   -0.0615322)
(0.638971,   -0.0805585)
(0.641373,   -0.112105)
(0.643776,   -0.11644)
(0.646178,   -0.0978214)
(0.64858,   -0.0700803)
(0.650982,   -0.047091)
(0.653384,   -0.0258456)
(0.655786,   -0.00546242)
(0.658189,   0.00557814)
(0.660591,   0.00137611)
(0.662993,   0.0167754)
(0.665395,   0.0288655)
(0.667797,   0.0269432)
(0.670199,   0.0341501)
(0.672601,   0.0389324)
(0.675004,   0.0314327)
(0.677406,   0.0152037)
(0.679808,   0.00303299)
(0.68221,   -0.017647)
(0.684612,   -0.0323818)
(0.687014,   -0.0299079)
(0.689416,   -0.00990994)
(0.691819,   0.00459989)
(0.694221,   0.010786)
(0.696623,   0.00827739)
(0.699025,   0.00994652)
(0.701427,   0.0241843)
(0.703829,   0.0564936)
(0.706231,   0.0819186)
(0.708634,   0.09666)
(0.711036,   0.0877166)
(0.713438,   0.0612577)
(0.71584,   0.0490259)
(0.718242,   0.0305564)
(0.720644,   0.0112636)
(0.723046,   -0.000800278)
(0.725449,   -0.0429147)
(0.727851,   -0.0569866)
(0.730253,   -0.0656274)
(0.732655,   -0.0695575)
(0.735057,   -0.0532941)
(0.737459,   -0.0475402)
(0.739861,   -0.049315)
(0.742264,   -0.0473953)
(0.744666,   -0.0478609)
(0.747068,   -0.0381409)
(0.74947,   -0.029282)
(0.751872,   -0.0180813)
(0.754274,   -0.0151894)
(0.756677,   -0.00918564)
(0.759079,   -0.00467089)
(0.761481,   0.00315982)
(0.763883,   0.00257519)
(0.766285,   0.00421873)
(0.768687,   -0.00710623)
(0.771089,   -0.0156642)
(0.773492,   -0.00505181)
(0.775894,   -0.00322627)
(0.778296,   0.0019563)
(0.780698,   -0.00769313)
(0.7831,   -0.039497)
(0.785502,   -0.0631413)
(0.787905,   -0.0705016)
(0.790307,   -0.0764804)
(0.792709,   -0.0547149)
(0.795111,   -0.023893)
(0.797513,   0.0265683)
(0.799915,   0.0384092)
(0.802317,   0.0404635)
(0.804719,   0.0268494)
(0.807122,   0.0260846)
(0.809524,   0.011293)
(0.811926,   0.00601464)
(0.814328,   0.000667634)
(0.81673,   -0.00777212)
(0.819132,   -0.0241936)
(0.821535,   -0.0407766)
(0.823937,   -0.0484549)
(0.826339,   -0.0438854)
(0.828741,   -0.0278078)
(0.831143,   0.00160979)
(0.833545,   0.0170696)
(0.835947,   0.0300982)
(0.83835,   0.0289987)
(0.840752,   0.0016232)
(0.843154,   -0.0134787)
(0.845556,   -0.0104338)
(0.847958,   0.0114922)
(0.85036,   0.00717652)
(0.852762,   -0.000780545)
(0.855165,   -0.0187018)
(0.857567,   -0.0343613)
(0.859969,   -0.0435065)
(0.862371,   -0.0496938)
(0.864773,   -0.0659274)
(0.867175,   -0.0527307)
(0.869577,   -0.0348792)
(0.87198,   -0.0283981)
(0.874382,   -0.0166617)
(0.876784,   -0.00254532)
(0.879186,   -0.00473874)
(0.881588,   -0.00825866)
(0.88399,   -0.0216392)
(0.886393,   -0.0326949)
(0.888795,   -0.0447357)
(0.891197,   -0.0636305)
(0.893599,   -0.0770125)
(0.896001,   -0.0828567)
(0.898403,   -0.0783426)
(0.900805,   -0.0891617)
(0.903208,   -0.0960728)
(0.90561,   -0.0978816)
(0.908012,   -0.0772847)
(0.910414,   -0.0611128)
(0.912816,   -0.0461073)
(0.915218,   -0.0202871)
(0.91762,   -0.00938285)
(0.920023,   0.0174753)
(0.922425,   0.0440015)
(0.924827,   0.0462822)
(0.927229,   0.0379745)
(0.929631,   0.0332994)
(0.932033,   0.0341891)
(0.934435,   0.0220242)
(0.936838,   0.00774963)
(0.93924,   0.00923895)
(0.941642,   0.0147294)
(0.944044,   0.00150471)
(0.946446,   0.008742)
(0.948848,   0.018538)
(0.951251,   0.036869)
(0.953653,   0.0516908)
(0.956055,   0.0552428)
(0.958457,   0.0468707)
(0.960859,   0.016606)
(0.963261,   0.00142912)
(0.965663,   -0.0057669)
(0.968066,   -0.0108441)
(0.970468,   -0.00726803)
(0.97287,   -0.00430621)
(0.975272,   0.00719457)
(0.977674,   0.00610731)
(0.980076,   -0.00783901)
(0.982478,   -0.000347403)
(0.984881,   0.0115818)
(0.987283,   0.0239364)
(0.989685,   0.0289212)
(0.992087,   0.0328436)
(0.994489,   0.0351377)
(0.996891,   0.0325932)
(0.999293,   0.0122706)
(1.0,   -0)
};

==> exp_plots/payload_comparison/y_da_no_fill.tex <==
\addplot[
    fill=none,draw = clr1,opacity=1.0,
    line width= \linew pt
    ]
 %%
coordinates {
(0,   -0)
(0,   0.106513)
(0.00240249,   0.101113)
(0.00480497,   0.100819)
(0.00720746,   0.0938862)
(0.00960995,   0.0788143)
(0.0120124,   0.0750521)
(0.0144149,   0.0494684)
(0.0168174,   0.0171746)
(0.0192199,   0.0206605)
(0.0216224,   0.0288047)
(0.0240249,   0.0349483)
(0.0264274,   0.0509007)
(0.0288298,   0.0660119)
(0.0312323,   0.0793285)
(0.0336348,   0.0808472)
(0.0360373,   0.101767)
(0.0384398,   0.111703)
(0.0408423,   0.110745)
(0.0432448,   0.129099)
(0.0456473,   0.132217)
(0.0480497,   0.131176)
(0.0504522,   0.125519)
(0.0528547,   0.118227)
(0.0552572,   0.095947)
(0.0576597,   0.0623532)
(0.0600622,   0.0333707)
(0.0624647,   -0.000176632)
(0.0648672,   -0.02861)
(0.0672696,   -0.033)
(0.0696721,   -0.0309263)
(0.0720746,   -0.0226555)
(0.0744771,   -0.0146728)
(0.0768796,   0.00626684)
(0.0792821,   0.0396045)
(0.0816846,   0.0492062)
(0.0840871,   0.0804667)
(0.0864895,   0.112252)
(0.088892,   0.125969)
(0.0912945,   0.138394)
(0.093697,   0.13845)
(0.0960995,   0.12597)
(0.098502,   0.108111)
(0.100904,   0.0850316)
(0.103307,   0.0756218)
(0.105709,   0.0695678)
(0.108112,   0.0575339)
(0.110514,   0.0543096)
(0.112917,   0.0597676)
(0.115319,   0.0683559)
(0.117722,   0.06527)
(0.120124,   0.06426)
(0.122527,   0.0645607)
(0.124929,   0.0980105)
(0.127332,   0.110584)
(0.129734,   0.102878)
(0.132137,   0.104963)
(0.134539,   0.0914177)
(0.136942,   0.0746977)
(0.139344,   0.0513777)
(0.141747,   0.044085)
(0.144149,   0.0203861)
(0.146552,   0.0165452)
(0.148954,   0.00186373)
(0.151357,   -0.000629264)
(0.153759,   -0.00335907)
(0.156162,   -0.00454252)
(0.158564,   0.00449806)
(0.160967,   0.0102911)
(0.163369,   0.0181933)
(0.165772,   0.0375892)
(0.168174,   0.0489467)
(0.170577,   0.0573984)
(0.172979,   0.0723285)
(0.175382,   0.0641592)
(0.177784,   0.0754885)
(0.180187,   0.0771213)
(0.182589,   0.096852)
(0.184992,   0.0997158)
(0.187394,   0.0922731)
(0.189796,   0.0809824)
(0.192199,   0.0671135)
(0.194601,   0.0651248)
(0.197004,   0.0603361)
(0.199406,   0.0585923)
(0.201809,   0.0429237)
(0.204211,   0.0180763)
(0.206614,   0.01975)
(0.209016,   0.0272619)
(0.211419,   0.0306709)
(0.213821,   0.0346873)
(0.216224,   0.0595127)
(0.218626,   0.0875467)
(0.221029,   0.0900618)
(0.223431,   0.0789063)
(0.225834,   0.0678135)
(0.228236,   0.0602247)
(0.230639,   0.0535)
(0.233041,   0.0469347)
(0.235444,   0.0360786)
(0.237846,   0.0315458)
(0.240249,   0.037735)
(0.242651,   0.0373989)
(0.245054,   0.0614719)
(0.247456,   0.0922794)
(0.249859,   0.0971911)
(0.252261,   0.107965)
(0.254664,   0.114025)
(0.257066,   0.100256)
(0.259469,   0.0783967)
(0.261871,   0.0937601)
(0.264274,   0.103691)
(0.266676,   0.0823575)
(0.269079,   0.0612747)
(0.271481,   0.0465986)
(0.273884,   0.0354171)
(0.276286,   0.0305962)
(0.278689,   0.0206322)
(0.281091,   0.0218376)
(0.283493,   0.0294263)
(0.285896,   0.04409)
(0.288298,   0.0426373)
(0.290701,   0.0413469)
(0.293103,   0.0406758)
(0.295506,   0.0511549)
(0.297908,   0.0597631)
(0.300311,   0.0679262)
(0.302713,   0.0700996)
(0.305116,   0.0680616)
(0.307518,   0.0569007)
(0.309921,   0.0492241)
(0.312323,   0.0360914)
(0.314726,   0.0299537)
(0.317128,   0.0216155)
(0.319531,   0.00197581)
(0.321933,   -0.0184565)
(0.324336,   -0.0189418)
(0.326738,   -0.00541469)
(0.329141,   0.00991158)
(0.331543,   0.0437005)
(0.333946,   0.0565804)
(0.336348,   0.0886329)
(0.338751,   0.0945798)
(0.341153,   0.10986)
(0.343556,   0.112413)
(0.345958,   0.113158)
(0.348361,   0.0878577)
(0.350763,   0.0676289)
(0.353166,   0.0321275)
(0.355568,   0.0243995)
(0.357971,   0.0256868)
(0.360373,   0.0476714)
(0.362776,   0.0591131)
(0.365178,   0.103977)
(0.367581,   0.119445)
(0.369983,   0.116414)
(0.372386,   0.103167)
(0.374788,   0.0908804)
(0.37719,   0.0857131)
(0.379593,   0.0771671)
(0.381995,   0.0721027)
(0.384398,   0.0559104)
(0.3868,   0.0478877)
(0.389203,   0.0367771)
(0.391605,   0.0250539)
(0.394008,   0.0172963)
(0.39641,   0.00880649)
(0.398813,   0.00324956)
(0.401215,   0.00665232)
(0.403618,   0.0170471)
(0.40602,   0.0730371)
(0.408423,   0.104924)
(0.410825,   0.116739)
(0.413228,   0.122903)
(0.41563,   0.125369)
(0.418033,   0.14226)
(0.420435,   0.146376)
(0.422838,   0.127214)
(0.42524,   0.0967271)
(0.427643,   0.0719512)
(0.430045,   0.0380205)
(0.432448,   0.0210127)
(0.43485,   0.022092)
(0.437253,   0.0255207)
(0.439655,   0.0252361)
(0.442058,   0.0318495)
(0.44446,   0.0414109)
(0.446863,   0.0466003)
(0.449265,   0.0347304)
(0.451668,   0.0231347)
(0.45407,   0.00481834)
(0.456473,   -0.00280734)
(0.458875,   0.00572016)
(0.461278,   0.0240691)
(0.46368,   0.0538436)
(0.466083,   0.0703188)
(0.468485,   0.0773066)
(0.470887,   0.105916)
(0.47329,   0.13045)
(0.475692,   0.144323)
(0.478095,   0.144866)
(0.480497,   0.140449)
(0.4829,   0.129744)
(0.485302,   0.109946)
(0.487705,   0.081016)
(0.490107,   0.0688724)
(0.49251,   0.0471624)
(0.494912,   0.0120678)
(0.497315,   -0.00975702)
(0.499717,   -0.0127172)
(0.50212,   0.00123779)
(0.504522,   0.0156909)
(0.506925,   0.0423293)
(0.509327,   0.0668028)
(0.51173,   0.0879062)
(0.514132,   0.0979992)
(0.516535,   0.110892)
(0.518937,   0.1194)
(0.52134,   0.136694)
(0.523742,   0.140112)
(0.526145,   0.136406)
(0.528547,   0.154105)
(0.53095,   0.150068)
(0.533352,   0.111485)
(0.535755,   0.0749092)
(0.538157,   0.0496548)
(0.54056,   0.0339667)
(0.542962,   0.019395)
(0.545365,   -0.0126587)
(0.547767,   -0.0322079)
(0.55017,   -0.0163637)
(0.552572,   0.0244772)
(0.554975,   0.0422398)
(0.557377,   0.0696854)
(0.55978,   0.0820718)
(0.562182,   0.097678)
(0.564584,   0.0878818)
(0.566987,   0.0852038)
(0.569389,   0.0952403)
(0.571792,   0.0831279)
(0.574194,   0.0555307)
(0.576597,   0.0561065)
(0.578999,   0.0650221)
(0.581402,   0.0714031)
(0.583804,   0.0749264)
(0.586207,   0.0724787)
(0.588609,   0.08001)
(0.591012,   0.10722)
(0.593414,   0.128778)
(0.595817,   0.141651)
(0.598219,   0.144383)
(0.600622,   0.15263)
(0.603024,   0.142521)
(0.605427,   0.110008)
(0.607829,   0.0653316)
(0.610232,   0.0258728)
(0.612634,   -0.0130114)
(0.615037,   -0.0294233)
(0.617439,   -0.0509436)
(0.619842,   -0.0703282)
(0.622244,   -0.0678305)
(0.624647,   -0.063358)
(0.627049,   -0.0454014)
(0.629452,   0.000112569)
(0.631854,   0.0508188)
(0.634257,   0.116739)
(0.636659,   0.149016)
(0.639062,   0.15433)
(0.641464,   0.18838)
(0.643867,   0.193739)
(0.646269,   0.20731)
(0.648672,   0.197578)
(0.651074,   0.171455)
(0.653477,   0.144597)
(0.655879,   0.129106)
(0.658282,   0.0547353)
(0.660684,   -0.00833688)
(0.663086,   -0.0234351)
(0.665489,   -0.0578486)
(0.667891,   -0.0607111)
(0.670294,   -0.0520977)
(0.672696,   -0.035584)
(0.675099,   -0.00633909)
(0.677501,   0.0127162)
(0.679904,   0.019218)
(0.682306,   0.0460844)
(0.684709,   0.0657371)
(0.687111,   0.0692908)
(0.689514,   0.0871236)
(0.691916,   0.0973045)
(0.694319,   0.0888505)
(0.696721,   0.0836036)
(0.699124,   0.0657328)
(0.701526,   0.0561643)
(0.703929,   0.0491863)
(0.706331,   0.037378)
(0.708734,   0.0328988)
(0.711136,   0.0254315)
(0.713539,   0.0240624)
(0.715941,   0.040266)
(0.718344,   0.0452124)
(0.720746,   0.0416768)
(0.723149,   0.0333525)
(0.725551,   0.0296012)
(0.727954,   0.028316)
(0.730356,   0.032339)
(0.732759,   0.0450478)
(0.735161,   0.0560427)
(0.737564,   0.045138)
(0.739966,   0.0414312)
(0.742369,   0.0517791)
(0.744771,   0.0660578)
(0.747173,   0.0724182)
(0.749576,   0.0831936)
(0.751978,   0.0798345)
(0.754381,   0.0763805)
(0.756783,   0.0759863)
(0.759186,   0.064222)
(0.761588,   0.050069)
(0.763991,   0.035334)
(0.766393,   0.0164016)
(0.768796,   -0.00750212)
(0.771198,   -0.0126547)
(0.773601,   -0.000562326)
(0.776003,   0.0197078)
(0.778406,   0.0397563)
(0.780808,   0.0538574)
(0.783211,   0.0717084)
(0.785613,   0.0715887)
(0.788016,   0.0738024)
(0.790418,   0.0688647)
(0.792821,   0.0541599)
(0.795223,   0.0451571)
(0.797626,   0.0453107)
(0.800028,   0.0428314)
(0.802431,   0.0381539)
(0.804833,   0.0446935)
(0.807236,   0.0293711)
(0.809638,   0.0306223)
(0.812041,   0.0486564)
(0.814443,   0.0461966)
(0.816846,   0.03731)
(0.819248,   0.0351978)
(0.821651,   0.0410715)
(0.824053,   0.0456466)
(0.826456,   0.0558654)
(0.828858,   0.0553521)
(0.831261,   0.0502325)
(0.833663,   0.0439376)
(0.836066,   0.0291362)
(0.838468,   0.012329)
(0.840871,   -0.00440093)
(0.843273,   -0.00335926)
(0.845675,   0.00350391)
(0.848078,   0.0220861)
(0.85048,   0.0387794)
(0.852883,   0.0555412)
(0.855285,   0.0764462)
(0.857688,   0.0977478)
(0.86009,   0.116984)
(0.862493,   0.118033)
(0.864895,   0.110978)
(0.867298,   0.101825)
(0.8697,   0.0899578)
(0.872103,   0.0475368)
(0.874505,   0.0387915)
(0.876908,   0.0487331)
(0.87931,   0.0700289)
(0.881713,   0.0915399)
(0.884115,   0.0951775)
(0.886518,   0.0930203)
(0.88892,   0.0971163)
(0.891323,   0.0881682)
(0.893725,   0.0874635)
(0.896128,   0.0653422)
(0.89853,   0.0449917)
(0.900933,   0.0300719)
(0.903335,   0.00269151)
(0.905738,   -0.0181623)
(0.90814,   -0.0272802)
(0.910543,   -0.0225257)
(0.912945,   -0.0115579)
(0.915348,   0.0112022)
(0.91775,   0.0330535)
(0.920153,   0.04603)
(0.922555,   0.0498365)
(0.924958,   0.0687848)
(0.92736,   0.0935171)
(0.929763,   0.115741)
(0.932165,   0.124849)
(0.934568,   0.11292)
(0.93697,   0.104078)
(0.939372,   0.0951662)
(0.941775,   0.0863521)
(0.944178,   0.0817254)
(0.94658,   0.0622094)
(0.948982,   0.0344538)
(0.951385,   0.0125647)
(0.953787,   -0.0123167)
(0.95619,   -0.0349791)
(0.958592,   -0.0138623)
(0.960995,   -0.00285315)
(0.963397,   0.0103363)
(0.9658,   0.0321738)
(0.968202,   0.0605509)
(0.970605,   0.0807524)
(0.973007,   0.0926196)
(0.97541,   0.10237)
(0.977812,   0.118706)
(0.980215,   0.0936655)
(0.982617,   0.0913867)
(0.98502,   0.0810596)
(0.987422,   0.0706553)
(0.989825,   0.0684683)
(0.992227,   0.0672044)
(0.99463,   0.0587733)
(0.997032,   0.0565652)
(0.999435,   0.0500484)
(1.0,   -0)
};

==> exp_plots/payload_comparison/y_tmdc_gt_no_fill.tex <==
\addplot[
    fill=none,draw = clr2,opacity=1.0,
    line width= \linew pt
    ]
 %%
coordinates {
(0,   -0)
(0,  0.00168501)
(0.00240657,   -0.0116324)
(0.00481314,   -0.00609741)
(0.00721971,  0.0113913)
(0.00962627,  0.0242981)
(0.0120328,  0.0386224)
(0.0144394,  0.0489322)
(0.016846,  0.0477639)
(0.0192525,  0.0526504)
(0.0216591,  0.0552356)
(0.0240657,  0.0539894)
(0.0264723,  0.0392771)
(0.0288788,  0.0320171)
(0.0312854,  0.032758)
(0.033692,  0.035037)
(0.0360985,  0.0329546)
(0.0385051,  0.0273994)
(0.0409117,  0.0312739)
(0.0433182,  0.0392917)
(0.0457248,  0.0367239)
(0.0481314,  0.0408961)
(0.0505379,  0.0482218)
(0.0529445,  0.0489727)
(0.0553511,  0.0557228)
(0.0577576,  0.059478)
(0.0601642,  0.0526421)
(0.0625708,  0.0440664)
(0.0649773,  0.0383835)
(0.0673839,  0.0259009)
(0.0697905,   -0.0127774)
(0.0721971,   -0.0387683)
(0.0746036,   -0.0358109)
(0.0770102,   -0.021688)
(0.0794168,   -0.0148747)
(0.0818233,   -0.0181194)
(0.0842299,  0.00442479)
(0.0866365,  0.0189484)
(0.089043,  0.0341896)
(0.0914496,  0.0455603)
(0.0938562,  0.057732)
(0.0962627,  0.0607829)
(0.0986693,  0.0595341)
(0.101076,  0.0576152)
(0.103482,  0.0525231)
(0.105889,  0.0463354)
(0.108296,  0.0275027)
(0.110702,  0.0156064)
(0.113109,   -0.00680807)
(0.115515,   -0.0274135)
(0.117922,   -0.0327209)
(0.120328,   -0.031035)
(0.122735,   -0.0285795)
(0.125142,   -0.0154314)
(0.127548,   -0.00267943)
(0.129955,   -0.00221763)
(0.132361,   -0.0130478)
(0.134768,  0.00928253)
(0.137174,  0.033578)
(0.139581,  0.073152)
(0.141988,  0.0835229)
(0.144394,  0.089509)
(0.146801,  0.0801065)
(0.149207,  0.0702758)
(0.151614,  0.0635303)
(0.15402,  0.0289878)
(0.156427,   -0.00418507)
(0.158834,   -0.011355)
(0.16124,  0.0103857)
(0.163647,  0.0320789)
(0.166053,  0.0463763)
(0.16846,  0.0591925)
(0.170866,  0.0654309)
(0.173273,  0.0891013)
(0.17568,  0.113814)
(0.178086,  0.136368)
(0.180493,  0.141174)
(0.182899,  0.155047)
(0.185306,  0.171418)
(0.187712,  0.172503)
(0.190119,  0.138435)
(0.192525,  0.0880885)
(0.194932,  0.0270257)
(0.197339,   -0.0149487)
(0.199745,   -0.0276599)
(0.202152,   -0.032889)
(0.204558,   -0.0426811)
(0.206965,   -0.0425139)
(0.209371,   -0.0139122)
(0.211778,  0.00645787)
(0.214185,  0.0166397)
(0.216591,  0.0555567)
(0.218998,  0.117095)
(0.221404,  0.127654)
(0.223811,  0.127477)
(0.226217,  0.129315)
(0.228624,  0.135726)
(0.231031,  0.125716)
(0.233437,  0.0996219)
(0.235844,  0.0641997)
(0.23825,  0.00592856)
(0.240657,   -0.0183206)
(0.243063,   -0.0446784)
(0.24547,   -0.0320755)
(0.247877,   -0.0317207)
(0.250283,   -0.00457641)
(0.25269,  0.0383926)
(0.255096,  0.0700125)
(0.257503,  0.0817413)
(0.259909,  0.0921357)
(0.262316,  0.0940951)
(0.264723,  0.0928184)
(0.267129,  0.0832362)
(0.269536,  0.0576426)
(0.271942,  0.0444051)
(0.274349,  0.0398624)
(0.276755,  0.0338681)
(0.279162,  0.008788)
(0.281568,   -0.015599)
(0.283975,   -0.0148484)
(0.286382,   -0.0107678)
(0.288788,   -0.00673314)
(0.291195,  0.00184422)
(0.293601,  0.0170345)
(0.296008,  0.0273587)
(0.298414,  0.057538)
(0.300821,  0.093875)
(0.303228,  0.108887)
(0.305634,  0.114565)
(0.308041,  0.118876)
(0.310447,  0.121278)
(0.312854,  0.11131)
(0.31526,  0.0786401)
(0.317667,  0.0445074)
(0.320074,  0.0174237)
(0.32248,  0.00430786)
(0.324887,   -0.00612003)
(0.327293,   -0.0277799)
(0.3297,   -0.0393786)
(0.332106,   -0.0562279)
(0.334513,   -0.0605009)
(0.33692,   -0.0476659)
(0.339326,   -0.0339614)
(0.341733,   -0.0260592)
(0.344139,   -0.00996726)
(0.346546,  0.00682927)
(0.348952,  0.0419875)
(0.351359,  0.0724335)
(0.353766,  0.0818005)
(0.356172,  0.102935)
(0.358579,  0.130521)
(0.360985,  0.130561)
(0.363392,  0.134045)
(0.365798,  0.123354)
(0.368205,  0.101088)
(0.370612,  0.0690356)
(0.373018,  0.0416182)
(0.375425,  0.0232185)
(0.377831,  0.00113436)
(0.380238,  0.00856917)
(0.382644,   -0.0107299)
(0.385051,   -0.0244693)
(0.387458,   -0.0188463)
(0.389864,  0.00975684)
(0.392271,  0.0221813)
(0.394677,  0.049611)
(0.397084,  0.0771336)
(0.39949,  0.0897485)
(0.401897,  0.070918)
(0.404304,  0.0683433)
(0.40671,  0.0604871)
(0.409117,  0.0552449)
(0.411523,  0.0403775)
(0.41393,  0.0326694)
(0.416336,  0.00937007)
(0.418743,   -0.0105414)
(0.421149,   -0.0398777)
(0.423556,   -0.0621397)
(0.425963,   -0.0764356)
(0.428369,   -0.0747372)
(0.430776,   -0.0737269)
(0.433182,   -0.0745279)
(0.435589,   -0.0498706)
(0.437995,   -0.0223391)
(0.440402,   -0.00145283)
(0.442809,  0.0392317)
(0.445215,  0.0757496)
(0.447622,  0.0879117)
(0.450028,  0.0938089)
(0.452435,  0.104305)
(0.454841,  0.115398)
(0.457248,  0.11528)
(0.459655,  0.108056)
(0.462061,  0.0937898)
(0.464468,  0.0728428)
(0.466874,  0.056793)
(0.469281,  0.0358257)
(0.471687,   -0.000151145)
(0.474094,   -0.0151463)
(0.476501,   -0.0146833)
(0.478907,   -0.00791022)
(0.481314,   -0.00862869)
(0.48372,  0.0317187)
(0.486127,  0.0567095)
(0.488533,  0.0665145)
(0.49094,  0.080876)
(0.493347,  0.0856463)
(0.495753,  0.0926127)
(0.49816,  0.0820555)
(0.500566,  0.0691941)
(0.502973,  0.0600165)
(0.505379,  0.0461318)
(0.507786,  0.0383048)
(0.510193,  0.0392195)
(0.512599,  0.0363521)
(0.515006,  0.0207838)
(0.517412,  0.000704478)
(0.519819,  0.00269507)
(0.522225,   -0.010439)
(0.524632,   -0.0259677)
(0.527039,   -0.00372898)
(0.529445,  0.0135148)
(0.531852,  0.0495363)
(0.534258,  0.0515501)
(0.536665,  0.0699885)
(0.539071,  0.0865144)
(0.541478,  0.0938662)
(0.543884,  0.118052)
(0.546291,  0.131915)
(0.548698,  0.127248)
(0.551104,  0.108668)
(0.553511,  0.0790158)
(0.555917,  0.0709626)
(0.558324,  0.0122231)
(0.56073,   -0.0367777)
(0.563137,   -0.0652372)
(0.565544,   -0.0618316)
(0.56795,   -0.0636769)
(0.570357,   -0.050715)
(0.572763,   -0.0235303)
(0.57517,   -0.00580707)
(0.577576,  0.0370316)
(0.579983,  0.045244)
(0.58239,  0.0665355)
(0.584796,  0.0860701)
(0.587203,  0.0861025)
(0.589609,  0.0946878)
(0.592016,  0.0963555)
(0.594422,  0.0858185)
(0.596829,  0.0553487)
(0.599236,  0.0353588)
(0.601642,  0.0106119)
(0.604049,   -0.00243727)
(0.606455,   -0.010779)
(0.608862,   -0.00924651)
(0.611268,   -0.0148658)
(0.613675,   -0.0199869)
(0.616082,   -0.0156224)
(0.618488,  0.0200595)
(0.620895,  0.0344298)
(0.623301,  0.05142)
(0.625708,  0.0551441)
(0.628114,  0.0880235)
(0.630521,  0.0993272)
(0.632927,  0.105298)
(0.635334,  0.0932625)
(0.637741,  0.0532226)
(0.640147,  0.024029)
(0.642554,  0.0221356)
(0.64496,  0.00489831)
(0.647367,  0.0130726)
(0.649774,  0.0214122)
(0.65218,  0.0282809)
(0.654587,  0.0363033)
(0.656993,  0.0454226)
(0.6594,  0.0657559)
(0.661806,  0.0910583)
(0.664213,  0.0874268)
(0.666619,  0.0745381)
(0.669026,  0.0657367)
(0.671433,  0.0513941)
(0.673839,  0.0483899)
(0.676246,  0.0355975)
(0.678652,  0.0232142)
(0.681059,   -0.0132616)
(0.683465,   -0.0248179)
(0.685872,   -0.0198266)
(0.688279,   -0.00845161)
(0.690685,  0.013001)
(0.693092,  0.0389715)
(0.695498,  0.0581762)
(0.697905,  0.0612299)
(0.700311,  0.0812873)
(0.702718,  0.0944959)
(0.705125,  0.0927052)
(0.707531,  0.0711272)
(0.709938,  0.044376)
(0.712344,  0.0361438)
(0.714751,   -0.00124347)
(0.717157,   -0.0324437)
(0.719564,   -0.0440278)
(0.72197,   -0.0505339)
(0.724377,   -0.0413028)
(0.726784,   -0.0234087)
(0.72919,   -0.00224635)
(0.731597,  0.0108195)
(0.734003,  0.0216667)
(0.73641,  0.0488513)
(0.738817,  0.0777903)
(0.741223,  0.123017)
(0.74363,  0.14262)
(0.746036,  0.152391)
(0.748443,  0.173484)
(0.750849,  0.182812)
(0.753256,  0.165078)
(0.755662,  0.115616)
(0.758069,  0.0718499)
(0.760476,  0.0459223)
(0.762882,  0.0360821)
(0.765289,  0.0239113)
(0.767695,  0.00731705)
(0.770102,   -0.000835327)
(0.772509,   -0.00224761)
(0.774915,  0.00724536)
(0.777322,  0.0102015)
(0.779728,  0.017716)
(0.782135,  0.0277539)
(0.784541,  0.056767)
(0.786948,  0.0837181)
(0.789355,  0.101862)
(0.791761,  0.118067)
(0.794168,  0.113071)
(0.796574,  0.120077)
(0.798981,  0.115911)
(0.801387,  0.0884612)
(0.803794,  0.078366)
(0.8062,  0.064208)
(0.808607,   -0.0295754)
(0.811014,   -0.0535126)
(0.81342,   -0.055097)
(0.815827,   -0.0509662)
(0.818233,   -0.0391897)
(0.82064,   -0.024296)
(0.823046,   -0.0100099)
(0.825453,  0.0393621)
(0.82786,  0.0442727)
(0.830266,  0.044743)
(0.832673,  0.0484824)
(0.835079,  0.0530293)
(0.837486,  0.0536903)
(0.839892,  0.0631323)
(0.842299,  0.0526958)
(0.844706,  0.0377289)
(0.847112,  0.0205391)
(0.849519,  0.00269782)
(0.851925,   -0.00171824)
(0.854332,  0.00498205)
(0.856738,  0.0157375)
(0.859145,  0.0419604)
(0.861552,  0.0583455)
(0.863958,  0.0907787)
(0.866365,  0.115175)
(0.868771,  0.118823)
(0.871178,  0.0949858)
(0.873584,  0.0835156)
(0.875991,  0.066365)
(0.878397,  0.0421466)
(0.880804,   -0.00453337)
(0.883211,   -0.0335281)
(0.885617,   -0.0348468)
(0.888024,   -0.0270191)
(0.89043,   -0.0326012)
(0.892837,   -0.0360297)
(0.895243,   -0.0245439)
(0.89765,  0.00629744)
(0.900057,  0.0414156)
(0.902463,  0.0549553)
(0.90487,  0.0521554)
(0.907276,  0.0540298)
(0.909683,  0.0574207)
(0.912089,  0.0545547)
(0.914496,  0.0589206)
(0.916903,  0.0428452)
(0.919309,  0.030027)
(0.921716,  0.0231051)
(0.924122,  0.0128042)
(0.926529,  0.00917297)
(0.928935,  0.039652)
(0.931342,  0.0448427)
(0.933749,  0.0506234)
(0.936155,  0.050767)
(0.938562,  0.0485208)
(0.940968,  0.0494609)
(0.943375,  0.0463837)
(0.945781,  0.0435835)
(0.948188,  0.0393321)
(0.950595,  0.0345339)
(0.953001,  0.0282009)
(0.955408,  0.0202142)
(0.957814,  0.0132545)
(0.960221,  0.00720083)
(0.962627,   -0.00477066)
(0.965034,   -0.0140744)
(0.967441,   -0.00934388)
(0.969847,   -0.00061305)
(0.972254,  0.0210606)
(0.97466,  0.030775)
(0.977067,  0.0396249)
(0.979473,  0.0557188)
(0.98188,  0.0612706)
(0.984286,  0.0596326)
(0.986693,  0.0581055)
(0.9891,  0.0470628)
(0.991506,  0.0415611)
(0.993913,  0.0447129)
(0.996319,  0.0316299)
(0.998726,  0.0256316)
(1.0,   -0)
};

==> exp_plots/payload_comparison/y_tmdc_no_fill.tex <==
\addplot[
    fill=none,draw = clr3,opacity=1.0,
    line width= \linew pt
    ]
 %%
coordinates {
(0,   -0)
(0,   -0.00631241)
(0.00240215,   0.00121764)
(0.0048043,   0.015806)
(0.00720644,   0.0234479)
(0.00960859,   0.0468983)
(0.0120107,   0.0720619)
(0.0144129,   0.0893672)
(0.016815,   0.0793187)
(0.0192172,   0.0784667)
(0.0216193,   0.068568)
(0.0240215,   0.0669021)
(0.0264236,   0.0491458)
(0.0288258,   0.0386657)
(0.0312279,   0.0543447)
(0.0336301,   0.0552464)
(0.0360322,   0.0435512)
(0.0384344,   0.0287776)
(0.0408365,   0.030596)
(0.0432387,   0.0390409)
(0.0456408,   0.0400664)
(0.048043,   0.0373032)
(0.0504451,   0.0445768)
(0.0528472,   0.0508481)
(0.0552494,   0.0639583)
(0.0576515,   0.0636996)
(0.0600537,   0.0691584)
(0.0624558,   0.0716546)
(0.064858,   0.0714057)
(0.0672601,   0.0698779)
(0.0696623,   0.0578218)
(0.0720644,   0.0488382)
(0.0744666,   0.0246037)
(0.0768687,   0.00621997)
(0.0792709,   0.00245471)
(0.081673,   0.00221569)
(0.0840752,   -0.000718464)
(0.0864773,   -0.00166905)
(0.0888795,   0.0020951)
(0.0912816,   0.0132353)
(0.0936838,   0.0201955)
(0.0960859,   0.0320009)
(0.0984881,   0.0332879)
(0.10089,   0.0359759)
(0.103292,   0.0413928)
(0.105694,   0.0435221)
(0.108097,   0.050665)
(0.110499,   0.0480149)
(0.112901,   0.0441181)
(0.115303,   0.0459717)
(0.117705,   0.0422672)
(0.120107,   0.0308536)
(0.12251,   0.0132885)
(0.124912,   0.00928486)
(0.127314,   0.00899284)
(0.129716,   0.00130557)
(0.132118,   0.00660331)
(0.13452,   0.011162)
(0.136922,   0.0171333)
(0.139325,   0.0375324)
(0.141727,   0.0393943)
(0.144129,   0.0413439)
(0.146531,   0.0386092)
(0.148933,   0.0446992)
(0.151335,   0.0450244)
(0.153737,   0.0437711)
(0.15614,   0.0532301)
(0.158542,   0.0664098)
(0.160944,   0.0722513)
(0.163346,   0.0783626)
(0.165748,   0.111107)
(0.16815,   0.121311)
(0.170552,   0.122044)
(0.172955,   0.118946)
(0.175357,   0.109136)
(0.177759,   0.0906902)
(0.180161,   0.0885176)
(0.182563,   0.061577)
(0.184965,   0.043402)
(0.187368,   0.0459333)
(0.18977,   0.0525787)
(0.192172,   0.0542803)
(0.194574,   0.0527377)
(0.196976,   0.065598)
(0.199378,   0.0898553)
(0.20178,   0.101769)
(0.204183,   0.108931)
(0.206585,   0.109036)
(0.208987,   0.10735)
(0.211389,   0.117826)
(0.213791,   0.118722)
(0.216193,   0.0969686)
(0.218595,   0.0840736)
(0.220998,   0.065397)
(0.2234,   0.0466898)
(0.225802,   0.0257251)
(0.228204,   -0.00890586)
(0.230606,   -0.0238833)
(0.233008,   -0.0212833)
(0.23541,   0.0126043)
(0.237813,   0.0516904)
(0.240215,   0.0789398)
(0.242617,   0.0950545)
(0.245019,   0.105763)
(0.247421,   0.12898)
(0.249823,   0.141006)
(0.252225,   0.144763)
(0.254628,   0.137832)
(0.25703,   0.133784)
(0.259432,   0.133277)
(0.261834,   0.0861276)
(0.264236,   0.0652769)
(0.266638,   0.0351563)
(0.269041,   0.000710947)
(0.271443,   -0.0223602)
(0.273845,   -0.0267558)
(0.276247,   -0.0137322)
(0.278649,   -0.0103888)
(0.281051,   -0.002956)
(0.283453,   0.0161813)
(0.285856,   0.0239264)
(0.288258,   0.0436134)
(0.29066,   0.05965)
(0.293062,   0.0523105)
(0.295464,   0.0651667)
(0.297866,   0.0758072)
(0.300268,   0.104073)
(0.302671,   0.123041)
(0.305073,   0.126955)
(0.307475,   0.126018)
(0.309877,   0.132015)
(0.312279,   0.129479)
(0.314681,   0.117107)
(0.317084,   0.0929575)
(0.319486,   0.0679904)
(0.321888,   0.0475429)
(0.32429,   0.0138099)
(0.326692,   -0.0181407)
(0.329094,   -0.0381693)
(0.331496,   -0.0391077)
(0.333899,   -0.0339978)
(0.336301,   -0.0144733)
(0.338703,   0.0217102)
(0.341105,   0.0450656)
(0.343507,   0.0737618)
(0.345909,   0.0958586)
(0.348311,   0.123268)
(0.350714,   0.157825)
(0.353116,   0.158985)
(0.355518,   0.152712)
(0.35792,   0.141089)
(0.360322,   0.123593)
(0.362724,   0.0922681)
(0.365126,   0.0740064)
(0.367529,   0.0444761)
(0.369931,   0.0319096)
(0.372333,   0.0177358)
(0.374735,   -0.00440454)
(0.377137,   -0.0136609)
(0.379539,   -0.00746632)
(0.381941,   0.00700482)
(0.384344,   0.0131454)
(0.386746,   0.0250854)
(0.389148,   0.0388758)
(0.39155,   0.0485327)
(0.393952,   0.0551936)
(0.396354,   0.0747437)
(0.398757,   0.0899217)
(0.401159,   0.0929827)
(0.403561,   0.1)
(0.405963,   0.098904)
(0.408365,   0.0762874)
(0.410767,   0.0405046)
(0.413169,   0.0307971)
(0.415572,   0.0113526)
(0.417974,   -0.00901133)
(0.420376,   -0.0151865)
(0.422778,   -0.00143829)
(0.42518,   0.00624036)
(0.427582,   0.017371)
(0.429984,   0.0231859)
(0.432387,   0.0427198)
(0.434789,   0.0688042)
(0.437191,   0.0751151)
(0.439593,   0.0840542)
(0.441995,   0.0999649)
(0.444397,   0.101464)
(0.446799,   0.0849421)
(0.449202,   0.0801646)
(0.451604,   0.083008)
(0.454006,   0.0755344)
(0.456408,   0.0476711)
(0.45881,   0.0202789)
(0.461212,   -0.0120736)
(0.463615,   -0.0322603)
(0.466017,   -0.0437634)
(0.468419,   -0.043012)
(0.470821,   -0.0318389)
(0.473223,   0.0115439)
(0.475625,   0.0399419)
(0.478027,   0.0734623)
(0.48043,   0.0951933)
(0.482832,   0.0986556)
(0.485234,   0.0980901)
(0.487636,   0.0925511)
(0.490038,   0.0901159)
(0.49244,   0.0871711)
(0.494842,   0.0914398)
(0.497245,   0.104096)
(0.499647,   0.0948422)
(0.502049,   0.0827215)
(0.504451,   0.0846168)
(0.506853,   0.0821159)
(0.509255,   0.0473026)
(0.511657,   0.0149575)
(0.51406,   0.00174165)
(0.516462,   -0.0162707)
(0.518864,   -0.00301641)
(0.521266,   0.00715501)
(0.523668,   0.0185488)
(0.52607,   0.0383754)
(0.528472,   0.0512396)
(0.530875,   0.0712263)
(0.533277,   0.110172)
(0.535679,   0.114918)
(0.538081,   0.132354)
(0.540483,   0.144811)
(0.542885,   0.150565)
(0.545288,   0.135816)
(0.54769,   0.114874)
(0.550092,   0.0846166)
(0.552494,   0.0652958)
(0.554896,   0.0474618)
(0.557298,   0.0414443)
(0.5597,   0.0455626)
(0.562103,   0.0355601)
(0.564505,   0.0235244)
(0.566907,   0.0196578)
(0.569309,   0.0131968)
(0.571711,   0.0137011)
(0.574113,   0.0174854)
(0.576515,   0.0197894)
(0.578918,   0.0174163)
(0.58132,   0.025958)
(0.583722,   0.0332343)
(0.586124,   0.0531897)
(0.588526,   0.0670967)
(0.590928,   0.0779935)
(0.593331,   0.083203)
(0.595733,   0.0853858)
(0.598135,   0.0961063)
(0.600537,   0.0848875)
(0.602939,   0.0734368)
(0.605341,   0.045528)
(0.607743,   0.0185782)
(0.610146,   0.00798386)
(0.612548,   0.00802904)
(0.61495,   0.0103981)
(0.617352,   0.0115155)
(0.619754,   0.00337394)
(0.622156,   0.00691593)
(0.624558,   0.00545754)
(0.626961,   0.0167132)
(0.629363,   0.0370474)
(0.631765,   0.0365399)
(0.634167,   0.0428238)
(0.636569,   0.0580198)
(0.638971,   0.0577619)
(0.641373,   0.059753)
(0.643776,   0.0729296)
(0.646178,   0.0817834)
(0.64858,   0.103883)
(0.650982,   0.120432)
(0.653384,   0.11829)
(0.655786,   0.124306)
(0.658189,   0.124638)
(0.660591,   0.127967)
(0.662993,   0.0890557)
(0.665395,   0.0619642)
(0.667797,   0.0550043)
(0.670199,   0.0494754)
(0.672601,   0.0432423)
(0.675004,   0.0413691)
(0.677406,   0.0368747)
(0.679808,   0.0397667)
(0.68221,   0.0538378)
(0.684612,   0.0669046)
(0.687014,   0.07226)
(0.689416,   0.0786436)
(0.691819,   0.084086)
(0.694221,   0.0850133)
(0.696623,   0.0789186)
(0.699025,   0.0745535)
(0.701427,   0.0597227)
(0.703829,   0.050835)
(0.706231,   0.0224182)
(0.708634,   -0.00518126)
(0.711036,   -0.0294073)
(0.713438,   -0.0396916)
(0.71584,   -0.0413858)
(0.718242,   -0.0372989)
(0.720644,   -0.0217282)
(0.723046,   0.00597499)
(0.725449,   0.0561255)
(0.727851,   0.0665984)
(0.730253,   0.0890864)
(0.732655,   0.11703)
(0.735057,   0.130008)
(0.737459,   0.152652)
(0.739861,   0.165404)
(0.742264,   0.155719)
(0.744666,   0.142679)
(0.747068,   0.113827)
(0.74947,   0.10951)
(0.751872,   0.083653)
(0.754274,   0.0628463)
(0.756677,   0.0527938)
(0.759079,   0.0317545)
(0.761481,   0.0289365)
(0.763883,   0.0445308)
(0.766285,   0.0577586)
(0.768687,   0.0910643)
(0.771089,   0.112873)
(0.773492,   0.134718)
(0.775894,   0.148635)
(0.778296,   0.1519)
(0.780698,   0.131885)
(0.7831,   0.0909401)
(0.785502,   0.0355724)
(0.787905,   0.0207237)
(0.790307,   0.0145217)
(0.792709,   0.0127319)
(0.795111,   0.00874612)
(0.797513,   -0.0134794)
(0.799915,   -0.0114799)
(0.802317,   0.0141754)
(0.804719,   0.0452817)
(0.807122,   0.05909)
(0.809524,   0.112292)
(0.811926,   0.141401)
(0.814328,   0.157902)
(0.81673,   0.164892)
(0.819132,   0.171237)
(0.821535,   0.150371)
(0.823937,   0.112591)
(0.826339,   0.094329)
(0.828741,   0.0786449)
(0.831143,   0.0573262)
(0.833545,   0.0556932)
(0.835947,   0.0302484)
(0.83835,   0.0147359)
(0.840752,   -0.00657663)
(0.843154,   -0.0292936)
(0.845556,   -0.0313141)
(0.847958,   -0.0169153)
(0.85036,   0.00369827)
(0.852762,   0.0240366)
(0.855165,   0.0506914)
(0.857567,   0.0607273)
(0.859969,   0.0602752)
(0.862371,   0.0762163)
(0.864773,   0.0964222)
(0.867175,   0.0961095)
(0.869577,   0.0933061)
(0.87198,   0.109567)
(0.874382,   0.110014)
(0.876784,   0.105539)
(0.879186,   0.0999149)
(0.881588,   0.0745791)
(0.88399,   0.0303491)
(0.886393,   -0.0292836)
(0.888795,   -0.0499787)
(0.891197,   -0.0593061)
(0.893599,   -0.0495399)
(0.896001,   -0.0194534)
(0.898403,   -0.00517331)
(0.900805,   0.0128713)
(0.903208,   0.0413699)
(0.90561,   0.0530826)
(0.908012,   0.0418887)
(0.910414,   0.047683)
(0.912816,   0.0602021)
(0.915218,   0.0576297)
(0.91762,   0.048742)
(0.920023,   0.0187425)
(0.922425,   -0.0073385)
(0.924827,   -0.010667)
(0.927229,   -0.0122226)
(0.929631,   -0.00969235)
(0.932033,   -0.000707611)
(0.934435,   0.0172688)
(0.936838,   0.042532)
(0.93924,   0.0613045)
(0.941642,   0.0691901)
(0.944044,   0.0802119)
(0.946446,   0.0770375)
(0.948848,   0.0788135)
(0.951251,   0.0681453)
(0.953653,   0.0531489)
(0.956055,   0.0437335)
(0.958457,   0.0279006)
(0.960859,   0.0176004)
(0.963261,   0.00940637)
(0.965663,   -0.00609706)
(0.968066,   -0.015886)
(0.970468,   -0.0241541)
(0.97287,   -0.013921)
(0.975272,   0.012799)
(0.977674,   0.0272691)
(0.980076,   0.0672016)
(0.982478,   0.0616688)
(0.984881,   0.0629332)
(0.987283,   0.0661558)
(0.989685,   0.0573783)
(0.992087,   0.0459832)
(0.994489,   0.0316104)
(0.996891,   0.0194988)
(0.999293,   0.00866625)
(1.0,   -0)
};

==> exp_plots/payload_comparison/z_da_no_fill.tex <==
\addplot[
    fill=none,draw = clr1,opacity=1.0,
    line width= \linew pt
    ]
 %%
coordinates {
(0,   -0)
(0,   -0.462634)
(0.00240249,   -0.521722)
(0.00480497,   -0.561393)
(0.00720746,   -0.58884)
(0.00960995,   -0.586814)
(0.0120124,   -0.589951)
(0.0144149,   -0.579818)
(0.0168174,   -0.532726)
(0.0192199,   -0.505197)
(0.0216224,   -0.448339)
(0.0240249,   -0.404651)
(0.0264274,   -0.353556)
(0.0288298,   -0.326005)
(0.0312323,   -0.305735)
(0.0336348,   -0.276146)
(0.0360373,   -0.225858)
(0.0384398,   -0.224995)
(0.0408423,   -0.242608)
(0.0432448,   -0.241987)
(0.0456473,   -0.242808)
(0.0480497,   -0.257748)
(0.0504522,   -0.291078)
(0.0528547,   -0.284491)
(0.0552572,   -0.289483)
(0.0576597,   -0.305264)
(0.0600622,   -0.310221)
(0.0624647,   -0.327032)
(0.0648672,   -0.362742)
(0.0672696,   -0.370519)
(0.0696721,   -0.389115)
(0.0720746,   -0.41472)
(0.0744771,   -0.439034)
(0.0768796,   -0.466491)
(0.0792821,   -0.481764)
(0.0816846,   -0.481341)
(0.0840871,   -0.507928)
(0.0864895,   -0.545503)
(0.088892,   -0.582368)
(0.0912945,   -0.580057)
(0.093697,   -0.585754)
(0.0960995,   -0.585091)
(0.098502,   -0.608687)
(0.100904,   -0.626006)
(0.103307,   -0.611055)
(0.105709,   -0.639509)
(0.108112,   -0.63542)
(0.110514,   -0.627803)
(0.112917,   -0.627217)
(0.115319,   -0.62524)
(0.117722,   -0.638534)
(0.120124,   -0.630838)
(0.122527,   -0.628306)
(0.124929,   -0.574597)
(0.127332,   -0.551536)
(0.129734,   -0.540667)
(0.132137,   -0.475029)
(0.134539,   -0.44975)
(0.136942,   -0.437562)
(0.139344,   -0.437057)
(0.141747,   -0.438712)
(0.144149,   -0.452094)
(0.146552,   -0.47608)
(0.148954,   -0.49972)
(0.151357,   -0.496779)
(0.153759,   -0.468)
(0.156162,   -0.438451)
(0.158564,   -0.425446)
(0.160967,   -0.370219)
(0.163369,   -0.336139)
(0.165772,   -0.25966)
(0.168174,   -0.255167)
(0.170577,   -0.257515)
(0.172979,   -0.259668)
(0.175382,   -0.240196)
(0.177784,   -0.250468)
(0.180187,   -0.277964)
(0.182589,   -0.308212)
(0.184992,   -0.331825)
(0.187394,   -0.350547)
(0.189796,   -0.38089)
(0.192199,   -0.384858)
(0.194601,   -0.405511)
(0.197004,   -0.404726)
(0.199406,   -0.405523)
(0.201809,   -0.396669)
(0.204211,   -0.352872)
(0.206614,   -0.333972)
(0.209016,   -0.319385)
(0.211419,   -0.292825)
(0.213821,   -0.277685)
(0.216224,   -0.287033)
(0.218626,   -0.317784)
(0.221029,   -0.33032)
(0.223431,   -0.320358)
(0.225834,   -0.333002)
(0.228236,   -0.35576)
(0.230639,   -0.382855)
(0.233041,   -0.389025)
(0.235444,   -0.401503)
(0.237846,   -0.404777)
(0.240249,   -0.41317)
(0.242651,   -0.4403)
(0.245054,   -0.4882)
(0.247456,   -0.543873)
(0.249859,   -0.557553)
(0.252261,   -0.575432)
(0.254664,   -0.642439)
(0.257066,   -0.638989)
(0.259469,   -0.631428)
(0.261871,   -0.706601)
(0.264274,   -0.774487)
(0.266676,   -0.799858)
(0.269079,   -0.802302)
(0.271481,   -0.772617)
(0.273884,   -0.7579)
(0.276286,   -0.723048)
(0.278689,   -0.712814)
(0.281091,   -0.711057)
(0.283493,   -0.674696)
(0.285896,   -0.631626)
(0.288298,   -0.618918)
(0.290701,   -0.609975)
(0.293103,   -0.602476)
(0.295506,   -0.579173)
(0.297908,   -0.55919)
(0.300311,   -0.545119)
(0.302713,   -0.541456)
(0.305116,   -0.539113)
(0.307518,   -0.527962)
(0.309921,   -0.54996)
(0.312323,   -0.570764)
(0.314726,   -0.563357)
(0.317128,   -0.558468)
(0.319531,   -0.572201)
(0.321933,   -0.60159)
(0.324336,   -0.649819)
(0.326738,   -0.643029)
(0.329141,   -0.626464)
(0.331543,   -0.611301)
(0.333946,   -0.586294)
(0.336348,   -0.568806)
(0.338751,   -0.569866)
(0.341153,   -0.572349)
(0.343556,   -0.574933)
(0.345958,   -0.558214)
(0.348361,   -0.495725)
(0.350763,   -0.438587)
(0.353166,   -0.350344)
(0.355568,   -0.293901)
(0.357971,   -0.270964)
(0.360373,   -0.256637)
(0.362776,   -0.256338)
(0.365178,   -0.268028)
(0.367581,   -0.300745)
(0.369983,   -0.33137)
(0.372386,   -0.396532)
(0.374788,   -0.457887)
(0.37719,   -0.487816)
(0.379593,   -0.495834)
(0.381995,   -0.524284)
(0.384398,   -0.534088)
(0.3868,   -0.519377)
(0.389203,   -0.52227)
(0.391605,   -0.519835)
(0.394008,   -0.49386)
(0.39641,   -0.47345)
(0.398813,   -0.454784)
(0.401215,   -0.434712)
(0.403618,   -0.418589)
(0.40602,   -0.37815)
(0.408423,   -0.376671)
(0.410825,   -0.374079)
(0.413228,   -0.362878)
(0.41563,   -0.375119)
(0.418033,   -0.389715)
(0.420435,   -0.411935)
(0.422838,   -0.459224)
(0.42524,   -0.507089)
(0.427643,   -0.524058)
(0.430045,   -0.575438)
(0.432448,   -0.586159)
(0.43485,   -0.589764)
(0.437253,   -0.615418)
(0.439655,   -0.626216)
(0.442058,   -0.647433)
(0.44446,   -0.661036)
(0.446863,   -0.665589)
(0.449265,   -0.650179)
(0.451668,   -0.639864)
(0.45407,   -0.611853)
(0.456473,   -0.563207)
(0.458875,   -0.49538)
(0.461278,   -0.452335)
(0.46368,   -0.438271)
(0.466083,   -0.42956)
(0.468485,   -0.439011)
(0.470887,   -0.413561)
(0.47329,   -0.414218)
(0.475692,   -0.412371)
(0.478095,   -0.405267)
(0.480497,   -0.382181)
(0.4829,   -0.366084)
(0.485302,   -0.358565)
(0.487705,   -0.346783)
(0.490107,   -0.340209)
(0.49251,   -0.33504)
(0.494912,   -0.358155)
(0.497315,   -0.366948)
(0.499717,   -0.381766)
(0.50212,   -0.388394)
(0.504522,   -0.393004)
(0.506925,   -0.396606)
(0.509327,   -0.389764)
(0.51173,   -0.366042)
(0.514132,   -0.331025)
(0.516535,   -0.295869)
(0.518937,   -0.261681)
(0.52134,   -0.234832)
(0.523742,   -0.228212)
(0.526145,   -0.22855)
(0.528547,   -0.252154)
(0.53095,   -0.298712)
(0.533352,   -0.331483)
(0.535755,   -0.336382)
(0.538157,   -0.350741)
(0.54056,   -0.353977)
(0.542962,   -0.34206)
(0.545365,   -0.351815)
(0.547767,   -0.36151)
(0.55017,   -0.369644)
(0.552572,   -0.367093)
(0.554975,   -0.367994)
(0.557377,   -0.369364)
(0.55978,   -0.373434)
(0.562182,   -0.400696)
(0.564584,   -0.409939)
(0.566987,   -0.432088)
(0.569389,   -0.444683)
(0.571792,   -0.493219)
(0.574194,   -0.520928)
(0.576597,   -0.508813)
(0.578999,   -0.513687)
(0.581402,   -0.557057)
(0.583804,   -0.607808)
(0.586207,   -0.633939)
(0.588609,   -0.657756)
(0.591012,   -0.70745)
(0.593414,   -0.721646)
(0.595817,   -0.743919)
(0.598219,   -0.762868)
(0.600622,   -0.769018)
(0.603024,   -0.786402)
(0.605427,   -0.807831)
(0.607829,   -0.839384)
(0.610232,   -0.849538)
(0.612634,   -0.845911)
(0.615037,   -0.843949)
(0.617439,   -0.817642)
(0.619842,   -0.808665)
(0.622244,   -0.781685)
(0.624647,   -0.649691)
(0.627049,   -0.605715)
(0.629452,   -0.52297)
(0.631854,   -0.48251)
(0.634257,   -0.453188)
(0.636659,   -0.431958)
(0.639062,   -0.420886)
(0.641464,   -0.402855)
(0.643867,   -0.408535)
(0.646269,   -0.391628)
(0.648672,   -0.415425)
(0.651074,   -0.427876)
(0.653477,   -0.438713)
(0.655879,   -0.477571)
(0.658282,   -0.520523)
(0.660684,   -0.561372)
(0.663086,   -0.584986)
(0.665489,   -0.58041)
(0.667891,   -0.574787)
(0.670294,   -0.566035)
(0.672696,   -0.55391)
(0.675099,   -0.568805)
(0.677501,   -0.597735)
(0.679904,   -0.613663)
(0.682306,   -0.640322)
(0.684709,   -0.659321)
(0.687111,   -0.67913)
(0.689514,   -0.681319)
(0.691916,   -0.663768)
(0.694319,   -0.633999)
(0.696721,   -0.598581)
(0.699124,   -0.519037)
(0.701526,   -0.500554)
(0.703929,   -0.487377)
(0.706331,   -0.457404)
(0.708734,   -0.455741)
(0.711136,   -0.4742)
(0.713539,   -0.474848)
(0.715941,   -0.483615)
(0.718344,   -0.491185)
(0.720746,   -0.501047)
(0.723149,   -0.510352)
(0.725551,   -0.548956)
(0.727954,   -0.576637)
(0.730356,   -0.582478)
(0.732759,   -0.619234)
(0.735161,   -0.663465)
(0.737564,   -0.69303)
(0.739966,   -0.709505)
(0.742369,   -0.703773)
(0.744771,   -0.663096)
(0.747173,   -0.646018)
(0.749576,   -0.571642)
(0.751978,   -0.520899)
(0.754381,   -0.513147)
(0.756783,   -0.496698)
(0.759186,   -0.505758)
(0.761588,   -0.504361)
(0.763991,   -0.495001)
(0.766393,   -0.494152)
(0.768796,   -0.478567)
(0.771198,   -0.468257)
(0.773601,   -0.448136)
(0.776003,   -0.436344)
(0.778406,   -0.431921)
(0.780808,   -0.440166)
(0.783211,   -0.460208)
(0.785613,   -0.459889)
(0.788016,   -0.479363)
(0.790418,   -0.485302)
(0.792821,   -0.514378)
(0.795223,   -0.520289)
(0.797626,   -0.576148)
(0.800028,   -0.581979)
(0.802431,   -0.58981)
(0.804833,   -0.624773)
(0.807236,   -0.651263)
(0.809638,   -0.645292)
(0.812041,   -0.625838)
(0.814443,   -0.621606)
(0.816846,   -0.601322)
(0.819248,   -0.594022)
(0.821651,   -0.577485)
(0.824053,   -0.554776)
(0.826456,   -0.530805)
(0.828858,   -0.534591)
(0.831261,   -0.54447)
(0.833663,   -0.548174)
(0.836066,   -0.517703)
(0.838468,   -0.466773)
(0.840871,   -0.439219)
(0.843273,   -0.415901)
(0.845675,   -0.388642)
(0.848078,   -0.385194)
(0.85048,   -0.3643)
(0.852883,   -0.351572)
(0.855285,   -0.374937)
(0.857688,   -0.408066)
(0.86009,   -0.437911)
(0.862493,   -0.452112)
(0.864895,   -0.499031)
(0.867298,   -0.528557)
(0.8697,   -0.543814)
(0.872103,   -0.560489)
(0.874505,   -0.55308)
(0.876908,   -0.560265)
(0.87931,   -0.578319)
(0.881713,   -0.607464)
(0.884115,   -0.57841)
(0.886518,   -0.568354)
(0.88892,   -0.514384)
(0.891323,   -0.474025)
(0.893725,   -0.470642)
(0.896128,   -0.467248)
(0.89853,   -0.487677)
(0.900933,   -0.493314)
(0.903335,   -0.487964)
(0.905738,   -0.481846)
(0.90814,   -0.470103)
(0.910543,   -0.463996)
(0.912945,   -0.460843)
(0.915348,   -0.460261)
(0.91775,   -0.445036)
(0.920153,   -0.418608)
(0.922555,   -0.404645)
(0.924958,   -0.406249)
(0.92736,   -0.404985)
(0.929763,   -0.41545)
(0.932165,   -0.418707)
(0.934568,   -0.423159)
(0.93697,   -0.434496)
(0.939372,   -0.448811)
(0.941775,   -0.46991)
(0.944178,   -0.458851)
(0.94658,   -0.476888)
(0.948982,   -0.498713)
(0.951385,   -0.5185)
(0.953787,   -0.548414)
(0.95619,   -0.578606)
(0.958592,   -0.598478)
(0.960995,   -0.615)
(0.963397,   -0.626262)
(0.9658,   -0.631759)
(0.968202,   -0.632808)
(0.970605,   -0.638591)
(0.973007,   -0.636391)
(0.97541,   -0.627016)
(0.977812,   -0.608188)
(0.980215,   -0.601226)
(0.982617,   -0.592549)
(0.98502,   -0.574861)
(0.987422,   -0.541107)
(0.989825,   -0.511317)
(0.992227,   -0.51611)
(0.99463,   -0.531456)
(0.997032,   -0.555909)
(0.999435,   -0.564051)
(1.0,   -0)
};

==> exp_plots/payload_comparison/z_tmdc_gt_no_fill.tex <==
\addplot[
    fill=none,draw = clr2,opacity=1.0,
    line width= \linew pt
    ]
 %%
coordinates {
(0,   -0)
(0,   -0.476197)
(0.00240657,   -0.500143)
(0.00481314,   -0.5216)
(0.00721971,   -0.541578)
(0.00962627,   -0.549259)
(0.0120328,   -0.547228)
(0.0144394,   -0.53756)
(0.016846,   -0.525364)
(0.0192525,   -0.516962)
(0.0216591,   -0.508084)
(0.0240657,   -0.514915)
(0.0264723,   -0.523123)
(0.0288788,   -0.532924)
(0.0312854,   -0.514067)
(0.033692,   -0.505681)
(0.0360985,   -0.503023)
(0.0385051,   -0.503725)
(0.0409117,   -0.510306)
(0.0433182,   -0.504957)
(0.0457248,   -0.501042)
(0.0481314,   -0.509563)
(0.0505379,   -0.524928)
(0.0529445,   -0.520283)
(0.0553511,   -0.512384)
(0.0577576,   -0.510519)
(0.0601642,   -0.497125)
(0.0625708,   -0.491074)
(0.0649773,   -0.487226)
(0.0673839,   -0.48646)
(0.0697905,   -0.48073)
(0.0721971,   -0.4899)
(0.0746036,   -0.470928)
(0.0770102,   -0.460233)
(0.0794168,   -0.467719)
(0.0818233,   -0.487827)
(0.0842299,   -0.512211)
(0.0866365,   -0.513027)
(0.089043,   -0.525037)
(0.0914496,   -0.534417)
(0.0938562,   -0.530133)
(0.0962627,   -0.514855)
(0.0986693,   -0.515312)
(0.101076,   -0.508532)
(0.103482,   -0.50852)
(0.105889,   -0.513595)
(0.108296,   -0.483935)
(0.110702,   -0.476753)
(0.113109,   -0.479671)
(0.115515,   -0.492598)
(0.117922,   -0.491559)
(0.120328,   -0.484867)
(0.122735,   -0.474771)
(0.125142,   -0.46987)
(0.127548,   -0.514608)
(0.129955,   -0.533907)
(0.132361,   -0.532387)
(0.134768,   -0.512012)
(0.137174,   -0.506552)
(0.139581,   -0.492654)
(0.141988,   -0.489684)
(0.144394,   -0.486156)
(0.146801,   -0.485672)
(0.149207,   -0.487475)
(0.151614,   -0.47851)
(0.15402,   -0.455631)
(0.156427,   -0.440612)
(0.158834,   -0.434351)
(0.16124,   -0.452194)
(0.163647,   -0.472486)
(0.166053,   -0.477444)
(0.16846,   -0.480299)
(0.170866,   -0.461207)
(0.173273,   -0.465353)
(0.17568,   -0.481901)
(0.178086,   -0.458641)
(0.180493,   -0.461862)
(0.182899,   -0.47753)
(0.185306,   -0.485763)
(0.187712,   -0.477328)
(0.190119,   -0.478573)
(0.192525,   -0.484171)
(0.194932,   -0.490551)
(0.197339,   -0.502446)
(0.199745,   -0.502965)
(0.202152,   -0.504033)
(0.204558,   -0.491852)
(0.206965,   -0.48246)
(0.209371,   -0.497644)
(0.211778,   -0.514896)
(0.214185,   -0.50662)
(0.216591,   -0.497881)
(0.218998,   -0.480492)
(0.221404,   -0.486912)
(0.223811,   -0.484501)
(0.226217,   -0.478079)
(0.228624,   -0.492657)
(0.231031,   -0.497304)
(0.233437,   -0.501738)
(0.235844,   -0.49812)
(0.23825,   -0.485602)
(0.240657,   -0.509914)
(0.243063,   -0.525393)
(0.24547,   -0.523121)
(0.247877,   -0.510458)
(0.250283,   -0.513453)
(0.25269,   -0.504578)
(0.255096,   -0.496512)
(0.257503,   -0.491964)
(0.259909,   -0.48598)
(0.262316,   -0.486597)
(0.264723,   -0.492259)
(0.267129,   -0.493824)
(0.269536,   -0.485628)
(0.271942,   -0.49167)
(0.274349,   -0.496615)
(0.276755,   -0.502571)
(0.279162,   -0.501778)
(0.281568,   -0.506204)
(0.283975,   -0.520553)
(0.286382,   -0.527575)
(0.288788,   -0.51681)
(0.291195,   -0.525065)
(0.293601,   -0.525221)
(0.296008,   -0.519981)
(0.298414,   -0.512393)
(0.300821,   -0.511693)
(0.303228,   -0.508942)
(0.305634,   -0.502595)
(0.308041,   -0.509496)
(0.310447,   -0.51993)
(0.312854,   -0.53151)
(0.31526,   -0.543555)
(0.317667,   -0.530434)
(0.320074,   -0.527341)
(0.32248,   -0.523161)
(0.324887,   -0.510394)
(0.327293,   -0.485723)
(0.3297,   -0.475633)
(0.332106,   -0.470479)
(0.334513,   -0.483071)
(0.33692,   -0.489403)
(0.339326,   -0.512906)
(0.341733,   -0.506419)
(0.344139,   -0.50934)
(0.346546,   -0.496583)
(0.348952,   -0.51885)
(0.351359,   -0.538948)
(0.353766,   -0.541606)
(0.356172,   -0.53577)
(0.358579,   -0.552807)
(0.360985,   -0.544782)
(0.363392,   -0.534176)
(0.365798,   -0.518802)
(0.368205,   -0.488188)
(0.370612,   -0.465957)
(0.373018,   -0.462761)
(0.375425,   -0.475289)
(0.377831,   -0.486895)
(0.380238,   -0.498473)
(0.382644,   -0.506184)
(0.385051,   -0.501356)
(0.387458,   -0.461622)
(0.389864,   -0.52351)
(0.392271,   -0.532105)
(0.394677,   -0.520355)
(0.397084,   -0.496662)
(0.39949,   -0.464771)
(0.401897,   -0.447023)
(0.404304,   -0.468272)
(0.40671,   -0.483311)
(0.409117,   -0.4805)
(0.411523,   -0.467509)
(0.41393,   -0.471011)
(0.416336,   -0.496192)
(0.418743,   -0.517636)
(0.421149,   -0.522422)
(0.423556,   -0.532577)
(0.425963,   -0.538939)
(0.428369,   -0.521033)
(0.430776,   -0.502336)
(0.433182,   -0.50318)
(0.435589,   -0.495758)
(0.437995,   -0.485074)
(0.440402,   -0.479103)
(0.442809,   -0.440154)
(0.445215,   -0.415924)
(0.447622,   -0.424505)
(0.450028,   -0.459694)
(0.452435,   -0.493917)
(0.454841,   -0.502195)
(0.457248,   -0.523387)
(0.459655,   -0.526037)
(0.462061,   -0.546872)
(0.464468,   -0.557109)
(0.466874,   -0.542985)
(0.469281,   -0.547468)
(0.471687,   -0.527188)
(0.474094,   -0.533186)
(0.476501,   -0.534824)
(0.478907,   -0.53526)
(0.481314,   -0.532376)
(0.48372,   -0.492499)
(0.486127,   -0.502252)
(0.488533,   -0.492203)
(0.49094,   -0.501836)
(0.493347,   -0.488262)
(0.495753,   -0.480514)
(0.49816,   -0.473365)
(0.500566,   -0.452848)
(0.502973,   -0.477667)
(0.505379,   -0.501959)
(0.507786,   -0.516816)
(0.510193,   -0.533486)
(0.512599,   -0.543002)
(0.515006,   -0.540511)
(0.517412,   -0.547767)
(0.519819,   -0.557774)
(0.522225,   -0.512022)
(0.524632,   -0.490582)
(0.527039,   -0.455368)
(0.529445,   -0.432523)
(0.531852,   -0.424068)
(0.534258,   -0.440364)
(0.536665,   -0.45685)
(0.539071,   -0.480632)
(0.541478,   -0.481603)
(0.543884,   -0.495961)
(0.546291,   -0.494507)
(0.548698,   -0.493677)
(0.551104,   -0.48679)
(0.553511,   -0.482293)
(0.555917,   -0.497555)
(0.558324,   -0.50305)
(0.56073,   -0.477641)
(0.563137,   -0.458947)
(0.565544,   -0.467465)
(0.56795,   -0.472189)
(0.570357,   -0.458845)
(0.572763,   -0.462943)
(0.57517,   -0.46321)
(0.577576,   -0.46689)
(0.579983,   -0.468401)
(0.58239,   -0.485156)
(0.584796,   -0.510004)
(0.587203,   -0.505837)
(0.589609,   -0.496941)
(0.592016,   -0.49712)
(0.594422,   -0.498206)
(0.596829,   -0.501002)
(0.599236,   -0.494455)
(0.601642,   -0.498829)
(0.604049,   -0.518813)
(0.606455,   -0.534158)
(0.608862,   -0.52991)
(0.611268,   -0.523856)
(0.613675,   -0.511664)
(0.616082,   -0.49277)
(0.618488,   -0.481772)
(0.620895,   -0.47574)
(0.623301,   -0.462737)
(0.625708,   -0.469106)
(0.628114,   -0.490629)
(0.630521,   -0.504248)
(0.632927,   -0.537818)
(0.635334,   -0.54081)
(0.637741,   -0.54876)
(0.640147,   -0.521657)
(0.642554,   -0.519064)
(0.64496,   -0.496559)
(0.647367,   -0.481241)
(0.649774,   -0.483173)
(0.65218,   -0.501811)
(0.654587,   -0.493958)
(0.656993,   -0.482229)
(0.6594,   -0.494102)
(0.661806,   -0.491764)
(0.664213,   -0.488878)
(0.666619,   -0.499147)
(0.669026,   -0.49964)
(0.671433,   -0.491942)
(0.673839,   -0.465203)
(0.676246,   -0.468812)
(0.678652,   -0.464478)
(0.681059,   -0.465681)
(0.683465,   -0.468961)
(0.685872,   -0.495654)
(0.688279,   -0.521775)
(0.690685,   -0.545792)
(0.693092,   -0.573162)
(0.695498,   -0.585403)
(0.697905,   -0.582924)
(0.700311,   -0.551365)
(0.702718,   -0.535632)
(0.705125,   -0.53737)
(0.707531,   -0.502228)
(0.709938,   -0.487807)
(0.712344,   -0.487855)
(0.714751,   -0.449533)
(0.717157,   -0.41387)
(0.719564,   -0.426961)
(0.72197,   -0.435258)
(0.724377,   -0.452207)
(0.726784,   -0.476631)
(0.72919,   -0.50585)
(0.731597,   -0.502583)
(0.734003,   -0.497809)
(0.73641,   -0.486289)
(0.738817,   -0.487837)
(0.741223,   -0.506834)
(0.74363,   -0.521867)
(0.746036,   -0.539829)
(0.748443,   -0.557044)
(0.750849,   -0.563825)
(0.753256,   -0.546188)
(0.755662,   -0.509503)
(0.758069,   -0.495722)
(0.760476,   -0.516139)
(0.762882,   -0.550947)
(0.765289,   -0.560394)
(0.767695,   -0.545765)
(0.770102,   -0.529583)
(0.772509,   -0.539501)
(0.774915,   -0.550325)
(0.777322,   -0.54243)
(0.779728,   -0.533784)
(0.782135,   -0.526511)
(0.784541,   -0.531495)
(0.786948,   -0.521896)
(0.789355,   -0.532544)
(0.791761,   -0.542708)
(0.794168,   -0.549581)
(0.796574,   -0.574325)
(0.798981,   -0.569143)
(0.801387,   -0.56345)
(0.803794,   -0.561222)
(0.8062,   -0.547361)
(0.808607,   -0.50611)
(0.811014,   -0.511619)
(0.81342,   -0.527)
(0.815827,   -0.544492)
(0.818233,   -0.555764)
(0.82064,   -0.565036)
(0.823046,   -0.579322)
(0.825453,   -0.527173)
(0.82786,   -0.47877)
(0.830266,   -0.455958)
(0.832673,   -0.453716)
(0.835079,   -0.460715)
(0.837486,   -0.474851)
(0.839892,   -0.499761)
(0.842299,   -0.502929)
(0.844706,   -0.493441)
(0.847112,   -0.493073)
(0.849519,   -0.499895)
(0.851925,   -0.509398)
(0.854332,   -0.515359)
(0.856738,   -0.515124)
(0.859145,   -0.518924)
(0.861552,   -0.511261)
(0.863958,   -0.494644)
(0.866365,   -0.489082)
(0.868771,   -0.488981)
(0.871178,   -0.490367)
(0.873584,   -0.487433)
(0.875991,   -0.490599)
(0.878397,   -0.510797)
(0.880804,   -0.551258)
(0.883211,   -0.585578)
(0.885617,   -0.580782)
(0.888024,   -0.543091)
(0.89043,   -0.524138)
(0.892837,   -0.517738)
(0.895243,   -0.518418)
(0.89765,   -0.524196)
(0.900057,   -0.51356)
(0.902463,   -0.506796)
(0.90487,   -0.521758)
(0.907276,   -0.523466)
(0.909683,   -0.517169)
(0.912089,   -0.524997)
(0.914496,   -0.544162)
(0.916903,   -0.543694)
(0.919309,   -0.532579)
(0.921716,   -0.51655)
(0.924122,   -0.498941)
(0.926529,   -0.480551)
(0.928935,   -0.473586)
(0.931342,   -0.479316)
(0.933749,   -0.488199)
(0.936155,   -0.490092)
(0.938562,   -0.48009)
(0.940968,   -0.490074)
(0.943375,   -0.506151)
(0.945781,   -0.507015)
(0.948188,   -0.503483)
(0.950595,   -0.522219)
(0.953001,   -0.533666)
(0.955408,   -0.518427)
(0.957814,   -0.502945)
(0.960221,   -0.490322)
(0.962627,   -0.480047)
(0.965034,   -0.474557)
(0.967441,   -0.483942)
(0.969847,   -0.492202)
(0.972254,   -0.505027)
(0.97466,   -0.499811)
(0.977067,   -0.49161)
(0.979473,   -0.482011)
(0.98188,   -0.476665)
(0.984286,   -0.457178)
(0.986693,   -0.450496)
(0.9891,   -0.475135)
(0.991506,   -0.48232)
(0.993913,   -0.485452)
(0.996319,   -0.497434)
(0.998726,   -0.495064)
(1.0,   -0)
};

==> exp_plots/payload_comparison/z_tmdc_no_fill.tex <==
\addplot[
    fill=none,draw = clr3,opacity=1.0,
    line width= \linew pt
    ]
 %%
coordinates {
(0,   -0)
(0,   -0.462303)
(0.00240215,   -0.479234)
(0.0048043,   -0.49212)
(0.00720644,   -0.49829)
(0.00960859,   -0.55584)
(0.0120107,   -0.617712)
(0.0144129,   -0.611686)
(0.016815,   -0.530662)
(0.0192172,   -0.470486)
(0.0216193,   -0.448949)
(0.0240215,   -0.449903)
(0.0264236,   -0.476271)
(0.0288258,   -0.500469)
(0.0312279,   -0.539062)
(0.0336301,   -0.555987)
(0.0360322,   -0.534883)
(0.0384344,   -0.521748)
(0.0408365,   -0.51814)
(0.0432387,   -0.517291)
(0.0456408,   -0.512272)
(0.048043,   -0.494311)
(0.0504451,   -0.499717)
(0.0528472,   -0.496329)
(0.0552494,   -0.493408)
(0.0576515,   -0.492699)
(0.0600537,   -0.500267)
(0.0624558,   -0.498692)
(0.064858,   -0.506791)
(0.0672601,   -0.50862)
(0.0696623,   -0.502892)
(0.0720644,   -0.496263)
(0.0744666,   -0.490176)
(0.0768687,   -0.472758)
(0.0792709,   -0.472803)
(0.081673,   -0.482753)
(0.0840752,   -0.482415)
(0.0864773,   -0.488351)
(0.0888795,   -0.515177)
(0.0912816,   -0.54035)
(0.0936838,   -0.541751)
(0.0960859,   -0.538456)
(0.0984881,   -0.529042)
(0.10089,   -0.509563)
(0.103292,   -0.496979)
(0.105694,   -0.501745)
(0.108097,   -0.517773)
(0.110499,   -0.502987)
(0.112901,   -0.475049)
(0.115303,   -0.45115)
(0.117705,   -0.473782)
(0.120107,   -0.492641)
(0.12251,   -0.502484)
(0.124912,   -0.498008)
(0.127314,   -0.492161)
(0.129716,   -0.490666)
(0.132118,   -0.47292)
(0.13452,   -0.475651)
(0.136922,   -0.500655)
(0.139325,   -0.516589)
(0.141727,   -0.509293)
(0.144129,   -0.492653)
(0.146531,   -0.483468)
(0.148933,   -0.485236)
(0.151335,   -0.477739)
(0.153737,   -0.468599)
(0.15614,   -0.440279)
(0.158542,   -0.430216)
(0.160944,   -0.41175)
(0.163346,   -0.422527)
(0.165748,   -0.449689)
(0.16815,   -0.471487)
(0.170552,   -0.49487)
(0.172955,   -0.487856)
(0.175357,   -0.49178)
(0.177759,   -0.499278)
(0.180161,   -0.50735)
(0.182563,   -0.507914)
(0.184965,   -0.515953)
(0.187368,   -0.547562)
(0.18977,   -0.534889)
(0.192172,   -0.541162)
(0.194574,   -0.538338)
(0.196976,   -0.518268)
(0.199378,   -0.482024)
(0.20178,   -0.453675)
(0.204183,   -0.42528)
(0.206585,   -0.411983)
(0.208987,   -0.428649)
(0.211389,   -0.482187)
(0.213791,   -0.515476)
(0.216193,   -0.522738)
(0.218595,   -0.537266)
(0.220998,   -0.551261)
(0.2234,   -0.544799)
(0.225802,   -0.510808)
(0.228204,   -0.505534)
(0.230606,   -0.485416)
(0.233008,   -0.474888)
(0.23541,   -0.472177)
(0.237813,   -0.465989)
(0.240215,   -0.465607)
(0.242617,   -0.470183)
(0.245019,   -0.465001)
(0.247421,   -0.483722)
(0.249823,   -0.491446)
(0.252225,   -0.505841)
(0.254628,   -0.521237)
(0.25703,   -0.546167)
(0.259432,   -0.54751)
(0.261834,   -0.530019)
(0.264236,   -0.509159)
(0.266638,   -0.473231)
(0.269041,   -0.452672)
(0.271443,   -0.439268)
(0.273845,   -0.438144)
(0.276247,   -0.436385)
(0.278649,   -0.434276)
(0.281051,   -0.444525)
(0.283453,   -0.461794)
(0.285856,   -0.461826)
(0.288258,   -0.449819)
(0.29066,   -0.451338)
(0.293062,   -0.459465)
(0.295464,   -0.449435)
(0.297866,   -0.451215)
(0.300268,   -0.466506)
(0.302671,   -0.485464)
(0.305073,   -0.504063)
(0.307475,   -0.522317)
(0.309877,   -0.504887)
(0.312279,   -0.511948)
(0.314681,   -0.535326)
(0.317084,   -0.54401)
(0.319486,   -0.547559)
(0.321888,   -0.537442)
(0.32429,   -0.512427)
(0.326692,   -0.488889)
(0.329094,   -0.475163)
(0.331496,   -0.484244)
(0.333899,   -0.473717)
(0.336301,   -0.497995)
(0.338703,   -0.509664)
(0.341105,   -0.505575)
(0.343507,   -0.504484)
(0.345909,   -0.50649)
(0.348311,   -0.524047)
(0.350714,   -0.55354)
(0.353116,   -0.544427)
(0.355518,   -0.522022)
(0.35792,   -0.517306)
(0.360322,   -0.526118)
(0.362724,   -0.522418)
(0.365126,   -0.519384)
(0.367529,   -0.527294)
(0.369931,   -0.535535)
(0.372333,   -0.541334)
(0.374735,   -0.512034)
(0.377137,   -0.506611)
(0.379539,   -0.503457)
(0.381941,   -0.487849)
(0.384344,   -0.4868)
(0.386746,   -0.476825)
(0.389148,   -0.465002)
(0.39155,   -0.458739)
(0.393952,   -0.447351)
(0.396354,   -0.447468)
(0.398757,   -0.460181)
(0.401159,   -0.445656)
(0.403561,   -0.447645)
(0.405963,   -0.464307)
(0.408365,   -0.501807)
(0.410767,   -0.526665)
(0.413169,   -0.54066)
(0.415572,   -0.552078)
(0.417974,   -0.549263)
(0.420376,   -0.553902)
(0.422778,   -0.563158)
(0.42518,   -0.555596)
(0.427582,   -0.538711)
(0.429984,   -0.511413)
(0.432387,   -0.49259)
(0.434789,   -0.446985)
(0.437191,   -0.442534)
(0.439593,   -0.47021)
(0.441995,   -0.471894)
(0.444397,   -0.46178)
(0.446799,   -0.470089)
(0.449202,   -0.46369)
(0.451604,   -0.481827)
(0.454006,   -0.483911)
(0.456408,   -0.460338)
(0.45881,   -0.469406)
(0.461212,   -0.474202)
(0.463615,   -0.447797)
(0.466017,   -0.431211)
(0.468419,   -0.45062)
(0.470821,   -0.483806)
(0.473223,   -0.508879)
(0.475625,   -0.485796)
(0.478027,   -0.460655)
(0.48043,   -0.448336)
(0.482832,   -0.447124)
(0.485234,   -0.473859)
(0.487636,   -0.482176)
(0.490038,   -0.476648)
(0.49244,   -0.485421)
(0.494842,   -0.508121)
(0.497245,   -0.52261)
(0.499647,   -0.504078)
(0.502049,   -0.503497)
(0.504451,   -0.49969)
(0.506853,   -0.496657)
(0.509255,   -0.496262)
(0.511657,   -0.477086)
(0.51406,   -0.468741)
(0.516462,   -0.470776)
(0.518864,   -0.496485)
(0.521266,   -0.517079)
(0.523668,   -0.509667)
(0.52607,   -0.51102)
(0.528472,   -0.539023)
(0.530875,   -0.558276)
(0.533277,   -0.587432)
(0.535679,   -0.579612)
(0.538081,   -0.558185)
(0.540483,   -0.5446)
(0.542885,   -0.545042)
(0.545288,   -0.544283)
(0.54769,   -0.54352)
(0.550092,   -0.51928)
(0.552494,   -0.505749)
(0.554896,   -0.509813)
(0.557298,   -0.536525)
(0.5597,   -0.557511)
(0.562103,   -0.574156)
(0.564505,   -0.549628)
(0.566907,   -0.516257)
(0.569309,   -0.501908)
(0.571711,   -0.505567)
(0.574113,   -0.475114)
(0.576515,   -0.446506)
(0.578918,   -0.415498)
(0.58132,   -0.413538)
(0.583722,   -0.420035)
(0.586124,   -0.502972)
(0.588526,   -0.527525)
(0.590928,   -0.548612)
(0.593331,   -0.524783)
(0.595733,   -0.499887)
(0.598135,   -0.488404)
(0.600537,   -0.510964)
(0.602939,   -0.53026)
(0.605341,   -0.540405)
(0.607743,   -0.55257)
(0.610146,   -0.551649)
(0.612548,   -0.536704)
(0.61495,   -0.535284)
(0.617352,   -0.518479)
(0.619754,   -0.504183)
(0.622156,   -0.495386)
(0.624558,   -0.500356)
(0.626961,   -0.496939)
(0.629363,   -0.494757)
(0.631765,   -0.499869)
(0.634167,   -0.489624)
(0.636569,   -0.478058)
(0.638971,   -0.48258)
(0.641373,   -0.495589)
(0.643776,   -0.508706)
(0.646178,   -0.48939)
(0.64858,   -0.507512)
(0.650982,   -0.523232)
(0.653384,   -0.507377)
(0.655786,   -0.466012)
(0.658189,   -0.458536)
(0.660591,   -0.464317)
(0.662993,   -0.485548)
(0.665395,   -0.499935)
(0.667797,   -0.51011)
(0.670199,   -0.514266)
(0.672601,   -0.511869)
(0.675004,   -0.494434)
(0.677406,   -0.476177)
(0.679808,   -0.471702)
(0.68221,   -0.463646)
(0.684612,   -0.465778)
(0.687014,   -0.469361)
(0.689416,   -0.479432)
(0.691819,   -0.484675)
(0.694221,   -0.487325)
(0.696623,   -0.490438)
(0.699025,   -0.490686)
(0.701427,   -0.510978)
(0.703829,   -0.535617)
(0.706231,   -0.543355)
(0.708634,   -0.543364)
(0.711036,   -0.540424)
(0.713438,   -0.537346)
(0.71584,   -0.552469)
(0.718242,   -0.547008)
(0.720644,   -0.530644)
(0.723046,   -0.515303)
(0.725449,   -0.50074)
(0.727851,   -0.510919)
(0.730253,   -0.505338)
(0.732655,   -0.493613)
(0.735057,   -0.494622)
(0.737459,   -0.468691)
(0.739861,   -0.47562)
(0.742264,   -0.518549)
(0.744666,   -0.52479)
(0.747068,   -0.50667)
(0.74947,   -0.509009)
(0.751872,   -0.487165)
(0.754274,   -0.482498)
(0.756677,   -0.486301)
(0.759079,   -0.507136)
(0.761481,   -0.521302)
(0.763883,   -0.522293)
(0.766285,   -0.499673)
(0.768687,   -0.482733)
(0.771089,   -0.482934)
(0.773492,   -0.48839)
(0.775894,   -0.452285)
(0.778296,   -0.451787)
(0.780698,   -0.458248)
(0.7831,   -0.456348)
(0.785502,   -0.477958)
(0.787905,   -0.468644)
(0.790307,   -0.475519)
(0.792709,   -0.472114)
(0.795111,   -0.467992)
(0.797513,   -0.463052)
(0.799915,   -0.469412)
(0.802317,   -0.480172)
(0.804719,   -0.489884)
(0.807122,   -0.508841)
(0.809524,   -0.519436)
(0.811926,   -0.528544)
(0.814328,   -0.52322)
(0.81673,   -0.502602)
(0.819132,   -0.487224)
(0.821535,   -0.492623)
(0.823937,   -0.473869)
(0.826339,   -0.468301)
(0.828741,   -0.459702)
(0.831143,   -0.447288)
(0.833545,   -0.449023)
(0.835947,   -0.468605)
(0.83835,   -0.468678)
(0.840752,   -0.47747)
(0.843154,   -0.483519)
(0.845556,   -0.473226)
(0.847958,   -0.481175)
(0.85036,   -0.482708)
(0.852762,   -0.481142)
(0.855165,   -0.477622)
(0.857567,   -0.465317)
(0.859969,   -0.458466)
(0.862371,   -0.47282)
(0.864773,   -0.493763)
(0.867175,   -0.510048)
(0.869577,   -0.511913)
(0.87198,   -0.51112)
(0.874382,   -0.517201)
(0.876784,   -0.521988)
(0.879186,   -0.525639)
(0.881588,   -0.507626)
(0.88399,   -0.502971)
(0.886393,   -0.49525)
(0.888795,   -0.486517)
(0.891197,   -0.458721)
(0.893599,   -0.456481)
(0.896001,   -0.435793)
(0.898403,   -0.428697)
(0.900805,   -0.428205)
(0.903208,   -0.452644)
(0.90561,   -0.461145)
(0.908012,   -0.467869)
(0.910414,   -0.483879)
(0.912816,   -0.490269)
(0.915218,   -0.500273)
(0.91762,   -0.510299)
(0.920023,   -0.502247)
(0.922425,   -0.514754)
(0.924827,   -0.510298)
(0.927229,   -0.506382)
(0.929631,   -0.496978)
(0.932033,   -0.497481)
(0.934435,   -0.514198)
(0.936838,   -0.545358)
(0.93924,   -0.541085)
(0.941642,   -0.519236)
(0.944044,   -0.496447)
(0.946446,   -0.4867)
(0.948848,   -0.479916)
(0.951251,   -0.478204)
(0.953653,   -0.483977)
(0.956055,   -0.491081)
(0.958457,   -0.484275)
(0.960859,   -0.48794)
(0.963261,   -0.490689)
(0.965663,   -0.491202)
(0.968066,   -0.480858)
(0.970468,   -0.475175)
(0.97287,   -0.479981)
(0.975272,   -0.499496)
(0.977674,   -0.509066)
(0.980076,   -0.514401)
(0.982478,   -0.500878)
(0.984881,   -0.497163)
(0.987283,   -0.510991)
(0.989685,   -0.524068)
(0.992087,   -0.531774)
(0.994489,   -0.531829)
(0.996891,   -0.534188)
(0.999293,   -0.525635)
(1.0,   -0)
};

==> exp_plots/step_responses/ex.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(10.1139, 0.0526296)
(10.3291, 0.0535037)
(10.5443, 0.0492299)
(10.7595, 0.0336662)
(10.9747, 0.0138871)
(11.1899, 0.0122927)
(11.4051, 0.0175614)
(11.6203, 0.0330953)
(11.8354, 0.0416144)
(12.0506, 0.0477712)
(12.2658, 0.0511876)
(12.481, 0.0513847)
(12.6962, 0.0433671)
(12.9114, 0.0409158)
(13.1266, 0.0320486)
(13.3418, 0.033055)
(13.557, 0.033823)
(13.7722, 0.0203828)
(13.9873, 0.0169903)
(14.2025, 0.0184458)
(14.4177, 0.0229428)
(14.6329, 0.0270529)
(14.8481, 0.0271219)
(15.0633, 0.0273824)
(15.2785, 0.0393813)
(15.4937, 0.0517422)
(15.7089, 0.0577402)
(15.9241, 0.0572094)
(16.1392, 0.0502418)
(16.3544, 0.0491737)
(16.5696, 0.0429081)
(16.7848, 0.0299239)
(17, 0.00826819)
(17.2152, 0.000895945)
(17.4304, 0.00628704)
(17.6456, 0.0110432)
(17.8608, 0.019165)
(18.076, 0.0151549)
(18.2911, 0.0142096)
(18.5063, 0.0112005)
(18.7215, 0.0108252)
(18.9367, 0.0158915)
(19.1519, 0.0163657)
(19.3671, 0.0226353)
(19.5823, 0.0304633)
(19.7975, 0.0242215)
(20.0127, 0.0181433)
(20.2278, 0.020423)
(20.443, 0.0328102)
(20.6582, 0.0286054)
(20.8734, 0.0236828)
(21.0886, 0.026831)
(21.3038, 0.0259879)
(21.519, 0.0193626)
(21.7342, 0.00182444)
(21.9494, -0.0122153)
(22.1646, -0.00976552)
(22.3797, 0.00453517)
(22.5949, 0.0116223)
(22.8101, 0.00985044)
(23.0253, 0.0144276)
(23.2405, 0.0195026)
(23.4557, 0.0380278)
(23.6709, 0.0355318)
(23.8861, 0.0453681)
(24.1013, 0.0484136)
(24.3165, 0.0543012)
(24.5316, 0.0465908)
(24.7468, 0.0383694)
(24.962, 0.0291229)
(25.1772, 0.0206167)
(25.3924, 0.00719932)
(25.6076, 0.0104685)
(25.8228, 0.00937754)
(26.038, 0.00774767)
(26.2532, 0.01009)
(26.4684, 0.00684595)
(26.6835, 0.306754)
(26.8987, 0.308899)
(27.1139, 0.282091)
(27.3291, 0.233668)
(27.5443, 0.187653)
(27.7595, 0.131908)
(27.9747, 0.0816382)
(28.1899, 0.0374568)
(28.4051, 0.0125046)
(28.6203, -0.00774187)
(28.8354, -0.0149951)
(29.0506, -0.0114215)
(29.2658, -0.00610679)
(29.481, 0.011138)
(29.6962, 0.0101671)
(29.9114, 0.029393)
(30.1266, 0.0560533)
(30.3418, 0.0624763)
(30.557, 0.0606347)
(30.7722, 0.0567627)
(30.9873, 0.0465885)
(31.2025, 0.0308784)
(31.4177, 0.00344688)
(31.6329, -0.00575078)
(31.8481, -0.00480443)
(32.0633, -0.00209165)
(32.2785, -0.00231653)
(32.4937, -0.00120467)
(32.7089, 0.00262961)
(32.9241, -0.00244564)
(33.1392, -0.00412977)
(33.3544, -0.0136423)
(33.5696, -0.0172656)
(33.7848, -0.0132406)
(34, -0.00200763)
(34.2152, 0.0102177)
(34.4304, 0.0176703)
(34.6456, 0.0163082)
(34.8608, 0.0198101)
(35.076, 0.0214411)
(35.2911, 0.00815269)
(35.5063, -0.00758749)
(35.7215, -0.0162699)
(35.9367, -0.0170757)
(36.1519, -0.00996864)
(36.3671, -0.00859958)
(36.5823, -0.00676337)
(36.7975, -0.311423)
(37.0127, -0.308855)
(37.2278, -0.283386)
(37.443, -0.240751)
(37.6582, -0.185114)
(37.8734, -0.131624)
(38.0886, -0.082183)
(38.3038, 0.00195279)
(38.519, 0.0581416)
(38.7342, 0.0837309)
(38.9494, 0.102702)
(39.1646, 0.0996397)
(39.3797, 0.0787375)
(39.5949, 0.061894)
(39.8101, 0.029994)
(40.0253, 0.0131872)
(40.2405, -0.00489358)
(40.4557, -0.00340413)
(40.6709, -0.00519221)
(40.8861, 0.000572987)
(41.1013, 0.000364138)
(41.3165, -0.00138907)
(41.5316, 0.00638004)
(41.7468, 0.0156597)
(41.962, 0.0231187)
(42.1772, 0.0302683)
(42.3924, 0.0252782)
(42.6076, 0.0117818)
(42.8228, -0.003635)
(43.038, -0.011656)
(43.2532, -0.0177039)
(43.4684, -0.0208363)
(43.6835, -0.0125834)
(43.8987, -0.00566028)
(44.1139, 0.0361763)
(44.3291, 0.0727785)
(44.5443, 0.0740226)
(44.7595, 0.0604757)
(44.9747, 0.0529322)
(45.1899, 0.0458205)
(45.4051, 0.0353804)
(45.6203, 0.00861348)
(45.8354, -0.0142903)
(46.0506, -0.0283005)
(46.2658, -0.0203945)
(46.481, -0.0108212)
(46.6962, -0.302248)
(46.9114, -0.298284)
(47.1266, -0.261794)
(47.3418, -0.220551)
(47.557, -0.189122)
(47.7722, -0.133196)
(47.9873, -0.0791638)
(48.2025, -0.00187895)
(48.4177, 0.0498843)
(48.6329, 0.0666732)
(48.8481, 0.0642147)
(49.0633, 0.0502617)
(49.2785, 0.0488258)
(49.4937, 0.0411241)
(49.7089, 0.0349394)
(49.9241, 0.0265685)
(50.1392, 0.0194475)
(50.3544, 0.0116716)
(50.5696, 0.00585115)
(50.7848, -0.00798464)
(51, -0.011997)
(51.2152, -0.00910595)
(51.4304, -0.00668657)
(51.6456, -0.00657755)
(51.8608, -0.0056549)
(52.076, 0.00552374)
(52.2911, -0.00927278)
(52.5063, -0.00747234)
(52.7215, -0.0195463)
(52.9367, -0.0209536)
(53.1519, -0.00199732)
(53.3671, 0.0264247)
(53.5823, 0.042676)
(53.7975, 0.0438683)
(54.0127, 0.043987)
(54.2278, 0.0381272)
(54.443, 0.0105977)
(54.6582, -0.00270572)
(54.8734, -0.00321621)
(55.0886, -0.00592619)
(55.3038, -0.00854453)
(55.519, -0.0179598)
(55.7342, -0.0114588)
(55.9494, -0.0116988)
(56.1646, -0.0191679)
(56.3797, -0.0281658)
(56.5949, 0.278029)
(56.8101, 0.298391)
(57.0253, 0.293074)
(57.2405, 0.271306)
(57.4557, 0.21426)
(57.6709, 0.159485)
(57.8861, 0.100233)
(58.1013, 0.0408828)
(58.3165, 0.00487944)
(58.5316, -0.00756553)
(58.7468, -0.0109915)
(58.962, -0.0131951)
(59.1772, -0.00751979)
(59.3924, 0.00420592)
(59.6076, 0.0313999)
(59.8228, 0.040298)
(60.038, 0.0458526)
(60.2532, 0.0422915)
(60.4684, 0.0343308)
(60.6835, 0.0238955)
(60.8987, 0.0225885)
(61.1139, 0.0246105)
(61.3291, 0.0240163)
(61.5443, 0.0187625)
(61.7595, 0.00860731)
(61.9747, -0.000723683)
(62.1899, -0.023603)
(62.4051, -0.0249522)
(62.6203, -0.026981)
(62.8354, -0.0326402)
(63.0506, -0.0383144)
(63.2658, -0.0295505)
(63.481, -0.0164215)
(63.6962, -0.016494)
(63.9114, -0.00286928)
(64.1266, 0.00476679)
(64.3418, 0.00182675)
(64.557, 0.00240194)
(64.7722, 0.00303897)
(64.9873, 0.00282554)
(65.2025, -0.00148351)
(65.4177, 0.00491024)
(65.6329, 0.00304721)
(65.8481, 0.00751525)
(66.0633, 0.00639611)
(66.2785, 0.00124566)
(66.4937, 0.00955782)
(66.7089, 0.0159269)
(66.924, 0.0183415)
(67.1392, 0.0187721)
(67.3544, 0.0168567)
(67.5696, 0.0141574)
(67.7848, 0.0140011)
(68, 0.0182997)
(68.2152, 0.0167519)
(68.4304, 0.0219321)
(68.6456, 0.0381139)
(68.8608, 0.0600352)
(69.076, 0.0604308)
(69.2911, 0.0490898)
(69.5063, 0.0380943)
(69.7215, 0.0288946)
(69.9367, 0.0256257)
(70.1519, 0.0304768)
};

==> exp_plots/step_responses/ey.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(10.1139, 0.0193167)
(10.3291, 0.0242235)
(10.5443, 0.0215293)
(10.7595, 0.0246933)
(10.9747, 0.0397573)
(11.1899, 0.0594422)
(11.4051, 0.067088)
(11.6203, 0.0650471)
(11.8354, 0.0678171)
(12.0506, 0.0684963)
(12.2658, 0.0640321)
(12.481, 0.0550659)
(12.6962, 0.0325342)
(12.9114, 0.0107493)
(13.1266, -0.00475237)
(13.3418, -0.00473532)
(13.557, -0.000982756)
(13.7722, 0.00571841)
(13.9873, 0.0140798)
(14.2025, 0.0368256)
(14.4177, 0.0432115)
(14.6329, 0.0500166)
(14.8481, 0.0552723)
(15.0633, 0.0547288)
(15.2785, 0.0551598)
(15.4937, 0.0684403)
(15.7089, 0.0744468)
(15.9241, 0.0723597)
(16.1392, 0.0682094)
(16.3544, 0.0535256)
(16.5696, 0.0473486)
(16.7848, 0.0348472)
(17, 0.0383801)
(17.2152, 0.0326765)
(17.4304, 0.0338917)
(17.6456, 0.0268649)
(17.8608, 0.0200444)
(18.076, 0.00656404)
(18.2911, -0.0110863)
(18.5063, -0.0117043)
(18.7215, -0.00675391)
(18.9367, -0.00245327)
(19.1519, 0.0137254)
(19.3671, 0.064348)
(19.5823, 0.102283)
(19.7975, 0.116881)
(20.0127, 0.111644)
(20.2278, 0.0977845)
(20.443, 0.0703524)
(20.6582, 0.0596225)
(20.8734, 0.0550405)
(21.0886, 0.0404227)
(21.3038, -0.0214917)
(21.519, -0.026927)
(21.7342, -0.0260302)
(21.9494, -0.00665966)
(22.1646, 0.0459021)
(22.3797, 0.0811031)
(22.5949, 0.0926058)
(22.8101, 0.0887169)
(23.0253, 0.0822048)
(23.2405, 0.0754977)
(23.4557, 0.0589844)
(23.6709, 0.0377072)
(23.8861, 0.0076656)
(24.1013, 0.00233572)
(24.3165, 0.0113285)
(24.5316, 0.0233694)
(24.7468, 0.0480524)
(24.962, 0.0805595)
(25.1772, 0.0859025)
(25.3924, 0.0972754)
(25.6076, 0.080287)
(25.8228, 0.0712214)
(26.038, 0.557448)
(26.2532, 0.54757)
(26.4684, 0.485891)
(26.6835, 0.382754)
(26.8987, 0.236809)
(27.1139, 0.136931)
(27.3291, 0.0171866)
(27.5443, -0.0339304)
(27.7595, -0.0185814)
(27.9747, -0.0225803)
(28.1899, -0.0323516)
(28.4051, -0.0193204)
(28.6203, -0.00599265)
(28.8354, 0.0192767)
(29.0506, 0.0531526)
(29.2658, 0.0851651)
(29.481, 0.135931)
(29.6962, 0.143763)
(29.9114, 0.149182)
(30.1266, 0.141973)
(30.3418, 0.105795)
(30.557, 0.0490494)
(30.7722, 0.0296937)
(30.9873, 0.032161)
(31.2025, 0.0369508)
(31.4177, 0.0406776)
(31.6329, 0.0382371)
(31.8481, 0.048407)
(32.0633, 0.0610456)
(32.2785, 0.0755674)
(32.4937, 0.064602)
(32.7089, 0.0549444)
(32.9241, 0.033127)
(33.1392, 0.0205423)
(33.3544, 0.0203361)
(33.5696, 0.0043658)
(33.7848, 0.00888896)
(34, 0.015082)
(34.2152, 0.0236444)
(34.4304, 0.0165336)
(34.6456, 0.0246395)
(34.8608, 0.0669287)
(35.076, 0.0649697)
(35.2911, 0.0698019)
(35.5063, 0.0680596)
(35.7215, 0.0586364)
(35.9367, -0.448393)
(36.1519, -0.473875)
(36.3671, -0.433027)
(36.5823, -0.266197)
(36.7975, -0.0636192)
(37.0127, 0.07978)
(37.2278, 0.156824)
(37.443, 0.169032)
(37.6582, 0.162418)
(37.8734, 0.118048)
(38.0886, 0.0900312)
(38.3038, 0.0524374)
(38.519, 0.00361752)
(38.7342, -0.0221166)
(38.9494, -0.035215)
(39.1646, -0.0274977)
(39.3797, -0.0130948)
(39.5949, -0.00617712)
(39.8101, 0.0373987)
(40.0253, 0.0634033)
(40.2405, 0.0623404)
(40.4557, 0.0524935)
(40.6709, 0.0489003)
(40.8861, 0.0513741)
(41.1013, 0.0513366)
(41.3165, 0.0416003)
(41.5316, 0.0351184)
(41.7468, 0.0255057)
(41.962, 0.0287504)
(42.1772, 0.0224091)
(42.3924, 0.01043)
(42.6076, 0.000939419)
(42.8228, 0.0043264)
(43.038, 0.0107211)
(43.2532, 0.0261693)
(43.4684, 0.0477755)
(43.6835, 0.0482737)
(43.8987, 0.0475367)
(44.1139, 0.0537263)
(44.3291, 0.042437)
(44.5443, 0.0397353)
(44.7595, 0.0361477)
(44.9747, 0.033738)
(45.1899, 0.0347949)
(45.4051, 0.0263543)
(45.6203, 0.0139315)
(45.8354, -0.496605)
(46.0506, -0.490228)
(46.2658, -0.436884)
(46.481, -0.319714)
(46.6962, -0.171983)
(46.9114, -0.0316434)
(47.1266, 0.0540123)
(47.3418, 0.111555)
(47.557, 0.161819)
(47.7722, 0.159892)
(47.9873, 0.120206)
(48.2025, 0.101722)
(48.4177, 0.0547415)
(48.6329, 0.00974429)
(48.8481, -0.022844)
(49.0633, -0.0293713)
(49.2785, -0.0325776)
(49.4937, -0.00357434)
(49.7089, 0.0258315)
(49.9241, 0.0851567)
(50.1392, 0.105342)
(50.3544, 0.0957665)
(50.5696, 0.0887485)
(50.7848, 0.0974877)
(51, 0.0357774)
(51.2152, -0.000873744)
(51.4304, -0.0262603)
(51.6456, -0.0314437)
(51.8608, -0.0142639)
(52.076, -0.00427535)
(52.2911, 0.012413)
(52.5063, 0.0401584)
(52.7215, 0.0563175)
(52.9367, 0.0603417)
(53.1519, 0.0623254)
(53.3671, 0.0618793)
(53.5823, 0.0615089)
(53.7975, 0.0528221)
(54.0127, 0.0426538)
(54.2278, 0.0136653)
(54.443, 0.00857121)
(54.6582, 0.0116492)
(54.8734, 0.0204172)
(55.0886, 0.0322922)
(55.3038, 0.0447367)
(55.519, 0.0396894)
(55.7342, 0.0379379)
(55.9494, 0.532791)
(56.1646, 0.540325)
(56.3797, 0.479753)
(56.5949, 0.381161)
(56.8101, 0.240658)
(57.0253, 0.130402)
(57.2405, 0.0771626)
(57.4557, 0.02094)
(57.6709, -0.0120937)
(57.8861, -0.0102113)
(58.1013, -0.00359574)
(58.3165, 0.0176873)
(58.5316, 0.0328726)
(58.7468, 0.0886643)
(58.962, 0.109976)
(59.1772, 0.113377)
(59.3924, 0.111791)
(59.6076, 0.115434)
(59.8228, 0.105166)
(60.038, 0.0968432)
(60.2532, 0.0790405)
(60.4684, 0.0535876)
(60.6835, 0.0429245)
(60.8987, 0.0378417)
(61.1139, 0.018382)
(61.3291, -0.00994683)
(61.5443, -0.0321199)
(61.7595, -0.0188791)
(61.9747, -0.00462783)
(62.1899, 0.0038334)
(62.4051, 0.0728204)
(62.6203, 0.1124)
(62.8354, 0.133962)
(63.0506, 0.12425)
(63.2658, 0.107188)
(63.481, 0.0778465)
(63.6962, 0.050693)
(63.9114, 0.0375736)
(64.1266, 0.0455195)
(64.3418, 0.042403)
(64.557, 0.0473395)
(64.7722, 0.061049)
(64.9873, 0.0628338)
(65.2025, 0.0611626)
(65.4177, 0.0647565)
(65.6329, 0.0495098)
(65.8481, 0.0300283)
(66.0633, 0.0227286)
(66.2785, 0.0219317)
(66.4937, 0.0303113)
(66.7089, 0.0448811)
(66.924, 0.0436601)
(67.1392, 0.0472059)
(67.3544, 0.0510785)
(67.5696, 0.057016)
(67.7848, 0.0572062)
(68, 0.0505555)
(68.2152, 0.0441438)
(68.4304, 0.0284644)
(68.6456, 0.0125175)
(68.8608, 0.00905988)
(69.076, 0.0125353)
(69.2911, 0.026839)
(69.5063, 0.055109)
(69.7215, 0.0672434)
(69.9367, 0.067277)
(70.1519, 0.0655097)
};

==> exp_plots/step_responses/ez.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(10.075, -0.0394625)
(10.2375, -0.0431382)
(10.4, -0.0390308)
(10.5625, -0.0409622)
(10.725, -0.0353613)
(10.8875, -0.024207)
(11.05, -0.0161124)
(11.2125, -0.00196803)
(11.375, -9.23872e-05)
(11.5375, 0.00892735)
(11.7, -0.000540972)
(11.8625, -0.000145614)
(12.025, -0.0056386)
(12.1875, -0.00568289)
(12.35, -0.00365019)
(12.5125, -0.00180411)
(12.675, -0.00125122)
(12.8375, -0.0138915)
(13, -0.0153361)
(13.1625, -0.00641561)
(13.325, -0.00761563)
(13.4875, -0.00836778)
(13.65, -0.0148094)
(13.8125, -0.0279987)
(13.975, -0.0243367)
(14.1375, -0.0114754)
(14.3, -0.00483346)
(14.4625, -0.00465322)
(14.625, -0.0128878)
(14.7875, -0.0179179)
(14.95, -0.0165158)
(15.1125, -0.00915796)
(15.275, -0.00675052)
(15.4375, -0.000125408)
(15.6, -0.0168849)
(15.7625, -0.0255762)
(15.925, -0.0360272)
(16.0875, -0.0360304)
(16.25, -0.0325301)
(16.4125, -0.0416451)
(16.575, -0.0449224)
(16.7375, -0.0434923)
(16.9, 0.261962)
(17.0625, 0.264428)
(17.225, 0.272586)
(17.3875, 0.269467)
(17.55, 0.219605)
(17.7125, 0.183965)
(17.875, 0.180087)
(18.0375, 0.156938)
(18.2, 0.121083)
(18.3625, 0.103042)
(18.525, 0.0625768)
(18.6875, 0.0358692)
(18.85, 0.0338502)
(19.0125, 0.0221666)
(19.175, 0.0257892)
(19.3375, 0.0299743)
(19.5, 0.0297864)
(19.6625, 0.0299982)
(19.825, 0.0297685)
(19.9875, 0.0297422)
(20.15, 0.0332016)
(20.3125, 0.0357602)
(20.475, 0.0362517)
(20.6375, 0.0109094)
(20.8, 0.00229144)
(20.9625, -0.00457221)
(21.125, -0.026116)
(21.2875, -0.0316015)
(21.45, -0.0374814)
(21.6125, -0.0440741)
(21.775, -0.0441708)
(21.9375, -0.0428823)
(22.1, -0.0230097)
(22.2625, -0.0370632)
(22.425, -0.0318524)
(22.5875, -0.0233942)
(22.75, -0.0284565)
(22.9125, -0.0304777)
(23.075, -0.030489)
(23.2375, -0.0312045)
(23.4, -0.0303997)
(23.5625, -0.0290272)
(23.725, -0.0389068)
(23.8875, -0.0508499)
(24.05, -0.0512871)
(24.2125, -0.0303547)
(24.375, -0.0203684)
(24.5375, 0.0130501)
(24.7, 0.0139951)
(24.8625, 0.0105116)
(25.025, 0.0211004)
(25.1875, 0.0301269)
(25.35, 0.0493741)
(25.5125, 0.0573176)
(25.675, 0.0512776)
(25.8375, 0.0337384)
(26, 0.024552)
(26.1625, 0.0267805)
(26.325, 0.0281696)
(26.4875, 0.0194855)
(26.65, 0.0154436)
(26.8125, -0.183465)
(26.975, -0.180613)
(27.1375, -0.18134)
(27.3, -0.188818)
(27.4625, -0.186391)
(27.625, -0.160331)
(27.7875, -0.12777)
(27.95, -0.0797339)
(28.1125, -0.0412413)
(28.275, -0.0170083)
(28.4375, -0.00785303)
(28.6, -0.000883937)
(28.7625, 0.0105579)
(28.925, 0.012877)
(29.0875, 0.0189815)
(29.25, 0.0230241)
(29.4125, 0.0229316)
(29.575, 0.0233271)
(29.7375, 0.0260727)
(29.9, 0.0158633)
(30.0625, 0.0152787)
(30.225, 0.0126316)
(30.3875, 0.00970078)
(30.55, 0.00675267)
(30.7125, -0.00471413)
(30.875, -0.00274742)
(31.0375, 0.00314927)
(31.2, -0.00349903)
(31.3625, -0.0103425)
(31.525, -0.0133699)
(31.6875, -0.0153821)
(31.85, -0.0116331)
(32.0125, -0.0165573)
(32.175, -0.017676)
(32.3375, -0.00592899)
(32.5, 6.59227e-05)
(32.6625, 0.00236511)
(32.825, 0.0170226)
(32.9875, 0.0254871)
(33.15, 0.0255316)
(33.3125, 0.0194417)
(33.475, 0.0215552)
(33.6375, 0.0183473)
(33.8, 0.0166573)
(33.9625, 0.0237437)
(34.125, 0.0201228)
(34.2875, 0.0171762)
(34.45, -0.00338554)
(34.6125, -0.00258195)
(34.775, -0.000753641)
(34.9375, 0.0062151)
(35.1, 0.0101809)
(35.2625, 0.0128025)
(35.425, 0.0122001)
(35.5875, 0.0153306)
(35.75, 0.0145777)
(35.9125, 0.00698733)
(36.075, 0.0128399)
(36.2375, 0.0136797)
(36.4, 0.0173619)
(36.5625, 0.0112854)
(36.725, 0.318108)
(36.8875, 0.322184)
(37.05, 0.322248)
(37.2125, 0.293787)
(37.375, 0.284469)
(37.5375, 0.271632)
(37.7, 0.181857)
(37.8625, 0.155332)
(38.025, 0.0768839)
(38.1875, 0.0407355)
(38.35, -0.0138172)
(38.5125, -0.0293141)
(38.675, -0.0250385)
(38.8375, -0.00230992)
(39, 0.00354177)
(39.1625, 0.00768656)
(39.325, 0.00262952)
(39.4875, -0.00089699)
(39.65, 0.00566715)
(39.8125, 0.0127686)
(39.975, 0.0191549)
(40.1375, 0.0201873)
(40.3, 0.00837803)
(40.4625, 0.00875485)
(40.625, 0.0153508)
(40.7875, 0.0153783)
(40.95, 0.00505382)
(41.1125, 0.00296271)
(41.275, 0.00343865)
(41.4375, 0.00771832)
(41.6, 0.00641733)
(41.7625, 0.00553876)
(41.925, 0.00187826)
(42.0875, 0.00583678)
(42.25, 0.00814092)
(42.4125, 0.006194)
(42.575, 0.00113142)
(42.7375, -0.00481617)
(42.9, -0.00302571)
(43.0625, 0.00198245)
(43.225, 0.00250602)
(43.3875, 0.00325882)
(43.55, -0.00257385)
(43.7125, -0.001683)
(43.875, 0.000555992)
(44.0375, -0.00574696)
(44.2, -0.0121248)
(44.3625, -0.00750953)
(44.525, -0.0030483)
(44.6875, -0.00123358)
(44.85, 0.0115072)
(45.0125, 0.0258699)
};

==> exp_plots/step_responses/yaw.tex <==
\addplot[
    fill=none,draw = currclr,
    line width= \linew pt
    ]
 %%
coordinates{
(0.000000, 0.000000)
(0.032907, 0.000000)
(0.062761, 0.000000)
(0.099156, 0.000000)
(0.129950, 0.000000)
(0.165753, 0.000000)
(0.193936, 0.000000)
(0.228391, 0.000000)
(0.261557, 0.000000)
(0.292392, 0.000000)
(0.329782, 0.000000)
(0.370253, 0.000000)
(0.397213, 0.000000)
(0.431646, 0.000000)
(0.468384, 0.000000)
(0.496521, 0.000000)
(0.533131, 0.000000)
(0.564640, 0.000000)
(0.593544, 0.000000)
(0.628394, 0.000000)
(0.660468, 0.000000)
(0.693515, 0.000000)
(0.729235, 0.000000)
(0.759240, 0.000000)
(0.796739, 0.000000)
(0.833988, 0.000000)
(0.860999, 0.000000)
(0.892442, 0.000000)
(0.933587, 0.000000)
(0.965986, 0.000000)
(0.997910, 0.000000)
(1.031624, 0.000000)
(1.060639, 0.000000)
(1.093038, 0.000000)
(1.133887, 0.000000)
(1.167951, 0.000000)
(1.194599, 0.000000)
(1.233194, 0.000000)
(1.263740, 0.000000)
(1.297482, 0.000000)
(1.332266, 0.000000)
(1.367385, 0.000000)
(1.398498, 0.000000)
(1.437015, 0.000000)
(1.464571, 0.000000)
(1.501024, 0.000000)
(1.534085, 0.000000)
(1.564686, 0.000000)
(1.599735, 0.000000)
(1.633415, 0.000000)
(1.668613, 0.000000)
(1.700257, 0.000000)
(1.734497, 0.000000)
(1.763916, 0.000000)
(1.796423, 0.000000)
(1.828718, 0.000000)
(1.862355, 0.000000)
(1.896293, 0.000000)
(1.930358, 0.000000)
(1.963977, 0.000000)
(2.000041, 0.000000)
(2.033801, 0.000000)
(2.064144, 0.000000)
(2.094071, 0.000000)
(2.130587, 0.000000)
(2.164670, 0.000000)
(2.202131, 0.000000)
(2.242026, 0.000000)
(2.274426, 0.000000)
(2.303855, 0.000000)
(2.340054, 0.000000)
(2.369298, 0.000000)
(2.401813, 0.000000)
(2.436782, 0.000000)
(2.467305, 0.000000)
(2.499388, 0.000000)
(2.542110, 0.000000)
(2.577655, 0.000000)
(2.600355, 0.000000)
(2.636051, 0.000000)
(2.672182, 0.000000)
(2.700814, 0.000000)
(2.732477, 0.000000)
(2.767115, 0.000000)
(2.794135, 0.000000)
(2.839942, 0.000000)
(2.867065, 0.000000)
(2.896712, 0.000000)
(2.931751, 0.000000)
(2.962636, 0.000000)
(3.000629, 0.000000)
(3.035074, 0.000000)
(3.067178, 0.000000)
(3.102053, 0.000000)
(3.136258, 0.000000)
(3.163260, 0.000000)
(3.195024, 0.000000)
(3.234490, 0.000000)
(3.262304, 0.000000)
(3.296017, 0.000000)
(3.332243, 0.000000)
(3.366571, 0.000000)
(3.399052, 0.000000)
(3.432454, 0.000000)
(3.464896, 0.000000)
(3.498586, 0.000000)
(3.531600, 0.000000)
(3.558043, 0.000000)
(3.595046, 0.000000)
(3.628058, 0.000000)
(3.661241, 0.000000)
(3.695175, 0.000000)
(3.733665, 0.000000)
(3.765017, 0.000000)
(3.794625, 0.000000)
(3.834481, 0.000000)
(3.868802, 0.000000)
(3.900775, 0.000000)
(3.930340, 0.000000)
(3.964797, 0.000000)
(3.996945, 0.000000)
(4.034101, 0.000000)
(4.065475, 0.000000)
(4.095451, 0.000000)
(4.133482, 0.000000)
(4.163567, 0.000000)
(4.195832, 0.000000)
(4.232382, 0.000000)
(4.266459, 0.000000)
(4.297679, 0.000000)
(4.331636, 0.000000)
(4.372817, 0.000000)
(4.392772, 0.000000)
(4.433208, 0.000000)
(4.464170, 0.000000)
(4.498114, 0.000000)
(4.531214, 0.000000)
(4.564336, 0.000000)
(4.596074, 0.000000)
(4.635769, 0.000000)
(4.671154, 0.000000)
(4.698308, 0.000000)
(4.731188, 0.000000)
(4.762158, 0.000000)
(4.799803, 0.000000)
(4.835503, 0.000000)
(4.865563, 0.000000)
(4.898664, 0.000000)
(4.933047, 0.000000)
(4.964197, 0.000000)
(4.994103, 0.000000)
(5.032923, 0.500000)
(5.064976, 0.500000)
(5.095844, 0.500000)
(5.131793, 0.500000)
(5.160636, 0.500000)
(5.197741, 0.500000)
(5.235407, 0.500000)
(5.268848, 0.500000)
(5.296447, 0.500000)
(5.330208, 0.500000)
(5.364277, 0.500000)
(5.397705, 0.500000)
(5.428033, 0.500000)
(5.462548, 0.500000)
(5.496419, 0.500000)
(5.531839, 0.500000)
(5.567320, 0.500000)
(5.597363, 0.500000)
(5.633064, 0.500000)
(5.662623, 0.500000)
(5.694250, 0.500000)
(5.733066, 0.500000)
(5.763326, 0.500000)
(5.793659, 0.500000)
(5.839064, 0.500000)
(5.862118, 0.500000)
(5.897129, 0.500000)
(5.934341, 0.500000)
(5.971149, 0.500000)
(5.996983, 0.500000)
(6.030978, 0.500000)
(6.065285, 0.500000)
(6.094917, 0.500000)
(6.139251, 0.500000)
(6.163533, 0.500000)
(6.195184, 0.500000)
(6.232700, 0.500000)
(6.262712, 0.500000)
(6.294273, 0.500000)
(6.330581, 0.500000)
(6.364866, 0.500000)
(6.391685, 0.500000)
(6.430264, 0.500000)
(6.464236, 0.500000)
(6.492829, 0.500000)
(6.531189, 0.500000)
(6.560291, 0.500000)
(6.595351, 0.500000)
(6.628312, 0.500000)
(6.664210, 0.500000)
(6.702124, 0.500000)
(6.731398, 0.500000)
(6.765063, 0.500000)
(6.793592, 0.500000)
(6.832159, 0.500000)
(6.860442, 0.500000)
(6.897730, 0.500000)
(6.933580, 0.500000)
(6.962202, 0.500000)
(6.996201, 0.500000)
(7.034192, 0.500000)
(7.064157, 0.500000)
(7.096715, 0.500000)
(7.133627, 0.500000)
(7.164630, 0.500000)
(7.199106, 0.500000)
(7.230481, 0.500000)
(7.266715, 0.500000)
(7.294021, 0.500000)
(7.328733, 0.500000)
(7.360404, 0.500000)
(7.399731, 0.500000)
(7.431434, 0.500000)
(7.470118, 0.500000)
(7.495596, 0.500000)
(7.530021, 0.500000)
(7.564131, 0.500000)
(7.592423, 0.500000)
(7.625953, 0.500000)
(7.662565, 0.500000)
(7.692568, 0.500000)
(7.729641, 0.500000)
(7.765351, 0.500000)
(7.796402, 0.500000)
(7.830523, 0.500000)
(7.861592, 0.500000)
(7.894241, 0.500000)
(7.928831, 0.500000)
(7.962272, 0.500000)
(7.995386, 0.500000)
(8.032472, 0.500000)
(8.067616, 0.500000)
(8.094709, 0.500000)
(8.131528, 0.500000)
(8.163263, 0.500000)
(8.196895, 0.500000)
(8.230722, 0.500000)
(8.269568, 0.500000)
(8.297719, 0.500000)
(8.329178, 0.500000)
(8.364059, 0.500000)
(8.395649, 0.500000)
(8.427168, 0.500000)
(8.465327, 0.500000)
(8.495017, 0.500000)
(8.530432, 0.500000)
(8.563704, 0.500000)
(8.602518, 0.500000)
(8.632129, 0.500000)
(8.668015, 0.500000)
(8.700492, 0.500000)
(8.731572, 0.500000)
(8.762015, 0.500000)
(8.797150, 0.500000)
(8.833573, 0.500000)
(8.867826, 0.500000)
(8.903646, 0.500000)
(8.929855, 0.500000)
(8.967199, 0.500000)
(8.997551, 0.500000)
(9.032206, 0.500000)
(9.062511, 0.500000)
(9.092272, 0.500000)
(9.133962, 0.500000)
(9.161540, 0.500000)
(9.197236, 0.500000)
(9.230119, 0.500000)
(9.264680, 0.500000)
(9.293431, 0.500000)
(9.330903, 0.500000)
(9.361966, 0.500000)
(9.395635, 0.500000)
(9.433397, 0.500000)
(9.463463, 0.500000)
(9.493546, 0.500000)
(9.533072, 0.500000)
(9.563852, 0.500000)
(9.600721, 0.500000)
(9.634478, 0.500000)
(9.665073, 0.500000)
(9.700306, 0.500000)
(9.733113, 0.500000)
(9.765276, 0.500000)
(9.799196, 0.500000)
(9.829104, 0.500000)
(9.866053, 0.500000)
(9.896494, 0.500000)
(9.934001, 0.500000)
(9.959985, 0.500000)
(9.993752, 0.500000)
(10.031167, 0.000000)
(10.063027, 0.000000)
(10.096301, 0.000000)
(10.135336, 0.000000)
(10.166135, 0.000000)
(10.201086, 0.000000)
(10.230821, 0.000000)
(10.265347, 0.000000)
(10.307892, 0.000000)
(10.333893, 0.000000)
(10.363275, 0.000000)
(10.397418, 0.000000)
(10.435137, 0.000000)
(10.465668, 0.000000)
(10.495579, 0.000000)
(10.526779, 0.000000)
(10.563776, 0.000000)
(10.595040, 0.000000)
(10.634655, 0.000000)
(10.663806, 0.000000)
(10.695578, 0.000000)
(10.728919, 0.000000)
(10.760738, 0.000000)
(10.794507, 0.000000)
(10.826254, 0.000000)
(10.866492, 0.000000)
(10.889975, 0.000000)
(10.928892, 0.000000)
(10.963261, 0.000000)
(10.995407, 0.000000)
(11.031898, 0.000000)
(11.061822, 0.000000)
(11.101187, 0.000000)
(11.126880, 0.000000)
(11.164371, 0.000000)
(11.199227, 0.000000)
(11.235794, 0.000000)
(11.266492, 0.000000)
(11.309587, 0.000000)
(11.332639, 0.000000)
(11.366953, 0.000000)
(11.396490, 0.000000)
(11.435691, 0.000000)
(11.470110, 0.000000)
(11.498376, 0.000000)
(11.533786, 0.000000)
(11.564941, 0.000000)
(11.598574, 0.000000)
(11.633995, 0.000000)
(11.665583, 0.000000)
(11.694270, 0.000000)
(11.733031, 0.000000)
(11.766126, 0.000000)
(11.801460, 0.000000)
(11.833681, 0.000000)
(11.863360, 0.000000)
(11.897003, 0.000000)
(11.932692, 0.000000)
(11.965088, 0.000000)
(11.999536, 0.000000)
(12.033054, 0.000000)
(12.061716, 0.000000)
(12.098525, 0.000000)
(12.140690, 0.000000)
(12.165751, 0.000000)
(12.196928, 0.000000)
(12.232549, 0.000000)
(12.264841, 0.000000)
(12.296071, 0.000000)
(12.330084, 0.000000)
(12.362422, 0.000000)
(12.394089, 0.000000)
(12.438736, 0.000000)
(12.463762, 0.000000)
(12.498752, 0.000000)
(12.530001, 0.000000)
(12.561997, 0.000000)
(12.592821, 0.000000)
(12.630338, 0.000000)
(12.662843, 0.000000)
(12.692714, 0.000000)
(12.736881, 0.000000)
(12.769895, 0.000000)
(12.796587, 0.000000)
(12.831881, 0.000000)
(12.862697, 0.000000)
(12.897333, 0.000000)
(12.927094, 0.000000)
(12.966120, 0.000000)
(12.995205, 0.000000)
(13.029028, 0.000000)
(13.061118, 0.000000)
(13.095151, 0.000000)
(13.130626, 0.000000)
(13.160268, 0.000000)
(13.192458, 0.000000)
(13.229842, 0.000000)
(13.262951, 0.000000)
(13.291424, 0.000000)
(13.327871, 0.000000)
(13.365177, 0.000000)
(13.393091, 0.000000)
(13.426115, 0.000000)
(13.461692, 0.000000)
(13.495413, 0.000000)
(13.531981, 0.000000)
(13.563937, 0.000000)
(13.597040, 0.000000)
(13.627987, 0.000000)
(13.666540, 0.000000)
(13.692537, 0.000000)
(13.730198, 0.000000)
(13.765574, 0.000000)
(13.793833, 0.000000)
(13.835137, 0.000000)
(13.860224, 0.000000)
(13.898758, 0.000000)
(13.934139, 0.000000)
(13.969197, 0.000000)
(13.997362, 0.000000)
(14.033179, 0.000000)
(14.068600, 0.000000)
(14.096314, 0.000000)
(14.133842, 0.000000)
(14.170678, 0.000000)
(14.198231, 0.000000)
(14.232775, 0.000000)
(14.272419, 0.000000)
(14.300295, 0.000000)
(14.335476, 0.000000)
(14.367599, 0.000000)
(14.395101, 0.000000)
(14.432243, 0.000000)
(14.468035, 0.000000)
(14.496995, 0.000000)
(14.536459, 0.000000)
(14.565752, 0.000000)
(14.596197, 0.000000)
(14.635535, 0.000000)
(14.664274, 0.000000)
(14.698331, 0.000000)
(14.733498, 0.000000)
(14.765669, 0.000000)
(14.794340, 0.000000)
(14.830121, 0.000000)
(14.862068, 0.000000)
(14.895944, 0.000000)
(14.932391, 0.000000)
(14.962316, 0.000000)
(14.996885, 0.000000)
(15.029431, -0.500000)
(15.062099, -0.500000)
(15.094184, -0.500000)
(15.133767, -0.500000)
(15.165980, -0.500000)
(15.196164, -0.500000)
(15.233513, -0.500000)
(15.267859, -0.500000)
(15.298458, -0.500000)
(15.333828, -0.500000)
(15.363088, -0.500000)
(15.396466, -0.500000)
(15.433797, -0.500000)
(15.460214, -0.500000)
(15.494213, -0.500000)
(15.535244, -0.500000)
(15.561469, -0.500000)
(15.593652, -0.500000)
(15.633888, -0.500000)
(15.663216, -0.500000)
(15.695759, -0.500000)
(15.730407, -0.500000)
(15.765191, -0.500000)
(15.798187, -0.500000)
(15.829816, -0.500000)
(15.862677, -0.500000)
(15.894365, -0.500000)
(15.930459, -0.500000)
(15.961542, -0.500000)
(15.998383, -0.500000)
(16.031139, -0.500000)
(16.064640, -0.500000)
(16.094805, -0.500000)
(16.133522, -0.500000)
(16.163528, -0.500000)
(16.195232, -0.500000)
(16.232773, -0.500000)
(16.266174, -0.500000)
(16.298170, -0.500000)
(16.332056, -0.500000)
(16.366823, -0.500000)
(16.397148, -0.500000)
(16.429585, -0.500000)
(16.464878, -0.500000)
(16.497740, -0.500000)
(16.526941, -0.500000)
(16.563902, -0.500000)
(16.593758, -0.500000)
(16.639233, -0.500000)
(16.666922, -0.500000)
(16.707029, -0.500000)
(16.735460, -0.500000)
(16.764395, -0.500000)
(16.798353, -0.500000)
(16.835455, -0.500000)
(16.864494, -0.500000)
(16.896738, -0.500000)
(16.928804, -0.500000)
(16.967268, -0.500000)
(17.001842, -0.500000)
(17.036844, -0.500000)
(17.065083, -0.500000)
(17.096169, -0.500000)
(17.129910, -0.500000)
(17.164614, -0.500000)
(17.196672, -0.500000)
(17.229876, -0.500000)
(17.261803, -0.500000)
(17.301132, -0.500000)
(17.332460, -0.500000)
(17.365841, -0.500000)
(17.394920, -0.500000)
(17.432362, -0.500000)
(17.462721, -0.500000)
(17.494738, -0.500000)
(17.528868, -0.500000)
(17.566523, -0.500000)
(17.595392, -0.500000)
(17.638868, -0.500000)
(17.671988, -0.500000)
(17.695316, -0.500000)
(17.733515, -0.500000)
(17.766481, -0.500000)
(17.800713, -0.500000)
(17.832922, -0.500000)
(17.865217, -0.500000)
(17.898865, -0.500000)
(17.931290, -0.500000)
(17.965231, -0.500000)
(17.999779, -0.500000)
(18.032166, -0.500000)
(18.071001, -0.500000)
(18.100548, -0.500000)
(18.138834, -0.500000)
(18.164602, -0.500000)
(18.199627, -0.500000)
(18.234806, -0.500000)
(18.267197, -0.500000)
(18.297958, -0.500000)
(18.331667, -0.500000)
(18.366722, -0.500000)
(18.397043, -0.500000)
(18.434376, -0.500000)
(18.463037, -0.500000)
(18.496124, -0.500000)
(18.531105, -0.500000)
(18.566057, -0.500000)
(18.595682, -0.500000)
(18.631454, -0.500000)
(18.661718, -0.500000)
(18.697771, -0.500000)
(18.730629, -0.500000)
(18.761671, -0.500000)
(18.793701, -0.500000)
(18.831175, -0.500000)
(18.865997, -0.500000)
(18.899878, -0.500000)
(18.936810, -0.500000)
(18.962761, -0.500000)
(18.994404, -0.500000)
(19.028652, -0.500000)
(19.065781, -0.500000)
(19.092823, -0.500000)
(19.127377, -0.500000)
(19.163515, -0.500000)
(19.196888, -0.500000)
(19.230200, -0.500000)
(19.269361, -0.500000)
(19.292789, -0.500000)
(19.328463, -0.500000)
(19.369968, -0.500000)
(19.405865, -0.500000)
(19.427862, -0.500000)
};

==> exp_plots/step_responses/yaw_des.tex <==
\addplot[
    fill=none,draw = desclr,
    dashed, line width= \linew pt,dash pattern=on \dashon pt off \dashoff pt,
    ]
 %%
coordinates {
(0.000000, 0.000000)
(0.032907, 0.000000)
(0.062761, 0.000000)
(0.099156, 0.000000)
(0.129950, 0.000000)
(0.165753, 0.000000)
(0.193936, 0.000000)
(0.228391, 0.000000)
(0.261557, 0.000000)
(0.292392, 0.000000)
(0.329782, 0.000000)
(0.370253, 0.000000)
(0.397213, 0.000000)
(0.431646, 0.000000)
(0.468384, 0.000000)
(0.496521, 0.000000)
(0.533131, 0.000000)
(0.564640, 0.000000)
(0.593544, 0.000000)
(0.628394, 0.000000)
(0.660468, 0.000000)
(0.693515, 0.000000)
(0.729235, 0.000000)
(0.759240, 0.000000)
(0.796739, 0.000000)
(0.833988, 0.000000)
(0.860999, 0.000000)
(0.892442, 0.000000)
(0.933587, 0.000000)
(0.965986, 0.000000)
(0.997910, 0.000000)
(1.031624, 0.000000)
(1.060639, 0.000000)
(1.093038, 0.000000)
(1.133887, 0.000000)
(1.167951, 0.000000)
(1.194599, 0.000000)
(1.233194, 0.000000)
(1.263740, 0.000000)
(1.297482, 0.000000)
(1.332266, 0.000000)
(1.367385, 0.000000)
(1.398498, 0.000000)
(1.437015, 0.000000)
(1.464571, 0.000000)
(1.501024, 0.000000)
(1.534085, 0.000000)
(1.564686, 0.000000)
(1.599735, 0.000000)
(1.633415, 0.000000)
(1.668613, 0.000000)
(1.700257, 0.000000)
(1.734497, 0.000000)
(1.763916, 0.000000)
(1.796423, 0.000000)
(1.828718, 0.000000)
(1.862355, 0.000000)
(1.896293, 0.000000)
(1.930358, 0.000000)
(1.963977, 0.000000)
(2.000041, 0.000000)
(2.033801, 0.000000)
(2.064144, 0.000000)
(2.094071, 0.000000)
(2.130587, 0.000000)
(2.164670, 0.000000)
(2.202131, 0.000000)
(2.242026, 0.000000)
(2.274426, 0.000000)
(2.303855, 0.000000)
(2.340054, 0.000000)
(2.369298, 0.000000)
(2.401813, 0.000000)
(2.436782, 0.000000)
(2.467305, 0.000000)
(2.499388, 0.000000)
(2.542110, 0.000000)
(2.577655, 0.000000)
(2.600355, 0.000000)
(2.636051, 0.000000)
(2.672182, 0.000000)
(2.700814, 0.000000)
(2.732477, 0.000000)
(2.767115, 0.000000)
(2.794135, 0.000000)
(2.839942, 0.000000)
(2.867065, 0.000000)
(2.896712, 0.000000)
(2.931751, 0.000000)
(2.962636, 0.000000)
(3.000629, 0.000000)
(3.035074, 0.000000)
(3.067178, 0.000000)
(3.102053, 0.000000)
(3.136258, 0.000000)
(3.163260, 0.000000)
(3.195024, 0.000000)
(3.234490, 0.000000)
(3.262304, 0.000000)
(3.296017, 0.000000)
(3.332243, 0.000000)
(3.366571, 0.000000)
(3.399052, 0.000000)
(3.432454, 0.000000)
(3.464896, 0.000000)
(3.498586, 0.000000)
(3.531600, 0.000000)
(3.558043, 0.000000)
(3.595046, 0.000000)
(3.628058, 0.000000)
(3.661241, 0.000000)
(3.695175, 0.000000)
(3.733665, 0.000000)
(3.765017, 0.000000)
(3.794625, 0.000000)
(3.834481, 0.000000)
(3.868802, 0.000000)
(3.900775, 0.000000)
(3.930340, 0.000000)
(3.964797, 0.000000)
(3.996945, 0.000000)
(4.034101, 0.000000)
(4.065475, 0.000000)
(4.095451, 0.000000)
(4.133482, 0.000000)
(4.163567, 0.000000)
(4.195832, 0.000000)
(4.232382, 0.000000)
(4.266459, 0.000000)
(4.297679, 0.000000)
(4.331636, 0.000000)
(4.372817, 0.000000)
(4.392772, 0.000000)
(4.433208, 0.000000)
(4.464170, 0.000000)
(4.498114, 0.000000)
(4.531214, 0.000000)
(4.564336, 0.000000)
(4.596074, 0.000000)
(4.635769, 0.000000)
(4.671154, 0.000000)
(4.698308, 0.000000)
(4.731188, 0.000000)
(4.762158, 0.000000)
(4.799803, 0.000000)
(4.835503, 0.000000)
(4.865563, 0.000000)
(4.898664, 0.000000)
(4.933047, 0.000000)
(4.964197, 0.000000)
(4.994103, 0.000000)
(5.032923, 0.500000)
(5.064976, 0.500000)
(5.095844, 0.500000)
(5.131793, 0.500000)
(5.160636, 0.500000)
(5.197741, 0.500000)
(5.235407, 0.500000)
(5.268848, 0.500000)
(5.296447, 0.500000)
(5.330208, 0.500000)
(5.364277, 0.500000)
(5.397705, 0.500000)
(5.428033, 0.500000)
(5.462548, 0.500000)
(5.496419, 0.500000)
(5.531839, 0.500000)
(5.567320, 0.500000)
(5.597363, 0.500000)
(5.633064, 0.500000)
(5.662623, 0.500000)
(5.694250, 0.500000)
(5.733066, 0.500000)
(5.763326, 0.500000)
(5.793659, 0.500000)
(5.839064, 0.500000)
(5.862118, 0.500000)
(5.897129, 0.500000)
(5.934341, 0.500000)
(5.971149, 0.500000)
(5.996983, 0.500000)
(6.030978, 0.500000)
(6.065285, 0.500000)
(6.094917, 0.500000)
(6.139251, 0.500000)
(6.163533, 0.500000)
(6.195184, 0.500000)
(6.232700, 0.500000)
(6.262712, 0.500000)
(6.294273, 0.500000)
(6.330581, 0.500000)
(6.364866, 0.500000)
(6.391685, 0.500000)
(6.430264, 0.500000)
(6.464236, 0.500000)
(6.492829, 0.500000)
(6.531189, 0.500000)
(6.560291, 0.500000)
(6.595351, 0.500000)
(6.628312, 0.500000)
(6.664210, 0.500000)
(6.702124, 0.500000)
(6.731398, 0.500000)
(6.765063, 0.500000)
(6.793592, 0.500000)
(6.832159, 0.500000)
(6.860442, 0.500000)
(6.897730, 0.500000)
(6.933580, 0.500000)
(6.962202, 0.500000)
(6.996201, 0.500000)
(7.034192, 0.500000)
(7.064157, 0.500000)
(7.096715, 0.500000)
(7.133627, 0.500000)
(7.164630, 0.500000)
(7.199106, 0.500000)
(7.230481, 0.500000)
(7.266715, 0.500000)
(7.294021, 0.500000)
(7.328733, 0.500000)
(7.360404, 0.500000)
(7.399731, 0.500000)
(7.431434, 0.500000)
(7.470118, 0.500000)
(7.495596, 0.500000)
(7.530021, 0.500000)
(7.564131, 0.500000)
(7.592423, 0.500000)
(7.625953, 0.500000)
(7.662565, 0.500000)
(7.692568, 0.500000)
(7.729641, 0.500000)
(7.765351, 0.500000)
(7.796402, 0.500000)
(7.830523, 0.500000)
(7.861592, 0.500000)
(7.894241, 0.500000)
(7.928831, 0.500000)
(7.962272, 0.500000)
(7.995386, 0.500000)
(8.032472, 0.500000)
(8.067616, 0.500000)
(8.094709, 0.500000)
(8.131528, 0.500000)
(8.163263, 0.500000)
(8.196895, 0.500000)
(8.230722, 0.500000)
(8.269568, 0.500000)
(8.297719, 0.500000)
(8.329178, 0.500000)
(8.364059, 0.500000)
(8.395649, 0.500000)
(8.427168, 0.500000)
(8.465327, 0.500000)
(8.495017, 0.500000)
(8.530432, 0.500000)
(8.563704, 0.500000)
(8.602518, 0.500000)
(8.632129, 0.500000)
(8.668015, 0.500000)
(8.700492, 0.500000)
(8.731572, 0.500000)
(8.762015, 0.500000)
(8.797150, 0.500000)
(8.833573, 0.500000)
(8.867826, 0.500000)
(8.903646, 0.500000)
(8.929855, 0.500000)
(8.967199, 0.500000)
(8.997551, 0.500000)
(9.032206, 0.500000)
(9.062511, 0.500000)
(9.092272, 0.500000)
(9.133962, 0.500000)
(9.161540, 0.500000)
(9.197236, 0.500000)
(9.230119, 0.500000)
(9.264680, 0.500000)
(9.293431, 0.500000)
(9.330903, 0.500000)
(9.361966, 0.500000)
(9.395635, 0.500000)
(9.433397, 0.500000)
(9.463463, 0.500000)
(9.493546, 0.500000)
(9.533072, 0.500000)
(9.563852, 0.500000)
(9.600721, 0.500000)
(9.634478, 0.500000)
(9.665073, 0.500000)
(9.700306, 0.500000)
(9.733113, 0.500000)
(9.765276, 0.500000)
(9.799196, 0.500000)
(9.829104, 0.500000)
(9.866053, 0.500000)
(9.896494, 0.500000)
(9.934001, 0.500000)
(9.959985, 0.500000)
(9.993752, 0.500000)
(10.031167, 0.000000)
(10.063027, 0.000000)
(10.096301, 0.000000)
(10.135336, 0.000000)
(10.166135, 0.000000)
(10.201086, 0.000000)
(10.230821, 0.000000)
(10.265347, 0.000000)
(10.307892, 0.000000)
(10.333893, 0.000000)
(10.363275, 0.000000)
(10.397418, 0.000000)
(10.435137, 0.000000)
(10.465668, 0.000000)
(10.495579, 0.000000)
(10.526779, 0.000000)
(10.563776, 0.000000)
(10.595040, 0.000000)
(10.634655, 0.000000)
(10.663806, 0.000000)
(10.695578, 0.000000)
(10.728919, 0.000000)
(10.760738, 0.000000)
(10.794507, 0.000000)
(10.826254, 0.000000)
(10.866492, 0.000000)
(10.889975, 0.000000)
(10.928892, 0.000000)
(10.963261, 0.000000)
(10.995407, 0.000000)
(11.031898, 0.000000)
(11.061822, 0.000000)
(11.101187, 0.000000)
(11.126880, 0.000000)
(11.164371, 0.000000)
(11.199227, 0.000000)
(11.235794, 0.000000)
(11.266492, 0.000000)
(11.309587, 0.000000)
(11.332639, 0.000000)
(11.366953, 0.000000)
(11.396490, 0.000000)
(11.435691, 0.000000)
(11.470110, 0.000000)
(11.498376, 0.000000)
(11.533786, 0.000000)
(11.564941, 0.000000)
(11.598574, 0.000000)
(11.633995, 0.000000)
(11.665583, 0.000000)
(11.694270, 0.000000)
(11.733031, 0.000000)
(11.766126, 0.000000)
(11.801460, 0.000000)
(11.833681, 0.000000)
(11.863360, 0.000000)
(11.897003, 0.000000)
(11.932692, 0.000000)
(11.965088, 0.000000)
(11.999536, 0.000000)
(12.033054, 0.000000)
(12.061716, 0.000000)
(12.098525, 0.000000)
(12.140690, 0.000000)
(12.165751, 0.000000)
(12.196928, 0.000000)
(12.232549, 0.000000)
(12.264841, 0.000000)
(12.296071, 0.000000)
(12.330084, 0.000000)
(12.362422, 0.000000)
(12.394089, 0.000000)
(12.438736, 0.000000)
(12.463762, 0.000000)
(12.498752, 0.000000)
(12.530001, 0.000000)
(12.561997, 0.000000)
(12.592821, 0.000000)
(12.630338, 0.000000)
(12.662843, 0.000000)
(12.692714, 0.000000)
(12.736881, 0.000000)
(12.769895, 0.000000)
(12.796587, 0.000000)
(12.831881, 0.000000)
(12.862697, 0.000000)
(12.897333, 0.000000)
(12.927094, 0.000000)
(12.966120, 0.000000)
(12.995205, 0.000000)
(13.029028, 0.000000)
(13.061118, 0.000000)
(13.095151, 0.000000)
(13.130626, 0.000000)
(13.160268, 0.000000)
(13.192458, 0.000000)
(13.229842, 0.000000)
(13.262951, 0.000000)
(13.291424, 0.000000)
(13.327871, 0.000000)
(13.365177, 0.000000)
(13.393091, 0.000000)
(13.426115, 0.000000)
(13.461692, 0.000000)
(13.495413, 0.000000)
(13.531981, 0.000000)
(13.563937, 0.000000)
(13.597040, 0.000000)
(13.627987, 0.000000)
(13.666540, 0.000000)
(13.692537, 0.000000)
(13.730198, 0.000000)
(13.765574, 0.000000)
(13.793833, 0.000000)
(13.835137, 0.000000)
(13.860224, 0.000000)
(13.898758, 0.000000)
(13.934139, 0.000000)
(13.969197, 0.000000)
(13.997362, 0.000000)
(14.033179, 0.000000)
(14.068600, 0.000000)
(14.096314, 0.000000)
(14.133842, 0.000000)
(14.170678, 0.000000)
(14.198231, 0.000000)
(14.232775, 0.000000)
(14.272419, 0.000000)
(14.300295, 0.000000)
(14.335476, 0.000000)
(14.367599, 0.000000)
(14.395101, 0.000000)
(14.432243, 0.000000)
(14.468035, 0.000000)
(14.496995, 0.000000)
(14.536459, 0.000000)
(14.565752, 0.000000)
(14.596197, 0.000000)
(14.635535, 0.000000)
(14.664274, 0.000000)
(14.698331, 0.000000)
(14.733498, 0.000000)
(14.765669, 0.000000)
(14.794340, 0.000000)
(14.830121, 0.000000)
(14.862068, 0.000000)
(14.895944, 0.000000)
(14.932391, 0.000000)
(14.962316, 0.000000)
(14.996885, 0.000000)
(15.029431, -0.500000)
(15.062099, -0.500000)
(15.094184, -0.500000)
(15.133767, -0.500000)
(15.165980, -0.500000)
(15.196164, -0.500000)
(15.233513, -0.500000)
(15.267859, -0.500000)
(15.298458, -0.500000)
(15.333828, -0.500000)
(15.363088, -0.500000)
(15.396466, -0.500000)
(15.433797, -0.500000)
(15.460214, -0.500000)
(15.494213, -0.500000)
(15.535244, -0.500000)
(15.561469, -0.500000)
(15.593652, -0.500000)
(15.633888, -0.500000)
(15.663216, -0.500000)
(15.695759, -0.500000)
(15.730407, -0.500000)
(15.765191, -0.500000)
(15.798187, -0.500000)
(15.829816, -0.500000)
(15.862677, -0.500000)
(15.894365, -0.500000)
(15.930459, -0.500000)
(15.961542, -0.500000)
(15.998383, -0.500000)
(16.031139, -0.500000)
(16.064640, -0.500000)
(16.094805, -0.500000)
(16.133522, -0.500000)
(16.163528, -0.500000)
(16.195232, -0.500000)
(16.232773, -0.500000)
(16.266174, -0.500000)
(16.298170, -0.500000)
(16.332056, -0.500000)
(16.366823, -0.500000)
(16.397148, -0.500000)
(16.429585, -0.500000)
(16.464878, -0.500000)
(16.497740, -0.500000)
(16.526941, -0.500000)
(16.563902, -0.500000)
(16.593758, -0.500000)
(16.639233, -0.500000)
(16.666922, -0.500000)
(16.707029, -0.500000)
(16.735460, -0.500000)
(16.764395, -0.500000)
(16.798353, -0.500000)
(16.835455, -0.500000)
(16.864494, -0.500000)
(16.896738, -0.500000)
(16.928804, -0.500000)
(16.967268, -0.500000)
(17.001842, -0.500000)
(17.036844, -0.500000)
(17.065083, -0.500000)
(17.096169, -0.500000)
(17.129910, -0.500000)
(17.164614, -0.500000)
(17.196672, -0.500000)
(17.229876, -0.500000)
(17.261803, -0.500000)
(17.301132, -0.500000)
(17.332460, -0.500000)
(17.365841, -0.500000)
(17.394920, -0.500000)
(17.432362, -0.500000)
(17.462721, -0.500000)
(17.494738, -0.500000)
(17.528868, -0.500000)
(17.566523, -0.500000)
(17.595392, -0.500000)
(17.638868, -0.500000)
(17.671988, -0.500000)
(17.695316, -0.500000)
(17.733515, -0.500000)
(17.766481, -0.500000)
(17.800713, -0.500000)
(17.832922, -0.500000)
(17.865217, -0.500000)
(17.898865, -0.500000)
(17.931290, -0.500000)
(17.965231, -0.500000)
(17.999779, -0.500000)
(18.032166, -0.500000)
(18.071001, -0.500000)
(18.100548, -0.500000)
(18.138834, -0.500000)
(18.164602, -0.500000)
(18.199627, -0.500000)
(18.234806, -0.500000)
(18.267197, -0.500000)
(18.297958, -0.500000)
(18.331667, -0.500000)
(18.366722, -0.500000)
(18.397043, -0.500000)
(18.434376, -0.500000)
(18.463037, -0.500000)
(18.496124, -0.500000)
(18.531105, -0.500000)
(18.566057, -0.500000)
(18.595682, -0.500000)
(18.631454, -0.500000)
(18.661718, -0.500000)
(18.697771, -0.500000)
(18.730629, -0.500000)
(18.761671, -0.500000)
(18.793701, -0.500000)
(18.831175, -0.500000)
(18.865997, -0.500000)
(18.899878, -0.500000)
(18.936810, -0.500000)
(18.962761, -0.500000)
(18.994404, -0.500000)
(19.028652, -0.500000)
(19.065781, -0.500000)
(19.092823, -0.500000)
(19.127377, -0.500000)
(19.163515, -0.500000)
(19.196888, -0.500000)
(19.230200, -0.500000)
(19.269361, -0.500000)
(19.292789, -0.500000)
(19.328463, -0.500000)
(19.369968, -0.500000)
(19.405865, -0.500000)
(19.427862, -0.500000)
};
